BayesHammer: Bayesian clustering for error correction in single-cell sequencing

Error correction of sequenced reads remains a difficult task, especially in single-cell sequencing projects with extremely non-uniform coverage. While existing error correction tools designed for standard (multi-cell) sequencing data usually come up short in single-cell sequencing projects, algorithms actually used for single-cell error correction have been so far very simplistic. We introduce several novel algorithms based on Hamming graphs and Bayesian subclustering in our new error correction tool BayesHammer. While BayesHammer was designed for single-cell sequencing, we demonstrate that it also improves on existing error correction tools for multi-cell sequencing data while working much faster on real-life datasets. We benchmark BayesHammer on both $k$-mer counts and actual assembly results with the SPAdes genome assembler.

==> covgraphs/ecoli.bh.log.cov.errors.tex <==
\addplot [sharp plot,color=lightblue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.000873675240576807)
(1, 0.000355630079102382)
(2, 0.000192317911846117)
(3, 0.000112263765511238)
(4, 9.44929411380743e-05)
(5, 6.95454376911325e-05)
(6, 5.82677991466245e-05)
(7, 5.74134325902224e-05)
(8, 5.28425715134711e-05)
(9, 5.39959663646139e-05)
(10, 7.49706653242859e-05)
(11, 8.78716003259579e-05)
(12, 4.97241335826033e-05)
(13, 4.97668519104234e-05)
(14, 5.1603740006688e-05)
(15, 4.6776568963016e-05)
(16, 4.78018088306985e-05)
(17, 9.21007147801484e-05)
(18, 5.05785001390054e-05)
(19, 5.46367412819155e-05)
(20, 7.25357206385399e-05)
(21, 0.000217581695300817)
(22, 0.000198931477004612)
(23, 0.000362816882017216)
(24, 0.000189701325801488)
(25, 0.000221450439927484)
(26, 0.000246904542644521)
(27, 0.000251580473369833)
(28, 0.000294953767436906)
(29, 0.000276714464874364)
(30, 0.000287035799470056)
(31, 0.000516174309267236)
(32, 0.000287158068589583)
(33, 0.000295604266114481)
(34, 0.00030836100506669)
(35, 0.000304089977744785)
(36, 0.000336966007113544)
(37, 0.000332270472676002)
(38, 0.000364607745475911)
(39, 0.000340043705988444)
(40, 0.000351489287241479)
(41, 0.000391134943299824)
(42, 0.000383095931335164)
(43, 0.000383363535877578)
(44, 0.000370565393686852)
(45, 0.000371813361365244)
(46, 0.000385333956608627)
(47, 0.00058242134162355)
(48, 0.000445681206973743)
(49, 0.000886450699706796)
(50, 0.000595301468423592)
(51, 0.00131860434658867)
(52, 0.000515635068908021)
(53, 0.000941857266003494)
(54, 0.000609297051767925)
(55, 0.000524097090334896)
(56, 0.000579719950115128)
(57, 0.000550348916325787)
(58, 0.000600575724315033)
(59, 0.000552020361695304)
(60, 0.00066377203821144)
(61, 0.000697396983921289)
(62, 0.000644241915750513)
(63, 0.00069582166082937)
(64, 0.000715566664485545)
(65, 0.000858029923452943)
(66, 0.00102492229749026)
(67, 0.000697488731144133)
(68, 0.000705364448931446)
(69, 0.000833078274801514)
(70, 0.000678474693876294)
(71, 0.00068659511711219)
(72, 0.000911367316863649)
(73, 0.00166482873631694)
(74, 0.00074071862080504)
(75, 0.000789741138909302)
(76, 0.000967411320410581)
(77, 0.000923009220170224)
(78, 0.00092015981321449)
(79, 0.000939530280592185)
(80, 0.00111887625066231)
(81, 0.000981052297659853)
(82, 0.00102624516272409)
(83, 0.00117958844703385)
(84, 0.0011585726119431)
(85, 0.00112288522935656)
(86, 0.00121605011996317)
(87, 0.00140194086544385)
(88, 0.00156521527846477)
(89, 0.00156267664193784)
(90, 0.00153070342971485)
(91, 0.00135706210967803)
(92, 0.00161317663440862)
(93, 0.0015331959772485)
(94, 0.00182891384226191)
(95, 0.00121937873112593)
(96, 0.0012625945048467)
(97, 0.00140580706277592)
(98, 0.0016554869407632)
(99, 0.000794304816899937)
(100, 0)
};


==> covgraphs/ecoli.hammer.log.cov.errors.tex <==
\addplot [sharp plot,color=lightblue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.000896777739635444)
(1, 0.000392003102458805)
(2, 0.000232992669678988)
(3, 0.000158967618985315)
(4, 0.000137004142405873)
(5, 0.0001119580726223)
(6, 0.000107676693172116)
(7, 0.000104679727556988)
(8, 9.95420722167673e-05)
(9, 0.000101982458503372)
(10, 0.00011919360389311)
(11, 0.000132251811216169)
(12, 9.32912582194993e-05)
(13, 9.25634237129681e-05)
(14, 9.1279009877913e-05)
(15, 9.02086650153672e-05)
(16, 8.94380167143341e-05)
(17, 0.000128270128327499)
(18, 9.30771892469901e-05)
(19, 9.44472306710489e-05)
(20, 0.000115896941716468)
(21, 0.000231005545461202)
(22, 0.000216396416969269)
(23, 0.000378726299733356)
(24, 0.000206867467510258)
(25, 0.000237367241498738)
(26, 0.000263878363427766)
(27, 0.000267845882950962)
(28, 0.000311715071746807)
(29, 0.000294397179305948)
(30, 0.000306697184194466)
(31, 0.000527023881628069)
(32, 0.000302571285280367)
(33, 0.000309318536817734)
(34, 0.000321985534432742)
(35, 0.000320581153956844)
(36, 0.000352285900892173)
(37, 0.00034859700464796)
(38, 0.000382719615248615)
(39, 0.000355901432823605)
(40, 0.000369660920119636)
(41, 0.000408321525383981)
(42, 0.000399936223783618)
(43, 0.000396237323364283)
(44, 0.000386677264878229)
(45, 0.000388567513495531)
(46, 0.000404081647578156)
(47, 0.000600823752274333)
(48, 0.000473070856194554)
(49, 0.000926257096767844)
(50, 0.000614673322657904)
(51, 0.0013424179756957)
(52, 0.00053336430220106)
(53, 0.000954729559582784)
(54, 0.000634266717599662)
(55, 0.000542605258571703)
(56, 0.000600605160883678)
(57, 0.000571098006312503)
(58, 0.000616486029631103)
(59, 0.00057354989281004)
(60, 0.000683399910195095)
(61, 0.000719882728781279)
(62, 0.000667134696527793)
(63, 0.00071929191072571)
(64, 0.000738346244799451)
(65, 0.000892877948475571)
(66, 0.00104896625448604)
(67, 0.000720995904388417)
(68, 0.000729479151693457)
(69, 0.000855586834135728)
(70, 0.00070318925535044)
(71, 0.000709934038100255)
(72, 0.000941122041187358)
(73, 0.00167210073239612)
(74, 0.000762284024435503)
(75, 0.000816655013004989)
(76, 0.000995945809081142)
(77, 0.000954547761803685)
(78, 0.00094808129813281)
(79, 0.000971856465635085)
(80, 0.00114757949831377)
(81, 0.00101209950295391)
(82, 0.00105830610146745)
(83, 0.00121098922343949)
(84, 0.00119357400509402)
(85, 0.00115261908197979)
(86, 0.00124488397932082)
(87, 0.00143243972000107)
(88, 0.00159837566043585)
(89, 0.00159723325732793)
(90, 0.00156240217835189)
(91, 0.00139067302858423)
(92, 0.001645181384349)
(93, 0.00157135901929863)
(94, 0.0018678991002421)
(95, 0.00124363403073769)
(96, 0.00129084739548624)
(97, 0.00143250840518966)
(98, 0.001678029288261)
(99, 0.000812450488983918)
(100, 0)
};


==> covgraphs/ecoli.hammernoext.log.cov.errors.tex <==
\addplot [sharp plot,color=lightblue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.00141712253809352)
(1, 0.0018125497820359)
(2, 0.00155191276179602)
(3, 0.00140922859472842)
(4, 0.00128762536312139)
(5, 0.00121288386467025)
(6, 0.00122319618374837)
(7, 0.00117971105064462)
(8, 0.00121963706477451)
(9, 0.00124058111104378)
(10, 0.00121105867545288)
(11, 0.00121840506205278)
(12, 0.00123369102174822)
(13, 0.00117697326681857)
(14, 0.00115849322599274)
(15, 0.00117368792622731)
(16, 0.00122305929455707)
(17, 0.00124071800023508)
(18, 0.00129565619567781)
(19, 0.0013895621809113)
(20, 0.00155784462675246)
(21, 0.0022067285999606)
(22, 0.00277395425749155)
(23, 0.00275739770026182)
(24, 0.00252499368991809)
(25, 0.00250694821322926)
(26, 0.00247527497784769)
(27, 0.00239771953126104)
(28, 0.00242928599852395)
(29, 0.00237259424820039)
(30, 0.0023699399289924)
(31, 0.00256216229651488)
(32, 0.00229154173201046)
(33, 0.00225247638669677)
(34, 0.0022323219425734)
(35, 0.00221298578617401)
(36, 0.00221385230287831)
(37, 0.00218179662027432)
(38, 0.00222371691371746)
(39, 0.00217118581781108)
(40, 0.00216968413435625)
(41, 0.00218244608497597)
(42, 0.00216245764423484)
(43, 0.00214760673666194)
(44, 0.00212764992092469)
(45, 0.00211645100234608)
(46, 0.00211068597200215)
(47, 0.0024968584110146)
(48, 0.0021809221009515)
(49, 0.00326793203264296)
(50, 0.00224646111373919)
(51, 0.00355086129182052)
(52, 0.00216387369501165)
(53, 0.00256132351872707)
(54, 0.0025171410146256)
(55, 0.00221023571753203)
(56, 0.00238342091602255)
(57, 0.00223936190835737)
(58, 0.00225026944264342)
(59, 0.00220182418794296)
(60, 0.00238659707944047)
(61, 0.00246188294684147)
(62, 0.00236394036583785)
(63, 0.00241629774327806)
(64, 0.00246313416242582)
(65, 0.0030428636269622)
(66, 0.00285617785872698)
(67, 0.00235476564655236)
(68, 0.00237560521163953)
(69, 0.00259604679536663)
(70, 0.00232144898904036)
(71, 0.00231048753496974)
(72, 0.00275394593431202)
(73, 0.00377305503953323)
(74, 0.00243526626083976)
(75, 0.0025630621070934)
(76, 0.00288850816865002)
(77, 0.00281753230047522)
(78, 0.0028328963241447)
(79, 0.00292706727889613)
(80, 0.00310558458964662)
(81, 0.00288952385348848)
(82, 0.00296523092327741)
(83, 0.00321721741075035)
(84, 0.00318949767657719)
(85, 0.003142675778893)
(86, 0.00324172085104514)
(87, 0.00358005896047881)
(88, 0.0038574718303044)
(89, 0.00377671952078905)
(90, 0.00372520378694122)
(91, 0.00345197341085355)
(92, 0.00385855298602863)
(93, 0.00373799321525554)
(94, 0.00449369915135951)
(95, 0.00306124594790524)
(96, 0.00308859160362725)
(97, 0.00327265640978968)
(98, 0.00344246267569118)
(99, 0.0017006957436142)
(100, 0)
};


==> covgraphs/graph.0.500.tex <==
\addplot[const plot,fill=magenta,draw=magenta] coordinates {
(-1, 0)
(0, 94.526)
(1, 93.456)
(2, 96.84)
(3, 97.758)
(4, 97.982)
(5, 96.82)
(6, 94.94)
(7, 95.406)
(8, 95.042)
(9, 97.636)
(10, 96.914)
(11, 98.67)
(12, 97.604)
(13, 97.842)
(14, 96.24)
(15, 96.05)
(16, 98.092)
(17, 97.606)
(18, 97.312)
(19, 97.494)
(20, 98.376)
(21, 95.456)
(22, 97.23)
(23, 97.236)
(24, 97.238)
(25, 96.576)
(26, 97.994)
(27, 97.586)
(28, 97.108)
(29, 95.888)
(30, 98.076)
(31, 99.498)
(32, 99.976)
(33, 96.108)
(34, 98.024)
(35, 97.358)
(36, 97.918)
(37, 97.702)
(38, 98.392)
(39, 98.31)
(40, 98.718)
(41, 98.474)
(42, 98.406)
(43, 97.94)
(44, 98.206)
(45, 97.136)
(46, 96.242)
(47, 96.816)
(48, 96.896)
(49, 97.178)
(50, 96.494)
(51, 95.408)
(52, 96.46)
(53, 97.388)
(54, 96.894)
(55, 94.298)
(56, 95.642)
(57, 98.184)
(58, 98.47)
(59, 98.186)
(60, 96.01)
(61, 97.554)
(62, 95.648)
(63, 97.68)
(64, 96.928)
(65, 93.628)
(66, 95.64)
(67, 97.188)
(68, 99.474)
(69, 97.598)
(70, 95.924)
(71, 92.65)
(72, 98.68)
(73, 95.06)
(74, 95.586)
(75, 97.05)
(76, 96.63)
(77, 92.718)
(78, 95.092)
(79, 95.998)
(80, 93.69)
(81, 95.462)
(82, 96.39)
(83, 96.278)
(84, 97.824)
(85, 92.614)
(86, 94.462)
(87, 92.574)
(88, 93.546)
(89, 93.976)
(90, 94.932)
(91, 93.838)
(92, 94.592)
(93, 95.262)
(94, 94.268)
(95, 85.43)
(96, 91.966)
(97, 94.878)
(98, 96.324)
(99, 95.522)
(100, 94.9)
(101, 92.862)
(102, 96.506)
(103, 97.014)
(104, 93.46)
(105, 95.442)
(106, 95.512)
(107, 94.248)
(108, 93.086)
(109, 95.142)
(110, 94.936)
(111, 97.5)
(112, 96.456)
(113, 95.094)
(114, 94.992)
(115, 94.708)
(116, 98.326)
(117, 98.668)
(118, 96.558)
(119, 97.034)
(120, 94.04)
(121, 94.666)
(122, 95.774)
(123, 93.612)
(124, 89.922)
(125, 91.458)
(126, 93.718)
(127, 89.544)
(128, 90.148)
(129, 89.934)
(130, 91.884)
(131, 90.962)
(132, 87.92)
(133, 89.44)
(134, 92.126)
(135, 86.274)
(136, 91.262)
(137, 87.408)
(138, 88.814)
(139, 92.988)
(140, 95.524)
(141, 92.648)
(142, 94.22)
(143, 84.012)
(144, 92.204)
(145, 93.044)
(146, 89.044)
(147, 81.316)
(148, 84.064)
(149, 89.332)
(150, 86.17)
(151, 92.972)
(152, 94.66)
(153, 94.234)
(154, 94.034)
(155, 94.854)
(156, 95.75)
(157, 95.512)
(158, 89.084)
(159, 88.714)
(160, 90.178)
(161, 91.35)
(162, 91.916)
(163, 78.368)
(164, 89.524)
(165, 91.182)
(166, 91.52)
(167, 95.83)
(168, 96.942)
(169, 95.924)
(170, 94.606)
(171, 90.518)
(172, 81.79)
(173, 89.626)
(174, 91.824)
(175, 95.604)
(176, 92.262)
(177, 90.02)
(178, 95.596)
(179, 95.068)
(180, 86.47)
(181, 82.756)
(182, 91.184)
(183, 91.906)
(184, 93.19)
(185, 80.878)
(186, 73.168)
(187, 88.198)
(188, 86.072)
(189, 85.572)
(190, 88.688)
(191, 91.142)
(192, 91.428)
(193, 94.014)
(194, 88.498)
(195, 93.654)
(196, 88.408)
(197, 93.768)
(198, 91.316)
(199, 94.004)
(200, 87.454)
(201, 94.382)
(202, 89.686)
(203, 90.086)
(204, 94.178)
(205, 97.932)
(206, 93.726)
(207, 96.704)
(208, 97.422)
(209, 95.196)
(210, 97.338)
(211, 97.744)
(212, 97.112)
(213, 97.91)
(214, 98.668)
(215, 96.322)
(216, 98.1)
(217, 97.424)
(218, 97.994)
(219, 96.258)
(220, 98.452)
(221, 96.528)
(222, 97.88)
(223, 98.192)
(224, 96.038)
(225, 97.522)
(226, 99.044)
(227, 98.376)
(228, 95.874)
(229, 98.496)
(230, 97.718)
(231, 94.868)
(232, 96.134)
(233, 92.006)
(234, 96.076)
(235, 97.176)
(236, 95.816)
(237, 94.718)
(238, 95.908)
(239, 94.97)
(240, 97.222)
(241, 95.2)
(242, 95.776)
(243, 98.08)
(244, 90.438)
(245, 89.894)
(246, 86.424)
(247, 90.41)
(248, 92.074)
(249, 85.078)
(250, 83.298)
(251, 84.882)
(252, 85.834)
(253, 78.692)
(254, 90.216)
(255, 92.528)
(256, 94.61)
(257, 93.396)
(258, 91.866)
(259, 85.818)
(260, 37.002)
(261, 30.418)
(262, 54.872)
(263, 59.35)
(264, 47.904)
(265, 33.836)
(266, 67.328)
(267, 62.234)
(268, 67.132)
(269, 70.298)
(270, 80.59)
(271, 80.818)
(272, 86.426)
(273, 87.482)
(274, 82.042)
(275, 83.822)
(276, 83.598)
(277, 89.546)
(278, 81.37)
(279, 82.29)
(280, 91.214)
(281, 87.576)
(282, 89.932)
(283, 91.058)
(284, 88.386)
(285, 95.042)
(286, 95.492)
(287, 94.89)
(288, 92.862)
(289, 95.01)
(290, 93.428)
(291, 93.82)
(292, 92.158)
(293, 94.432)
(294, 95.944)
(295, 97.688)
(296, 96.822)
(297, 93.028)
(298, 91.858)
(299, 97.604)
(300, 98.986)
(301, 98.452)
(302, 98.32)
(303, 97.176)
(304, 98.188)
(305, 98.622)
(306, 97.276)
(307, 97.054)
(308, 96.748)
(309, 96.8)
(310, 97.758)
(311, 97.418)
(312, 97.344)
(313, 96.534)
(314, 97.136)
(315, 93.434)
(316, 92.832)
(317, 93.632)
(318, 93.742)
(319, 93.188)
(320, 91.922)
(321, 97.37)
(322, 96.652)
(323, 90.512)
(324, 85.906)
(325, 91.572)
(326, 83.338)
(327, 86.666)
(328, 93.332)
(329, 92.806)
(330, 95.804)
(331, 96.016)
(332, 95.332)
(333, 95.506)
(334, 95.756)
(335, 93.616)
(336, 94.71)
(337, 97.868)
(338, 97.388)
(339, 95.108)
(340, 91.116)
(341, 94.238)
(342, 95.674)
(343, 90.822)
(344, 87.622)
(345, 88.822)
(346, 91.522)
(347, 95.202)
(348, 94.636)
(349, 97.35)
(350, 93.752)
(351, 95.38)
(352, 96.384)
(353, 97.69)
(354, 94.332)
(355, 97.862)
(356, 96.988)
(357, 96.67)
(358, 97.87)
(359, 96.468)
(360, 98.766)
(361, 97.896)
(362, 97.59)
(363, 97.774)
(364, 98.602)
(365, 97.152)
(366, 96.954)
(367, 98.56)
(368, 97.866)
(369, 97.776)
(370, 96.552)
(371, 97.126)
(372, 96.522)
(373, 96.426)
(374, 95.618)
(375, 95.436)
(376, 96.622)
(377, 97.07)
(378, 96.962)
(379, 98.464)
(380, 98.324)
(381, 98.26)
(382, 98.33)
(383, 97.796)
(384, 97.054)
(385, 98.166)
(386, 97.646)
(387, 95.652)
(388, 97.388)
(389, 98.452)
(390, 98.842)
(391, 98)
(392, 98.568)
(393, 98.058)
(394, 98.756)
(395, 98.148)
(396, 99.05)
(397, 98.966)
(398, 98.966)
(399, 99.07)
(400, 98.974)
(401, 99.392)
(402, 99.122)
(403, 98.9)
(404, 99.346)
(405, 98.582)
(406, 98.81)
(407, 99.406)
(408, 96.748)
(409, 98.538)
(410, 98.484)
(411, 98.314)
(412, 98.564)
(413, 93.29)
(414, 93.456)
(415, 99.296)
(416, 99.004)
(417, 99.452)
(418, 99.16)
(419, 99.84)
(420, 99.514)
(421, 99.104)
(422, 99.224)
(423, 99.802)
(424, 99.448)
(425, 98.87)
(426, 97.042)
(427, 99.606)
(428, 99.692)
(429, 99.408)
(430, 99.13)
(431, 99.71)
(432, 99.856)
(433, 99.754)
(434, 99.496)
(435, 99.528)
(436, 96.044)
(437, 99.108)
(438, 99.398)
(439, 99.692)
(440, 99.798)
(441, 99.766)
(442, 99.436)
(443, 99.048)
(444, 99.584)
(445, 99.81)
(446, 99.616)
(447, 92.412)
(448, 99.48)
(449, 93.91)
(450, 99.718)
(451, 89.64)
(452, 95.704)
(453, 99.44)
(454, 99.92)
(455, 99.736)
(456, 99.59)
(457, 99.98)
(458, 100)
(459, 100)
(460, 100)
(461, 99.978)
(462, 99.884)
(463, 99.88)
(464, 99.994)
(465, 99.988)
(466, 99.868)
(467, 99.998)
(468, 100)
(469, 99.976)
(470, 99.824)
(471, 99.922)
(472, 99.906)
(473, 99.936)
(474, 99.998)
(475, 99.99)
(476, 99.996)
(477, 99.99)
(478, 99.824)
(479, 95.466)
(480, 99.942)
(481, 99.694)
(482, 99.302)
(483, 98.968)
(484, 97.966)
(485, 97.908)
(486, 99.728)
(487, 99.218)
(488, 99.648)
(489, 99.428)
(490, 99.492)
(491, 99.76)
(492, 99.79)
(493, 99.328)
(494, 98.734)
(495, 99.744)
(496, 98.944)
(497, 98.466)
(498, 92.6)
(499, 95.776)
(500, 98.888)
(501, 97.052)
(502, 99.05)
(503, 99.166)
(504, 99.77)
(505, 99.706)
(506, 99.712)
(507, 98.434)
(508, 99.518)
(509, 99.466)
(510, 98.234)
(511, 99.704)
(512, 99.156)
(513, 95.968)
(514, 98.882)
(515, 94.652)
(516, 99.308)
(517, 99.46)
(518, 99.232)
(519, 97.4)
(520, 94.698)
(521, 94.93)
(522, 97.904)
(523, 98.368)
(524, 99.52)
(525, 97.17)
(526, 87.216)
(527, 97.568)
(528, 97.426)
(529, 99.002)
(530, 99.544)
(531, 98.448)
(532, 97.564)
(533, 98.034)
(534, 97.594)
(535, 98.336)
(536, 99.042)
(537, 99.552)
(538, 99.532)
(539, 98.574)
(540, 97.636)
(541, 99.5)
(542, 98.148)
(543, 98.626)
(544, 97.014)
(545, 99.238)
(546, 99.598)
(547, 98.388)
(548, 98.454)
(549, 97.52)
(550, 98.288)
(551, 98.738)
(552, 97.268)
(553, 96.448)
(554, 98.504)
(555, 97.95)
(556, 93.154)
(557, 89.214)
(558, 99.482)
(559, 99.468)
(560, 96.124)
(561, 89.852)
(562, 96.032)
(563, 94.46)
(564, 91.038)
(565, 85.226)
(566, 74.598)
(567, 90.842)
(568, 90.714)
(569, 95.6)
(570, 90.844)
(571, 91.436)
(572, 88.952)
(573, 85.484)
(574, 92.66)
(575, 87.526)
(576, 97.194)
(577, 92.882)
(578, 96.382)
(579, 93.992)
(580, 88.686)
(581, 98.754)
(582, 99.624)
(583, 99.644)
(584, 99.72)
(585, 99.754)
(586, 99.816)
(587, 99.806)
(588, 99.586)
(589, 99.84)
(590, 99.818)
(591, 95.264)
(592, 99.836)
(593, 98.854)
(594, 95.958)
(595, 97.28)
(596, 98.68)
(597, 93.748)
(598, 95.922)
(599, 92.354)
(600, 97.428)
(601, 95.788)
(602, 98.128)
(603, 97.638)
(604, 99.738)
(605, 99.796)
(606, 99.608)
(607, 99.252)
(608, 99.186)
(609, 98.902)
(610, 98.654)
(611, 98.678)
(612, 98.6)
(613, 93.87)
(614, 97.428)
(615, 96.344)
(616, 99.026)
(617, 97.49)
(618, 99.266)
(619, 99.482)
(620, 99.726)
(621, 99.898)
(622, 99.76)
(623, 99.842)
(624, 99.896)
(625, 99.874)
(626, 99.908)
(627, 99.618)
(628, 99.746)
(629, 94.644)
(630, 92.522)
(631, 95.132)
(632, 99.868)
(633, 99.948)
(634, 99.85)
(635, 99.944)
(636, 99.522)
(637, 99.806)
(638, 99.776)
(639, 99.402)
(640, 99.72)
(641, 99.764)
(642, 99.584)
(643, 99.584)
(644, 99.7)
(645, 99.738)
(646, 99.73)
(647, 99.922)
(648, 99.96)
(649, 99.732)
(650, 96.59)
(651, 98.528)
(652, 98.766)
(653, 98.24)
(654, 96.322)
(655, 95.472)
(656, 97.962)
(657, 99.46)
(658, 98.612)
(659, 98.064)
(660, 98.28)
(661, 99.714)
(662, 99.976)
(663, 99.942)
(664, 99.88)
(665, 99.92)
(666, 99.642)
(667, 99.67)
(668, 99.75)
(669, 99.762)
(670, 99.718)
(671, 99.786)
(672, 99.262)
(673, 95.75)
(674, 98.794)
(675, 96.302)
(676, 97.834)
(677, 97.898)
(678, 95.838)
(679, 96.964)
(680, 99.158)
(681, 98.264)
(682, 99.408)
(683, 99.57)
(684, 99.258)
(685, 99.108)
(686, 99.982)
(687, 99.83)
(688, 99.992)
(689, 99.922)
(690, 99.658)
(691, 99.97)
(692, 99.02)
(693, 98.284)
(694, 99.242)
(695, 99.892)
(696, 98.636)
(697, 77.432)
(698, 91.526)
(699, 96.77)
(700, 99.368)
(701, 96.422)
(702, 98.89)
(703, 99.44)
(704, 98.036)
(705, 96.884)
(706, 97.296)
(707, 99.23)
(708, 99.57)
(709, 98.99)
(710, 99.406)
(711, 99.686)
(712, 99.212)
(713, 90.578)
(714, 93.43)
(715, 98.614)
(716, 98.392)
(717, 98.088)
(718, 98.41)
(719, 96.722)
(720, 99.306)
(721, 99.806)
(722, 99.498)
(723, 99.616)
(724, 99.452)
(725, 98.918)
(726, 98.198)
(727, 98.352)
(728, 98.084)
(729, 98.682)
(730, 98.53)
(731, 98.562)
(732, 98.308)
(733, 98.536)
(734, 97.24)
(735, 98.912)
(736, 98.492)
(737, 94.294)
(738, 97.03)
(739, 97.158)
(740, 98.312)
(741, 97.78)
(742, 99.116)
(743, 97.368)
(744, 98.614)
(745, 97.938)
(746, 98.916)
(747, 94.062)
(748, 90.116)
(749, 98.754)
(750, 96.686)
(751, 98.9)
(752, 99.808)
(753, 99.052)
(754, 99.708)
(755, 99.686)
(756, 99.486)
(757, 99.478)
(758, 96.752)
(759, 99.734)
(760, 99.884)
(761, 96.844)
(762, 92.936)
(763, 99.382)
(764, 98.458)
(765, 99.622)
(766, 99.934)
(767, 99.938)
(768, 99.928)
(769, 99.002)
(770, 99.026)
(771, 98.884)
(772, 96.274)
(773, 99.068)
(774, 99.622)
(775, 99.662)
(776, 98.922)
(777, 99.792)
(778, 99.996)
(779, 99.99)
(780, 99.99)
(781, 99.98)
(782, 98.568)
(783, 99.688)
(784, 99.92)
(785, 99.884)
(786, 99.924)
(787, 99.984)
(788, 99.872)
(789, 99.08)
(790, 99.346)
(791, 99.672)
(792, 99.812)
(793, 99.184)
(794, 99.606)
(795, 99.53)
(796, 98.596)
(797, 99.894)
(798, 99.792)
(799, 99.778)
(800, 99.98)
(801, 99.97)
(802, 99.296)
(803, 99.72)
(804, 99.622)
(805, 99.796)
(806, 98.902)
(807, 99.778)
(808, 99.442)
(809, 99.778)
(810, 99.298)
(811, 99.612)
(812, 99.978)
(813, 99.968)
(814, 99.946)
(815, 99.756)
(816, 99.83)
(817, 99.862)
(818, 99.612)
(819, 99.102)
(820, 99.492)
(821, 99.854)
(822, 99.148)
(823, 99.674)
(824, 99.742)
(825, 99.434)
(826, 98.638)
(827, 98.7)
(828, 99.172)
(829, 99.02)
(830, 99.47)
(831, 98.912)
(832, 99.672)
(833, 97.75)
(834, 98.886)
(835, 99.374)
(836, 99.786)
(837, 98.052)
(838, 98.314)
(839, 99.082)
(840, 99.034)
(841, 99.002)
(842, 99.262)
(843, 98.892)
(844, 98.192)
(845, 98.116)
(846, 98.9)
(847, 99.102)
(848, 99.462)
(849, 98.98)
(850, 99.492)
(851, 99.44)
(852, 99.81)
(853, 99.686)
(854, 99.508)
(855, 99.616)
(856, 99.79)
(857, 99.234)
(858, 99.524)
(859, 99.956)
(860, 99.846)
(861, 99.814)
(862, 99.928)
(863, 99.968)
(864, 99.688)
(865, 97.356)
(866, 99.57)
(867, 99.572)
(868, 99.172)
(869, 99.802)
(870, 98.896)
(871, 99.624)
(872, 99.552)
(873, 99.704)
(874, 99.3)
(875, 99.378)
(876, 99.732)
(877, 99.794)
(878, 99.544)
(879, 99.7)
(880, 99.106)
(881, 99.484)
(882, 99.246)
(883, 99.642)
(884, 97.1)
(885, 98.57)
(886, 99.464)
(887, 99.792)
(888, 99.848)
(889, 97.854)
(890, 99.248)
(891, 99.306)
(892, 96.546)
(893, 99.468)
(894, 99.054)
(895, 99.33)
(896, 99.118)
(897, 98.352)
(898, 98.816)
(899, 98.242)
(900, 98.754)
(901, 99.708)
(902, 98.596)
(903, 97.874)
(904, 98.38)
(905, 99.05)
(906, 99.476)
(907, 99.742)
(908, 99.706)
(909, 99.608)
(910, 99.136)
(911, 99.812)
(912, 99.586)
(913, 99.586)
(914, 99.382)
(915, 99.53)
(916, 99.608)
(917, 99.628)
(918, 99.454)
(919, 99.6)
(920, 99.612)
(921, 99.814)
(922, 99.802)
(923, 99.348)
(924, 98.782)
(925, 99.56)
(926, 99.79)
(927, 99.94)
(928, 99.606)
(929, 99.638)
(930, 99.374)
(931, 99.624)
(932, 99.58)
(933, 99.87)
(934, 99.738)
(935, 98.888)
(936, 99.592)
(937, 99.75)
(938, 99.786)
(939, 98.098)
(940, 99.02)
(941, 99.704)
(942, 99.072)
(943, 99.622)
(944, 99.686)
(945, 98.938)
(946, 97.306)
(947, 99.8)
(948, 99.882)
(949, 99.63)
(950, 99.492)
(951, 99.788)
(952, 99.92)
(953, 99.812)
(954, 99.96)
(955, 99.936)
(956, 99.978)
(957, 99.958)
(958, 99.986)
(959, 99.994)
(960, 99.942)
(961, 99.746)
(962, 99.758)
(963, 99.876)
(964, 99.506)
(965, 98.508)
(966, 99.27)
(967, 99.528)
(968, 99.734)
(969, 99.826)
(970, 99.964)
(971, 99.902)
(972, 99.804)
(973, 99.788)
(974, 99.734)
(975, 99.406)
(976, 99.818)
(977, 99.87)
(978, 99.736)
(979, 96.186)
(980, 99.372)
(981, 99.8)
(982, 99.226)
(983, 98.98)
(984, 97.138)
(985, 92.6)
(986, 99.824)
(987, 99.29)
(988, 99.784)
(989, 99.718)
(990, 99.888)
(991, 99.696)
(992, 99.842)
(993, 99.582)
(994, 98.984)
(995, 98.294)
(996, 99.53)
(997, 99.748)
(998, 99.7)
(999, 99.722)
(1000, 99.332)
(1001, 99.686)
(1002, 99.476)
(1003, 99.33)
(1004, 99.22)
(1005, 99.628)
(1006, 98.782)
(1007, 99.028)
(1008, 99.754)
(1009, 99.384)
(1010, 99.87)
(1011, 99.498)
(1012, 99.878)
(1013, 99.574)
(1014, 99.572)
(1015, 90.562)
(1016, 99.05)
(1017, 97.24)
(1018, 98.3)
(1019, 97.994)
(1020, 97.028)
(1021, 99.742)
(1022, 99.394)
(1023, 99.12)
(1024, 99.444)
(1025, 98.736)
(1026, 98.738)
(1027, 97.208)
(1028, 99.21)
(1029, 99.73)
(1030, 99.842)
(1031, 99.848)
(1032, 99.808)
(1033, 99.482)
(1034, 99.484)
(1035, 99.286)
(1036, 99.012)
(1037, 99.148)
(1038, 98.85)
(1039, 98.176)
(1040, 98.984)
(1041, 97.084)
(1042, 98.21)
(1043, 98.456)
(1044, 99.84)
(1045, 93.586)
(1046, 92.662)
(1047, 95.25)
(1048, 91.43)
(1049, 90.868)
(1050, 90.896)
(1051, 97.04)
(1052, 99.864)
(1053, 99.996)
(1054, 96.5)
(1055, 100)
(1056, 100)
(1057, 99.956)
(1058, 99.892)
(1059, 99.808)
(1060, 99.49)
(1061, 99.728)
(1062, 99.87)
(1063, 99.894)
(1064, 99.824)
(1065, 99.816)
(1066, 99.876)
(1067, 99.792)
(1068, 99.854)
(1069, 99.96)
(1070, 99.924)
(1071, 99.99)
(1072, 99.976)
(1073, 99.978)
(1074, 99.994)
(1075, 99.954)
(1076, 99.982)
(1077, 99.91)
(1078, 99.958)
(1079, 99.972)
(1080, 99.664)
(1081, 99.878)
(1082, 99.454)
(1083, 99.44)
(1084, 99.99)
(1085, 99.996)
(1086, 99.974)
(1087, 99.94)
(1088, 99.298)
(1089, 99.774)
(1090, 99.54)
(1091, 99.966)
(1092, 99.504)
(1093, 97.746)
(1094, 98.382)
(1095, 87.816)
(1096, 99.684)
(1097, 99.346)
(1098, 99.49)
(1099, 98.98)
(1100, 99.444)
(1101, 99.666)
(1102, 99.626)
(1103, 99.046)
(1104, 99.73)
(1105, 99.74)
(1106, 99.91)
(1107, 99.99)
(1108, 99.484)
(1109, 99.744)
(1110, 99.642)
(1111, 99.774)
(1112, 99.808)
(1113, 98.72)
(1114, 99.536)
(1115, 99.96)
(1116, 99.982)
(1117, 99.986)
(1118, 99.996)
(1119, 99.958)
(1120, 99.924)
(1121, 99.59)
(1122, 99.95)
(1123, 99.994)
(1124, 99.736)
(1125, 99.596)
(1126, 100)
(1127, 99.994)
(1128, 99.974)
(1129, 99.962)
(1130, 99.898)
(1131, 99.752)
(1132, 94.946)
(1133, 92.872)
(1134, 95.276)
(1135, 99.926)
(1136, 99.998)
(1137, 99.992)
(1138, 100)
(1139, 100)
(1140, 99.996)
(1141, 100)
(1142, 100)
(1143, 99.992)
(1144, 99.92)
(1145, 99.914)
(1146, 99.99)
(1147, 99.91)
(1148, 98.892)
(1149, 98.012)
(1150, 100)
(1151, 99.968)
(1152, 99.996)
(1153, 99.996)
(1154, 100)
(1155, 99.94)
(1156, 100)
(1157, 100)
(1158, 100)
(1159, 99.98)
(1160, 99.82)
(1161, 99.952)
(1162, 100)
(1163, 100)
(1164, 100)
(1165, 100)
(1166, 100)
(1167, 100)
(1168, 99.996)
(1169, 99.988)
(1170, 100)
(1171, 99.928)
(1172, 99.956)
(1173, 99.788)
(1174, 99.936)
(1175, 98.726)
(1176, 99.828)
(1177, 99.692)
(1178, 99.91)
(1179, 99.884)
(1180, 99.918)
(1181, 99.796)
(1182, 99.914)
(1183, 99.786)
(1184, 99.954)
(1185, 99.804)
(1186, 99.92)
(1187, 99.918)
(1188, 99.664)
(1189, 99.946)
(1190, 97.714)
(1191, 98.286)
(1192, 99.94)
(1193, 98.924)
(1194, 97.856)
(1195, 98.1)
(1196, 99.106)
(1197, 96.698)
(1198, 99.14)
(1199, 97.82)
(1200, 98.398)
(1201, 98.014)
(1202, 99.392)
(1203, 99.088)
(1204, 99.76)
(1205, 99.806)
(1206, 99.61)
(1207, 99.722)
(1208, 99.388)
(1209, 99.868)
(1210, 99.526)
(1211, 99.568)
(1212, 99.166)
(1213, 99.694)
(1214, 99.424)
(1215, 99.708)
(1216, 99.966)
(1217, 99.81)
(1218, 99.524)
(1219, 99.294)
(1220, 99.36)
(1221, 98.544)
(1222, 97.218)
(1223, 99.416)
(1224, 98.51)
(1225, 98.13)
(1226, 97.288)
(1227, 98.3)
(1228, 95.448)
(1229, 97.534)
(1230, 97.412)
(1231, 95.694)
(1232, 96.078)
(1233, 98.256)
(1234, 99.45)
(1235, 98.82)
(1236, 99.532)
(1237, 99.018)
(1238, 98.328)
(1239, 97.286)
(1240, 97.396)
(1241, 94.816)
(1242, 96.16)
(1243, 97.83)
(1244, 93.694)
(1245, 98.546)
(1246, 97.008)
(1247, 98.428)
(1248, 97.564)
(1249, 98.864)
(1250, 98.296)
(1251, 99.144)
(1252, 98.054)
(1253, 98.812)
(1254, 98.746)
(1255, 98.91)
(1256, 98.46)
(1257, 98.794)
(1258, 98.28)
(1259, 99.366)
(1260, 98.766)
(1261, 99.502)
(1262, 99.796)
(1263, 99.364)
(1264, 98.834)
(1265, 99.74)
(1266, 99.33)
(1267, 99.814)
(1268, 99.832)
(1269, 99.938)
(1270, 99.838)
(1271, 99.984)
(1272, 99.992)
(1273, 99.992)
(1274, 99.772)
(1275, 99.986)
(1276, 99.916)
(1277, 98.952)
(1278, 98.798)
(1279, 98.264)
(1280, 98.484)
(1281, 98.964)
(1282, 99.682)
(1283, 98.98)
(1284, 98.828)
(1285, 99.312)
(1286, 99.682)
(1287, 99.016)
(1288, 99.408)
(1289, 99.37)
(1290, 97.358)
(1291, 97.798)
(1292, 98.202)
(1293, 97.736)
(1294, 98.542)
(1295, 98.42)
(1296, 98.436)
(1297, 96.844)
(1298, 97.742)
(1299, 97.716)
(1300, 98.218)
(1301, 99.452)
(1302, 99.77)
(1303, 99.348)
(1304, 99.4)
(1305, 99.326)
(1306, 99.606)
(1307, 99.352)
(1308, 99.714)
(1309, 98.298)
(1310, 99.834)
(1311, 99.802)
(1312, 99.76)
(1313, 99.826)
(1314, 99.622)
(1315, 98.378)
(1316, 99.73)
(1317, 99.432)
(1318, 99.428)
(1319, 99.796)
(1320, 99.876)
(1321, 99.956)
(1322, 99.748)
(1323, 99.952)
(1324, 99.89)
(1325, 99.668)
(1326, 99.466)
(1327, 98.606)
(1328, 98.126)
(1329, 99.334)
(1330, 99.648)
(1331, 99.362)
(1332, 99.396)
(1333, 99.422)
(1334, 99.528)
(1335, 96.33)
(1336, 99.546)
(1337, 99.714)
(1338, 99.43)
(1339, 99.08)
(1340, 99.572)
(1341, 99.174)
(1342, 98.902)
(1343, 98.584)
(1344, 99.042)
(1345, 97.732)
(1346, 98.384)
(1347, 94.552)
(1348, 99.438)
(1349, 99.564)
(1350, 99.29)
(1351, 99.672)
(1352, 99.616)
(1353, 99.518)
(1354, 99.57)
(1355, 99.416)
(1356, 99.52)
(1357, 99.826)
(1358, 98.93)
(1359, 99.53)
(1360, 99.65)
(1361, 97.994)
(1362, 99.66)
(1363, 99.068)
(1364, 99.64)
(1365, 99.744)
(1366, 99.032)
(1367, 99.542)
(1368, 99.398)
(1369, 99.308)
(1370, 93.72)
(1371, 99.434)
(1372, 99.468)
(1373, 99.364)
(1374, 99.084)
(1375, 98.658)
(1376, 99.104)
(1377, 97.728)
(1378, 98.978)
(1379, 97.5)
(1380, 99.144)
(1381, 99.15)
(1382, 99.082)
(1383, 99.218)
(1384, 95.996)
(1385, 98.782)
(1386, 96.838)
(1387, 97.708)
(1388, 98.26)
(1389, 98.486)
(1390, 97.888)
(1391, 99.112)
(1392, 99.292)
(1393, 99.276)
(1394, 99.594)
(1395, 99.414)
(1396, 99.426)
(1397, 99.476)
(1398, 98.976)
(1399, 99.298)
(1400, 99.07)
(1401, 98.074)
(1402, 99.52)
(1403, 99.21)
(1404, 99.444)
(1405, 99.312)
(1406, 98.552)
(1407, 94.364)
(1408, 98.966)
(1409, 97.944)
(1410, 99.618)
(1411, 99.506)
(1412, 99.132)
(1413, 99.616)
(1414, 99.686)
(1415, 99.39)
(1416, 99.3)
(1417, 99.122)
(1418, 99.716)
(1419, 99.786)
(1420, 99.688)
(1421, 99.51)
(1422, 99.504)
(1423, 99.312)
(1424, 99.626)
(1425, 99.516)
(1426, 97.166)
(1427, 98.71)
(1428, 98.672)
(1429, 99.694)
(1430, 99.852)
(1431, 99.826)
(1432, 99.792)
(1433, 99.514)
(1434, 99.432)
(1435, 99.54)
(1436, 99.808)
(1437, 99.356)
(1438, 99.466)
(1439, 99.698)
(1440, 99.336)
(1441, 97.632)
(1442, 98.928)
(1443, 96.304)
(1444, 97.75)
(1445, 95.592)
(1446, 95.268)
(1447, 97.402)
(1448, 97.792)
(1449, 95.79)
(1450, 95.2)
(1451, 95.968)
(1452, 96.946)
(1453, 92.546)
(1454, 98.13)
(1455, 97.534)
(1456, 98.582)
(1457, 92.928)
(1458, 72.172)
(1459, 83.852)
(1460, 93.758)
(1461, 74.924)
(1462, 82.632)
(1463, 69.516)
(1464, 81.364)
(1465, 99.364)
(1466, 91.466)
(1467, 73.798)
(1468, 90.2)
(1469, 99.676)
(1470, 99.744)
(1471, 99.868)
(1472, 83.952)
(1473, 77.424)
(1474, 99.86)
(1475, 94.67)
(1476, 97.73)
(1477, 95.554)
(1478, 97.208)
(1479, 97.324)
(1480, 99.494)
(1481, 99.694)
(1482, 99.042)
(1483, 99.728)
(1484, 99.048)
(1485, 95.316)
(1486, 98.396)
(1487, 98.638)
(1488, 99.622)
(1489, 98.462)
(1490, 99.504)
(1491, 99.612)
(1492, 98.762)
(1493, 99.522)
(1494, 99.944)
(1495, 99.924)
(1496, 99.818)
(1497, 99.872)
(1498, 99.514)
(1499, 99.712)
(1500, 99.508)
(1501, 99.392)
(1502, 99.222)
(1503, 99.78)
(1504, 98.11)
(1505, 99.618)
(1506, 99.608)
(1507, 99.944)
(1508, 99.56)
(1509, 99.518)
(1510, 98.396)
(1511, 98.262)
(1512, 98.876)
(1513, 99.36)
(1514, 99.01)
(1515, 99.294)
(1516, 99.35)
(1517, 99.084)
(1518, 98.702)
(1519, 98.726)
(1520, 98.23)
(1521, 98.836)
(1522, 98.386)
(1523, 98.936)
(1524, 99.384)
(1525, 99.24)
(1526, 98.98)
(1527, 99.074)
(1528, 99.452)
(1529, 99.774)
(1530, 99.136)
(1531, 93.704)
(1532, 98.428)
(1533, 99.328)
(1534, 99.262)
(1535, 99.206)
(1536, 99.638)
(1537, 99.902)
(1538, 99.754)
(1539, 99.802)
(1540, 99.93)
(1541, 99.872)
(1542, 99.664)
(1543, 99.14)
(1544, 99.582)
(1545, 99.498)
(1546, 99.79)
(1547, 99.914)
(1548, 99.934)
(1549, 99.548)
(1550, 99.53)
(1551, 98.146)
(1552, 95.182)
(1553, 99.96)
(1554, 99.63)
(1555, 99.862)
(1556, 99.884)
(1557, 99.914)
(1558, 99.624)
(1559, 99.806)
(1560, 99.434)
(1561, 99.762)
(1562, 99.978)
(1563, 99.584)
(1564, 99.562)
(1565, 99.972)
(1566, 99.87)
(1567, 99.854)
(1568, 98.104)
(1569, 99.994)
(1570, 99.652)
(1571, 99.24)
(1572, 99.942)
(1573, 99.95)
(1574, 99.586)
(1575, 99.21)
(1576, 99.496)
(1577, 99.69)
(1578, 99.454)
(1579, 99.416)
(1580, 99.328)
(1581, 99.636)
(1582, 99.896)
(1583, 99.562)
(1584, 99.832)
(1585, 99.682)
(1586, 99.69)
(1587, 99.766)
(1588, 99.868)
(1589, 99.766)
(1590, 99.564)
(1591, 99.81)
(1592, 99.822)
(1593, 99.704)
(1594, 99.862)
(1595, 99.804)
(1596, 99.478)
(1597, 99.808)
(1598, 99.792)
(1599, 99.986)
(1600, 99.686)
(1601, 99.938)
(1602, 99.76)
(1603, 99.78)
(1604, 99.856)
(1605, 99.644)
(1606, 99.4)
(1607, 99.682)
(1608, 99.814)
(1609, 99.748)
(1610, 99.622)
(1611, 99.85)
(1612, 99.624)
(1613, 99.804)
(1614, 99.046)
(1615, 99.41)
(1616, 99.356)
(1617, 99.652)
(1618, 99.676)
(1619, 96.236)
(1620, 99.118)
(1621, 93.268)
(1622, 99.102)
(1623, 99.122)
(1624, 99.882)
(1625, 99.864)
(1626, 99.904)
(1627, 98.572)
(1628, 99.916)
(1629, 99.946)
(1630, 99.882)
(1631, 99.602)
(1632, 99.742)
(1633, 98.93)
(1634, 99.714)
(1635, 99.472)
(1636, 99.082)
(1637, 99.456)
(1638, 99.924)
(1639, 99.936)
(1640, 99.99)
(1641, 99.942)
(1642, 99.776)
(1643, 99.33)
(1644, 99.494)
(1645, 99.576)
(1646, 99.098)
(1647, 99.852)
(1648, 99.326)
(1649, 99.85)
(1650, 99.734)
(1651, 99.772)
(1652, 99.562)
(1653, 98.214)
(1654, 99.678)
(1655, 99.398)
(1656, 98.476)
(1657, 98.844)
(1658, 98.422)
(1659, 99.32)
(1660, 98.308)
(1661, 99.552)
(1662, 95.49)
(1663, 99.744)
(1664, 99.54)
(1665, 99.384)
(1666, 98.332)
(1667, 99.64)
(1668, 99.56)
(1669, 97.556)
(1670, 99.122)
(1671, 98.276)
(1672, 99.182)
(1673, 97.938)
(1674, 99.888)
(1675, 99.66)
(1676, 99.072)
(1677, 99.2)
(1678, 99.154)
(1679, 99.514)
(1680, 98.72)
(1681, 99.718)
(1682, 99.706)
(1683, 99.734)
(1684, 99.114)
(1685, 99.4)
(1686, 99.378)
(1687, 99.8)
(1688, 99.408)
(1689, 99.576)
(1690, 99.726)
(1691, 99.756)
(1692, 99.706)
(1693, 99.83)
(1694, 99.936)
(1695, 99.804)
(1696, 99.95)
(1697, 99.572)
(1698, 99.94)
(1699, 99.896)
(1700, 99.936)
(1701, 99.84)
(1702, 99.814)
(1703, 99.866)
(1704, 99.966)
(1705, 99.818)
(1706, 99.8)
(1707, 99.864)
(1708, 98.88)
(1709, 99.512)
(1710, 99.71)
(1711, 99.72)
(1712, 99.908)
(1713, 99.7)
(1714, 99.906)
(1715, 99.83)
(1716, 99.908)
(1717, 99.962)
(1718, 99.962)
(1719, 98.434)
(1720, 99.242)
(1721, 99.772)
(1722, 99.548)
(1723, 99.838)
(1724, 99.63)
(1725, 99.676)
(1726, 99.664)
(1727, 99.906)
(1728, 99.672)
(1729, 99.534)
(1730, 99.25)
(1731, 99.882)
(1732, 99.21)
(1733, 99.412)
(1734, 99.724)
(1735, 99.686)
(1736, 99.626)
(1737, 99.886)
(1738, 99.792)
(1739, 99.824)
(1740, 99.392)
(1741, 99.054)
(1742, 99.856)
(1743, 99.798)
(1744, 99.998)
(1745, 100)
(1746, 100)
(1747, 99.992)
(1748, 100)
(1749, 100)
(1750, 99.928)
(1751, 100)
(1752, 99.994)
(1753, 99.798)
(1754, 100)
(1755, 100)
(1756, 99.952)
(1757, 99.994)
(1758, 100)
(1759, 100)
(1760, 100)
(1761, 99.98)
(1762, 100)
(1763, 99.974)
(1764, 99.97)
(1765, 100)
(1766, 99.846)
(1767, 99.822)
(1768, 100)
(1769, 100)
(1770, 99.776)
(1771, 99.806)
(1772, 99.968)
(1773, 99.99)
(1774, 99.986)
(1775, 99.986)
(1776, 99.946)
(1777, 99.992)
(1778, 99.998)
(1779, 99.996)
(1780, 99.986)
(1781, 99.89)
(1782, 99.858)
(1783, 99.65)
(1784, 99.97)
(1785, 99.996)
(1786, 99.974)
(1787, 99.948)
(1788, 99.842)
(1789, 99.838)
(1790, 99.9)
(1791, 99.972)
(1792, 99.846)
(1793, 99.844)
(1794, 99.934)
(1795, 99.946)
(1796, 99.102)
(1797, 99.988)
(1798, 99.998)
(1799, 99.97)
(1800, 99.97)
(1801, 99.842)
(1802, 99.912)
(1803, 99.946)
(1804, 99.944)
(1805, 99.984)
(1806, 99.958)
(1807, 99.966)
(1808, 99.762)
(1809, 99.902)
(1810, 99.77)
(1811, 99.996)
(1812, 99.854)
(1813, 99.81)
(1814, 99.49)
(1815, 99.876)
(1816, 98.208)
(1817, 99.858)
(1818, 99.97)
(1819, 99.682)
(1820, 94.316)
(1821, 99.59)
(1822, 99.794)
(1823, 99.842)
(1824, 99.574)
(1825, 99.82)
(1826, 99.84)
(1827, 99.73)
(1828, 99.232)
(1829, 99.882)
(1830, 99.898)
(1831, 99.466)
(1832, 99.544)
(1833, 99.834)
(1834, 99.756)
(1835, 99.878)
(1836, 99.936)
(1837, 99.452)
(1838, 99.932)
(1839, 99.742)
(1840, 97.792)
(1841, 99.834)
(1842, 99.964)
(1843, 99.996)
(1844, 99.968)
(1845, 99.918)
(1846, 99.972)
(1847, 99.968)
(1848, 99.998)
(1849, 99.992)
(1850, 99.95)
(1851, 100)
(1852, 99.974)
(1853, 99.998)
(1854, 99.998)
(1855, 99.968)
(1856, 99.952)
(1857, 99.876)
(1858, 99.948)
(1859, 99.892)
(1860, 99.98)
(1861, 99.886)
(1862, 99.988)
(1863, 99.988)
(1864, 99.99)
(1865, 99.938)
(1866, 99.566)
(1867, 99.788)
(1868, 99.614)
(1869, 97.222)
(1870, 99.972)
(1871, 99.86)
(1872, 99.928)
(1873, 99.91)
(1874, 99.524)
(1875, 99.926)
(1876, 99.702)
(1877, 99.952)
(1878, 99.938)
(1879, 99.688)
(1880, 99.438)
(1881, 98.742)
(1882, 99.752)
(1883, 99.96)
(1884, 99.75)
(1885, 98.726)
(1886, 99.81)
(1887, 99.74)
(1888, 99.934)
(1889, 99.98)
(1890, 99.896)
(1891, 99.946)
(1892, 99.98)
(1893, 99.954)
(1894, 99.97)
(1895, 98.774)
(1896, 99.914)
(1897, 99.982)
(1898, 99.996)
(1899, 99.992)
(1900, 99.954)
(1901, 99.922)
(1902, 99.924)
(1903, 99.936)
(1904, 99.896)
(1905, 99.99)
(1906, 99.926)
(1907, 99.868)
(1908, 99.742)
(1909, 99.958)
(1910, 99.838)
(1911, 99.924)
(1912, 99.928)
(1913, 99.964)
(1914, 99.76)
(1915, 99.92)
(1916, 99.538)
(1917, 99.932)
(1918, 99.99)
(1919, 99.958)
(1920, 99.908)
(1921, 99.756)
(1922, 99.968)
(1923, 99.946)
(1924, 99.862)
(1925, 99.884)
(1926, 99.956)
(1927, 99.912)
(1928, 99.888)
(1929, 99.8)
(1930, 99.968)
(1931, 99.922)
(1932, 99.976)
(1933, 99.908)
(1934, 99.16)
(1935, 89.478)
(1936, 97.132)
(1937, 98.294)
(1938, 98.244)
(1939, 99.058)
(1940, 96.844)
(1941, 99.112)
(1942, 98.128)
(1943, 98.116)
(1944, 98.686)
(1945, 98.136)
(1946, 98.53)
(1947, 96.642)
(1948, 96.966)
(1949, 98.948)
(1950, 98.842)
(1951, 96.672)
(1952, 98.328)
(1953, 97.886)
(1954, 98.144)
(1955, 99.024)
(1956, 98.834)
(1957, 98.962)
(1958, 99.34)
(1959, 99.096)
(1960, 95.692)
(1961, 98.228)
(1962, 98.688)
(1963, 99.306)
(1964, 99.402)
(1965, 99.428)
(1966, 99.24)
(1967, 99.53)
(1968, 99.072)
(1969, 99.094)
(1970, 99.834)
(1971, 99.582)
(1972, 99.738)
(1973, 99.474)
(1974, 99.23)
(1975, 98.546)
(1976, 98.826)
(1977, 99.042)
(1978, 98.784)
(1979, 99.508)
(1980, 98.7)
(1981, 99.224)
(1982, 98.488)
(1983, 97.952)
(1984, 97.126)
(1985, 96.8)
(1986, 95.332)
(1987, 94.66)
(1988, 93.978)
(1989, 92.24)
(1990, 97.764)
(1991, 96.916)
(1992, 96.864)
(1993, 99.108)
(1994, 99.004)
(1995, 99.218)
(1996, 98.622)
(1997, 99.138)
(1998, 98.97)
(1999, 99.212)
(2000, 99.088)
(2001, 98.854)
(2002, 98.824)
(2003, 99.158)
(2004, 99.088)
(2005, 99.328)
(2006, 97.892)
(2007, 99.206)
(2008, 99.248)
(2009, 99.468)
(2010, 99.522)
(2011, 98.93)
(2012, 98.96)
(2013, 99.51)
(2014, 98.568)
(2015, 96.462)
(2016, 98.954)
(2017, 98.82)
(2018, 99.242)
(2019, 98.76)
(2020, 98.712)
(2021, 98.662)
(2022, 98.976)
(2023, 98.744)
(2024, 99.518)
(2025, 99.254)
(2026, 99.408)
(2027, 99.172)
(2028, 99.172)
(2029, 99.694)
(2030, 98.774)
(2031, 99.752)
(2032, 99.506)
(2033, 98.998)
(2034, 99.166)
(2035, 99.586)
(2036, 99.65)
(2037, 99.258)
(2038, 99.508)
(2039, 99.668)
(2040, 99.702)
(2041, 99.504)
(2042, 99.29)
(2043, 99.442)
(2044, 99.17)
(2045, 98.384)
(2046, 99.54)
(2047, 99.292)
(2048, 98.568)
(2049, 99.57)
(2050, 99.472)
(2051, 99.002)
(2052, 99.714)
(2053, 99.554)
(2054, 99.58)
(2055, 99.46)
(2056, 99.14)
(2057, 97.81)
(2058, 97.154)
(2059, 98.584)
(2060, 99.304)
(2061, 99.53)
(2062, 98.72)
(2063, 96.894)
(2064, 94.028)
(2065, 98.466)
(2066, 98.232)
(2067, 97.062)
(2068, 95.55)
(2069, 97.042)
(2070, 96.87)
(2071, 97.486)
(2072, 98.122)
(2073, 99.18)
(2074, 99.074)
(2075, 98.85)
(2076, 99.198)
(2077, 98.228)
(2078, 99.414)
(2079, 99.294)
(2080, 98.73)
(2081, 99.016)
(2082, 98.422)
(2083, 99.18)
(2084, 99.228)
(2085, 99.276)
(2086, 99.51)
(2087, 99.384)
(2088, 99.23)
(2089, 99.53)
(2090, 99.192)
(2091, 98.5)
(2092, 99.28)
(2093, 99.218)
(2094, 99.298)
(2095, 99.204)
(2096, 99.36)
(2097, 94.908)
(2098, 86.814)
(2099, 89.676)
(2100, 99.872)
(2101, 99.784)
(2102, 99.782)
(2103, 99.558)
(2104, 99.334)
(2105, 99.206)
(2106, 98.958)
(2107, 98.824)
(2108, 98.82)
(2109, 98.738)
(2110, 99.404)
(2111, 98.96)
(2112, 98.602)
(2113, 99.444)
(2114, 99.712)
(2115, 99.192)
(2116, 99.408)
(2117, 97.758)
(2118, 99.456)
(2119, 99.43)
(2120, 99.242)
(2121, 99.068)
(2122, 98.95)
(2123, 99.212)
(2124, 99.08)
(2125, 98.022)
(2126, 99.978)
(2127, 99.996)
(2128, 99.998)
(2129, 99.576)
(2130, 99.706)
(2131, 99.926)
(2132, 99.732)
(2133, 99.698)
(2134, 94.34)
(2135, 96.37)
(2136, 99.648)
(2137, 98.946)
(2138, 98.112)
(2139, 98.598)
(2140, 98.352)
(2141, 97.876)
(2142, 99.322)
(2143, 96.546)
(2144, 99.58)
(2145, 99.526)
(2146, 99.892)
(2147, 99.588)
(2148, 97.428)
(2149, 98.162)
(2150, 99.42)
(2151, 99.136)
(2152, 99.26)
(2153, 99.446)
(2154, 99.518)
(2155, 98.962)
(2156, 99.938)
(2157, 99.464)
(2158, 99.4)
(2159, 99.34)
(2160, 99.626)
(2161, 99.85)
(2162, 99.722)
(2163, 99.942)
(2164, 99.546)
(2165, 99.384)
(2166, 99.95)
(2167, 98.938)
(2168, 99.99)
(2169, 99.884)
(2170, 99.996)
(2171, 99.996)
(2172, 99.99)
(2173, 99.986)
(2174, 100)
(2175, 100)
(2176, 99.998)
(2177, 99.86)
(2178, 99.996)
(2179, 99.956)
(2180, 99.98)
(2181, 99.95)
(2182, 99.98)
(2183, 99.996)
(2184, 100)
(2185, 100)
(2186, 99.99)
(2187, 99.432)
(2188, 99.028)
(2189, 99.988)
(2190, 99.998)
(2191, 99.994)
(2192, 81.502)
(2193, 99.706)
(2194, 99.996)
(2195, 99.956)
(2196, 99.984)
(2197, 99.9)
(2198, 99.136)
(2199, 99.932)
(2200, 99.974)
(2201, 99.96)
(2202, 100)
(2203, 99.974)
(2204, 99.998)
(2205, 99.918)
(2206, 99.256)
(2207, 99.962)
(2208, 99.998)
(2209, 99.998)
(2210, 99.762)
(2211, 99.856)
(2212, 99.872)
(2213, 99.946)
(2214, 99.99)
(2215, 99.978)
(2216, 99.98)
(2217, 99.994)
(2218, 99.946)
(2219, 99.918)
(2220, 99.792)
(2221, 99.94)
(2222, 99.154)
(2223, 99.89)
(2224, 99.734)
(2225, 99.95)
(2226, 99.946)
(2227, 99.72)
(2228, 98.496)
(2229, 99.934)
(2230, 99.842)
(2231, 99.988)
(2232, 99.932)
(2233, 99.612)
(2234, 99.768)
(2235, 98.612)
(2236, 99.886)
(2237, 99.568)
(2238, 99.576)
(2239, 99.38)
(2240, 99.89)
(2241, 97.224)
(2242, 99.322)
(2243, 98.744)
(2244, 99.732)
(2245, 97.514)
(2246, 99.05)
(2247, 98.838)
(2248, 99.06)
(2249, 99.648)
(2250, 99.668)
(2251, 99.262)
(2252, 99.028)
(2253, 99.234)
(2254, 98.648)
(2255, 98.37)
(2256, 99.428)
(2257, 99.406)
(2258, 99.334)
(2259, 99.058)
(2260, 99.108)
(2261, 99.014)
(2262, 99.02)
(2263, 98.932)
(2264, 99.46)
(2265, 98.912)
(2266, 96.268)
(2267, 99.314)
(2268, 98.564)
(2269, 98.46)
(2270, 98.762)
(2271, 99.054)
(2272, 97.906)
(2273, 99.25)
(2274, 98.716)
(2275, 97.648)
(2276, 99.358)
(2277, 99.004)
(2278, 99.436)
(2279, 98.686)
(2280, 99.426)
(2281, 97.074)
(2282, 97.474)
(2283, 95.982)
(2284, 99.344)
(2285, 97.034)
(2286, 99.212)
(2287, 99.57)
(2288, 99.13)
(2289, 99.502)
(2290, 99.43)
(2291, 99.792)
(2292, 99.608)
(2293, 99.466)
(2294, 99.124)
(2295, 99.242)
(2296, 99.244)
(2297, 99.276)
(2298, 96.194)
(2299, 99.486)
(2300, 99.66)
(2301, 99.856)
(2302, 99.728)
(2303, 99.6)
(2304, 99.62)
(2305, 99.79)
(2306, 99.844)
(2307, 99.832)
(2308, 99.88)
(2309, 99.746)
(2310, 99.7)
(2311, 99.86)
(2312, 99.882)
(2313, 99.93)
(2314, 99.404)
(2315, 99.198)
(2316, 99.8)
(2317, 99.736)
(2318, 99.518)
(2319, 99.898)
(2320, 99.774)
(2321, 99.884)
(2322, 99.8)
(2323, 99.404)
(2324, 99.604)
(2325, 99.362)
(2326, 99.794)
(2327, 99.886)
(2328, 99.966)
(2329, 99.918)
(2330, 99.516)
(2331, 99.856)
(2332, 99.804)
(2333, 99.264)
(2334, 99.854)
(2335, 99.976)
(2336, 99.964)
(2337, 99.788)
(2338, 99.218)
(2339, 99.9)
(2340, 99.614)
(2341, 99.598)
(2342, 99.048)
(2343, 99.576)
(2344, 98.134)
(2345, 99.75)
(2346, 99.76)
(2347, 97.808)
(2348, 99.89)
(2349, 99.862)
(2350, 99.866)
(2351, 99.724)
(2352, 99.456)
(2353, 99.676)
(2354, 99.898)
(2355, 99.92)
(2356, 99.84)
(2357, 99.938)
(2358, 99.966)
(2359, 99.986)
(2360, 99.99)
(2361, 99.996)
(2362, 99.982)
(2363, 99.934)
(2364, 99.938)
(2365, 99.894)
(2366, 99.938)
(2367, 99.998)
(2368, 99.944)
(2369, 99.992)
(2370, 99.976)
(2371, 99.998)
(2372, 99.948)
(2373, 99.98)
(2374, 99.786)
(2375, 99.912)
(2376, 99.962)
(2377, 99.942)
(2378, 99.986)
(2379, 99.996)
(2380, 99.982)
(2381, 99.86)
(2382, 99.83)
(2383, 99.482)
(2384, 99.968)
(2385, 99.976)
(2386, 99.278)
(2387, 99.83)
(2388, 99.99)
(2389, 99.99)
(2390, 99.966)
(2391, 99.996)
(2392, 100)
(2393, 100)
(2394, 100)
(2395, 100)
(2396, 100)
(2397, 100)
(2398, 99.998)
(2399, 99.994)
(2400, 99.864)
(2401, 99.99)
(2402, 99.992)
(2403, 99.972)
(2404, 99.972)
(2405, 99.946)
(2406, 99.962)
(2407, 99.49)
(2408, 99.868)
(2409, 99.8)
(2410, 99.74)
(2411, 99.712)
(2412, 99.426)
(2413, 99.84)
(2414, 99.994)
(2415, 99.986)
(2416, 99.996)
(2417, 99.982)
(2418, 99.984)
(2419, 100)
(2420, 100)
(2421, 100)
(2422, 100)
(2423, 100)
(2424, 100)
(2425, 99.958)
(2426, 99.996)
(2427, 100)
(2428, 99.992)
(2429, 100)
(2430, 100)
(2431, 100)
(2432, 100)
(2433, 100)
(2434, 100)
(2435, 99.998)
(2436, 100)
(2437, 100)
(2438, 100)
(2439, 100)
(2440, 100)
(2441, 99.988)
(2442, 99.028)
(2443, 99.976)
(2444, 100)
(2445, 100)
(2446, 99.998)
(2447, 100)
(2448, 99.996)
(2449, 99.992)
(2450, 100)
(2451, 99.998)
(2452, 100)
(2453, 99.998)
(2454, 99.106)
(2455, 99.994)
(2456, 99.984)
(2457, 100)
(2458, 99.994)
(2459, 99.998)
(2460, 99.99)
(2461, 99.984)
(2462, 99.968)
(2463, 99.738)
(2464, 99.968)
(2465, 99.976)
(2466, 99.93)
(2467, 99.97)
(2468, 99.992)
(2469, 99.94)
(2470, 99.988)
(2471, 99.984)
(2472, 99.966)
(2473, 99.892)
(2474, 99.648)
(2475, 99.854)
(2476, 99.824)
(2477, 98.082)
(2478, 99.808)
(2479, 99.872)
(2480, 99.89)
(2481, 99.874)
(2482, 99.966)
(2483, 99.864)
(2484, 99.884)
(2485, 99.922)
(2486, 99.974)
(2487, 99.946)
(2488, 99.732)
(2489, 99.94)
(2490, 99.856)
(2491, 99.87)
(2492, 99.974)
(2493, 99.994)
(2494, 99.978)
(2495, 99.896)
(2496, 99.682)
(2497, 99.742)
(2498, 99.72)
(2499, 98.94)
(2500, 99.844)
(2501, 99.756)
(2502, 99.744)
(2503, 99.74)
(2504, 99.814)
(2505, 99.914)
(2506, 99.546)
(2507, 99.346)
(2508, 99.258)
(2509, 99.78)
(2510, 99.894)
(2511, 99.92)
(2512, 99.622)
(2513, 99.68)
(2514, 99.642)
(2515, 99.584)
(2516, 96.45)
(2517, 93.388)
(2518, 97.054)
(2519, 97.44)
(2520, 96.69)
(2521, 96.138)
(2522, 97.09)
(2523, 90.034)
(2524, 90.346)
(2525, 91.058)
(2526, 88.058)
(2527, 89.57)
(2528, 94.428)
(2529, 84.338)
(2530, 90.08)
(2531, 83.35)
(2532, 91.706)
(2533, 90.364)
(2534, 93.93)
(2535, 92.104)
(2536, 75.59)
(2537, 76.616)
(2538, 84.654)
(2539, 83.826)
(2540, 93.28)
(2541, 84.73)
(2542, 94.876)
(2543, 92.044)
(2544, 91.738)
(2545, 95.814)
(2546, 93.76)
(2547, 92.54)
(2548, 92.242)
(2549, 94.552)
(2550, 91.014)
(2551, 91.204)
(2552, 79.25)
(2553, 94.852)
(2554, 93.626)
(2555, 90.554)
(2556, 88.124)
(2557, 95.7)
(2558, 92.082)
(2559, 89.166)
(2560, 90.208)
(2561, 68.752)
(2562, 90.59)
(2563, 86.346)
(2564, 90.642)
(2565, 87.024)
(2566, 91.056)
(2567, 91.15)
(2568, 92.158)
(2569, 89.668)
(2570, 92.366)
(2571, 92.956)
(2572, 92.278)
(2573, 97.394)
(2574, 98.032)
(2575, 97.286)
(2576, 97.672)
(2577, 97.346)
(2578, 97.112)
(2579, 97.462)
(2580, 98.216)
(2581, 97.846)
(2582, 97.792)
(2583, 97.92)
(2584, 98.902)
(2585, 98.962)
(2586, 98.432)
(2587, 95.252)
(2588, 92.948)
(2589, 97.168)
(2590, 98.044)
(2591, 97.746)
(2592, 96.626)
(2593, 97.516)
(2594, 97.89)
(2595, 98.812)
(2596, 98.154)
(2597, 93.826)
(2598, 98.366)
(2599, 98.946)
(2600, 98.338)
(2601, 98.554)
(2602, 98.156)
(2603, 98.556)
(2604, 97.276)
(2605, 98.216)
(2606, 98.316)
(2607, 97.65)
(2608, 98.764)
(2609, 98.542)
(2610, 98.312)
(2611, 98.096)
(2612, 98.044)
(2613, 98.7)
(2614, 99.156)
(2615, 99.202)
(2616, 99.298)
(2617, 98.454)
(2618, 93.974)
(2619, 97.61)
(2620, 97.434)
(2621, 98.548)
(2622, 98.316)
(2623, 99.136)
(2624, 97.518)
(2625, 99.216)
(2626, 99.044)
(2627, 97.256)
(2628, 97.646)
(2629, 97.554)
(2630, 97.062)
(2631, 96.238)
(2632, 97.168)
(2633, 96.436)
(2634, 96.456)
(2635, 94.55)
(2636, 87.46)
(2637, 89.968)
(2638, 94.864)
(2639, 91.994)
(2640, 94.24)
(2641, 96.92)
(2642, 96.024)
(2643, 95.256)
(2644, 97.62)
(2645, 97.088)
(2646, 98.038)
(2647, 97.028)
(2648, 97.334)
(2649, 96.72)
(2650, 96.618)
(2651, 97.222)
(2652, 95.444)
(2653, 96.446)
(2654, 97.1)
(2655, 96.084)
(2656, 97.11)
(2657, 98.074)
(2658, 97.004)
(2659, 97.098)
(2660, 97.842)
(2661, 97.432)
(2662, 97.424)
(2663, 98.348)
(2664, 97.764)
(2665, 97.824)
(2666, 98.044)
(2667, 96.936)
(2668, 94.718)
(2669, 96.224)
(2670, 94.452)
(2671, 97.24)
(2672, 96.736)
(2673, 97.606)
(2674, 98.172)
(2675, 96.722)
(2676, 97.522)
(2677, 95.706)
(2678, 96.804)
(2679, 98.262)
(2680, 97.106)
(2681, 96.542)
(2682, 98.368)
(2683, 98.824)
(2684, 98.082)
(2685, 98.128)
(2686, 98.192)
(2687, 98.656)
(2688, 97.87)
(2689, 95.944)
(2690, 95.57)
(2691, 95.224)
(2692, 96.55)
(2693, 96.228)
(2694, 97.554)
(2695, 95.684)
(2696, 96.526)
(2697, 98.14)
(2698, 95.26)
(2699, 96.538)
(2700, 96.468)
(2701, 96.058)
(2702, 96.032)
(2703, 94.45)
(2704, 88.568)
(2705, 95.01)
(2706, 96.046)
(2707, 91.926)
(2708, 88.594)
(2709, 94.536)
(2710, 96.336)
(2711, 93.39)
(2712, 90.624)
(2713, 88.188)
(2714, 90.008)
(2715, 85.458)
(2716, 81.738)
(2717, 90.168)
(2718, 85.21)
(2719, 90.298)
(2720, 92.378)
(2721, 87.002)
(2722, 70.054)
(2723, 73.396)
(2724, 85.68)
(2725, 83.082)
(2726, 72.53)
(2727, 85)
(2728, 75.564)
(2729, 88.218)
(2730, 90.762)
(2731, 90.238)
(2732, 90.824)
(2733, 94.036)
(2734, 91.488)
(2735, 93.996)
(2736, 95.106)
(2737, 95.596)
(2738, 93.272)
(2739, 95.992)
(2740, 94.174)
(2741, 92.734)
(2742, 79.514)
(2743, 93.388)
(2744, 89.768)
(2745, 89.948)
(2746, 80.682)
(2747, 85.774)
(2748, 83.996)
(2749, 80.098)
(2750, 86.624)
(2751, 91.476)
(2752, 92.01)
(2753, 90.612)
(2754, 88.122)
(2755, 93.78)
(2756, 94.42)
(2757, 91.182)
(2758, 91.792)
(2759, 96.582)
(2760, 94.116)
(2761, 92.586)
(2762, 96.822)
(2763, 95.962)
(2764, 95.2)
(2765, 84.734)
(2766, 93.364)
(2767, 90.858)
(2768, 93.466)
(2769, 96.662)
(2770, 95.278)
(2771, 95.51)
(2772, 96.2)
(2773, 97.336)
(2774, 96.526)
(2775, 96.986)
(2776, 96.244)
(2777, 98.27)
(2778, 95.458)
(2779, 97.396)
(2780, 97.596)
(2781, 98.152)
(2782, 97.104)
(2783, 97.344)
(2784, 97.938)
(2785, 98.078)
(2786, 97.444)
(2787, 98.29)
(2788, 99.622)
(2789, 98.804)
(2790, 98.548)
(2791, 97.36)
(2792, 95.766)
(2793, 96.02)
(2794, 95.652)
(2795, 96.388)
(2796, 96.486)
(2797, 97.368)
(2798, 94.524)
(2799, 96.47)
(2800, 94.256)
(2801, 92.732)
(2802, 95.03)
(2803, 93.106)
(2804, 95.52)
(2805, 96.742)
(2806, 95.784)
(2807, 97.41)
(2808, 93.918)
(2809, 95.944)
(2810, 96.466)
(2811, 97.894)
(2812, 94.41)
(2813, 96.65)
(2814, 96.64)
(2815, 94.104)
(2816, 97.158)
(2817, 94.934)
(2818, 97.084)
(2819, 97.614)
(2820, 94.556)
(2821, 96.49)
(2822, 95.3)
(2823, 94.276)
(2824, 91.5)
(2825, 90.33)
(2826, 78.462)
(2827, 75.258)
(2828, 65.804)
(2829, 70.766)
(2830, 89.73)
(2831, 71.884)
(2832, 76.806)
(2833, 68.15)
(2834, 67.332)
(2835, 51.888)
(2836, 66.778)
(2837, 66.098)
(2838, 50.79)
(2839, 60.08)
(2840, 40.768)
(2841, 70.36)
(2842, 61.074)
(2843, 67.444)
(2844, 73.346)
(2845, 84.694)
(2846, 71.966)
(2847, 65.188)
(2848, 85.254)
(2849, 78.382)
(2850, 77.456)
(2851, 79.086)
(2852, 82.776)
(2853, 85.96)
(2854, 69.7)
(2855, 33.276)
(2856, 44.604)
(2857, 84.694)
(2858, 83.654)
(2859, 81.118)
(2860, 86.496)
(2861, 87.556)
(2862, 84.624)
(2863, 88.892)
(2864, 90.932)
(2865, 90.994)
(2866, 92.944)
(2867, 92.324)
(2868, 87.402)
(2869, 89.592)
(2870, 82.254)
(2871, 71.454)
(2872, 61.462)
(2873, 60.058)
(2874, 80.814)
(2875, 63.69)
(2876, 70.466)
(2877, 50.596)
(2878, 64.22)
(2879, 75.284)
(2880, 68.482)
(2881, 60.31)
(2882, 46.794)
(2883, 51.016)
(2884, 66.256)
(2885, 41.584)
(2886, 66.796)
(2887, 75.346)
(2888, 67.266)
(2889, 66.364)
(2890, 44.674)
(2891, 43.486)
(2892, 37.042)
(2893, 48.912)
(2894, 58.516)
(2895, 59.946)
(2896, 42.178)
(2897, 63.37)
(2898, 62.6)
(2899, 49.95)
(2900, 31.268)
(2901, 47.51)
(2902, 25.1)
(2903, 16.648)
(2904, 18.056)
(2905, 20.924)
(2906, 45.706)
(2907, 16.674)
(2908, 18.224)
(2909, 6.552)
(2910, 16.946)
(2911, 4.556)
(2912, 23.22)
(2913, 21.11)
(2914, 28.536)
(2915, 8.304)
(2916, 13.538)
(2917, 27.14)
(2918, 41.968)
(2919, 38.502)
(2920, 40.874)
(2921, 24.858)
(2922, 63.404)
(2923, 59.34)
(2924, 45.708)
(2925, 68.06)
(2926, 81.544)
(2927, 76.88)
(2928, 65.866)
(2929, 67.502)
(2930, 80.812)
(2931, 92.476)
(2932, 99.83)
(2933, 92.814)
(2934, 95.58)
(2935, 96.246)
(2936, 68.84)
(2937, 91.098)
(2938, 93.074)
(2939, 93.328)
(2940, 92.724)
(2941, 90.504)
(2942, 88.318)
(2943, 88.234)
(2944, 95.63)
(2945, 92.332)
(2946, 94.054)
(2947, 96.938)
(2948, 97.788)
(2949, 97.564)
(2950, 95.76)
(2951, 97.834)
(2952, 96.156)
(2953, 97.264)
(2954, 96.718)
(2955, 95.436)
(2956, 94.164)
(2957, 95.462)
(2958, 95.394)
(2959, 91.126)
(2960, 94.592)
(2961, 96.054)
(2962, 95.644)
(2963, 94.036)
(2964, 94.68)
(2965, 95.488)
(2966, 93.168)
(2967, 91.35)
(2968, 94.958)
(2969, 95.442)
(2970, 94.39)
(2971, 96.782)
(2972, 96.934)
(2973, 96.628)
(2974, 95.224)
(2975, 97.048)
(2976, 97.172)
(2977, 98.49)
(2978, 96.824)
(2979, 97.72)
(2980, 97.854)
(2981, 97.538)
(2982, 94.85)
(2983, 95.226)
(2984, 97.564)
(2985, 98.034)
(2986, 97.714)
(2987, 97.586)
(2988, 96.936)
(2989, 97.424)
(2990, 96.738)
(2991, 97.358)
(2992, 95.602)
(2993, 98.516)
(2994, 97.93)
(2995, 98.138)
(2996, 97.706)
(2997, 96.318)
(2998, 95.68)
(2999, 98.034)
(3000, 98.608)
(3001, 97.974)
(3002, 98.328)
(3003, 98.83)
(3004, 97.552)
(3005, 95.408)
(3006, 96.114)
(3007, 96.234)
(3008, 98.414)
(3009, 97.338)
(3010, 98.156)
(3011, 97.19)
(3012, 96.262)
(3013, 98.618)
(3014, 98.678)
(3015, 98.918)
(3016, 97.36)
(3017, 97.138)
(3018, 97.614)
(3019, 96.714)
(3020, 97.718)
(3021, 97.5)
(3022, 98.098)
(3023, 97.032)
(3024, 97.528)
(3025, 96.526)
(3026, 97.506)
(3027, 98.102)
(3028, 97.558)
(3029, 98.452)
(3030, 98.894)
(3031, 97.846)
(3032, 98.256)
(3033, 97.504)
(3034, 97.404)
(3035, 97.286)
(3036, 91.794)
(3037, 99.444)
(3038, 98.614)
(3039, 97.772)
(3040, 97.034)
(3041, 94.786)
(3042, 98.648)
(3043, 97.03)
(3044, 98.332)
(3045, 97.744)
(3046, 96.592)
(3047, 96.596)
(3048, 97.962)
(3049, 98.54)
(3050, 98.988)
(3051, 96.988)
(3052, 81.236)
(3053, 88.972)
(3054, 94.65)
(3055, 98.69)
(3056, 99.218)
(3057, 99.452)
(3058, 99.588)
(3059, 92.546)
(3060, 86.884)
(3061, 99.862)
(3062, 99.38)
(3063, 99.48)
(3064, 98.908)
(3065, 99.144)
(3066, 99.402)
(3067, 99.146)
(3068, 99.034)
(3069, 99.074)
(3070, 96.158)
(3071, 98.03)
(3072, 98.024)
(3073, 92.53)
(3074, 96.792)
(3075, 97.144)
(3076, 97.222)
(3077, 95.724)
(3078, 97)
(3079, 91.876)
(3080, 91.19)
(3081, 97.322)
(3082, 97.4)
(3083, 99.012)
(3084, 99.244)
(3085, 99.35)
(3086, 99.56)
(3087, 99.156)
(3088, 98.104)
(3089, 99.086)
(3090, 97.806)
(3091, 98.108)
(3092, 97.934)
(3093, 97.552)
(3094, 97.772)
(3095, 96.09)
(3096, 98.512)
(3097, 95.26)
(3098, 98.184)
(3099, 98.914)
(3100, 99.146)
(3101, 98.582)
(3102, 96.11)
(3103, 97.336)
(3104, 94.064)
(3105, 96.362)
(3106, 92.602)
(3107, 98.038)
(3108, 98.484)
(3109, 94.588)
(3110, 93.984)
(3111, 93.16)
(3112, 92.722)
(3113, 94.422)
(3114, 83.286)
(3115, 70.112)
(3116, 0)
(3117, 4.68)
(3118, 0.012)
(3119, 7.444)
(3120, 7.564)
(3121, 0)
(3122, 0)
(3123, 4.396)
(3124, 16.338)
(3125, 18.062)
(3126, 14.838)
(3127, 4.56)
(3128, 0)
(3129, 0.006)
(3130, 8.808)
(3131, 0)
(3132, 0)
(3133, 5.112)
(3134, 5.888)
(3135, 16.53)
(3136, 0)
(3137, 50.038)
(3138, 74.442)
(3139, 58.092)
(3140, 13.05)
(3141, 76.554)
(3142, 76.084)
(3143, 80.348)
(3144, 91.492)
(3145, 89.924)
(3146, 89.658)
(3147, 92.958)
(3148, 90.78)
(3149, 90.122)
(3150, 92.572)
(3151, 93.082)
(3152, 94.054)
(3153, 96.554)
(3154, 95.552)
(3155, 96.594)
(3156, 97.436)
(3157, 96.026)
(3158, 96.286)
(3159, 90.546)
(3160, 96.608)
(3161, 97.576)
(3162, 97.566)
(3163, 98.268)
(3164, 97.93)
(3165, 96.146)
(3166, 95.982)
(3167, 97.312)
(3168, 97.428)
(3169, 97.954)
(3170, 97.49)
(3171, 98.046)
(3172, 98.412)
(3173, 98.404)
(3174, 98.208)
(3175, 98.608)
(3176, 98.326)
(3177, 98.498)
(3178, 90.492)
(3179, 97.744)
(3180, 97.142)
(3181, 97.696)
(3182, 94.054)
(3183, 93.044)
(3184, 91.438)
(3185, 88.75)
(3186, 89.38)
(3187, 95.292)
(3188, 94.926)
(3189, 95.338)
(3190, 93.57)
(3191, 89.37)
(3192, 93.296)
(3193, 88.074)
(3194, 88.042)
(3195, 87.284)
(3196, 83.61)
(3197, 70.954)
(3198, 91.928)
(3199, 81.942)
(3200, 71.058)
(3201, 75.438)
(3202, 40.236)
(3203, 43.658)
(3204, 52.466)
(3205, 57.7)
(3206, 72.3)
(3207, 70.788)
(3208, 83.292)
(3209, 74.986)
(3210, 89.634)
(3211, 82.036)
(3212, 91.042)
(3213, 88.814)
(3214, 87.862)
(3215, 84.824)
(3216, 85.72)
(3217, 91.7)
(3218, 88.296)
(3219, 86.2)
(3220, 70.962)
(3221, 77.464)
(3222, 78.524)
(3223, 74.794)
(3224, 69.65)
(3225, 78.19)
(3226, 82.918)
(3227, 81.516)
(3228, 89.588)
(3229, 78.186)
(3230, 74.722)
(3231, 78.448)
(3232, 68.2)
(3233, 66.834)
(3234, 68.996)
(3235, 44.666)
(3236, 75.504)
(3237, 53.598)
(3238, 72.56)
(3239, 60.26)
(3240, 57.776)
(3241, 46.81)
(3242, 51.98)
(3243, 71.942)
(3244, 61.05)
(3245, 72.896)
(3246, 32.458)
(3247, 62.468)
(3248, 40.17)
(3249, 23.99)
(3250, 43.894)
(3251, 27.134)
(3252, 53.382)
(3253, 51.608)
(3254, 26.888)
(3255, 35.024)
(3256, 19.602)
(3257, 15.476)
(3258, 20.784)
(3259, 86.206)
(3260, 86.238)
(3261, 66.212)
(3262, 81.57)
(3263, 61.838)
(3264, 78.078)
(3265, 81.502)
(3266, 50.288)
(3267, 66.454)
(3268, 62.33)
(3269, 62.804)
(3270, 89.586)
(3271, 82.246)
(3272, 89.292)
(3273, 83.922)
(3274, 81.364)
(3275, 99.996)
(3276, 99.982)
(3277, 100)
(3278, 100)
(3279, 100)
(3280, 92.4)
(3281, 71.958)
(3282, 64.432)
(3283, 79.164)
(3284, 54.028)
(3285, 78.13)
(3286, 85.54)
(3287, 91.18)
(3288, 84.55)
(3289, 83.304)
(3290, 81.236)
(3291, 75.78)
(3292, 90.642)
(3293, 84.556)
(3294, 72.014)
(3295, 79.048)
(3296, 74.39)
(3297, 88.444)
(3298, 92.572)
(3299, 93.288)
(3300, 91.946)
(3301, 92.8)
(3302, 88.888)
(3303, 90.648)
(3304, 89.27)
(3305, 91.866)
(3306, 91.056)
(3307, 92.256)
(3308, 93.89)
(3309, 94.662)
(3310, 94.964)
(3311, 89.98)
(3312, 81.306)
(3313, 84.668)
(3314, 85.852)
(3315, 89.834)
(3316, 80.078)
(3317, 87.888)
(3318, 73.794)
(3319, 80.576)
(3320, 93.882)
(3321, 88.362)
(3322, 77.842)
(3323, 89.142)
(3324, 92.668)
(3325, 87.332)
(3326, 93.26)
(3327, 86.718)
(3328, 92.374)
(3329, 90.742)
(3330, 95.102)
(3331, 89.642)
(3332, 87.992)
(3333, 89.736)
(3334, 85.606)
(3335, 87.946)
(3336, 94.048)
(3337, 90.736)
(3338, 90.294)
(3339, 91.996)
(3340, 89.642)
(3341, 83.292)
(3342, 86.494)
(3343, 96.076)
(3344, 93.04)
(3345, 91.18)
(3346, 95.352)
(3347, 84.054)
(3348, 93.076)
(3349, 90.378)
(3350, 88.186)
(3351, 93.95)
(3352, 94.94)
(3353, 93.17)
(3354, 86.488)
(3355, 89.174)
(3356, 92.19)
(3357, 93.312)
(3358, 91.158)
(3359, 92.05)
(3360, 95.144)
(3361, 95.502)
(3362, 92.8)
(3363, 91.244)
(3364, 91.498)
(3365, 88.8)
(3366, 92.712)
(3367, 91.79)
(3368, 90.766)
(3369, 89.242)
(3370, 92.01)
(3371, 92.262)
(3372, 91.526)
(3373, 92.952)
(3374, 92.542)
(3375, 93.194)
(3376, 92.91)
(3377, 93.39)
(3378, 94.866)
(3379, 87.406)
(3380, 92.616)
(3381, 91.164)
(3382, 89.512)
(3383, 83.674)
(3384, 67.158)
(3385, 86.82)
(3386, 84.098)
(3387, 88.976)
(3388, 80.018)
(3389, 87.818)
(3390, 88.292)
(3391, 88.83)
(3392, 89.396)
(3393, 81.482)
(3394, 85.964)
(3395, 73.468)
(3396, 67.922)
(3397, 87.88)
(3398, 88.01)
(3399, 75.528)
(3400, 84.846)
(3401, 82.992)
(3402, 82.348)
(3403, 74.002)
(3404, 92.252)
(3405, 94.254)
(3406, 88.512)
(3407, 81.298)
(3408, 74.906)
(3409, 79.64)
(3410, 76.616)
(3411, 85.238)
(3412, 80.314)
(3413, 59.06)
(3414, 78.892)
(3415, 89.938)
(3416, 80.29)
(3417, 88.868)
(3418, 90.308)
(3419, 92.876)
(3420, 95.9)
(3421, 94.088)
(3422, 87.702)
(3423, 92)
(3424, 90.606)
(3425, 92.744)
(3426, 86.518)
(3427, 90.204)
(3428, 91.01)
(3429, 90.556)
(3430, 86.69)
(3431, 81.33)
(3432, 93.326)
(3433, 84.498)
(3434, 86.44)
(3435, 94.704)
(3436, 88.986)
(3437, 94.238)
(3438, 92.834)
(3439, 86.61)
(3440, 88.964)
(3441, 88.564)
(3442, 90.798)
(3443, 83.314)
(3444, 77.286)
(3445, 83.762)
(3446, 84.142)
(3447, 82.45)
(3448, 92.26)
(3449, 74.968)
(3450, 80.424)
(3451, 87.562)
(3452, 89.416)
(3453, 77.886)
(3454, 61.314)
(3455, 56.54)
(3456, 84.564)
(3457, 77.466)
(3458, 83.22)
(3459, 89.306)
(3460, 87.376)
(3461, 87.448)
(3462, 91.256)
(3463, 90.108)
(3464, 96.888)
(3465, 93.594)
(3466, 96.2)
(3467, 94.654)
(3468, 94.834)
(3469, 84.45)
(3470, 92.136)
(3471, 95.388)
(3472, 91.436)
(3473, 85.574)
(3474, 93.122)
(3475, 91.21)
(3476, 90.372)
(3477, 93.454)
(3478, 94.668)
(3479, 94.394)
(3480, 95.798)
(3481, 95.22)
(3482, 95.77)
(3483, 90.3)
(3484, 90.974)
(3485, 88.988)
(3486, 92.752)
(3487, 88.128)
(3488, 90.24)
(3489, 88.564)
(3490, 84.86)
(3491, 90.246)
(3492, 90.926)
(3493, 80.802)
(3494, 77.578)
(3495, 79.808)
(3496, 63.694)
(3497, 71.136)
(3498, 62.52)
(3499, 53.12)
(3500, 65.132)
(3501, 37.728)
(3502, 37.154)
(3503, 40.942)
(3504, 27.812)
(3505, 36.598)
(3506, 12.058)
(3507, 21.842)
(3508, 0)
(3509, 0)
(3510, 0)
(3511, 0)
(3512, 0)
(3513, 3.082)
(3514, 3.08)
(3515, 0)
(3516, 0)
(3517, 0)
(3518, 0)
(3519, 0)
(3520, 0)
(3521, 0)
(3522, 0)
(3523, 0)
(3524, 0)
(3525, 4.16)
(3526, 0.056)
(3527, 0)
(3528, 0)
(3529, 0)
(3530, 0)
(3531, 0)
(3532, 0)
(3533, 0)
(3534, 0)
(3535, 0)
(3536, 0)
(3537, 0)
(3538, 0)
(3539, 0)
(3540, 0)
(3541, 0)
(3542, 0)
(3543, 0)
(3544, 0)
(3545, 0)
(3546, 0)
(3547, 0)
(3548, 0)
(3549, 0)
(3550, 4.97)
(3551, 4.27)
(3552, 0)
(3553, 0)
(3554, 0)
(3555, 0)
(3556, 0)
(3557, 0.756)
(3558, 0)
(3559, 0)
(3560, 0)
(3561, 4.16)
(3562, 7.656)
(3563, 0)
(3564, 2.314)
(3565, 16.86)
(3566, 0)
(3567, 0)
(3568, 0)
(3569, 0)
(3570, 0)
(3571, 6.12)
(3572, 8.064)
(3573, 0.012)
(3574, 17.462)
(3575, 10.52)
(3576, 0)
(3577, 0)
(3578, 3.192)
(3579, 0)
(3580, 0)
(3581, 4.16)
(3582, 0)
(3583, 35.606)
(3584, 0.006)
(3585, 0)
(3586, 0)
(3587, 0)
(3588, 3.422)
(3589, 15.08)
(3590, 4.106)
(3591, 0.87)
(3592, 0.002)
(3593, 9.356)
(3594, 0)
(3595, 7.656)
(3596, 0)
(3597, 3.08)
(3598, 0)
(3599, 0)
(3600, 0)
(3601, 16.752)
(3602, 12.312)
(3603, 1.122)
(3604, 0)
(3605, 0)
(3606, 0.488)
(3607, 0)
(3608, 4.826)
(3609, 9.29)
(3610, 0)
(3611, 9.12)
(3612, 0)
(3613, 0)
(3614, 0)
(3615, 1.332)
(3616, 0)
(3617, 9.312)
(3618, 0)
(3619, 0)
(3620, 4.308)
(3621, 0)
(3622, 0)
(3623, 10.332)
(3624, 0)
(3625, 0)
(3626, 0)
(3627, 0)
(3628, 0.062)
(3629, 0)
(3630, 1.56)
(3631, 0)
(3632, 0)
(3633, 0)
(3634, 0)
(3635, 0)
(3636, 0)
(3637, 10.1)
(3638, 0)
(3639, 0)
(3640, 0)
(3641, 0)
(3642, 0)
(3643, 0)
(3644, 0)
(3645, 0)
(3646, 0)
(3647, 0)
(3648, 0)
(3649, 0)
(3650, 0)
(3651, 0)
(3652, 0)
(3653, 0)
(3654, 0)
(3655, 0)
(3656, 0)
(3657, 0)
(3658, 0)
(3659, 0)
(3660, 0)
(3661, 0)
(3662, 0)
(3663, 4.556)
(3664, 0)
(3665, 0)
(3666, 0)
(3667, 0)
(3668, 0)
(3669, 0)
(3670, 0)
(3671, 0)
(3672, 0)
(3673, 0)
(3674, 0)
(3675, 0)
(3676, 0)
(3677, 0)
(3678, 0)
(3679, 3.306)
(3680, 0)
(3681, 1.19)
(3682, 2.97)
(3683, 0)
(3684, 8.372)
(3685, 0)
(3686, 5.7)
(3687, 0)
(3688, 0)
(3689, 0)
(3690, 0)
(3691, 8.556)
(3692, 0)
(3693, 0)
(3694, 0)
(3695, 4.97)
(3696, 0)
(3697, 0)
(3698, 0)
(3699, 0)
(3700, 0)
(3701, 5.148)
(3702, 9.452)
(3703, 38.43)
(3704, 0.38)
(3705, 6.48)
(3706, 9.562)
(3707, 7.142)
(3708, 0)
(3709, 0)
(3710, 0)
(3711, 0)
(3712, 0)
(3713, 0)
(3714, 0)
(3715, 0)
(3716, 0)
(3717, 0)
(3718, 11.324)
(3719, 11.898)
(3720, 15.512)
(3721, 0)
(3722, 0)
(3723, 0)
(3724, 2.652)
(3725, 16.444)
(3726, 36.508)
(3727, 49.356)
(3728, 35.484)
(3729, 42.352)
(3730, 54.336)
(3731, 44.246)
(3732, 40.254)
(3733, 67.168)
(3734, 53.356)
(3735, 52.496)
(3736, 33.686)
(3737, 65.814)
(3738, 77.524)
(3739, 85.658)
(3740, 67.964)
(3741, 41.814)
(3742, 65.992)
(3743, 40.066)
(3744, 69.182)
(3745, 56.014)
(3746, 54.76)
(3747, 54.314)
(3748, 34.958)
(3749, 48.674)
(3750, 24.256)
(3751, 47.57)
(3752, 70.51)
(3753, 65.9)
(3754, 60.01)
(3755, 68.408)
(3756, 73.194)
(3757, 61.178)
(3758, 65.152)
(3759, 42.274)
(3760, 59.788)
(3761, 78.85)
(3762, 88.744)
(3763, 74.338)
(3764, 74.842)
(3765, 84.318)
(3766, 74.558)
(3767, 90.864)
(3768, 88.768)
(3769, 88.24)
(3770, 87.268)
(3771, 88.636)
(3772, 83.664)
(3773, 87.744)
(3774, 84.262)
(3775, 86.214)
(3776, 67.678)
(3777, 72.77)
(3778, 69.224)
(3779, 74.298)
(3780, 87.598)
(3781, 78.474)
(3782, 78.69)
(3783, 91.288)
(3784, 94.32)
(3785, 94.22)
(3786, 91.174)
(3787, 92.408)
(3788, 89.322)
(3789, 93.28)
(3790, 92.616)
(3791, 90.58)
(3792, 94.326)
(3793, 93.592)
(3794, 95.762)
(3795, 92.312)
(3796, 92.754)
(3797, 93.312)
(3798, 94.406)
(3799, 97.514)
(3800, 95.762)
(3801, 96.642)
(3802, 98.144)
(3803, 97.908)
(3804, 94.952)
(3805, 97.784)
(3806, 98.728)
(3807, 96.638)
(3808, 97.302)
(3809, 96.94)
(3810, 98.706)
(3811, 99.41)
(3812, 99.462)
(3813, 99.402)
(3814, 99.358)
(3815, 98.998)
(3816, 98.51)
(3817, 97.22)
(3818, 95.04)
(3819, 96.986)
(3820, 96.922)
(3821, 98.542)
(3822, 96.346)
(3823, 95.136)
(3824, 97.582)
(3825, 97.074)
(3826, 95.74)
(3827, 96.816)
(3828, 97.544)
(3829, 95.67)
(3830, 96.688)
(3831, 95.506)
(3832, 95.802)
(3833, 94.996)
(3834, 94.068)
(3835, 96.91)
(3836, 97.196)
(3837, 97.18)
(3838, 96.844)
(3839, 95.96)
(3840, 98.366)
(3841, 98.466)
(3842, 98.7)
(3843, 98.344)
(3844, 97.366)
(3845, 98.152)
(3846, 98.37)
(3847, 98.566)
(3848, 97.802)
(3849, 97.928)
(3850, 98.77)
(3851, 97.876)
(3852, 98.23)
(3853, 98.81)
(3854, 98.174)
(3855, 98.512)
(3856, 98.628)
(3857, 98.382)
(3858, 98.33)
(3859, 97.954)
(3860, 97.428)
(3861, 97.958)
(3862, 98.234)
(3863, 96.722)
(3864, 97.698)
(3865, 98.69)
(3866, 98.986)
(3867, 98.768)
(3868, 98.81)
(3869, 98.888)
(3870, 98.364)
(3871, 98.716)
(3872, 98.118)
(3873, 98.136)
(3874, 98.69)
(3875, 98.326)
(3876, 97.946)
(3877, 99.162)
(3878, 98.272)
(3879, 99.428)
(3880, 99.1)
(3881, 99.408)
(3882, 99.378)
(3883, 98.76)
(3884, 98.812)
(3885, 99.13)
(3886, 98.208)
(3887, 99.126)
(3888, 99.854)
(3889, 98.928)
(3890, 98.268)
(3891, 99.022)
(3892, 98.172)
(3893, 98.604)
(3894, 98.068)
(3895, 99.016)
(3896, 98.662)
(3897, 98.822)
(3898, 98.788)
(3899, 98.212)
(3900, 99.486)
(3901, 99.49)
(3902, 99.534)
(3903, 98.472)
(3904, 99.312)
(3905, 99.464)
(3906, 99.704)
(3907, 97.948)
(3908, 99.57)
(3909, 98.902)
(3910, 97.794)
(3911, 99.58)
(3912, 98.904)
(3913, 97.71)
(3914, 99.06)
(3915, 99.326)
(3916, 98.83)
(3917, 99.244)
(3918, 99.312)
(3919, 99.526)
(3920, 99.942)
(3921, 99.216)
(3922, 98.714)
(3923, 99.184)
(3924, 98.52)
(3925, 98.864)
(3926, 98.71)
(3927, 99.148)
(3928, 99.408)
(3929, 98.768)
(3930, 99.164)
(3931, 97.946)
(3932, 98.966)
(3933, 97.754)
(3934, 98.764)
(3935, 96.852)
(3936, 97.93)
(3937, 98.944)
(3938, 95.926)
(3939, 97.066)
(3940, 99.428)
(3941, 99.184)
(3942, 98.894)
(3943, 97.128)
(3944, 98.674)
(3945, 97.432)
(3946, 98.892)
(3947, 97.882)
(3948, 98.836)
(3949, 97.954)
(3950, 98.208)
(3951, 99.292)
(3952, 99.634)
(3953, 98.808)
(3954, 99.24)
(3955, 99.742)
(3956, 99.412)
(3957, 99.464)
(3958, 98.826)
(3959, 98.274)
(3960, 99.346)
(3961, 99.466)
(3962, 99.418)
(3963, 99.37)
(3964, 98.84)
(3965, 99.424)
(3966, 99.162)
(3967, 97.014)
(3968, 99.396)
(3969, 99.876)
(3970, 99.752)
(3971, 99.67)
(3972, 99.62)
(3973, 99.812)
(3974, 99.558)
(3975, 99.348)
(3976, 99.414)
(3977, 99.484)
(3978, 99.142)
(3979, 99.61)
(3980, 99.206)
(3981, 98.852)
(3982, 99.076)
(3983, 98.164)
(3984, 99.564)
(3985, 99.74)
(3986, 99.242)
(3987, 99.698)
(3988, 99.476)
(3989, 99.424)
(3990, 98.128)
(3991, 99.102)
(3992, 96.374)
(3993, 99.132)
(3994, 99.284)
(3995, 99.018)
(3996, 99.664)
(3997, 99.56)
(3998, 99.346)
(3999, 98.982)
(4000, 99.708)
(4001, 99.784)
(4002, 99.64)
(4003, 99.706)
(4004, 99.196)
(4005, 99.42)
(4006, 99.506)
(4007, 99.682)
(4008, 99.486)
(4009, 99.864)
(4010, 99.502)
(4011, 98.832)
(4012, 99.712)
(4013, 98.24)
(4014, 99.668)
(4015, 99.874)
(4016, 99.598)
(4017, 99.958)
(4018, 99.976)
(4019, 99.994)
(4020, 99.986)
(4021, 99.728)
(4022, 99.584)
(4023, 99.59)
(4024, 99.638)
(4025, 98.994)
(4026, 97.148)
(4027, 99.21)
(4028, 99.294)
(4029, 99.138)
(4030, 99.102)
(4031, 99.046)
(4032, 99.868)
(4033, 99.676)
(4034, 99.69)
(4035, 99.808)
(4036, 99.722)
(4037, 99.84)
(4038, 99.72)
(4039, 99.742)
(4040, 99.912)
(4041, 99.874)
(4042, 99.978)
(4043, 100)
(4044, 100)
(4045, 99.994)
(4046, 99.996)
(4047, 99.964)
(4048, 99.946)
(4049, 99.98)
(4050, 99.994)
(4051, 100)
(4052, 99.982)
(4053, 99.736)
(4054, 99.832)
(4055, 99.38)
(4056, 99.802)
(4057, 99.724)
(4058, 99.82)
(4059, 99.752)
(4060, 99.9)
(4061, 99.772)
(4062, 99.928)
(4063, 99.958)
(4064, 99.992)
(4065, 99.996)
(4066, 99.988)
(4067, 99.976)
(4068, 99.82)
(4069, 99.956)
(4070, 100)
(4071, 99.99)
(4072, 99.962)
(4073, 99.992)
(4074, 99.944)
(4075, 99.594)
(4076, 99.516)
(4077, 99.954)
(4078, 99.984)
(4079, 99.998)
(4080, 99.988)
(4081, 99.998)
(4082, 99.982)
(4083, 99.984)
(4084, 99.996)
(4085, 99.996)
(4086, 99.96)
(4087, 99.838)
(4088, 99.768)
(4089, 99.884)
(4090, 99.998)
(4091, 99.952)
(4092, 99.918)
(4093, 99.24)
(4094, 100)
(4095, 99.97)
(4096, 99.998)
(4097, 99.982)
(4098, 99.996)
(4099, 99.996)
(4100, 100)
(4101, 100)
(4102, 100)
(4103, 99.96)
(4104, 99.998)
(4105, 100)
(4106, 100)
(4107, 99.966)
(4108, 99.988)
(4109, 100)
(4110, 100)
(4111, 100)
(4112, 99.982)
(4113, 99.996)
(4114, 99.95)
(4115, 100)
(4116, 99.996)
(4117, 99.996)
(4118, 99.98)
(4119, 99.982)
(4120, 99.996)
(4121, 99.934)
(4122, 99.986)
(4123, 99.936)
(4124, 99.976)
(4125, 97.976)
(4126, 99.914)
(4127, 99.96)
(4128, 89.824)
(4129, 90.746)
(4130, 91.376)
(4131, 99.998)
(4132, 99.918)
(4133, 99.896)
(4134, 99.838)
(4135, 92.992)
(4136, 99.854)
(4137, 98.066)
(4138, 97.68)
(4139, 98.884)
(4140, 98.268)
(4141, 97.412)
(4142, 99.488)
(4143, 98.892)
(4144, 99.234)
(4145, 99.718)
(4146, 99.852)
(4147, 99.982)
(4148, 99.816)
(4149, 99.878)
(4150, 99.19)
(4151, 99.888)
(4152, 99.994)
(4153, 99.99)
(4154, 99.992)
(4155, 99.976)
(4156, 99.942)
(4157, 99.982)
(4158, 99.962)
(4159, 99.99)
(4160, 99.898)
(4161, 99.948)
(4162, 99.964)
(4163, 99.9)
(4164, 99.896)
(4165, 99.896)
(4166, 99.828)
(4167, 99.926)
(4168, 99.756)
(4169, 99.812)
(4170, 99.874)
(4171, 99.742)
(4172, 99.76)
(4173, 99.756)
(4174, 99.924)
(4175, 99.91)
(4176, 98.572)
(4177, 99.39)
(4178, 98.806)
(4179, 97.744)
(4180, 98.816)
(4181, 98.606)
(4182, 99.544)
(4183, 99.622)
(4184, 99.678)
(4185, 98.96)
(4186, 99.036)
(4187, 99.548)
(4188, 99.756)
(4189, 97.134)
(4190, 99.898)
(4191, 99.988)
(4192, 99.958)
(4193, 99.894)
(4194, 99.994)
(4195, 99.958)
(4196, 99.932)
(4197, 99.9)
(4198, 99.98)
(4199, 99.928)
(4200, 98.744)
(4201, 98.134)
(4202, 100)
(4203, 99.994)
(4204, 99.992)
(4205, 99.986)
(4206, 99.986)
(4207, 99.992)
(4208, 99.972)
(4209, 99.994)
(4210, 99.99)
(4211, 99.976)
(4212, 99.962)
(4213, 99.964)
(4214, 99.958)
(4215, 99.968)
(4216, 99.798)
(4217, 99.716)
(4218, 99.652)
(4219, 99.688)
(4220, 99.77)
(4221, 99.722)
(4222, 99.62)
(4223, 98.142)
(4224, 98.262)
(4225, 99.748)
(4226, 99.256)
(4227, 98.264)
(4228, 97.942)
(4229, 98.22)
(4230, 98.574)
(4231, 98.844)
(4232, 96.482)
(4233, 97.028)
(4234, 98.142)
(4235, 98.076)
(4236, 97.874)
(4237, 96.414)
(4238, 96.516)
(4239, 97.24)
(4240, 97.862)
(4241, 97.79)
(4242, 98.154)
(4243, 97.716)
(4244, 91.986)
(4245, 94.3)
(4246, 96.734)
(4247, 94.392)
(4248, 94.922)
(4249, 95.348)
(4250, 96.796)
(4251, 96.98)
(4252, 98.428)
(4253, 98.52)
(4254, 98.372)
(4255, 99.158)
(4256, 98.762)
(4257, 98.074)
(4258, 96.506)
(4259, 97.106)
(4260, 94.72)
(4261, 97.89)
(4262, 98.206)
(4263, 98.144)
(4264, 97.378)
(4265, 97.852)
(4266, 96.888)
(4267, 95.73)
(4268, 97.404)
(4269, 95.176)
(4270, 98.358)
(4271, 99.14)
(4272, 97.558)
(4273, 97.412)
(4274, 97.756)
(4275, 97.228)
(4276, 97.34)
(4277, 96.07)
(4278, 96.066)
(4279, 92.374)
(4280, 97.63)
(4281, 98.266)
(4282, 98.486)
(4283, 95.562)
(4284, 97.282)
(4285, 97.822)
(4286, 97.914)
(4287, 97.62)
(4288, 98.812)
(4289, 97.812)
(4290, 92.72)
(4291, 95.348)
(4292, 92.282)
(4293, 95.756)
(4294, 97.974)
(4295, 96.654)
(4296, 98.498)
(4297, 98.236)
(4298, 99.384)
(4299, 95.538)
(4300, 98.022)
(4301, 98.71)
(4302, 99.256)
(4303, 98.792)
(4304, 94.608)
(4305, 98.584)
(4306, 96.35)
(4307, 93.836)
(4308, 98.098)
(4309, 98.178)
(4310, 96.5)
(4311, 96.54)
(4312, 94.226)
(4313, 94.724)
(4314, 94.846)
(4315, 96.936)
(4316, 97.27)
(4317, 97.372)
(4318, 94.246)
(4319, 96.718)
(4320, 98.38)
(4321, 99.17)
(4322, 98.128)
(4323, 96.804)
(4324, 98.38)
(4325, 98.882)
(4326, 99.48)
(4327, 99.378)
(4328, 98.62)
(4329, 99.528)
(4330, 99.58)
(4331, 99.728)
(4332, 99.816)
(4333, 99.428)
(4334, 99.444)
(4335, 99.596)
(4336, 99.688)
(4337, 92.192)
(4338, 91.754)
(4339, 98.474)
(4340, 99.448)
(4341, 99.654)
(4342, 93.304)
(4343, 99.036)
(4344, 99.32)
(4345, 99.6)
(4346, 99.39)
(4347, 98.756)
(4348, 99.096)
(4349, 97.982)
(4350, 99.028)
(4351, 98.95)
(4352, 99.128)
(4353, 99.166)
(4354, 99.216)
(4355, 99.33)
(4356, 99.212)
(4357, 98.13)
(4358, 97.5)
(4359, 97.192)
(4360, 99.35)
(4361, 99.378)
(4362, 98.52)
(4363, 99.288)
(4364, 98.724)
(4365, 98.078)
(4366, 98.61)
(4367, 99.448)
(4368, 99.518)
(4369, 99.65)
(4370, 99.582)
(4371, 99.864)
(4372, 99.856)
(4373, 99.612)
(4374, 99.57)
(4375, 92.492)
(4376, 99.716)
(4377, 99.7)
(4378, 99.648)
(4379, 99.508)
(4380, 99.39)
(4381, 99.232)
(4382, 99.054)
(4383, 98.87)
(4384, 99.052)
(4385, 98.686)
(4386, 98.622)
(4387, 98.29)
(4388, 98.222)
(4389, 99.564)
(4390, 99.606)
(4391, 99.428)
(4392, 99.632)
(4393, 98.612)
(4394, 98.74)
(4395, 97.98)
(4396, 99.052)
(4397, 96.532)
(4398, 99.056)
(4399, 96.946)
(4400, 99.7)
(4401, 99.528)
(4402, 99.692)
(4403, 99.69)
(4404, 99.898)
(4405, 99.474)
(4406, 99.11)
(4407, 97.824)
(4408, 99.482)
(4409, 97.84)
(4410, 98.906)
(4411, 98.448)
(4412, 99.236)
(4413, 98.948)
(4414, 95.516)
(4415, 98.116)
(4416, 98.902)
(4417, 99.26)
(4418, 99.978)
(4419, 99.82)
(4420, 99.684)
(4421, 99.906)
(4422, 99.822)
(4423, 99.764)
(4424, 99.338)
(4425, 99.812)
(4426, 99.52)
(4427, 98.742)
(4428, 99.05)
(4429, 98.3)
(4430, 99.512)
(4431, 98.41)
(4432, 97.666)
(4433, 95.72)
(4434, 97.374)
(4435, 99.398)
(4436, 98.918)
(4437, 99.098)
(4438, 98.832)
(4439, 99.448)
(4440, 97.852)
(4441, 98.832)
(4442, 99.344)
(4443, 98.572)
(4444, 99.45)
(4445, 96.544)
(4446, 99.434)
(4447, 99.614)
(4448, 99.306)
(4449, 98.65)
(4450, 99.282)
(4451, 98.694)
(4452, 98.15)
(4453, 99.722)
(4454, 87.776)
(4455, 98.864)
(4456, 99.344)
(4457, 99.888)
(4458, 98.472)
(4459, 99.814)
(4460, 99.59)
(4461, 99.662)
(4462, 99.924)
(4463, 99.9)
(4464, 99.748)
(4465, 99.612)
(4466, 99.804)
(4467, 99.726)
(4468, 99.826)
(4469, 99.702)
(4470, 99.834)
(4471, 99.964)
(4472, 99.916)
(4473, 99.924)
(4474, 99.93)
(4475, 99.9)
(4476, 99.906)
(4477, 99.694)
(4478, 99.934)
(4479, 99.83)
(4480, 97.982)
(4481, 99.68)
(4482, 99.94)
(4483, 99.942)
(4484, 99.612)
(4485, 99.744)
(4486, 99.898)
(4487, 99.156)
(4488, 99.726)
(4489, 99.902)
(4490, 99.536)
(4491, 99.71)
(4492, 99.896)
(4493, 99.914)
(4494, 99.492)
(4495, 99.876)
(4496, 99.362)
(4497, 99.834)
(4498, 99.76)
(4499, 99.874)
(4500, 99.874)
(4501, 99.244)
(4502, 99.818)
(4503, 99.926)
(4504, 99.738)
(4505, 99.358)
(4506, 99.882)
(4507, 99.978)
(4508, 99.87)
(4509, 99.746)
(4510, 99.878)
(4511, 99.818)
(4512, 99.182)
(4513, 99.832)
(4514, 99.99)
(4515, 99.702)
(4516, 99.21)
(4517, 99.19)
(4518, 99.09)
(4519, 99.218)
(4520, 99.702)
(4521, 98.612)
(4522, 99.496)
(4523, 99.828)
(4524, 99.16)
(4525, 99.222)
(4526, 99.7)
(4527, 99.556)
(4528, 99.922)
(4529, 99.62)
(4530, 98.712)
(4531, 99.864)
(4532, 99.742)
(4533, 99.868)
(4534, 99.974)
(4535, 99.992)
(4536, 99.992)
(4537, 99.862)
(4538, 99.964)
(4539, 99.904)
(4540, 99.916)
(4541, 99.898)
(4542, 99.952)
(4543, 99.764)
(4544, 99.636)
(4545, 99.842)
(4546, 99.858)
(4547, 99.488)
(4548, 99.824)
(4549, 99.684)
(4550, 99.914)
(4551, 99.99)
(4552, 99.98)
(4553, 99.082)
(4554, 98.786)
(4555, 99.122)
(4556, 99.916)
(4557, 99.378)
(4558, 99.95)
(4559, 99.828)
(4560, 99.552)
(4561, 99.942)
(4562, 99.962)
(4563, 99.984)
(4564, 99.85)
(4565, 99.848)
(4566, 99.932)
(4567, 99.99)
(4568, 99.938)
(4569, 99.952)
(4570, 99.826)
(4571, 99.99)
(4572, 99.95)
(4573, 99.896)
(4574, 98.83)
(4575, 98.286)
(4576, 99.958)
(4577, 99.848)
(4578, 99.816)
(4579, 99.45)
(4580, 97.124)
(4581, 99.306)
(4582, 98.818)
(4583, 99.266)
(4584, 99.234)
(4585, 98.896)
(4586, 99.566)
(4587, 99.038)
(4588, 99.012)
(4589, 98.474)
(4590, 98.686)
(4591, 99.464)
(4592, 99.144)
(4593, 98.502)
(4594, 98.968)
(4595, 98.376)
(4596, 96.1)
(4597, 98.754)
(4598, 98.2)
(4599, 99.25)
(4600, 98.896)
(4601, 91.392)
(4602, 98.648)
(4603, 99.554)
(4604, 98.71)
(4605, 90.946)
(4606, 98.528)
(4607, 99.52)
(4608, 98.244)
(4609, 99.418)
(4610, 99.238)
(4611, 98.782)
(4612, 99.468)
(4613, 99.332)
(4614, 96.924)
(4615, 98.962)
(4616, 99.51)
(4617, 96.14)
(4618, 99.258)
(4619, 99.822)
(4620, 99.58)
(4621, 99.904)
(4622, 99.934)
(4623, 99.694)
(4624, 99.5)
(4625, 99.678)
(4626, 99.85)
(4627, 99.896)
(4628, 99.938)
(4629, 99.944)
(4630, 99.73)
(4631, 99.456)
(4632, 99.734)
(4633, 99.916)
(4634, 99.854)
(4635, 99.898)
(4636, 99.916)
(4637, 99.802)
(4638, 99.834)
(4639, 99.9)
(4640, 99.66)
(4641, 99.81)
(4642, 99.83)
(4643, 99.748)
(4644, 99.08)
(4645, 99.686)
(4646, 99.79)
(4647, 99.764)
(4648, 99.752)
(4649, 98.72)
(4650, 99.808)
(4651, 99.83)
(4652, 99.534)
(4653, 99.486)
(4654, 99.904)
(4655, 99.824)
(4656, 98.678)
(4657, 99.096)
(4658, 98.914)
(4659, 99.244)
(4660, 99.906)
(4661, 99.178)
(4662, 99.224)
(4663, 97.288)
(4664, 99.75)
(4665, 97.662)
(4666, 99.834)
(4667, 99.734)
(4668, 99.958)
(4669, 99.86)
(4670, 99.778)
(4671, 99.364)
(4672, 99.622)
(4673, 99.786)
(4674, 99.572)
(4675, 99.69)
(4676, 99.876)
(4677, 99.496)
(4678, 99.14)
(4679, 99.832)
(4680, 99.582)
(4681, 99.576)
(4682, 99.848)
(4683, 99.894)
(4684, 99.962)
(4685, 99.952)
(4686, 99.492)
(4687, 99.526)
(4688, 99.73)
(4689, 99.802)
(4690, 99.226)
(4691, 99.92)
(4692, 99.858)
(4693, 99.802)
(4694, 99.864)
(4695, 99.978)
(4696, 99.976)
(4697, 99.856)
(4698, 99.338)
(4699, 98.148)
(4700, 99.672)
(4701, 98.898)
(4702, 99.51)
(4703, 98.796)
(4704, 99.632)
(4705, 99.634)
(4706, 99.07)
(4707, 99.228)
(4708, 99.896)
(4709, 99.954)
(4710, 99.914)
(4711, 97.52)
(4712, 99.64)
(4713, 99.402)
(4714, 99.448)
(4715, 99.834)
(4716, 99.91)
(4717, 99.754)
(4718, 99.608)
(4719, 99.65)
(4720, 99.864)
(4721, 99.708)
(4722, 99.602)
(4723, 99.658)
(4724, 99.764)
(4725, 99.934)
(4726, 99.966)
(4727, 99.982)
(4728, 99.916)
(4729, 99.516)
(4730, 98.646)
(4731, 99.874)
(4732, 99.902)
(4733, 99.516)
(4734, 99.946)
(4735, 99.87)
(4736, 99.508)
(4737, 99.974)
(4738, 99.928)
(4739, 99.734)
(4740, 99.862)
(4741, 99.756)
(4742, 99.998)
(4743, 99.944)
(4744, 98.954)
(4745, 99.336)
(4746, 98.314)
(4747, 99.558)
(4748, 99.372)
(4749, 99.672)
(4750, 99.554)
(4751, 99.524)
(4752, 99.2)
(4753, 98.938)
(4754, 97.996)
(4755, 99.704)
(4756, 99.608)
(4757, 99.928)
(4758, 99.986)
(4759, 99.932)
(4760, 99.746)
(4761, 100)
(4762, 99.996)
(4763, 99.986)
(4764, 99.988)
(4765, 99.928)
(4766, 99.922)
(4767, 99.9)
(4768, 99.858)
(4769, 99.95)
(4770, 99.984)
(4771, 99.996)
(4772, 99.972)
(4773, 99.988)
(4774, 99.99)
(4775, 99.932)
(4776, 99.206)
(4777, 98.334)
(4778, 99.75)
(4779, 99.524)
(4780, 98.664)
(4781, 99.746)
(4782, 99.646)
(4783, 99.55)
(4784, 98.958)
(4785, 98.956)
(4786, 98.128)
(4787, 99.848)
(4788, 97.352)
(4789, 98.92)
(4790, 99.55)
(4791, 98.922)
(4792, 99.658)
(4793, 99.54)
(4794, 99.524)
(4795, 99.588)
(4796, 99.36)
(4797, 99.254)
(4798, 99.158)
(4799, 99.614)
(4800, 99.428)
(4801, 99.106)
(4802, 99.76)
(4803, 99.908)
(4804, 99.948)
(4805, 99.642)
(4806, 99.998)
(4807, 99.474)
(4808, 99.918)
(4809, 99.894)
(4810, 99.984)
(4811, 99.932)
(4812, 99.86)
(4813, 99.9)
(4814, 99.908)
(4815, 99.566)
(4816, 99.718)
(4817, 99.176)
(4818, 99.83)
(4819, 98.99)
(4820, 99.802)
(4821, 99.67)
(4822, 99.94)
(4823, 99.75)
(4824, 99.53)
(4825, 99.14)
(4826, 99.592)
(4827, 97.958)
(4828, 99.66)
(4829, 99.546)
(4830, 99.874)
(4831, 99.482)
(4832, 99.73)
(4833, 99.606)
(4834, 99.886)
(4835, 99.514)
(4836, 99.786)
(4837, 99.348)
(4838, 99.782)
(4839, 99.812)
(4840, 99.206)
(4841, 99.878)
(4842, 99.972)
(4843, 99.818)
(4844, 99.756)
(4845, 99.854)
(4846, 99.842)
(4847, 99.846)
(4848, 99.812)
(4849, 99.96)
(4850, 99.834)
(4851, 99.91)
(4852, 99.906)
(4853, 99.92)
(4854, 99.74)
(4855, 99.554)
(4856, 99.896)
(4857, 99.93)
(4858, 98.446)
(4859, 99.504)
(4860, 99.022)
(4861, 98.892)
(4862, 99.462)
(4863, 99.916)
(4864, 99.742)
(4865, 99.446)
(4866, 98.98)
(4867, 98.696)
(4868, 98.87)
(4869, 99.744)
(4870, 99.536)
(4871, 99.446)
(4872, 99.56)
(4873, 99.514)
(4874, 98.872)
(4875, 99.34)
(4876, 99.484)
(4877, 99.332)
(4878, 98.888)
(4879, 99.688)
(4880, 99.45)
(4881, 98.308)
(4882, 99.818)
(4883, 99.776)
(4884, 99.606)
(4885, 99.658)
(4886, 99.494)
(4887, 99.836)
(4888, 98.066)
(4889, 99.388)
(4890, 98.726)
(4891, 99.77)
(4892, 99.826)
(4893, 99.776)
(4894, 99.082)
(4895, 99.984)
(4896, 99.968)
(4897, 99.994)
(4898, 99.986)
(4899, 99.938)
(4900, 98.408)
(4901, 99.504)
(4902, 99.786)
(4903, 99.652)
(4904, 99.864)
(4905, 99.992)
(4906, 99.968)
(4907, 99.966)
(4908, 99.998)
(4909, 99.954)
(4910, 99.95)
(4911, 99.99)
(4912, 99.864)
(4913, 99.85)
(4914, 99.37)
(4915, 99.82)
(4916, 99.814)
(4917, 99.97)
(4918, 99.984)
(4919, 99.968)
(4920, 99.994)
(4921, 99.976)
(4922, 100)
(4923, 100)
(4924, 99.95)
(4925, 99.97)
(4926, 99.916)
(4927, 99.978)
(4928, 99.996)
(4929, 99.994)
(4930, 99.992)
(4931, 99.996)
(4932, 100)
(4933, 100)
(4934, 100)
(4935, 100)
(4936, 100)
(4937, 100)
(4938, 99.998)
(4939, 99.982)
(4940, 99.98)
(4941, 99.942)
(4942, 99.982)
(4943, 99.996)
(4944, 99.796)
(4945, 100)
(4946, 100)
(4947, 99.998)
(4948, 100)
(4949, 100)
(4950, 100)
(4951, 100)
(4952, 100)
(4953, 99.984)
(4954, 99.998)
(4955, 100)
(4956, 99.99)
(4957, 99.998)
(4958, 100)
(4959, 100)
(4960, 100)
(4961, 99.996)
(4962, 100)
(4963, 100)
(4964, 100)
(4965, 100)
(4966, 100)
(4967, 100)
(4968, 100)
(4969, 100)
(4970, 100)
(4971, 100)
(4972, 99.998)
(4973, 100)
(4974, 99.9)
(4975, 100)
(4976, 99.972)
(4977, 99.972)
(4978, 99.464)
(4979, 99.986)
(4980, 100)
(4981, 99.988)
(4982, 100)
(4983, 100)
(4984, 99.998)
(4985, 100)
(4986, 99.996)
(4987, 100)
(4988, 99.992)
(4989, 100)
(4990, 99.962)
(4991, 99.952)
(4992, 99.926)
(4993, 99.904)
(4994, 99.92)
(4995, 99.998)
(4996, 99.996)
(4997, 99.994)
(4998, 99.924)
(4999, 99.984)
(5000, 99.998)
(5001, 99.892)
(5002, 98.52)
(5003, 99.948)
(5004, 99.786)
(5005, 99.476)
(5006, 99.268)
(5007, 99.898)
(5008, 99.746)
(5009, 99.498)
(5010, 99.246)
(5011, 99.524)
(5012, 99.936)
(5013, 99.942)
(5014, 100)
(5015, 99.844)
(5016, 99.91)
(5017, 99.338)
(5018, 99.924)
(5019, 99.898)
(5020, 99.984)
(5021, 99.99)
(5022, 99.998)
(5023, 99.938)
(5024, 99.75)
(5025, 99.656)
(5026, 99.974)
(5027, 99.99)
(5028, 99.998)
(5029, 99.98)
(5030, 99.07)
(5031, 99.996)
(5032, 99.994)
(5033, 100)
(5034, 99.92)
(5035, 99.972)
(5036, 99.978)
(5037, 99.962)
(5038, 99.8)
(5039, 100)
(5040, 100)
(5041, 100)
(5042, 99.994)
(5043, 99.99)
(5044, 99.922)
(5045, 99.948)
(5046, 99.988)
(5047, 99.3)
(5048, 99.79)
(5049, 99.984)
(5050, 99.778)
(5051, 99.956)
(5052, 99.926)
(5053, 99.868)
(5054, 99.874)
(5055, 99.552)
(5056, 99.978)
(5057, 99.04)
(5058, 99.924)
(5059, 99.918)
(5060, 99.872)
(5061, 99.37)
(5062, 99.974)
(5063, 99.866)
(5064, 99.97)
(5065, 99.92)
(5066, 97.39)
(5067, 99.99)
(5068, 99.88)
(5069, 99.908)
(5070, 99.924)
(5071, 99.986)
(5072, 99.998)
(5073, 99.472)
(5074, 99.752)
(5075, 98.922)
(5076, 98.816)
(5077, 98.398)
(5078, 98.974)
(5079, 99.616)
(5080, 98.934)
(5081, 99.47)
(5082, 98.756)
(5083, 99.132)
(5084, 98.878)
(5085, 99.82)
(5086, 99.628)
(5087, 99.264)
(5088, 98.96)
(5089, 99.792)
(5090, 99.456)
(5091, 96.72)
(5092, 99.59)
(5093, 99.522)
(5094, 99.334)
(5095, 99.732)
(5096, 99.352)
(5097, 99.838)
(5098, 99.44)
(5099, 99.704)
(5100, 99.734)
(5101, 99.86)
(5102, 99.098)
(5103, 97.646)
(5104, 98.064)
(5105, 99.72)
(5106, 95.472)
(5107, 98.782)
(5108, 98.642)
(5109, 98.992)
(5110, 98.812)
(5111, 99.402)
(5112, 99.662)
(5113, 99.59)
(5114, 99.618)
(5115, 98.17)
(5116, 99.946)
(5117, 99.944)
(5118, 99.968)
(5119, 99.982)
(5120, 99.938)
(5121, 99.958)
(5122, 99.842)
(5123, 99.942)
(5124, 100)
(5125, 99.972)
(5126, 99.994)
(5127, 99.832)
(5128, 99.506)
(5129, 99.93)
(5130, 99.91)
(5131, 99.756)
(5132, 99.716)
(5133, 99.816)
(5134, 99.808)
(5135, 99.862)
(5136, 96.5)
(5137, 99.196)
(5138, 99.444)
(5139, 98.49)
(5140, 99.098)
(5141, 98.506)
(5142, 99.766)
(5143, 98.422)
(5144, 99.216)
(5145, 99.592)
(5146, 99.928)
(5147, 99.912)
(5148, 99.924)
(5149, 99.798)
(5150, 98.624)
(5151, 99.332)
(5152, 99.932)
(5153, 99.938)
(5154, 99.894)
(5155, 99.776)
(5156, 99.662)
(5157, 99.65)
(5158, 99.526)
(5159, 99.808)
(5160, 99.536)
(5161, 99.814)
(5162, 99.942)
(5163, 99.418)
(5164, 99.288)
(5165, 99.666)
(5166, 99.53)
(5167, 99.97)
(5168, 99.884)
(5169, 99.92)
(5170, 99.908)
(5171, 99.954)
(5172, 99.874)
(5173, 99.904)
(5174, 99.978)
(5175, 99.842)
(5176, 99.438)
(5177, 99.956)
(5178, 99.944)
(5179, 99.846)
(5180, 99.94)
(5181, 99.988)
(5182, 99.5)
(5183, 99.974)
(5184, 99.762)
(5185, 99.788)
(5186, 98.762)
(5187, 99.914)
(5188, 99.874)
(5189, 99.832)
(5190, 99.974)
(5191, 99.928)
(5192, 99.8)
(5193, 99.76)
(5194, 99.122)
(5195, 99.962)
(5196, 99.97)
(5197, 99.992)
(5198, 99.904)
(5199, 99.89)
(5200, 99.328)
(5201, 99.692)
(5202, 99.652)
(5203, 99.4)
(5204, 99.866)
(5205, 99.856)
(5206, 99.306)
(5207, 98.6)
(5208, 99.828)
(5209, 99.782)
(5210, 99.968)
(5211, 99.688)
(5212, 97.674)
(5213, 99.694)
(5214, 99.896)
(5215, 99.822)
(5216, 99.804)
(5217, 98.584)
(5218, 96.846)
(5219, 98.946)
(5220, 99.968)
(5221, 99.968)
(5222, 99.826)
(5223, 99.92)
(5224, 99.894)
(5225, 99.724)
(5226, 99.946)
(5227, 98.436)
(5228, 99.986)
(5229, 99.78)
(5230, 99.544)
(5231, 99.972)
(5232, 99.93)
(5233, 99.908)
(5234, 99.274)
(5235, 97.93)
(5236, 99.972)
(5237, 99.974)
(5238, 100)
(5239, 99.978)
(5240, 99.98)
(5241, 99.892)
(5242, 99.998)
(5243, 99.98)
(5244, 99.74)
(5245, 99.902)
(5246, 99.982)
(5247, 99.996)
(5248, 99.066)
(5249, 99.99)
(5250, 100)
(5251, 99.998)
(5252, 100)
(5253, 100)
(5254, 100)
(5255, 100)
(5256, 99.918)
(5257, 99.934)
(5258, 99.996)
(5259, 99.958)
(5260, 99.97)
(5261, 99.958)
(5262, 99.974)
(5263, 99.996)
(5264, 99.994)
(5265, 99.908)
(5266, 99.764)
(5267, 99.988)
(5268, 99.972)
(5269, 99.992)
(5270, 99.978)
(5271, 99.98)
(5272, 99.974)
(5273, 99.996)
(5274, 99.982)
(5275, 99.934)
(5276, 99.93)
(5277, 99.952)
(5278, 99.79)
(5279, 99.98)
(5280, 97.494)
(5281, 99.988)
(5282, 99.942)
(5283, 99.87)
(5284, 99.878)
(5285, 99.96)
(5286, 99.64)
(5287, 99.256)
(5288, 99.95)
(5289, 99.77)
(5290, 99.498)
(5291, 99.902)
(5292, 99.946)
(5293, 99.936)
(5294, 99.75)
(5295, 99.912)
(5296, 99.81)
(5297, 99.96)
(5298, 99.946)
(5299, 99.826)
(5300, 99.866)
(5301, 99.944)
(5302, 98.886)
(5303, 99.986)
(5304, 99.98)
(5305, 99.936)
(5306, 98.142)
(5307, 99.928)
(5308, 99.918)
(5309, 99.968)
(5310, 99.766)
(5311, 99.65)
(5312, 99.284)
(5313, 96.406)
(5314, 99.828)
(5315, 99.95)
(5316, 99.9)
(5317, 99.936)
(5318, 99.906)
(5319, 99.918)
(5320, 99.524)
(5321, 99.694)
(5322, 99.646)
(5323, 98.894)
(5324, 99.376)
(5325, 99.858)
(5326, 99.94)
(5327, 99.658)
(5328, 99.648)
(5329, 99.778)
(5330, 99.47)
(5331, 99.918)
(5332, 99.968)
(5333, 99.96)
(5334, 99.858)
(5335, 99.874)
(5336, 99.564)
(5337, 99.802)
(5338, 99.646)
(5339, 99.556)
(5340, 99.61)
(5341, 99.688)
(5342, 99.956)
(5343, 99.902)
(5344, 98.654)
(5345, 99.94)
(5346, 99.91)
(5347, 99.528)
(5348, 99.464)
(5349, 99.95)
(5350, 99.844)
(5351, 99.366)
(5352, 99.364)
(5353, 99.948)
(5354, 99.686)
(5355, 99.83)
(5356, 99.83)
(5357, 99.584)
(5358, 99.536)
(5359, 99.926)
(5360, 98.768)
(5361, 99.894)
(5362, 99.794)
(5363, 99.92)
(5364, 99.934)
(5365, 99.858)
(5366, 99.962)
(5367, 99.994)
(5368, 99.9)
(5369, 99.922)
(5370, 99.97)
(5371, 99.938)
(5372, 99.424)
(5373, 99.894)
(5374, 99.582)
(5375, 99.986)
(5376, 99.964)
(5377, 99.888)
(5378, 99.994)
(5379, 99.966)
(5380, 99.9)
(5381, 99.84)
(5382, 97.512)
(5383, 98.974)
(5384, 98.14)
(5385, 99.654)
(5386, 99.798)
(5387, 99.958)
(5388, 99.988)
(5389, 99.98)
(5390, 99.994)
(5391, 99.942)
(5392, 99.912)
(5393, 99.334)
(5394, 99.736)
(5395, 100)
(5396, 100)
(5397, 99.952)
(5398, 99.908)
(5399, 99.91)
(5400, 99.876)
(5401, 99.994)
(5402, 99.842)
(5403, 99.984)
(5404, 99.862)
(5405, 99.984)
(5406, 99.71)
(5407, 99.976)
(5408, 99.968)
(5409, 99.756)
(5410, 99.962)
(5411, 99.928)
(5412, 99.996)
(5413, 99.99)
(5414, 99.964)
(5415, 99.992)
(5416, 99.982)
(5417, 99.946)
(5418, 99.96)
(5419, 99.958)
(5420, 99.762)
(5421, 99.446)
(5422, 99.47)
(5423, 99.974)
(5424, 99.998)
(5425, 99.996)
(5426, 99.992)
(5427, 99.992)
(5428, 100)
(5429, 100)
(5430, 99.972)
(5431, 99.922)
(5432, 99.878)
(5433, 99.954)
(5434, 99.998)
(5435, 99.968)
(5436, 99.906)
(5437, 99.622)
(5438, 99.996)
(5439, 99.922)
(5440, 100)
(5441, 100)
(5442, 100)
(5443, 100)
(5444, 99.896)
(5445, 100)
(5446, 100)
(5447, 100)
(5448, 99.998)
(5449, 99.996)
(5450, 99.998)
(5451, 99.982)
(5452, 99.988)
(5453, 99.978)
(5454, 99.994)
(5455, 99.984)
(5456, 99.942)
(5457, 99.582)
(5458, 99.952)
(5459, 99.996)
(5460, 99.976)
(5461, 99.976)
(5462, 99.936)
(5463, 99.944)
(5464, 99.882)
(5465, 98.858)
(5466, 99.086)
(5467, 99.966)
(5468, 99.918)
(5469, 99.914)
(5470, 99.998)
(5471, 99.996)
(5472, 99.982)
(5473, 99.952)
(5474, 99.994)
(5475, 99.93)
(5476, 99.774)
(5477, 99.868)
(5478, 99.992)
(5479, 99.996)
(5480, 100)
(5481, 99.952)
(5482, 99.984)
(5483, 99.976)
(5484, 99.942)
(5485, 99.982)
(5486, 99.848)
(5487, 99.972)
(5488, 99.866)
(5489, 99.552)
(5490, 99.668)
(5491, 99.832)
(5492, 99.732)
(5493, 99.904)
(5494, 99.916)
(5495, 99.902)
(5496, 99.878)
(5497, 99.988)
(5498, 99.904)
(5499, 99.712)
(5500, 99.866)
(5501, 99.898)
(5502, 99.83)
(5503, 99.976)
(5504, 99.898)
(5505, 99.884)
(5506, 99.886)
(5507, 99.938)
(5508, 99.956)
(5509, 99.978)
(5510, 99.956)
(5511, 100)
(5512, 100)
(5513, 99.982)
(5514, 99.998)
(5515, 99.996)
(5516, 100)
(5517, 100)
(5518, 99.994)
(5519, 100)
(5520, 99.988)
(5521, 100)
(5522, 99.992)
(5523, 100)
(5524, 99.998)
(5525, 100)
(5526, 100)
(5527, 99.994)
(5528, 100)
(5529, 100)
(5530, 100)
(5531, 99.988)
(5532, 99.98)
(5533, 99.954)
(5534, 99.98)
(5535, 99.668)
(5536, 99.91)
(5537, 99.928)
(5538, 100)
(5539, 99.958)
(5540, 99.984)
(5541, 99.776)
(5542, 99.954)
(5543, 100)
(5544, 100)
(5545, 100)
(5546, 99.998)
(5547, 99.972)
(5548, 99.944)
(5549, 99.944)
(5550, 98.718)
(5551, 99.982)
(5552, 99.942)
(5553, 98.912)
(5554, 98.262)
(5555, 99.822)
(5556, 99.932)
(5557, 99.994)
(5558, 99.93)
(5559, 99.98)
(5560, 99.996)
(5561, 100)
(5562, 99.982)
(5563, 99.996)
(5564, 99.996)
(5565, 99.994)
(5566, 99.976)
(5567, 99.97)
(5568, 99.986)
(5569, 99.948)
(5570, 99.954)
(5571, 99.972)
(5572, 99.938)
(5573, 99.802)
(5574, 99.356)
(5575, 99.246)
(5576, 97.796)
(5577, 98.528)
(5578, 98.386)
(5579, 94.712)
(5580, 97.702)
(5581, 99.108)
(5582, 98.424)
(5583, 96.67)
(5584, 98.496)
(5585, 99.224)
(5586, 99.818)
(5587, 99.554)
(5588, 99.528)
(5589, 99.71)
(5590, 99.788)
(5591, 99.902)
(5592, 99.7)
(5593, 99.94)
(5594, 99.818)
(5595, 99.4)
(5596, 99.57)
(5597, 99.408)
(5598, 98.32)
(5599, 99.162)
(5600, 99.758)
(5601, 99.266)
(5602, 99.49)
(5603, 99.676)
(5604, 99.85)
(5605, 99.914)
(5606, 99.796)
(5607, 99.708)
(5608, 97.412)
(5609, 96.51)
(5610, 99.442)
(5611, 99.708)
(5612, 99.47)
(5613, 98.782)
(5614, 98.748)
(5615, 99.256)
(5616, 99.242)
(5617, 99.716)
(5618, 99.684)
(5619, 99.376)
(5620, 98.842)
(5621, 99.326)
(5622, 98.178)
(5623, 95.7)
(5624, 99.474)
(5625, 98.922)
(5626, 99.45)
(5627, 99.832)
(5628, 99.71)
(5629, 99.788)
(5630, 99.634)
(5631, 99.66)
(5632, 99.356)
(5633, 99.568)
(5634, 98.95)
(5635, 99.278)
(5636, 99.54)
(5637, 99.718)
(5638, 99.096)
(5639, 99.576)
(5640, 99.524)
(5641, 99.708)
(5642, 98.754)
(5643, 97.5)
(5644, 97.65)
(5645, 97.194)
(5646, 98.532)
(5647, 99.708)
(5648, 95.316)
(5649, 97.936)
(5650, 97.584)
(5651, 97.854)
(5652, 99.004)
(5653, 98.006)
(5654, 99.1)
(5655, 99.046)
(5656, 96.012)
(5657, 96.78)
(5658, 97.2)
(5659, 97.266)
(5660, 98.796)
(5661, 99.01)
(5662, 98.686)
(5663, 96.076)
(5664, 98.256)
(5665, 98)
(5666, 97.108)
(5667, 92.948)
(5668, 98.2)
(5669, 93.772)
(5670, 95.246)
(5671, 96.082)
(5672, 99.14)
(5673, 97.762)
(5674, 98.428)
(5675, 97.616)
(5676, 97.008)
(5677, 86.328)
(5678, 98.19)
(5679, 98.46)
(5680, 98.498)
(5681, 95.076)
(5682, 98.338)
(5683, 92.544)
(5684, 96.6)
(5685, 95.838)
(5686, 95.608)
(5687, 98.184)
(5688, 98.366)
(5689, 95.24)
(5690, 93.288)
(5691, 93.78)
(5692, 96.24)
(5693, 93.142)
(5694, 95.11)
(5695, 93.382)
(5696, 98.65)
(5697, 97.412)
(5698, 98.078)
(5699, 96.918)
(5700, 98.51)
(5701, 98.404)
(5702, 96.9)
(5703, 96.4)
(5704, 99.026)
(5705, 99.156)
(5706, 99.036)
(5707, 98.688)
(5708, 97.628)
(5709, 99.308)
(5710, 98.944)
(5711, 98.276)
(5712, 96.688)
(5713, 99.144)
(5714, 98.09)
(5715, 99.486)
(5716, 99.734)
(5717, 98.096)
(5718, 99.452)
(5719, 98.66)
(5720, 99.094)
(5721, 98.736)
(5722, 98.804)
(5723, 99.04)
(5724, 99.506)
(5725, 99.22)
(5726, 99.614)
(5727, 98.34)
(5728, 99.34)
(5729, 99.71)
(5730, 99.456)
(5731, 99.508)
(5732, 99.226)
(5733, 99.376)
(5734, 99.046)
(5735, 95.006)
(5736, 99.028)
(5737, 98.852)
(5738, 99.188)
(5739, 98.29)
(5740, 98.008)
(5741, 99.24)
(5742, 99.748)
(5743, 99.114)
(5744, 97.446)
(5745, 99.044)
(5746, 99.314)
(5747, 99.322)
(5748, 99.456)
(5749, 99.324)
(5750, 99.816)
(5751, 98.904)
(5752, 97.416)
(5753, 99.67)
(5754, 99.734)
(5755, 99.666)
(5756, 99.732)
(5757, 99.292)
(5758, 99.81)
(5759, 99.764)
(5760, 99.48)
(5761, 99.832)
(5762, 99.57)
(5763, 99.63)
(5764, 99.578)
(5765, 99.192)
(5766, 99.288)
(5767, 99.394)
(5768, 99.318)
(5769, 99.554)
(5770, 99.372)
(5771, 99.202)
(5772, 98.66)
(5773, 97.248)
(5774, 95.814)
(5775, 95.972)
(5776, 97.506)
(5777, 96.412)
(5778, 96.792)
(5779, 98.414)
(5780, 99.056)
(5781, 98.234)
(5782, 98.138)
(5783, 97.99)
(5784, 98.998)
(5785, 98.536)
(5786, 97.888)
(5787, 97.306)
(5788, 96.47)
(5789, 97.656)
(5790, 98.222)
(5791, 98.244)
(5792, 98.232)
(5793, 98.462)
(5794, 99.2)
(5795, 99.396)
(5796, 99.538)
(5797, 99.414)
(5798, 99.436)
(5799, 98.856)
(5800, 99.024)
(5801, 99.464)
(5802, 99.602)
(5803, 99.864)
(5804, 99.374)
(5805, 99.838)
(5806, 99.528)
(5807, 99.964)
(5808, 99.878)
(5809, 99.488)
(5810, 99.83)
(5811, 99.504)
(5812, 99.322)
(5813, 99.818)
(5814, 99.602)
(5815, 99.15)
(5816, 99.638)
(5817, 99.828)
(5818, 99.734)
(5819, 98.472)
(5820, 98.604)
(5821, 99.478)
(5822, 98.982)
(5823, 99.282)
(5824, 99.488)
(5825, 99.57)
(5826, 99.6)
(5827, 99.402)
(5828, 99.682)
(5829, 99.514)
(5830, 99.636)
(5831, 99.856)
(5832, 99.128)
(5833, 99.196)
(5834, 99.718)
(5835, 98.634)
(5836, 99.298)
(5837, 99.564)
(5838, 99.492)
(5839, 99.552)
(5840, 99.786)
(5841, 99.672)
(5842, 98.884)
(5843, 99.218)
(5844, 99.792)
(5845, 99.92)
(5846, 99.836)
(5847, 99.818)
(5848, 99.76)
(5849, 99.34)
(5850, 99.186)
(5851, 99.884)
(5852, 99.302)
(5853, 99.704)
(5854, 99.77)
(5855, 99.592)
(5856, 98.948)
(5857, 98.956)
(5858, 95.606)
(5859, 99.456)
(5860, 99.686)
(5861, 99.708)
(5862, 99.496)
(5863, 99.886)
(5864, 99.796)
(5865, 99.748)
(5866, 99.538)
(5867, 98.33)
(5868, 99.272)
(5869, 96.89)
(5870, 99.49)
(5871, 99.776)
(5872, 99.674)
(5873, 99.906)
(5874, 99.65)
(5875, 99.97)
(5876, 99.386)
(5877, 99.844)
(5878, 99.656)
(5879, 97.132)
(5880, 99.886)
(5881, 99.942)
(5882, 99.894)
(5883, 99.794)
(5884, 99.492)
(5885, 99.764)
(5886, 99.602)
(5887, 99.876)
(5888, 99.664)
(5889, 99.674)
(5890, 99.406)
(5891, 99.548)
(5892, 99.792)
(5893, 99.502)
(5894, 99.868)
(5895, 99.578)
(5896, 99.846)
(5897, 99.626)
(5898, 99.376)
(5899, 98.488)
(5900, 99.748)
(5901, 99.696)
(5902, 99.416)
(5903, 99.576)
(5904, 98.828)
(5905, 99.716)
(5906, 99.474)
(5907, 99.142)
(5908, 99.772)
(5909, 99.5)
(5910, 99.792)
(5911, 99.808)
(5912, 99.82)
(5913, 99.702)
(5914, 99.746)
(5915, 98.972)
(5916, 99.75)
(5917, 99.09)
(5918, 99.498)
(5919, 99.532)
(5920, 99.556)
(5921, 99.616)
(5922, 99.796)
(5923, 99.612)
(5924, 99.482)
(5925, 99.79)
(5926, 99.866)
(5927, 99.486)
(5928, 99.744)
(5929, 99.88)
(5930, 99.784)
(5931, 98.578)
(5932, 99.892)
(5933, 99.942)
(5934, 99.996)
(5935, 99.95)
(5936, 99.922)
(5937, 99.976)
(5938, 100)
(5939, 99.54)
(5940, 99.978)
(5941, 99.932)
(5942, 99.756)
(5943, 99.954)
(5944, 99.79)
(5945, 99.994)
(5946, 99.922)
(5947, 99.986)
(5948, 100)
(5949, 99.992)
(5950, 99.896)
(5951, 99.972)
(5952, 99.974)
(5953, 99.628)
(5954, 99.988)
(5955, 99.952)
(5956, 99.976)
(5957, 99.994)
(5958, 99.992)
(5959, 99.99)
(5960, 100)
(5961, 99.998)
(5962, 99.954)
(5963, 99.996)
(5964, 99.994)
(5965, 99.886)
(5966, 99.996)
(5967, 100)
(5968, 100)
(5969, 100)
(5970, 100)
(5971, 100)
(5972, 100)
(5973, 100)
(5974, 99.998)
(5975, 100)
(5976, 100)
(5977, 100)
(5978, 100)
(5979, 100)
(5980, 100)
(5981, 100)
(5982, 100)
(5983, 100)
(5984, 100)
(5985, 100)
(5986, 100)
(5987, 100)
(5988, 99.98)
(5989, 99.772)
(5990, 92.124)
(5991, 99.998)
(5992, 99.994)
(5993, 100)
(5994, 99.99)
(5995, 99.98)
(5996, 99.992)
(5997, 99.928)
(5998, 99.876)
(5999, 99.962)
(6000, 99.958)
(6001, 99.972)
(6002, 99.86)
(6003, 99.062)
(6004, 100)
(6005, 99.994)
(6006, 100)
(6007, 99.998)
(6008, 99.99)
(6009, 99.972)
(6010, 99.988)
(6011, 99.956)
(6012, 99.83)
(6013, 99.958)
(6014, 100)
(6015, 99.99)
(6016, 99.966)
(6017, 99.96)
(6018, 99.99)
(6019, 99.966)
(6020, 99.982)
(6021, 99.998)
(6022, 99.988)
(6023, 99.99)
(6024, 99.774)
(6025, 99.974)
(6026, 100)
(6027, 99.998)
(6028, 99.574)
(6029, 99.95)
(6030, 99.7)
(6031, 98.956)
(6032, 99.792)
(6033, 99.842)
(6034, 99.938)
(6035, 99.88)
(6036, 99.946)
(6037, 99.372)
(6038, 99.238)
(6039, 99.956)
(6040, 99.79)
(6041, 99.85)
(6042, 99.954)
(6043, 99.972)
(6044, 99.986)
(6045, 99.994)
(6046, 99.764)
(6047, 99.998)
(6048, 99.998)
(6049, 99.998)
(6050, 99.992)
(6051, 99.976)
(6052, 99.916)
(6053, 99.588)
(6054, 99.916)
(6055, 99.758)
(6056, 99.942)
(6057, 99.94)
(6058, 99.998)
(6059, 99.822)
(6060, 99.94)
(6061, 99.984)
(6062, 99.99)
(6063, 99.988)
(6064, 99.986)
(6065, 99.83)
(6066, 99.974)
(6067, 99.824)
(6068, 99.858)
(6069, 98.84)
(6070, 99.712)
(6071, 99.882)
(6072, 99.892)
(6073, 99.968)
(6074, 99.822)
(6075, 99.862)
(6076, 99.868)
(6077, 99.928)
(6078, 99.774)
(6079, 99.806)
(6080, 99.624)
(6081, 99.488)
(6082, 99.99)
(6083, 99.966)
(6084, 99.902)
(6085, 99.918)
(6086, 98.534)
(6087, 99.73)
(6088, 99.372)
(6089, 99.606)
(6090, 99.206)
(6091, 99.442)
(6092, 99.75)
(6093, 99.38)
(6094, 99.816)
(6095, 99.626)
(6096, 99.278)
(6097, 99.922)
(6098, 99.694)
(6099, 99.848)
(6100, 98.066)
(6101, 99.152)
(6102, 97.05)
(6103, 99.852)
(6104, 99.43)
(6105, 99.764)
(6106, 99.812)
(6107, 99.962)
(6108, 99.73)
(6109, 99.92)
(6110, 99.814)
(6111, 99.334)
(6112, 99.848)
(6113, 99.794)
(6114, 99.81)
(6115, 99.32)
(6116, 99.29)
(6117, 99.74)
(6118, 99.008)
(6119, 99.74)
(6120, 99.062)
(6121, 99.246)
(6122, 99.526)
(6123, 99.794)
(6124, 99.706)
(6125, 99.77)
(6126, 99.686)
(6127, 99.816)
(6128, 99.956)
(6129, 99.986)
(6130, 99.96)
(6131, 99.9)
(6132, 99.982)
(6133, 99.964)
(6134, 99.864)
(6135, 99.942)
(6136, 99.96)
(6137, 99.926)
(6138, 99.962)
(6139, 99.8)
(6140, 99.852)
(6141, 99.958)
(6142, 99.918)
(6143, 99.974)
(6144, 99.978)
(6145, 99.972)
(6146, 99.822)
(6147, 99.232)
(6148, 98.41)
(6149, 98.73)
(6150, 99.92)
(6151, 99.788)
(6152, 99.734)
(6153, 99.854)
(6154, 99.918)
(6155, 99.492)
(6156, 99.108)
(6157, 99.284)
(6158, 99.18)
(6159, 99.878)
(6160, 99.694)
(6161, 99.66)
(6162, 99.516)
(6163, 99.334)
(6164, 99.756)
(6165, 99.49)
(6166, 99.72)
(6167, 99.894)
(6168, 99.944)
(6169, 99.928)
(6170, 99.758)
(6171, 99.82)
(6172, 99.848)
(6173, 99.712)
(6174, 99.8)
(6175, 99.724)
(6176, 99.59)
(6177, 99.6)
(6178, 99.796)
(6179, 99.638)
(6180, 99.57)
(6181, 98.902)
(6182, 99.848)
(6183, 99.784)
(6184, 99.828)
(6185, 99.498)
(6186, 99.788)
(6187, 96.918)
(6188, 99.56)
(6189, 99.868)
(6190, 99.696)
(6191, 99.724)
(6192, 99.718)
(6193, 99.99)
(6194, 99.948)
(6195, 99.152)
(6196, 99.822)
(6197, 99.99)
(6198, 99.964)
(6199, 99.912)
(6200, 99.938)
(6201, 99.674)
(6202, 99.606)
(6203, 93.854)
(6204, 99.816)
(6205, 99.9)
(6206, 93.644)
(6207, 99.974)
(6208, 99.972)
(6209, 99.94)
(6210, 99.928)
(6211, 99.444)
(6212, 99.8)
(6213, 99.484)
(6214, 99.846)
(6215, 99.998)
(6216, 99.946)
(6217, 99.67)
(6218, 99.848)
(6219, 98.174)
(6220, 99.902)
(6221, 99.946)
(6222, 99.964)
(6223, 99.844)
(6224, 99.63)
(6225, 99.8)
(6226, 99.612)
(6227, 99.924)
(6228, 99.954)
(6229, 99.876)
(6230, 99.822)
(6231, 99.708)
(6232, 99.818)
(6233, 99.582)
(6234, 99.898)
(6235, 99.24)
(6236, 99.826)
(6237, 98.944)
(6238, 99.964)
(6239, 99.938)
(6240, 99.832)
(6241, 99.854)
(6242, 98.204)
(6243, 99.492)
(6244, 99.542)
(6245, 98.68)
(6246, 99.088)
(6247, 98.42)
(6248, 98.152)
(6249, 99.434)
(6250, 98.422)
(6251, 98.526)
(6252, 99.494)
(6253, 97.904)
(6254, 99.516)
(6255, 99.846)
(6256, 99.88)
(6257, 99.126)
(6258, 99.064)
(6259, 99.47)
(6260, 99.702)
(6261, 99.708)
(6262, 99.436)
(6263, 99.922)
(6264, 99.946)
(6265, 98.76)
(6266, 99.612)
(6267, 99.788)
(6268, 99.824)
(6269, 99.802)
(6270, 99.776)
(6271, 99.856)
(6272, 99.632)
(6273, 99.76)
(6274, 99.62)
(6275, 99.604)
(6276, 98.306)
(6277, 99.532)
(6278, 99.662)
(6279, 99.852)
(6280, 99.03)
(6281, 99.85)
(6282, 99.622)
(6283, 97.47)
(6284, 99.378)
(6285, 99.26)
(6286, 98.65)
(6287, 97.378)
(6288, 99.702)
(6289, 99.872)
(6290, 98.746)
(6291, 99.894)
(6292, 99.634)
(6293, 98.346)
(6294, 99.936)
(6295, 99.802)
(6296, 99.518)
(6297, 99.86)
(6298, 99.524)
(6299, 99.622)
(6300, 99.842)
(6301, 99.298)
(6302, 99.824)
(6303, 98.612)
(6304, 99.556)
(6305, 99.35)
(6306, 99.854)
(6307, 99.322)
(6308, 99.522)
(6309, 99.764)
(6310, 99.758)
(6311, 99.85)
(6312, 99.748)
(6313, 99.666)
(6314, 98.488)
(6315, 99.664)
(6316, 99.364)
(6317, 99.08)
(6318, 99.444)
(6319, 99.34)
(6320, 99.012)
(6321, 98.786)
(6322, 99.706)
(6323, 99.184)
(6324, 99.164)
(6325, 99.41)
(6326, 99.252)
(6327, 99.294)
(6328, 99.554)
(6329, 99.63)
(6330, 99.328)
(6331, 99.77)
(6332, 99.97)
(6333, 99.414)
(6334, 99.718)
(6335, 99.834)
(6336, 99.668)
(6337, 99.89)
(6338, 99.834)
(6339, 99.826)
(6340, 99.982)
(6341, 99.872)
(6342, 99.95)
(6343, 99.894)
(6344, 99.598)
(6345, 99.51)
(6346, 99.502)
(6347, 97.904)
(6348, 98.71)
(6349, 99.772)
(6350, 99.49)
(6351, 99.568)
(6352, 99.71)
(6353, 99.478)
(6354, 99.788)
(6355, 99.618)
(6356, 96.408)
(6357, 99.66)
(6358, 99.85)
(6359, 99.496)
(6360, 99.388)
(6361, 98.924)
(6362, 99.662)
(6363, 99.84)
(6364, 99.604)
(6365, 99.622)
(6366, 99.97)
(6367, 99.846)
(6368, 98.25)
(6369, 94.886)
(6370, 95.912)
(6371, 99.986)
(6372, 99.976)
(6373, 99.978)
(6374, 99.95)
(6375, 99.79)
(6376, 99.992)
(6377, 99.988)
(6378, 99.956)
(6379, 99.978)
(6380, 99.98)
(6381, 99.958)
(6382, 99.936)
(6383, 99.84)
(6384, 99.442)
(6385, 99.956)
(6386, 99.934)
(6387, 99.28)
(6388, 99.828)
(6389, 99.574)
(6390, 99.374)
(6391, 98.672)
(6392, 99.13)
(6393, 99.304)
(6394, 93.546)
(6395, 97.846)
(6396, 98.892)
(6397, 96.92)
(6398, 99.75)
(6399, 98.532)
(6400, 99.436)
(6401, 98.74)
(6402, 98.45)
(6403, 98.964)
(6404, 98.482)
(6405, 97.352)
(6406, 98.872)
(6407, 99.32)
(6408, 99.384)
(6409, 97.994)
(6410, 92.358)
(6411, 98.198)
(6412, 98.336)
(6413, 96.81)
(6414, 98.358)
(6415, 94.398)
(6416, 96.874)
(6417, 98.85)
(6418, 98.972)
(6419, 96.93)
(6420, 98.602)
(6421, 98.854)
(6422, 98.674)
(6423, 99.044)
(6424, 99.018)
(6425, 97.268)
(6426, 98.91)
(6427, 97.962)
(6428, 95.94)
(6429, 97.836)
(6430, 97.862)
(6431, 96.71)
(6432, 97.186)
(6433, 97.216)
(6434, 99.42)
(6435, 97.708)
(6436, 95.372)
(6437, 97.448)
(6438, 99.372)
(6439, 98.238)
(6440, 98.166)
(6441, 98.436)
(6442, 98.81)
(6443, 98.026)
(6444, 97.752)
(6445, 96.596)
(6446, 95.768)
(6447, 97.864)
(6448, 98.902)
(6449, 97.346)
(6450, 98.154)
(6451, 98.61)
(6452, 98.242)
(6453, 97.624)
(6454, 98.27)
(6455, 97.56)
(6456, 96.938)
(6457, 96.754)
(6458, 95.578)
(6459, 96.288)
(6460, 96.186)
(6461, 94.15)
(6462, 96.502)
(6463, 98.398)
(6464, 99.582)
(6465, 98.18)
(6466, 97.95)
(6467, 98.34)
(6468, 98.906)
(6469, 98.696)
(6470, 98.666)
(6471, 95.794)
(6472, 98.602)
(6473, 98.39)
(6474, 97.926)
(6475, 96.55)
(6476, 98.818)
(6477, 97.052)
(6478, 98.428)
(6479, 99.034)
(6480, 97.93)
(6481, 98.17)
(6482, 98.056)
(6483, 98.328)
(6484, 97.882)
(6485, 99.148)
(6486, 98.114)
(6487, 98.166)
(6488, 98.326)
(6489, 99.102)
(6490, 99.19)
(6491, 97.648)
(6492, 98.762)
(6493, 99.154)
(6494, 99.718)
(6495, 98.838)
(6496, 98.842)
(6497, 99.622)
(6498, 99.444)
(6499, 99.488)
(6500, 99.784)
(6501, 99.418)
(6502, 99.388)
(6503, 98.486)
(6504, 99.396)
(6505, 99.552)
(6506, 99.104)
(6507, 98.272)
(6508, 96.97)
(6509, 99.412)
(6510, 98.734)
(6511, 99.458)
(6512, 99.39)
(6513, 97.972)
(6514, 98.434)
(6515, 98.68)
(6516, 98.706)
(6517, 98.27)
(6518, 98.86)
(6519, 99.018)
(6520, 99.304)
(6521, 99.426)
(6522, 98.088)
(6523, 99.408)
(6524, 99.53)
(6525, 99.526)
(6526, 99.616)
(6527, 99.558)
(6528, 99.692)
(6529, 99.308)
(6530, 99.666)
(6531, 99.56)
(6532, 99.732)
(6533, 99.778)
(6534, 99.71)
(6535, 99.224)
(6536, 89.13)
(6537, 97.678)
(6538, 96.496)
(6539, 97.238)
(6540, 97.594)
(6541, 95.99)
(6542, 97.654)
(6543, 98.256)
(6544, 98.316)
(6545, 98.57)
(6546, 99.42)
(6547, 97.642)
(6548, 98.918)
(6549, 98.258)
(6550, 95.266)
(6551, 99.598)
(6552, 99.074)
(6553, 99.698)
(6554, 95.782)
(6555, 98.678)
(6556, 98.906)
(6557, 98.498)
(6558, 98.076)
(6559, 99.624)
(6560, 96.828)
(6561, 98.592)
(6562, 97.532)
(6563, 99.086)
(6564, 99.778)
(6565, 99.506)
(6566, 98.182)
(6567, 98.956)
(6568, 99.548)
(6569, 99.65)
(6570, 99.914)
(6571, 99.732)
(6572, 99.77)
(6573, 99.808)
(6574, 99.888)
(6575, 99.812)
(6576, 99.728)
(6577, 96.31)
(6578, 99.838)
(6579, 99.764)
(6580, 99.65)
(6581, 96.044)
(6582, 99.682)
(6583, 97.728)
(6584, 92.956)
(6585, 98.912)
(6586, 99.11)
(6587, 95.92)
(6588, 97.15)
(6589, 99.408)
(6590, 99.37)
(6591, 98.962)
(6592, 99.75)
(6593, 99.222)
(6594, 99.62)
(6595, 99.556)
(6596, 98.96)
(6597, 99.616)
(6598, 99.87)
(6599, 98.356)
(6600, 98.858)
(6601, 99.132)
(6602, 98.004)
(6603, 98.43)
(6604, 99.238)
(6605, 99.24)
(6606, 99.728)
(6607, 99.648)
(6608, 97.216)
(6609, 99.514)
(6610, 99.534)
(6611, 99.876)
(6612, 99.926)
(6613, 99.862)
(6614, 99.588)
(6615, 99.212)
(6616, 98)
(6617, 99.7)
(6618, 99.66)
(6619, 99.83)
(6620, 99.778)
(6621, 99.756)
(6622, 99.926)
(6623, 99.896)
(6624, 99.47)
(6625, 99.148)
(6626, 99.546)
(6627, 99.748)
(6628, 99.572)
(6629, 98.892)
(6630, 99.702)
(6631, 99.706)
(6632, 99.78)
(6633, 99.262)
(6634, 99.704)
(6635, 99.764)
(6636, 99.5)
(6637, 99.892)
(6638, 99.938)
(6639, 99.978)
(6640, 99.826)
(6641, 99.622)
(6642, 99.296)
(6643, 99.04)
(6644, 99.172)
(6645, 99.736)
(6646, 99.714)
(6647, 98.958)
(6648, 98.934)
(6649, 99.85)
(6650, 99.648)
(6651, 99.846)
(6652, 99.82)
(6653, 99.738)
(6654, 98.486)
(6655, 98.052)
(6656, 99.212)
(6657, 99.784)
(6658, 98.282)
(6659, 98.718)
(6660, 99.238)
(6661, 99.094)
(6662, 99.36)
(6663, 99.034)
(6664, 98.618)
(6665, 99.496)
(6666, 99.336)
(6667, 98.706)
(6668, 99.366)
(6669, 99.398)
(6670, 99.036)
(6671, 99.438)
(6672, 99.494)
(6673, 98.204)
(6674, 98.992)
(6675, 99.028)
(6676, 99.414)
(6677, 98.686)
(6678, 99.562)
(6679, 99.67)
(6680, 99.828)
(6681, 99.342)
(6682, 99.95)
(6683, 99.962)
(6684, 99.476)
(6685, 99.818)
(6686, 99.58)
(6687, 99.908)
(6688, 99.976)
(6689, 99.858)
(6690, 99.9)
(6691, 99.884)
(6692, 99.978)
(6693, 99.98)
(6694, 99.844)
(6695, 99.864)
(6696, 99.926)
(6697, 99.932)
(6698, 99.882)
(6699, 98.684)
(6700, 99.25)
(6701, 99.724)
(6702, 99.474)
(6703, 99.268)
(6704, 99.934)
(6705, 98.778)
(6706, 97.954)
(6707, 98.506)
(6708, 99.306)
(6709, 98.686)
(6710, 98.146)
(6711, 98.642)
(6712, 98.002)
(6713, 96.052)
(6714, 99.53)
(6715, 98.778)
(6716, 99.132)
(6717, 99.634)
(6718, 99.946)
(6719, 99.92)
(6720, 99.954)
(6721, 99.84)
(6722, 99.94)
(6723, 99.852)
(6724, 99.886)
(6725, 99.86)
(6726, 99.928)
(6727, 99.266)
(6728, 98.464)
(6729, 98.842)
(6730, 99.914)
(6731, 99.948)
(6732, 99.77)
(6733, 99.94)
(6734, 99.72)
(6735, 96.528)
(6736, 98.45)
(6737, 96.046)
(6738, 99.284)
(6739, 99.19)
(6740, 99.018)
(6741, 99.612)
(6742, 98.726)
(6743, 99.764)
(6744, 99.772)
(6745, 99.748)
(6746, 99.54)
(6747, 99.684)
(6748, 99.496)
(6749, 99.616)
(6750, 99.808)
(6751, 99.904)
(6752, 99.794)
(6753, 99.94)
(6754, 99.724)
(6755, 99.778)
(6756, 99.77)
(6757, 99.82)
(6758, 99.85)
(6759, 99.542)
(6760, 99.766)
(6761, 99.568)
(6762, 99.92)
(6763, 99.782)
(6764, 99.894)
(6765, 99.972)
(6766, 99.948)
(6767, 99.876)
(6768, 99.522)
(6769, 99.528)
(6770, 99.58)
(6771, 99.614)
(6772, 99.272)
(6773, 99.216)
(6774, 99.874)
(6775, 99.574)
(6776, 98.382)
(6777, 99.878)
(6778, 98.042)
(6779, 99.496)
(6780, 96.54)
(6781, 98.764)
(6782, 99.748)
(6783, 98.088)
(6784, 99.884)
(6785, 99.744)
(6786, 99.36)
(6787, 99.37)
(6788, 99.694)
(6789, 99.702)
(6790, 99.57)
(6791, 99.672)
(6792, 99.372)
(6793, 98.704)
(6794, 98.454)
(6795, 98.948)
(6796, 98.16)
(6797, 98.706)
(6798, 99.646)
(6799, 99.616)
(6800, 99.498)
(6801, 99.612)
(6802, 99.828)
(6803, 98.468)
(6804, 99.402)
(6805, 99.962)
(6806, 99.896)
(6807, 99.196)
(6808, 98.826)
(6809, 99.61)
(6810, 99.846)
(6811, 98.652)
(6812, 99.676)
(6813, 99.464)
(6814, 99.68)
(6815, 99.614)
(6816, 99.952)
(6817, 99.934)
(6818, 99.976)
(6819, 99.988)
(6820, 99.962)
(6821, 99.99)
(6822, 99.996)
(6823, 99.988)
(6824, 99.788)
(6825, 99.988)
(6826, 99.812)
(6827, 99.986)
(6828, 99.996)
(6829, 100)
(6830, 99.984)
(6831, 99.996)
(6832, 100)
(6833, 99.992)
(6834, 99.902)
(6835, 100)
(6836, 100)
(6837, 100)
(6838, 99.922)
(6839, 99.996)
(6840, 100)
(6841, 100)
(6842, 99.956)
(6843, 99.998)
(6844, 97.08)
(6845, 100)
(6846, 99.99)
(6847, 99.966)
(6848, 99.958)
(6849, 100)
(6850, 99.992)
(6851, 99.954)
(6852, 99.652)
(6853, 99.91)
(6854, 99.998)
(6855, 99.998)
(6856, 99.998)
(6857, 99.992)
(6858, 99.984)
(6859, 100)
(6860, 100)
(6861, 99.806)
(6862, 99.94)
(6863, 99.998)
(6864, 99.97)
(6865, 99.99)
(6866, 99.998)
(6867, 99.962)
(6868, 100)
(6869, 99.988)
(6870, 99.988)
(6871, 99.996)
(6872, 100)
(6873, 100)
(6874, 100)
(6875, 98.98)
(6876, 99.992)
(6877, 99.988)
(6878, 100)
(6879, 99.984)
(6880, 99.994)
(6881, 100)
(6882, 99.978)
(6883, 99.986)
(6884, 99.916)
(6885, 99.962)
(6886, 99.978)
(6887, 99.96)
(6888, 99.946)
(6889, 99.834)
(6890, 99.932)
(6891, 99.974)
(6892, 99.966)
(6893, 99.972)
(6894, 99.842)
(6895, 99.964)
(6896, 99.97)
(6897, 99.9)
(6898, 99.852)
(6899, 99.946)
(6900, 99.9)
(6901, 99.82)
(6902, 99.84)
(6903, 99.812)
(6904, 99.9)
(6905, 99.834)
(6906, 99.254)
(6907, 99.954)
(6908, 99.88)
(6909, 99.712)
(6910, 99.784)
(6911, 99.61)
(6912, 99.698)
(6913, 99.796)
(6914, 99.628)
(6915, 99.806)
(6916, 99.904)
(6917, 99.738)
(6918, 99.836)
(6919, 99.608)
(6920, 99.876)
(6921, 99.778)
(6922, 99.77)
(6923, 99.91)
(6924, 99.864)
(6925, 99.888)
(6926, 99.92)
(6927, 99.87)
(6928, 99.672)
(6929, 99.94)
(6930, 99.824)
(6931, 99.85)
(6932, 99.666)
(6933, 99.206)
(6934, 99.48)
(6935, 99.8)
(6936, 98.87)
(6937, 98.102)
(6938, 99.332)
(6939, 99.758)
(6940, 99.724)
(6941, 99.642)
(6942, 99.592)
(6943, 99.652)
(6944, 99.702)
(6945, 99.768)
(6946, 99.49)
(6947, 99.754)
(6948, 99.758)
(6949, 99.444)
(6950, 99.758)
(6951, 97.756)
(6952, 99.354)
(6953, 99.052)
(6954, 98.592)
(6955, 97.142)
(6956, 97.782)
(6957, 94.822)
(6958, 96.892)
(6959, 98.002)
(6960, 98.362)
(6961, 98.254)
(6962, 97.154)
(6963, 96.104)
(6964, 98.854)
(6965, 98.602)
(6966, 99.35)
(6967, 99.322)
(6968, 99.338)
(6969, 99.11)
(6970, 98.566)
(6971, 98.026)
(6972, 98.242)
(6973, 98.306)
(6974, 98.174)
(6975, 98.102)
(6976, 99.048)
(6977, 98.108)
(6978, 95.012)
(6979, 96.538)
(6980, 98.892)
(6981, 98.016)
(6982, 98.472)
(6983, 98.21)
(6984, 97.434)
(6985, 97.682)
(6986, 96.48)
(6987, 96.818)
(6988, 97.092)
(6989, 98.538)
(6990, 96.114)
(6991, 97.132)
(6992, 96.29)
(6993, 98.868)
(6994, 99.176)
(6995, 98.7)
(6996, 96.988)
(6997, 98.236)
(6998, 98.636)
(6999, 96.348)
(7000, 96.784)
(7001, 98.814)
(7002, 98.304)
(7003, 98.046)
(7004, 98.634)
(7005, 98.29)
(7006, 98.116)
(7007, 94.674)
(7008, 97.32)
(7009, 98.464)
(7010, 97.654)
(7011, 99.172)
(7012, 98.016)
(7013, 97.692)
(7014, 98.102)
(7015, 97.74)
(7016, 98.718)
(7017, 97.726)
(7018, 98.026)
(7019, 96.636)
(7020, 98.498)
(7021, 97.814)
(7022, 98.092)
(7023, 96.15)
(7024, 96.968)
(7025, 97.652)
(7026, 97.412)
(7027, 97.726)
(7028, 92.286)
(7029, 94.264)
(7030, 97.788)
(7031, 93.974)
(7032, 95.402)
(7033, 96.606)
(7034, 97.666)
(7035, 95.194)
(7036, 92.806)
(7037, 93.842)
(7038, 94.32)
(7039, 88.892)
(7040, 81.132)
(7041, 91.926)
(7042, 86.622)
(7043, 81.644)
(7044, 85.94)
(7045, 88.686)
(7046, 91.882)
(7047, 92.272)
(7048, 95.32)
(7049, 95.334)
(7050, 91.838)
(7051, 94.2)
(7052, 89.052)
(7053, 94.84)
(7054, 90.908)
(7055, 94.884)
(7056, 91.738)
(7057, 96.12)
(7058, 93.554)
(7059, 92.004)
(7060, 95.492)
(7061, 95.01)
(7062, 92.382)
(7063, 93.004)
(7064, 87.102)
(7065, 80.492)
(7066, 87.142)
(7067, 90.396)
(7068, 85.024)
(7069, 96.088)
(7070, 92.366)
(7071, 90.218)
(7072, 83.438)
(7073, 90.47)
(7074, 94.276)
(7075, 91.212)
(7076, 97.536)
(7077, 94.076)
(7078, 91.12)
(7079, 93.174)
(7080, 94.232)
(7081, 91.042)
(7082, 97.604)
(7083, 96.54)
(7084, 90.472)
(7085, 93.88)
(7086, 86.678)
(7087, 95.752)
(7088, 96.104)
(7089, 93.568)
(7090, 92.516)
(7091, 93.95)
(7092, 92.218)
(7093, 91.502)
(7094, 90.156)
(7095, 86.644)
(7096, 91.444)
(7097, 92.4)
(7098, 90.364)
(7099, 83.024)
(7100, 91.814)
(7101, 95.342)
(7102, 94.634)
(7103, 96.194)
(7104, 87.786)
(7105, 93.188)
(7106, 95.102)
(7107, 94.79)
(7108, 80.67)
(7109, 88.208)
(7110, 95.936)
(7111, 88.782)
(7112, 94.298)
(7113, 89.88)
(7114, 90.19)
(7115, 84.668)
(7116, 82.374)
(7117, 94.994)
(7118, 89.464)
(7119, 92.972)
(7120, 92.562)
(7121, 93.204)
(7122, 88.974)
(7123, 97.744)
(7124, 96.154)
(7125, 95.918)
(7126, 94.648)
(7127, 94.15)
(7128, 90.07)
(7129, 92.422)
(7130, 86.1)
(7131, 91.054)
(7132, 88.262)
(7133, 89.984)
(7134, 89.678)
(7135, 96.93)
(7136, 90.41)
(7137, 93.318)
(7138, 86.328)
(7139, 93.38)
(7140, 94.69)
(7141, 95.41)
(7142, 95.638)
(7143, 90.734)
(7144, 92.522)
(7145, 97.948)
(7146, 97.926)
(7147, 94.256)
(7148, 95.57)
(7149, 96.098)
(7150, 98.194)
(7151, 96.09)
(7152, 96.968)
(7153, 96.722)
(7154, 97.804)
(7155, 97.636)
(7156, 97.658)
(7157, 98.19)
(7158, 97.37)
(7159, 99.154)
(7160, 99.378)
(7161, 99.55)
(7162, 99.29)
(7163, 98.448)
(7164, 99.226)
(7165, 99.45)
(7166, 97.194)
(7167, 98.488)
(7168, 98.136)
(7169, 95.014)
(7170, 97.984)
(7171, 95.228)
(7172, 91.784)
(7173, 97.156)
(7174, 97.032)
(7175, 97.204)
(7176, 96.134)
(7177, 94.868)
(7178, 96.522)
(7179, 97.566)
(7180, 99.312)
(7181, 98.75)
(7182, 97.634)
(7183, 97.274)
(7184, 97.49)
(7185, 93.542)
(7186, 96.486)
(7187, 94.84)
(7188, 96.92)
(7189, 95.792)
(7190, 96.444)
(7191, 99.172)
(7192, 96.502)
(7193, 96.484)
(7194, 95.852)
(7195, 98.4)
(7196, 97.37)
(7197, 98.462)
(7198, 96.52)
(7199, 97.168)
(7200, 93.402)
(7201, 97.448)
(7202, 96.59)
(7203, 87.25)
(7204, 96.28)
(7205, 95.47)
(7206, 97.486)
(7207, 97.508)
(7208, 95.312)
(7209, 96.052)
(7210, 90.626)
(7211, 85.028)
(7212, 94.652)
(7213, 96.704)
(7214, 98.898)
(7215, 96.074)
(7216, 98.028)
(7217, 94.718)
(7218, 94.828)
(7219, 98.624)
(7220, 98.168)
(7221, 98.618)
(7222, 97.122)
(7223, 97.624)
(7224, 98.464)
(7225, 98.18)
(7226, 92.608)
(7227, 93.518)
(7228, 90.356)
(7229, 93.914)
(7230, 88.652)
(7231, 96.908)
(7232, 92.09)
(7233, 97.62)
(7234, 89.248)
(7235, 78.944)
(7236, 92.386)
(7237, 92.84)
(7238, 88.414)
(7239, 85.758)
(7240, 73.704)
(7241, 91.318)
(7242, 99.478)
(7243, 99.71)
(7244, 99.844)
(7245, 99.194)
(7246, 95.278)
(7247, 99.176)
(7248, 99.314)
(7249, 98.314)
(7250, 98.966)
(7251, 95.738)
(7252, 97.728)
(7253, 96.484)
(7254, 97.936)
(7255, 96.766)
(7256, 96.538)
(7257, 99.388)
(7258, 99.898)
(7259, 99.882)
(7260, 99.93)
(7261, 99.842)
(7262, 99.856)
(7263, 99.856)
(7264, 99.82)
(7265, 99.81)
(7266, 99.36)
(7267, 99.634)
(7268, 99.074)
(7269, 98.18)
(7270, 99.362)
(7271, 99.01)
(7272, 98.456)
(7273, 98.48)
(7274, 99.05)
(7275, 98.682)
(7276, 99.256)
(7277, 99.484)
(7278, 98.918)
(7279, 99.402)
(7280, 98.956)
(7281, 96.61)
(7282, 97.592)
(7283, 98.268)
(7284, 99.032)
(7285, 98.288)
(7286, 98.916)
(7287, 99.046)
(7288, 96.024)
(7289, 98.29)
(7290, 98.674)
(7291, 99.614)
(7292, 99.898)
(7293, 99.428)
(7294, 98.47)
(7295, 99.422)
(7296, 99.786)
(7297, 99.844)
(7298, 99.954)
(7299, 99.946)
(7300, 98.994)
(7301, 97.964)
(7302, 99.592)
(7303, 99.874)
(7304, 99.772)
(7305, 99.82)
(7306, 99.744)
(7307, 98.49)
(7308, 99.576)
(7309, 99.776)
(7310, 99.68)
(7311, 99.724)
(7312, 99.942)
(7313, 99.89)
(7314, 99.18)
(7315, 97.466)
(7316, 98.788)
(7317, 99.39)
(7318, 98.898)
(7319, 99.194)
(7320, 99.282)
(7321, 98.478)
(7322, 99.48)
(7323, 99.662)
(7324, 99.856)
(7325, 99.872)
(7326, 99.844)
(7327, 99.864)
(7328, 98.736)
(7329, 96.782)
(7330, 98.776)
(7331, 99.456)
(7332, 99.522)
(7333, 99.402)
(7334, 99.78)
(7335, 99.208)
(7336, 98.634)
(7337, 98.532)
(7338, 98.944)
(7339, 99.676)
(7340, 99.858)
(7341, 99.394)
(7342, 97.662)
(7343, 98.45)
(7344, 99.192)
(7345, 98.302)
(7346, 97.304)
(7347, 98.876)
(7348, 99.012)
(7349, 98.476)
(7350, 98.04)
(7351, 98.504)
(7352, 97.072)
(7353, 98.72)
(7354, 98.32)
(7355, 96.154)
(7356, 96.898)
(7357, 98.392)
(7358, 95.184)
(7359, 96.474)
(7360, 97.22)
(7361, 95.332)
(7362, 98.956)
(7363, 98.314)
(7364, 98.544)
(7365, 98.65)
(7366, 97.62)
(7367, 95.522)
(7368, 97.378)
(7369, 92.85)
(7370, 92.862)
(7371, 94.252)
(7372, 96.454)
(7373, 96.752)
(7374, 96.86)
(7375, 96.482)
(7376, 94.978)
(7377, 96.124)
(7378, 97.162)
(7379, 96.684)
(7380, 95.934)
(7381, 96.636)
(7382, 96.326)
(7383, 95.63)
(7384, 96.608)
(7385, 95.404)
(7386, 91.164)
(7387, 96.248)
(7388, 97.952)
(7389, 97.964)
(7390, 95.034)
(7391, 96.4)
(7392, 95.812)
(7393, 93.92)
(7394, 94.652)
(7395, 93.312)
(7396, 96.744)
(7397, 97.36)
(7398, 97.118)
(7399, 89.942)
(7400, 91.752)
(7401, 91.13)
(7402, 92.088)
(7403, 94.088)
(7404, 87.926)
(7405, 87.884)
(7406, 93.258)
(7407, 94.396)
(7408, 95.12)
(7409, 94.714)
(7410, 95.206)
(7411, 97.628)
(7412, 90.708)
(7413, 94.2)
(7414, 94.992)
(7415, 95.75)
(7416, 93.252)
(7417, 97.728)
(7418, 97.104)
(7419, 95.426)
(7420, 96.212)
(7421, 95.962)
(7422, 96.788)
(7423, 96.258)
(7424, 95.008)
(7425, 91.176)
(7426, 92.936)
(7427, 95.702)
(7428, 94.956)
(7429, 91.646)
(7430, 94.84)
(7431, 94.796)
(7432, 94.744)
(7433, 97.576)
(7434, 97.7)
(7435, 97.194)
(7436, 96.204)
(7437, 97.816)
(7438, 97.356)
(7439, 98.428)
(7440, 96.92)
(7441, 95.148)
(7442, 93.638)
(7443, 92.528)
(7444, 91.462)
(7445, 94.314)
(7446, 95.844)
(7447, 97.272)
(7448, 96.316)
(7449, 97.516)
(7450, 98.524)
(7451, 97.192)
(7452, 89.712)
(7453, 94.358)
(7454, 89.816)
(7455, 95.046)
(7456, 94.5)
(7457, 94.438)
(7458, 95.818)
(7459, 92.35)
(7460, 95.276)
(7461, 95.88)
(7462, 92.498)
(7463, 93.632)
(7464, 91.556)
(7465, 92.576)
(7466, 93.716)
(7467, 95.568)
(7468, 96.218)
(7469, 97.176)
(7470, 97.454)
(7471, 93.646)
(7472, 93.926)
(7473, 95.5)
(7474, 92.712)
(7475, 96.17)
(7476, 96.374)
(7477, 97.328)
(7478, 89.878)
(7479, 96.866)
(7480, 96.082)
(7481, 96.964)
(7482, 93.526)
(7483, 96.01)
(7484, 98.272)
(7485, 95.246)
(7486, 82.956)
(7487, 96.78)
(7488, 97.528)
(7489, 96.632)
(7490, 88.904)
(7491, 94.646)
(7492, 88.122)
(7493, 92.64)
(7494, 86.186)
(7495, 95.3)
(7496, 94.34)
(7497, 96.084)
(7498, 96.186)
(7499, 97.916)
(7500, 98.668)
(7501, 97.366)
(7502, 95.716)
(7503, 96.726)
(7504, 99.042)
(7505, 98.062)
(7506, 92.79)
(7507, 97.054)
(7508, 94.968)
(7509, 97.238)
(7510, 88.42)
(7511, 97.324)
(7512, 95.958)
(7513, 86.048)
(7514, 91.586)
(7515, 94.624)
(7516, 92.876)
(7517, 88.072)
(7518, 96.198)
(7519, 95.972)
(7520, 92.444)
(7521, 79.938)
(7522, 87.732)
(7523, 91.644)
(7524, 89.294)
(7525, 85.702)
(7526, 70.172)
(7527, 96.304)
(7528, 99.508)
(7529, 89.81)
(7530, 85.556)
(7531, 99.496)
(7532, 99.894)
(7533, 99.908)
(7534, 99.976)
(7535, 99.944)
(7536, 99.798)
(7537, 99.584)
(7538, 99.414)
(7539, 99.584)
(7540, 97.378)
(7541, 99.262)
(7542, 99.592)
(7543, 99.572)
(7544, 99.31)
(7545, 99.63)
(7546, 99.494)
(7547, 99.672)
(7548, 99.66)
(7549, 99.836)
(7550, 99.948)
(7551, 99.302)
(7552, 98.994)
(7553, 99.172)
(7554, 99.352)
(7555, 99.56)
(7556, 99.32)
(7557, 99.538)
(7558, 99.536)
(7559, 99.292)
(7560, 99.666)
(7561, 99.122)
(7562, 99.134)
(7563, 99.668)
(7564, 99.792)
(7565, 99.794)
(7566, 99.782)
(7567, 99.444)
(7568, 99.742)
(7569, 99.784)
(7570, 99.826)
(7571, 98.026)
(7572, 99.558)
(7573, 99.936)
(7574, 99.994)
(7575, 99.818)
(7576, 99.976)
(7577, 99.628)
(7578, 99.93)
(7579, 99.126)
(7580, 99.804)
(7581, 99.994)
(7582, 99.99)
(7583, 99.972)
(7584, 99.744)
(7585, 99.826)
(7586, 99.442)
(7587, 99.242)
(7588, 99.846)
(7589, 99.828)
(7590, 99.998)
(7591, 100)
(7592, 99.998)
(7593, 100)
(7594, 100)
(7595, 100)
(7596, 99.998)
(7597, 100)
(7598, 100)
(7599, 99.996)
(7600, 99.996)
(7601, 99.996)
(7602, 99.994)
(7603, 99.98)
(7604, 99.99)
(7605, 99.978)
(7606, 99.982)
(7607, 99.95)
(7608, 99.06)
(7609, 99.974)
(7610, 99.926)
(7611, 99.918)
(7612, 99.966)
(7613, 99.566)
(7614, 98.618)
(7615, 99.648)
(7616, 99.706)
(7617, 99.628)
(7618, 99.804)
(7619, 99.874)
(7620, 99.854)
(7621, 96.852)
(7622, 97.56)
(7623, 97.208)
(7624, 99.374)
(7625, 99.668)
(7626, 99.286)
(7627, 99.668)
(7628, 98.976)
(7629, 99.436)
(7630, 99.364)
(7631, 99.896)
(7632, 99.566)
(7633, 98.93)
(7634, 99.604)
(7635, 99.528)
(7636, 94.968)
(7637, 99.422)
(7638, 99.534)
(7639, 99.2)
(7640, 98.746)
(7641, 98.972)
(7642, 98.896)
(7643, 97.56)
(7644, 97.678)
(7645, 98.078)
(7646, 99.048)
(7647, 96.774)
(7648, 97.348)
(7649, 97.912)
(7650, 98.004)
(7651, 98.516)
(7652, 98.764)
(7653, 99.434)
(7654, 97.936)
(7655, 98.008)
(7656, 96.458)
(7657, 98.62)
(7658, 98.19)
(7659, 96.066)
(7660, 98.958)
(7661, 98.094)
(7662, 99.4)
(7663, 99.178)
(7664, 99.568)
(7665, 99.364)
(7666, 99.472)
(7667, 99.596)
(7668, 98.904)
(7669, 99.592)
(7670, 99.368)
(7671, 99.44)
(7672, 99.588)
(7673, 99.378)
(7674, 99.4)
(7675, 99.486)
(7676, 99.794)
(7677, 98.756)
(7678, 98.198)
(7679, 99.116)
(7680, 98.656)
(7681, 99.006)
(7682, 99.21)
(7683, 99.254)
(7684, 98.534)
(7685, 97.326)
(7686, 95.406)
(7687, 97.442)
(7688, 98.574)
(7689, 97.71)
(7690, 97.848)
(7691, 97.376)
(7692, 96.688)
(7693, 97.908)
(7694, 97.504)
(7695, 95.126)
(7696, 95.734)
(7697, 96.748)
(7698, 96.768)
(7699, 95.804)
(7700, 95.856)
(7701, 95.446)
(7702, 98.186)
(7703, 98.596)
(7704, 96.9)
(7705, 89.558)
(7706, 91.448)
(7707, 98.416)
(7708, 97.766)
(7709, 97.642)
(7710, 97.918)
(7711, 98.116)
(7712, 95.05)
(7713, 97.062)
(7714, 96.188)
(7715, 98.034)
(7716, 99.258)
(7717, 97.874)
(7718, 97.272)
(7719, 97.424)
(7720, 98.334)
(7721, 93.92)
(7722, 98.146)
(7723, 98.484)
(7724, 96.512)
(7725, 96.674)
(7726, 96.536)
(7727, 98.374)
(7728, 99.034)
(7729, 98.574)
(7730, 98.384)
(7731, 98.114)
(7732, 97.272)
(7733, 97.454)
(7734, 96.838)
(7735, 97.914)
(7736, 98.406)
(7737, 97.64)
(7738, 97.134)
(7739, 98.374)
(7740, 93.472)
(7741, 96.23)
(7742, 94.716)
(7743, 95.674)
(7744, 97.538)
(7745, 97.108)
(7746, 98.706)
(7747, 99.332)
(7748, 98.89)
(7749, 95.652)
(7750, 98.188)
(7751, 91.134)
(7752, 93.992)
(7753, 93.144)
(7754, 97.536)
(7755, 96.726)
(7756, 97.544)
(7757, 97.104)
(7758, 97.648)
(7759, 94.462)
(7760, 95.25)
(7761, 97.558)
(7762, 93.192)
(7763, 96.804)
(7764, 98.09)
(7765, 96.52)
(7766, 94.5)
(7767, 97.176)
(7768, 97.59)
(7769, 96.338)
(7770, 96.732)
(7771, 95.31)
(7772, 97.65)
(7773, 91.896)
(7774, 98.7)
(7775, 96.276)
(7776, 99.118)
(7777, 98.508)
(7778, 97.576)
(7779, 94.272)
(7780, 97.58)
(7781, 96.506)
(7782, 96.436)
(7783, 97.182)
(7784, 97.038)
(7785, 94.978)
(7786, 96.844)
(7787, 96.21)
(7788, 97)
(7789, 98.562)
(7790, 97.548)
(7791, 98.67)
(7792, 98.844)
(7793, 98.442)
(7794, 98.426)
(7795, 96.782)
(7796, 98.394)
(7797, 98.666)
(7798, 98.72)
(7799, 98.134)
(7800, 98.454)
(7801, 97.478)
(7802, 93.976)
(7803, 97.13)
(7804, 94.936)
(7805, 93.422)
(7806, 96.3)
(7807, 96.642)
(7808, 96.592)
(7809, 95.474)
(7810, 91.754)
(7811, 94.062)
(7812, 90.436)
(7813, 85.488)
(7814, 77.376)
(7815, 77.774)
(7816, 81.61)
(7817, 93.122)
(7818, 89.716)
(7819, 92.29)
(7820, 87.122)
(7821, 93.516)
(7822, 91.32)
(7823, 88.122)
(7824, 89.686)
(7825, 82.152)
(7826, 92.394)
(7827, 85.564)
(7828, 87.29)
(7829, 87.47)
(7830, 76.924)
(7831, 64.378)
(7832, 67.34)
(7833, 87.482)
(7834, 84.826)
(7835, 87.71)
(7836, 81.776)
(7837, 79.228)
(7838, 66.744)
(7839, 73.198)
(7840, 77.866)
(7841, 85.93)
(7842, 79.522)
(7843, 71.438)
(7844, 53.638)
(7845, 65.966)
(7846, 38.188)
(7847, 49.77)
(7848, 59.26)
(7849, 58.332)
(7850, 61.586)
(7851, 48.514)
(7852, 43.736)
(7853, 27.472)
(7854, 71.196)
(7855, 49.42)
(7856, 45.162)
(7857, 67.748)
(7858, 44.544)
(7859, 25.596)
(7860, 19.828)
(7861, 39.556)
(7862, 41.992)
(7863, 20.344)
(7864, 43.37)
(7865, 45.962)
(7866, 20.282)
(7867, 18.19)
(7868, 15.694)
(7869, 52.572)
(7870, 30.946)
(7871, 43.396)
(7872, 28.346)
(7873, 28.978)
(7874, 54.142)
(7875, 39.764)
(7876, 21.866)
(7877, 51.166)
(7878, 57.566)
(7879, 73.5)
(7880, 91.078)
(7881, 99.228)
(7882, 96.056)
(7883, 86.62)
(7884, 89.3)
(7885, 99.072)
(7886, 99.906)
(7887, 94.62)
(7888, 98.812)
(7889, 95.458)
(7890, 90.206)
(7891, 85.302)
(7892, 91.872)
(7893, 78.96)
(7894, 79.672)
(7895, 87.786)
(7896, 84.81)
(7897, 72.004)
(7898, 73.384)
(7899, 76.15)
(7900, 82.294)
(7901, 70.93)
(7902, 74.004)
(7903, 51.23)
(7904, 66.428)
(7905, 55.902)
(7906, 75.398)
(7907, 39.892)
(7908, 72.494)
(7909, 64.874)
(7910, 64.072)
(7911, 68.66)
(7912, 74.972)
(7913, 77.29)
(7914, 87.144)
(7915, 85.564)
(7916, 91.348)
(7917, 74.704)
(7918, 71.322)
(7919, 92.906)
(7920, 81.262)
(7921, 92.414)
(7922, 91.694)
(7923, 90.652)
(7924, 90.684)
(7925, 90.966)
(7926, 83.122)
(7927, 90.232)
(7928, 90.046)
(7929, 90.636)
(7930, 90.03)
(7931, 93.978)
(7932, 91.006)
(7933, 89.754)
(7934, 85.096)
(7935, 90.374)
(7936, 82.498)
(7937, 90.624)
(7938, 92.466)
(7939, 91.59)
(7940, 84.68)
(7941, 89.072)
(7942, 87.782)
(7943, 90.848)
(7944, 89.67)
(7945, 92.65)
(7946, 86.968)
(7947, 90.478)
(7948, 90.176)
(7949, 94.702)
(7950, 95.85)
(7951, 94.946)
(7952, 96.538)
(7953, 96.318)
(7954, 95.584)
(7955, 96.396)
(7956, 95.662)
(7957, 95.424)
(7958, 93.388)
(7959, 93.542)
(7960, 96.462)
(7961, 96.692)
(7962, 95.16)
(7963, 95.302)
(7964, 93.288)
(7965, 94.742)
(7966, 94.764)
(7967, 93.234)
(7968, 98.646)
(7969, 93.618)
(7970, 96.422)
(7971, 93.506)
(7972, 97.634)
(7973, 95.826)
(7974, 97.332)
(7975, 94.256)
(7976, 92.62)
(7977, 97.796)
(7978, 97.548)
(7979, 96.634)
(7980, 95.986)
(7981, 96.616)
(7982, 96.986)
(7983, 91.318)
(7984, 97.276)
(7985, 95.28)
(7986, 94.824)
(7987, 93.56)
(7988, 95.462)
(7989, 95.166)
(7990, 95.052)
(7991, 93.784)
(7992, 83.52)
(7993, 93.734)
(7994, 91.366)
(7995, 92.188)
(7996, 97.846)
(7997, 98.498)
(7998, 98.582)
(7999, 94.682)
(8000, 97.214)
(8001, 99.16)
(8002, 97.104)
(8003, 95.74)
(8004, 94.398)
(8005, 98.268)
(8006, 97.042)
(8007, 97.686)
(8008, 93.136)
(8009, 92.466)
(8010, 96.672)
(8011, 97.61)
(8012, 96.528)
(8013, 97.626)
(8014, 98.212)
(8015, 95.982)
(8016, 98.298)
(8017, 96.924)
(8018, 97.284)
(8019, 94.634)
(8020, 95.858)
(8021, 92.932)
(8022, 96.894)
(8023, 96.578)
(8024, 96.82)
(8025, 96.47)
(8026, 96.634)
(8027, 97.218)
(8028, 98.588)
(8029, 96.768)
(8030, 98.59)
(8031, 97.64)
(8032, 97.13)
(8033, 98.516)
(8034, 97.494)
(8035, 98.166)
(8036, 96.33)
(8037, 98.296)
(8038, 99.192)
(8039, 99.072)
(8040, 98.32)
(8041, 98.666)
(8042, 99.33)
(8043, 94.736)
(8044, 98.822)
(8045, 98.708)
(8046, 98.448)
(8047, 98.002)
(8048, 99.49)
(8049, 99.186)
(8050, 98.324)
(8051, 98.08)
(8052, 96.212)
(8053, 94.946)
(8054, 97.564)
(8055, 98.472)
(8056, 97.834)
(8057, 97.4)
(8058, 98.362)
(8059, 98.378)
(8060, 98.678)
(8061, 94.928)
(8062, 98.154)
(8063, 98.496)
(8064, 97.88)
(8065, 99.33)
(8066, 95.754)
(8067, 82.394)
(8068, 98.604)
(8069, 99.9)
(8070, 99.792)
(8071, 83.476)
(8072, 99.312)
(8073, 99.746)
(8074, 99.802)
(8075, 99.89)
(8076, 99.76)
(8077, 99.632)
(8078, 99.98)
(8079, 99.974)
(8080, 99.98)
(8081, 96.26)
(8082, 99.856)
(8083, 99.958)
(8084, 99.988)
(8085, 100)
(8086, 99.994)
(8087, 99.982)
(8088, 99.998)
(8089, 99.998)
(8090, 99.368)
(8091, 99.898)
(8092, 99.98)
(8093, 99.918)
(8094, 99.836)
(8095, 99.91)
(8096, 99.92)
(8097, 99.944)
(8098, 99.948)
(8099, 97.822)
(8100, 99.884)
(8101, 99.844)
(8102, 99.988)
(8103, 99.502)
(8104, 97.81)
(8105, 99.7)
(8106, 99.52)
(8107, 99.308)
(8108, 99.792)
(8109, 99.83)
(8110, 99.882)
(8111, 99.914)
(8112, 99.914)
(8113, 99.278)
(8114, 99.722)
(8115, 99.684)
(8116, 99.79)
(8117, 99.62)
(8118, 99.95)
(8119, 99.962)
(8120, 99.984)
(8121, 99.928)
(8122, 99.772)
(8123, 99.92)
(8124, 99.818)
(8125, 99.944)
(8126, 99.766)
(8127, 99.722)
(8128, 99.416)
(8129, 99.498)
(8130, 99.156)
(8131, 98.792)
(8132, 99.634)
(8133, 99.704)
(8134, 99.91)
(8135, 99.808)
(8136, 99.454)
(8137, 98.732)
(8138, 99.236)
(8139, 99.112)
(8140, 98.99)
(8141, 96.5)
(8142, 98.544)
(8143, 98.828)
(8144, 98.722)
(8145, 99.12)
(8146, 99.478)
(8147, 99.632)
(8148, 99.734)
(8149, 99.528)
(8150, 99.224)
(8151, 99.286)
(8152, 99.108)
(8153, 99.664)
(8154, 99.614)
(8155, 99.758)
(8156, 99.44)
(8157, 99.046)
(8158, 98.474)
(8159, 98.756)
(8160, 97.902)
(8161, 97.582)
(8162, 95.684)
(8163, 98.014)
(8164, 98.654)
(8165, 98.466)
(8166, 97.802)
(8167, 98.356)
(8168, 97.88)
(8169, 97.828)
(8170, 99.336)
(8171, 99.41)
(8172, 98.718)
(8173, 98.296)
(8174, 99.028)
(8175, 98.002)
(8176, 97.656)
(8177, 98.606)
(8178, 89.274)
(8179, 96.226)
(8180, 98.702)
(8181, 99.016)
(8182, 99.096)
(8183, 97.886)
(8184, 85.91)
(8185, 93.34)
(8186, 98.198)
(8187, 98.838)
(8188, 98.52)
(8189, 97.79)
(8190, 98.994)
(8191, 99.392)
(8192, 98.23)
(8193, 99.038)
(8194, 98.88)
(8195, 98.194)
(8196, 99.258)
(8197, 98.426)
(8198, 98.25)
(8199, 98.692)
(8200, 98.358)
(8201, 98.676)
(8202, 98.458)
(8203, 96.726)
(8204, 98.608)
(8205, 97.992)
(8206, 98.982)
(8207, 99.194)
(8208, 99.156)
(8209, 97.848)
(8210, 98.818)
(8211, 98.244)
(8212, 98.334)
(8213, 99.272)
(8214, 99.002)
(8215, 98.638)
(8216, 97.94)
(8217, 98.844)
(8218, 96.494)
(8219, 99.226)
(8220, 99.042)
(8221, 99.408)
(8222, 99.398)
(8223, 98.928)
(8224, 98.772)
(8225, 97.492)
(8226, 92.876)
(8227, 97.456)
(8228, 97.424)
(8229, 98.768)
(8230, 98.428)
(8231, 98.796)
(8232, 99.436)
(8233, 97.996)
(8234, 98.68)
(8235, 96.9)
(8236, 98.176)
(8237, 97.448)
(8238, 97.686)
(8239, 95.634)
(8240, 97.066)
(8241, 89.802)
(8242, 95.938)
(8243, 96.184)
(8244, 97.65)
(8245, 95.184)
(8246, 85.066)
(8247, 94.754)
(8248, 90.496)
(8249, 97.076)
(8250, 96.174)
(8251, 95.454)
(8252, 97.392)
(8253, 93.508)
(8254, 95.374)
(8255, 94.38)
(8256, 92.338)
(8257, 89.156)
(8258, 87.558)
(8259, 93.18)
(8260, 95.654)
(8261, 96.684)
(8262, 95.966)
(8263, 95.696)
(8264, 93.21)
(8265, 94.14)
(8266, 93.712)
(8267, 95.828)
(8268, 96.298)
(8269, 94.462)
(8270, 96.648)
(8271, 96.742)
(8272, 92.486)
(8273, 94.688)
(8274, 93.708)
(8275, 92.878)
(8276, 80.088)
(8277, 93.768)
(8278, 88.068)
(8279, 91.108)
(8280, 93.544)
(8281, 88.298)
(8282, 84.25)
(8283, 94.464)
(8284, 92.836)
(8285, 92.546)
(8286, 94.146)
(8287, 89.124)
(8288, 94.49)
(8289, 92.256)
(8290, 93.512)
(8291, 94.774)
(8292, 92.552)
(8293, 96.548)
(8294, 95.902)
(8295, 92.406)
(8296, 97.566)
(8297, 91.774)
(8298, 90.852)
(8299, 91.064)
(8300, 93.018)
(8301, 96.008)
(8302, 94.9)
(8303, 91.414)
(8304, 95.294)
(8305, 94.706)
(8306, 94.158)
(8307, 93.408)
(8308, 94.278)
(8309, 93.922)
(8310, 91.296)
(8311, 94.548)
(8312, 96.626)
(8313, 95.706)
(8314, 91.164)
(8315, 96.052)
(8316, 98.31)
(8317, 96.302)
(8318, 96.356)
(8319, 96.556)
(8320, 96.882)
(8321, 97.182)
(8322, 96.748)
(8323, 94.86)
(8324, 97.954)
(8325, 97.456)
(8326, 97.314)
(8327, 97.674)
(8328, 97.458)
(8329, 89.822)
(8330, 99.286)
(8331, 99.63)
(8332, 99.278)
(8333, 92.734)
(8334, 99.55)
(8335, 98.992)
(8336, 99.806)
(8337, 99.82)
(8338, 99.536)
(8339, 92.31)
(8340, 99.754)
(8341, 99.518)
(8342, 99.29)
(8343, 99.61)
(8344, 99.838)
(8345, 99.662)
(8346, 99.678)
(8347, 98.364)
(8348, 87.064)
(8349, 90.594)
(8350, 97.98)
(8351, 98.504)
(8352, 98.684)
(8353, 99.358)
(8354, 98.25)
(8355, 99.64)
(8356, 99.48)
(8357, 99.424)
(8358, 99.732)
(8359, 99.448)
(8360, 98.982)
(8361, 98.98)
(8362, 99.204)
(8363, 99.332)
(8364, 98.948)
(8365, 98.718)
(8366, 99.35)
(8367, 99.37)
(8368, 99.034)
(8369, 99.314)
(8370, 99.714)
(8371, 99.246)
(8372, 99.206)
(8373, 99.358)
(8374, 98.13)
(8375, 99.672)
(8376, 99.882)
(8377, 99.05)
(8378, 98.426)
(8379, 96.268)
(8380, 92.56)
(8381, 96.602)
(8382, 96.334)
(8383, 93.602)
(8384, 93.704)
(8385, 98.14)
(8386, 97.696)
(8387, 96.848)
(8388, 98.494)
(8389, 99.094)
(8390, 97.848)
(8391, 96.766)
(8392, 96.828)
(8393, 97.78)
(8394, 96.45)
(8395, 99.356)
(8396, 99.504)
(8397, 98.812)
(8398, 98.418)
(8399, 99.28)
(8400, 98.554)
(8401, 98.444)
(8402, 98.886)
(8403, 97.15)
(8404, 97.654)
(8405, 95.08)
(8406, 94.8)
(8407, 96.088)
(8408, 94.97)
(8409, 96.938)
(8410, 97.518)
(8411, 99.114)
(8412, 99.042)
(8413, 98.946)
(8414, 99.68)
(8415, 96.154)
(8416, 89.198)
(8417, 99.538)
(8418, 99.366)
(8419, 99.77)
(8420, 99.926)
(8421, 99.476)
(8422, 99.964)
(8423, 99.704)
(8424, 99.788)
(8425, 99.656)
(8426, 99.622)
(8427, 99.664)
(8428, 99.104)
(8429, 98.874)
(8430, 98.242)
(8431, 97.62)
(8432, 98.812)
(8433, 98.954)
(8434, 96.872)
(8435, 98.476)
(8436, 97.232)
(8437, 99.368)
(8438, 99.416)
(8439, 96.06)
(8440, 98.874)
(8441, 98.666)
(8442, 97.18)
(8443, 97.85)
(8444, 92.924)
(8445, 91.63)
(8446, 97.552)
(8447, 94.988)
(8448, 96.05)
(8449, 91.916)
(8450, 97.622)
(8451, 97.668)
(8452, 94.526)
(8453, 96.718)
(8454, 97.414)
(8455, 96.354)
(8456, 97.216)
(8457, 97.138)
(8458, 97.17)
(8459, 97.5)
(8460, 96.332)
(8461, 93.904)
(8462, 94.898)
(8463, 96.354)
(8464, 96.54)
(8465, 95.426)
(8466, 95.76)
(8467, 94.3)
(8468, 84.484)
(8469, 89.906)
(8470, 80.798)
(8471, 91.64)
(8472, 93.966)
(8473, 90.428)
(8474, 94.006)
(8475, 94.316)
(8476, 94.384)
(8477, 94.814)
(8478, 95.366)
(8479, 95.714)
(8480, 94.894)
(8481, 91.374)
(8482, 91.688)
(8483, 89.904)
(8484, 93.33)
(8485, 94.928)
(8486, 95.276)
(8487, 95.88)
(8488, 95.838)
(8489, 94.492)
(8490, 90.792)
(8491, 88.108)
(8492, 92.96)
(8493, 95.53)
(8494, 92.04)
(8495, 93.584)
(8496, 88.18)
(8497, 96.938)
(8498, 97.55)
(8499, 97.996)
(8500, 97.15)
(8501, 93.236)
(8502, 93.814)
(8503, 96.602)
(8504, 94.922)
(8505, 95.782)
(8506, 93.642)
(8507, 92.524)
(8508, 93.472)
(8509, 96.436)
(8510, 93.604)
(8511, 95.786)
(8512, 95.536)
(8513, 81.338)
(8514, 96.132)
(8515, 97.244)
(8516, 98.132)
(8517, 98.372)
(8518, 98.696)
(8519, 97.288)
(8520, 95.22)
(8521, 96.688)
(8522, 97.888)
(8523, 95.842)
(8524, 93.914)
(8525, 96.666)
(8526, 95.824)
(8527, 96.102)
(8528, 92.528)
(8529, 94.684)
(8530, 95.642)
(8531, 95.236)
(8532, 97.566)
(8533, 98.2)
(8534, 98.484)
(8535, 96.034)
(8536, 96.246)
(8537, 96.072)
(8538, 93.682)
(8539, 92.728)
(8540, 90.566)
(8541, 93.472)
(8542, 88.318)
(8543, 94.942)
(8544, 93.38)
(8545, 89.03)
(8546, 97.56)
(8547, 97.192)
(8548, 97.434)
(8549, 96.718)
(8550, 94.2)
(8551, 95.424)
(8552, 97.202)
(8553, 95.038)
(8554, 92.982)
(8555, 95.47)
(8556, 92.018)
(8557, 83.874)
(8558, 90.568)
(8559, 96.642)
(8560, 97.864)
(8561, 97.448)
(8562, 93.14)
(8563, 89.646)
(8564, 93.398)
(8565, 89.782)
(8566, 93.068)
(8567, 88.504)
(8568, 82.762)
(8569, 81.24)
(8570, 94.168)
(8571, 94.486)
(8572, 89.87)
(8573, 93.786)
(8574, 92.634)
(8575, 83.328)
(8576, 86.036)
(8577, 87.09)
(8578, 77.336)
(8579, 82.938)
(8580, 81.236)
(8581, 83.144)
(8582, 92.49)
(8583, 90.968)
(8584, 95.744)
(8585, 89.374)
(8586, 91.71)
(8587, 93.756)
(8588, 79.108)
(8589, 94.56)
(8590, 93.848)
(8591, 90.752)
(8592, 88.818)
(8593, 92.974)
(8594, 88.552)
(8595, 80.764)
(8596, 90.146)
(8597, 87.384)
(8598, 87.292)
(8599, 91.51)
(8600, 90.73)
(8601, 90.534)
(8602, 81.738)
(8603, 79.714)
(8604, 95.916)
(8605, 90.684)
(8606, 84.422)
(8607, 89.758)
(8608, 86.848)
(8609, 95.448)
(8610, 91.422)
(8611, 93.828)
(8612, 93.282)
(8613, 92.872)
(8614, 87.774)
(8615, 94.732)
(8616, 95.672)
(8617, 94.888)
(8618, 92.51)
(8619, 94.418)
(8620, 95.488)
(8621, 93.786)
(8622, 93.474)
(8623, 92.954)
(8624, 86.522)
(8625, 85.464)
(8626, 88.872)
(8627, 74.326)
(8628, 82.172)
(8629, 62.476)
(8630, 78.162)
(8631, 86.31)
(8632, 59.844)
(8633, 85.786)
(8634, 82.498)
(8635, 76.744)
(8636, 61.802)
(8637, 78)
(8638, 79.722)
(8639, 64.064)
(8640, 89.692)
(8641, 78.946)
(8642, 81.25)
(8643, 92.446)
(8644, 93.494)
(8645, 87.15)
(8646, 95.56)
(8647, 91.692)
(8648, 90.496)
(8649, 98.436)
(8650, 98.16)
(8651, 95.236)
(8652, 95.582)
(8653, 97.84)
(8654, 97.51)
(8655, 96.208)
(8656, 97.646)
(8657, 98.426)
(8658, 97.976)
(8659, 96.122)
(8660, 98.102)
(8661, 95.698)
(8662, 96.31)
(8663, 97.036)
(8664, 97.214)
(8665, 94.804)
(8666, 97.47)
(8667, 98.238)
(8668, 88.144)
(8669, 95.82)
(8670, 98.176)
(8671, 98.386)
(8672, 97.804)
(8673, 97.152)
(8674, 92.226)
(8675, 97.528)
(8676, 95.51)
(8677, 98.03)
(8678, 98.036)
(8679, 97.944)
(8680, 96.63)
(8681, 97.054)
(8682, 97.066)
(8683, 99.01)
(8684, 99.188)
(8685, 98.888)
(8686, 97.794)
(8687, 96.192)
(8688, 97.776)
(8689, 96.134)
(8690, 98.296)
(8691, 97.262)
(8692, 98.744)
(8693, 99.224)
(8694, 99.188)
(8695, 98.508)
(8696, 98.578)
(8697, 98.884)
(8698, 97.994)
(8699, 99.184)
(8700, 99.668)
(8701, 99.796)
(8702, 99.272)
(8703, 99.528)
(8704, 99.124)
(8705, 99.324)
(8706, 98.002)
(8707, 98.404)
(8708, 97.114)
(8709, 98.944)
(8710, 98.456)
(8711, 98.994)
(8712, 99.36)
(8713, 98.822)
(8714, 98.186)
(8715, 99.112)
(8716, 99.34)
(8717, 99.304)
(8718, 98.992)
(8719, 97.3)
(8720, 99.012)
(8721, 97.198)
(8722, 97.564)
(8723, 97.452)
(8724, 94.318)
(8725, 96.46)
(8726, 96.584)
(8727, 97.504)
(8728, 97.85)
(8729, 98.22)
(8730, 97.194)
(8731, 98.554)
(8732, 99.122)
(8733, 97.566)
(8734, 96.044)
(8735, 96.89)
(8736, 92.154)
(8737, 95.422)
(8738, 97.514)
(8739, 96.982)
(8740, 96.336)
(8741, 94.582)
(8742, 97.926)
(8743, 98.488)
(8744, 98.514)
(8745, 97.676)
(8746, 96.068)
(8747, 98.25)
(8748, 97.654)
(8749, 97.95)
(8750, 91.636)
(8751, 96.23)
(8752, 94.4)
(8753, 88.778)
(8754, 96.13)
(8755, 92.624)
(8756, 95.204)
(8757, 92.386)
(8758, 90.602)
(8759, 87.562)
(8760, 94.406)
(8761, 93.51)
(8762, 94.41)
(8763, 96.672)
(8764, 95.322)
(8765, 94.75)
(8766, 93.07)
(8767, 95.086)
(8768, 88.708)
(8769, 93.434)
(8770, 89.082)
(8771, 88.434)
(8772, 84.918)
(8773, 88.786)
(8774, 87.44)
(8775, 93.234)
(8776, 93.516)
(8777, 82.992)
(8778, 90.398)
(8779, 93.838)
(8780, 92.614)
(8781, 94.46)
(8782, 87.122)
(8783, 92.064)
(8784, 74.814)
(8785, 79.478)
(8786, 73.97)
(8787, 91.534)
(8788, 81.566)
(8789, 85.57)
(8790, 92.126)
(8791, 87.228)
(8792, 87.568)
(8793, 88.162)
(8794, 89.288)
(8795, 87.708)
(8796, 93.662)
(8797, 92.94)
(8798, 90.842)
(8799, 93.03)
(8800, 90.484)
(8801, 95.336)
(8802, 95.96)
(8803, 94.858)
(8804, 96.64)
(8805, 97.54)
(8806, 96.2)
(8807, 93.796)
(8808, 96.962)
(8809, 95.742)
(8810, 93.504)
(8811, 96.182)
(8812, 93.796)
(8813, 97.524)
(8814, 97.634)
(8815, 94.554)
(8816, 99.23)
(8817, 99.096)
(8818, 90.474)
(8819, 99.07)
(8820, 98.466)
(8821, 98.18)
(8822, 98.1)
(8823, 98.108)
(8824, 97.802)
(8825, 97.51)
(8826, 98.69)
(8827, 99.122)
(8828, 99.468)
(8829, 99.49)
(8830, 97.798)
(8831, 98.296)
(8832, 99.018)
(8833, 98.184)
(8834, 96.672)
(8835, 99.32)
(8836, 98.938)
(8837, 98.25)
(8838, 96.484)
(8839, 97.86)
(8840, 98.304)
(8841, 93.89)
(8842, 97.24)
(8843, 95.566)
(8844, 98.506)
(8845, 99.614)
(8846, 98.778)
(8847, 97.158)
(8848, 98.78)
(8849, 99.592)
(8850, 99.784)
(8851, 99.694)
(8852, 98.268)
(8853, 95.698)
(8854, 98.524)
(8855, 99.334)
(8856, 98.118)
(8857, 98.576)
(8858, 98.552)
(8859, 98.87)
(8860, 97.944)
(8861, 98.502)
(8862, 97.668)
(8863, 97.674)
(8864, 97.61)
(8865, 95.73)
(8866, 97.712)
(8867, 98.706)
(8868, 98.664)
(8869, 98.37)
(8870, 92.258)
(8871, 99.328)
(8872, 99.424)
(8873, 99.144)
(8874, 98.262)
(8875, 98.794)
(8876, 97.972)
(8877, 97.598)
(8878, 98.994)
(8879, 92.704)
(8880, 98.464)
(8881, 98.512)
(8882, 97.974)
(8883, 97.332)
(8884, 96.722)
(8885, 97.912)
(8886, 96.462)
(8887, 96.014)
(8888, 97.01)
(8889, 95.196)
(8890, 98.752)
(8891, 99.104)
(8892, 99.04)
(8893, 98.866)
(8894, 98.472)
(8895, 98.858)
(8896, 98.266)
(8897, 98.838)
(8898, 99.008)
(8899, 98.35)
(8900, 97.12)
(8901, 88.434)
(8902, 96.296)
(8903, 98.924)
(8904, 97.72)
(8905, 98.502)
(8906, 98.336)
(8907, 98.374)
(8908, 97.576)
(8909, 96.032)
(8910, 98.388)
(8911, 98.208)
(8912, 96.236)
(8913, 96.946)
(8914, 98.754)
(8915, 98.966)
(8916, 98.432)
(8917, 97.784)
(8918, 97.002)
(8919, 94.312)
(8920, 95.868)
(8921, 98.61)
(8922, 96.802)
(8923, 97.614)
(8924, 96.948)
(8925, 95.074)
(8926, 96.118)
(8927, 96.932)
(8928, 96.46)
(8929, 98.306)
(8930, 97.998)
(8931, 96.968)
(8932, 95.768)
(8933, 98.09)
(8934, 97.022)
(8935, 97.506)
(8936, 96.58)
(8937, 97.454)
(8938, 98.082)
(8939, 97.526)
(8940, 96.422)
(8941, 98.886)
(8942, 98.13)
(8943, 94.852)
(8944, 96.936)
(8945, 96.422)
(8946, 98.682)
(8947, 99.128)
(8948, 99.41)
(8949, 99.484)
(8950, 99.304)
(8951, 98.104)
(8952, 98.664)
(8953, 99.07)
(8954, 97.746)
(8955, 99.29)
(8956, 99.238)
(8957, 99.132)
(8958, 95.266)
(8959, 95.166)
(8960, 97.182)
(8961, 96.11)
(8962, 96.052)
(8963, 96.252)
(8964, 95.876)
(8965, 92.04)
(8966, 95.47)
(8967, 97.306)
(8968, 96.492)
(8969, 95.526)
(8970, 96.746)
(8971, 94.03)
(8972, 92.444)
(8973, 95.754)
(8974, 95.506)
(8975, 94.658)
(8976, 96.516)
(8977, 96.848)
(8978, 92.45)
(8979, 95.376)
(8980, 91.464)
(8981, 93.212)
(8982, 95.014)
(8983, 94.448)
(8984, 95.538)
(8985, 96.218)
(8986, 88.938)
(8987, 89.672)
(8988, 94.02)
(8989, 94.154)
(8990, 96.38)
(8991, 95.456)
(8992, 97.62)
(8993, 97.006)
(8994, 92.246)
(8995, 97.33)
(8996, 97.236)
(8997, 96.666)
(8998, 92.906)
(8999, 95.428)
(9000, 97.136)
(9001, 90.342)
(9002, 93.78)
(9003, 97.088)
(9004, 98.29)
(9005, 97.766)
(9006, 98.02)
(9007, 98.642)
(9008, 97.45)
(9009, 97.634)
(9010, 98.474)
(9011, 71.086)
(9012, 98.66)
(9013, 97.586)
(9014, 93.28)
(9015, 93.554)
(9016, 95.622)
(9017, 93.048)
(9018, 94.856)
(9019, 85.988)
(9020, 71.01)
(9021, 87.678)
(9022, 86.614)
(9023, 86.074)
(9024, 83.024)
(9025, 90.694)
(9026, 88.454)
(9027, 74.016)
(9028, 76.232)
(9029, 93.6)
(9030, 80.648)
(9031, 88.588)
(9032, 96.218)
(9033, 87.884)
(9034, 97.22)
(9035, 94.066)
(9036, 96.306)
(9037, 93.492)
(9038, 91.368)
(9039, 92.248)
(9040, 94.418)
(9041, 92.874)
(9042, 88.72)
(9043, 84.768)
(9044, 92.324)
(9045, 90.724)
(9046, 96.188)
(9047, 92.67)
(9048, 91.034)
(9049, 90.99)
(9050, 86.008)
(9051, 85.75)
(9052, 89.11)
(9053, 89.556)
(9054, 91.144)
(9055, 89.124)
(9056, 88.574)
(9057, 91.74)
(9058, 80.032)
(9059, 93.666)
(9060, 91.578)
(9061, 68.08)
(9062, 82.35)
(9063, 87.004)
(9064, 93.306)
(9065, 93.762)
(9066, 93.52)
(9067, 95.606)
(9068, 94.13)
(9069, 93.522)
(9070, 91.092)
(9071, 93.608)
(9072, 92.39)
(9073, 94.358)
(9074, 86.682)
(9075, 94.846)
(9076, 92.114)
(9077, 91.934)
(9078, 91.214)
(9079, 89.238)
(9080, 87.676)
(9081, 83.04)
(9082, 78.474)
(9083, 78.646)
(9084, 77.17)
(9085, 93.978)
(9086, 85.48)
(9087, 92.192)
(9088, 90.212)
(9089, 87.876)
(9090, 83.71)
(9091, 92.15)
(9092, 93.422)
(9093, 90.434)
(9094, 93.656)
(9095, 93.708)
(9096, 93.992)
(9097, 86.434)
(9098, 95.178)
(9099, 93.654)
(9100, 93.184)
(9101, 91.848)
(9102, 92.336)
(9103, 89.306)
(9104, 87.698)
(9105, 92.34)
(9106, 86.754)
(9107, 96.242)
(9108, 97.524)
(9109, 97.188)
(9110, 95.9)
(9111, 95.168)
(9112, 94.534)
(9113, 86.036)
(9114, 90.138)
(9115, 87.198)
(9116, 93.646)
(9117, 97.68)
(9118, 96.634)
(9119, 94.816)
(9120, 95.414)
(9121, 97.894)
(9122, 98.094)
(9123, 96.622)
(9124, 95.264)
(9125, 94.264)
(9126, 93.502)
(9127, 95.396)
(9128, 92.68)
(9129, 93.36)
(9130, 90.302)
(9131, 95.142)
(9132, 93.232)
(9133, 97.342)
(9134, 93.182)
(9135, 97.538)
(9136, 96.434)
(9137, 94.578)
(9138, 80.418)
(9139, 96.988)
(9140, 98.6)
(9141, 98.19)
(9142, 98.392)
(9143, 98.61)
(9144, 98.542)
(9145, 97.876)
(9146, 98.168)
(9147, 98.052)
(9148, 98.61)
(9149, 98.166)
(9150, 99.23)
(9151, 99.182)
(9152, 99.158)
(9153, 98.966)
(9154, 98.74)
(9155, 94.016)
(9156, 98.218)
(9157, 99.09)
(9158, 99.068)
(9159, 96.42)
(9160, 91.242)
(9161, 96.882)
(9162, 95.872)
(9163, 95.054)
(9164, 95.268)
(9165, 95.578)
(9166, 95.098)
(9167, 96.552)
(9168, 97.022)
(9169, 97.568)
(9170, 95.958)
(9171, 96.494)
(9172, 94.894)
(9173, 94.498)
(9174, 96.928)
(9175, 91.878)
(9176, 93.802)
(9177, 91.866)
(9178, 97.344)
(9179, 97.43)
(9180, 95.22)
(9181, 92.592)
(9182, 93.44)
(9183, 96.5)
(9184, 96.354)
(9185, 97.706)
(9186, 97.44)
(9187, 98.412)
(9188, 94.642)
(9189, 93.932)
(9190, 97.864)
(9191, 97.426)
(9192, 97.73)
(9193, 97.862)
(9194, 97.422)
(9195, 98.842)
(9196, 97.93)
(9197, 97.654)
(9198, 94.676)
(9199, 96.878)
(9200, 94.602)
(9201, 98.166)
(9202, 99.112)
(9203, 99.006)
(9204, 98.306)
(9205, 98.394)
(9206, 98.062)
(9207, 97.928)
(9208, 89.744)
(9209, 94.816)
(9210, 94.432)
(9211, 94.41)
(9212, 93.944)
(9213, 96.098)
(9214, 96.074)
(9215, 96.558)
(9216, 96.47)
(9217, 97.098)
(9218, 97.95)
(9219, 96.24)
(9220, 97.336)
(9221, 95.564)
(9222, 94.2)
(9223, 94.066)
(9224, 88.302)
(9225, 92.708)
(9226, 90.614)
(9227, 95.446)
(9228, 96.77)
(9229, 96.792)
(9230, 98.128)
(9231, 95.584)
(9232, 94.78)
(9233, 93.114)
(9234, 94.568)
(9235, 96.636)
(9236, 95.044)
(9237, 96.058)
(9238, 97.25)
(9239, 96.912)
(9240, 96.332)
(9241, 96.414)
(9242, 94.796)
(9243, 93.586)
(9244, 92.05)
(9245, 95.932)
(9246, 93.752)
(9247, 89.478)
(9248, 93.138)
(9249, 94.266)
(9250, 95.166)
(9251, 96.392)
(9252, 97.538)
(9253, 98.21)
(9254, 96.684)
(9255, 96.976)
(9256, 95.84)
(9257, 95.07)
(9258, 94.47)
(9259, 95.418)
(9260, 97.56)
(9261, 97.02)
(9262, 94.53)
(9263, 93.856)
(9264, 96.07)
(9265, 96.362)
(9266, 96.742)
(9267, 96.794)
(9268, 95.334)
(9269, 94.838)
(9270, 95.654)
(9271, 96.538)
(9272, 97.354)
(9273, 95.602)
(9274, 97.61)
(9275, 97.114)
(9276, 98.782)
(9277, 98.92)
(9278, 96.828)
(9279, 70.3714285714286)
(9280, 0)
};


==> covgraphs/graph.0.errors.tex <==
\addplot [sharp plot,color=magenta,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.000412264908314335)
(1, 0.000220831136816001)
(2, 8.0160455030667e-05)
(3, 2.83056859690001e-05)
(4, 1.59853047483334e-05)
(5, 1.18135300945001e-05)
(6, 1.18915071908334e-05)
(7, 1.01370225233334e-05)
(8, 7.9926523741667e-06)
(9, 9.27927446366671e-06)
(10, 1.45037399180001e-05)
(11, 2.23404380995001e-05)
(12, 8.42152640400004e-06)
(13, 1.00200568788334e-05)
(14, 8.49950350033337e-06)
(15, 8.18759511500004e-06)
(16, 8.2265836631667e-06)
(17, 1.50885681405001e-05)
(18, 7.71973253700003e-06)
(19, 8.81141188566671e-06)
(20, 9.70814849350004e-06)
(21, 1.03319652641667e-05)
(22, 9.16230881916671e-06)
(23, 2.33151518036668e-05)
(24, 7.68074398883337e-06)
(25, 7.79770963333337e-06)
(26, 1.85585489273334e-05)
(27, 1.04489309086667e-05)
(28, 1.15406102573334e-05)
(29, 9.98106833066671e-06)
(30, 1.02149996196667e-05)
(31, 1.58683391038334e-05)
(32, 1.08778049385e-05)
(33, 1.20474613835001e-05)
(34, 1.31391407321667e-05)
(35, 1.12287018720001e-05)
(36, 1.12287018720001e-05)
(37, 1.18525186426667e-05)
(38, 1.32561063766667e-05)
(39, 1.32950949248334e-05)
(40, 1.38799231473334e-05)
(41, 1.60242932965001e-05)
(42, 1.98451710168334e-05)
(43, 1.57123849111667e-05)
(44, 1.62582245855001e-05)
(45, 1.53224994295001e-05)
(46, 1.71939497415001e-05)
(47, 2.99042164438335e-05)
(48, 1.96892168241668e-05)
(49, 3.70391207583335e-05)
(50, 1.96112397278334e-05)
(51, 3.88325939740002e-05)
(52, 2.40559342188334e-05)
(53, 3.78188917216668e-05)
(54, 6.4253127378667e-05)
(55, 8.8519377662053e-05)
(56, 9.54260415170565e-05)
(57, 8.3271950232904e-05)
(58, 8.02204414948042e-05)
(59, 7.82229030033851e-05)
(60, 8.36357386815854e-05)
(61, 0.000100194580843433)
(62, 8.30221870198768e-05)
(63, 7.91926249874877e-05)
(64, 7.77454844913825e-05)
(65, 9.95056061467561e-05)
(66, 0.000108052250588736)
(67, 7.68348835919152e-05)
(68, 7.29207014448616e-05)
(69, 7.76459045608638e-05)
(70, 7.37951367715244e-05)
(71, 7.15228471490021e-05)
(72, 8.37977000030579e-05)
(73, 9.15638414390157e-05)
(74, 7.91514357233262e-05)
(75, 7.31921952413646e-05)
(76, 8.18871268265921e-05)
(77, 7.44007047337596e-05)
(78, 8.20906715131171e-05)
(79, 8.63313774099415e-05)
(80, 8.66372846254769e-05)
(81, 8.26984303368954e-05)
(82, 8.01126961319027e-05)
(83, 7.8262730890608e-05)
(84, 7.95850763561185e-05)
(85, 8.07716052346895e-05)
(86, 8.69133537427621e-05)
(87, 9.27779851588473e-05)
(88, 9.15986594328013e-05)
(89, 9.15179301637403e-05)
(90, 8.47438872398916e-05)
(91, 8.28459995393928e-05)
(92, 9.64761862035397e-05)
(93, 9.4260738019093e-05)
(94, 0.000109029811382186)
(95, 8.38080386187442e-05)
(96, 9.56800768543752e-05)
(97, 0.000128658178015792)
(98, 0.000182162494800912)
(99, 0.000175134943123947)
(100, 0)
};



==> covgraphs/graph.1.500.tex <==
\addplot[const plot,fill=darkgreen,draw=darkgreen] coordinates {
(-1, 0)
(0, 94.448)
(1, 92.87)
(2, 96.49)
(3, 97.57)
(4, 97.922)
(5, 96.8)
(6, 94.216)
(7, 95.236)
(8, 94.788)
(9, 96.956)
(10, 96.668)
(11, 98.6)
(12, 97.412)
(13, 96.598)
(14, 96.106)
(15, 95.456)
(16, 97.806)
(17, 97.502)
(18, 97.102)
(19, 97.284)
(20, 98.348)
(21, 95.196)
(22, 97.098)
(23, 96.776)
(24, 97.084)
(25, 96.32)
(26, 97.902)
(27, 97.498)
(28, 96.976)
(29, 95.652)
(30, 97.886)
(31, 99.454)
(32, 99.974)
(33, 95.576)
(34, 97.992)
(35, 97.238)
(36, 97.758)
(37, 97.62)
(38, 98.334)
(39, 98.22)
(40, 98.68)
(41, 98.452)
(42, 98.338)
(43, 97.84)
(44, 98.194)
(45, 97.038)
(46, 96.184)
(47, 96.682)
(48, 96.862)
(49, 97.12)
(50, 96.088)
(51, 94.78)
(52, 96.404)
(53, 97.22)
(54, 96.796)
(55, 94.246)
(56, 95.194)
(57, 98.098)
(58, 98.412)
(59, 98.112)
(60, 95.888)
(61, 97.522)
(62, 95.416)
(63, 96.708)
(64, 95.806)
(65, 93.444)
(66, 94.952)
(67, 97.128)
(68, 99.428)
(69, 97.544)
(70, 95.828)
(71, 91.958)
(72, 98.65)
(73, 94.754)
(74, 95.446)
(75, 96.614)
(76, 96.568)
(77, 91.942)
(78, 94.728)
(79, 95.902)
(80, 93.23)
(81, 94.978)
(82, 96.304)
(83, 96.156)
(84, 97.684)
(85, 92.544)
(86, 94.308)
(87, 91.208)
(88, 93.164)
(89, 93.864)
(90, 94.734)
(91, 93.838)
(92, 93.644)
(93, 95.184)
(94, 93.676)
(95, 84.642)
(96, 91.642)
(97, 94.128)
(98, 96.072)
(99, 94.854)
(100, 94.51)
(101, 89.822)
(102, 96.264)
(103, 96.922)
(104, 93.392)
(105, 95.186)
(106, 95.424)
(107, 93.554)
(108, 92.77)
(109, 94.712)
(110, 94.716)
(111, 97.46)
(112, 96.354)
(113, 94.856)
(114, 94.904)
(115, 94.612)
(116, 98.204)
(117, 98.63)
(118, 96.462)
(119, 96.962)
(120, 93.786)
(121, 94.634)
(122, 95.77)
(123, 86.164)
(124, 89.808)
(125, 90.044)
(126, 93.454)
(127, 88.866)
(128, 89.808)
(129, 89.43)
(130, 91.038)
(131, 90.85)
(132, 86.676)
(133, 85.416)
(134, 91.968)
(135, 81.838)
(136, 91.214)
(137, 87.29)
(138, 86.254)
(139, 92.842)
(140, 95.478)
(141, 92.352)
(142, 92.488)
(143, 82.11)
(144, 91.946)
(145, 92.902)
(146, 83.122)
(147, 76.116)
(148, 82.206)
(149, 88.734)
(150, 85.712)
(151, 92.83)
(152, 94.522)
(153, 93.898)
(154, 93.848)
(155, 94.762)
(156, 94.858)
(157, 95.058)
(158, 87.334)
(159, 86.37)
(160, 89.362)
(161, 87.78)
(162, 88.198)
(163, 73.816)
(164, 84.722)
(165, 87.104)
(166, 89.564)
(167, 95.528)
(168, 96.864)
(169, 95.728)
(170, 93.93)
(171, 90.244)
(172, 79.848)
(173, 89.49)
(174, 91.428)
(175, 95.218)
(176, 92.182)
(177, 89.84)
(178, 95.518)
(179, 94.51)
(180, 86.224)
(181, 79.836)
(182, 87.76)
(183, 91.218)
(184, 93.118)
(185, 80.784)
(186, 63.854)
(187, 85.204)
(188, 83.426)
(189, 82.84)
(190, 88.412)
(191, 90.588)
(192, 90.188)
(193, 93.91)
(194, 88.208)
(195, 93.236)
(196, 85.726)
(197, 93.554)
(198, 91.122)
(199, 93.03)
(200, 86.268)
(201, 94.226)
(202, 89.542)
(203, 89.458)
(204, 94.106)
(205, 97.826)
(206, 93.51)
(207, 96.696)
(208, 97.386)
(209, 95.12)
(210, 97.278)
(211, 97.554)
(212, 97.034)
(213, 97.898)
(214, 98.634)
(215, 96.292)
(216, 98.056)
(217, 97.38)
(218, 97.804)
(219, 95.832)
(220, 98.392)
(221, 96.404)
(222, 97.688)
(223, 98.138)
(224, 95.96)
(225, 97.392)
(226, 99.026)
(227, 98.344)
(228, 95.752)
(229, 98.488)
(230, 97.622)
(231, 94.726)
(232, 95.964)
(233, 91.84)
(234, 95.946)
(235, 97.138)
(236, 95.66)
(237, 94.658)
(238, 95.724)
(239, 94.168)
(240, 97.068)
(241, 94.27)
(242, 95.76)
(243, 97.94)
(244, 88.642)
(245, 89.442)
(246, 84.154)
(247, 89.802)
(248, 89.418)
(249, 84.042)
(250, 80.69)
(251, 82.91)
(252, 78.306)
(253, 69.73)
(254, 87.424)
(255, 91.774)
(256, 94.258)
(257, 93.314)
(258, 91.484)
(259, 80.592)
(260, 25.362)
(261, 18.248)
(262, 41.66)
(263, 54.528)
(264, 19.45)
(265, 16.236)
(266, 57.76)
(267, 57.43)
(268, 60.43)
(269, 66.66)
(270, 78.268)
(271, 80.31)
(272, 86.426)
(273, 86.858)
(274, 69.31)
(275, 67.618)
(276, 82.43)
(277, 88.918)
(278, 80.956)
(279, 80.074)
(280, 91.174)
(281, 84.134)
(282, 86.724)
(283, 88.5)
(284, 86.796)
(285, 94.916)
(286, 95.488)
(287, 94.854)
(288, 92.532)
(289, 94.732)
(290, 92.206)
(291, 93.568)
(292, 91.09)
(293, 94.362)
(294, 95.892)
(295, 97.622)
(296, 96.742)
(297, 92.374)
(298, 91.796)
(299, 97.46)
(300, 98.882)
(301, 98.368)
(302, 98.224)
(303, 96.996)
(304, 98.028)
(305, 98.58)
(306, 97.118)
(307, 96.814)
(308, 96.686)
(309, 96.764)
(310, 97.698)
(311, 97.326)
(312, 97.266)
(313, 96.41)
(314, 97.034)
(315, 93.062)
(316, 92.482)
(317, 93.386)
(318, 93.592)
(319, 92.998)
(320, 91.796)
(321, 97.302)
(322, 96.482)
(323, 89.934)
(324, 83.976)
(325, 91.216)
(326, 78.268)
(327, 86.502)
(328, 90.102)
(329, 88.65)
(330, 95.558)
(331, 95.83)
(332, 95.142)
(333, 95.258)
(334, 95.25)
(335, 93.504)
(336, 94.646)
(337, 97.696)
(338, 97.35)
(339, 94.93)
(340, 90.936)
(341, 93.842)
(342, 94.886)
(343, 89.336)
(344, 86.614)
(345, 87.172)
(346, 90.19)
(347, 94.838)
(348, 94.35)
(349, 97.222)
(350, 93.458)
(351, 95.218)
(352, 96.268)
(353, 96.99)
(354, 94.034)
(355, 97.794)
(356, 96.916)
(357, 96.408)
(358, 97.804)
(359, 96.354)
(360, 98.724)
(361, 97.848)
(362, 97.382)
(363, 97.75)
(364, 98.568)
(365, 96.368)
(366, 96.848)
(367, 98.126)
(368, 97.704)
(369, 97.662)
(370, 96.356)
(371, 97.086)
(372, 96.35)
(373, 96.424)
(374, 95.268)
(375, 95.378)
(376, 96.422)
(377, 96.934)
(378, 96.742)
(379, 98.414)
(380, 98.294)
(381, 98.224)
(382, 98.284)
(383, 97.678)
(384, 96.796)
(385, 97.978)
(386, 97.572)
(387, 95.428)
(388, 97.336)
(389, 98.424)
(390, 98.784)
(391, 97.962)
(392, 98.368)
(393, 97.854)
(394, 98.672)
(395, 98.11)
(396, 99.04)
(397, 98.916)
(398, 98.922)
(399, 99.068)
(400, 98.916)
(401, 99.364)
(402, 99.116)
(403, 98.77)
(404, 99.244)
(405, 98.524)
(406, 98.71)
(407, 99.372)
(408, 96.35)
(409, 98.21)
(410, 98.406)
(411, 98.248)
(412, 98.406)
(413, 92.816)
(414, 93.38)
(415, 99.14)
(416, 98.988)
(417, 99.416)
(418, 99.112)
(419, 99.82)
(420, 99.47)
(421, 99.058)
(422, 99.206)
(423, 99.776)
(424, 99.414)
(425, 98.224)
(426, 96.75)
(427, 99.528)
(428, 99.688)
(429, 99.378)
(430, 99.078)
(431, 99.674)
(432, 99.818)
(433, 99.74)
(434, 99.48)
(435, 99.496)
(436, 95.9)
(437, 99.048)
(438, 99.368)
(439, 99.662)
(440, 99.776)
(441, 99.692)
(442, 99.424)
(443, 98.99)
(444, 99.558)
(445, 99.798)
(446, 99.572)
(447, 89.104)
(448, 99.424)
(449, 93.81)
(450, 99.716)
(451, 86.288)
(452, 85.216)
(453, 89.332)
(454, 99.916)
(455, 99.722)
(456, 99.596)
(457, 99.974)
(458, 100)
(459, 100)
(460, 100)
(461, 99.978)
(462, 99.878)
(463, 99.804)
(464, 99.994)
(465, 99.984)
(466, 99.862)
(467, 99.998)
(468, 100)
(469, 99.97)
(470, 99.798)
(471, 99.916)
(472, 99.874)
(473, 99.936)
(474, 99.996)
(475, 99.984)
(476, 99.996)
(477, 99.99)
(478, 99.77)
(479, 95.022)
(480, 99.938)
(481, 99.678)
(482, 99.262)
(483, 98.752)
(484, 97.69)
(485, 97.74)
(486, 99.716)
(487, 99.146)
(488, 99.628)
(489, 99.398)
(490, 99.428)
(491, 99.726)
(492, 99.744)
(493, 99.264)
(494, 98.608)
(495, 99.734)
(496, 98.912)
(497, 98.364)
(498, 91.992)
(499, 95.5)
(500, 98.852)
(501, 97.004)
(502, 98.926)
(503, 99.134)
(504, 99.762)
(505, 99.674)
(506, 99.692)
(507, 98.416)
(508, 99.494)
(509, 99.438)
(510, 97.996)
(511, 99.686)
(512, 98.854)
(513, 95.698)
(514, 98.786)
(515, 94.592)
(516, 99.252)
(517, 99.446)
(518, 99.214)
(519, 97.32)
(520, 94.456)
(521, 94.576)
(522, 97.598)
(523, 98.324)
(524, 99.446)
(525, 97.154)
(526, 86.002)
(527, 97.568)
(528, 97.324)
(529, 98.938)
(530, 99.508)
(531, 98.374)
(532, 97.36)
(533, 97.97)
(534, 97.522)
(535, 98.224)
(536, 98.98)
(537, 99.492)
(538, 99.514)
(539, 98.534)
(540, 97.544)
(541, 99.472)
(542, 98.116)
(543, 98.586)
(544, 96.6)
(545, 99.176)
(546, 99.522)
(547, 98.256)
(548, 98.414)
(549, 97.164)
(550, 98.24)
(551, 98.706)
(552, 96.942)
(553, 95.664)
(554, 98.404)
(555, 97.5)
(556, 93.116)
(557, 89.166)
(558, 99.446)
(559, 99.434)
(560, 95.5)
(561, 89.174)
(562, 95.974)
(563, 94.046)
(564, 90.774)
(565, 82.94)
(566, 69.534)
(567, 89.894)
(568, 88.794)
(569, 95.432)
(570, 90.276)
(571, 90.646)
(572, 88.186)
(573, 84.092)
(574, 92.082)
(575, 86.324)
(576, 96.866)
(577, 92.232)
(578, 96.302)
(579, 93.82)
(580, 88.544)
(581, 98.728)
(582, 99.59)
(583, 99.62)
(584, 99.702)
(585, 99.752)
(586, 99.802)
(587, 99.8)
(588, 99.548)
(589, 99.832)
(590, 99.812)
(591, 94.98)
(592, 99.824)
(593, 98.766)
(594, 95.746)
(595, 97.06)
(596, 98.566)
(597, 93.022)
(598, 95.088)
(599, 91.46)
(600, 96.962)
(601, 94.914)
(602, 98.11)
(603, 97.306)
(604, 99.728)
(605, 99.786)
(606, 99.574)
(607, 99.244)
(608, 98.98)
(609, 98.862)
(610, 98.604)
(611, 98.522)
(612, 98.538)
(613, 93.662)
(614, 97.182)
(615, 96.212)
(616, 98.802)
(617, 97.304)
(618, 99.246)
(619, 99.444)
(620, 99.714)
(621, 99.886)
(622, 99.752)
(623, 99.82)
(624, 99.89)
(625, 99.868)
(626, 99.888)
(627, 99.61)
(628, 99.65)
(629, 94.366)
(630, 92.508)
(631, 95.036)
(632, 99.86)
(633, 99.936)
(634, 99.844)
(635, 99.938)
(636, 99.488)
(637, 99.746)
(638, 99.77)
(639, 99.384)
(640, 99.712)
(641, 99.756)
(642, 99.52)
(643, 99.57)
(644, 99.696)
(645, 99.702)
(646, 99.72)
(647, 99.918)
(648, 99.956)
(649, 99.716)
(650, 96.462)
(651, 98.358)
(652, 98.716)
(653, 98.156)
(654, 96.076)
(655, 95.168)
(656, 97.698)
(657, 99.404)
(658, 98.41)
(659, 98.002)
(660, 98.228)
(661, 99.706)
(662, 99.974)
(663, 99.936)
(664, 99.868)
(665, 99.914)
(666, 99.64)
(667, 99.646)
(668, 99.738)
(669, 99.742)
(670, 99.704)
(671, 99.778)
(672, 99.21)
(673, 95.51)
(674, 98.556)
(675, 96.258)
(676, 97.8)
(677, 97.7)
(678, 95.16)
(679, 96.598)
(680, 99.108)
(681, 98.02)
(682, 99.302)
(683, 99.546)
(684, 99.22)
(685, 99.038)
(686, 99.978)
(687, 99.83)
(688, 99.988)
(689, 99.922)
(690, 99.626)
(691, 99.97)
(692, 98.994)
(693, 98.004)
(694, 99.202)
(695, 99.884)
(696, 98.512)
(697, 77.344)
(698, 90.74)
(699, 96.238)
(700, 99.348)
(701, 96.146)
(702, 98.82)
(703, 99.382)
(704, 97.996)
(705, 96.692)
(706, 97.22)
(707, 99.164)
(708, 99.554)
(709, 98.876)
(710, 99.37)
(711, 99.666)
(712, 99.184)
(713, 89.102)
(714, 92.512)
(715, 98.552)
(716, 98.306)
(717, 97.948)
(718, 98.21)
(719, 96.548)
(720, 99.258)
(721, 99.8)
(722, 99.482)
(723, 99.604)
(724, 99.408)
(725, 98.852)
(726, 97.938)
(727, 98.264)
(728, 97.996)
(729, 98.64)
(730, 98.406)
(731, 98.392)
(732, 98.2)
(733, 98.51)
(734, 97.068)
(735, 98.874)
(736, 98.44)
(737, 94.15)
(738, 96.752)
(739, 96.864)
(740, 98.044)
(741, 97.254)
(742, 99.06)
(743, 97.186)
(744, 98.552)
(745, 97.87)
(746, 98.862)
(747, 93.654)
(748, 75.374)
(749, 98.692)
(750, 96.636)
(751, 98.858)
(752, 99.796)
(753, 99.036)
(754, 99.702)
(755, 99.676)
(756, 99.464)
(757, 99.442)
(758, 96.042)
(759, 99.724)
(760, 99.876)
(761, 96.816)
(762, 92.794)
(763, 99.374)
(764, 98.438)
(765, 99.598)
(766, 99.928)
(767, 99.93)
(768, 99.924)
(769, 98.904)
(770, 98.808)
(771, 98.738)
(772, 96.002)
(773, 99.016)
(774, 99.58)
(775, 99.592)
(776, 98.858)
(777, 99.786)
(778, 99.996)
(779, 99.99)
(780, 99.988)
(781, 99.968)
(782, 98.364)
(783, 99.62)
(784, 99.912)
(785, 99.86)
(786, 99.918)
(787, 99.98)
(788, 99.854)
(789, 99.032)
(790, 99.314)
(791, 99.67)
(792, 99.798)
(793, 99.148)
(794, 99.59)
(795, 99.49)
(796, 98.582)
(797, 99.882)
(798, 99.778)
(799, 99.768)
(800, 99.98)
(801, 99.968)
(802, 99.272)
(803, 99.694)
(804, 99.568)
(805, 99.79)
(806, 98.814)
(807, 99.77)
(808, 99.39)
(809, 99.748)
(810, 99.252)
(811, 99.584)
(812, 99.978)
(813, 99.962)
(814, 99.946)
(815, 99.75)
(816, 99.814)
(817, 99.852)
(818, 99.606)
(819, 98.948)
(820, 99.472)
(821, 99.828)
(822, 99.104)
(823, 99.652)
(824, 99.738)
(825, 99.418)
(826, 98.574)
(827, 98.646)
(828, 99.102)
(829, 98.986)
(830, 99.402)
(831, 98.796)
(832, 99.662)
(833, 97.676)
(834, 98.86)
(835, 99.34)
(836, 99.776)
(837, 98.034)
(838, 98.238)
(839, 98.98)
(840, 98.998)
(841, 98.846)
(842, 99.212)
(843, 98.84)
(844, 97.99)
(845, 97.962)
(846, 98.84)
(847, 99.014)
(848, 99.412)
(849, 98.94)
(850, 99.458)
(851, 99.432)
(852, 99.786)
(853, 99.658)
(854, 99.476)
(855, 99.592)
(856, 99.78)
(857, 99.222)
(858, 99.478)
(859, 99.948)
(860, 99.84)
(861, 99.766)
(862, 99.926)
(863, 99.964)
(864, 99.682)
(865, 97.302)
(866, 99.474)
(867, 99.542)
(868, 99.15)
(869, 99.796)
(870, 98.786)
(871, 99.594)
(872, 99.546)
(873, 99.7)
(874, 99.202)
(875, 99.262)
(876, 99.692)
(877, 99.784)
(878, 99.514)
(879, 99.686)
(880, 99.04)
(881, 99.466)
(882, 99.138)
(883, 99.59)
(884, 96.984)
(885, 98.38)
(886, 99.46)
(887, 99.772)
(888, 99.842)
(889, 97.724)
(890, 99.23)
(891, 99.22)
(892, 96.37)
(893, 99.396)
(894, 98.886)
(895, 99.302)
(896, 99.066)
(897, 98.248)
(898, 98.568)
(899, 98.194)
(900, 98.598)
(901, 99.664)
(902, 98.458)
(903, 97.71)
(904, 98.284)
(905, 99.028)
(906, 99.462)
(907, 99.73)
(908, 99.682)
(909, 99.6)
(910, 99.112)
(911, 99.798)
(912, 99.562)
(913, 99.554)
(914, 99.346)
(915, 99.49)
(916, 99.598)
(917, 99.586)
(918, 99.426)
(919, 99.58)
(920, 99.61)
(921, 99.806)
(922, 99.778)
(923, 99.334)
(924, 98.73)
(925, 99.528)
(926, 99.784)
(927, 99.93)
(928, 99.574)
(929, 99.628)
(930, 99.362)
(931, 99.604)
(932, 99.532)
(933, 99.848)
(934, 99.726)
(935, 98.88)
(936, 99.546)
(937, 99.7)
(938, 99.774)
(939, 98.032)
(940, 98.876)
(941, 99.656)
(942, 99.042)
(943, 99.618)
(944, 99.65)
(945, 98.822)
(946, 96.998)
(947, 99.76)
(948, 99.87)
(949, 99.612)
(950, 99.484)
(951, 99.738)
(952, 99.91)
(953, 99.81)
(954, 99.958)
(955, 99.922)
(956, 99.976)
(957, 99.95)
(958, 99.986)
(959, 99.994)
(960, 99.942)
(961, 99.72)
(962, 99.756)
(963, 99.866)
(964, 99.484)
(965, 98.43)
(966, 99.258)
(967, 99.47)
(968, 99.732)
(969, 99.786)
(970, 99.954)
(971, 99.896)
(972, 99.792)
(973, 99.772)
(974, 99.694)
(975, 99.376)
(976, 99.81)
(977, 99.846)
(978, 99.71)
(979, 95.41)
(980, 99.346)
(981, 99.788)
(982, 99.182)
(983, 98.912)
(984, 97.068)
(985, 92.274)
(986, 99.818)
(987, 99.23)
(988, 99.778)
(989, 99.698)
(990, 99.884)
(991, 99.688)
(992, 99.824)
(993, 99.546)
(994, 98.922)
(995, 98.208)
(996, 99.506)
(997, 99.74)
(998, 99.694)
(999, 99.714)
(1000, 99.268)
(1001, 99.68)
(1002, 99.456)
(1003, 99.238)
(1004, 99.186)
(1005, 99.534)
(1006, 98.618)
(1007, 98.968)
(1008, 99.704)
(1009, 99.352)
(1010, 99.858)
(1011, 99.462)
(1012, 99.866)
(1013, 99.512)
(1014, 99.564)
(1015, 89.524)
(1016, 98.992)
(1017, 96.894)
(1018, 98.084)
(1019, 97.746)
(1020, 96.44)
(1021, 99.736)
(1022, 99.372)
(1023, 99.09)
(1024, 99.376)
(1025, 98.644)
(1026, 98.674)
(1027, 96.614)
(1028, 99.13)
(1029, 99.714)
(1030, 99.834)
(1031, 99.844)
(1032, 99.794)
(1033, 99.474)
(1034, 99.47)
(1035, 99.182)
(1036, 98.98)
(1037, 99.072)
(1038, 98.788)
(1039, 97.862)
(1040, 98.904)
(1041, 97.026)
(1042, 98.038)
(1043, 98.386)
(1044, 99.834)
(1045, 92.266)
(1046, 92.17)
(1047, 94.394)
(1048, 89.806)
(1049, 90.002)
(1050, 89.774)
(1051, 95.562)
(1052, 99.84)
(1053, 99.994)
(1054, 96.37)
(1055, 100)
(1056, 100)
(1057, 99.948)
(1058, 99.892)
(1059, 99.786)
(1060, 99.482)
(1061, 99.704)
(1062, 99.81)
(1063, 99.89)
(1064, 99.82)
(1065, 99.808)
(1066, 99.86)
(1067, 99.77)
(1068, 99.842)
(1069, 99.958)
(1070, 99.916)
(1071, 99.99)
(1072, 99.972)
(1073, 99.976)
(1074, 99.992)
(1075, 99.95)
(1076, 99.98)
(1077, 99.904)
(1078, 99.95)
(1079, 99.96)
(1080, 99.648)
(1081, 99.838)
(1082, 99.404)
(1083, 99.28)
(1084, 99.984)
(1085, 99.994)
(1086, 99.972)
(1087, 99.936)
(1088, 99.246)
(1089, 99.76)
(1090, 99.522)
(1091, 99.958)
(1092, 99.408)
(1093, 97.654)
(1094, 98.2)
(1095, 87.742)
(1096, 99.666)
(1097, 99.3)
(1098, 99.452)
(1099, 98.956)
(1100, 99.352)
(1101, 99.576)
(1102, 99.616)
(1103, 98.96)
(1104, 99.724)
(1105, 99.714)
(1106, 99.896)
(1107, 99.99)
(1108, 99.428)
(1109, 99.726)
(1110, 99.61)
(1111, 99.758)
(1112, 99.788)
(1113, 98.71)
(1114, 99.528)
(1115, 99.96)
(1116, 99.976)
(1117, 99.984)
(1118, 99.994)
(1119, 99.95)
(1120, 99.91)
(1121, 99.574)
(1122, 99.938)
(1123, 99.992)
(1124, 99.724)
(1125, 99.58)
(1126, 100)
(1127, 99.994)
(1128, 99.968)
(1129, 99.96)
(1130, 99.886)
(1131, 99.75)
(1132, 94.898)
(1133, 92.838)
(1134, 95.142)
(1135, 99.926)
(1136, 99.998)
(1137, 99.99)
(1138, 100)
(1139, 100)
(1140, 99.996)
(1141, 100)
(1142, 100)
(1143, 99.992)
(1144, 99.826)
(1145, 99.898)
(1146, 99.99)
(1147, 99.906)
(1148, 98.882)
(1149, 98.008)
(1150, 100)
(1151, 99.968)
(1152, 99.996)
(1153, 99.996)
(1154, 100)
(1155, 99.938)
(1156, 100)
(1157, 100)
(1158, 100)
(1159, 99.98)
(1160, 99.814)
(1161, 99.944)
(1162, 100)
(1163, 100)
(1164, 100)
(1165, 100)
(1166, 100)
(1167, 100)
(1168, 99.996)
(1169, 99.988)
(1170, 100)
(1171, 99.922)
(1172, 99.956)
(1173, 99.776)
(1174, 99.926)
(1175, 98.708)
(1176, 99.8)
(1177, 99.682)
(1178, 99.896)
(1179, 99.872)
(1180, 99.904)
(1181, 99.776)
(1182, 99.902)
(1183, 99.774)
(1184, 99.942)
(1185, 99.8)
(1186, 99.9)
(1187, 99.912)
(1188, 99.648)
(1189, 99.94)
(1190, 97.682)
(1191, 98.194)
(1192, 99.936)
(1193, 98.788)
(1194, 97.488)
(1195, 98.072)
(1196, 99.036)
(1197, 96.53)
(1198, 99.022)
(1199, 97.776)
(1200, 98.268)
(1201, 97.978)
(1202, 99.328)
(1203, 99.052)
(1204, 99.744)
(1205, 99.792)
(1206, 99.608)
(1207, 99.694)
(1208, 99.374)
(1209, 99.85)
(1210, 99.51)
(1211, 99.496)
(1212, 99.044)
(1213, 99.66)
(1214, 99.39)
(1215, 99.664)
(1216, 99.964)
(1217, 99.792)
(1218, 99.514)
(1219, 99.276)
(1220, 99.31)
(1221, 98.412)
(1222, 97.156)
(1223, 99.334)
(1224, 98.456)
(1225, 98.028)
(1226, 97.104)
(1227, 98.244)
(1228, 95.192)
(1229, 97.426)
(1230, 97.39)
(1231, 94.596)
(1232, 96.074)
(1233, 98.204)
(1234, 99.426)
(1235, 98.754)
(1236, 99.446)
(1237, 98.972)
(1238, 98.224)
(1239, 97.024)
(1240, 97.118)
(1241, 94.448)
(1242, 95.902)
(1243, 97.726)
(1244, 93.198)
(1245, 98.454)
(1246, 96.958)
(1247, 98.314)
(1248, 97.468)
(1249, 98.818)
(1250, 98.272)
(1251, 99.106)
(1252, 97.97)
(1253, 98.714)
(1254, 98.626)
(1255, 98.862)
(1256, 98.192)
(1257, 98.722)
(1258, 98.164)
(1259, 99.3)
(1260, 98.506)
(1261, 99.484)
(1262, 99.792)
(1263, 99.264)
(1264, 98.75)
(1265, 99.696)
(1266, 99.176)
(1267, 99.794)
(1268, 99.808)
(1269, 99.93)
(1270, 99.832)
(1271, 99.984)
(1272, 99.99)
(1273, 99.992)
(1274, 99.766)
(1275, 99.986)
(1276, 99.904)
(1277, 98.924)
(1278, 98.754)
(1279, 98.12)
(1280, 98.236)
(1281, 98.946)
(1282, 99.652)
(1283, 98.932)
(1284, 98.652)
(1285, 99.29)
(1286, 99.672)
(1287, 98.856)
(1288, 99.388)
(1289, 99.32)
(1290, 97.282)
(1291, 97.766)
(1292, 97.782)
(1293, 97.612)
(1294, 98.458)
(1295, 98.302)
(1296, 98.286)
(1297, 96.612)
(1298, 97.508)
(1299, 97.39)
(1300, 98.044)
(1301, 99.418)
(1302, 99.754)
(1303, 99.304)
(1304, 99.338)
(1305, 99.286)
(1306, 99.572)
(1307, 99.3)
(1308, 99.684)
(1309, 98.048)
(1310, 99.818)
(1311, 99.8)
(1312, 99.75)
(1313, 99.724)
(1314, 99.608)
(1315, 98.32)
(1316, 99.72)
(1317, 99.392)
(1318, 99.362)
(1319, 99.784)
(1320, 99.866)
(1321, 99.956)
(1322, 99.732)
(1323, 99.942)
(1324, 99.88)
(1325, 99.662)
(1326, 99.428)
(1327, 98.396)
(1328, 97.696)
(1329, 99.29)
(1330, 99.642)
(1331, 99.342)
(1332, 99.336)
(1333, 99.316)
(1334, 99.46)
(1335, 95.904)
(1336, 99.524)
(1337, 99.684)
(1338, 99.35)
(1339, 99.024)
(1340, 99.568)
(1341, 99.074)
(1342, 98.748)
(1343, 98.462)
(1344, 98.988)
(1345, 97.474)
(1346, 98.328)
(1347, 94.216)
(1348, 99.418)
(1349, 99.564)
(1350, 99.266)
(1351, 99.666)
(1352, 99.604)
(1353, 99.508)
(1354, 99.558)
(1355, 99.384)
(1356, 99.516)
(1357, 99.806)
(1358, 98.912)
(1359, 99.512)
(1360, 99.634)
(1361, 97.71)
(1362, 99.63)
(1363, 99.054)
(1364, 99.634)
(1365, 99.738)
(1366, 98.996)
(1367, 99.526)
(1368, 99.39)
(1369, 99.256)
(1370, 93.256)
(1371, 99.37)
(1372, 99.426)
(1373, 99.346)
(1374, 99.068)
(1375, 98.572)
(1376, 99.062)
(1377, 97.554)
(1378, 98.806)
(1379, 97.346)
(1380, 99.124)
(1381, 99.108)
(1382, 99.05)
(1383, 99.162)
(1384, 95.6)
(1385, 98.768)
(1386, 96.588)
(1387, 97.602)
(1388, 98.202)
(1389, 98.38)
(1390, 97.844)
(1391, 98.912)
(1392, 99.23)
(1393, 99.16)
(1394, 99.578)
(1395, 99.386)
(1396, 99.404)
(1397, 99.432)
(1398, 98.952)
(1399, 99.28)
(1400, 99.04)
(1401, 97.96)
(1402, 99.498)
(1403, 99.194)
(1404, 99.428)
(1405, 99.302)
(1406, 98.388)
(1407, 94.036)
(1408, 98.93)
(1409, 97.874)
(1410, 99.554)
(1411, 99.488)
(1412, 99.072)
(1413, 99.548)
(1414, 99.634)
(1415, 99.37)
(1416, 99.29)
(1417, 99.07)
(1418, 99.706)
(1419, 99.772)
(1420, 99.674)
(1421, 99.5)
(1422, 99.48)
(1423, 99.29)
(1424, 99.606)
(1425, 99.494)
(1426, 97.096)
(1427, 98.652)
(1428, 98.552)
(1429, 99.67)
(1430, 99.852)
(1431, 99.818)
(1432, 99.774)
(1433, 99.384)
(1434, 99.416)
(1435, 99.512)
(1436, 99.788)
(1437, 99.296)
(1438, 99.424)
(1439, 99.666)
(1440, 99.332)
(1441, 97.558)
(1442, 98.898)
(1443, 96.258)
(1444, 97.584)
(1445, 95.468)
(1446, 94.85)
(1447, 97.232)
(1448, 97.724)
(1449, 95.746)
(1450, 94.726)
(1451, 95.766)
(1452, 96.888)
(1453, 92.414)
(1454, 98.046)
(1455, 97.374)
(1456, 98.524)
(1457, 92.646)
(1458, 66.51)
(1459, 83.14)
(1460, 93.346)
(1461, 72.816)
(1462, 81.238)
(1463, 67.842)
(1464, 81.06)
(1465, 99.338)
(1466, 91.43)
(1467, 70.4)
(1468, 90.068)
(1469, 99.648)
(1470, 99.734)
(1471, 99.862)
(1472, 81.55)
(1473, 66.14)
(1474, 99.85)
(1475, 94.238)
(1476, 94.404)
(1477, 93.006)
(1478, 97.076)
(1479, 97.27)
(1480, 99.478)
(1481, 99.67)
(1482, 99)
(1483, 99.7)
(1484, 99.012)
(1485, 95.192)
(1486, 98.146)
(1487, 98.558)
(1488, 99.54)
(1489, 98.358)
(1490, 99.458)
(1491, 99.578)
(1492, 98.472)
(1493, 99.492)
(1494, 99.938)
(1495, 99.918)
(1496, 99.81)
(1497, 99.866)
(1498, 99.492)
(1499, 99.7)
(1500, 99.498)
(1501, 99.374)
(1502, 99.114)
(1503, 99.772)
(1504, 98.076)
(1505, 99.606)
(1506, 99.596)
(1507, 99.94)
(1508, 99.554)
(1509, 99.502)
(1510, 98.336)
(1511, 98.086)
(1512, 98.796)
(1513, 99.188)
(1514, 98.974)
(1515, 99.102)
(1516, 99.324)
(1517, 99.016)
(1518, 98.636)
(1519, 98.556)
(1520, 98.124)
(1521, 98.742)
(1522, 98.276)
(1523, 98.918)
(1524, 99.352)
(1525, 99.17)
(1526, 98.89)
(1527, 99.022)
(1528, 99.412)
(1529, 99.756)
(1530, 99.056)
(1531, 93.59)
(1532, 98.238)
(1533, 99.246)
(1534, 99.146)
(1535, 99.122)
(1536, 99.606)
(1537, 99.896)
(1538, 99.74)
(1539, 99.786)
(1540, 99.924)
(1541, 99.87)
(1542, 99.64)
(1543, 99.12)
(1544, 99.57)
(1545, 99.474)
(1546, 99.788)
(1547, 99.906)
(1548, 99.934)
(1549, 99.524)
(1550, 99.53)
(1551, 97.86)
(1552, 94.686)
(1553, 99.96)
(1554, 99.606)
(1555, 99.854)
(1556, 99.874)
(1557, 99.91)
(1558, 99.612)
(1559, 99.782)
(1560, 99.36)
(1561, 99.75)
(1562, 99.97)
(1563, 99.57)
(1564, 99.542)
(1565, 99.972)
(1566, 99.828)
(1567, 99.848)
(1568, 98.088)
(1569, 99.99)
(1570, 99.638)
(1571, 99.222)
(1572, 99.936)
(1573, 99.948)
(1574, 99.524)
(1575, 99.142)
(1576, 99.43)
(1577, 99.684)
(1578, 99.402)
(1579, 99.384)
(1580, 99.32)
(1581, 99.626)
(1582, 99.896)
(1583, 99.478)
(1584, 99.818)
(1585, 99.678)
(1586, 99.662)
(1587, 99.746)
(1588, 99.85)
(1589, 99.756)
(1590, 99.54)
(1591, 99.776)
(1592, 99.806)
(1593, 99.662)
(1594, 99.842)
(1595, 99.79)
(1596, 99.456)
(1597, 99.792)
(1598, 99.742)
(1599, 99.986)
(1600, 99.666)
(1601, 99.936)
(1602, 99.736)
(1603, 99.776)
(1604, 99.824)
(1605, 99.638)
(1606, 99.312)
(1607, 99.668)
(1608, 99.806)
(1609, 99.714)
(1610, 99.602)
(1611, 99.848)
(1612, 99.608)
(1613, 99.8)
(1614, 98.946)
(1615, 99.398)
(1616, 99.316)
(1617, 99.624)
(1618, 99.656)
(1619, 95.956)
(1620, 98.86)
(1621, 90.426)
(1622, 99.03)
(1623, 99.088)
(1624, 99.838)
(1625, 99.86)
(1626, 99.892)
(1627, 98.482)
(1628, 99.91)
(1629, 99.944)
(1630, 99.864)
(1631, 99.544)
(1632, 99.692)
(1633, 98.894)
(1634, 99.7)
(1635, 99.438)
(1636, 98.968)
(1637, 99.27)
(1638, 99.922)
(1639, 99.93)
(1640, 99.986)
(1641, 99.934)
(1642, 99.742)
(1643, 99.32)
(1644, 99.436)
(1645, 99.498)
(1646, 99.072)
(1647, 99.84)
(1648, 99.296)
(1649, 99.838)
(1650, 99.718)
(1651, 99.754)
(1652, 99.514)
(1653, 98.172)
(1654, 99.644)
(1655, 99.36)
(1656, 98.446)
(1657, 98.702)
(1658, 98.364)
(1659, 99.292)
(1660, 98.282)
(1661, 99.526)
(1662, 94.394)
(1663, 99.716)
(1664, 99.518)
(1665, 99.33)
(1666, 98.242)
(1667, 99.61)
(1668, 99.542)
(1669, 97.35)
(1670, 98.902)
(1671, 98.214)
(1672, 98.996)
(1673, 97.828)
(1674, 99.884)
(1675, 99.62)
(1676, 99.066)
(1677, 99.094)
(1678, 99.108)
(1679, 99.482)
(1680, 98.524)
(1681, 99.712)
(1682, 99.696)
(1683, 99.726)
(1684, 99.016)
(1685, 99.394)
(1686, 99.288)
(1687, 99.784)
(1688, 99.382)
(1689, 99.48)
(1690, 99.692)
(1691, 99.724)
(1692, 99.7)
(1693, 99.772)
(1694, 99.93)
(1695, 99.798)
(1696, 99.95)
(1697, 99.512)
(1698, 99.932)
(1699, 99.89)
(1700, 99.928)
(1701, 99.824)
(1702, 99.802)
(1703, 99.82)
(1704, 99.966)
(1705, 99.812)
(1706, 99.786)
(1707, 99.852)
(1708, 98.87)
(1709, 99.506)
(1710, 99.706)
(1711, 99.712)
(1712, 99.902)
(1713, 99.678)
(1714, 99.898)
(1715, 99.826)
(1716, 99.892)
(1717, 99.96)
(1718, 99.96)
(1719, 98.28)
(1720, 98.986)
(1721, 99.746)
(1722, 99.516)
(1723, 99.822)
(1724, 99.618)
(1725, 99.666)
(1726, 99.642)
(1727, 99.896)
(1728, 99.632)
(1729, 99.504)
(1730, 99.126)
(1731, 99.866)
(1732, 99.082)
(1733, 99.288)
(1734, 99.714)
(1735, 99.668)
(1736, 99.584)
(1737, 99.87)
(1738, 99.768)
(1739, 99.808)
(1740, 99.382)
(1741, 98.954)
(1742, 99.85)
(1743, 99.788)
(1744, 99.998)
(1745, 100)
(1746, 100)
(1747, 99.99)
(1748, 100)
(1749, 100)
(1750, 99.928)
(1751, 100)
(1752, 99.994)
(1753, 99.798)
(1754, 100)
(1755, 100)
(1756, 99.952)
(1757, 99.992)
(1758, 100)
(1759, 100)
(1760, 100)
(1761, 99.978)
(1762, 99.998)
(1763, 99.972)
(1764, 99.966)
(1765, 100)
(1766, 99.832)
(1767, 99.798)
(1768, 100)
(1769, 100)
(1770, 99.774)
(1771, 99.74)
(1772, 99.966)
(1773, 99.99)
(1774, 99.972)
(1775, 99.984)
(1776, 99.946)
(1777, 99.99)
(1778, 99.998)
(1779, 99.992)
(1780, 99.98)
(1781, 99.872)
(1782, 99.83)
(1783, 99.61)
(1784, 99.968)
(1785, 99.996)
(1786, 99.974)
(1787, 99.94)
(1788, 99.814)
(1789, 99.824)
(1790, 99.89)
(1791, 99.968)
(1792, 99.83)
(1793, 99.79)
(1794, 99.92)
(1795, 99.932)
(1796, 99.048)
(1797, 99.986)
(1798, 99.998)
(1799, 99.966)
(1800, 99.968)
(1801, 99.814)
(1802, 99.902)
(1803, 99.944)
(1804, 99.924)
(1805, 99.976)
(1806, 99.956)
(1807, 99.964)
(1808, 99.722)
(1809, 99.89)
(1810, 99.748)
(1811, 99.994)
(1812, 99.848)
(1813, 99.79)
(1814, 99.464)
(1815, 99.87)
(1816, 98.178)
(1817, 99.836)
(1818, 99.948)
(1819, 99.63)
(1820, 93.872)
(1821, 99.466)
(1822, 99.79)
(1823, 99.818)
(1824, 99.536)
(1825, 99.768)
(1826, 99.834)
(1827, 99.73)
(1828, 99.152)
(1829, 99.872)
(1830, 99.89)
(1831, 99.434)
(1832, 99.516)
(1833, 99.818)
(1834, 99.702)
(1835, 99.872)
(1836, 99.932)
(1837, 99.404)
(1838, 99.924)
(1839, 99.726)
(1840, 97.688)
(1841, 99.824)
(1842, 99.962)
(1843, 99.994)
(1844, 99.958)
(1845, 99.908)
(1846, 99.972)
(1847, 99.964)
(1848, 99.998)
(1849, 99.99)
(1850, 99.94)
(1851, 100)
(1852, 99.972)
(1853, 99.998)
(1854, 99.998)
(1855, 99.966)
(1856, 99.926)
(1857, 99.87)
(1858, 99.948)
(1859, 99.88)
(1860, 99.98)
(1861, 99.88)
(1862, 99.986)
(1863, 99.986)
(1864, 99.99)
(1865, 99.926)
(1866, 99.42)
(1867, 99.652)
(1868, 99.566)
(1869, 95.726)
(1870, 99.968)
(1871, 99.86)
(1872, 99.928)
(1873, 99.89)
(1874, 99.49)
(1875, 99.914)
(1876, 99.68)
(1877, 99.952)
(1878, 99.912)
(1879, 99.68)
(1880, 99.352)
(1881, 98.614)
(1882, 99.736)
(1883, 99.958)
(1884, 99.73)
(1885, 98.704)
(1886, 99.792)
(1887, 99.702)
(1888, 99.93)
(1889, 99.98)
(1890, 99.862)
(1891, 99.94)
(1892, 99.98)
(1893, 99.944)
(1894, 99.968)
(1895, 98.772)
(1896, 99.914)
(1897, 99.98)
(1898, 99.996)
(1899, 99.99)
(1900, 99.946)
(1901, 99.922)
(1902, 99.92)
(1903, 99.934)
(1904, 99.896)
(1905, 99.99)
(1906, 99.92)
(1907, 99.806)
(1908, 99.664)
(1909, 99.954)
(1910, 99.822)
(1911, 99.914)
(1912, 99.92)
(1913, 99.962)
(1914, 99.758)
(1915, 99.916)
(1916, 99.376)
(1917, 99.916)
(1918, 99.988)
(1919, 99.95)
(1920, 99.896)
(1921, 99.738)
(1922, 99.968)
(1923, 99.942)
(1924, 99.836)
(1925, 99.876)
(1926, 99.956)
(1927, 99.912)
(1928, 99.868)
(1929, 99.8)
(1930, 99.96)
(1931, 99.906)
(1932, 99.972)
(1933, 99.9)
(1934, 99.012)
(1935, 89.236)
(1936, 96.904)
(1937, 98.158)
(1938, 98.096)
(1939, 98.98)
(1940, 96.798)
(1941, 98.992)
(1942, 98.1)
(1943, 98.078)
(1944, 98.676)
(1945, 98.026)
(1946, 98.44)
(1947, 96.598)
(1948, 96.006)
(1949, 98.898)
(1950, 98.762)
(1951, 96.32)
(1952, 98.226)
(1953, 97.836)
(1954, 97.97)
(1955, 98.918)
(1956, 98.8)
(1957, 98.888)
(1958, 99.3)
(1959, 99.086)
(1960, 95.628)
(1961, 98.096)
(1962, 98.54)
(1963, 99.278)
(1964, 99.352)
(1965, 99.418)
(1966, 99.222)
(1967, 99.516)
(1968, 99.06)
(1969, 99.064)
(1970, 99.78)
(1971, 99.544)
(1972, 99.726)
(1973, 99.424)
(1974, 99.218)
(1975, 98.516)
(1976, 98.79)
(1977, 98.84)
(1978, 98.678)
(1979, 99.49)
(1980, 98.612)
(1981, 99.158)
(1982, 98.402)
(1983, 97.816)
(1984, 96.894)
(1985, 96.314)
(1986, 95.298)
(1987, 94.316)
(1988, 93.002)
(1989, 91.738)
(1990, 97.528)
(1991, 96.662)
(1992, 96.858)
(1993, 99.06)
(1994, 98.842)
(1995, 99.178)
(1996, 98.586)
(1997, 99.126)
(1998, 98.956)
(1999, 99.136)
(2000, 99.03)
(2001, 98.77)
(2002, 98.71)
(2003, 99.138)
(2004, 99.052)
(2005, 99.246)
(2006, 97.832)
(2007, 99.172)
(2008, 99.186)
(2009, 99.43)
(2010, 99.496)
(2011, 98.906)
(2012, 98.842)
(2013, 99.488)
(2014, 98.278)
(2015, 96.254)
(2016, 98.902)
(2017, 98.812)
(2018, 99.238)
(2019, 98.716)
(2020, 98.624)
(2021, 98.508)
(2022, 98.93)
(2023, 98.684)
(2024, 99.51)
(2025, 99.212)
(2026, 99.356)
(2027, 99.102)
(2028, 99.044)
(2029, 99.662)
(2030, 98.74)
(2031, 99.74)
(2032, 99.484)
(2033, 98.92)
(2034, 99.108)
(2035, 99.57)
(2036, 99.644)
(2037, 99.196)
(2038, 99.466)
(2039, 99.652)
(2040, 99.686)
(2041, 99.488)
(2042, 99.26)
(2043, 99.398)
(2044, 99.084)
(2045, 98.264)
(2046, 99.508)
(2047, 99.272)
(2048, 98.486)
(2049, 99.528)
(2050, 99.444)
(2051, 98.958)
(2052, 99.702)
(2053, 99.53)
(2054, 99.554)
(2055, 99.446)
(2056, 99.1)
(2057, 97.702)
(2058, 97.114)
(2059, 98.344)
(2060, 99.268)
(2061, 99.508)
(2062, 98.658)
(2063, 96.762)
(2064, 93.688)
(2065, 98.346)
(2066, 97.93)
(2067, 96.716)
(2068, 95.366)
(2069, 96.88)
(2070, 96.7)
(2071, 96.856)
(2072, 97.938)
(2073, 99.14)
(2074, 99.042)
(2075, 98.732)
(2076, 99.128)
(2077, 98.126)
(2078, 99.358)
(2079, 99.254)
(2080, 98.696)
(2081, 98.988)
(2082, 98.344)
(2083, 99.138)
(2084, 99.202)
(2085, 99.252)
(2086, 99.498)
(2087, 99.37)
(2088, 99.19)
(2089, 99.51)
(2090, 99.134)
(2091, 98.47)
(2092, 99.238)
(2093, 99.2)
(2094, 99.222)
(2095, 99.184)
(2096, 99.336)
(2097, 94.608)
(2098, 86.834)
(2099, 89.622)
(2100, 99.866)
(2101, 99.774)
(2102, 99.77)
(2103, 99.548)
(2104, 99.292)
(2105, 99.132)
(2106, 98.908)
(2107, 98.794)
(2108, 98.728)
(2109, 98.546)
(2110, 99.372)
(2111, 98.924)
(2112, 98.476)
(2113, 99.414)
(2114, 99.682)
(2115, 99.144)
(2116, 99.394)
(2117, 97.548)
(2118, 99.382)
(2119, 99.356)
(2120, 99.186)
(2121, 99.01)
(2122, 98.842)
(2123, 99.204)
(2124, 98.982)
(2125, 97.926)
(2126, 99.974)
(2127, 99.996)
(2128, 99.998)
(2129, 99.55)
(2130, 99.672)
(2131, 99.918)
(2132, 99.67)
(2133, 99.688)
(2134, 93.444)
(2135, 95.698)
(2136, 99.614)
(2137, 98.634)
(2138, 98.038)
(2139, 98.528)
(2140, 98.202)
(2141, 97.802)
(2142, 99.304)
(2143, 96.406)
(2144, 99.528)
(2145, 99.496)
(2146, 99.886)
(2147, 99.566)
(2148, 97.39)
(2149, 98.134)
(2150, 99.396)
(2151, 99.098)
(2152, 99.238)
(2153, 99.416)
(2154, 99.484)
(2155, 98.638)
(2156, 99.932)
(2157, 99.398)
(2158, 99.258)
(2159, 99.298)
(2160, 99.608)
(2161, 99.842)
(2162, 99.696)
(2163, 99.928)
(2164, 99.54)
(2165, 99.378)
(2166, 99.948)
(2167, 98.646)
(2168, 99.988)
(2169, 99.822)
(2170, 99.996)
(2171, 99.996)
(2172, 99.99)
(2173, 99.984)
(2174, 100)
(2175, 100)
(2176, 99.998)
(2177, 99.852)
(2178, 99.994)
(2179, 99.952)
(2180, 99.978)
(2181, 99.948)
(2182, 99.976)
(2183, 99.996)
(2184, 100)
(2185, 100)
(2186, 99.986)
(2187, 99.374)
(2188, 99.008)
(2189, 99.988)
(2190, 99.998)
(2191, 99.994)
(2192, 81.196)
(2193, 99.394)
(2194, 99.996)
(2195, 99.956)
(2196, 99.982)
(2197, 99.882)
(2198, 99.024)
(2199, 99.926)
(2200, 99.964)
(2201, 99.954)
(2202, 100)
(2203, 99.968)
(2204, 99.998)
(2205, 99.908)
(2206, 99.256)
(2207, 99.942)
(2208, 99.998)
(2209, 99.998)
(2210, 99.742)
(2211, 99.846)
(2212, 99.87)
(2213, 99.942)
(2214, 99.982)
(2215, 99.974)
(2216, 99.976)
(2217, 99.994)
(2218, 99.944)
(2219, 99.902)
(2220, 99.772)
(2221, 99.924)
(2222, 99.076)
(2223, 99.888)
(2224, 99.676)
(2225, 99.91)
(2226, 99.924)
(2227, 99.692)
(2228, 98.36)
(2229, 99.934)
(2230, 99.83)
(2231, 99.986)
(2232, 99.924)
(2233, 99.602)
(2234, 99.76)
(2235, 98.566)
(2236, 99.88)
(2237, 99.538)
(2238, 99.554)
(2239, 99.33)
(2240, 99.882)
(2241, 97.072)
(2242, 99.294)
(2243, 98.724)
(2244, 99.728)
(2245, 97.24)
(2246, 98.854)
(2247, 98.776)
(2248, 99.038)
(2249, 99.64)
(2250, 99.654)
(2251, 99.22)
(2252, 98.974)
(2253, 99.184)
(2254, 98.614)
(2255, 98.264)
(2256, 99.378)
(2257, 99.332)
(2258, 99.25)
(2259, 98.962)
(2260, 99.07)
(2261, 98.848)
(2262, 98.978)
(2263, 98.822)
(2264, 99.424)
(2265, 98.786)
(2266, 95.918)
(2267, 99.276)
(2268, 98.436)
(2269, 98.378)
(2270, 98.714)
(2271, 98.972)
(2272, 97.806)
(2273, 99.132)
(2274, 98.492)
(2275, 97.58)
(2276, 99.322)
(2277, 98.902)
(2278, 99.382)
(2279, 98.662)
(2280, 99.382)
(2281, 96.632)
(2282, 97.374)
(2283, 94.004)
(2284, 99.31)
(2285, 96.878)
(2286, 99.128)
(2287, 99.566)
(2288, 99.108)
(2289, 99.43)
(2290, 99.388)
(2291, 99.784)
(2292, 99.6)
(2293, 99.416)
(2294, 99.078)
(2295, 99.188)
(2296, 99.208)
(2297, 99.224)
(2298, 95.216)
(2299, 99.446)
(2300, 99.654)
(2301, 99.854)
(2302, 99.722)
(2303, 99.58)
(2304, 99.606)
(2305, 99.744)
(2306, 99.83)
(2307, 99.8)
(2308, 99.872)
(2309, 99.728)
(2310, 99.68)
(2311, 99.834)
(2312, 99.862)
(2313, 99.92)
(2314, 99.384)
(2315, 99.19)
(2316, 99.778)
(2317, 99.73)
(2318, 99.48)
(2319, 99.896)
(2320, 99.758)
(2321, 99.874)
(2322, 99.792)
(2323, 99.324)
(2324, 99.594)
(2325, 99.268)
(2326, 99.72)
(2327, 99.886)
(2328, 99.966)
(2329, 99.914)
(2330, 99.506)
(2331, 99.848)
(2332, 99.794)
(2333, 99.212)
(2334, 99.838)
(2335, 99.976)
(2336, 99.964)
(2337, 99.78)
(2338, 99.204)
(2339, 99.894)
(2340, 99.592)
(2341, 99.562)
(2342, 99.006)
(2343, 99.572)
(2344, 98.038)
(2345, 99.572)
(2346, 99.75)
(2347, 97.762)
(2348, 99.888)
(2349, 99.85)
(2350, 99.856)
(2351, 99.684)
(2352, 99.418)
(2353, 99.616)
(2354, 99.89)
(2355, 99.912)
(2356, 99.836)
(2357, 99.934)
(2358, 99.96)
(2359, 99.984)
(2360, 99.99)
(2361, 99.994)
(2362, 99.978)
(2363, 99.93)
(2364, 99.932)
(2365, 99.888)
(2366, 99.936)
(2367, 99.998)
(2368, 99.938)
(2369, 99.99)
(2370, 99.972)
(2371, 99.996)
(2372, 99.932)
(2373, 99.976)
(2374, 99.786)
(2375, 99.91)
(2376, 99.96)
(2377, 99.928)
(2378, 99.984)
(2379, 99.996)
(2380, 99.982)
(2381, 99.854)
(2382, 99.812)
(2383, 99.444)
(2384, 99.96)
(2385, 99.972)
(2386, 99.204)
(2387, 99.826)
(2388, 99.99)
(2389, 99.99)
(2390, 99.964)
(2391, 99.996)
(2392, 100)
(2393, 100)
(2394, 100)
(2395, 100)
(2396, 100)
(2397, 100)
(2398, 99.998)
(2399, 99.992)
(2400, 99.85)
(2401, 99.99)
(2402, 99.988)
(2403, 99.972)
(2404, 99.968)
(2405, 99.942)
(2406, 99.956)
(2407, 99.408)
(2408, 99.858)
(2409, 99.682)
(2410, 99.712)
(2411, 99.692)
(2412, 99.402)
(2413, 99.784)
(2414, 99.992)
(2415, 99.986)
(2416, 99.996)
(2417, 99.978)
(2418, 99.98)
(2419, 100)
(2420, 100)
(2421, 100)
(2422, 100)
(2423, 100)
(2424, 100)
(2425, 99.958)
(2426, 99.996)
(2427, 100)
(2428, 99.992)
(2429, 100)
(2430, 100)
(2431, 100)
(2432, 100)
(2433, 100)
(2434, 100)
(2435, 99.998)
(2436, 100)
(2437, 100)
(2438, 100)
(2439, 100)
(2440, 100)
(2441, 99.988)
(2442, 99.004)
(2443, 99.974)
(2444, 100)
(2445, 100)
(2446, 99.996)
(2447, 100)
(2448, 99.994)
(2449, 99.992)
(2450, 100)
(2451, 99.996)
(2452, 100)
(2453, 99.998)
(2454, 99.084)
(2455, 99.992)
(2456, 99.984)
(2457, 100)
(2458, 99.994)
(2459, 99.998)
(2460, 99.986)
(2461, 99.984)
(2462, 99.966)
(2463, 99.654)
(2464, 99.962)
(2465, 99.976)
(2466, 99.916)
(2467, 99.966)
(2468, 99.988)
(2469, 99.936)
(2470, 99.988)
(2471, 99.984)
(2472, 99.966)
(2473, 99.856)
(2474, 99.636)
(2475, 99.838)
(2476, 99.818)
(2477, 98.008)
(2478, 99.768)
(2479, 99.864)
(2480, 99.874)
(2481, 99.852)
(2482, 99.962)
(2483, 99.84)
(2484, 99.878)
(2485, 99.92)
(2486, 99.968)
(2487, 99.944)
(2488, 99.73)
(2489, 99.932)
(2490, 99.85)
(2491, 99.808)
(2492, 99.972)
(2493, 99.994)
(2494, 99.974)
(2495, 99.892)
(2496, 99.668)
(2497, 99.7)
(2498, 99.708)
(2499, 98.92)
(2500, 99.824)
(2501, 99.72)
(2502, 99.688)
(2503, 99.73)
(2504, 99.8)
(2505, 99.91)
(2506, 99.51)
(2507, 99.294)
(2508, 99.196)
(2509, 99.762)
(2510, 99.888)
(2511, 99.92)
(2512, 99.604)
(2513, 99.67)
(2514, 99.634)
(2515, 99.534)
(2516, 96.164)
(2517, 93.328)
(2518, 96.95)
(2519, 96.952)
(2520, 96.376)
(2521, 96.074)
(2522, 96.968)
(2523, 90.034)
(2524, 90.08)
(2525, 90.65)
(2526, 87.562)
(2527, 88.68)
(2528, 94.052)
(2529, 80.542)
(2530, 90.078)
(2531, 79.326)
(2532, 90.602)
(2533, 89.636)
(2534, 93.514)
(2535, 91.58)
(2536, 70.15)
(2537, 73.69)
(2538, 83.734)
(2539, 87.51)
(2540, 93.248)
(2541, 84.51)
(2542, 94.706)
(2543, 91.638)
(2544, 91.626)
(2545, 95.424)
(2546, 93.646)
(2547, 92.29)
(2548, 91.958)
(2549, 94.552)
(2550, 90.78)
(2551, 78.488)
(2552, 75.066)
(2553, 94.04)
(2554, 93.452)
(2555, 90.528)
(2556, 87.706)
(2557, 95.116)
(2558, 92.052)
(2559, 88.676)
(2560, 89.724)
(2561, 62.092)
(2562, 90.566)
(2563, 84.148)
(2564, 90.224)
(2565, 85.036)
(2566, 90.756)
(2567, 89.726)
(2568, 91.466)
(2569, 88.618)
(2570, 91.73)
(2571, 87.298)
(2572, 91.088)
(2573, 97.25)
(2574, 97.962)
(2575, 97.256)
(2576, 97.666)
(2577, 97.256)
(2578, 96.892)
(2579, 97.204)
(2580, 98.16)
(2581, 97.814)
(2582, 97.736)
(2583, 97.862)
(2584, 98.852)
(2585, 98.91)
(2586, 98.364)
(2587, 95.09)
(2588, 92.81)
(2589, 97.138)
(2590, 97.992)
(2591, 97.496)
(2592, 96.586)
(2593, 97.46)
(2594, 97.872)
(2595, 98.766)
(2596, 98.062)
(2597, 93.804)
(2598, 98.23)
(2599, 98.902)
(2600, 98.31)
(2601, 98.52)
(2602, 98.042)
(2603, 98.496)
(2604, 96.612)
(2605, 98.068)
(2606, 98.256)
(2607, 97.412)
(2608, 98.686)
(2609, 98.496)
(2610, 98.236)
(2611, 97.984)
(2612, 97.968)
(2613, 98.544)
(2614, 99.114)
(2615, 99.158)
(2616, 99.25)
(2617, 98.352)
(2618, 93.138)
(2619, 97.582)
(2620, 96.966)
(2621, 98.466)
(2622, 98.258)
(2623, 99.11)
(2624, 97.118)
(2625, 99.174)
(2626, 99.014)
(2627, 97.122)
(2628, 97.42)
(2629, 97.234)
(2630, 96.952)
(2631, 96.036)
(2632, 96.976)
(2633, 96.404)
(2634, 96.306)
(2635, 94.266)
(2636, 86.668)
(2637, 87.208)
(2638, 94.724)
(2639, 91.908)
(2640, 93.512)
(2641, 96.89)
(2642, 95.664)
(2643, 95.034)
(2644, 97.616)
(2645, 96.87)
(2646, 97.994)
(2647, 96.97)
(2648, 97.218)
(2649, 96.13)
(2650, 96.248)
(2651, 96.888)
(2652, 94.766)
(2653, 96.13)
(2654, 96.686)
(2655, 95.844)
(2656, 97.008)
(2657, 98.056)
(2658, 96.992)
(2659, 97.026)
(2660, 97.812)
(2661, 97.416)
(2662, 97.324)
(2663, 98.122)
(2664, 97.754)
(2665, 97.784)
(2666, 97.95)
(2667, 96.408)
(2668, 94.66)
(2669, 96.172)
(2670, 94.41)
(2671, 97.044)
(2672, 96.698)
(2673, 97.528)
(2674, 98.08)
(2675, 96.588)
(2676, 97.396)
(2677, 95.55)
(2678, 96.76)
(2679, 98.222)
(2680, 97.052)
(2681, 96.536)
(2682, 98.332)
(2683, 98.784)
(2684, 98.008)
(2685, 97.974)
(2686, 97.84)
(2687, 98.648)
(2688, 97.088)
(2689, 95.63)
(2690, 95.298)
(2691, 95.042)
(2692, 96.55)
(2693, 96.006)
(2694, 97.546)
(2695, 95.602)
(2696, 96.456)
(2697, 98.076)
(2698, 93.712)
(2699, 96.058)
(2700, 96.082)
(2701, 95.794)
(2702, 95.784)
(2703, 94.18)
(2704, 88.476)
(2705, 94.93)
(2706, 95.712)
(2707, 91.76)
(2708, 87.164)
(2709, 93.99)
(2710, 96.074)
(2711, 93.382)
(2712, 89.708)
(2713, 86.488)
(2714, 89.656)
(2715, 83.396)
(2716, 78.856)
(2717, 79.79)
(2718, 83.878)
(2719, 90.046)
(2720, 92.166)
(2721, 83.848)
(2722, 68.816)
(2723, 72.996)
(2724, 84.976)
(2725, 82.21)
(2726, 56.362)
(2727, 76.776)
(2728, 72.674)
(2729, 87.604)
(2730, 89.812)
(2731, 89.47)
(2732, 90.7)
(2733, 94.028)
(2734, 89.726)
(2735, 92.43)
(2736, 94.818)
(2737, 95.122)
(2738, 93.016)
(2739, 95.938)
(2740, 94.03)
(2741, 92.61)
(2742, 77.184)
(2743, 92.676)
(2744, 89.084)
(2745, 89.59)
(2746, 76.844)
(2747, 82.172)
(2748, 83.584)
(2749, 76.63)
(2750, 85.476)
(2751, 90.744)
(2752, 91.926)
(2753, 87.956)
(2754, 83.74)
(2755, 93.714)
(2756, 93.94)
(2757, 89.62)
(2758, 89.308)
(2759, 96.558)
(2760, 93.754)
(2761, 91.572)
(2762, 96.732)
(2763, 95.884)
(2764, 94.692)
(2765, 73.84)
(2766, 93.286)
(2767, 90.06)
(2768, 92.842)
(2769, 96.552)
(2770, 95.156)
(2771, 95.24)
(2772, 96.156)
(2773, 97.072)
(2774, 96.412)
(2775, 96.93)
(2776, 95.926)
(2777, 98.09)
(2778, 95.38)
(2779, 97.358)
(2780, 97.48)
(2781, 98.052)
(2782, 96.954)
(2783, 97.236)
(2784, 97.848)
(2785, 97.97)
(2786, 97.33)
(2787, 98.266)
(2788, 99.608)
(2789, 98.798)
(2790, 98.532)
(2791, 97.122)
(2792, 95.706)
(2793, 95.73)
(2794, 94.946)
(2795, 96.186)
(2796, 96.34)
(2797, 97.144)
(2798, 94.084)
(2799, 96.252)
(2800, 93.156)
(2801, 92.612)
(2802, 95.014)
(2803, 92.736)
(2804, 95.432)
(2805, 96.598)
(2806, 95.73)
(2807, 97.39)
(2808, 93.13)
(2809, 95.51)
(2810, 96.42)
(2811, 97.884)
(2812, 94.29)
(2813, 96.632)
(2814, 96.534)
(2815, 93.998)
(2816, 96.912)
(2817, 94.698)
(2818, 96.916)
(2819, 97.56)
(2820, 94.406)
(2821, 96.12)
(2822, 95.154)
(2823, 94.006)
(2824, 91.5)
(2825, 89.684)
(2826, 70.182)
(2827, 65.052)
(2828, 55.818)
(2829, 70.182)
(2830, 89.394)
(2831, 68.702)
(2832, 76.038)
(2833, 58.924)
(2834, 62.972)
(2835, 44.066)
(2836, 70.752)
(2837, 61.324)
(2838, 47.074)
(2839, 52.242)
(2840, 31.576)
(2841, 66.164)
(2842, 53.552)
(2843, 67.092)
(2844, 71.918)
(2845, 84.58)
(2846, 71.182)
(2847, 64.734)
(2848, 84.718)
(2849, 75.094)
(2850, 61.862)
(2851, 78.212)
(2852, 82.722)
(2853, 82.798)
(2854, 63.072)
(2855, 12.552)
(2856, 31.454)
(2857, 82.054)
(2858, 83.624)
(2859, 76.886)
(2860, 83.648)
(2861, 87.542)
(2862, 82.76)
(2863, 88.892)
(2864, 88.954)
(2865, 90.326)
(2866, 92.944)
(2867, 90.188)
(2868, 84.398)
(2869, 89.262)
(2870, 74.974)
(2871, 67.746)
(2872, 58.15)
(2873, 47.73)
(2874, 78.968)
(2875, 52.368)
(2876, 54.6)
(2877, 49.76)
(2878, 50.836)
(2879, 64.97)
(2880, 59.386)
(2881, 56.718)
(2882, 38.248)
(2883, 32.35)
(2884, 65.582)
(2885, 28.404)
(2886, 62.164)
(2887, 73.53)
(2888, 67.8)
(2889, 55.824)
(2890, 41.024)
(2891, 38.226)
(2892, 27.712)
(2893, 38.468)
(2894, 53.414)
(2895, 49.02)
(2896, 34.954)
(2897, 59.252)
(2898, 59.548)
(2899, 41.242)
(2900, 16.7)
(2901, 47.134)
(2902, 23.604)
(2903, 16.648)
(2904, 8.052)
(2905, 12.87)
(2906, 27.122)
(2907, 9.702)
(2908, 13.71)
(2909, 6.916)
(2910, 16.946)
(2911, 4.556)
(2912, 15.212)
(2913, 16.76)
(2914, 26.706)
(2915, 3.306)
(2916, 0)
(2917, 10.64)
(2918, 25.444)
(2919, 34.96)
(2920, 25.944)
(2921, 13.602)
(2922, 57.244)
(2923, 50.064)
(2924, 32.364)
(2925, 61.434)
(2926, 79.632)
(2927, 74.608)
(2928, 63.71)
(2929, 54.764)
(2930, 80.356)
(2931, 92.19)
(2932, 99.778)
(2933, 92.728)
(2934, 95.576)
(2935, 96.22)
(2936, 68.64)
(2937, 90.498)
(2938, 92.576)
(2939, 91.332)
(2940, 92.54)
(2941, 87.124)
(2942, 87.904)
(2943, 86.016)
(2944, 95.386)
(2945, 92.22)
(2946, 93.964)
(2947, 96.782)
(2948, 97.648)
(2949, 97.522)
(2950, 95.656)
(2951, 97.794)
(2952, 95.718)
(2953, 97.178)
(2954, 96.616)
(2955, 95.366)
(2956, 93.46)
(2957, 95.438)
(2958, 95.394)
(2959, 89.164)
(2960, 94.196)
(2961, 95.684)
(2962, 95.436)
(2963, 91.876)
(2964, 94.646)
(2965, 95.464)
(2966, 92.582)
(2967, 91.318)
(2968, 94.768)
(2969, 95.362)
(2970, 93.966)
(2971, 96.732)
(2972, 96.82)
(2973, 96.61)
(2974, 95.026)
(2975, 96.75)
(2976, 97.118)
(2977, 98.322)
(2978, 96.638)
(2979, 97.684)
(2980, 97.774)
(2981, 97.332)
(2982, 94.756)
(2983, 95.208)
(2984, 97.486)
(2985, 97.892)
(2986, 97.71)
(2987, 97.482)
(2988, 96.818)
(2989, 97.152)
(2990, 96.702)
(2991, 96.726)
(2992, 95.422)
(2993, 98.446)
(2994, 97.866)
(2995, 98.054)
(2996, 97.582)
(2997, 96.26)
(2998, 95.254)
(2999, 98)
(3000, 98.504)
(3001, 97.968)
(3002, 98.27)
(3003, 98.818)
(3004, 97.362)
(3005, 95.04)
(3006, 95.874)
(3007, 96.03)
(3008, 98.336)
(3009, 97.156)
(3010, 98.048)
(3011, 97.1)
(3012, 96.142)
(3013, 98.558)
(3014, 98.624)
(3015, 98.878)
(3016, 97.238)
(3017, 96.806)
(3018, 97.472)
(3019, 96.438)
(3020, 97.654)
(3021, 97.344)
(3022, 98.092)
(3023, 96.676)
(3024, 97.378)
(3025, 96.444)
(3026, 97.424)
(3027, 98.002)
(3028, 97.478)
(3029, 98.34)
(3030, 98.816)
(3031, 97.684)
(3032, 98.162)
(3033, 97.44)
(3034, 97.31)
(3035, 97.136)
(3036, 91.014)
(3037, 99.432)
(3038, 98.56)
(3039, 97.544)
(3040, 96.986)
(3041, 94.706)
(3042, 98.636)
(3043, 96.932)
(3044, 98.204)
(3045, 97.584)
(3046, 96.094)
(3047, 96.174)
(3048, 97.94)
(3049, 98.358)
(3050, 98.92)
(3051, 96.868)
(3052, 80.256)
(3053, 87.166)
(3054, 92.324)
(3055, 98.638)
(3056, 99.21)
(3057, 99.402)
(3058, 99.574)
(3059, 88.884)
(3060, 86.548)
(3061, 94.394)
(3062, 99.34)
(3063, 99.448)
(3064, 98.702)
(3065, 99.092)
(3066, 99.368)
(3067, 99.07)
(3068, 98.902)
(3069, 99.028)
(3070, 96.078)
(3071, 97.71)
(3072, 97.924)
(3073, 91.6)
(3074, 96.664)
(3075, 96.83)
(3076, 97.04)
(3077, 95.5)
(3078, 96.754)
(3079, 91.136)
(3080, 90.252)
(3081, 97.282)
(3082, 97.212)
(3083, 99.006)
(3084, 99.21)
(3085, 99.314)
(3086, 99.554)
(3087, 99.042)
(3088, 98.064)
(3089, 99.064)
(3090, 97.648)
(3091, 98.02)
(3092, 97.932)
(3093, 97.386)
(3094, 97.664)
(3095, 96.058)
(3096, 98.454)
(3097, 94.984)
(3098, 98.036)
(3099, 98.824)
(3100, 99.126)
(3101, 98.532)
(3102, 95.68)
(3103, 97.262)
(3104, 93.348)
(3105, 96.22)
(3106, 91.836)
(3107, 97.954)
(3108, 98.446)
(3109, 94.248)
(3110, 93.824)
(3111, 93)
(3112, 92.696)
(3113, 94.158)
(3114, 82.09)
(3115, 66.544)
(3116, 0)
(3117, 0)
(3118, 0)
(3119, 7.444)
(3120, 7.564)
(3121, 0)
(3122, 0)
(3123, 3.64)
(3124, 1.19)
(3125, 18.062)
(3126, 10.1)
(3127, 0)
(3128, 0)
(3129, 0.006)
(3130, 8.808)
(3131, 0)
(3132, 0)
(3133, 5.112)
(3134, 0)
(3135, 11.978)
(3136, 0)
(3137, 49.852)
(3138, 74.304)
(3139, 58.074)
(3140, 6.244)
(3141, 71.59)
(3142, 70.348)
(3143, 80.272)
(3144, 91.44)
(3145, 89.26)
(3146, 88.85)
(3147, 92.482)
(3148, 88.044)
(3149, 89.322)
(3150, 92.564)
(3151, 93.062)
(3152, 94.002)
(3153, 96.53)
(3154, 94.786)
(3155, 96.306)
(3156, 97.312)
(3157, 95.898)
(3158, 95.972)
(3159, 90.734)
(3160, 96.466)
(3161, 97.464)
(3162, 97.428)
(3163, 98.244)
(3164, 97.92)
(3165, 96.118)
(3166, 95.91)
(3167, 97.288)
(3168, 97.358)
(3169, 97.916)
(3170, 97.214)
(3171, 97.998)
(3172, 98.404)
(3173, 98.248)
(3174, 98.162)
(3175, 98.564)
(3176, 98.038)
(3177, 98.48)
(3178, 90.584)
(3179, 97.706)
(3180, 96.902)
(3181, 97.648)
(3182, 93.994)
(3183, 92.338)
(3184, 87.868)
(3185, 88.07)
(3186, 89.08)
(3187, 94.95)
(3188, 94.852)
(3189, 94.884)
(3190, 93.512)
(3191, 87.54)
(3192, 93.064)
(3193, 86.906)
(3194, 85.752)
(3195, 84.228)
(3196, 82.912)
(3197, 66.932)
(3198, 91.86)
(3199, 80.184)
(3200, 62.234)
(3201, 74.874)
(3202, 34.064)
(3203, 17.118)
(3204, 41.766)
(3205, 52.32)
(3206, 63.45)
(3207, 60.88)
(3208, 80.426)
(3209, 74.504)
(3210, 87.054)
(3211, 80.436)
(3212, 90.93)
(3213, 88.272)
(3214, 87.596)
(3215, 82.74)
(3216, 84.762)
(3217, 90.816)
(3218, 85.152)
(3219, 84.176)
(3220, 62.976)
(3221, 76.132)
(3222, 78.46)
(3223, 63.16)
(3224, 61.944)
(3225, 77.266)
(3226, 78.082)
(3227, 78.228)
(3228, 89.532)
(3229, 73.866)
(3230, 69.348)
(3231, 75.93)
(3232, 59.624)
(3233, 66.834)
(3234, 67.2)
(3235, 43.526)
(3236, 75.23)
(3237, 44.256)
(3238, 65.478)
(3239, 47.764)
(3240, 37.976)
(3241, 45.328)
(3242, 48.888)
(3243, 70.99)
(3244, 56.05)
(3245, 66.258)
(3246, 27.51)
(3247, 58.336)
(3248, 33.042)
(3249, 5.106)
(3250, 27.83)
(3251, 16.108)
(3252, 41.888)
(3253, 51.174)
(3254, 23.282)
(3255, 31.412)
(3256, 13.702)
(3257, 7.052)
(3258, 14.22)
(3259, 84.114)
(3260, 84.982)
(3261, 54.608)
(3262, 81.174)
(3263, 61.278)
(3264, 76.27)
(3265, 81.214)
(3266, 51.186)
(3267, 66.82)
(3268, 58.768)
(3269, 58.932)
(3270, 88.878)
(3271, 81.586)
(3272, 87.398)
(3273, 82.998)
(3274, 81.364)
(3275, 99.996)
(3276, 99.98)
(3277, 100)
(3278, 100)
(3279, 100)
(3280, 86.306)
(3281, 69.684)
(3282, 63.73)
(3283, 77.05)
(3284, 39.626)
(3285, 67.752)
(3286, 82.592)
(3287, 91.18)
(3288, 83.182)
(3289, 78.694)
(3290, 72.898)
(3291, 70.89)
(3292, 90.624)
(3293, 84.556)
(3294, 66.746)
(3295, 72.348)
(3296, 68.318)
(3297, 88.214)
(3298, 92.114)
(3299, 93.002)
(3300, 90.826)
(3301, 91.846)
(3302, 85.772)
(3303, 90.378)
(3304, 87.42)
(3305, 91.828)
(3306, 91.056)
(3307, 91.926)
(3308, 93.82)
(3309, 94.662)
(3310, 94.942)
(3311, 88.496)
(3312, 80.658)
(3313, 81.258)
(3314, 85.232)
(3315, 89.45)
(3316, 79.648)
(3317, 87.714)
(3318, 71.34)
(3319, 79.932)
(3320, 93.86)
(3321, 87.862)
(3322, 74.586)
(3323, 88.454)
(3324, 92.484)
(3325, 87.316)
(3326, 93.192)
(3327, 83.222)
(3328, 92.22)
(3329, 89.674)
(3330, 95.096)
(3331, 88.714)
(3332, 86.25)
(3333, 89.422)
(3334, 80.466)
(3335, 86.52)
(3336, 93.602)
(3337, 90.716)
(3338, 89.754)
(3339, 90.336)
(3340, 88.814)
(3341, 82.62)
(3342, 85)
(3343, 95.896)
(3344, 92.572)
(3345, 88.674)
(3346, 95.058)
(3347, 83.856)
(3348, 93.004)
(3349, 89.926)
(3350, 88.008)
(3351, 93.926)
(3352, 94.94)
(3353, 92.866)
(3354, 85.674)
(3355, 85.78)
(3356, 91.692)
(3357, 93.19)
(3358, 90.348)
(3359, 92.014)
(3360, 94.98)
(3361, 95.282)
(3362, 92.394)
(3363, 91.04)
(3364, 91.314)
(3365, 82.53)
(3366, 92.618)
(3367, 91.754)
(3368, 90.136)
(3369, 85.472)
(3370, 91.964)
(3371, 92.218)
(3372, 91.476)
(3373, 92.166)
(3374, 91.822)
(3375, 93.194)
(3376, 92.84)
(3377, 92.502)
(3378, 93.92)
(3379, 87.086)
(3380, 91.962)
(3381, 90.77)
(3382, 88.592)
(3383, 82.41)
(3384, 56.896)
(3385, 85.898)
(3386, 83.494)
(3387, 86.72)
(3388, 73.922)
(3389, 86.222)
(3390, 86.198)
(3391, 88.418)
(3392, 88.852)
(3393, 80.77)
(3394, 84.794)
(3395, 71.322)
(3396, 50.716)
(3397, 86.698)
(3398, 87.17)
(3399, 65.422)
(3400, 83.008)
(3401, 79.166)
(3402, 79.958)
(3403, 66.082)
(3404, 92.182)
(3405, 94.254)
(3406, 88.218)
(3407, 78.742)
(3408, 72.452)
(3409, 77.77)
(3410, 76.432)
(3411, 78.63)
(3412, 76.662)
(3413, 42.028)
(3414, 76.56)
(3415, 88.798)
(3416, 78.022)
(3417, 88.868)
(3418, 90.226)
(3419, 92.124)
(3420, 95.89)
(3421, 93.978)
(3422, 86.488)
(3423, 91.436)
(3424, 88.642)
(3425, 92.728)
(3426, 84.556)
(3427, 89.76)
(3428, 90.562)
(3429, 90.232)
(3430, 85.832)
(3431, 81.244)
(3432, 92.99)
(3433, 83.366)
(3434, 84.878)
(3435, 94.69)
(3436, 87.74)
(3437, 93.56)
(3438, 92.834)
(3439, 86.3)
(3440, 88.886)
(3441, 87.864)
(3442, 90.164)
(3443, 75.728)
(3444, 75.584)
(3445, 80.302)
(3446, 81.668)
(3447, 81.366)
(3448, 91.542)
(3449, 66.22)
(3450, 79.328)
(3451, 87.508)
(3452, 88.728)
(3453, 70.908)
(3454, 49.692)
(3455, 45.916)
(3456, 83.56)
(3457, 68.154)
(3458, 81.78)
(3459, 89.17)
(3460, 86.078)
(3461, 83.986)
(3462, 91.124)
(3463, 87.808)
(3464, 96.678)
(3465, 93.5)
(3466, 95.882)
(3467, 94.654)
(3468, 94.656)
(3469, 84.45)
(3470, 91.996)
(3471, 95.386)
(3472, 89.604)
(3473, 84.492)
(3474, 92.72)
(3475, 90.496)
(3476, 90.144)
(3477, 92.516)
(3478, 94.308)
(3479, 94.156)
(3480, 95.672)
(3481, 95.056)
(3482, 95.734)
(3483, 89.386)
(3484, 90.746)
(3485, 87.958)
(3486, 92.322)
(3487, 87.874)
(3488, 89.75)
(3489, 87.92)
(3490, 83.466)
(3491, 87.288)
(3492, 87.912)
(3493, 77.832)
(3494, 74.014)
(3495, 78.17)
(3496, 58.702)
(3497, 54.912)
(3498, 39.842)
(3499, 49.38)
(3500, 59.038)
(3501, 33.704)
(3502, 21.498)
(3503, 30.968)
(3504, 11.882)
(3505, 36.486)
(3506, 4.748)
(3507, 6.972)
(3508, 0)
(3509, 0)
(3510, 0)
(3511, 0)
(3512, 0)
(3513, 2.806)
(3514, 2.45)
(3515, 0)
(3516, 0)
(3517, 0)
(3518, 0)
(3519, 0)
(3520, 0)
(3521, 0)
(3522, 0)
(3523, 0)
(3524, 0)
(3525, 4.16)
(3526, 2.84)
(3527, 0.24)
(3528, 0)
(3529, 0)
(3530, 0)
(3531, 0)
(3532, 0)
(3533, 0)
(3534, 0)
(3535, 0)
(3536, 0)
(3537, 0)
(3538, 0)
(3539, 0)
(3540, 0)
(3541, 0)
(3542, 0)
(3543, 0)
(3544, 0)
(3545, 0)
(3546, 0)
(3547, 0)
(3548, 0)
(3549, 0)
(3550, 5.112)
(3551, 0)
(3552, 0)
(3553, 0)
(3554, 0)
(3555, 0)
(3556, 0)
(3557, 0)
(3558, 0)
(3559, 0)
(3560, 0)
(3561, 4.16)
(3562, 0)
(3563, 0)
(3564, 0)
(3565, 6.806)
(3566, 0)
(3567, 0)
(3568, 0)
(3569, 0)
(3570, 0)
(3571, 6.03)
(3572, 1.98)
(3573, 0)
(3574, 0)
(3575, 4.97)
(3576, 0)
(3577, 0)
(3578, 0)
(3579, 0)
(3580, 0)
(3581, 0)
(3582, 0)
(3583, 22.002)
(3584, 0.002)
(3585, 0)
(3586, 0)
(3587, 0)
(3588, 0)
(3589, 6.8)
(3590, 4.106)
(3591, 0.87)
(3592, 0)
(3593, 0)
(3594, 0)
(3595, 7.656)
(3596, 0)
(3597, 0)
(3598, 0)
(3599, 0)
(3600, 0)
(3601, 8.742)
(3602, 0)
(3603, 0)
(3604, 0)
(3605, 0)
(3606, 0)
(3607, 0)
(3608, 4.826)
(3609, 9.29)
(3610, 0)
(3611, 0)
(3612, 0)
(3613, 0)
(3614, 0)
(3615, 0)
(3616, 0)
(3617, 9.312)
(3618, 0)
(3619, 0)
(3620, 0)
(3621, 0)
(3622, 0)
(3623, 3.192)
(3624, 0)
(3625, 0)
(3626, 0)
(3627, 0)
(3628, 0)
(3629, 0)
(3630, 1.56)
(3631, 0)
(3632, 0)
(3633, 0)
(3634, 0)
(3635, 0)
(3636, 0)
(3637, 9.702)
(3638, 0)
(3639, 0)
(3640, 0)
(3641, 0)
(3642, 0)
(3643, 0)
(3644, 0)
(3645, 0)
(3646, 0)
(3647, 0)
(3648, 0)
(3649, 0)
(3650, 0)
(3651, 0)
(3652, 0)
(3653, 0)
(3654, 0)
(3655, 0)
(3656, 0)
(3657, 0)
(3658, 0)
(3659, 0)
(3660, 0)
(3661, 0)
(3662, 0)
(3663, 4.556)
(3664, 0)
(3665, 0)
(3666, 0)
(3667, 0)
(3668, 0)
(3669, 0)
(3670, 0)
(3671, 0)
(3672, 0)
(3673, 0)
(3674, 0)
(3675, 0)
(3676, 0)
(3677, 0)
(3678, 0)
(3679, 3.306)
(3680, 0)
(3681, 1.19)
(3682, 2.97)
(3683, 0)
(3684, 8.372)
(3685, 0)
(3686, 5.7)
(3687, 0)
(3688, 0)
(3689, 0)
(3690, 0)
(3691, 8.556)
(3692, 0)
(3693, 0)
(3694, 0)
(3695, 4.97)
(3696, 0)
(3697, 0)
(3698, 0)
(3699, 0)
(3700, 0)
(3701, 5.148)
(3702, 9.342)
(3703, 38.056)
(3704, 0.38)
(3705, 6.48)
(3706, 3.192)
(3707, 7.14)
(3708, 0)
(3709, 0)
(3710, 0)
(3711, 0)
(3712, 0)
(3713, 0)
(3714, 0)
(3715, 0)
(3716, 0)
(3717, 0)
(3718, 1.032)
(3719, 10.302)
(3720, 13.838)
(3721, 0)
(3722, 0)
(3723, 0)
(3724, 0)
(3725, 7.562)
(3726, 23.116)
(3727, 43.242)
(3728, 27.438)
(3729, 27.568)
(3730, 38.918)
(3731, 36.254)
(3732, 33.228)
(3733, 64.588)
(3734, 35.16)
(3735, 31.264)
(3736, 30.558)
(3737, 64.952)
(3738, 77.084)
(3739, 77.988)
(3740, 56.266)
(3741, 34.542)
(3742, 57.04)
(3743, 33.194)
(3744, 67.568)
(3745, 30.602)
(3746, 37.572)
(3747, 43.344)
(3748, 24.512)
(3749, 38.614)
(3750, 8.982)
(3751, 40.762)
(3752, 60.196)
(3753, 59.646)
(3754, 58.634)
(3755, 67.216)
(3756, 64.922)
(3757, 57.566)
(3758, 63.258)
(3759, 41.12)
(3760, 54.112)
(3761, 69.878)
(3762, 88.744)
(3763, 62.786)
(3764, 70.004)
(3765, 84.132)
(3766, 73.788)
(3767, 90.584)
(3768, 81.686)
(3769, 83.916)
(3770, 85.552)
(3771, 86.296)
(3772, 80.618)
(3773, 85.88)
(3774, 81.482)
(3775, 83.426)
(3776, 59.672)
(3777, 58.27)
(3778, 62.104)
(3779, 68.29)
(3780, 86.418)
(3781, 77.202)
(3782, 77.718)
(3783, 89.842)
(3784, 93.932)
(3785, 93.672)
(3786, 90.874)
(3787, 92.408)
(3788, 89.032)
(3789, 92.902)
(3790, 92.142)
(3791, 88.468)
(3792, 93.924)
(3793, 93.54)
(3794, 95.604)
(3795, 91.856)
(3796, 91.358)
(3797, 93.15)
(3798, 93.956)
(3799, 97.302)
(3800, 95.48)
(3801, 96.498)
(3802, 98.126)
(3803, 97.852)
(3804, 94.628)
(3805, 97.67)
(3806, 98.696)
(3807, 96.58)
(3808, 97.186)
(3809, 96.722)
(3810, 98.65)
(3811, 99.402)
(3812, 99.454)
(3813, 99.392)
(3814, 99.328)
(3815, 98.916)
(3816, 98.39)
(3817, 97.132)
(3818, 95.02)
(3819, 96.516)
(3820, 96.554)
(3821, 98.49)
(3822, 96.042)
(3823, 95.024)
(3824, 97.552)
(3825, 97.048)
(3826, 95.282)
(3827, 96.554)
(3828, 97.52)
(3829, 95.67)
(3830, 96.632)
(3831, 95.302)
(3832, 95.654)
(3833, 94.73)
(3834, 94.014)
(3835, 96.648)
(3836, 97.08)
(3837, 96.97)
(3838, 96.708)
(3839, 95.564)
(3840, 98.276)
(3841, 98.414)
(3842, 98.692)
(3843, 98.288)
(3844, 97.28)
(3845, 98.148)
(3846, 98.348)
(3847, 98.526)
(3848, 97.7)
(3849, 97.862)
(3850, 98.766)
(3851, 97.728)
(3852, 98.088)
(3853, 98.756)
(3854, 98.144)
(3855, 98.31)
(3856, 98.58)
(3857, 98.142)
(3858, 98.266)
(3859, 97.93)
(3860, 97.302)
(3861, 97.662)
(3862, 98.138)
(3863, 96.536)
(3864, 97.578)
(3865, 98.636)
(3866, 98.934)
(3867, 98.74)
(3868, 98.792)
(3869, 98.866)
(3870, 98.306)
(3871, 98.672)
(3872, 98.04)
(3873, 98.078)
(3874, 98.612)
(3875, 98.184)
(3876, 97.834)
(3877, 99.094)
(3878, 98.258)
(3879, 99.394)
(3880, 99.06)
(3881, 99.37)
(3882, 99.362)
(3883, 98.608)
(3884, 98.69)
(3885, 99.084)
(3886, 98.188)
(3887, 99.076)
(3888, 99.85)
(3889, 98.816)
(3890, 97.99)
(3891, 98.812)
(3892, 98.058)
(3893, 98.582)
(3894, 98.044)
(3895, 98.96)
(3896, 98.634)
(3897, 98.764)
(3898, 98.728)
(3899, 97.81)
(3900, 99.478)
(3901, 99.474)
(3902, 99.52)
(3903, 98.456)
(3904, 99.258)
(3905, 99.432)
(3906, 99.692)
(3907, 97.838)
(3908, 99.538)
(3909, 98.712)
(3910, 97.688)
(3911, 99.548)
(3912, 98.876)
(3913, 97.656)
(3914, 98.99)
(3915, 99.304)
(3916, 98.706)
(3917, 99.214)
(3918, 99.284)
(3919, 99.52)
(3920, 99.936)
(3921, 99.204)
(3922, 98.696)
(3923, 99.164)
(3924, 98.47)
(3925, 98.812)
(3926, 98.62)
(3927, 99.08)
(3928, 99.328)
(3929, 98.7)
(3930, 99.078)
(3931, 97.93)
(3932, 98.952)
(3933, 97.634)
(3934, 98.718)
(3935, 96.29)
(3936, 97.496)
(3937, 98.91)
(3938, 95.73)
(3939, 96.924)
(3940, 99.406)
(3941, 99.102)
(3942, 98.828)
(3943, 97.034)
(3944, 98.608)
(3945, 97.396)
(3946, 98.844)
(3947, 97.838)
(3948, 98.754)
(3949, 97.922)
(3950, 98.118)
(3951, 99.254)
(3952, 99.612)
(3953, 98.798)
(3954, 99.226)
(3955, 99.73)
(3956, 99.4)
(3957, 99.444)
(3958, 98.11)
(3959, 98.206)
(3960, 99.332)
(3961, 99.406)
(3962, 99.378)
(3963, 99.354)
(3964, 98.802)
(3965, 99.39)
(3966, 99.13)
(3967, 96.944)
(3968, 99.38)
(3969, 99.874)
(3970, 99.744)
(3971, 99.648)
(3972, 99.606)
(3973, 99.792)
(3974, 99.464)
(3975, 99.318)
(3976, 99.394)
(3977, 99.458)
(3978, 99.084)
(3979, 99.582)
(3980, 99.074)
(3981, 98.82)
(3982, 99.032)
(3983, 98.118)
(3984, 99.528)
(3985, 99.72)
(3986, 99.232)
(3987, 99.688)
(3988, 99.432)
(3989, 99.396)
(3990, 97.962)
(3991, 99.056)
(3992, 96.202)
(3993, 99.066)
(3994, 99.278)
(3995, 98.998)
(3996, 99.636)
(3997, 99.538)
(3998, 99.288)
(3999, 98.788)
(4000, 99.696)
(4001, 99.778)
(4002, 99.63)
(4003, 99.678)
(4004, 99.154)
(4005, 99.388)
(4006, 99.49)
(4007, 99.678)
(4008, 99.462)
(4009, 99.856)
(4010, 99.476)
(4011, 98.728)
(4012, 99.672)
(4013, 98.218)
(4014, 99.578)
(4015, 99.864)
(4016, 99.576)
(4017, 99.954)
(4018, 99.976)
(4019, 99.994)
(4020, 99.984)
(4021, 99.716)
(4022, 99.564)
(4023, 99.558)
(4024, 99.614)
(4025, 98.908)
(4026, 97.018)
(4027, 99.134)
(4028, 99.284)
(4029, 99.084)
(4030, 98.992)
(4031, 98.974)
(4032, 99.826)
(4033, 99.658)
(4034, 99.674)
(4035, 99.796)
(4036, 99.71)
(4037, 99.778)
(4038, 99.67)
(4039, 99.696)
(4040, 99.912)
(4041, 99.87)
(4042, 99.972)
(4043, 99.998)
(4044, 100)
(4045, 99.992)
(4046, 99.994)
(4047, 99.956)
(4048, 99.94)
(4049, 99.978)
(4050, 99.994)
(4051, 100)
(4052, 99.972)
(4053, 99.718)
(4054, 99.828)
(4055, 99.32)
(4056, 99.77)
(4057, 99.712)
(4058, 99.802)
(4059, 99.728)
(4060, 99.878)
(4061, 99.756)
(4062, 99.922)
(4063, 99.958)
(4064, 99.99)
(4065, 99.994)
(4066, 99.986)
(4067, 99.97)
(4068, 99.808)
(4069, 99.95)
(4070, 100)
(4071, 99.99)
(4072, 99.962)
(4073, 99.982)
(4074, 99.942)
(4075, 99.486)
(4076, 99.472)
(4077, 99.944)
(4078, 99.984)
(4079, 99.996)
(4080, 99.988)
(4081, 99.998)
(4082, 99.978)
(4083, 99.98)
(4084, 99.996)
(4085, 99.994)
(4086, 99.952)
(4087, 99.818)
(4088, 99.752)
(4089, 99.88)
(4090, 99.998)
(4091, 99.948)
(4092, 99.916)
(4093, 99.198)
(4094, 100)
(4095, 99.968)
(4096, 99.998)
(4097, 99.982)
(4098, 99.996)
(4099, 99.996)
(4100, 100)
(4101, 100)
(4102, 100)
(4103, 99.956)
(4104, 99.998)
(4105, 100)
(4106, 100)
(4107, 99.962)
(4108, 99.984)
(4109, 100)
(4110, 100)
(4111, 100)
(4112, 99.982)
(4113, 99.996)
(4114, 99.948)
(4115, 100)
(4116, 99.996)
(4117, 99.996)
(4118, 99.978)
(4119, 99.98)
(4120, 99.996)
(4121, 99.934)
(4122, 99.984)
(4123, 99.932)
(4124, 99.958)
(4125, 97.942)
(4126, 99.888)
(4127, 99.956)
(4128, 89.818)
(4129, 90.488)
(4130, 89.268)
(4131, 99.998)
(4132, 99.912)
(4133, 99.88)
(4134, 99.812)
(4135, 92.832)
(4136, 99.85)
(4137, 98.05)
(4138, 97.634)
(4139, 98.564)
(4140, 98.128)
(4141, 97.13)
(4142, 99.452)
(4143, 98.518)
(4144, 99.198)
(4145, 99.704)
(4146, 99.834)
(4147, 99.98)
(4148, 99.81)
(4149, 99.872)
(4150, 99.184)
(4151, 99.888)
(4152, 99.992)
(4153, 99.99)
(4154, 99.992)
(4155, 99.972)
(4156, 99.938)
(4157, 99.978)
(4158, 99.952)
(4159, 99.988)
(4160, 99.89)
(4161, 99.942)
(4162, 99.964)
(4163, 99.898)
(4164, 99.89)
(4165, 99.894)
(4166, 99.816)
(4167, 99.906)
(4168, 99.734)
(4169, 99.796)
(4170, 99.854)
(4171, 99.732)
(4172, 99.748)
(4173, 99.738)
(4174, 99.918)
(4175, 99.91)
(4176, 98.552)
(4177, 99.316)
(4178, 98.518)
(4179, 97.624)
(4180, 98.718)
(4181, 98.484)
(4182, 99.51)
(4183, 99.576)
(4184, 99.668)
(4185, 98.916)
(4186, 98.968)
(4187, 99.428)
(4188, 99.702)
(4189, 97.068)
(4190, 99.88)
(4191, 99.986)
(4192, 99.958)
(4193, 99.89)
(4194, 99.99)
(4195, 99.954)
(4196, 99.926)
(4197, 99.896)
(4198, 99.978)
(4199, 99.922)
(4200, 98.718)
(4201, 98.132)
(4202, 100)
(4203, 99.994)
(4204, 99.992)
(4205, 99.986)
(4206, 99.986)
(4207, 99.992)
(4208, 99.972)
(4209, 99.994)
(4210, 99.988)
(4211, 99.974)
(4212, 99.96)
(4213, 99.958)
(4214, 99.946)
(4215, 99.966)
(4216, 99.794)
(4217, 99.702)
(4218, 99.646)
(4219, 99.674)
(4220, 99.746)
(4221, 99.704)
(4222, 99.6)
(4223, 98.096)
(4224, 98.212)
(4225, 99.718)
(4226, 99.228)
(4227, 98.212)
(4228, 97.898)
(4229, 98.028)
(4230, 98.546)
(4231, 98.766)
(4232, 96.34)
(4233, 96.866)
(4234, 98.1)
(4235, 98)
(4236, 97.596)
(4237, 96.214)
(4238, 96.296)
(4239, 97.106)
(4240, 97.816)
(4241, 97.724)
(4242, 97.998)
(4243, 97.578)
(4244, 91.346)
(4245, 94.242)
(4246, 96.44)
(4247, 94.128)
(4248, 93.694)
(4249, 94.868)
(4250, 96.568)
(4251, 96.864)
(4252, 98.388)
(4253, 98.48)
(4254, 98.322)
(4255, 99.15)
(4256, 98.742)
(4257, 97.952)
(4258, 96.036)
(4259, 96.982)
(4260, 94.538)
(4261, 97.826)
(4262, 98.122)
(4263, 97.906)
(4264, 97.328)
(4265, 97.704)
(4266, 96.788)
(4267, 95.48)
(4268, 97.392)
(4269, 95.11)
(4270, 98.318)
(4271, 99.096)
(4272, 97.406)
(4273, 97.076)
(4274, 97.528)
(4275, 97.132)
(4276, 97.154)
(4277, 95.53)
(4278, 95.984)
(4279, 88.558)
(4280, 97.108)
(4281, 98.258)
(4282, 98.446)
(4283, 95.436)
(4284, 97.234)
(4285, 97.744)
(4286, 97.854)
(4287, 97.534)
(4288, 98.73)
(4289, 97.462)
(4290, 92.518)
(4291, 94.742)
(4292, 92.018)
(4293, 95.256)
(4294, 97.668)
(4295, 96.458)
(4296, 98.416)
(4297, 98.136)
(4298, 99.35)
(4299, 95.13)
(4300, 97.936)
(4301, 98.598)
(4302, 99.246)
(4303, 98.744)
(4304, 91.836)
(4305, 98.488)
(4306, 95.96)
(4307, 92.934)
(4308, 98.074)
(4309, 98.168)
(4310, 96.4)
(4311, 96.256)
(4312, 93.77)
(4313, 93.726)
(4314, 93.922)
(4315, 96.664)
(4316, 97.026)
(4317, 97.098)
(4318, 93.68)
(4319, 96.144)
(4320, 98.002)
(4321, 99.138)
(4322, 98.082)
(4323, 96.634)
(4324, 97.812)
(4325, 98.804)
(4326, 99.45)
(4327, 99.37)
(4328, 98.444)
(4329, 99.496)
(4330, 99.532)
(4331, 99.702)
(4332, 99.804)
(4333, 99.394)
(4334, 99.414)
(4335, 99.562)
(4336, 99.666)
(4337, 91.944)
(4338, 91.724)
(4339, 98.316)
(4340, 99.394)
(4341, 99.636)
(4342, 93.026)
(4343, 99.014)
(4344, 99.23)
(4345, 99.57)
(4346, 99.368)
(4347, 98.638)
(4348, 99.06)
(4349, 97.84)
(4350, 98.994)
(4351, 98.87)
(4352, 99.072)
(4353, 99.104)
(4354, 99.194)
(4355, 99.276)
(4356, 99.208)
(4357, 98.074)
(4358, 97.412)
(4359, 96.522)
(4360, 99.318)
(4361, 99.36)
(4362, 98.43)
(4363, 99.248)
(4364, 98.68)
(4365, 97.81)
(4366, 98.514)
(4367, 99.408)
(4368, 99.482)
(4369, 99.642)
(4370, 99.566)
(4371, 99.854)
(4372, 99.842)
(4373, 99.572)
(4374, 99.564)
(4375, 91.936)
(4376, 99.68)
(4377, 99.69)
(4378, 99.616)
(4379, 99.488)
(4380, 99.298)
(4381, 99.156)
(4382, 99.03)
(4383, 98.808)
(4384, 99.03)
(4385, 98.534)
(4386, 98.562)
(4387, 97.974)
(4388, 98.176)
(4389, 99.53)
(4390, 99.586)
(4391, 99.42)
(4392, 99.594)
(4393, 98.542)
(4394, 98.68)
(4395, 97.924)
(4396, 98.948)
(4397, 96.51)
(4398, 98.956)
(4399, 96.896)
(4400, 99.644)
(4401, 99.506)
(4402, 99.668)
(4403, 99.672)
(4404, 99.896)
(4405, 99.438)
(4406, 98.85)
(4407, 97.49)
(4408, 99.448)
(4409, 97.654)
(4410, 98.706)
(4411, 98.404)
(4412, 99.192)
(4413, 98.882)
(4414, 94.44)
(4415, 97.954)
(4416, 98.738)
(4417, 99.256)
(4418, 99.968)
(4419, 99.814)
(4420, 99.676)
(4421, 99.904)
(4422, 99.804)
(4423, 99.76)
(4424, 99.22)
(4425, 99.782)
(4426, 99.49)
(4427, 98.692)
(4428, 98.944)
(4429, 98.17)
(4430, 99.472)
(4431, 98.372)
(4432, 97.558)
(4433, 95.324)
(4434, 97.26)
(4435, 99.34)
(4436, 98.9)
(4437, 99.07)
(4438, 98.784)
(4439, 99.388)
(4440, 97.792)
(4441, 98.616)
(4442, 99.284)
(4443, 98.524)
(4444, 99.432)
(4445, 96.496)
(4446, 99.406)
(4447, 99.606)
(4448, 99.27)
(4449, 98.514)
(4450, 99.216)
(4451, 98.474)
(4452, 98.034)
(4453, 99.708)
(4454, 87.706)
(4455, 98.504)
(4456, 99.29)
(4457, 99.884)
(4458, 98.282)
(4459, 99.774)
(4460, 99.558)
(4461, 99.53)
(4462, 99.918)
(4463, 99.896)
(4464, 99.744)
(4465, 99.58)
(4466, 99.786)
(4467, 99.714)
(4468, 99.796)
(4469, 99.694)
(4470, 99.826)
(4471, 99.96)
(4472, 99.898)
(4473, 99.924)
(4474, 99.92)
(4475, 99.896)
(4476, 99.902)
(4477, 99.676)
(4478, 99.93)
(4479, 99.772)
(4480, 97.908)
(4481, 99.646)
(4482, 99.938)
(4483, 99.942)
(4484, 99.594)
(4485, 99.73)
(4486, 99.874)
(4487, 99.092)
(4488, 99.694)
(4489, 99.884)
(4490, 99.496)
(4491, 99.694)
(4492, 99.88)
(4493, 99.912)
(4494, 99.474)
(4495, 99.856)
(4496, 99.3)
(4497, 99.82)
(4498, 99.748)
(4499, 99.852)
(4500, 99.856)
(4501, 99.172)
(4502, 99.77)
(4503, 99.918)
(4504, 99.716)
(4505, 99.32)
(4506, 99.88)
(4507, 99.97)
(4508, 99.844)
(4509, 99.736)
(4510, 99.87)
(4511, 99.796)
(4512, 99.158)
(4513, 99.826)
(4514, 99.988)
(4515, 99.648)
(4516, 99.076)
(4517, 98.92)
(4518, 99.038)
(4519, 99.19)
(4520, 99.664)
(4521, 98.368)
(4522, 99.462)
(4523, 99.82)
(4524, 99.138)
(4525, 99.188)
(4526, 99.61)
(4527, 99.524)
(4528, 99.92)
(4529, 99.592)
(4530, 98.696)
(4531, 99.86)
(4532, 99.718)
(4533, 99.86)
(4534, 99.972)
(4535, 99.99)
(4536, 99.988)
(4537, 99.846)
(4538, 99.96)
(4539, 99.896)
(4540, 99.904)
(4541, 99.898)
(4542, 99.944)
(4543, 99.74)
(4544, 99.59)
(4545, 99.82)
(4546, 99.852)
(4547, 99.274)
(4548, 99.794)
(4549, 99.652)
(4550, 99.91)
(4551, 99.984)
(4552, 99.976)
(4553, 99.042)
(4554, 98.488)
(4555, 99.078)
(4556, 99.908)
(4557, 99.36)
(4558, 99.948)
(4559, 99.804)
(4560, 99.538)
(4561, 99.934)
(4562, 99.942)
(4563, 99.982)
(4564, 99.85)
(4565, 99.794)
(4566, 99.93)
(4567, 99.986)
(4568, 99.928)
(4569, 99.94)
(4570, 99.776)
(4571, 99.99)
(4572, 99.934)
(4573, 99.89)
(4574, 98.804)
(4575, 98.244)
(4576, 99.958)
(4577, 99.838)
(4578, 99.8)
(4579, 99.35)
(4580, 97.118)
(4581, 99.284)
(4582, 98.712)
(4583, 99.194)
(4584, 99.198)
(4585, 98.688)
(4586, 99.554)
(4587, 99.01)
(4588, 98.578)
(4589, 98.382)
(4590, 98.32)
(4591, 99.424)
(4592, 99.078)
(4593, 98.338)
(4594, 98.882)
(4595, 98.284)
(4596, 95.82)
(4597, 98.626)
(4598, 98.07)
(4599, 99.23)
(4600, 98.842)
(4601, 90.962)
(4602, 98.292)
(4603, 99.406)
(4604, 98.626)
(4605, 83.65)
(4606, 98.488)
(4607, 99.436)
(4608, 98.11)
(4609, 99.388)
(4610, 99.158)
(4611, 98.674)
(4612, 99.452)
(4613, 99.19)
(4614, 96.772)
(4615, 98.89)
(4616, 99.506)
(4617, 95.586)
(4618, 99.232)
(4619, 99.796)
(4620, 99.528)
(4621, 99.902)
(4622, 99.93)
(4623, 99.658)
(4624, 99.45)
(4625, 99.65)
(4626, 99.838)
(4627, 99.892)
(4628, 99.932)
(4629, 99.936)
(4630, 99.696)
(4631, 99.42)
(4632, 99.702)
(4633, 99.9)
(4634, 99.852)
(4635, 99.89)
(4636, 99.91)
(4637, 99.78)
(4638, 99.824)
(4639, 99.898)
(4640, 99.632)
(4641, 99.794)
(4642, 99.828)
(4643, 99.74)
(4644, 99.062)
(4645, 99.686)
(4646, 99.78)
(4647, 99.742)
(4648, 99.722)
(4649, 98.71)
(4650, 99.798)
(4651, 99.762)
(4652, 99.522)
(4653, 99.486)
(4654, 99.89)
(4655, 99.812)
(4656, 98.658)
(4657, 99.01)
(4658, 98.8)
(4659, 99.224)
(4660, 99.9)
(4661, 98.908)
(4662, 99.19)
(4663, 97.214)
(4664, 99.714)
(4665, 97.64)
(4666, 99.826)
(4667, 99.712)
(4668, 99.954)
(4669, 99.85)
(4670, 99.778)
(4671, 99.306)
(4672, 99.604)
(4673, 99.776)
(4674, 99.546)
(4675, 99.652)
(4676, 99.87)
(4677, 99.464)
(4678, 99.084)
(4679, 99.828)
(4680, 99.428)
(4681, 99.516)
(4682, 99.802)
(4683, 99.878)
(4684, 99.96)
(4685, 99.946)
(4686, 99.456)
(4687, 99.498)
(4688, 99.71)
(4689, 99.788)
(4690, 99.206)
(4691, 99.914)
(4692, 99.854)
(4693, 99.79)
(4694, 99.818)
(4695, 99.972)
(4696, 99.972)
(4697, 99.84)
(4698, 99.248)
(4699, 98.118)
(4700, 99.65)
(4701, 98.76)
(4702, 99.484)
(4703, 98.706)
(4704, 99.574)
(4705, 99.612)
(4706, 98.974)
(4707, 99.162)
(4708, 99.888)
(4709, 99.954)
(4710, 99.91)
(4711, 97.07)
(4712, 99.62)
(4713, 99.282)
(4714, 99.424)
(4715, 99.81)
(4716, 99.908)
(4717, 99.724)
(4718, 99.564)
(4719, 99.59)
(4720, 99.854)
(4721, 99.696)
(4722, 99.528)
(4723, 99.636)
(4724, 99.758)
(4725, 99.928)
(4726, 99.962)
(4727, 99.974)
(4728, 99.912)
(4729, 99.476)
(4730, 98.59)
(4731, 99.856)
(4732, 99.846)
(4733, 99.476)
(4734, 99.914)
(4735, 99.866)
(4736, 99.46)
(4737, 99.968)
(4738, 99.928)
(4739, 99.554)
(4740, 99.856)
(4741, 99.742)
(4742, 99.998)
(4743, 99.94)
(4744, 98.948)
(4745, 99.26)
(4746, 98.276)
(4747, 99.542)
(4748, 98.954)
(4749, 99.578)
(4750, 99.482)
(4751, 99.454)
(4752, 99.138)
(4753, 98.806)
(4754, 97.892)
(4755, 99.684)
(4756, 99.588)
(4757, 99.92)
(4758, 99.986)
(4759, 99.93)
(4760, 99.71)
(4761, 100)
(4762, 99.996)
(4763, 99.986)
(4764, 99.988)
(4765, 99.92)
(4766, 99.92)
(4767, 99.886)
(4768, 99.798)
(4769, 99.942)
(4770, 99.982)
(4771, 99.996)
(4772, 99.97)
(4773, 99.986)
(4774, 99.99)
(4775, 99.928)
(4776, 99.112)
(4777, 98.32)
(4778, 99.74)
(4779, 99.502)
(4780, 98.618)
(4781, 99.69)
(4782, 99.628)
(4783, 99.508)
(4784, 98.834)
(4785, 98.81)
(4786, 98.1)
(4787, 99.842)
(4788, 97.326)
(4789, 98.862)
(4790, 99.512)
(4791, 98.824)
(4792, 99.62)
(4793, 99.436)
(4794, 99.504)
(4795, 99.572)
(4796, 99.32)
(4797, 99.244)
(4798, 98.96)
(4799, 99.588)
(4800, 99.388)
(4801, 99.014)
(4802, 99.756)
(4803, 99.902)
(4804, 99.934)
(4805, 99.612)
(4806, 99.994)
(4807, 99.442)
(4808, 99.91)
(4809, 99.878)
(4810, 99.982)
(4811, 99.932)
(4812, 99.856)
(4813, 99.87)
(4814, 99.9)
(4815, 99.498)
(4816, 99.7)
(4817, 99.15)
(4818, 99.816)
(4819, 98.942)
(4820, 99.794)
(4821, 99.61)
(4822, 99.94)
(4823, 99.72)
(4824, 99.484)
(4825, 99.128)
(4826, 99.576)
(4827, 97.688)
(4828, 99.622)
(4829, 99.492)
(4830, 99.852)
(4831, 99.448)
(4832, 99.704)
(4833, 99.562)
(4834, 99.872)
(4835, 99.446)
(4836, 99.782)
(4837, 99.32)
(4838, 99.742)
(4839, 99.792)
(4840, 99.144)
(4841, 99.876)
(4842, 99.97)
(4843, 99.808)
(4844, 99.748)
(4845, 99.836)
(4846, 99.832)
(4847, 99.832)
(4848, 99.806)
(4849, 99.96)
(4850, 99.824)
(4851, 99.91)
(4852, 99.896)
(4853, 99.918)
(4854, 99.716)
(4855, 99.472)
(4856, 99.89)
(4857, 99.924)
(4858, 98.39)
(4859, 99.406)
(4860, 98.896)
(4861, 98.862)
(4862, 99.43)
(4863, 99.914)
(4864, 99.726)
(4865, 99.44)
(4866, 98.922)
(4867, 98.626)
(4868, 98.826)
(4869, 99.736)
(4870, 99.516)
(4871, 99.43)
(4872, 99.54)
(4873, 99.482)
(4874, 98.828)
(4875, 99.326)
(4876, 99.46)
(4877, 99.128)
(4878, 98.812)
(4879, 99.682)
(4880, 99.342)
(4881, 98.216)
(4882, 99.812)
(4883, 99.746)
(4884, 99.576)
(4885, 99.614)
(4886, 99.47)
(4887, 99.762)
(4888, 97.952)
(4889, 99.358)
(4890, 98.582)
(4891, 99.73)
(4892, 99.8)
(4893, 99.744)
(4894, 98.862)
(4895, 99.978)
(4896, 99.964)
(4897, 99.994)
(4898, 99.984)
(4899, 99.932)
(4900, 98.402)
(4901, 99.46)
(4902, 99.774)
(4903, 99.634)
(4904, 99.826)
(4905, 99.988)
(4906, 99.966)
(4907, 99.966)
(4908, 99.998)
(4909, 99.954)
(4910, 99.95)
(4911, 99.99)
(4912, 99.862)
(4913, 99.838)
(4914, 99.326)
(4915, 99.792)
(4916, 99.794)
(4917, 99.97)
(4918, 99.984)
(4919, 99.966)
(4920, 99.994)
(4921, 99.972)
(4922, 100)
(4923, 100)
(4924, 99.946)
(4925, 99.968)
(4926, 99.908)
(4927, 99.972)
(4928, 99.996)
(4929, 99.994)
(4930, 99.992)
(4931, 99.996)
(4932, 100)
(4933, 100)
(4934, 100)
(4935, 100)
(4936, 100)
(4937, 99.998)
(4938, 99.998)
(4939, 99.98)
(4940, 99.978)
(4941, 99.942)
(4942, 99.98)
(4943, 99.996)
(4944, 99.736)
(4945, 100)
(4946, 100)
(4947, 99.998)
(4948, 100)
(4949, 100)
(4950, 100)
(4951, 100)
(4952, 100)
(4953, 99.982)
(4954, 99.998)
(4955, 100)
(4956, 99.99)
(4957, 99.998)
(4958, 100)
(4959, 100)
(4960, 100)
(4961, 99.996)
(4962, 100)
(4963, 100)
(4964, 100)
(4965, 100)
(4966, 100)
(4967, 100)
(4968, 100)
(4969, 100)
(4970, 100)
(4971, 100)
(4972, 99.998)
(4973, 100)
(4974, 99.882)
(4975, 100)
(4976, 99.972)
(4977, 99.972)
(4978, 99.458)
(4979, 99.984)
(4980, 100)
(4981, 99.988)
(4982, 100)
(4983, 100)
(4984, 99.998)
(4985, 99.996)
(4986, 99.994)
(4987, 100)
(4988, 99.99)
(4989, 100)
(4990, 99.958)
(4991, 99.946)
(4992, 99.916)
(4993, 99.9)
(4994, 99.91)
(4995, 99.996)
(4996, 99.992)
(4997, 99.994)
(4998, 99.922)
(4999, 99.984)
(5000, 99.996)
(5001, 99.886)
(5002, 98.024)
(5003, 99.94)
(5004, 99.756)
(5005, 99.406)
(5006, 99.264)
(5007, 99.886)
(5008, 99.742)
(5009, 99.45)
(5010, 99.176)
(5011, 99.516)
(5012, 99.934)
(5013, 99.938)
(5014, 99.998)
(5015, 99.82)
(5016, 99.872)
(5017, 99.288)
(5018, 99.906)
(5019, 99.88)
(5020, 99.982)
(5021, 99.988)
(5022, 99.998)
(5023, 99.936)
(5024, 99.748)
(5025, 99.652)
(5026, 99.974)
(5027, 99.988)
(5028, 99.998)
(5029, 99.98)
(5030, 98.914)
(5031, 99.996)
(5032, 99.994)
(5033, 100)
(5034, 99.918)
(5035, 99.968)
(5036, 99.94)
(5037, 99.96)
(5038, 99.788)
(5039, 100)
(5040, 99.998)
(5041, 100)
(5042, 99.994)
(5043, 99.988)
(5044, 99.92)
(5045, 99.948)
(5046, 99.988)
(5047, 99.286)
(5048, 99.78)
(5049, 99.982)
(5050, 99.752)
(5051, 99.956)
(5052, 99.924)
(5053, 99.86)
(5054, 99.862)
(5055, 99.544)
(5056, 99.978)
(5057, 98.93)
(5058, 99.866)
(5059, 99.896)
(5060, 99.862)
(5061, 99.302)
(5062, 99.958)
(5063, 99.856)
(5064, 99.966)
(5065, 99.908)
(5066, 97.174)
(5067, 99.988)
(5068, 99.87)
(5069, 99.888)
(5070, 99.922)
(5071, 99.986)
(5072, 99.998)
(5073, 99.382)
(5074, 99.748)
(5075, 98.89)
(5076, 98.706)
(5077, 98.31)
(5078, 98.802)
(5079, 99.442)
(5080, 98.8)
(5081, 99.384)
(5082, 98.72)
(5083, 98.986)
(5084, 98.856)
(5085, 99.802)
(5086, 99.61)
(5087, 99.256)
(5088, 98.94)
(5089, 99.784)
(5090, 99.426)
(5091, 96.394)
(5092, 99.578)
(5093, 99.504)
(5094, 99.282)
(5095, 99.688)
(5096, 99.3)
(5097, 99.808)
(5098, 99.37)
(5099, 99.682)
(5100, 99.72)
(5101, 99.838)
(5102, 98.966)
(5103, 97.306)
(5104, 97.494)
(5105, 99.71)
(5106, 95.404)
(5107, 98.658)
(5108, 98.604)
(5109, 98.872)
(5110, 98.78)
(5111, 99.372)
(5112, 99.602)
(5113, 99.584)
(5114, 99.598)
(5115, 98.084)
(5116, 99.934)
(5117, 99.944)
(5118, 99.968)
(5119, 99.98)
(5120, 99.902)
(5121, 99.946)
(5122, 99.838)
(5123, 99.94)
(5124, 100)
(5125, 99.97)
(5126, 99.994)
(5127, 99.826)
(5128, 99.452)
(5129, 99.918)
(5130, 99.908)
(5131, 99.74)
(5132, 99.674)
(5133, 99.804)
(5134, 99.788)
(5135, 99.806)
(5136, 96.416)
(5137, 99.128)
(5138, 99.374)
(5139, 98.462)
(5140, 99.092)
(5141, 98.156)
(5142, 99.726)
(5143, 98.246)
(5144, 99.004)
(5145, 99.578)
(5146, 99.914)
(5147, 99.9)
(5148, 99.922)
(5149, 99.788)
(5150, 98.58)
(5151, 99.276)
(5152, 99.924)
(5153, 99.936)
(5154, 99.888)
(5155, 99.77)
(5156, 99.642)
(5157, 99.622)
(5158, 99.436)
(5159, 99.796)
(5160, 99.47)
(5161, 99.806)
(5162, 99.938)
(5163, 99.41)
(5164, 99.278)
(5165, 99.654)
(5166, 99.52)
(5167, 99.968)
(5168, 99.862)
(5169, 99.912)
(5170, 99.9)
(5171, 99.948)
(5172, 99.868)
(5173, 99.894)
(5174, 99.976)
(5175, 99.828)
(5176, 99.412)
(5177, 99.952)
(5178, 99.942)
(5179, 99.842)
(5180, 99.932)
(5181, 99.984)
(5182, 99.5)
(5183, 99.966)
(5184, 99.636)
(5185, 99.782)
(5186, 98.662)
(5187, 99.876)
(5188, 99.872)
(5189, 99.826)
(5190, 99.962)
(5191, 99.928)
(5192, 99.774)
(5193, 99.748)
(5194, 99.108)
(5195, 99.96)
(5196, 99.968)
(5197, 99.992)
(5198, 99.888)
(5199, 99.87)
(5200, 99.302)
(5201, 99.67)
(5202, 99.6)
(5203, 99.368)
(5204, 99.858)
(5205, 99.856)
(5206, 99.104)
(5207, 98.246)
(5208, 99.794)
(5209, 99.774)
(5210, 99.964)
(5211, 99.658)
(5212, 97.638)
(5213, 99.686)
(5214, 99.89)
(5215, 99.804)
(5216, 99.796)
(5217, 98.53)
(5218, 96.546)
(5219, 98.832)
(5220, 99.964)
(5221, 99.964)
(5222, 99.804)
(5223, 99.914)
(5224, 99.87)
(5225, 99.718)
(5226, 99.93)
(5227, 98.4)
(5228, 99.986)
(5229, 99.756)
(5230, 99.51)
(5231, 99.962)
(5232, 99.918)
(5233, 99.9)
(5234, 99.238)
(5235, 97.906)
(5236, 99.968)
(5237, 99.968)
(5238, 100)
(5239, 99.974)
(5240, 99.974)
(5241, 99.882)
(5242, 99.998)
(5243, 99.976)
(5244, 99.714)
(5245, 99.896)
(5246, 99.98)
(5247, 99.996)
(5248, 99.046)
(5249, 99.99)
(5250, 100)
(5251, 99.998)
(5252, 100)
(5253, 100)
(5254, 100)
(5255, 100)
(5256, 99.902)
(5257, 99.934)
(5258, 99.99)
(5259, 99.958)
(5260, 99.964)
(5261, 99.95)
(5262, 99.968)
(5263, 99.996)
(5264, 99.992)
(5265, 99.884)
(5266, 99.764)
(5267, 99.988)
(5268, 99.968)
(5269, 99.99)
(5270, 99.974)
(5271, 99.98)
(5272, 99.972)
(5273, 99.996)
(5274, 99.98)
(5275, 99.932)
(5276, 99.912)
(5277, 99.928)
(5278, 99.758)
(5279, 99.978)
(5280, 97.466)
(5281, 99.986)
(5282, 99.94)
(5283, 99.86)
(5284, 99.876)
(5285, 99.954)
(5286, 99.602)
(5287, 99.15)
(5288, 99.938)
(5289, 99.702)
(5290, 99.352)
(5291, 99.896)
(5292, 99.94)
(5293, 99.922)
(5294, 99.75)
(5295, 99.894)
(5296, 99.78)
(5297, 99.952)
(5298, 99.946)
(5299, 99.81)
(5300, 99.866)
(5301, 99.932)
(5302, 98.874)
(5303, 99.986)
(5304, 99.98)
(5305, 99.93)
(5306, 98.088)
(5307, 99.926)
(5308, 99.906)
(5309, 99.968)
(5310, 99.75)
(5311, 99.606)
(5312, 99.214)
(5313, 96.296)
(5314, 99.798)
(5315, 99.944)
(5316, 99.888)
(5317, 99.92)
(5318, 99.9)
(5319, 99.916)
(5320, 99.518)
(5321, 99.664)
(5322, 99.632)
(5323, 98.888)
(5324, 99.326)
(5325, 99.834)
(5326, 99.932)
(5327, 99.648)
(5328, 99.608)
(5329, 99.76)
(5330, 99.43)
(5331, 99.904)
(5332, 99.966)
(5333, 99.96)
(5334, 99.838)
(5335, 99.864)
(5336, 99.468)
(5337, 99.712)
(5338, 99.634)
(5339, 99.532)
(5340, 99.562)
(5341, 99.586)
(5342, 99.956)
(5343, 99.888)
(5344, 98.238)
(5345, 99.936)
(5346, 99.886)
(5347, 99.456)
(5348, 99.436)
(5349, 99.95)
(5350, 99.82)
(5351, 99.338)
(5352, 99.292)
(5353, 99.946)
(5354, 99.684)
(5355, 99.818)
(5356, 99.812)
(5357, 99.56)
(5358, 99.514)
(5359, 99.916)
(5360, 98.694)
(5361, 99.88)
(5362, 99.784)
(5363, 99.91)
(5364, 99.934)
(5365, 99.846)
(5366, 99.954)
(5367, 99.994)
(5368, 99.9)
(5369, 99.908)
(5370, 99.97)
(5371, 99.93)
(5372, 99.406)
(5373, 99.892)
(5374, 99.55)
(5375, 99.982)
(5376, 99.96)
(5377, 99.886)
(5378, 99.99)
(5379, 99.96)
(5380, 99.886)
(5381, 99.83)
(5382, 97.258)
(5383, 98.92)
(5384, 98.024)
(5385, 99.606)
(5386, 99.784)
(5387, 99.952)
(5388, 99.988)
(5389, 99.98)
(5390, 99.99)
(5391, 99.938)
(5392, 99.906)
(5393, 99.33)
(5394, 99.734)
(5395, 100)
(5396, 100)
(5397, 99.95)
(5398, 99.904)
(5399, 99.906)
(5400, 99.858)
(5401, 99.994)
(5402, 99.84)
(5403, 99.98)
(5404, 99.852)
(5405, 99.98)
(5406, 99.622)
(5407, 99.974)
(5408, 99.95)
(5409, 99.746)
(5410, 99.956)
(5411, 99.922)
(5412, 99.994)
(5413, 99.99)
(5414, 99.964)
(5415, 99.99)
(5416, 99.982)
(5417, 99.938)
(5418, 99.96)
(5419, 99.958)
(5420, 99.762)
(5421, 99.41)
(5422, 99.468)
(5423, 99.974)
(5424, 99.998)
(5425, 99.996)
(5426, 99.992)
(5427, 99.992)
(5428, 100)
(5429, 100)
(5430, 99.97)
(5431, 99.918)
(5432, 99.872)
(5433, 99.95)
(5434, 99.998)
(5435, 99.966)
(5436, 99.902)
(5437, 99.578)
(5438, 99.992)
(5439, 99.906)
(5440, 100)
(5441, 100)
(5442, 100)
(5443, 100)
(5444, 99.892)
(5445, 100)
(5446, 100)
(5447, 99.994)
(5448, 99.996)
(5449, 99.994)
(5450, 99.996)
(5451, 99.982)
(5452, 99.988)
(5453, 99.966)
(5454, 99.994)
(5455, 99.984)
(5456, 99.94)
(5457, 94.28)
(5458, 99.948)
(5459, 99.996)
(5460, 99.974)
(5461, 99.974)
(5462, 99.928)
(5463, 99.942)
(5464, 99.874)
(5465, 98.826)
(5466, 99.072)
(5467, 99.962)
(5468, 99.91)
(5469, 99.906)
(5470, 99.998)
(5471, 99.994)
(5472, 99.982)
(5473, 99.95)
(5474, 99.988)
(5475, 99.922)
(5476, 99.76)
(5477, 99.864)
(5478, 99.992)
(5479, 99.996)
(5480, 100)
(5481, 99.95)
(5482, 99.978)
(5483, 99.974)
(5484, 99.94)
(5485, 99.976)
(5486, 99.836)
(5487, 99.968)
(5488, 99.852)
(5489, 99.524)
(5490, 99.6)
(5491, 99.828)
(5492, 99.622)
(5493, 99.902)
(5494, 99.914)
(5495, 99.892)
(5496, 99.868)
(5497, 99.986)
(5498, 99.898)
(5499, 99.702)
(5500, 99.856)
(5501, 99.892)
(5502, 99.784)
(5503, 99.974)
(5504, 99.892)
(5505, 99.864)
(5506, 99.882)
(5507, 99.928)
(5508, 99.954)
(5509, 99.97)
(5510, 99.954)
(5511, 100)
(5512, 100)
(5513, 99.982)
(5514, 99.998)
(5515, 99.996)
(5516, 100)
(5517, 100)
(5518, 99.994)
(5519, 100)
(5520, 99.988)
(5521, 99.998)
(5522, 99.99)
(5523, 100)
(5524, 99.998)
(5525, 100)
(5526, 100)
(5527, 99.994)
(5528, 100)
(5529, 100)
(5530, 100)
(5531, 99.986)
(5532, 99.976)
(5533, 99.946)
(5534, 99.976)
(5535, 99.666)
(5536, 99.902)
(5537, 99.924)
(5538, 100)
(5539, 99.958)
(5540, 99.98)
(5541, 99.774)
(5542, 99.954)
(5543, 100)
(5544, 100)
(5545, 100)
(5546, 99.998)
(5547, 99.964)
(5548, 99.944)
(5549, 99.936)
(5550, 98.714)
(5551, 99.982)
(5552, 99.942)
(5553, 98.868)
(5554, 98.192)
(5555, 99.8)
(5556, 99.924)
(5557, 99.992)
(5558, 99.888)
(5559, 99.98)
(5560, 99.992)
(5561, 100)
(5562, 99.982)
(5563, 99.996)
(5564, 99.996)
(5565, 99.992)
(5566, 99.962)
(5567, 99.97)
(5568, 99.986)
(5569, 99.944)
(5570, 99.954)
(5571, 99.972)
(5572, 99.93)
(5573, 99.794)
(5574, 99.294)
(5575, 99.198)
(5576, 97.582)
(5577, 98.342)
(5578, 98.362)
(5579, 94.456)
(5580, 97.548)
(5581, 98.848)
(5582, 98.384)
(5583, 96.414)
(5584, 98.338)
(5585, 99.094)
(5586, 99.806)
(5587, 99.48)
(5588, 99.468)
(5589, 99.69)
(5590, 99.768)
(5591, 99.89)
(5592, 99.686)
(5593, 99.932)
(5594, 99.802)
(5595, 99.338)
(5596, 99.56)
(5597, 99.398)
(5598, 98.25)
(5599, 99.12)
(5600, 99.736)
(5601, 99.264)
(5602, 99.466)
(5603, 99.652)
(5604, 99.842)
(5605, 99.91)
(5606, 99.786)
(5607, 99.69)
(5608, 97.312)
(5609, 96.206)
(5610, 99.38)
(5611, 99.692)
(5612, 99.42)
(5613, 98.726)
(5614, 98.586)
(5615, 98.952)
(5616, 99.174)
(5617, 99.682)
(5618, 99.67)
(5619, 99.362)
(5620, 98.806)
(5621, 99.282)
(5622, 98.028)
(5623, 95.214)
(5624, 99.432)
(5625, 98.728)
(5626, 99.41)
(5627, 99.81)
(5628, 99.694)
(5629, 99.778)
(5630, 99.616)
(5631, 99.634)
(5632, 99.272)
(5633, 99.434)
(5634, 98.944)
(5635, 99.262)
(5636, 99.52)
(5637, 99.714)
(5638, 99.08)
(5639, 99.526)
(5640, 99.482)
(5641, 99.678)
(5642, 98.722)
(5643, 97.28)
(5644, 97.546)
(5645, 97.048)
(5646, 98.264)
(5647, 99.668)
(5648, 94.746)
(5649, 97.672)
(5650, 97.41)
(5651, 97.77)
(5652, 98.956)
(5653, 97.9)
(5654, 99.062)
(5655, 98.966)
(5656, 95.838)
(5657, 96.404)
(5658, 96.748)
(5659, 97.046)
(5660, 98.736)
(5661, 98.938)
(5662, 98.42)
(5663, 95.898)
(5664, 98.086)
(5665, 97.77)
(5666, 96.412)
(5667, 92.866)
(5668, 98.186)
(5669, 93.552)
(5670, 95.156)
(5671, 95.878)
(5672, 99.056)
(5673, 97.714)
(5674, 98.374)
(5675, 97.412)
(5676, 96.866)
(5677, 83.726)
(5678, 98.148)
(5679, 98.394)
(5680, 98.482)
(5681, 94.652)
(5682, 98.198)
(5683, 91.804)
(5684, 96.396)
(5685, 95.834)
(5686, 94.94)
(5687, 98.06)
(5688, 98.182)
(5689, 95.114)
(5690, 92.474)
(5691, 93.564)
(5692, 95.724)
(5693, 92.582)
(5694, 94.97)
(5695, 93.088)
(5696, 98.6)
(5697, 97.344)
(5698, 97.992)
(5699, 96.778)
(5700, 98.43)
(5701, 98.328)
(5702, 96.724)
(5703, 96.336)
(5704, 99.004)
(5705, 99.14)
(5706, 99.03)
(5707, 98.346)
(5708, 97.45)
(5709, 99.27)
(5710, 98.89)
(5711, 98.174)
(5712, 96.666)
(5713, 99.092)
(5714, 97.886)
(5715, 99.43)
(5716, 99.702)
(5717, 98.018)
(5718, 99.432)
(5719, 98.616)
(5720, 99.076)
(5721, 98.622)
(5722, 98.688)
(5723, 99.004)
(5724, 99.484)
(5725, 99.202)
(5726, 99.526)
(5727, 98.158)
(5728, 99.294)
(5729, 99.702)
(5730, 99.448)
(5731, 99.47)
(5732, 99.22)
(5733, 99.24)
(5734, 98.976)
(5735, 94.608)
(5736, 98.92)
(5737, 98.758)
(5738, 99.13)
(5739, 98.238)
(5740, 97.94)
(5741, 99.148)
(5742, 99.738)
(5743, 99.092)
(5744, 97.29)
(5745, 99.012)
(5746, 99.296)
(5747, 99.294)
(5748, 99.43)
(5749, 99.304)
(5750, 99.792)
(5751, 98.798)
(5752, 97.218)
(5753, 99.66)
(5754, 99.698)
(5755, 99.658)
(5756, 99.712)
(5757, 99.284)
(5758, 99.788)
(5759, 99.75)
(5760, 99.402)
(5761, 99.828)
(5762, 99.548)
(5763, 99.626)
(5764, 99.556)
(5765, 99.184)
(5766, 99.252)
(5767, 99.358)
(5768, 99.286)
(5769, 99.522)
(5770, 99.354)
(5771, 99.132)
(5772, 98.582)
(5773, 97.176)
(5774, 95.466)
(5775, 95.476)
(5776, 97.382)
(5777, 95.886)
(5778, 96.556)
(5779, 98.26)
(5780, 98.988)
(5781, 98.188)
(5782, 97.988)
(5783, 97.89)
(5784, 98.85)
(5785, 98.44)
(5786, 97.696)
(5787, 97.136)
(5788, 96.15)
(5789, 97.5)
(5790, 97.76)
(5791, 98.142)
(5792, 98.13)
(5793, 98.448)
(5794, 99.152)
(5795, 99.37)
(5796, 99.51)
(5797, 99.376)
(5798, 99.422)
(5799, 98.844)
(5800, 98.946)
(5801, 99.454)
(5802, 99.578)
(5803, 99.85)
(5804, 99.354)
(5805, 99.816)
(5806, 99.492)
(5807, 99.964)
(5808, 99.878)
(5809, 99.438)
(5810, 99.816)
(5811, 99.452)
(5812, 99.282)
(5813, 99.804)
(5814, 99.564)
(5815, 99.132)
(5816, 99.624)
(5817, 99.818)
(5818, 99.72)
(5819, 98.378)
(5820, 98.32)
(5821, 99.466)
(5822, 98.772)
(5823, 99.258)
(5824, 99.46)
(5825, 99.564)
(5826, 99.586)
(5827, 99.394)
(5828, 99.664)
(5829, 99.454)
(5830, 99.612)
(5831, 99.854)
(5832, 99.06)
(5833, 99.088)
(5834, 99.706)
(5835, 98.582)
(5836, 99.248)
(5837, 99.45)
(5838, 99.474)
(5839, 99.54)
(5840, 99.784)
(5841, 99.648)
(5842, 98.824)
(5843, 99.202)
(5844, 99.788)
(5845, 99.916)
(5846, 99.832)
(5847, 99.798)
(5848, 99.754)
(5849, 99.246)
(5850, 99.154)
(5851, 99.856)
(5852, 99.276)
(5853, 99.688)
(5854, 99.76)
(5855, 99.578)
(5856, 98.814)
(5857, 98.828)
(5858, 95.498)
(5859, 99.406)
(5860, 99.662)
(5861, 99.696)
(5862, 99.346)
(5863, 99.88)
(5864, 99.782)
(5865, 99.734)
(5866, 99.508)
(5867, 98.2)
(5868, 99.212)
(5869, 96.732)
(5870, 99.446)
(5871, 99.726)
(5872, 99.63)
(5873, 99.906)
(5874, 99.642)
(5875, 99.966)
(5876, 99.202)
(5877, 99.828)
(5878, 99.61)
(5879, 97.118)
(5880, 99.876)
(5881, 99.934)
(5882, 99.882)
(5883, 99.768)
(5884, 99.418)
(5885, 99.742)
(5886, 99.584)
(5887, 99.872)
(5888, 99.654)
(5889, 99.66)
(5890, 99.394)
(5891, 99.526)
(5892, 99.778)
(5893, 99.462)
(5894, 99.854)
(5895, 99.564)
(5896, 99.824)
(5897, 99.614)
(5898, 99.34)
(5899, 98.368)
(5900, 99.73)
(5901, 99.682)
(5902, 99.354)
(5903, 99.536)
(5904, 98.79)
(5905, 99.688)
(5906, 99.454)
(5907, 99.078)
(5908, 99.75)
(5909, 99.46)
(5910, 99.766)
(5911, 99.772)
(5912, 99.796)
(5913, 99.644)
(5914, 99.72)
(5915, 98.888)
(5916, 99.724)
(5917, 99.038)
(5918, 99.494)
(5919, 99.512)
(5920, 99.522)
(5921, 99.602)
(5922, 99.78)
(5923, 99.57)
(5924, 99.464)
(5925, 99.76)
(5926, 99.862)
(5927, 99.446)
(5928, 99.736)
(5929, 99.874)
(5930, 99.766)
(5931, 98.55)
(5932, 99.884)
(5933, 99.938)
(5934, 99.996)
(5935, 99.946)
(5936, 99.914)
(5937, 99.976)
(5938, 100)
(5939, 99.494)
(5940, 99.974)
(5941, 99.926)
(5942, 99.726)
(5943, 99.948)
(5944, 99.788)
(5945, 99.988)
(5946, 99.912)
(5947, 99.982)
(5948, 100)
(5949, 99.992)
(5950, 99.86)
(5951, 99.968)
(5952, 99.972)
(5953, 99.624)
(5954, 99.988)
(5955, 99.942)
(5956, 99.966)
(5957, 99.992)
(5958, 99.99)
(5959, 99.988)
(5960, 100)
(5961, 99.998)
(5962, 99.954)
(5963, 99.996)
(5964, 99.99)
(5965, 99.876)
(5966, 99.994)
(5967, 100)
(5968, 100)
(5969, 100)
(5970, 100)
(5971, 100)
(5972, 100)
(5973, 100)
(5974, 99.998)
(5975, 100)
(5976, 100)
(5977, 100)
(5978, 100)
(5979, 100)
(5980, 100)
(5981, 100)
(5982, 100)
(5983, 100)
(5984, 100)
(5985, 100)
(5986, 100)
(5987, 100)
(5988, 99.98)
(5989, 99.738)
(5990, 91.826)
(5991, 99.998)
(5992, 99.994)
(5993, 100)
(5994, 99.99)
(5995, 99.974)
(5996, 99.99)
(5997, 99.922)
(5998, 99.86)
(5999, 99.95)
(6000, 99.956)
(6001, 99.97)
(6002, 99.86)
(6003, 99.046)
(6004, 100)
(6005, 99.992)
(6006, 100)
(6007, 99.998)
(6008, 99.99)
(6009, 99.972)
(6010, 99.986)
(6011, 99.952)
(6012, 99.826)
(6013, 99.958)
(6014, 99.998)
(6015, 99.986)
(6016, 99.964)
(6017, 99.954)
(6018, 99.988)
(6019, 99.956)
(6020, 99.982)
(6021, 99.998)
(6022, 99.988)
(6023, 99.976)
(6024, 99.774)
(6025, 99.972)
(6026, 100)
(6027, 99.998)
(6028, 99.572)
(6029, 99.95)
(6030, 99.676)
(6031, 98.952)
(6032, 99.772)
(6033, 99.828)
(6034, 99.932)
(6035, 99.866)
(6036, 99.946)
(6037, 99.358)
(6038, 99.208)
(6039, 99.948)
(6040, 99.784)
(6041, 99.826)
(6042, 99.952)
(6043, 99.968)
(6044, 99.986)
(6045, 99.992)
(6046, 99.76)
(6047, 99.992)
(6048, 99.998)
(6049, 99.996)
(6050, 99.992)
(6051, 99.976)
(6052, 99.912)
(6053, 99.55)
(6054, 99.896)
(6055, 99.742)
(6056, 99.93)
(6057, 99.938)
(6058, 99.998)
(6059, 99.78)
(6060, 99.93)
(6061, 99.982)
(6062, 99.99)
(6063, 99.984)
(6064, 99.984)
(6065, 99.824)
(6066, 99.966)
(6067, 99.798)
(6068, 99.82)
(6069, 98.464)
(6070, 99.706)
(6071, 99.87)
(6072, 99.89)
(6073, 99.944)
(6074, 99.808)
(6075, 99.842)
(6076, 99.856)
(6077, 99.924)
(6078, 99.732)
(6079, 99.792)
(6080, 99.578)
(6081, 99.394)
(6082, 99.99)
(6083, 99.962)
(6084, 99.886)
(6085, 99.918)
(6086, 98.412)
(6087, 99.722)
(6088, 99.332)
(6089, 99.562)
(6090, 99.128)
(6091, 99.412)
(6092, 99.736)
(6093, 99.352)
(6094, 99.806)
(6095, 99.596)
(6096, 99.242)
(6097, 99.912)
(6098, 99.662)
(6099, 99.826)
(6100, 97.908)
(6101, 99.104)
(6102, 96.852)
(6103, 99.842)
(6104, 99.408)
(6105, 99.742)
(6106, 99.798)
(6107, 99.96)
(6108, 99.698)
(6109, 99.92)
(6110, 99.802)
(6111, 99.252)
(6112, 99.844)
(6113, 99.78)
(6114, 99.784)
(6115, 99.312)
(6116, 99.152)
(6117, 99.712)
(6118, 98.79)
(6119, 99.722)
(6120, 99.014)
(6121, 99.188)
(6122, 99.472)
(6123, 99.786)
(6124, 99.668)
(6125, 99.72)
(6126, 99.656)
(6127, 99.792)
(6128, 99.948)
(6129, 99.982)
(6130, 99.956)
(6131, 99.896)
(6132, 99.978)
(6133, 99.964)
(6134, 99.854)
(6135, 99.936)
(6136, 99.958)
(6137, 99.916)
(6138, 99.962)
(6139, 99.792)
(6140, 99.844)
(6141, 99.954)
(6142, 99.914)
(6143, 99.974)
(6144, 99.976)
(6145, 99.968)
(6146, 99.81)
(6147, 99.114)
(6148, 98.374)
(6149, 98.636)
(6150, 99.902)
(6151, 99.776)
(6152, 99.724)
(6153, 99.85)
(6154, 99.916)
(6155, 99.482)
(6156, 99.04)
(6157, 99.16)
(6158, 99.158)
(6159, 99.872)
(6160, 99.678)
(6161, 99.624)
(6162, 99.506)
(6163, 99.32)
(6164, 99.72)
(6165, 99.466)
(6166, 99.706)
(6167, 99.886)
(6168, 99.93)
(6169, 99.922)
(6170, 99.74)
(6171, 99.796)
(6172, 99.836)
(6173, 99.694)
(6174, 99.778)
(6175, 99.652)
(6176, 99.574)
(6177, 99.582)
(6178, 99.778)
(6179, 99.606)
(6180, 99.506)
(6181, 98.892)
(6182, 99.842)
(6183, 99.712)
(6184, 99.822)
(6185, 99.448)
(6186, 99.78)
(6187, 96.812)
(6188, 99.528)
(6189, 99.848)
(6190, 99.678)
(6191, 99.71)
(6192, 99.714)
(6193, 99.988)
(6194, 99.946)
(6195, 99.128)
(6196, 99.812)
(6197, 99.99)
(6198, 99.962)
(6199, 99.906)
(6200, 99.928)
(6201, 99.67)
(6202, 99.574)
(6203, 93.734)
(6204, 99.802)
(6205, 99.89)
(6206, 92.094)
(6207, 99.972)
(6208, 99.97)
(6209, 99.934)
(6210, 99.922)
(6211, 99.398)
(6212, 99.784)
(6213, 99.398)
(6214, 99.84)
(6215, 99.992)
(6216, 99.942)
(6217, 99.656)
(6218, 99.834)
(6219, 98.068)
(6220, 99.892)
(6221, 99.938)
(6222, 99.96)
(6223, 99.824)
(6224, 99.604)
(6225, 99.778)
(6226, 99.592)
(6227, 99.916)
(6228, 99.948)
(6229, 99.85)
(6230, 99.806)
(6231, 99.7)
(6232, 99.808)
(6233, 99.568)
(6234, 99.898)
(6235, 98.948)
(6236, 99.81)
(6237, 98.818)
(6238, 99.964)
(6239, 99.936)
(6240, 99.82)
(6241, 99.838)
(6242, 98.146)
(6243, 99.41)
(6244, 99.5)
(6245, 98.634)
(6246, 99.076)
(6247, 98.38)
(6248, 98.068)
(6249, 99.41)
(6250, 98.186)
(6251, 98.38)
(6252, 99.448)
(6253, 97.718)
(6254, 99.47)
(6255, 99.834)
(6256, 99.876)
(6257, 99.126)
(6258, 99.052)
(6259, 99.436)
(6260, 99.632)
(6261, 99.692)
(6262, 99.388)
(6263, 99.918)
(6264, 99.942)
(6265, 98.678)
(6266, 99.576)
(6267, 99.754)
(6268, 99.82)
(6269, 99.796)
(6270, 99.758)
(6271, 99.792)
(6272, 99.598)
(6273, 99.752)
(6274, 99.6)
(6275, 99.562)
(6276, 98.108)
(6277, 99.522)
(6278, 99.648)
(6279, 99.838)
(6280, 98.994)
(6281, 99.842)
(6282, 99.594)
(6283, 97.318)
(6284, 99.332)
(6285, 99.218)
(6286, 98.628)
(6287, 96.804)
(6288, 99.678)
(6289, 99.854)
(6290, 98.724)
(6291, 99.892)
(6292, 99.6)
(6293, 98.278)
(6294, 99.922)
(6295, 99.794)
(6296, 99.496)
(6297, 99.85)
(6298, 99.51)
(6299, 99.592)
(6300, 99.826)
(6301, 99.262)
(6302, 99.812)
(6303, 98.454)
(6304, 99.526)
(6305, 99.246)
(6306, 99.848)
(6307, 99.252)
(6308, 99.476)
(6309, 99.742)
(6310, 99.744)
(6311, 99.826)
(6312, 99.714)
(6313, 99.648)
(6314, 98.458)
(6315, 99.642)
(6316, 99.342)
(6317, 98.898)
(6318, 99.4)
(6319, 99.232)
(6320, 98.976)
(6321, 98.748)
(6322, 99.688)
(6323, 99.148)
(6324, 99.072)
(6325, 99.402)
(6326, 99.204)
(6327, 99.238)
(6328, 99.542)
(6329, 99.592)
(6330, 99.242)
(6331, 99.714)
(6332, 99.97)
(6333, 99.408)
(6334, 99.708)
(6335, 99.828)
(6336, 99.658)
(6337, 99.886)
(6338, 99.82)
(6339, 99.814)
(6340, 99.982)
(6341, 99.87)
(6342, 99.95)
(6343, 99.888)
(6344, 99.58)
(6345, 99.482)
(6346, 99.464)
(6347, 97.884)
(6348, 98.654)
(6349, 99.762)
(6350, 99.354)
(6351, 99.532)
(6352, 99.696)
(6353, 99.418)
(6354, 99.77)
(6355, 99.592)
(6356, 96.07)
(6357, 99.646)
(6358, 99.842)
(6359, 99.488)
(6360, 99.36)
(6361, 98.86)
(6362, 99.614)
(6363, 99.836)
(6364, 99.586)
(6365, 99.566)
(6366, 99.966)
(6367, 99.834)
(6368, 97.94)
(6369, 94.854)
(6370, 95.914)
(6371, 99.986)
(6372, 99.972)
(6373, 99.978)
(6374, 99.944)
(6375, 99.758)
(6376, 99.99)
(6377, 99.988)
(6378, 99.952)
(6379, 99.978)
(6380, 99.978)
(6381, 99.95)
(6382, 99.934)
(6383, 99.832)
(6384, 99.42)
(6385, 99.954)
(6386, 99.932)
(6387, 99.238)
(6388, 99.826)
(6389, 99.546)
(6390, 99.324)
(6391, 98.66)
(6392, 99.11)
(6393, 99.28)
(6394, 93.418)
(6395, 97.544)
(6396, 98.836)
(6397, 96.716)
(6398, 99.736)
(6399, 98.384)
(6400, 99.406)
(6401, 98.63)
(6402, 98.43)
(6403, 98.898)
(6404, 98.442)
(6405, 97.322)
(6406, 98.674)
(6407, 99.27)
(6408, 99.346)
(6409, 97.852)
(6410, 91.388)
(6411, 98.136)
(6412, 98.3)
(6413, 96.724)
(6414, 98.228)
(6415, 93.546)
(6416, 96.734)
(6417, 98.784)
(6418, 98.894)
(6419, 96.192)
(6420, 98.46)
(6421, 98.84)
(6422, 98.452)
(6423, 98.944)
(6424, 98.942)
(6425, 97.088)
(6426, 98.888)
(6427, 97.672)
(6428, 95.842)
(6429, 97.83)
(6430, 97.796)
(6431, 96.676)
(6432, 96.792)
(6433, 97.076)
(6434, 99.406)
(6435, 97.688)
(6436, 95.332)
(6437, 97.304)
(6438, 99.296)
(6439, 98.202)
(6440, 98.024)
(6441, 98.398)
(6442, 98.74)
(6443, 98.018)
(6444, 97.732)
(6445, 96.044)
(6446, 95.598)
(6447, 97.798)
(6448, 98.87)
(6449, 97.046)
(6450, 97.918)
(6451, 98.566)
(6452, 97.732)
(6453, 97.512)
(6454, 98.238)
(6455, 97.528)
(6456, 96.818)
(6457, 96.198)
(6458, 95.404)
(6459, 95.976)
(6460, 95.728)
(6461, 93.854)
(6462, 96.2)
(6463, 98.318)
(6464, 99.552)
(6465, 98.122)
(6466, 97.79)
(6467, 98.212)
(6468, 98.832)
(6469, 98.554)
(6470, 98.546)
(6471, 95.776)
(6472, 98.5)
(6473, 98.212)
(6474, 97.792)
(6475, 96.148)
(6476, 98.784)
(6477, 96.66)
(6478, 98.298)
(6479, 98.936)
(6480, 97.648)
(6481, 98.094)
(6482, 97.992)
(6483, 98.268)
(6484, 97.77)
(6485, 99.114)
(6486, 97.564)
(6487, 97.842)
(6488, 98.236)
(6489, 99.09)
(6490, 99.184)
(6491, 97.584)
(6492, 98.622)
(6493, 99.132)
(6494, 99.698)
(6495, 98.814)
(6496, 98.75)
(6497, 99.588)
(6498, 99.42)
(6499, 99.472)
(6500, 99.766)
(6501, 99.37)
(6502, 99.258)
(6503, 98.168)
(6504, 99.374)
(6505, 99.526)
(6506, 99.08)
(6507, 98.21)
(6508, 96.278)
(6509, 99.318)
(6510, 98.432)
(6511, 99.388)
(6512, 99.37)
(6513, 97.938)
(6514, 98.356)
(6515, 98.532)
(6516, 98.684)
(6517, 98.108)
(6518, 98.616)
(6519, 98.984)
(6520, 99.186)
(6521, 99.414)
(6522, 98.028)
(6523, 99.382)
(6524, 99.516)
(6525, 99.506)
(6526, 99.572)
(6527, 99.534)
(6528, 99.674)
(6529, 99.18)
(6530, 99.66)
(6531, 99.526)
(6532, 99.716)
(6533, 99.772)
(6534, 99.692)
(6535, 99.206)
(6536, 83.386)
(6537, 97.426)
(6538, 96.114)
(6539, 97.176)
(6540, 97.332)
(6541, 95.474)
(6542, 97.41)
(6543, 98.244)
(6544, 98.284)
(6545, 98.52)
(6546, 99.33)
(6547, 97.458)
(6548, 98.844)
(6549, 98.254)
(6550, 94.79)
(6551, 99.554)
(6552, 99.05)
(6553, 99.664)
(6554, 95.652)
(6555, 98.566)
(6556, 98.88)
(6557, 98.46)
(6558, 97.974)
(6559, 99.44)
(6560, 96.73)
(6561, 98.536)
(6562, 97.36)
(6563, 99.018)
(6564, 99.768)
(6565, 99.412)
(6566, 97.644)
(6567, 98.784)
(6568, 99.506)
(6569, 99.554)
(6570, 99.906)
(6571, 99.696)
(6572, 99.742)
(6573, 99.772)
(6574, 99.874)
(6575, 99.802)
(6576, 99.696)
(6577, 96.16)
(6578, 99.83)
(6579, 99.736)
(6580, 99.62)
(6581, 95.944)
(6582, 99.626)
(6583, 97.664)
(6584, 92.81)
(6585, 98.838)
(6586, 98.856)
(6587, 95.058)
(6588, 97.13)
(6589, 99.348)
(6590, 99.286)
(6591, 98.862)
(6592, 99.726)
(6593, 99.212)
(6594, 99.564)
(6595, 99.55)
(6596, 98.902)
(6597, 99.586)
(6598, 99.858)
(6599, 98.216)
(6600, 98.81)
(6601, 99.072)
(6602, 97.92)
(6603, 98.228)
(6604, 99.18)
(6605, 99.226)
(6606, 99.706)
(6607, 99.576)
(6608, 97.01)
(6609, 99.416)
(6610, 99.502)
(6611, 99.868)
(6612, 99.904)
(6613, 99.822)
(6614, 99.558)
(6615, 99.194)
(6616, 97.902)
(6617, 99.67)
(6618, 99.646)
(6619, 99.826)
(6620, 99.772)
(6621, 99.734)
(6622, 99.924)
(6623, 99.89)
(6624, 99.45)
(6625, 99.12)
(6626, 99.512)
(6627, 99.734)
(6628, 99.534)
(6629, 98.84)
(6630, 99.68)
(6631, 99.686)
(6632, 99.774)
(6633, 99.258)
(6634, 99.684)
(6635, 99.734)
(6636, 99.486)
(6637, 99.892)
(6638, 99.934)
(6639, 99.976)
(6640, 99.806)
(6641, 99.572)
(6642, 99.242)
(6643, 98.99)
(6644, 99.094)
(6645, 99.73)
(6646, 99.694)
(6647, 98.942)
(6648, 98.914)
(6649, 99.838)
(6650, 99.622)
(6651, 99.824)
(6652, 99.812)
(6653, 99.728)
(6654, 98.306)
(6655, 97.978)
(6656, 99.188)
(6657, 99.748)
(6658, 98.186)
(6659, 98.642)
(6660, 99.23)
(6661, 99.03)
(6662, 99.322)
(6663, 98.968)
(6664, 98.582)
(6665, 99.47)
(6666, 99.316)
(6667, 98.698)
(6668, 99.332)
(6669, 99.37)
(6670, 98.802)
(6671, 99.37)
(6672, 99.466)
(6673, 98.15)
(6674, 98.938)
(6675, 98.984)
(6676, 99.36)
(6677, 98.49)
(6678, 99.49)
(6679, 99.614)
(6680, 99.816)
(6681, 99.3)
(6682, 99.924)
(6683, 99.954)
(6684, 99.454)
(6685, 99.8)
(6686, 99.46)
(6687, 99.902)
(6688, 99.974)
(6689, 99.854)
(6690, 99.894)
(6691, 99.86)
(6692, 99.972)
(6693, 99.974)
(6694, 99.818)
(6695, 99.858)
(6696, 99.92)
(6697, 99.91)
(6698, 99.868)
(6699, 98.6)
(6700, 99.19)
(6701, 99.7)
(6702, 99.444)
(6703, 99.234)
(6704, 99.928)
(6705, 98.7)
(6706, 97.552)
(6707, 98.458)
(6708, 99.11)
(6709, 98.602)
(6710, 98.05)
(6711, 98.598)
(6712, 97.87)
(6713, 95.676)
(6714, 99.46)
(6715, 98.734)
(6716, 99.084)
(6717, 99.606)
(6718, 99.942)
(6719, 99.914)
(6720, 99.952)
(6721, 99.804)
(6722, 99.936)
(6723, 99.832)
(6724, 99.884)
(6725, 99.858)
(6726, 99.928)
(6727, 99.19)
(6728, 98.448)
(6729, 98.838)
(6730, 99.908)
(6731, 99.946)
(6732, 99.748)
(6733, 99.922)
(6734, 99.714)
(6735, 95.652)
(6736, 98.386)
(6737, 95.722)
(6738, 99.258)
(6739, 99.154)
(6740, 98.912)
(6741, 99.586)
(6742, 98.698)
(6743, 99.75)
(6744, 99.76)
(6745, 99.742)
(6746, 99.408)
(6747, 99.672)
(6748, 99.478)
(6749, 99.594)
(6750, 99.77)
(6751, 99.904)
(6752, 99.74)
(6753, 99.938)
(6754, 99.724)
(6755, 99.774)
(6756, 99.766)
(6757, 99.81)
(6758, 99.842)
(6759, 99.512)
(6760, 99.75)
(6761, 99.536)
(6762, 99.884)
(6763, 99.774)
(6764, 99.884)
(6765, 99.97)
(6766, 99.944)
(6767, 99.87)
(6768, 99.484)
(6769, 99.52)
(6770, 99.546)
(6771, 99.592)
(6772, 99.21)
(6773, 99.174)
(6774, 99.848)
(6775, 99.568)
(6776, 98.334)
(6777, 99.874)
(6778, 97.88)
(6779, 99.482)
(6780, 95.626)
(6781, 98.696)
(6782, 99.712)
(6783, 98.032)
(6784, 99.878)
(6785, 99.72)
(6786, 99.336)
(6787, 99.346)
(6788, 99.678)
(6789, 99.682)
(6790, 99.49)
(6791, 99.664)
(6792, 99.338)
(6793, 98.674)
(6794, 98.288)
(6795, 98.836)
(6796, 98.118)
(6797, 98.67)
(6798, 99.634)
(6799, 99.588)
(6800, 99.494)
(6801, 99.606)
(6802, 99.818)
(6803, 98.326)
(6804, 99.324)
(6805, 99.954)
(6806, 99.894)
(6807, 99.14)
(6808, 98.742)
(6809, 99.584)
(6810, 99.808)
(6811, 98.47)
(6812, 99.604)
(6813, 99.432)
(6814, 99.66)
(6815, 99.61)
(6816, 99.952)
(6817, 99.922)
(6818, 99.97)
(6819, 99.982)
(6820, 99.962)
(6821, 99.986)
(6822, 99.99)
(6823, 99.986)
(6824, 99.77)
(6825, 99.988)
(6826, 99.798)
(6827, 99.984)
(6828, 99.996)
(6829, 100)
(6830, 99.976)
(6831, 99.996)
(6832, 100)
(6833, 99.992)
(6834, 99.902)
(6835, 100)
(6836, 100)
(6837, 100)
(6838, 99.888)
(6839, 99.992)
(6840, 100)
(6841, 100)
(6842, 99.952)
(6843, 99.998)
(6844, 89.486)
(6845, 99.998)
(6846, 99.988)
(6847, 99.96)
(6848, 99.952)
(6849, 98.74)
(6850, 99.992)
(6851, 99.95)
(6852, 99.054)
(6853, 93.09)
(6854, 99.998)
(6855, 99.996)
(6856, 99.998)
(6857, 99.992)
(6858, 99.982)
(6859, 100)
(6860, 100)
(6861, 99.802)
(6862, 99.936)
(6863, 99.998)
(6864, 99.97)
(6865, 99.99)
(6866, 99.994)
(6867, 99.962)
(6868, 100)
(6869, 99.986)
(6870, 99.986)
(6871, 99.996)
(6872, 100)
(6873, 100)
(6874, 100)
(6875, 98.952)
(6876, 99.99)
(6877, 99.984)
(6878, 100)
(6879, 99.984)
(6880, 99.992)
(6881, 100)
(6882, 99.972)
(6883, 99.986)
(6884, 99.9)
(6885, 99.96)
(6886, 99.976)
(6887, 99.946)
(6888, 99.942)
(6889, 99.822)
(6890, 99.916)
(6891, 99.974)
(6892, 99.958)
(6893, 99.968)
(6894, 99.806)
(6895, 99.958)
(6896, 99.966)
(6897, 99.896)
(6898, 99.832)
(6899, 99.94)
(6900, 99.892)
(6901, 99.81)
(6902, 99.84)
(6903, 99.796)
(6904, 99.894)
(6905, 99.828)
(6906, 99.222)
(6907, 99.95)
(6908, 99.872)
(6909, 99.668)
(6910, 99.762)
(6911, 99.596)
(6912, 99.67)
(6913, 99.786)
(6914, 99.6)
(6915, 99.798)
(6916, 99.89)
(6917, 99.69)
(6918, 99.812)
(6919, 99.596)
(6920, 99.856)
(6921, 99.75)
(6922, 99.712)
(6923, 99.908)
(6924, 99.846)
(6925, 99.878)
(6926, 99.906)
(6927, 99.866)
(6928, 99.65)
(6929, 99.936)
(6930, 99.818)
(6931, 99.846)
(6932, 99.628)
(6933, 99.132)
(6934, 99.442)
(6935, 99.792)
(6936, 98.858)
(6937, 98.022)
(6938, 99.262)
(6939, 99.746)
(6940, 99.714)
(6941, 99.612)
(6942, 99.53)
(6943, 99.642)
(6944, 99.672)
(6945, 99.756)
(6946, 99.468)
(6947, 99.73)
(6948, 99.726)
(6949, 99.42)
(6950, 99.75)
(6951, 97.474)
(6952, 99.342)
(6953, 99.016)
(6954, 98.452)
(6955, 97.046)
(6956, 97.178)
(6957, 94.036)
(6958, 96.714)
(6959, 97.916)
(6960, 98.344)
(6961, 98.178)
(6962, 96.97)
(6963, 95.72)
(6964, 98.718)
(6965, 98.566)
(6966, 99.344)
(6967, 99.308)
(6968, 99.294)
(6969, 99.09)
(6970, 98.462)
(6971, 97.994)
(6972, 98.11)
(6973, 98.226)
(6974, 97.976)
(6975, 97.956)
(6976, 98.934)
(6977, 97.814)
(6978, 94.558)
(6979, 96.344)
(6980, 98.816)
(6981, 97.61)
(6982, 98.338)
(6983, 98.106)
(6984, 97.406)
(6985, 97.662)
(6986, 96.26)
(6987, 96.784)
(6988, 96.792)
(6989, 98.448)
(6990, 95.984)
(6991, 96.934)
(6992, 95.846)
(6993, 98.812)
(6994, 99.166)
(6995, 98.546)
(6996, 96.976)
(6997, 98.128)
(6998, 98.568)
(6999, 96.194)
(7000, 96.702)
(7001, 98.76)
(7002, 98.214)
(7003, 97.892)
(7004, 98.526)
(7005, 98.24)
(7006, 97.638)
(7007, 94.164)
(7008, 97.266)
(7009, 98.388)
(7010, 97.108)
(7011, 99.16)
(7012, 98.01)
(7013, 97.576)
(7014, 98.038)
(7015, 97.542)
(7016, 98.56)
(7017, 97.62)
(7018, 97.956)
(7019, 96.348)
(7020, 98.456)
(7021, 97.752)
(7022, 97.984)
(7023, 95.964)
(7024, 96.658)
(7025, 97.468)
(7026, 97.35)
(7027, 97.642)
(7028, 92.002)
(7029, 93.65)
(7030, 97.694)
(7031, 93.406)
(7032, 95.314)
(7033, 96.498)
(7034, 97.626)
(7035, 94.882)
(7036, 92.776)
(7037, 92.95)
(7038, 94.204)
(7039, 88.33)
(7040, 74.128)
(7041, 91.75)
(7042, 84.674)
(7043, 80.872)
(7044, 81.032)
(7045, 84.444)
(7046, 91.324)
(7047, 92.132)
(7048, 95.13)
(7049, 95.062)
(7050, 91.67)
(7051, 93.986)
(7052, 88.99)
(7053, 94.652)
(7054, 90.572)
(7055, 94.798)
(7056, 91.476)
(7057, 96.026)
(7058, 91.766)
(7059, 91.794)
(7060, 95.216)
(7061, 94.978)
(7062, 92.348)
(7063, 92.022)
(7064, 85.394)
(7065, 78.658)
(7066, 85.014)
(7067, 89.782)
(7068, 83.51)
(7069, 95.924)
(7070, 92.266)
(7071, 90.042)
(7072, 78.596)
(7073, 89.604)
(7074, 93.818)
(7075, 90.338)
(7076, 97.506)
(7077, 93.596)
(7078, 90.87)
(7079, 92.766)
(7080, 94.054)
(7081, 91.004)
(7082, 97.48)
(7083, 96.23)
(7084, 89.606)
(7085, 93.424)
(7086, 85.02)
(7087, 95.508)
(7088, 96.072)
(7089, 93.24)
(7090, 91.94)
(7091, 92.644)
(7092, 92.074)
(7093, 89.852)
(7094, 90.104)
(7095, 85.622)
(7096, 91.088)
(7097, 91.832)
(7098, 88.562)
(7099, 81.7)
(7100, 91.226)
(7101, 95.116)
(7102, 94.504)
(7103, 96.05)
(7104, 87.066)
(7105, 92.258)
(7106, 94.99)
(7107, 90.318)
(7108, 80.58)
(7109, 86.686)
(7110, 95.9)
(7111, 88.608)
(7112, 94.078)
(7113, 89.182)
(7114, 88.27)
(7115, 83.52)
(7116, 81.356)
(7117, 94.626)
(7118, 89.38)
(7119, 92.682)
(7120, 92.274)
(7121, 92.466)
(7122, 85.7)
(7123, 97.37)
(7124, 96.126)
(7125, 95.694)
(7126, 94.452)
(7127, 90.494)
(7128, 89.646)
(7129, 91.418)
(7130, 77.96)
(7131, 90.756)
(7132, 87.318)
(7133, 89.352)
(7134, 89.116)
(7135, 96.864)
(7136, 88.294)
(7137, 92.842)
(7138, 84.426)
(7139, 92.85)
(7140, 94.544)
(7141, 94.862)
(7142, 95.452)
(7143, 89.892)
(7144, 92.4)
(7145, 97.61)
(7146, 97.892)
(7147, 94.118)
(7148, 95.47)
(7149, 96.088)
(7150, 98.168)
(7151, 96.032)
(7152, 96.888)
(7153, 96.442)
(7154, 97.766)
(7155, 97.616)
(7156, 97.352)
(7157, 98.178)
(7158, 97.274)
(7159, 99.124)
(7160, 99.36)
(7161, 99.538)
(7162, 99.284)
(7163, 98.384)
(7164, 99.234)
(7165, 99.362)
(7166, 96.728)
(7167, 98.402)
(7168, 98.016)
(7169, 94.9)
(7170, 97.842)
(7171, 94.936)
(7172, 91.234)
(7173, 96.996)
(7174, 96.596)
(7175, 97.17)
(7176, 95.978)
(7177, 94.524)
(7178, 96.334)
(7179, 97.462)
(7180, 99.286)
(7181, 98.74)
(7182, 97.49)
(7183, 97.132)
(7184, 97.244)
(7185, 93.022)
(7186, 95.868)
(7187, 94.602)
(7188, 96.904)
(7189, 95.322)
(7190, 96.392)
(7191, 99.14)
(7192, 96.428)
(7193, 96.276)
(7194, 95.704)
(7195, 98.262)
(7196, 97.312)
(7197, 98.38)
(7198, 95.956)
(7199, 97.02)
(7200, 93.206)
(7201, 97.372)
(7202, 96.154)
(7203, 87.152)
(7204, 95.446)
(7205, 95.098)
(7206, 97.198)
(7207, 97.37)
(7208, 94.976)
(7209, 95.964)
(7210, 90.498)
(7211, 84.256)
(7212, 93.95)
(7213, 96.198)
(7214, 98.842)
(7215, 96.022)
(7216, 97.932)
(7217, 92.986)
(7218, 94.592)
(7219, 98.546)
(7220, 97.992)
(7221, 98.564)
(7222, 96.536)
(7223, 97.568)
(7224, 98.364)
(7225, 98.092)
(7226, 92.014)
(7227, 93.12)
(7228, 89.858)
(7229, 93.302)
(7230, 87.53)
(7231, 96.614)
(7232, 91.092)
(7233, 97.464)
(7234, 86.226)
(7235, 76.368)
(7236, 91.614)
(7237, 92.388)
(7238, 87.938)
(7239, 85.278)
(7240, 69.11)
(7241, 91.074)
(7242, 99.458)
(7243, 99.69)
(7244, 99.838)
(7245, 99.194)
(7246, 95.272)
(7247, 99.128)
(7248, 99.23)
(7249, 98.142)
(7250, 98.942)
(7251, 94.696)
(7252, 97.326)
(7253, 96.376)
(7254, 97.836)
(7255, 96.17)
(7256, 96.298)
(7257, 99.368)
(7258, 99.896)
(7259, 99.882)
(7260, 99.928)
(7261, 99.826)
(7262, 99.836)
(7263, 99.856)
(7264, 99.808)
(7265, 99.79)
(7266, 99.354)
(7267, 99.626)
(7268, 98.82)
(7269, 97.962)
(7270, 99.32)
(7271, 98.954)
(7272, 98.402)
(7273, 98.114)
(7274, 98.984)
(7275, 98.674)
(7276, 98.902)
(7277, 99.44)
(7278, 98.584)
(7279, 99.352)
(7280, 98.87)
(7281, 96.41)
(7282, 97.566)
(7283, 98.252)
(7284, 99.02)
(7285, 98.23)
(7286, 98.796)
(7287, 98.908)
(7288, 95.748)
(7289, 98.12)
(7290, 98.598)
(7291, 99.608)
(7292, 99.882)
(7293, 99.418)
(7294, 98.38)
(7295, 99.348)
(7296, 99.776)
(7297, 99.836)
(7298, 99.942)
(7299, 99.946)
(7300, 98.998)
(7301, 97.956)
(7302, 99.584)
(7303, 99.872)
(7304, 99.758)
(7305, 99.816)
(7306, 99.704)
(7307, 98.308)
(7308, 99.566)
(7309, 99.766)
(7310, 99.664)
(7311, 99.724)
(7312, 99.932)
(7313, 99.882)
(7314, 99.126)
(7315, 97.444)
(7316, 98.774)
(7317, 99.364)
(7318, 98.776)
(7319, 99.138)
(7320, 99.252)
(7321, 98.43)
(7322, 99.398)
(7323, 99.652)
(7324, 99.85)
(7325, 99.86)
(7326, 99.822)
(7327, 99.828)
(7328, 98.584)
(7329, 96.732)
(7330, 98.764)
(7331, 99.44)
(7332, 99.472)
(7333, 99.382)
(7334, 99.764)
(7335, 99.134)
(7336, 98.532)
(7337, 98.464)
(7338, 98.812)
(7339, 99.662)
(7340, 99.852)
(7341, 99.342)
(7342, 97.472)
(7343, 98.404)
(7344, 99.162)
(7345, 98.274)
(7346, 97.07)
(7347, 98.844)
(7348, 98.942)
(7349, 98.342)
(7350, 97.832)
(7351, 98.46)
(7352, 96.978)
(7353, 98.662)
(7354, 98.202)
(7355, 95.984)
(7356, 96.874)
(7357, 98.334)
(7358, 94.956)
(7359, 96.458)
(7360, 96.974)
(7361, 94.136)
(7362, 98.94)
(7363, 98.31)
(7364, 98.504)
(7365, 98.54)
(7366, 97.54)
(7367, 95.024)
(7368, 97.226)
(7369, 92.546)
(7370, 92.538)
(7371, 94.122)
(7372, 95.248)
(7373, 96.452)
(7374, 96.588)
(7375, 96.41)
(7376, 94.652)
(7377, 96.064)
(7378, 96.864)
(7379, 96.538)
(7380, 95.176)
(7381, 96.522)
(7382, 96.292)
(7383, 95.502)
(7384, 96.436)
(7385, 95.238)
(7386, 90.82)
(7387, 95.86)
(7388, 97.908)
(7389, 97.93)
(7390, 94.694)
(7391, 96.354)
(7392, 95.604)
(7393, 93.414)
(7394, 94.482)
(7395, 92.958)
(7396, 96.582)
(7397, 97.326)
(7398, 96.966)
(7399, 89.668)
(7400, 91.334)
(7401, 90.786)
(7402, 91.076)
(7403, 93.206)
(7404, 86.296)
(7405, 85.234)
(7406, 93.014)
(7407, 94.314)
(7408, 95.024)
(7409, 94.24)
(7410, 94.98)
(7411, 97.534)
(7412, 90.502)
(7413, 93.668)
(7414, 94.868)
(7415, 95.4)
(7416, 93.072)
(7417, 97.232)
(7418, 97.022)
(7419, 95.096)
(7420, 95.94)
(7421, 95.922)
(7422, 96.526)
(7423, 95.968)
(7424, 94.814)
(7425, 90.364)
(7426, 92.874)
(7427, 95.302)
(7428, 94.692)
(7429, 89.724)
(7430, 94.612)
(7431, 94.538)
(7432, 94.728)
(7433, 97.538)
(7434, 97.668)
(7435, 97.132)
(7436, 96.09)
(7437, 97.684)
(7438, 97.226)
(7439, 98.336)
(7440, 96.744)
(7441, 95.116)
(7442, 93.512)
(7443, 92.486)
(7444, 91.294)
(7445, 94.028)
(7446, 95.816)
(7447, 97.184)
(7448, 96.14)
(7449, 97.304)
(7450, 98.5)
(7451, 97.152)
(7452, 87.9)
(7453, 93.836)
(7454, 89.744)
(7455, 95.024)
(7456, 94.102)
(7457, 94.432)
(7458, 95.742)
(7459, 92.29)
(7460, 95.2)
(7461, 95.862)
(7462, 91.598)
(7463, 92.608)
(7464, 91.084)
(7465, 88.734)
(7466, 93.644)
(7467, 94.574)
(7468, 96.172)
(7469, 97.022)
(7470, 97.446)
(7471, 93.242)
(7472, 93.914)
(7473, 95.412)
(7474, 91.906)
(7475, 94.698)
(7476, 96.3)
(7477, 97.228)
(7478, 86.466)
(7479, 96.836)
(7480, 95.842)
(7481, 96.816)
(7482, 93.19)
(7483, 95.728)
(7484, 98.212)
(7485, 95.07)
(7486, 80.14)
(7487, 96.562)
(7488, 97.402)
(7489, 96.378)
(7490, 88.484)
(7491, 94.222)
(7492, 86.576)
(7493, 91.912)
(7494, 82.832)
(7495, 94.88)
(7496, 94.254)
(7497, 96.042)
(7498, 96.022)
(7499, 97.912)
(7500, 98.658)
(7501, 97.342)
(7502, 94.814)
(7503, 96.3)
(7504, 98.952)
(7505, 97.998)
(7506, 92.734)
(7507, 96.912)
(7508, 94.826)
(7509, 97.096)
(7510, 86.444)
(7511, 96.646)
(7512, 95.886)
(7513, 83.99)
(7514, 89.938)
(7515, 94.188)
(7516, 92.168)
(7517, 86.982)
(7518, 96.146)
(7519, 95.888)
(7520, 89.812)
(7521, 78.816)
(7522, 86.96)
(7523, 91.348)
(7524, 80.782)
(7525, 85.07)
(7526, 67.024)
(7527, 95.978)
(7528, 83.274)
(7529, 89.78)
(7530, 85.084)
(7531, 99.45)
(7532, 99.89)
(7533, 99.902)
(7534, 99.974)
(7535, 99.938)
(7536, 99.788)
(7537, 99.544)
(7538, 99.388)
(7539, 99.53)
(7540, 97.284)
(7541, 99.196)
(7542, 99.57)
(7543, 99.556)
(7544, 99.268)
(7545, 99.592)
(7546, 99.45)
(7547, 99.646)
(7548, 99.614)
(7549, 99.824)
(7550, 99.946)
(7551, 99.284)
(7552, 98.88)
(7553, 99.134)
(7554, 99.302)
(7555, 99.552)
(7556, 99.278)
(7557, 99.502)
(7558, 99.476)
(7559, 99.268)
(7560, 99.656)
(7561, 98.712)
(7562, 99.032)
(7563, 99.648)
(7564, 99.768)
(7565, 99.774)
(7566, 99.744)
(7567, 99.42)
(7568, 99.722)
(7569, 99.758)
(7570, 99.824)
(7571, 97.974)
(7572, 99.528)
(7573, 99.926)
(7574, 99.992)
(7575, 99.812)
(7576, 99.97)
(7577, 99.528)
(7578, 99.922)
(7579, 99.012)
(7580, 99.796)
(7581, 99.994)
(7582, 99.988)
(7583, 99.972)
(7584, 99.606)
(7585, 99.82)
(7586, 99.422)
(7587, 99.214)
(7588, 99.838)
(7589, 99.81)
(7590, 99.998)
(7591, 100)
(7592, 99.998)
(7593, 100)
(7594, 99.996)
(7595, 100)
(7596, 99.998)
(7597, 100)
(7598, 100)
(7599, 99.996)
(7600, 99.992)
(7601, 99.996)
(7602, 99.992)
(7603, 99.98)
(7604, 99.99)
(7605, 99.978)
(7606, 99.978)
(7607, 99.946)
(7608, 99.048)
(7609, 99.964)
(7610, 99.926)
(7611, 99.914)
(7612, 99.964)
(7613, 99.55)
(7614, 98.61)
(7615, 99.632)
(7616, 99.546)
(7617, 99.548)
(7618, 99.798)
(7619, 99.858)
(7620, 99.836)
(7621, 96.644)
(7622, 97.484)
(7623, 97.158)
(7624, 99.346)
(7625, 99.646)
(7626, 99.224)
(7627, 99.548)
(7628, 98.92)
(7629, 99.412)
(7630, 99.326)
(7631, 99.886)
(7632, 99.546)
(7633, 98.798)
(7634, 99.554)
(7635, 99.488)
(7636, 94.884)
(7637, 99.386)
(7638, 99.5)
(7639, 99.17)
(7640, 98.556)
(7641, 98.922)
(7642, 98.79)
(7643, 97.398)
(7644, 97.61)
(7645, 98.04)
(7646, 99.006)
(7647, 96.67)
(7648, 96.998)
(7649, 97.724)
(7650, 97.964)
(7651, 98.458)
(7652, 98.542)
(7653, 99.404)
(7654, 97.84)
(7655, 97.744)
(7656, 96.332)
(7657, 98.564)
(7658, 98.08)
(7659, 95.964)
(7660, 98.936)
(7661, 97.956)
(7662, 99.36)
(7663, 99.156)
(7664, 99.54)
(7665, 99.286)
(7666, 99.444)
(7667, 99.592)
(7668, 98.85)
(7669, 99.588)
(7670, 99.358)
(7671, 99.428)
(7672, 99.58)
(7673, 99.35)
(7674, 99.368)
(7675, 99.476)
(7676, 99.778)
(7677, 98.684)
(7678, 98.092)
(7679, 99.072)
(7680, 98.63)
(7681, 98.942)
(7682, 99.158)
(7683, 99.242)
(7684, 98.464)
(7685, 97.082)
(7686, 95.152)
(7687, 97.026)
(7688, 98.376)
(7689, 97.54)
(7690, 97.634)
(7691, 96.626)
(7692, 96.626)
(7693, 97.8)
(7694, 97.404)
(7695, 94.406)
(7696, 95.68)
(7697, 96.69)
(7698, 96.746)
(7699, 95.464)
(7700, 95.616)
(7701, 95.116)
(7702, 98.138)
(7703, 98.52)
(7704, 96.866)
(7705, 89.07)
(7706, 90.588)
(7707, 98.342)
(7708, 97.754)
(7709, 97.486)
(7710, 97.768)
(7711, 98.04)
(7712, 94.574)
(7713, 96.866)
(7714, 95.788)
(7715, 97.966)
(7716, 99.224)
(7717, 97.832)
(7718, 97.134)
(7719, 97.242)
(7720, 98.078)
(7721, 93.34)
(7722, 98.132)
(7723, 98.292)
(7724, 96.092)
(7725, 96.608)
(7726, 96.442)
(7727, 98.254)
(7728, 99.024)
(7729, 98.466)
(7730, 98.174)
(7731, 97.968)
(7732, 97.012)
(7733, 97.35)
(7734, 96.612)
(7735, 97.834)
(7736, 98.38)
(7737, 97.574)
(7738, 97.098)
(7739, 98.342)
(7740, 92.782)
(7741, 96.066)
(7742, 94.376)
(7743, 94.706)
(7744, 97.012)
(7745, 97.03)
(7746, 98.666)
(7747, 99.322)
(7748, 98.848)
(7749, 95.33)
(7750, 97.768)
(7751, 90.912)
(7752, 93.4)
(7753, 92.556)
(7754, 97.246)
(7755, 96.242)
(7756, 97.508)
(7757, 96.918)
(7758, 97.582)
(7759, 94.336)
(7760, 94.524)
(7761, 97.51)
(7762, 92.98)
(7763, 96.766)
(7764, 97.768)
(7765, 95.896)
(7766, 94.256)
(7767, 97.136)
(7768, 97.294)
(7769, 96.23)
(7770, 96.556)
(7771, 95.262)
(7772, 97.634)
(7773, 91.508)
(7774, 98.602)
(7775, 96.068)
(7776, 98.99)
(7777, 98.424)
(7778, 97.312)
(7779, 94.244)
(7780, 97.556)
(7781, 96.432)
(7782, 96.028)
(7783, 97.114)
(7784, 96.878)
(7785, 94.836)
(7786, 96.694)
(7787, 95.98)
(7788, 96.94)
(7789, 98.466)
(7790, 97.444)
(7791, 98.604)
(7792, 98.796)
(7793, 98.35)
(7794, 98.374)
(7795, 96.722)
(7796, 98.346)
(7797, 98.646)
(7798, 98.604)
(7799, 98.074)
(7800, 98.414)
(7801, 97.384)
(7802, 93.53)
(7803, 96.876)
(7804, 94.568)
(7805, 93.318)
(7806, 96.028)
(7807, 96.622)
(7808, 96.534)
(7809, 95.226)
(7810, 90.198)
(7811, 93.926)
(7812, 90.024)
(7813, 80.71)
(7814, 77.306)
(7815, 74.878)
(7816, 78.588)
(7817, 92.786)
(7818, 88.662)
(7819, 91.298)
(7820, 84.66)
(7821, 93.214)
(7822, 91.076)
(7823, 84.866)
(7824, 88.534)
(7825, 77.004)
(7826, 92.056)
(7827, 83.44)
(7828, 85.652)
(7829, 87.21)
(7830, 63.318)
(7831, 52.09)
(7832, 65.21)
(7833, 86.932)
(7834, 79.094)
(7835, 85.078)
(7836, 81.728)
(7837, 75.068)
(7838, 54.674)
(7839, 69.978)
(7840, 76.4)
(7841, 83.306)
(7842, 74.118)
(7843, 64.476)
(7844, 51.84)
(7845, 43.356)
(7846, 25.114)
(7847, 47.962)
(7848, 57.35)
(7849, 58.084)
(7850, 61.122)
(7851, 28.792)
(7852, 40.538)
(7853, 26.608)
(7854, 69.168)
(7855, 37.03)
(7856, 31.764)
(7857, 57.666)
(7858, 35.106)
(7859, 18.548)
(7860, 7.042)
(7861, 19.146)
(7862, 29.11)
(7863, 10.1)
(7864, 8.372)
(7865, 36.162)
(7866, 6.918)
(7867, 3.54)
(7868, 8.01)
(7869, 38.074)
(7870, 24.254)
(7871, 27.802)
(7872, 17.752)
(7873, 18.976)
(7874, 36.884)
(7875, 24.696)
(7876, 3.306)
(7877, 43.98)
(7878, 48.628)
(7879, 66.398)
(7880, 91.056)
(7881, 99.216)
(7882, 90.006)
(7883, 86.58)
(7884, 87.7)
(7885, 99.06)
(7886, 99.826)
(7887, 84.858)
(7888, 94.186)
(7889, 80.5)
(7890, 90.162)
(7891, 83.22)
(7892, 90.822)
(7893, 74.864)
(7894, 77.11)
(7895, 86.214)
(7896, 84.024)
(7897, 64.632)
(7898, 67.07)
(7899, 72.002)
(7900, 79.63)
(7901, 62.648)
(7902, 72.008)
(7903, 38.954)
(7904, 63.646)
(7905, 43.122)
(7906, 60.77)
(7907, 26.242)
(7908, 53.072)
(7909, 54.276)
(7910, 37.372)
(7911, 55.79)
(7912, 68.18)
(7913, 69.634)
(7914, 86.352)
(7915, 85.284)
(7916, 90.588)
(7917, 66.706)
(7918, 61.374)
(7919, 92.786)
(7920, 81.256)
(7921, 91.912)
(7922, 91.576)
(7923, 90.182)
(7924, 90.684)
(7925, 90.298)
(7926, 80.548)
(7927, 89.542)
(7928, 86.418)
(7929, 90.636)
(7930, 89.946)
(7931, 93.976)
(7932, 90.922)
(7933, 89.476)
(7934, 80.402)
(7935, 89.332)
(7936, 80.532)
(7937, 88.782)
(7938, 87.34)
(7939, 91.396)
(7940, 84.464)
(7941, 86.44)
(7942, 87.338)
(7943, 90.444)
(7944, 89.67)
(7945, 92.044)
(7946, 82.328)
(7947, 88.984)
(7948, 85.968)
(7949, 94.222)
(7950, 95.432)
(7951, 94.806)
(7952, 96.406)
(7953, 96.318)
(7954, 95.052)
(7955, 96.372)
(7956, 95.196)
(7957, 95.366)
(7958, 93.352)
(7959, 92.19)
(7960, 96.188)
(7961, 96.424)
(7962, 94.982)
(7963, 95.114)
(7964, 92.796)
(7965, 94.698)
(7966, 94.59)
(7967, 92.914)
(7968, 98.374)
(7969, 93.406)
(7970, 96.182)
(7971, 93.064)
(7972, 97.532)
(7973, 95.548)
(7974, 97.118)
(7975, 94.252)
(7976, 92.378)
(7977, 97.776)
(7978, 97.454)
(7979, 96.482)
(7980, 95.724)
(7981, 96.554)
(7982, 96.918)
(7983, 89.694)
(7984, 96.976)
(7985, 94.212)
(7986, 94.336)
(7987, 92.988)
(7988, 95.408)
(7989, 94.662)
(7990, 94.818)
(7991, 92.996)
(7992, 80.9)
(7993, 93.648)
(7994, 90.774)
(7995, 92.042)
(7996, 97.468)
(7997, 98.46)
(7998, 98.54)
(7999, 94.646)
(8000, 96.9)
(8001, 99.144)
(8002, 96.936)
(8003, 94.548)
(8004, 94.238)
(8005, 98.066)
(8006, 97.01)
(8007, 97.628)
(8008, 92.908)
(8009, 92.134)
(8010, 96.542)
(8011, 97.514)
(8012, 96.338)
(8013, 97.458)
(8014, 98.024)
(8015, 95.832)
(8016, 98.212)
(8017, 96.52)
(8018, 97.21)
(8019, 94.464)
(8020, 95.7)
(8021, 92.052)
(8022, 96.774)
(8023, 96.45)
(8024, 96.544)
(8025, 96.298)
(8026, 96.512)
(8027, 97.026)
(8028, 98.584)
(8029, 96.668)
(8030, 98.484)
(8031, 97.48)
(8032, 97.088)
(8033, 98.488)
(8034, 97.288)
(8035, 98.026)
(8036, 95.882)
(8037, 98.254)
(8038, 99.148)
(8039, 99.01)
(8040, 98.278)
(8041, 98.646)
(8042, 99.26)
(8043, 94.556)
(8044, 98.698)
(8045, 98.686)
(8046, 98.348)
(8047, 97.838)
(8048, 99.474)
(8049, 99.174)
(8050, 98.238)
(8051, 97.972)
(8052, 95.69)
(8053, 94.898)
(8054, 97.5)
(8055, 98.448)
(8056, 97.788)
(8057, 97.226)
(8058, 98.31)
(8059, 98.26)
(8060, 98.494)
(8061, 94.076)
(8062, 98.016)
(8063, 98.366)
(8064, 97.748)
(8065, 99.324)
(8066, 95.712)
(8067, 82.19)
(8068, 98.594)
(8069, 99.89)
(8070, 99.774)
(8071, 83.252)
(8072, 99.334)
(8073, 99.742)
(8074, 99.806)
(8075, 99.896)
(8076, 94.5)
(8077, 99.552)
(8078, 99.98)
(8079, 99.97)
(8080, 99.98)
(8081, 96.222)
(8082, 99.842)
(8083, 99.956)
(8084, 99.986)
(8085, 100)
(8086, 99.994)
(8087, 99.98)
(8088, 99.998)
(8089, 99.998)
(8090, 99.358)
(8091, 99.886)
(8092, 99.976)
(8093, 99.916)
(8094, 99.824)
(8095, 99.91)
(8096, 99.912)
(8097, 99.942)
(8098, 99.946)
(8099, 97.36)
(8100, 99.868)
(8101, 99.838)
(8102, 99.984)
(8103, 99.496)
(8104, 97.688)
(8105, 99.668)
(8106, 99.502)
(8107, 99.24)
(8108, 99.788)
(8109, 99.824)
(8110, 99.86)
(8111, 99.91)
(8112, 99.914)
(8113, 99.266)
(8114, 99.692)
(8115, 99.662)
(8116, 99.774)
(8117, 99.598)
(8118, 99.942)
(8119, 99.962)
(8120, 99.982)
(8121, 99.924)
(8122, 99.766)
(8123, 99.904)
(8124, 99.806)
(8125, 99.93)
(8126, 99.75)
(8127, 99.704)
(8128, 99.318)
(8129, 99.288)
(8130, 99.116)
(8131, 98.588)
(8132, 99.604)
(8133, 99.696)
(8134, 99.906)
(8135, 99.8)
(8136, 99.334)
(8137, 98.472)
(8138, 99.204)
(8139, 98.98)
(8140, 98.894)
(8141, 96.192)
(8142, 98.476)
(8143, 98.78)
(8144, 98.618)
(8145, 99.104)
(8146, 99.452)
(8147, 99.61)
(8148, 99.726)
(8149, 99.514)
(8150, 99.164)
(8151, 99.258)
(8152, 98.96)
(8153, 99.658)
(8154, 99.594)
(8155, 99.75)
(8156, 99.414)
(8157, 98.984)
(8158, 98.312)
(8159, 98.608)
(8160, 97.536)
(8161, 97.528)
(8162, 95.618)
(8163, 97.822)
(8164, 98.644)
(8165, 98.198)
(8166, 97.732)
(8167, 98.216)
(8168, 97.766)
(8169, 97.69)
(8170, 99.304)
(8171, 99.374)
(8172, 98.528)
(8173, 98.19)
(8174, 98.992)
(8175, 97.978)
(8176, 97.552)
(8177, 98.434)
(8178, 88.55)
(8179, 95.902)
(8180, 98.624)
(8181, 98.922)
(8182, 99.038)
(8183, 97.768)
(8184, 85.744)
(8185, 93.094)
(8186, 98.042)
(8187, 98.77)
(8188, 98.378)
(8189, 97.7)
(8190, 98.972)
(8191, 99.304)
(8192, 98.12)
(8193, 98.966)
(8194, 98.87)
(8195, 98.188)
(8196, 99.206)
(8197, 98.302)
(8198, 98.134)
(8199, 98.596)
(8200, 98.304)
(8201, 98.648)
(8202, 98.29)
(8203, 96.684)
(8204, 98.586)
(8205, 97.866)
(8206, 98.94)
(8207, 99.164)
(8208, 99.1)
(8209, 97.738)
(8210, 98.67)
(8211, 98.172)
(8212, 98.01)
(8213, 99.214)
(8214, 98.97)
(8215, 98.482)
(8216, 97.838)
(8217, 98.756)
(8218, 96.402)
(8219, 99.128)
(8220, 98.924)
(8221, 99.278)
(8222, 99.348)
(8223, 98.872)
(8224, 98.708)
(8225, 97.308)
(8226, 91.948)
(8227, 97.382)
(8228, 97.282)
(8229, 98.74)
(8230, 98.408)
(8231, 98.784)
(8232, 99.414)
(8233, 97.942)
(8234, 98.61)
(8235, 96.764)
(8236, 98.11)
(8237, 97.258)
(8238, 97.546)
(8239, 95.42)
(8240, 96.858)
(8241, 89.622)
(8242, 95.464)
(8243, 96.182)
(8244, 97.436)
(8245, 95.062)
(8246, 84.104)
(8247, 94.514)
(8248, 90.254)
(8249, 97.06)
(8250, 96.154)
(8251, 94.932)
(8252, 97.362)
(8253, 93.118)
(8254, 95.056)
(8255, 94.352)
(8256, 91.932)
(8257, 88.69)
(8258, 86.576)
(8259, 93.018)
(8260, 95.112)
(8261, 96.532)
(8262, 95.804)
(8263, 95.64)
(8264, 92.954)
(8265, 93.978)
(8266, 93.546)
(8267, 95.386)
(8268, 96.178)
(8269, 94.21)
(8270, 96.61)
(8271, 96.656)
(8272, 92.33)
(8273, 94.526)
(8274, 93.534)
(8275, 92.562)
(8276, 78.554)
(8277, 93.706)
(8278, 87.408)
(8279, 90.984)
(8280, 93.192)
(8281, 87.958)
(8282, 84.048)
(8283, 93.998)
(8284, 92.572)
(8285, 92.442)
(8286, 94.146)
(8287, 89.106)
(8288, 94.114)
(8289, 92.15)
(8290, 93.478)
(8291, 94.036)
(8292, 92.146)
(8293, 96.384)
(8294, 95.802)
(8295, 91.846)
(8296, 97.466)
(8297, 90.496)
(8298, 89.884)
(8299, 90.708)
(8300, 92.896)
(8301, 95.782)
(8302, 94.834)
(8303, 91.186)
(8304, 94.95)
(8305, 93.032)
(8306, 94.122)
(8307, 93.044)
(8308, 93.796)
(8309, 93.646)
(8310, 91.058)
(8311, 94.116)
(8312, 96.474)
(8313, 95.088)
(8314, 91.158)
(8315, 95.9)
(8316, 98.278)
(8317, 96.08)
(8318, 96.042)
(8319, 96.542)
(8320, 96.88)
(8321, 97.038)
(8322, 96.338)
(8323, 94.58)
(8324, 97.832)
(8325, 97.412)
(8326, 97.314)
(8327, 97.606)
(8328, 97.458)
(8329, 88.958)
(8330, 99.27)
(8331, 99.628)
(8332, 99.168)
(8333, 87.418)
(8334, 99.544)
(8335, 99.018)
(8336, 99.802)
(8337, 99.81)
(8338, 99.354)
(8339, 87.19)
(8340, 99.732)
(8341, 99.49)
(8342, 99.256)
(8343, 99.6)
(8344, 99.814)
(8345, 99.648)
(8346, 99.666)
(8347, 98.25)
(8348, 86.972)
(8349, 90.588)
(8350, 97.874)
(8351, 98.46)
(8352, 98.638)
(8353, 99.338)
(8354, 98.236)
(8355, 99.622)
(8356, 99.458)
(8357, 99.412)
(8358, 99.73)
(8359, 99.376)
(8360, 98.926)
(8361, 98.84)
(8362, 99.184)
(8363, 99.27)
(8364, 98.88)
(8365, 98.634)
(8366, 99.332)
(8367, 99.314)
(8368, 99.018)
(8369, 99.238)
(8370, 99.71)
(8371, 99.206)
(8372, 99.19)
(8373, 99.342)
(8374, 98.082)
(8375, 99.668)
(8376, 99.882)
(8377, 98.952)
(8378, 98.274)
(8379, 95.844)
(8380, 92.326)
(8381, 96.522)
(8382, 95.882)
(8383, 93.092)
(8384, 91.616)
(8385, 98.092)
(8386, 97.556)
(8387, 96.576)
(8388, 98.212)
(8389, 99.074)
(8390, 97.708)
(8391, 96.684)
(8392, 96.732)
(8393, 97.716)
(8394, 96.44)
(8395, 99.304)
(8396, 99.462)
(8397, 98.78)
(8398, 98.286)
(8399, 99.272)
(8400, 98.526)
(8401, 98.41)
(8402, 98.856)
(8403, 97.09)
(8404, 96.814)
(8405, 94.454)
(8406, 94.096)
(8407, 95.312)
(8408, 94.762)
(8409, 96.728)
(8410, 97.358)
(8411, 99.08)
(8412, 98.958)
(8413, 98.93)
(8414, 99.668)
(8415, 95.954)
(8416, 88.044)
(8417, 99.526)
(8418, 99.404)
(8419, 99.764)
(8420, 99.928)
(8421, 95.392)
(8422, 99.832)
(8423, 99.686)
(8424, 99.768)
(8425, 99.642)
(8426, 99.602)
(8427, 99.632)
(8428, 98.958)
(8429, 98.844)
(8430, 98.068)
(8431, 97.428)
(8432, 98.76)
(8433, 98.932)
(8434, 96.688)
(8435, 98.396)
(8436, 97.164)
(8437, 99.334)
(8438, 99.386)
(8439, 95.95)
(8440, 98.78)
(8441, 98.604)
(8442, 96.982)
(8443, 97.758)
(8444, 92.086)
(8445, 90.754)
(8446, 97.482)
(8447, 94.734)
(8448, 95.85)
(8449, 91.444)
(8450, 97.356)
(8451, 97.306)
(8452, 94.272)
(8453, 96.63)
(8454, 97.252)
(8455, 96.13)
(8456, 97.114)
(8457, 97.046)
(8458, 97.126)
(8459, 96.724)
(8460, 96.074)
(8461, 93.778)
(8462, 94.8)
(8463, 96.198)
(8464, 96.182)
(8465, 94.978)
(8466, 95.298)
(8467, 94.214)
(8468, 82.278)
(8469, 89.25)
(8470, 77.742)
(8471, 90.65)
(8472, 93.862)
(8473, 90.398)
(8474, 93.27)
(8475, 94.288)
(8476, 94.248)
(8477, 94.622)
(8478, 95.034)
(8479, 94.664)
(8480, 94.814)
(8481, 91.176)
(8482, 91.154)
(8483, 89.732)
(8484, 93.274)
(8485, 94.56)
(8486, 95.262)
(8487, 95.206)
(8488, 95.364)
(8489, 94.084)
(8490, 90.286)
(8491, 86.762)
(8492, 92.762)
(8493, 95.52)
(8494, 91.346)
(8495, 93.548)
(8496, 87.072)
(8497, 96.938)
(8498, 97.532)
(8499, 97.914)
(8500, 96.864)
(8501, 93.134)
(8502, 93.792)
(8503, 96.402)
(8504, 94.6)
(8505, 95.752)
(8506, 92.9)
(8507, 92.218)
(8508, 93.22)
(8509, 96.366)
(8510, 93.078)
(8511, 95.488)
(8512, 95.322)
(8513, 81.08)
(8514, 95.938)
(8515, 97.226)
(8516, 98.066)
(8517, 98.302)
(8518, 98.678)
(8519, 97.22)
(8520, 94.876)
(8521, 96.606)
(8522, 97.784)
(8523, 95.696)
(8524, 93.312)
(8525, 96.638)
(8526, 95.708)
(8527, 95.518)
(8528, 92.21)
(8529, 94.684)
(8530, 95.612)
(8531, 95.194)
(8532, 97.524)
(8533, 98.15)
(8534, 98.406)
(8535, 95.852)
(8536, 96.168)
(8537, 96.056)
(8538, 93.59)
(8539, 92.44)
(8540, 90.276)
(8541, 93.256)
(8542, 87.652)
(8543, 94.416)
(8544, 92.148)
(8545, 87.508)
(8546, 97.476)
(8547, 97.092)
(8548, 97.408)
(8549, 96.174)
(8550, 94.096)
(8551, 95.284)
(8552, 97.092)
(8553, 94.73)
(8554, 91.358)
(8555, 93.668)
(8556, 91.63)
(8557, 82.842)
(8558, 89.726)
(8559, 96.606)
(8560, 97.826)
(8561, 97.404)
(8562, 92.422)
(8563, 86.026)
(8564, 92.69)
(8565, 89.77)
(8566, 93.012)
(8567, 86.382)
(8568, 78.092)
(8569, 73.816)
(8570, 93.422)
(8571, 94.33)
(8572, 88.874)
(8573, 93.666)
(8574, 92.084)
(8575, 79.09)
(8576, 83.376)
(8577, 83.182)
(8578, 69.93)
(8579, 77.71)
(8580, 74.658)
(8581, 82.624)
(8582, 92.334)
(8583, 90.782)
(8584, 95.596)
(8585, 88.59)
(8586, 91.666)
(8587, 93.306)
(8588, 77.524)
(8589, 94.114)
(8590, 93.262)
(8591, 87.628)
(8592, 88.134)
(8593, 92.886)
(8594, 87.75)
(8595, 73.554)
(8596, 90.112)
(8597, 86.798)
(8598, 85.832)
(8599, 87.894)
(8600, 90.69)
(8601, 90.246)
(8602, 76.014)
(8603, 76.392)
(8604, 95.814)
(8605, 90.362)
(8606, 83.744)
(8607, 88.41)
(8608, 86)
(8609, 94.064)
(8610, 90.858)
(8611, 93.79)
(8612, 92.796)
(8613, 92.872)
(8614, 87.198)
(8615, 94.312)
(8616, 95.636)
(8617, 94.424)
(8618, 92.454)
(8619, 94.012)
(8620, 95.434)
(8621, 93.65)
(8622, 93.054)
(8623, 91.118)
(8624, 85.56)
(8625, 84.43)
(8626, 86.792)
(8627, 65.43)
(8628, 78.086)
(8629, 39.486)
(8630, 73.296)
(8631, 80.612)
(8632, 56.638)
(8633, 82.132)
(8634, 75.052)
(8635, 70.848)
(8636, 49.86)
(8637, 75.194)
(8638, 73.784)
(8639, 56.81)
(8640, 86.69)
(8641, 66.38)
(8642, 80.174)
(8643, 92.364)
(8644, 93.188)
(8645, 85.668)
(8646, 95.398)
(8647, 82.248)
(8648, 83.676)
(8649, 98.322)
(8650, 98.066)
(8651, 94.756)
(8652, 94.934)
(8653, 97.816)
(8654, 97.392)
(8655, 95.998)
(8656, 97.638)
(8657, 98.416)
(8658, 97.878)
(8659, 95.684)
(8660, 97.914)
(8661, 95.476)
(8662, 96.182)
(8663, 96.86)
(8664, 97.17)
(8665, 94.716)
(8666, 97.39)
(8667, 98.022)
(8668, 87.794)
(8669, 95.566)
(8670, 98.138)
(8671, 98.33)
(8672, 97.802)
(8673, 97.082)
(8674, 91.972)
(8675, 97.24)
(8676, 95.402)
(8677, 97.9)
(8678, 97.982)
(8679, 97.712)
(8680, 96.522)
(8681, 96.67)
(8682, 96.93)
(8683, 98.956)
(8684, 99.082)
(8685, 98.874)
(8686, 97.718)
(8687, 96.058)
(8688, 97.616)
(8689, 95.664)
(8690, 97.92)
(8691, 97.2)
(8692, 98.676)
(8693, 99.162)
(8694, 99.138)
(8695, 98.314)
(8696, 98.558)
(8697, 98.8)
(8698, 97.984)
(8699, 99.12)
(8700, 99.642)
(8701, 99.78)
(8702, 99.244)
(8703, 99.514)
(8704, 99.11)
(8705, 99.302)
(8706, 97.964)
(8707, 97.908)
(8708, 96.92)
(8709, 98.898)
(8710, 98.378)
(8711, 98.982)
(8712, 99.334)
(8713, 98.758)
(8714, 98.004)
(8715, 99.108)
(8716, 99.33)
(8717, 99.298)
(8718, 98.972)
(8719, 97.186)
(8720, 98.99)
(8721, 97.088)
(8722, 97.51)
(8723, 97.418)
(8724, 94.246)
(8725, 96.128)
(8726, 96.49)
(8727, 97.34)
(8728, 97.752)
(8729, 98.154)
(8730, 97.178)
(8731, 98.52)
(8732, 99.118)
(8733, 97.308)
(8734, 95.736)
(8735, 96.518)
(8736, 92.086)
(8737, 95.394)
(8738, 97.36)
(8739, 96.96)
(8740, 95.964)
(8741, 94.408)
(8742, 97.708)
(8743, 98.448)
(8744, 98.45)
(8745, 97.66)
(8746, 95.998)
(8747, 98.23)
(8748, 97.464)
(8749, 97.932)
(8750, 90.638)
(8751, 96.104)
(8752, 94.312)
(8753, 86.752)
(8754, 95.798)
(8755, 91.322)
(8756, 95.064)
(8757, 92.018)
(8758, 89.994)
(8759, 86.36)
(8760, 93.59)
(8761, 93.4)
(8762, 94.026)
(8763, 96.582)
(8764, 95.27)
(8765, 94.718)
(8766, 92.71)
(8767, 94.874)
(8768, 84.628)
(8769, 92.606)
(8770, 88.064)
(8771, 87.528)
(8772, 81.44)
(8773, 87.54)
(8774, 82.874)
(8775, 92.728)
(8776, 93.386)
(8777, 77.202)
(8778, 89.692)
(8779, 93.674)
(8780, 92.076)
(8781, 94.164)
(8782, 84.044)
(8783, 91.956)
(8784, 71.264)
(8785, 76.096)
(8786, 67.28)
(8787, 83.176)
(8788, 81.122)
(8789, 83.7)
(8790, 91.45)
(8791, 85.056)
(8792, 87.528)
(8793, 87.322)
(8794, 84.974)
(8795, 87.646)
(8796, 93.512)
(8797, 92.28)
(8798, 90.664)
(8799, 92.336)
(8800, 89.766)
(8801, 94.966)
(8802, 95.724)
(8803, 94.26)
(8804, 95.834)
(8805, 97.458)
(8806, 96.17)
(8807, 93.436)
(8808, 96.686)
(8809, 95.52)
(8810, 93.45)
(8811, 95.74)
(8812, 93.77)
(8813, 97.4)
(8814, 97.536)
(8815, 94.216)
(8816, 99.196)
(8817, 99.06)
(8818, 88.528)
(8819, 98.956)
(8820, 98.436)
(8821, 98.016)
(8822, 97.838)
(8823, 97.936)
(8824, 97.78)
(8825, 97.482)
(8826, 98.576)
(8827, 99.056)
(8828, 99.454)
(8829, 99.396)
(8830, 97.73)
(8831, 98.262)
(8832, 98.966)
(8833, 98.062)
(8834, 96.556)
(8835, 99.29)
(8836, 98.934)
(8837, 97.886)
(8838, 96.368)
(8839, 97.764)
(8840, 98.232)
(8841, 93.434)
(8842, 97.13)
(8843, 95.35)
(8844, 98.414)
(8845, 99.568)
(8846, 98.722)
(8847, 97.11)
(8848, 98.708)
(8849, 99.586)
(8850, 99.752)
(8851, 99.672)
(8852, 98.246)
(8853, 94.976)
(8854, 98.432)
(8855, 99.32)
(8856, 97.956)
(8857, 98.506)
(8858, 98.432)
(8859, 98.78)
(8860, 97.778)
(8861, 98.458)
(8862, 97.086)
(8863, 97.668)
(8864, 97.304)
(8865, 95.348)
(8866, 97.552)
(8867, 98.674)
(8868, 98.624)
(8869, 98.316)
(8870, 91.922)
(8871, 99.304)
(8872, 99.408)
(8873, 99.136)
(8874, 98.202)
(8875, 98.718)
(8876, 97.724)
(8877, 97.334)
(8878, 98.918)
(8879, 92.57)
(8880, 98.388)
(8881, 98.406)
(8882, 97.9)
(8883, 97.11)
(8884, 96.65)
(8885, 97.84)
(8886, 96.302)
(8887, 95.688)
(8888, 96.224)
(8889, 95.032)
(8890, 98.682)
(8891, 99.024)
(8892, 99.006)
(8893, 98.828)
(8894, 98.396)
(8895, 98.826)
(8896, 98.172)
(8897, 98.732)
(8898, 98.872)
(8899, 98.276)
(8900, 96.92)
(8901, 87.806)
(8902, 95.788)
(8903, 98.834)
(8904, 97.644)
(8905, 98.448)
(8906, 98.268)
(8907, 98.336)
(8908, 97.53)
(8909, 95.12)
(8910, 98.244)
(8911, 98.082)
(8912, 96.232)
(8913, 96.812)
(8914, 98.698)
(8915, 98.938)
(8916, 98.412)
(8917, 97.716)
(8918, 96.912)
(8919, 93.85)
(8920, 95.348)
(8921, 98.588)
(8922, 96.7)
(8923, 97.442)
(8924, 96.93)
(8925, 95.032)
(8926, 96.002)
(8927, 96.744)
(8928, 96.288)
(8929, 98.24)
(8930, 97.934)
(8931, 96.956)
(8932, 95.372)
(8933, 98.038)
(8934, 96.87)
(8935, 97.464)
(8936, 96.4)
(8937, 97.338)
(8938, 98.044)
(8939, 97.444)
(8940, 96.146)
(8941, 98.814)
(8942, 97.876)
(8943, 94.818)
(8944, 96.868)
(8945, 95.932)
(8946, 98.622)
(8947, 99.1)
(8948, 99.382)
(8949, 99.472)
(8950, 99.256)
(8951, 97.948)
(8952, 98.644)
(8953, 99.006)
(8954, 97.746)
(8955, 99.26)
(8956, 99.186)
(8957, 99.124)
(8958, 95.18)
(8959, 94.866)
(8960, 97.076)
(8961, 96.012)
(8962, 95.616)
(8963, 96.206)
(8964, 95.31)
(8965, 91.028)
(8966, 95.406)
(8967, 97.096)
(8968, 96.186)
(8969, 95.35)
(8970, 96.65)
(8971, 93.848)
(8972, 92.158)
(8973, 95.652)
(8974, 95.352)
(8975, 94.658)
(8976, 96.438)
(8977, 96.78)
(8978, 90.046)
(8979, 95.376)
(8980, 88.976)
(8981, 93.202)
(8982, 94.766)
(8983, 94.29)
(8984, 95.406)
(8985, 95.874)
(8986, 87.952)
(8987, 89.13)
(8988, 93.838)
(8989, 94.154)
(8990, 96.28)
(8991, 95.308)
(8992, 97.53)
(8993, 96.996)
(8994, 92.656)
(8995, 97.184)
(8996, 97.208)
(8997, 96.364)
(8998, 92.37)
(8999, 95.402)
(9000, 97.088)
(9001, 88.568)
(9002, 90.868)
(9003, 97.032)
(9004, 98.288)
(9005, 97.724)
(9006, 97.88)
(9007, 98.61)
(9008, 97.008)
(9009, 97.43)
(9010, 98.454)
(9011, 70.658)
(9012, 98.624)
(9013, 97.57)
(9014, 93.084)
(9015, 93.418)
(9016, 95.586)
(9017, 92.606)
(9018, 94.65)
(9019, 85.31)
(9020, 63.848)
(9021, 83.608)
(9022, 86.348)
(9023, 85.09)
(9024, 82.664)
(9025, 90.55)
(9026, 86.442)
(9027, 67.35)
(9028, 70.37)
(9029, 93.336)
(9030, 78.558)
(9031, 87.006)
(9032, 96.204)
(9033, 87.746)
(9034, 97.046)
(9035, 93.594)
(9036, 96.168)
(9037, 93.282)
(9038, 90.794)
(9039, 91.012)
(9040, 94.166)
(9041, 91.834)
(9042, 84.83)
(9043, 77.772)
(9044, 92.184)
(9045, 90.428)
(9046, 96.164)
(9047, 92.622)
(9048, 90.836)
(9049, 89.588)
(9050, 83.164)
(9051, 81.748)
(9052, 88.632)
(9053, 89.33)
(9054, 88.79)
(9055, 86.96)
(9056, 82.892)
(9057, 90.838)
(9058, 77.454)
(9059, 93.292)
(9060, 91.448)
(9061, 64.71)
(9062, 77.964)
(9063, 86.222)
(9064, 93.07)
(9065, 93.672)
(9066, 92.716)
(9067, 95.462)
(9068, 94.058)
(9069, 93.226)
(9070, 90.758)
(9071, 92.756)
(9072, 92.332)
(9073, 94.064)
(9074, 85.158)
(9075, 94.61)
(9076, 91.794)
(9077, 91.934)
(9078, 90.614)
(9079, 89.238)
(9080, 85.114)
(9081, 83.04)
(9082, 78.306)
(9083, 72.956)
(9084, 69.002)
(9085, 93.54)
(9086, 84.08)
(9087, 91.486)
(9088, 90.118)
(9089, 86.63)
(9090, 82.358)
(9091, 91.776)
(9092, 92.682)
(9093, 89.682)
(9094, 93.17)
(9095, 93.244)
(9096, 93.786)
(9097, 84.174)
(9098, 94.356)
(9099, 93.606)
(9100, 93.096)
(9101, 88.014)
(9102, 91.438)
(9103, 89.134)
(9104, 84.894)
(9105, 90.55)
(9106, 86.43)
(9107, 96.18)
(9108, 97.446)
(9109, 97.08)
(9110, 95.736)
(9111, 94.95)
(9112, 94.328)
(9113, 79.756)
(9114, 90.014)
(9115, 86.86)
(9116, 93.168)
(9117, 97.634)
(9118, 96.294)
(9119, 94.394)
(9120, 95.104)
(9121, 97.734)
(9122, 98.086)
(9123, 96.526)
(9124, 95.088)
(9125, 93.568)
(9126, 92.116)
(9127, 95.32)
(9128, 92.204)
(9129, 92.954)
(9130, 89.316)
(9131, 94.698)
(9132, 92.852)
(9133, 97.23)
(9134, 92.966)
(9135, 97.462)
(9136, 95.98)
(9137, 94.302)
(9138, 78.412)
(9139, 96.732)
(9140, 98.538)
(9141, 97.962)
(9142, 98.376)
(9143, 98.486)
(9144, 98.532)
(9145, 97.528)
(9146, 98.02)
(9147, 98.012)
(9148, 98.524)
(9149, 98.102)
(9150, 99.206)
(9151, 99.118)
(9152, 99.14)
(9153, 98.908)
(9154, 98.438)
(9155, 93.628)
(9156, 98.152)
(9157, 99.068)
(9158, 98.956)
(9159, 96.214)
(9160, 90.77)
(9161, 96.812)
(9162, 95.79)
(9163, 94.956)
(9164, 95.158)
(9165, 95.512)
(9166, 94.974)
(9167, 96.42)
(9168, 96.818)
(9169, 97.454)
(9170, 95.782)
(9171, 96.056)
(9172, 94.55)
(9173, 94.096)
(9174, 96.832)
(9175, 91.418)
(9176, 93.752)
(9177, 86.184)
(9178, 97.146)
(9179, 97.412)
(9180, 94.65)
(9181, 92.592)
(9182, 93.404)
(9183, 96.352)
(9184, 96.32)
(9185, 97.534)
(9186, 97.112)
(9187, 98.396)
(9188, 94.124)
(9189, 92.424)
(9190, 97.756)
(9191, 97.39)
(9192, 97.65)
(9193, 97.67)
(9194, 97.342)
(9195, 98.814)
(9196, 97.862)
(9197, 97.548)
(9198, 94.58)
(9199, 96.554)
(9200, 94.294)
(9201, 98.142)
(9202, 99.036)
(9203, 98.938)
(9204, 98.198)
(9205, 98.354)
(9206, 98.024)
(9207, 97.798)
(9208, 89.516)
(9209, 94.618)
(9210, 94.204)
(9211, 94.074)
(9212, 93.688)
(9213, 95.396)
(9214, 95.806)
(9215, 96.45)
(9216, 96.33)
(9217, 96.946)
(9218, 97.94)
(9219, 96.158)
(9220, 97.272)
(9221, 94.598)
(9222, 93.51)
(9223, 93.408)
(9224, 87.496)
(9225, 92.304)
(9226, 89.62)
(9227, 95.278)
(9228, 96.716)
(9229, 96.68)
(9230, 98.072)
(9231, 95.188)
(9232, 94.672)
(9233, 92.874)
(9234, 94.048)
(9235, 96.57)
(9236, 94.724)
(9237, 95.952)
(9238, 97.214)
(9239, 96.794)
(9240, 95.886)
(9241, 96.172)
(9242, 94.574)
(9243, 93.234)
(9244, 90.424)
(9245, 95.87)
(9246, 92.536)
(9247, 86.554)
(9248, 92.506)
(9249, 94.048)
(9250, 95.074)
(9251, 96.268)
(9252, 97.44)
(9253, 98.19)
(9254, 96.638)
(9255, 96.946)
(9256, 95.64)
(9257, 94.62)
(9258, 94.098)
(9259, 94.748)
(9260, 97.472)
(9261, 96.97)
(9262, 93.614)
(9263, 93.74)
(9264, 95.836)
(9265, 96.058)
(9266, 96.572)
(9267, 96.718)
(9268, 95.246)
(9269, 94.62)
(9270, 95.626)
(9271, 96.23)
(9272, 97.274)
(9273, 95.412)
(9274, 97.566)
(9275, 97.102)
(9276, 98.664)
(9277, 98.818)
(9278, 96.662)
(9279, 70.36)
(9280, 0)
};


==> covgraphs/graph.1.errors.tex <==
\addplot [sharp plot,color=darkgreen,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.000113087525631794)
(1, 7.41620106224253e-05)
(2, 2.79432618640242e-05)
(3, 7.20842870543871e-06)
(4, 4.83388748482361e-06)
(5, 2.20493113342831e-06)
(6, 1.56889330647784e-06)
(7, 1.31447817569765e-06)
(8, 8.05647914137268e-07)
(9, 1.10246556671416e-06)
(10, 8.48050435933966e-07)
(11, 9.75258001324061e-07)
(12, 6.78440348747173e-07)
(13, 8.05647914137268e-07)
(14, 1.06006304491746e-06)
(15, 1.39928321929104e-06)
(16, 1.06006304491746e-06)
(17, 1.35688069749435e-06)
(18, 1.61129582827454e-06)
(19, 1.44168574108774e-06)
(20, 1.01766052312076e-06)
(21, 1.61129582827454e-06)
(22, 9.32855479527363e-07)
(23, 1.18727061030755e-06)
(24, 1.10246556671416e-06)
(25, 1.39928321929104e-06)
(26, 6.36037826950475e-07)
(27, 1.27207565390095e-06)
(28, 5.93635305153776e-07)
(29, 1.35688069749435e-06)
(30, 1.01766052312076e-06)
(31, 9.75258001324061e-07)
(32, 8.05647914137268e-07)
(33, 6.36037826950475e-07)
(34, 1.48408826288444e-06)
(35, 6.36037826950475e-07)
(36, 7.20842870543871e-07)
(37, 8.05647914137268e-07)
(38, 8.90452957730665e-07)
(39, 8.48050435933966e-07)
(40, 7.20842870543871e-07)
(41, 1.18727061030755e-06)
(42, 5.93635305153776e-07)
(43, 5.93635305153776e-07)
(44, 1.01766052312076e-06)
(45, 9.75258001324061e-07)
(46, 1.35688069749435e-06)
(47, 9.32855479527363e-07)
(48, 1.06006304491746e-06)
(49, 1.69610087186793e-06)
(50, 9.32855479527363e-07)
(51, 2.5441513078019e-06)
(52, 3.05298156936228e-06)
(53, 5.17310765919719e-06)
(54, 1.11518632325317e-05)
(55, 6.63967019211931e-06)
(56, 6.99340590386069e-06)
(57, 6.61496307403581e-06)
(58, 5.91043838829733e-06)
(59, 5.80308821785072e-06)
(60, 6.30450566207654e-06)
(61, 6.39269698296666e-06)
(62, 6.48316777988652e-06)
(63, 6.28957728418149e-06)
(64, 7.53517836415117e-06)
(65, 1.12347939243397e-05)
(66, 6.892677058575e-06)
(67, 7.05222199980599e-06)
(68, 7.01752115770187e-06)
(69, 9.05472722407869e-06)
(70, 8.4967153326637e-06)
(71, 7.98107568526159e-06)
(72, 9.02435271134851e-06)
(73, 9.57375718271133e-06)
(74, 8.63093517045665e-06)
(75, 1.03361490680512e-05)
(76, 8.99202524647923e-06)
(77, 8.84078594587059e-06)
(78, 1.03562682867246e-05)
(79, 1.06349466333119e-05)
(80, 1.14153717255274e-05)
(81, 1.05112306156144e-05)
(82, 1.1132444537823e-05)
(83, 1.07540966386883e-05)
(84, 1.22222128150793e-05)
(85, 1.04519881109609e-05)
(86, 1.21410068477269e-05)
(87, 1.11192097894332e-05)
(88, 1.21985000230949e-05)
(89, 1.22747444900346e-05)
(90, 1.32138310448304e-05)
(91, 1.23134967005986e-05)
(92, 1.554173147322e-05)
(93, 1.72001191430279e-05)
(94, 1.89199660105581e-05)
(95, 1.81990928527511e-05)
(96, 3.0500447778858e-05)
(97, 4.827636766815e-05)
(98, 8.38249638625005e-05)
(99, 0.000101400846745769)
(100, 0)
};



==> covgraphs/graph.1000.0.tex <==
\addplot[const plot,fill=lightblue,draw=lightblue] coordinates {
(-1, 0)
(0, 93.991)
(1, 97.299)
(2, 97.401)
(3, 95.173)
(4, 96.339)
(5, 97.792)
(6, 97.723)
(7, 96.145)
(8, 97.849)
(9, 97.403)
(10, 96.916)
(11, 97.233)
(12, 96.907)
(13, 97.79)
(14, 96.498)
(15, 98.787)
(16, 98.042)
(17, 97.691)
(18, 97.81)
(19, 98.351)
(20, 98.596)
(21, 98.173)
(22, 97.671)
(23, 96.529)
(24, 97.037)
(25, 95.951)
(26, 96.924)
(27, 95.596)
(28, 96.913)
(29, 98.328)
(30, 96.782)
(31, 96.664)
(32, 95.278)
(33, 96.414)
(34, 98.536)
(35, 94.287)
(36, 96.87)
(37, 96.318)
(38, 94.674)
(39, 95.545)
(40, 94.576)
(41, 96.334)
(42, 95.219)
(43, 93.518)
(44, 93.761)
(45, 94.385)
(46, 94.927)
(47, 89.849)
(48, 93.422)
(49, 95.923)
(50, 93.881)
(51, 96.76)
(52, 94.451)
(53, 94.88)
(54, 94.114)
(55, 96.218)
(56, 95.775)
(57, 94.85)
(58, 98.497)
(59, 96.796)
(60, 94.353)
(61, 94.693)
(62, 90.69)
(63, 91.631)
(64, 90.041)
(65, 91.423)
(66, 88.68)
(67, 89.1)
(68, 89.335)
(69, 90.901)
(70, 94.086)
(71, 89.116)
(72, 92.624)
(73, 85.177)
(74, 86.698)
(75, 89.571)
(76, 94.447)
(77, 94.444)
(78, 95.631)
(79, 88.446)
(80, 90.764)
(81, 85.142)
(82, 90.353)
(83, 93.675)
(84, 96.433)
(85, 92.562)
(86, 85.006)
(87, 93.714)
(88, 91.141)
(89, 95.332)
(90, 84.613)
(91, 91.545)
(92, 87.034)
(93, 80.501)
(94, 85.172)
(95, 89.915)
(96, 92.671)
(97, 91.076)
(98, 91.088)
(99, 92.66)
(100, 90.918)
(101, 89.886)
(102, 96.055)
(103, 95.215)
(104, 96.309)
(105, 97.541)
(106, 97.511)
(107, 97.495)
(108, 97.761)
(109, 97.126)
(110, 97.49)
(111, 98.036)
(112, 96.78)
(113, 98.71)
(114, 97.185)
(115, 96.293)
(116, 94.051)
(117, 96.61)
(118, 95.267)
(119, 95.439)
(120, 96.211)
(121, 96.928)
(122, 90.154)
(123, 88.417)
(124, 88.56)
(125, 83.894)
(126, 82.129)
(127, 91.372)
(128, 94.003)
(129, 88.617)
(130, 30.747)
(131, 54.897)
(132, 39.201)
(133, 64.612)
(134, 68.715)
(135, 80.704)
(136, 86.954)
(137, 82.932)
(138, 86.572)
(139, 81.83)
(140, 89.395)
(141, 90.495)
(142, 91.714)
(143, 95.191)
(144, 93.936)
(145, 93.624)
(146, 93.295)
(147, 96.816)
(148, 94.925)
(149, 94.731)
(150, 98.719)
(151, 97.748)
(152, 98.405)
(153, 97.165)
(154, 96.774)
(155, 97.588)
(156, 96.939)
(157, 95.285)
(158, 93.232)
(159, 93.465)
(160, 94.646)
(161, 93.582)
(162, 88.739)
(163, 85.002)
(164, 93.069)
(165, 95.91)
(166, 95.419)
(167, 94.686)
(168, 96.289)
(169, 96.248)
(170, 92.677)
(171, 93.248)
(172, 88.222)
(173, 93.362)
(174, 95.993)
(175, 94.566)
(176, 97.037)
(177, 96.097)
(178, 96.829)
(179, 97.169)
(180, 98.331)
(181, 97.682)
(182, 97.877)
(183, 97.757)
(184, 97.821)
(185, 96.839)
(186, 96.474)
(187, 95.527)
(188, 96.846)
(189, 97.713)
(190, 98.292)
(191, 98.063)
(192, 97.61)
(193, 96.649)
(194, 97.92)
(195, 98.421)
(196, 98.313)
(197, 98.452)
(198, 99.008)
(199, 99.018)
(200, 99.183)
(201, 99.011)
(202, 98.964)
(203, 99.108)
(204, 97.643)
(205, 98.399)
(206, 95.927)
(207, 96.376)
(208, 99.228)
(209, 99.5)
(210, 99.309)
(211, 99.513)
(212, 99.159)
(213, 98.324)
(214, 99.55)
(215, 99.42)
(216, 99.805)
(217, 99.512)
(218, 97.576)
(219, 99.545)
(220, 99.782)
(221, 99.242)
(222, 99.697)
(223, 96.014)
(224, 94.294)
(225, 91.722)
(226, 97.569)
(227, 99.816)
(228, 99.785)
(229, 100)
(230, 99.989)
(231, 99.882)
(232, 99.991)
(233, 99.933)
(234, 99.988)
(235, 99.873)
(236, 99.921)
(237, 99.994)
(238, 99.993)
(239, 97.645)
(240, 99.818)
(241, 99.135)
(242, 97.937)
(243, 99.473)
(244, 99.538)
(245, 99.626)
(246, 99.559)
(247, 99.239)
(248, 98.705)
(249, 94.188)
(250, 97.97)
(251, 99.108)
(252, 99.738)
(253, 99.073)
(254, 99.492)
(255, 98.969)
(256, 97.562)
(257, 95.011)
(258, 99.384)
(259, 98.316)
(260, 94.814)
(261, 98.136)
(262, 98.345)
(263, 90.969)
(264, 98.214)
(265, 98.996)
(266, 97.799)
(267, 97.965)
(268, 99.297)
(269, 99.053)
(270, 98.568)
(271, 98.387)
(272, 98.126)
(273, 98.993)
(274, 97.987)
(275, 98.513)
(276, 96.858)
(277, 98.227)
(278, 88.928)
(279, 99.475)
(280, 92.988)
(281, 95.246)
(282, 88.132)
(283, 82.341)
(284, 93.157)
(285, 91.14)
(286, 86.929)
(287, 90.093)
(288, 95.038)
(289, 92.726)
(290, 93.72)
(291, 99.634)
(292, 99.737)
(293, 99.811)
(294, 99.713)
(295, 97.541)
(296, 99.345)
(297, 96.619)
(298, 96.214)
(299, 94.138)
(300, 96.608)
(301, 97.883)
(302, 99.767)
(303, 99.43)
(304, 99.044)
(305, 98.666)
(306, 96.235)
(307, 96.886)
(308, 98.258)
(309, 99.374)
(310, 99.812)
(311, 99.801)
(312, 99.885)
(313, 99.763)
(314, 97.195)
(315, 93.785)
(316, 99.908)
(317, 99.897)
(318, 99.664)
(319, 99.589)
(320, 99.742)
(321, 99.584)
(322, 99.719)
(323, 99.826)
(324, 99.846)
(325, 97.559)
(326, 98.503)
(327, 95.897)
(328, 98.711)
(329, 98.338)
(330, 98.997)
(331, 99.959)
(332, 99.9)
(333, 99.656)
(334, 99.756)
(335, 99.752)
(336, 97.506)
(337, 97.548)
(338, 97.866)
(339, 96.401)
(340, 98.711)
(341, 99.489)
(342, 99.183)
(343, 99.906)
(344, 99.957)
(345, 99.814)
(346, 98.652)
(347, 99.567)
(348, 87.073)
(349, 94.148)
(350, 97.895)
(351, 99.165)
(352, 97.46)
(353, 98.263)
(354, 99.28)
(355, 99.546)
(356, 94.634)
(357, 96.022)
(358, 98.24)
(359, 97.566)
(360, 99.556)
(361, 99.557)
(362, 99.185)
(363, 98.275)
(364, 98.383)
(365, 98.546)
(366, 98.422)
(367, 98.076)
(368, 96.393)
(369, 97.094)
(370, 98.046)
(371, 98.242)
(372, 98.276)
(373, 96.489)
(374, 92.482)
(375, 97.793)
(376, 99.43)
(377, 99.697)
(378, 99.482)
(379, 98.242)
(380, 98.364)
(381, 96.159)
(382, 99.04)
(383, 99.936)
(384, 99.465)
(385, 98.955)
(386, 97.671)
(387, 99.642)
(388, 99.357)
(389, 99.993)
(390, 99.985)
(391, 99.128)
(392, 99.902)
(393, 99.954)
(394, 99.476)
(395, 99.509)
(396, 99.498)
(397, 99.568)
(398, 99.245)
(399, 99.785)
(400, 99.975)
(401, 99.508)
(402, 99.709)
(403, 99.34)
(404, 99.61)
(405, 99.455)
(406, 99.973)
(407, 99.851)
(408, 99.846)
(409, 99.357)
(410, 99.673)
(411, 99.411)
(412, 99.588)
(413, 98.669)
(414, 99.096)
(415, 99.191)
(416, 98.711)
(417, 99.13)
(418, 98.919)
(419, 98.698)
(420, 99.018)
(421, 99.077)
(422, 98.154)
(423, 99.001)
(424, 99.221)
(425, 99.466)
(426, 99.748)
(427, 99.562)
(428, 99.512)
(429, 99.74)
(430, 99.83)
(431, 99.948)
(432, 98.522)
(433, 99.571)
(434, 99.487)
(435, 99.26)
(436, 99.628)
(437, 99.339)
(438, 99.763)
(439, 99.622)
(440, 99.295)
(441, 99.444)
(442, 97.835)
(443, 99.628)
(444, 98.851)
(445, 99.277)
(446, 98.007)
(447, 99.192)
(448, 98.735)
(449, 98.529)
(450, 99.231)
(451, 98.235)
(452, 98.715)
(453, 99.609)
(454, 99.657)
(455, 99.474)
(456, 99.586)
(457, 99.456)
(458, 99.618)
(459, 99.527)
(460, 99.713)
(461, 99.575)
(462, 99.171)
(463, 99.865)
(464, 99.622)
(465, 99.499)
(466, 99.725)
(467, 99.313)
(468, 99.671)
(469, 98.942)
(470, 99.362)
(471, 99.347)
(472, 99.312)
(473, 98.553)
(474, 99.756)
(475, 99.64)
(476, 99.866)
(477, 99.948)
(478, 99.968)
(479, 99.99)
(480, 99.844)
(481, 99.817)
(482, 99.007)
(483, 99.399)
(484, 99.78)
(485, 99.933)
(486, 99.796)
(487, 99.57)
(488, 99.844)
(489, 97.961)
(490, 99.586)
(491, 99.103)
(492, 94.869)
(493, 99.557)
(494, 99.751)
(495, 99.792)
(496, 99.712)
(497, 98.639)
(498, 99.639)
(499, 99.711)
(500, 99.509)
(501, 99.403)
(502, 99.424)
(503, 98.905)
(504, 99.569)
(505, 99.684)
(506, 99.726)
(507, 94.647)
(508, 98.145)
(509, 98.147)
(510, 98.385)
(511, 99.257)
(512, 99.09)
(513, 97.973)
(514, 99.47)
(515, 99.845)
(516, 99.645)
(517, 99.385)
(518, 99.08)
(519, 98.513)
(520, 98.034)
(521, 98.333)
(522, 96.713)
(523, 93.956)
(524, 91.149)
(525, 93.968)
(526, 99.93)
(527, 98.25)
(528, 99.978)
(529, 99.85)
(530, 99.609)
(531, 99.882)
(532, 99.82)
(533, 99.834)
(534, 99.907)
(535, 99.957)
(536, 99.977)
(537, 99.974)
(538, 99.946)
(539, 99.965)
(540, 99.771)
(541, 99.447)
(542, 99.993)
(543, 99.957)
(544, 99.536)
(545, 99.753)
(546, 98.625)
(547, 88.818)
(548, 99.515)
(549, 99.235)
(550, 99.555)
(551, 99.336)
(552, 99.735)
(553, 99.95)
(554, 99.614)
(555, 99.708)
(556, 99.264)
(557, 99.748)
(558, 99.984)
(559, 99.977)
(560, 99.757)
(561, 99.972)
(562, 99.666)
(563, 99.997)
(564, 99.968)
(565, 99.825)
(566, 93.909)
(567, 97.601)
(568, 99.995)
(569, 100)
(570, 99.998)
(571, 99.996)
(572, 99.917)
(573, 99.95)
(574, 98.452)
(575, 99.984)
(576, 99.996)
(577, 99.97)
(578, 100)
(579, 99.99)
(580, 99.886)
(581, 100)
(582, 100)
(583, 100)
(584, 99.992)
(585, 99.964)
(586, 99.872)
(587, 99.331)
(588, 99.76)
(589, 99.897)
(590, 99.857)
(591, 99.85)
(592, 99.879)
(593, 99.919)
(594, 99.805)
(595, 98)
(596, 99.432)
(597, 97.978)
(598, 97.902)
(599, 98.48)
(600, 98.206)
(601, 99.24)
(602, 99.783)
(603, 99.666)
(604, 99.628)
(605, 99.547)
(606, 99.43)
(607, 99.566)
(608, 99.888)
(609, 99.409)
(610, 98.952)
(611, 98.317)
(612, 98.32)
(613, 97.794)
(614, 96.491)
(615, 96.553)
(616, 97.167)
(617, 99.135)
(618, 99.275)
(619, 97.807)
(620, 96.106)
(621, 96.995)
(622, 96.12)
(623, 97.718)
(624, 98.214)
(625, 98.72)
(626, 98.433)
(627, 98.828)
(628, 98.627)
(629, 98.823)
(630, 99.134)
(631, 99.58)
(632, 99.287)
(633, 99.572)
(634, 99.885)
(635, 99.911)
(636, 99.992)
(637, 99.879)
(638, 99.434)
(639, 98.531)
(640, 98.724)
(641, 99.331)
(642, 99.07)
(643, 99.349)
(644, 99.389)
(645, 97.578)
(646, 97.969)
(647, 98.481)
(648, 97.64)
(649, 97.729)
(650, 98.835)
(651, 99.559)
(652, 99.363)
(653, 99.479)
(654, 99.006)
(655, 99.818)
(656, 99.793)
(657, 99)
(658, 99.581)
(659, 99.612)
(660, 99.916)
(661, 99.85)
(662, 99.779)
(663, 99.036)
(664, 98.73)
(665, 99.505)
(666, 99.409)
(667, 97.929)
(668, 99.63)
(669, 99.255)
(670, 99.373)
(671, 98.743)
(672, 98.387)
(673, 96.468)
(674, 99.501)
(675, 99.481)
(676, 99.567)
(677, 99.493)
(678, 99.673)
(679, 99.23)
(680, 98.822)
(681, 99.364)
(682, 99.692)
(683, 99.287)
(684, 99.353)
(685, 96.577)
(686, 99.416)
(687, 98.871)
(688, 98.416)
(689, 98.239)
(690, 99.147)
(691, 99.15)
(692, 97.389)
(693, 97.273)
(694, 98.373)
(695, 98.5)
(696, 99.284)
(697, 99.504)
(698, 99.451)
(699, 99.137)
(700, 98.572)
(701, 99.365)
(702, 99.378)
(703, 96.458)
(704, 98.455)
(705, 99.562)
(706, 99.374)
(707, 99.538)
(708, 99.211)
(709, 99.751)
(710, 99.599)
(711, 99.408)
(712, 99.571)
(713, 97.938)
(714, 99.183)
(715, 99.839)
(716, 99.653)
(717, 99.486)
(718, 99.582)
(719, 99.582)
(720, 98.484)
(721, 97.616)
(722, 96.671)
(723, 96.335)
(724, 96.791)
(725, 95.584)
(726, 94.746)
(727, 97.832)
(728, 95.755)
(729, 78.012)
(730, 84.341)
(731, 74.592)
(732, 90.364)
(733, 82.008)
(734, 94.938)
(735, 99.806)
(736, 76.942)
(737, 97.265)
(738, 96.642)
(739, 97.266)
(740, 99.594)
(741, 99.385)
(742, 97.182)
(743, 98.517)
(744, 99.042)
(745, 99.558)
(746, 99.142)
(747, 99.934)
(748, 99.845)
(749, 99.613)
(750, 99.45)
(751, 99.501)
(752, 98.864)
(753, 99.776)
(754, 99.539)
(755, 98.329)
(756, 99.118)
(757, 99.152)
(758, 99.217)
(759, 98.714)
(760, 98.533)
(761, 98.661)
(762, 99.312)
(763, 99.027)
(764, 99.613)
(765, 96.42)
(766, 98.878)
(767, 99.234)
(768, 99.77)
(769, 99.778)
(770, 99.901)
(771, 99.402)
(772, 99.54)
(773, 99.852)
(774, 99.741)
(775, 98.838)
(776, 97.571)
(777, 99.746)
(778, 99.899)
(779, 99.715)
(780, 99.598)
(781, 99.781)
(782, 99.767)
(783, 99.862)
(784, 99.049)
(785, 99.446)
(786, 99.946)
(787, 99.398)
(788, 99.593)
(789, 99.435)
(790, 99.482)
(791, 99.729)
(792, 99.757)
(793, 99.728)
(794, 99.817)
(795, 99.687)
(796, 99.763)
(797, 99.833)
(798, 99.643)
(799, 99.889)
(800, 99.812)
(801, 99.77)
(802, 99.75)
(803, 99.541)
(804, 99.781)
(805, 99.736)
(806, 99.714)
(807, 99.228)
(808, 99.504)
(809, 97.956)
(810, 96.193)
(811, 99.112)
(812, 99.873)
(813, 99.238)
(814, 99.931)
(815, 99.742)
(816, 99.336)
(817, 99.593)
(818, 99.269)
(819, 99.93)
(820, 99.966)
(821, 99.553)
(822, 99.535)
(823, 99.475)
(824, 99.588)
(825, 99.753)
(826, 98.888)
(827, 99.538)
(828, 98.66)
(829, 98.871)
(830, 98.93)
(831, 97.617)
(832, 99.462)
(833, 98.986)
(834, 98.558)
(835, 98.699)
(836, 98.56)
(837, 99.774)
(838, 99.136)
(839, 99.334)
(840, 99.219)
(841, 99.72)
(842, 99.257)
(843, 99.589)
(844, 99.492)
(845, 99.741)
(846, 99.768)
(847, 99.87)
(848, 99.761)
(849, 99.918)
(850, 99.888)
(851, 99.84)
(852, 99.892)
(853, 99.832)
(854, 99.196)
(855, 99.715)
(856, 99.804)
(857, 99.868)
(858, 99.935)
(859, 99.198)
(860, 99.507)
(861, 99.693)
(862, 99.653)
(863, 99.785)
(864, 99.603)
(865, 99.566)
(866, 99.311)
(867, 99.705)
(868, 99.756)
(869, 99.808)
(870, 99.198)
(871, 99.827)
(872, 99.999)
(873, 99.996)
(874, 100)
(875, 99.964)
(876, 99.896)
(877, 100)
(878, 99.973)
(879, 100)
(880, 99.99)
(881, 99.987)
(882, 99.985)
(883, 99.834)
(884, 100)
(885, 99.791)
(886, 99.979)
(887, 99.986)
(888, 99.969)
(889, 99.997)
(890, 99.938)
(891, 99.754)
(892, 99.983)
(893, 99.961)
(894, 99.84)
(895, 99.936)
(896, 99.845)
(897, 99.94)
(898, 99.545)
(899, 99.984)
(900, 99.906)
(901, 99.929)
(902, 99.964)
(903, 99.962)
(904, 99.832)
(905, 99.883)
(906, 99.832)
(907, 99.683)
(908, 99.033)
(909, 99.826)
(910, 96.953)
(911, 99.818)
(912, 99.697)
(913, 99.785)
(914, 99.557)
(915, 99.682)
(916, 99.689)
(917, 99.817)
(918, 99.694)
(919, 99.837)
(920, 98.813)
(921, 99.98)
(922, 99.943)
(923, 99.97)
(924, 99.995)
(925, 99.975)
(926, 99.986)
(927, 99.983)
(928, 99.914)
(929, 99.92)
(930, 99.933)
(931, 99.988)
(932, 99.964)
(933, 99.677)
(934, 98.412)
(935, 99.916)
(936, 99.919)
(937, 99.725)
(938, 99.827)
(939, 99.813)
(940, 99.09)
(941, 99.856)
(942, 99.238)
(943, 99.775)
(944, 99.957)
(945, 99.921)
(946, 99.967)
(947, 99.372)
(948, 99.948)
(949, 99.994)
(950, 99.938)
(951, 99.93)
(952, 99.943)
(953, 99.897)
(954, 99.85)
(955, 99.881)
(956, 99.946)
(957, 99.84)
(958, 99.735)
(959, 99.974)
(960, 99.832)
(961, 99.957)
(962, 99.873)
(963, 99.934)
(964, 99.844)
(965, 99.945)
(966, 99.942)
(967, 94.319)
(968, 97.713)
(969, 98.651)
(970, 97.978)
(971, 98.122)
(972, 98.411)
(973, 97.586)
(974, 97.957)
(975, 97.757)
(976, 98.107)
(977, 98.584)
(978, 98.898)
(979, 99.218)
(980, 96.96)
(981, 98.997)
(982, 99.415)
(983, 99.385)
(984, 99.083)
(985, 99.708)
(986, 99.606)
(987, 98.888)
(988, 98.934)
(989, 99.146)
(990, 98.962)
(991, 98.22)
(992, 96.963)
(993, 94.996)
(994, 93.109)
(995, 97.34)
(996, 97.986)
(997, 99.111)
(998, 98.88)
(999, 99.091)
(1000, 98.971)
(1001, 98.991)
(1002, 99.208)
(1003, 98.549)
(1004, 99.358)
(1005, 99.226)
(1006, 99.235)
(1007, 97.515)
(1008, 98.887)
(1009, 99.001)
(1010, 98.687)
(1011, 98.86)
(1012, 99.386)
(1013, 99.29)
(1014, 99.433)
(1015, 99.263)
(1016, 99.252)
(1017, 99.376)
(1018, 99.454)
(1019, 99.588)
(1020, 99.603)
(1021, 99.366)
(1022, 98.777)
(1023, 99.416)
(1024, 99.069)
(1025, 99.237)
(1026, 99.634)
(1027, 99.52)
(1028, 98.475)
(1029, 97.869)
(1030, 99.417)
(1031, 97.807)
(1032, 96.247)
(1033, 97.647)
(1034, 96.296)
(1035, 97.178)
(1036, 98.651)
(1037, 98.962)
(1038, 98.713)
(1039, 99.354)
(1040, 98.873)
(1041, 98.801)
(1042, 99.252)
(1043, 99.447)
(1044, 99.38)
(1045, 98.846)
(1046, 99.249)
(1047, 99.251)
(1048, 97.134)
(1049, 86.175)
(1050, 99.828)
(1051, 99.67)
(1052, 99.27)
(1053, 98.891)
(1054, 98.779)
(1055, 99.182)
(1056, 99.023)
(1057, 99.452)
(1058, 98.583)
(1059, 99.443)
(1060, 99.155)
(1061, 99.081)
(1062, 98.551)
(1063, 99.987)
(1064, 99.787)
(1065, 99.816)
(1066, 99.715)
(1067, 95.355)
(1068, 99.297)
(1069, 98.355)
(1070, 98.114)
(1071, 97.934)
(1072, 99.553)
(1073, 99.74)
(1074, 97.795)
(1075, 99.278)
(1076, 99.353)
(1077, 99.24)
(1078, 99.701)
(1079, 99.37)
(1080, 99.738)
(1081, 99.832)
(1082, 99.465)
(1083, 99.444)
(1084, 99.937)
(1085, 99.996)
(1086, 99.988)
(1087, 100)
(1088, 99.929)
(1089, 99.976)
(1090, 99.965)
(1091, 99.988)
(1092, 100)
(1093, 99.711)
(1094, 99.508)
(1095, 99.996)
(1096, 90.604)
(1097, 99.976)
(1098, 99.942)
(1099, 99.534)
(1100, 99.967)
(1101, 99.987)
(1102, 99.958)
(1103, 99.609)
(1104, 99.998)
(1105, 99.809)
(1106, 99.909)
(1107, 99.984)
(1108, 99.987)
(1109, 99.932)
(1110, 99.866)
(1111, 99.522)
(1112, 99.842)
(1113, 99.833)
(1114, 99.215)
(1115, 99.915)
(1116, 99.772)
(1117, 99.19)
(1118, 99.727)
(1119, 99.478)
(1120, 98.557)
(1121, 99.033)
(1122, 98.623)
(1123, 98.944)
(1124, 99.354)
(1125, 99.465)
(1126, 99.131)
(1127, 98.509)
(1128, 99.417)
(1129, 99.196)
(1130, 99.061)
(1131, 98.976)
(1132, 99.186)
(1133, 97.791)
(1134, 98.512)
(1135, 98.908)
(1136, 98.578)
(1137, 98.182)
(1138, 99.181)
(1139, 99.061)
(1140, 98.25)
(1141, 96.728)
(1142, 98.189)
(1143, 99.391)
(1144, 99.316)
(1145, 99.611)
(1146, 99.537)
(1147, 99.183)
(1148, 99.26)
(1149, 97.84)
(1150, 99.758)
(1151, 99.664)
(1152, 99.705)
(1153, 99.838)
(1154, 99.813)
(1155, 99.78)
(1156, 99.906)
(1157, 99.301)
(1158, 99.768)
(1159, 99.708)
(1160, 99.829)
(1161, 99.602)
(1162, 99.483)
(1163, 99.84)
(1164, 99.942)
(1165, 99.686)
(1166, 99.534)
(1167, 99.915)
(1168, 99.876)
(1169, 99.559)
(1170, 99.606)
(1171, 99.312)
(1172, 98.942)
(1173, 98.784)
(1174, 99.876)
(1175, 99.795)
(1176, 99.566)
(1177, 99.909)
(1178, 99.889)
(1179, 99.976)
(1180, 99.993)
(1181, 99.958)
(1182, 99.916)
(1183, 99.968)
(1184, 99.968)
(1185, 99.987)
(1186, 99.964)
(1187, 99.849)
(1188, 99.952)
(1189, 99.991)
(1190, 99.921)
(1191, 99.656)
(1192, 99.972)
(1193, 99.554)
(1194, 99.99)
(1195, 99.981)
(1196, 100)
(1197, 100)
(1198, 100)
(1199, 99.996)
(1200, 99.927)
(1201, 99.982)
(1202, 99.959)
(1203, 99.726)
(1204, 99.834)
(1205, 99.726)
(1206, 99.633)
(1207, 99.99)
(1208, 99.989)
(1209, 99.992)
(1210, 100)
(1211, 100)
(1212, 99.979)
(1213, 99.998)
(1214, 99.996)
(1215, 100)
(1216, 100)
(1217, 99.999)
(1218, 100)
(1219, 100)
(1220, 99.994)
(1221, 99.502)
(1222, 100)
(1223, 99.999)
(1224, 99.994)
(1225, 99.999)
(1226, 99.999)
(1227, 99.55)
(1228, 99.992)
(1229, 99.996)
(1230, 99.987)
(1231, 99.853)
(1232, 99.972)
(1233, 99.95)
(1234, 99.966)
(1235, 99.986)
(1236, 99.929)
(1237, 99.751)
(1238, 98.953)
(1239, 99.84)
(1240, 99.882)
(1241, 99.915)
(1242, 99.903)
(1243, 99.96)
(1244, 99.836)
(1245, 99.863)
(1246, 99.984)
(1247, 99.937)
(1248, 99.712)
(1249, 99.33)
(1250, 99.8)
(1251, 99.742)
(1252, 99.864)
(1253, 99.446)
(1254, 99.519)
(1255, 99.907)
(1256, 99.651)
(1257, 99.613)
(1258, 94.915)
(1259, 97.247)
(1260, 96.414)
(1261, 93.562)
(1262, 90.702)
(1263, 88.814)
(1264, 89.383)
(1265, 86.715)
(1266, 91.035)
(1267, 93.017)
(1268, 74.303)
(1269, 84.24)
(1270, 87.849)
(1271, 93.46)
(1272, 93.776)
(1273, 93.15)
(1274, 93.397)
(1275, 91.109)
(1276, 86.973)
(1277, 92.09)
(1278, 91.912)
(1279, 90.624)
(1280, 77.634)
(1281, 88.468)
(1282, 88.833)
(1283, 91.103)
(1284, 90.913)
(1285, 92.661)
(1286, 94.836)
(1287, 97.659)
(1288, 97.509)
(1289, 97.287)
(1290, 98.031)
(1291, 97.856)
(1292, 98.932)
(1293, 96.842)
(1294, 95.058)
(1295, 97.895)
(1296, 97.071)
(1297, 98.351)
(1298, 93.873)
(1299, 98.656)
(1300, 98.446)
(1301, 98.356)
(1302, 97.746)
(1303, 97.983)
(1304, 98.653)
(1305, 98.204)
(1306, 98.372)
(1307, 99.179)
(1308, 98.876)
(1309, 95.792)
(1310, 97.991)
(1311, 98.726)
(1312, 98.367)
(1313, 98.15)
(1314, 97.6)
(1315, 96.65)
(1316, 96.802)
(1317, 95.503)
(1318, 88.714)
(1319, 93.429)
(1320, 95.58)
(1321, 95.64)
(1322, 97.354)
(1323, 97.533)
(1324, 97.027)
(1325, 96.92)
(1326, 95.945)
(1327, 96.592)
(1328, 97.592)
(1329, 97.051)
(1330, 97.637)
(1331, 97.886)
(1332, 97.794)
(1333, 97.49)
(1334, 95.471)
(1335, 95.846)
(1336, 97.171)
(1337, 97.447)
(1338, 96.614)
(1339, 97.533)
(1340, 96.824)
(1341, 98.596)
(1342, 98.105)
(1343, 98.424)
(1344, 96.877)
(1345, 95.397)
(1346, 96.389)
(1347, 96.619)
(1348, 97.333)
(1349, 95.899)
(1350, 96.263)
(1351, 95.241)
(1352, 91.789)
(1353, 93.986)
(1354, 91.565)
(1355, 94.863)
(1356, 89.406)
(1357, 87.733)
(1358, 85.352)
(1359, 87.754)
(1360, 89.69)
(1361, 71.722)
(1362, 84.381)
(1363, 78.765)
(1364, 81.701)
(1365, 90.5)
(1366, 92.43)
(1367, 92.742)
(1368, 95.351)
(1369, 94.632)
(1370, 93.454)
(1371, 86.451)
(1372, 89.858)
(1373, 83.228)
(1374, 82.047)
(1375, 88.744)
(1376, 91.311)
(1377, 90.951)
(1378, 92.801)
(1379, 94.187)
(1380, 93.351)
(1381, 96.392)
(1382, 89.967)
(1383, 92.111)
(1384, 95.064)
(1385, 95.394)
(1386, 96.768)
(1387, 96.756)
(1388, 97.257)
(1389, 96.427)
(1390, 97.87)
(1391, 97.224)
(1392, 98.008)
(1393, 97.867)
(1394, 99.213)
(1395, 97.95)
(1396, 95.893)
(1397, 96.02)
(1398, 96.927)
(1399, 95.497)
(1400, 93.494)
(1401, 94.068)
(1402, 96.131)
(1403, 96.597)
(1404, 94.931)
(1405, 97.18)
(1406, 95.53)
(1407, 95.372)
(1408, 96.046)
(1409, 97.349)
(1410, 95.523)
(1411, 94.788)
(1412, 90.915)
(1413, 76.215)
(1414, 67.391)
(1415, 78.974)
(1416, 71.096)
(1417, 50.519)
(1418, 65.79)
(1419, 53.381)
(1420, 50.691)
(1421, 61.117)
(1422, 78.864)
(1423, 67.147)
(1424, 81.818)
(1425, 75.943)
(1426, 82.647)
(1427, 46.095)
(1428, 62.843)
(1429, 81.436)
(1430, 87.026)
(1431, 86.758)
(1432, 90.963)
(1433, 92.634)
(1434, 87.821)
(1435, 76.85)
(1436, 58.113)
(1437, 69.164)
(1438, 57.213)
(1439, 68.911)
(1440, 60.239)
(1441, 47.012)
(1442, 51.313)
(1443, 68.043)
(1444, 64.005)
(1445, 43.468)
(1446, 40.763)
(1447, 59.23)
(1448, 51.257)
(1449, 53.938)
(1450, 38.737)
(1451, 20.7)
(1452, 18.059)
(1453, 30.948)
(1454, 11.86)
(1455, 10.751)
(1456, 21.994)
(1457, 17.159)
(1458, 19.783)
(1459, 40.144)
(1460, 29.922)
(1461, 59.936)
(1462, 54.954)
(1463, 79.208)
(1464, 66.414)
(1465, 86.644)
(1466, 96.322)
(1467, 95.913)
(1468, 79.969)
(1469, 93.201)
(1470, 91.614)
(1471, 88.276)
(1472, 93.981)
(1473, 95.496)
(1474, 97.676)
(1475, 96.797)
(1476, 96.71)
(1477, 96.077)
(1478, 94.813)
(1479, 93.26)
(1480, 95.323)
(1481, 94.84)
(1482, 95.084)
(1483, 92.259)
(1484, 95.2)
(1485, 95.586)
(1486, 96.781)
(1487, 96.136)
(1488, 97.831)
(1489, 97.272)
(1490, 97.696)
(1491, 95.038)
(1492, 97.799)
(1493, 97.65)
(1494, 97.18)
(1495, 97.048)
(1496, 97.059)
(1497, 98.034)
(1498, 97.012)
(1499, 96.857)
(1500, 98.291)
(1501, 98.579)
(1502, 96.48)
(1503, 96.174)
(1504, 97.876)
(1505, 97.673)
(1506, 97.44)
(1507, 98.798)
(1508, 97.249)
(1509, 97.164)
(1510, 97.609)
(1511, 97.565)
(1512, 97.027)
(1513, 97.804)
(1514, 98.005)
(1515, 98.37)
(1516, 97.88)
(1517, 97.345)
(1518, 95.33)
(1519, 98.193)
(1520, 95.91)
(1521, 97.839)
(1522, 98.038)
(1523, 96.594)
(1524, 98.251)
(1525, 97.988)
(1526, 85.048)
(1527, 96.654)
(1528, 99.335)
(1529, 96.067)
(1530, 90.972)
(1531, 99.43)
(1532, 99.026)
(1533, 99.274)
(1534, 99.054)
(1535, 97.094)
(1536, 95.277)
(1537, 96.968)
(1538, 96.473)
(1539, 94.396)
(1540, 92.149)
(1541, 98.206)
(1542, 99.297)
(1543, 99.358)
(1544, 98.595)
(1545, 97.957)
(1546, 97.743)
(1547, 96.931)
(1548, 96.886)
(1549, 98.549)
(1550, 98.864)
(1551, 96.723)
(1552, 95.213)
(1553, 95.32)
(1554, 96.536)
(1555, 93.572)
(1556, 93.572)
(1557, 75.719)
(1558, 2.34)
(1559, 3.728)
(1560, 3.782)
(1561, 1.82)
(1562, 16.013)
(1563, 8.959)
(1564, 0)
(1565, 3.081)
(1566, 2.556)
(1567, 9.006)
(1568, 25.019)
(1569, 66.267)
(1570, 44.802)
(1571, 78.216)
(1572, 90.708)
(1573, 91.308)
(1574, 90.451)
(1575, 92.827)
(1576, 95.304)
(1577, 96.073)
(1578, 96.731)
(1579, 91.012)
(1580, 97.092)
(1581, 97.917)
(1582, 97.038)
(1583, 96.647)
(1584, 97.691)
(1585, 97.768)
(1586, 98.408)
(1587, 98.408)
(1588, 98.412)
(1589, 91.769)
(1590, 97.419)
(1591, 93.549)
(1592, 90.094)
(1593, 92.336)
(1594, 95.132)
(1595, 91.47)
(1596, 90.685)
(1597, 87.553)
(1598, 77.282)
(1599, 86.886)
(1600, 70.929)
(1601, 41.902)
(1602, 55.083)
(1603, 70.422)
(1604, 78.958)
(1605, 85.835)
(1606, 89.928)
(1607, 86.271)
(1608, 88.71)
(1609, 87.248)
(1610, 74.213)
(1611, 76.659)
(1612, 73.92)
(1613, 82.107)
(1614, 83.887)
(1615, 75.597)
(1616, 67.177)
(1617, 56.831)
(1618, 64.489)
(1619, 66.41)
(1620, 51.725)
(1621, 61.441)
(1622, 66.973)
(1623, 47.463)
(1624, 30.359)
(1625, 34.108)
(1626, 52.459)
(1627, 30.956)
(1628, 14.202)
(1629, 53.495)
(1630, 76.225)
(1631, 71.522)
(1632, 79.79)
(1633, 56.632)
(1634, 62.467)
(1635, 85.916)
(1636, 85.07)
(1637, 90.68)
(1638, 99.991)
(1639, 100)
(1640, 80.798)
(1641, 71.644)
(1642, 65.854)
(1643, 88.36)
(1644, 83.927)
(1645, 78.108)
(1646, 87.599)
(1647, 75.531)
(1648, 81.325)
(1649, 92.93)
(1650, 92.373)
(1651, 89.768)
(1652, 90.568)
(1653, 91.656)
(1654, 94.276)
(1655, 92.472)
(1656, 82.987)
(1657, 87.843)
(1658, 83.983)
(1659, 77.185)
(1660, 91.122)
(1661, 83.072)
(1662, 90)
(1663, 89.989)
(1664, 91.558)
(1665, 92.372)
(1666, 88.864)
(1667, 86.76)
(1668, 92.392)
(1669, 91.145)
(1670, 86.467)
(1671, 91.285)
(1672, 92.11)
(1673, 89.703)
(1674, 91.727)
(1675, 91.068)
(1676, 94.055)
(1677, 87.831)
(1678, 92.751)
(1679, 91.604)
(1680, 95.323)
(1681, 92.022)
(1682, 90.149)
(1683, 92.251)
(1684, 90.004)
(1685, 92.136)
(1686, 92.239)
(1687, 92.868)
(1688, 93.15)
(1689, 90.607)
(1690, 91.89)
(1691, 86.593)
(1692, 76.989)
(1693, 86.537)
(1694, 83.918)
(1695, 88.561)
(1696, 85.439)
(1697, 79.715)
(1698, 77.901)
(1699, 81.769)
(1700, 83.763)
(1701, 77.274)
(1702, 93.253)
(1703, 84.905)
(1704, 77.273)
(1705, 78.671)
(1706, 69.615)
(1707, 84.045)
(1708, 84.579)
(1709, 91.592)
(1710, 94.994)
(1711, 89.851)
(1712, 91.675)
(1713, 88.361)
(1714, 90.783)
(1715, 84.01)
(1716, 88.912)
(1717, 90.572)
(1718, 91.612)
(1719, 89.722)
(1720, 88.764)
(1721, 87.056)
(1722, 80.524)
(1723, 83.296)
(1724, 83.612)
(1725, 83.993)
(1726, 83.651)
(1727, 58.927)
(1728, 81.015)
(1729, 86.263)
(1730, 87.412)
(1731, 90.682)
(1732, 95.241)
(1733, 95.427)
(1734, 89.642)
(1735, 93.762)
(1736, 88.493)
(1737, 92.166)
(1738, 91.913)
(1739, 94.531)
(1740, 95.509)
(1741, 93.035)
(1742, 89.981)
(1743, 90.44)
(1744, 89.402)
(1745, 87.553)
(1746, 85.864)
(1747, 78.369)
(1748, 67.415)
(1749, 55.971)
(1750, 50.528)
(1751, 37.625)
(1752, 30.762)
(1753, 16.95)
(1754, 0)
(1755, 0)
(1756, 1.541)
(1757, 1.54)
(1758, 0)
(1759, 0)
(1760, 0)
(1761, 0)
(1762, 2.08)
(1763, 0)
(1764, 0)
(1765, 0)
(1766, 0)
(1767, 0)
(1768, 0)
(1769, 0)
(1770, 0)
(1771, 0)
(1772, 0)
(1773, 0)
(1774, 0)
(1775, 1.54)
(1776, 0)
(1777, 0)
(1778, 0)
(1779, 0)
(1780, 2.08)
(1781, 3.828)
(1782, 9.587)
(1783, 0)
(1784, 0)
(1785, 3.06)
(1786, 4.038)
(1787, 13.946)
(1788, 0)
(1789, 1.596)
(1790, 2.08)
(1791, 15.838)
(1792, 0.003)
(1793, 0)
(1794, 9.251)
(1795, 2.488)
(1796, 2.346)
(1797, 3.828)
(1798, 1.54)
(1799, 0)
(1800, 8.376)
(1801, 6.717)
(1802, 0)
(1803, 0)
(1804, 7.058)
(1805, 4.56)
(1806, 0)
(1807, 0)
(1808, 4.656)
(1809, 0)
(1810, 2.08)
(1811, 5.166)
(1812, 0)
(1813, 0)
(1814, 0)
(1815, 0)
(1816, 0)
(1817, 0)
(1818, 5.05)
(1819, 0)
(1820, 0)
(1821, 0)
(1822, 0)
(1823, 0)
(1824, 0)
(1825, 0)
(1826, 0)
(1827, 0)
(1828, 0)
(1829, 0)
(1830, 0)
(1831, 2.278)
(1832, 0)
(1833, 0)
(1834, 0)
(1835, 0)
(1836, 0)
(1837, 0)
(1838, 0)
(1839, 1.653)
(1840, 0.595)
(1841, 1.485)
(1842, 4.186)
(1843, 2.85)
(1844, 0)
(1845, 4.278)
(1846, 0)
(1847, 2.485)
(1848, 0)
(1849, 0)
(1850, 2.574)
(1851, 23.941)
(1852, 3.43)
(1853, 8.351)
(1854, 0)
(1855, 0)
(1856, 0)
(1857, 0)
(1858, 0)
(1859, 11.611)
(1860, 7.756)
(1861, 0)
(1862, 7.198)
(1863, 40.444)
(1864, 38.918)
(1865, 48.985)
(1866, 52.309)
(1867, 52.87)
(1868, 49.389)
(1869, 81.571)
(1870, 54.889)
(1871, 52.073)
(1872, 58.316)
(1873, 53.138)
(1874, 40.171)
(1875, 35.913)
(1876, 68.112)
(1877, 63.738)
(1878, 65.038)
(1879, 52.352)
(1880, 68.668)
(1881, 80.499)
(1882, 79.499)
(1883, 82.711)
(1884, 88.504)
(1885, 87.952)
(1886, 85.704)
(1887, 84.797)
(1888, 69.196)
(1889, 71.76)
(1890, 83.036)
(1891, 84.989)
(1892, 94.27)
(1893, 91.791)
(1894, 91.301)
(1895, 91.598)
(1896, 93.959)
(1897, 94.037)
(1898, 93.033)
(1899, 95.96)
(1900, 96.202)
(1901, 98.026)
(1902, 96.368)
(1903, 97.683)
(1904, 97.121)
(1905, 99.058)
(1906, 99.432)
(1907, 99.178)
(1908, 97.865)
(1909, 96.013)
(1910, 97.732)
(1911, 95.741)
(1912, 97.328)
(1913, 96.278)
(1914, 96.607)
(1915, 96.097)
(1916, 95.399)
(1917, 95.489)
(1918, 97.188)
(1919, 96.402)
(1920, 98.416)
(1921, 98.522)
(1922, 97.759)
(1923, 98.468)
(1924, 97.865)
(1925, 98.323)
(1926, 98.52)
(1927, 98.343)
(1928, 98.505)
(1929, 98.142)
(1930, 97.693)
(1931, 97.478)
(1932, 98.194)
(1933, 98.877)
(1934, 98.849)
(1935, 98.54)
(1936, 98.127)
(1937, 98.508)
(1938, 98.554)
(1939, 98.85)
(1940, 99.254)
(1941, 99.069)
(1942, 98.971)
(1943, 98.667)
(1944, 99.391)
(1945, 98.645)
(1946, 98.388)
(1947, 98.542)
(1948, 98.742)
(1949, 98.5)
(1950, 99.488)
(1951, 99.003)
(1952, 99.388)
(1953, 98.826)
(1954, 99.236)
(1955, 98.687)
(1956, 98.307)
(1957, 99.193)
(1958, 99.037)
(1959, 99.419)
(1960, 99.579)
(1961, 98.949)
(1962, 98.692)
(1963, 98.929)
(1964, 99.088)
(1965, 98.555)
(1966, 98.36)
(1967, 97.808)
(1968, 98.437)
(1969, 96.496)
(1970, 99.306)
(1971, 98.011)
(1972, 98.053)
(1973, 98.387)
(1974, 98.395)
(1975, 98.75)
(1976, 99.221)
(1977, 99.491)
(1978, 99.438)
(1979, 98.55)
(1980, 99.406)
(1981, 99.394)
(1982, 99.132)
(1983, 98.088)
(1984, 99.636)
(1985, 99.711)
(1986, 99.716)
(1987, 99.453)
(1988, 99.449)
(1989, 99.376)
(1990, 99.029)
(1991, 98.62)
(1992, 99.652)
(1993, 99.47)
(1994, 99.45)
(1995, 98.615)
(1996, 97.753)
(1997, 99.151)
(1998, 99.612)
(1999, 99.164)
(2000, 99.746)
(2001, 99.673)
(2002, 99.308)
(2003, 99.594)
(2004, 99.675)
(2005, 99.167)
(2006, 98.976)
(2007, 99.771)
(2008, 99.778)
(2009, 99.985)
(2010, 99.857)
(2011, 99.587)
(2012, 99.316)
(2013, 98.179)
(2014, 99.216)
(2015, 99.074)
(2016, 99.772)
(2017, 99.749)
(2018, 99.781)
(2019, 99.731)
(2020, 99.893)
(2021, 99.989)
(2022, 99.997)
(2023, 99.98)
(2024, 99.963)
(2025, 99.997)
(2026, 99.859)
(2027, 99.606)
(2028, 99.763)
(2029, 99.786)
(2030, 99.836)
(2031, 99.943)
(2032, 99.994)
(2033, 99.982)
(2034, 99.888)
(2035, 99.995)
(2036, 99.977)
(2037, 99.769)
(2038, 99.735)
(2039, 99.991)
(2040, 99.993)
(2041, 99.983)
(2042, 99.996)
(2043, 99.899)
(2044, 99.826)
(2045, 99.975)
(2046, 99.579)
(2047, 99.985)
(2048, 99.99)
(2049, 99.996)
(2050, 100)
(2051, 99.98)
(2052, 99.999)
(2053, 99.983)
(2054, 99.994)
(2055, 100)
(2056, 99.989)
(2057, 99.975)
(2058, 99.996)
(2059, 99.981)
(2060, 99.965)
(2061, 99.961)
(2062, 98.976)
(2063, 99.937)
(2064, 90.285)
(2065, 95.566)
(2066, 99.907)
(2067, 96.415)
(2068, 98.96)
(2069, 98.282)
(2070, 97.84)
(2071, 99.19)
(2072, 99.476)
(2073, 99.917)
(2074, 99.847)
(2075, 99.539)
(2076, 99.992)
(2077, 99.984)
(2078, 99.962)
(2079, 99.976)
(2080, 99.923)
(2081, 99.932)
(2082, 99.896)
(2083, 99.877)
(2084, 99.784)
(2085, 99.808)
(2086, 99.758)
(2087, 99.917)
(2088, 98.981)
(2089, 98.275)
(2090, 98.711)
(2091, 99.583)
(2092, 99.319)
(2093, 99.292)
(2094, 98.445)
(2095, 99.943)
(2096, 99.926)
(2097, 99.976)
(2098, 99.916)
(2099, 99.954)
(2100, 98.439)
(2101, 99.997)
(2102, 99.989)
(2103, 99.989)
(2104, 99.983)
(2105, 99.983)
(2106, 99.963)
(2107, 99.963)
(2108, 99.757)
(2109, 99.67)
(2110, 99.746)
(2111, 98.881)
(2112, 99.005)
(2113, 98.76)
(2114, 98.081)
(2115, 98.709)
(2116, 96.755)
(2117, 98.109)
(2118, 97.144)
(2119, 96.878)
(2120, 97.826)
(2121, 97.935)
(2122, 93.143)
(2123, 95.563)
(2124, 95.135)
(2125, 96.888)
(2126, 98.474)
(2127, 98.765)
(2128, 98.418)
(2129, 96.806)
(2130, 96.305)
(2131, 98.175)
(2132, 97.615)
(2133, 96.309)
(2134, 96.29)
(2135, 98.749)
(2136, 97.485)
(2137, 97.492)
(2138, 96.705)
(2139, 94.22)
(2140, 97.948)
(2141, 97.024)
(2142, 97.552)
(2143, 97.767)
(2144, 98.312)
(2145, 94.034)
(2146, 94.019)
(2147, 97.314)
(2148, 98.367)
(2149, 97.461)
(2150, 98.366)
(2151, 99.024)
(2152, 96.596)
(2153, 95.093)
(2154, 98.138)
(2155, 96.52)
(2156, 94.475)
(2157, 95.891)
(2158, 97.321)
(2159, 95.482)
(2160, 98.775)
(2161, 97.466)
(2162, 98.631)
(2163, 99.429)
(2164, 99.074)
(2165, 99.654)
(2166, 99.622)
(2167, 99.52)
(2168, 95.94)
(2169, 95.114)
(2170, 99.551)
(2171, 94.004)
(2172, 99.46)
(2173, 99.073)
(2174, 98.539)
(2175, 98.989)
(2176, 99.147)
(2177, 99.273)
(2178, 98.671)
(2179, 97.346)
(2180, 99.364)
(2181, 98.904)
(2182, 98.401)
(2183, 99.029)
(2184, 99.584)
(2185, 99.723)
(2186, 99.734)
(2187, 96.031)
(2188, 99.708)
(2189, 99.578)
(2190, 99.311)
(2191, 98.962)
(2192, 98.869)
(2193, 98.456)
(2194, 98.893)
(2195, 99.517)
(2196, 99.122)
(2197, 98.36)
(2198, 97.792)
(2199, 98.001)
(2200, 99.614)
(2201, 99.691)
(2202, 99.686)
(2203, 98.467)
(2204, 98.661)
(2205, 98.677)
(2206, 99.092)
(2207, 96.816)
(2208, 99.081)
(2209, 99.899)
(2210, 99.795)
(2211, 99.793)
(2212, 99.575)
(2213, 99.131)
(2214, 98.675)
(2215, 98.961)
(2216, 96.693)
(2217, 98.386)
(2218, 99.008)
(2219, 99.14)
(2220, 98.342)
(2221, 98.958)
(2222, 97.997)
(2223, 99.524)
(2224, 98.978)
(2225, 98.988)
(2226, 98.936)
(2227, 93.32)
(2228, 99.616)
(2229, 99.143)
(2230, 99.626)
(2231, 99.912)
(2232, 99.68)
(2233, 99.765)
(2234, 99.764)
(2235, 99.899)
(2236, 99.92)
(2237, 99.915)
(2238, 99.8)
(2239, 99.882)
(2240, 98.831)
(2241, 99.941)
(2242, 99.678)
(2243, 99.527)
(2244, 99.814)
(2245, 99.623)
(2246, 99.905)
(2247, 99.684)
(2248, 99.598)
(2249, 99.817)
(2250, 99.559)
(2251, 99.872)
(2252, 99.548)
(2253, 99.93)
(2254, 99.808)
(2255, 99.848)
(2256, 99.507)
(2257, 99.846)
(2258, 99.2)
(2259, 99.154)
(2260, 99.157)
(2261, 99.662)
(2262, 99.191)
(2263, 99.628)
(2264, 99.771)
(2265, 99.288)
(2266, 99.805)
(2267, 99.983)
(2268, 99.927)
(2269, 99.934)
(2270, 99.907)
(2271, 99.858)
(2272, 99.739)
(2273, 99.673)
(2274, 99.754)
(2275, 99.952)
(2276, 99.531)
(2277, 98.954)
(2278, 99.647)
(2279, 99.889)
(2280, 99.747)
(2281, 99.973)
(2282, 99.849)
(2283, 99.961)
(2284, 99.945)
(2285, 99.908)
(2286, 99.923)
(2287, 98.558)
(2288, 99.903)
(2289, 99.633)
(2290, 98.215)
(2291, 99.042)
(2292, 99.065)
(2293, 99.302)
(2294, 98.743)
(2295, 99.075)
(2296, 98.823)
(2297, 98.672)
(2298, 97.427)
(2299, 98.725)
(2300, 94.724)
(2301, 99.101)
(2302, 93.971)
(2303, 99.024)
(2304, 98.831)
(2305, 99.01)
(2306, 99.4)
(2307, 97.943)
(2308, 97.825)
(2309, 99.54)
(2310, 99.742)
(2311, 99.814)
(2312, 99.589)
(2313, 99.873)
(2314, 99.941)
(2315, 99.593)
(2316, 99.825)
(2317, 99.876)
(2318, 99.859)
(2319, 99.867)
(2320, 99.735)
(2321, 99.789)
(2322, 99.383)
(2323, 99.777)
(2324, 99.236)
(2325, 99.819)
(2326, 99.51)
(2327, 99.864)
(2328, 98.887)
(2329, 99.079)
(2330, 99.542)
(2331, 98.256)
(2332, 98.706)
(2333, 99.784)
(2334, 99.909)
(2335, 99.571)
(2336, 99.704)
(2337, 99.631)
(2338, 99.686)
(2339, 99.486)
(2340, 99.579)
(2341, 99.871)
(2342, 99.957)
(2343, 99.509)
(2344, 99.766)
(2345, 99.573)
(2346, 99.83)
(2347, 99.921)
(2348, 99.916)
(2349, 98.743)
(2350, 99.285)
(2351, 99.153)
(2352, 99.633)
(2353, 99.149)
(2354, 99.925)
(2355, 98.717)
(2356, 99.521)
(2357, 99.641)
(2358, 99.832)
(2359, 99.629)
(2360, 99.786)
(2361, 99.63)
(2362, 99.849)
(2363, 99.974)
(2364, 99.716)
(2365, 99.26)
(2366, 99.709)
(2367, 99.908)
(2368, 99.741)
(2369, 99.831)
(2370, 99.809)
(2371, 99.971)
(2372, 99.145)
(2373, 98.936)
(2374, 99.522)
(2375, 99.539)
(2376, 99.069)
(2377, 98.85)
(2378, 99.768)
(2379, 99.959)
(2380, 99.873)
(2381, 99.991)
(2382, 99.958)
(2383, 99.911)
(2384, 99.904)
(2385, 99.99)
(2386, 99.98)
(2387, 99.961)
(2388, 98.77)
(2389, 99.637)
(2390, 99.205)
(2391, 99.598)
(2392, 98.957)
(2393, 98.988)
(2394, 98.136)
(2395, 99.236)
(2396, 99.599)
(2397, 99.556)
(2398, 99.307)
(2399, 99.386)
(2400, 99.267)
(2401, 99.834)
(2402, 99.795)
(2403, 99.736)
(2404, 99.906)
(2405, 99.958)
(2406, 99.88)
(2407, 99.737)
(2408, 99.447)
(2409, 99.41)
(2410, 99.736)
(2411, 99.845)
(2412, 99.335)
(2413, 98.775)
(2414, 99.603)
(2415, 99.678)
(2416, 99.668)
(2417, 99.7)
(2418, 99.567)
(2419, 99.797)
(2420, 99.542)
(2421, 99.895)
(2422, 99.805)
(2423, 99.844)
(2424, 99.886)
(2425, 99.872)
(2426, 99.913)
(2427, 99.647)
(2428, 99.913)
(2429, 98.975)
(2430, 98.957)
(2431, 99.689)
(2432, 99.594)
(2433, 98.838)
(2434, 99.307)
(2435, 99.491)
(2436, 99.537)
(2437, 99.106)
(2438, 99.408)
(2439, 99.288)
(2440, 98.879)
(2441, 99.797)
(2442, 99.632)
(2443, 99.665)
(2444, 98.727)
(2445, 99.248)
(2446, 99.801)
(2447, 99.533)
(2448, 99.981)
(2449, 99.962)
(2450, 98.956)
(2451, 99.719)
(2452, 99.928)
(2453, 99.967)
(2454, 99.976)
(2455, 99.97)
(2456, 99.857)
(2457, 99.595)
(2458, 99.892)
(2459, 99.976)
(2460, 99.985)
(2461, 100)
(2462, 99.96)
(2463, 99.947)
(2464, 99.995)
(2465, 99.994)
(2466, 100)
(2467, 100)
(2468, 100)
(2469, 99.99)
(2470, 99.961)
(2471, 99.989)
(2472, 99.898)
(2473, 99.999)
(2474, 100)
(2475, 100)
(2476, 99.992)
(2477, 99.999)
(2478, 99.994)
(2479, 100)
(2480, 99.998)
(2481, 100)
(2482, 100)
(2483, 100)
(2484, 100)
(2485, 100)
(2486, 99.999)
(2487, 99.95)
(2488, 99.972)
(2489, 99.725)
(2490, 99.994)
(2491, 100)
(2492, 99.999)
(2493, 99.998)
(2494, 99.996)
(2495, 99.957)
(2496, 99.915)
(2497, 99.959)
(2498, 99.995)
(2499, 99.954)
(2500, 99.945)
(2501, 99.234)
(2502, 99.631)
(2503, 99.583)
(2504, 99.622)
(2505, 99.385)
(2506, 99.939)
(2507, 99.922)
(2508, 99.624)
(2509, 99.911)
(2510, 99.987)
(2511, 99.968)
(2512, 99.703)
(2513, 99.982)
(2514, 99.989)
(2515, 99.533)
(2516, 99.997)
(2517, 99.946)
(2518, 99.97)
(2519, 99.9)
(2520, 100)
(2521, 99.992)
(2522, 99.935)
(2523, 99.644)
(2524, 99.887)
(2525, 99.867)
(2526, 99.897)
(2527, 99.713)
(2528, 99.509)
(2529, 99.921)
(2530, 99.621)
(2531, 99.92)
(2532, 99.945)
(2533, 98.69)
(2534, 99.894)
(2535, 99.955)
(2536, 99.735)
(2537, 99.337)
(2538, 98.607)
(2539, 99.295)
(2540, 99.202)
(2541, 98.944)
(2542, 99.349)
(2543, 99.446)
(2544, 99.376)
(2545, 98.088)
(2546, 99.556)
(2547, 99.533)
(2548, 99.595)
(2549, 99.572)
(2550, 99.797)
(2551, 98.372)
(2552, 98.892)
(2553, 97.127)
(2554, 98.817)
(2555, 99.107)
(2556, 99.626)
(2557, 98.894)
(2558, 99.945)
(2559, 99.975)
(2560, 99.948)
(2561, 99.892)
(2562, 99.986)
(2563, 99.913)
(2564, 99.718)
(2565, 99.833)
(2566, 99.766)
(2567, 99.835)
(2568, 97.848)
(2569, 98.967)
(2570, 98.802)
(2571, 99.094)
(2572, 99.404)
(2573, 99.92)
(2574, 99.861)
(2575, 98.978)
(2576, 99.935)
(2577, 99.835)
(2578, 99.656)
(2579, 99.667)
(2580, 99.675)
(2581, 99.68)
(2582, 99.477)
(2583, 99.75)
(2584, 99.902)
(2585, 99.931)
(2586, 99.889)
(2587, 99.91)
(2588, 99.697)
(2589, 99.895)
(2590, 99.964)
(2591, 99.737)
(2592, 99.775)
(2593, 99.338)
(2594, 99.853)
(2595, 99.951)
(2596, 99.78)
(2597, 99.54)
(2598, 99.981)
(2599, 99.897)
(2600, 99.51)
(2601, 99.526)
(2602, 99.861)
(2603, 98.953)
(2604, 99.805)
(2605, 99.828)
(2606, 98.684)
(2607, 99.859)
(2608, 99.194)
(2609, 97.896)
(2610, 99.968)
(2611, 99.873)
(2612, 99.809)
(2613, 99.191)
(2614, 99.883)
(2615, 99.758)
(2616, 99.919)
(2617, 98.602)
(2618, 99.973)
(2619, 99.989)
(2620, 99.936)
(2621, 99.989)
(2622, 99.821)
(2623, 99.989)
(2624, 99.528)
(2625, 99.999)
(2626, 100)
(2627, 100)
(2628, 99.926)
(2629, 99.977)
(2630, 99.964)
(2631, 99.985)
(2632, 99.951)
(2633, 99.876)
(2634, 99.982)
(2635, 99.979)
(2636, 99.985)
(2637, 99.958)
(2638, 99.941)
(2639, 99.885)
(2640, 98.741)
(2641, 99.906)
(2642, 99.919)
(2643, 99.448)
(2644, 99.86)
(2645, 99.7)
(2646, 99.941)
(2647, 99.831)
(2648, 99.885)
(2649, 99.886)
(2650, 99.905)
(2651, 99.436)
(2652, 99.958)
(2653, 99.035)
(2654, 99.943)
(2655, 99.708)
(2656, 97.845)
(2657, 99.889)
(2658, 99.918)
(2659, 99.912)
(2660, 99.609)
(2661, 99.27)
(2662, 99.617)
(2663, 99.799)
(2664, 99.713)
(2665, 99.694)
(2666, 99.964)
(2667, 99.866)
(2668, 99.683)
(2669, 99.601)
(2670, 99.649)
(2671, 99.929)
(2672, 99.297)
(2673, 99.719)
(2674, 99.707)
(2675, 99.605)
(2676, 99.656)
(2677, 99.758)
(2678, 99.707)
(2679, 99.731)
(2680, 99.331)
(2681, 99.857)
(2682, 99.896)
(2683, 99.978)
(2684, 99.911)
(2685, 99.954)
(2686, 99.659)
(2687, 99.784)
(2688, 99.926)
(2689, 99.98)
(2690, 99.87)
(2691, 98.243)
(2692, 98.897)
(2693, 99.878)
(2694, 99.984)
(2695, 99.968)
(2696, 99.623)
(2697, 99.868)
(2698, 99.976)
(2699, 99.909)
(2700, 99.935)
(2701, 99.913)
(2702, 99.923)
(2703, 99.843)
(2704, 99.862)
(2705, 99.945)
(2706, 99.993)
(2707, 99.978)
(2708, 99.964)
(2709, 99.959)
(2710, 99.604)
(2711, 99.722)
(2712, 99.997)
(2713, 99.992)
(2714, 100)
(2715, 99.947)
(2716, 99.916)
(2717, 99.983)
(2718, 99.764)
(2719, 99.959)
(2720, 100)
(2721, 100)
(2722, 99.948)
(2723, 100)
(2724, 99.997)
(2725, 99.99)
(2726, 99.983)
(2727, 99.989)
(2728, 99.762)
(2729, 99.974)
(2730, 99.976)
(2731, 99.94)
(2732, 99.37)
(2733, 99.526)
(2734, 99.916)
(2735, 99.997)
(2736, 99.967)
(2737, 99.962)
(2738, 99.821)
(2739, 99.994)
(2740, 99.976)
(2741, 99.98)
(2742, 99.962)
(2743, 99.91)
(2744, 99.709)
(2745, 99.75)
(2746, 99.818)
(2747, 99.909)
(2748, 99.933)
(2749, 99.808)
(2750, 99.882)
(2751, 99.903)
(2752, 99.891)
(2753, 99.912)
(2754, 99.967)
(2755, 99.978)
(2756, 99.991)
(2757, 99.997)
(2758, 100)
(2759, 99.997)
(2760, 99.994)
(2761, 99.996)
(2762, 99.999)
(2763, 99.997)
(2764, 100)
(2765, 99.994)
(2766, 99.967)
(2767, 99.824)
(2768, 99.919)
(2769, 99.979)
(2770, 99.88)
(2771, 99.977)
(2772, 100)
(2773, 99.985)
(2774, 99.944)
(2775, 99.35)
(2776, 99.427)
(2777, 99.042)
(2778, 99.963)
(2779, 99.955)
(2780, 99.998)
(2781, 99.989)
(2782, 99.995)
(2783, 99.973)
(2784, 99.967)
(2785, 99.963)
(2786, 99.87)
(2787, 99.301)
(2788, 98.162)
(2789, 96.549)
(2790, 98.405)
(2791, 97.547)
(2792, 98.86)
(2793, 99.686)
(2794, 99.619)
(2795, 99.845)
(2796, 99.82)
(2797, 99.609)
(2798, 99.489)
(2799, 98.741)
(2800, 99.512)
(2801, 99.583)
(2802, 99.882)
(2803, 99.752)
(2804, 96.961)
(2805, 99.575)
(2806, 99.126)
(2807, 99.002)
(2808, 99.478)
(2809, 99.53)
(2810, 99.084)
(2811, 96.939)
(2812, 99.198)
(2813, 99.641)
(2814, 99.749)
(2815, 99.647)
(2816, 99.462)
(2817, 99.114)
(2818, 99.629)
(2819, 99.336)
(2820, 99.616)
(2821, 98.127)
(2822, 97.422)
(2823, 99.12)
(2824, 96.626)
(2825, 97.719)
(2826, 98.505)
(2827, 99.073)
(2828, 96.396)
(2829, 97.233)
(2830, 98.903)
(2831, 97.381)
(2832, 98.128)
(2833, 95.028)
(2834, 95.986)
(2835, 95.664)
(2836, 98.451)
(2837, 98.022)
(2838, 91.667)
(2839, 98.325)
(2840, 96.787)
(2841, 95.441)
(2842, 96.219)
(2843, 96.896)
(2844, 96.803)
(2845, 93.534)
(2846, 94.691)
(2847, 94.246)
(2848, 98.031)
(2849, 97.498)
(2850, 98.457)
(2851, 96.65)
(2852, 99.091)
(2853, 98.862)
(2854, 98.468)
(2855, 98.61)
(2856, 97.916)
(2857, 98.788)
(2858, 98.915)
(2859, 99.056)
(2860, 98.915)
(2861, 98.922)
(2862, 99.363)
(2863, 98.977)
(2864, 99.525)
(2865, 99.482)
(2866, 99.301)
(2867, 97.026)
(2868, 98.94)
(2869, 98.739)
(2870, 98.624)
(2871, 99.431)
(2872, 98.245)
(2873, 99.318)
(2874, 99.39)
(2875, 99.34)
(2876, 98.543)
(2877, 99.7)
(2878, 99.512)
(2879, 99.787)
(2880, 99.656)
(2881, 99.6)
(2882, 99.385)
(2883, 99.341)
(2884, 99.436)
(2885, 99.287)
(2886, 97.954)
(2887, 95.893)
(2888, 96.959)
(2889, 97.603)
(2890, 98.645)
(2891, 98.064)
(2892, 98.767)
(2893, 97.597)
(2894, 97.063)
(2895, 98.233)
(2896, 98.347)
(2897, 99.298)
(2898, 99.476)
(2899, 99.146)
(2900, 99.244)
(2901, 99.733)
(2902, 99.606)
(2903, 99.746)
(2904, 99.683)
(2905, 99.667)
(2906, 99.57)
(2907, 99.376)
(2908, 99.733)
(2909, 99.103)
(2910, 99.041)
(2911, 99.132)
(2912, 99.529)
(2913, 99.501)
(2914, 99.598)
(2915, 99.746)
(2916, 99.162)
(2917, 99.176)
(2918, 99.431)
(2919, 99.522)
(2920, 99.729)
(2921, 99.051)
(2922, 99.856)
(2923, 99.827)
(2924, 99.55)
(2925, 99.535)
(2926, 99.503)
(2927, 99.681)
(2928, 98.952)
(2929, 97.531)
(2930, 99.697)
(2931, 99.691)
(2932, 99.772)
(2933, 98.934)
(2934, 98.081)
(2935, 99.633)
(2936, 99.79)
(2937, 99.81)
(2938, 99.615)
(2939, 98.394)
(2940, 99.914)
(2941, 99.844)
(2942, 99.628)
(2943, 99.739)
(2944, 99.669)
(2945, 99.477)
(2946, 99.647)
(2947, 99.723)
(2948, 99.736)
(2949, 98.932)
(2950, 99.722)
(2951, 99.496)
(2952, 99.272)
(2953, 99.308)
(2954, 99.636)
(2955, 99.8)
(2956, 99.761)
(2957, 99.359)
(2958, 99.42)
(2959, 99.515)
(2960, 99.586)
(2961, 99.704)
(2962, 99.636)
(2963, 99.676)
(2964, 99.812)
(2965, 99.181)
(2966, 99.917)
(2967, 99.973)
(2968, 99.949)
(2969, 99.77)
(2970, 99.955)
(2971, 99.855)
(2972, 99.892)
(2973, 99.954)
(2974, 99.996)
(2975, 99.934)
(2976, 99.801)
(2977, 99.97)
(2978, 99.985)
(2979, 99.991)
(2980, 99.999)
(2981, 99.975)
(2982, 99.94)
(2983, 99.998)
(2984, 100)
(2985, 100)
(2986, 100)
(2987, 99.999)
(2988, 100)
(2989, 100)
(2990, 100)
(2991, 100)
(2992, 100)
(2993, 100)
(2994, 99.876)
(2995, 96.061)
(2996, 99.997)
(2997, 99.985)
(2998, 99.96)
(2999, 99.919)
(3000, 99.965)
(3001, 99.461)
(3002, 99.997)
(3003, 99.999)
(3004, 99.981)
(3005, 99.972)
(3006, 99.894)
(3007, 99.995)
(3008, 99.963)
(3009, 99.978)
(3010, 99.99)
(3011, 99.989)
(3012, 99.874)
(3013, 99.999)
(3014, 99.762)
(3015, 99.328)
(3016, 99.817)
(3017, 99.909)
(3018, 99.659)
(3019, 99.597)
(3020, 99.82)
(3021, 99.963)
(3022, 99.99)
(3023, 99.881)
(3024, 99.998)
(3025, 99.984)
(3026, 99.752)
(3027, 99.837)
(3028, 99.941)
(3029, 99.91)
(3030, 99.962)
(3031, 99.989)
(3032, 99.908)
(3033, 99.899)
(3034, 99.349)
(3035, 99.797)
(3036, 99.93)
(3037, 99.842)
(3038, 99.898)
(3039, 99.79)
(3040, 99.556)
(3041, 99.978)
(3042, 99.91)
(3043, 99.132)
(3044, 99.489)
(3045, 99.324)
(3046, 99.565)
(3047, 99.721)
(3048, 99.6)
(3049, 99.771)
(3050, 98.609)
(3051, 98.451)
(3052, 99.597)
(3053, 99.887)
(3054, 99.825)
(3055, 99.574)
(3056, 99.821)
(3057, 99.565)
(3058, 99.515)
(3059, 99.374)
(3060, 99.154)
(3061, 99.66)
(3062, 99.738)
(3063, 99.751)
(3064, 99.971)
(3065, 99.93)
(3066, 99.973)
(3067, 99.903)
(3068, 99.943)
(3069, 99.881)
(3070, 99.905)
(3071, 99.946)
(3072, 99.975)
(3073, 99.527)
(3074, 98.57)
(3075, 99.854)
(3076, 99.794)
(3077, 99.705)
(3078, 99.196)
(3079, 99.529)
(3080, 99.677)
(3081, 99.425)
(3082, 99.623)
(3083, 99.807)
(3084, 99.936)
(3085, 99.789)
(3086, 99.78)
(3087, 99.762)
(3088, 99.595)
(3089, 99.717)
(3090, 99.236)
(3091, 99.816)
(3092, 99.663)
(3093, 98.353)
(3094, 99.714)
(3095, 99.71)
(3096, 99.854)
(3097, 99.55)
(3098, 99.906)
(3099, 99.938)
(3100, 99.806)
(3101, 96.73)
(3102, 99.858)
(3103, 96.809)
(3104, 99.956)
(3105, 99.686)
(3106, 99.642)
(3107, 99.922)
(3108, 99.808)
(3109, 99.011)
(3110, 99.924)
(3111, 99.904)
(3112, 99.715)
(3113, 99.768)
(3114, 99.915)
(3115, 99.765)
(3116, 99.7)
(3117, 99.569)
(3118, 99.385)
(3119, 99.951)
(3120, 99.843)
(3121, 98.848)
(3122, 99.111)
(3123, 98.754)
(3124, 98.793)
(3125, 98.474)
(3126, 98.699)
(3127, 99.681)
(3128, 99.503)
(3129, 99.262)
(3130, 99.705)
(3131, 99.679)
(3132, 99.353)
(3133, 99.7)
(3134, 99.813)
(3135, 99.816)
(3136, 99.696)
(3137, 99.612)
(3138, 98.919)
(3139, 99.757)
(3140, 99.44)
(3141, 98.546)
(3142, 99.319)
(3143, 98.014)
(3144, 99.787)
(3145, 99.32)
(3146, 98.99)
(3147, 99.869)
(3148, 99.689)
(3149, 99.573)
(3150, 99.57)
(3151, 99.218)
(3152, 99.453)
(3153, 99.588)
(3154, 99.643)
(3155, 99.804)
(3156, 99.707)
(3157, 99.076)
(3158, 99.222)
(3159, 99.392)
(3160, 98.899)
(3161, 99.445)
(3162, 99.287)
(3163, 99.273)
(3164, 99.592)
(3165, 99.549)
(3166, 99.692)
(3167, 99.776)
(3168, 99.779)
(3169, 99.83)
(3170, 99.927)
(3171, 99.922)
(3172, 99.554)
(3173, 98.703)
(3174, 99.241)
(3175, 99.529)
(3176, 99.594)
(3177, 99.703)
(3178, 98.034)
(3179, 99.673)
(3180, 99.156)
(3181, 99.751)
(3182, 99.613)
(3183, 99.908)
(3184, 96.568)
(3185, 97.949)
(3186, 99.977)
(3187, 99.87)
(3188, 99.99)
(3189, 99.967)
(3190, 99.969)
(3191, 99.888)
(3192, 99.699)
(3193, 99.607)
(3194, 99.701)
(3195, 99.023)
(3196, 99.217)
(3197, 95.666)
(3198, 97.906)
(3199, 99.141)
(3200, 99.088)
(3201, 98.707)
(3202, 97.917)
(3203, 99.096)
(3204, 98.689)
(3205, 95.278)
(3206, 97.573)
(3207, 96.378)
(3208, 97.862)
(3209, 97.951)
(3210, 98.728)
(3211, 98.859)
(3212, 98.143)
(3213, 98.436)
(3214, 96.888)
(3215, 97.286)
(3216, 97.201)
(3217, 98.564)
(3218, 96.41)
(3219, 98.805)
(3220, 98.301)
(3221, 98.418)
(3222, 97.174)
(3223, 96.816)
(3224, 98.124)
(3225, 98.382)
(3226, 97.933)
(3227, 97.915)
(3228, 96.846)
(3229, 95.933)
(3230, 95.168)
(3231, 97.45)
(3232, 98.881)
(3233, 98.145)
(3234, 98.801)
(3235, 97.23)
(3236, 98.496)
(3237, 97.238)
(3238, 97.935)
(3239, 98.731)
(3240, 98.05)
(3241, 98.192)
(3242, 98.515)
(3243, 98.14)
(3244, 98.714)
(3245, 98.419)
(3246, 98.958)
(3247, 99.278)
(3248, 99.232)
(3249, 99.466)
(3250, 99.601)
(3251, 98.937)
(3252, 99.474)
(3253, 98.688)
(3254, 98.191)
(3255, 99.096)
(3256, 98.681)
(3257, 98.557)
(3258, 98.488)
(3259, 98.939)
(3260, 99.365)
(3261, 98.748)
(3262, 99.528)
(3263, 99.587)
(3264, 99.5)
(3265, 99.613)
(3266, 99.755)
(3267, 99.467)
(3268, 93.043)
(3269, 96.867)
(3270, 96.792)
(3271, 97.955)
(3272, 98.443)
(3273, 98.531)
(3274, 98.588)
(3275, 97.432)
(3276, 99.386)
(3277, 97.23)
(3278, 98.702)
(3279, 98.85)
(3280, 97.71)
(3281, 98.309)
(3282, 99.642)
(3283, 98.569)
(3284, 99.599)
(3285, 99.823)
(3286, 99.789)
(3287, 99.85)
(3288, 98.019)
(3289, 99.801)
(3290, 97.847)
(3291, 98.705)
(3292, 95.934)
(3293, 97.515)
(3294, 98.279)
(3295, 99.166)
(3296, 99.486)
(3297, 99.588)
(3298, 99.288)
(3299, 99.113)
(3300, 98.995)
(3301, 98.217)
(3302, 99.239)
(3303, 99.688)
(3304, 98.365)
(3305, 99.705)
(3306, 99.894)
(3307, 99.4)
(3308, 98.85)
(3309, 99.745)
(3310, 99.767)
(3311, 99.911)
(3312, 99.309)
(3313, 99.647)
(3314, 99.232)
(3315, 99.704)
(3316, 99.521)
(3317, 99.734)
(3318, 99.696)
(3319, 99.958)
(3320, 99.724)
(3321, 99.168)
(3322, 99.454)
(3323, 99.336)
(3324, 99.392)
(3325, 99.747)
(3326, 99.779)
(3327, 98.269)
(3328, 99.498)
(3329, 98.5)
(3330, 99.166)
(3331, 99.197)
(3332, 99.057)
(3333, 99.021)
(3334, 99.382)
(3335, 99.237)
(3336, 98.849)
(3337, 99.01)
(3338, 99.05)
(3339, 99.616)
(3340, 99.585)
(3341, 99.956)
(3342, 99.647)
(3343, 99.744)
(3344, 99.917)
(3345, 99.892)
(3346, 99.979)
(3347, 99.854)
(3348, 99.929)
(3349, 99.283)
(3350, 99.487)
(3351, 99.371)
(3352, 99.356)
(3353, 98.23)
(3354, 98.996)
(3355, 98.394)
(3356, 97.027)
(3357, 99.154)
(3358, 99.383)
(3359, 99.933)
(3360, 99.897)
(3361, 99.896)
(3362, 99.873)
(3363, 99.597)
(3364, 98.653)
(3365, 99.931)
(3366, 99.855)
(3367, 98.124)
(3368, 97.248)
(3369, 99.237)
(3370, 99.315)
(3371, 99.245)
(3372, 99.76)
(3373, 99.612)
(3374, 99.556)
(3375, 99.856)
(3376, 99.867)
(3377, 99.751)
(3378, 99.795)
(3379, 99.696)
(3380, 99.667)
(3381, 99.851)
(3382, 99.933)
(3383, 99.912)
(3384, 99.525)
(3385, 99.597)
(3386, 99.244)
(3387, 99.724)
(3388, 99.13)
(3389, 98.769)
(3390, 97.652)
(3391, 98.918)
(3392, 99.814)
(3393, 99.365)
(3394, 99.698)
(3395, 99.621)
(3396, 99.038)
(3397, 98.701)
(3398, 98.433)
(3399, 99.631)
(3400, 99.555)
(3401, 99.148)
(3402, 99.682)
(3403, 99.546)
(3404, 99.218)
(3405, 99.249)
(3406, 99.57)
(3407, 99.647)
(3408, 99.943)
(3409, 99.982)
(3410, 99.976)
(3411, 99.992)
(3412, 99.888)
(3413, 99.899)
(3414, 99.998)
(3415, 99.99)
(3416, 99.996)
(3417, 99.951)
(3418, 100)
(3419, 99.959)
(3420, 100)
(3421, 99.977)
(3422, 94.743)
(3423, 99.978)
(3424, 99.979)
(3425, 99.973)
(3426, 99.781)
(3427, 99.998)
(3428, 99.995)
(3429, 99.992)
(3430, 99.903)
(3431, 99.969)
(3432, 99.98)
(3433, 99.98)
(3434, 99.994)
(3435, 99.992)
(3436, 100)
(3437, 99.49)
(3438, 99.99)
(3439, 99.992)
(3440, 99.997)
(3441, 99.982)
(3442, 99.939)
(3443, 99.969)
(3444, 99.89)
(3445, 99.953)
(3446, 99.969)
(3447, 99.903)
(3448, 99.935)
(3449, 99.899)
(3450, 99.86)
(3451, 99.826)
(3452, 99.867)
(3453, 99.604)
(3454, 99.796)
(3455, 99.697)
(3456, 99.747)
(3457, 99.717)
(3458, 99.821)
(3459, 99.722)
(3460, 99.827)
(3461, 99.84)
(3462, 99.876)
(3463, 99.895)
(3464, 99.806)
(3465, 99.837)
(3466, 99.436)
(3467, 99.64)
(3468, 98.486)
(3469, 99.545)
(3470, 99.683)
(3471, 99.622)
(3472, 99.735)
(3473, 99.622)
(3474, 99.601)
(3475, 98.757)
(3476, 99.203)
(3477, 97.867)
(3478, 96.302)
(3479, 97.447)
(3480, 98.308)
(3481, 96.629)
(3482, 98.728)
(3483, 99.336)
(3484, 99.224)
(3485, 98.296)
(3486, 98.274)
(3487, 98.138)
(3488, 98.578)
(3489, 95.775)
(3490, 98.454)
(3491, 98.341)
(3492, 97.558)
(3493, 96.649)
(3494, 97.815)
(3495, 96.623)
(3496, 97.579)
(3497, 98.938)
(3498, 97.612)
(3499, 97.492)
(3500, 97.799)
(3501, 98.175)
(3502, 98.462)
(3503, 96.395)
(3504, 97.892)
(3505, 98.413)
(3506, 97.854)
(3507, 97.921)
(3508, 98.222)
(3509, 97.331)
(3510, 98.156)
(3511, 97.121)
(3512, 97.31)
(3513, 97.569)
(3514, 93.275)
(3515, 95.881)
(3516, 96.004)
(3517, 96.43)
(3518, 93.324)
(3519, 91.606)
(3520, 86.529)
(3521, 83.404)
(3522, 87.313)
(3523, 92.077)
(3524, 95.327)
(3525, 93.019)
(3526, 91.946)
(3527, 92.896)
(3528, 93.929)
(3529, 92.779)
(3530, 95.251)
(3531, 92.693)
(3532, 83.797)
(3533, 88.769)
(3534, 90.556)
(3535, 91.292)
(3536, 86.954)
(3537, 92.744)
(3538, 95.806)
(3539, 92.147)
(3540, 92.637)
(3541, 97.072)
(3542, 92.176)
(3543, 91.215)
(3544, 94.836)
(3545, 93.233)
(3546, 91.86)
(3547, 88.4)
(3548, 91.922)
(3549, 86.694)
(3550, 93.578)
(3551, 95.389)
(3552, 90.487)
(3553, 94.946)
(3554, 84.438)
(3555, 92.359)
(3556, 92.089)
(3557, 87.429)
(3558, 88.684)
(3559, 91.218)
(3560, 92.883)
(3561, 93.359)
(3562, 96.036)
(3563, 94.399)
(3564, 91.246)
(3565, 87)
(3566, 89.123)
(3567, 93.304)
(3568, 91.864)
(3569, 89.838)
(3570, 95.05)
(3571, 93.186)
(3572, 95.235)
(3573, 96.091)
(3574, 95.834)
(3575, 97.142)
(3576, 96.845)
(3577, 97.72)
(3578, 97.924)
(3579, 98.262)
(3580, 99.464)
(3581, 98.869)
(3582, 99.338)
(3583, 97.841)
(3584, 96.575)
(3585, 96.606)
(3586, 94.47)
(3587, 97.118)
(3588, 95.501)
(3589, 97.044)
(3590, 99.031)
(3591, 97.454)
(3592, 95.516)
(3593, 95.663)
(3594, 96.356)
(3595, 97.808)
(3596, 96.493)
(3597, 97.126)
(3598, 97.916)
(3599, 96.844)
(3600, 95.425)
(3601, 91.92)
(3602, 95.875)
(3603, 97.497)
(3604, 95.682)
(3605, 87.827)
(3606, 95.678)
(3607, 97.486)
(3608, 96.373)
(3609, 96.726)
(3610, 98.393)
(3611, 97.373)
(3612, 98.322)
(3613, 93.063)
(3614, 92.135)
(3615, 92.78)
(3616, 94.855)
(3617, 84.096)
(3618, 92.613)
(3619, 87.086)
(3620, 80.11)
(3621, 99.594)
(3622, 99.519)
(3623, 94.826)
(3624, 98.814)
(3625, 97.352)
(3626, 97.106)
(3627, 97.351)
(3628, 97.963)
(3629, 99.89)
(3630, 99.886)
(3631, 99.856)
(3632, 99.815)
(3633, 99.497)
(3634, 98.627)
(3635, 99.186)
(3636, 98.468)
(3637, 98.866)
(3638, 99.37)
(3639, 99.16)
(3640, 97.783)
(3641, 97.93)
(3642, 98.66)
(3643, 98.981)
(3644, 97.157)
(3645, 99.144)
(3646, 99.663)
(3647, 98.946)
(3648, 99.815)
(3649, 99.95)
(3650, 98.479)
(3651, 99.733)
(3652, 99.796)
(3653, 99.036)
(3654, 99.676)
(3655, 99.702)
(3656, 99.916)
(3657, 98.323)
(3658, 99.089)
(3659, 99.046)
(3660, 98.88)
(3661, 99.571)
(3662, 99.864)
(3663, 99.854)
(3664, 97.759)
(3665, 99.116)
(3666, 99.462)
(3667, 99.494)
(3668, 98.583)
(3669, 99.31)
(3670, 99.626)
(3671, 98.056)
(3672, 98.747)
(3673, 98.09)
(3674, 98.744)
(3675, 98.272)
(3676, 97.896)
(3677, 97.237)
(3678, 97.645)
(3679, 95.829)
(3680, 96.276)
(3681, 98.635)
(3682, 98.597)
(3683, 96.571)
(3684, 95.114)
(3685, 93.557)
(3686, 96.603)
(3687, 96.671)
(3688, 95.551)
(3689, 96.923)
(3690, 96.285)
(3691, 95.978)
(3692, 96.006)
(3693, 93.706)
(3694, 97.958)
(3695, 95.717)
(3696, 94.866)
(3697, 93.982)
(3698, 97.052)
(3699, 93.526)
(3700, 91.299)
(3701, 93.088)
(3702, 87.905)
(3703, 93.827)
(3704, 94.917)
(3705, 96.417)
(3706, 92.454)
(3707, 95.371)
(3708, 95.49)
(3709, 96.265)
(3710, 96.087)
(3711, 96.523)
(3712, 93.092)
(3713, 94.319)
(3714, 93.301)
(3715, 94.818)
(3716, 96.16)
(3717, 97.447)
(3718, 97.01)
(3719, 97.892)
(3720, 96.034)
(3721, 93.083)
(3722, 92.888)
(3723, 96.558)
(3724, 96.916)
(3725, 97.858)
(3726, 92.035)
(3727, 92.431)
(3728, 94.469)
(3729, 94.084)
(3730, 95.578)
(3731, 93.065)
(3732, 92.066)
(3733, 94.642)
(3734, 96.697)
(3735, 95.55)
(3736, 94.713)
(3737, 94.441)
(3738, 96.851)
(3739, 93.372)
(3740, 96.523)
(3741, 94.768)
(3742, 96.759)
(3743, 89.868)
(3744, 97.08)
(3745, 91.775)
(3746, 90.381)
(3747, 90.743)
(3748, 95.212)
(3749, 97.051)
(3750, 98.017)
(3751, 96.221)
(3752, 98.552)
(3753, 94.922)
(3754, 96.103)
(3755, 92.872)
(3756, 91.003)
(3757, 93.105)
(3758, 90.474)
(3759, 96.085)
(3760, 86.191)
(3761, 89.688)
(3762, 87.498)
(3763, 81.122)
(3764, 94.659)
(3765, 92.419)
(3766, 99.901)
(3767, 99.96)
(3768, 99.691)
(3769, 99.499)
(3770, 98.32)
(3771, 99.582)
(3772, 99.47)
(3773, 99.583)
(3774, 99.748)
(3775, 99.625)
(3776, 99.083)
(3777, 99.456)
(3778, 99.429)
(3779, 99.414)
(3780, 99.394)
(3781, 99.401)
(3782, 99.793)
(3783, 99.613)
(3784, 99.763)
(3785, 98.926)
(3786, 99.747)
(3787, 99.906)
(3788, 99.802)
(3789, 99.528)
(3790, 99.899)
(3791, 99.981)
(3792, 99.785)
(3793, 99.342)
(3794, 99.837)
(3795, 99.999)
(3796, 99.999)
(3797, 100)
(3798, 99.999)
(3799, 99.998)
(3800, 99.996)
(3801, 99.987)
(3802, 99.984)
(3803, 99.966)
(3804, 99.517)
(3805, 99.922)
(3806, 99.766)
(3807, 99.133)
(3808, 99.667)
(3809, 99.839)
(3810, 98.353)
(3811, 97.384)
(3812, 99.521)
(3813, 99.477)
(3814, 99.206)
(3815, 99.63)
(3816, 99.248)
(3817, 99.566)
(3818, 97.195)
(3819, 99.367)
(3820, 98.859)
(3821, 98.228)
(3822, 97.878)
(3823, 97.911)
(3824, 97.63)
(3825, 98.26)
(3826, 99.099)
(3827, 97.972)
(3828, 97.539)
(3829, 97.128)
(3830, 98.526)
(3831, 99.289)
(3832, 99.466)
(3833, 99.534)
(3834, 99.248)
(3835, 99.404)
(3836, 99.483)
(3837, 99.443)
(3838, 99.275)
(3839, 98.657)
(3840, 98.831)
(3841, 99.232)
(3842, 97.93)
(3843, 96.424)
(3844, 98.142)
(3845, 97.612)
(3846, 97.298)
(3847, 96.315)
(3848, 96.241)
(3849, 96.286)
(3850, 95.651)
(3851, 98.391)
(3852, 93.229)
(3853, 94.932)
(3854, 97.704)
(3855, 98.017)
(3856, 96.056)
(3857, 97.111)
(3858, 98.566)
(3859, 97.348)
(3860, 96.127)
(3861, 98.315)
(3862, 96.593)
(3863, 97.455)
(3864, 98.804)
(3865, 98.249)
(3866, 97.363)
(3867, 97.376)
(3868, 98.023)
(3869, 97.754)
(3870, 94.851)
(3871, 95.195)
(3872, 97.323)
(3873, 99.019)
(3874, 97.271)
(3875, 94.661)
(3876, 93.568)
(3877, 97.131)
(3878, 97.324)
(3879, 96.055)
(3880, 96.404)
(3881, 94.998)
(3882, 97.305)
(3883, 95.838)
(3884, 96.964)
(3885, 96.021)
(3886, 94.088)
(3887, 97.488)
(3888, 98.813)
(3889, 95.924)
(3890, 97.043)
(3891, 96.809)
(3892, 96.008)
(3893, 96.527)
(3894, 97.781)
(3895, 98.109)
(3896, 98.643)
(3897, 97.604)
(3898, 98.53)
(3899, 98.427)
(3900, 97.966)
(3901, 95.553)
(3902, 94.163)
(3903, 96.471)
(3904, 96.033)
(3905, 92.908)
(3906, 87.962)
(3907, 77.375)
(3908, 87.366)
(3909, 91.001)
(3910, 90.319)
(3911, 89.721)
(3912, 85.919)
(3913, 88.979)
(3914, 87.38)
(3915, 70.651)
(3916, 77.411)
(3917, 86.264)
(3918, 80.502)
(3919, 68.829)
(3920, 81.898)
(3921, 75.48)
(3922, 59.802)
(3923, 43.861)
(3924, 58.796)
(3925, 53.41)
(3926, 35.075)
(3927, 59.888)
(3928, 56.057)
(3929, 33.463)
(3930, 28.878)
(3931, 30.272)
(3932, 44.186)
(3933, 18.666)
(3934, 34.133)
(3935, 36.881)
(3936, 28.362)
(3937, 46.57)
(3938, 36.22)
(3939, 63.127)
(3940, 95.153)
(3941, 91.337)
(3942, 93.373)
(3943, 96.396)
(3944, 96.918)
(3945, 87.754)
(3946, 85.416)
(3947, 83.729)
(3948, 78.124)
(3949, 74.168)
(3950, 76.611)
(3951, 60.365)
(3952, 59.719)
(3953, 56.19)
(3954, 68.603)
(3955, 62.384)
(3956, 75.962)
(3957, 84.548)
(3958, 83.026)
(3959, 82.114)
(3960, 86.838)
(3961, 91.173)
(3962, 90.825)
(3963, 86.677)
(3964, 90.341)
(3965, 92.004)
(3966, 90.38)
(3967, 87.735)
(3968, 86.561)
(3969, 92.028)
(3970, 86.876)
(3971, 89.315)
(3972, 91.16)
(3973, 88.723)
(3974, 92.439)
(3975, 95.398)
(3976, 96.428)
(3977, 95.99)
(3978, 95.543)
(3979, 93.465)
(3980, 96.577)
(3981, 95.231)
(3982, 94.015)
(3983, 93.999)
(3984, 96.132)
(3985, 94.964)
(3986, 96.73)
(3987, 95.794)
(3988, 95.208)
(3989, 97.091)
(3990, 96.301)
(3991, 94.152)
(3992, 96.278)
(3993, 94.192)
(3994, 95.314)
(3995, 94.418)
(3996, 88.607)
(3997, 91.777)
(3998, 98.172)
(3999, 96.632)
(4000, 98.187)
(4001, 96.422)
(4002, 96.333)
(4003, 97.364)
(4004, 92.801)
(4005, 97.141)
(4006, 97.077)
(4007, 97.097)
(4008, 97.611)
(4009, 95.959)
(4010, 94.395)
(4011, 96.736)
(4012, 96.645)
(4013, 96.926)
(4014, 97.678)
(4015, 98.115)
(4016, 97.823)
(4017, 97.83)
(4018, 97.313)
(4019, 99.132)
(4020, 98.493)
(4021, 97.033)
(4022, 98.765)
(4023, 98.225)
(4024, 99.338)
(4025, 98.202)
(4026, 95.579)
(4027, 98.018)
(4028, 97.617)
(4029, 98.37)
(4030, 96.803)
(4031, 98.325)
(4032, 98.605)
(4033, 88.975)
(4034, 99.252)
(4035, 91.522)
(4036, 99.528)
(4037, 99.846)
(4038, 99.695)
(4039, 99.977)
(4040, 98.12)
(4041, 99.907)
(4042, 99.994)
(4043, 99.988)
(4044, 99.998)
(4045, 99.633)
(4046, 99.949)
(4047, 99.873)
(4048, 99.932)
(4049, 98.885)
(4050, 99.864)
(4051, 99.745)
(4052, 98.755)
(4053, 99.414)
(4054, 99.811)
(4055, 99.898)
(4056, 99.596)
(4057, 99.703)
(4058, 99.705)
(4059, 99.956)
(4060, 99.956)
(4061, 99.846)
(4062, 99.881)
(4063, 99.744)
(4064, 99.457)
(4065, 98.974)
(4066, 99.669)
(4067, 99.859)
(4068, 99.093)
(4069, 99.174)
(4070, 97.745)
(4071, 98.686)
(4072, 98.921)
(4073, 99.555)
(4074, 99.631)
(4075, 99.255)
(4076, 99.386)
(4077, 99.686)
(4078, 99.243)
(4079, 98.615)
(4080, 97.742)
(4081, 96.849)
(4082, 98.56)
(4083, 98.079)
(4084, 97.854)
(4085, 99.373)
(4086, 98.507)
(4087, 98.515)
(4088, 98.131)
(4089, 92.75)
(4090, 98.859)
(4091, 98.491)
(4092, 87.555)
(4093, 98.518)
(4094, 98.155)
(4095, 99.193)
(4096, 98.634)
(4097, 98.537)
(4098, 98.842)
(4099, 98.471)
(4100, 98.517)
(4101, 97.592)
(4102, 98.3)
(4103, 99.088)
(4104, 98.502)
(4105, 98.531)
(4106, 98.803)
(4107, 98.82)
(4108, 98.392)
(4109, 97.86)
(4110, 99.225)
(4111, 99.163)
(4112, 98.132)
(4113, 95.166)
(4114, 98.096)
(4115, 98.612)
(4116, 98.716)
(4117, 97.79)
(4118, 97.812)
(4119, 96.66)
(4120, 93.434)
(4121, 96.061)
(4122, 96.417)
(4123, 89.91)
(4124, 93.786)
(4125, 95.814)
(4126, 95.45)
(4127, 94.877)
(4128, 90.747)
(4129, 90.333)
(4130, 96.169)
(4131, 95.831)
(4132, 93.675)
(4133, 94.77)
(4134, 95.38)
(4135, 96.695)
(4136, 93.587)
(4137, 93.293)
(4138, 86.894)
(4139, 89.588)
(4140, 90.921)
(4141, 89.357)
(4142, 92.691)
(4143, 91.635)
(4144, 93.373)
(4145, 94.143)
(4146, 94.55)
(4147, 94.154)
(4148, 94.67)
(4149, 90.958)
(4150, 94.513)
(4151, 93.157)
(4152, 95)
(4153, 93.783)
(4154, 94.1)
(4155, 92.922)
(4156, 96.166)
(4157, 93.608)
(4158, 97.306)
(4159, 96.456)
(4160, 97.032)
(4161, 95.804)
(4162, 97.705)
(4163, 97.494)
(4164, 93.64)
(4165, 99.458)
(4166, 95.753)
(4167, 99.271)
(4168, 99.813)
(4169, 92.677)
(4170, 99.636)
(4171, 99.45)
(4172, 99.75)
(4173, 99.021)
(4174, 88.829)
(4175, 98.242)
(4176, 99.021)
(4177, 98.944)
(4178, 99.452)
(4179, 99.59)
(4180, 98.981)
(4181, 99.268)
(4182, 98.833)
(4183, 99.36)
(4184, 99.174)
(4185, 99.48)
(4186, 99.282)
(4187, 98.901)
(4188, 99.466)
(4189, 97.347)
(4190, 94.581)
(4191, 94.968)
(4192, 95.922)
(4193, 97.272)
(4194, 98.794)
(4195, 97.307)
(4196, 97.304)
(4197, 97.903)
(4198, 99.158)
(4199, 98.849)
(4200, 98.499)
(4201, 98.018)
(4202, 96.367)
(4203, 95.444)
(4204, 95.954)
(4205, 98.316)
(4206, 98.994)
(4207, 97.868)
(4208, 93.968)
(4209, 99.566)
(4210, 99.68)
(4211, 99.834)
(4212, 99.722)
(4213, 99.643)
(4214, 98.989)
(4215, 97.931)
(4216, 98.883)
(4217, 97.674)
(4218, 98.3)
(4219, 97.738)
(4220, 98.77)
(4221, 97.515)
(4222, 92.277)
(4223, 96.27)
(4224, 93.983)
(4225, 97.645)
(4226, 95.622)
(4227, 96.884)
(4228, 97.177)
(4229, 97.335)
(4230, 95.118)
(4231, 95.626)
(4232, 95.983)
(4233, 95.03)
(4234, 87.195)
(4235, 86.219)
(4236, 92.197)
(4237, 94.161)
(4238, 94.599)
(4239, 95.54)
(4240, 93.134)
(4241, 90.796)
(4242, 94.129)
(4243, 95.578)
(4244, 95.165)
(4245, 89.444)
(4246, 94.245)
(4247, 92.812)
(4248, 92.559)
(4249, 97.773)
(4250, 95.193)
(4251, 95.208)
(4252, 95.352)
(4253, 93.083)
(4254, 94.954)
(4255, 94.695)
(4256, 88.437)
(4257, 96.688)
(4258, 98.252)
(4259, 97.992)
(4260, 95.954)
(4261, 96.865)
(4262, 95.29)
(4263, 95.963)
(4264, 93.606)
(4265, 95.439)
(4266, 97.883)
(4267, 97.259)
(4268, 96.159)
(4269, 93.205)
(4270, 92.019)
(4271, 91.621)
(4272, 91.205)
(4273, 97.376)
(4274, 97.076)
(4275, 94.812)
(4276, 96.12)
(4277, 94.226)
(4278, 87.946)
(4279, 93.605)
(4280, 97.656)
(4281, 91.393)
(4282, 91.59)
(4283, 90.786)
(4284, 82.001)
(4285, 94.327)
(4286, 91.828)
(4287, 87.981)
(4288, 86.563)
(4289, 79.993)
(4290, 82.19)
(4291, 91.729)
(4292, 92.559)
(4293, 92.733)
(4294, 86.233)
(4295, 92.3)
(4296, 90.896)
(4297, 84.658)
(4298, 88.765)
(4299, 89.401)
(4300, 90.632)
(4301, 80.726)
(4302, 93.3)
(4303, 87.09)
(4304, 91.148)
(4305, 92.625)
(4306, 93.077)
(4307, 91.253)
(4308, 95.28)
(4309, 93.464)
(4310, 94.637)
(4311, 93.214)
(4312, 85.993)
(4313, 81.599)
(4314, 72.324)
(4315, 82.223)
(4316, 71.193)
(4317, 79.621)
(4318, 69.901)
(4319, 71.188)
(4320, 84.319)
(4321, 86.848)
(4322, 90.322)
(4323, 93.626)
(4324, 94.466)
(4325, 96.698)
(4326, 96.711)
(4327, 96.859)
(4328, 98.034)
(4329, 97.049)
(4330, 96.9)
(4331, 96.673)
(4332, 96.009)
(4333, 97.854)
(4334, 91.982)
(4335, 98.281)
(4336, 97.478)
(4337, 94.877)
(4338, 96.77)
(4339, 97.99)
(4340, 96.842)
(4341, 98.038)
(4342, 99.038)
(4343, 96.993)
(4344, 96.955)
(4345, 97.779)
(4346, 98.984)
(4347, 98.848)
(4348, 98.731)
(4349, 98.589)
(4350, 99.732)
(4351, 99.4)
(4352, 99.224)
(4353, 98.203)
(4354, 98.029)
(4355, 98.725)
(4356, 99.091)
(4357, 98.649)
(4358, 99.322)
(4359, 98.146)
(4360, 98.105)
(4361, 97.508)
(4362, 95.389)
(4363, 97.044)
(4364, 98.035)
(4365, 97.874)
(4366, 98.344)
(4367, 96.467)
(4368, 93.788)
(4369, 97.248)
(4370, 95.459)
(4371, 98.207)
(4372, 98.095)
(4373, 97.159)
(4374, 97.802)
(4375, 93.933)
(4376, 91.589)
(4377, 94.377)
(4378, 93.795)
(4379, 89.082)
(4380, 93.936)
(4381, 95.541)
(4382, 95.036)
(4383, 94.078)
(4384, 91.071)
(4385, 88.758)
(4386, 86.852)
(4387, 90.337)
(4388, 88.254)
(4389, 92.118)
(4390, 93.537)
(4391, 89.593)
(4392, 77.146)
(4393, 82.651)
(4394, 83.568)
(4395, 89.677)
(4396, 87.865)
(4397, 88.498)
(4398, 93.301)
(4399, 91.936)
(4400, 92.91)
(4401, 95.409)
(4402, 97.09)
(4403, 94.998)
(4404, 96.352)
(4405, 94.843)
(4406, 95.66)
(4407, 96.094)
(4408, 99.163)
(4409, 94.772)
(4410, 98.323)
(4411, 98.104)
(4412, 97.656)
(4413, 98.906)
(4414, 99.479)
(4415, 98.047)
(4416, 98.601)
(4417, 97.996)
(4418, 98.594)
(4419, 97.172)
(4420, 96.097)
(4421, 96.403)
(4422, 99.06)
(4423, 97.968)
(4424, 99.186)
(4425, 99.739)
(4426, 96.983)
(4427, 98.929)
(4428, 98.347)
(4429, 98.711)
(4430, 98.223)
(4431, 97.671)
(4432, 96.67)
(4433, 98.209)
(4434, 98.517)
(4435, 95.793)
(4436, 99.284)
(4437, 98.528)
(4438, 97.785)
(4439, 95.849)
(4440, 98.488)
(4441, 97.653)
(4442, 97.317)
(4443, 96.238)
(4444, 96.103)
(4445, 98.928)
(4446, 98.953)
(4447, 98.665)
(4448, 98.552)
(4449, 98.679)
(4450, 92.777)
(4451, 97.61)
(4452, 98.111)
(4453, 98.355)
(4454, 96.804)
(4455, 98.298)
(4456, 96.591)
(4457, 98.86)
(4458, 98.108)
(4459, 95.657)
(4460, 97.239)
(4461, 97.208)
(4462, 96.011)
(4463, 96.525)
(4464, 97.383)
(4465, 97.483)
(4466, 96.929)
(4467, 97.264)
(4468, 97.017)
(4469, 97.804)
(4470, 97.654)
(4471, 96.491)
(4472, 96.679)
(4473, 98.905)
(4474, 99.447)
(4475, 98.704)
(4476, 98.867)
(4477, 98.518)
(4478, 99.185)
(4479, 95.216)
(4480, 96.646)
(4481, 96.152)
(4482, 93.958)
(4483, 96.388)
(4484, 96.009)
(4485, 95.388)
(4486, 94.099)
(4487, 95.082)
(4488, 96.682)
(4489, 93.913)
(4490, 92.338)
(4491, 94.731)
(4492, 95.878)
(4493, 89.305)
(4494, 94.087)
(4495, 95.918)
(4496, 97.313)
(4497, 94.788)
(4498, 96.951)
(4499, 94.167)
(4500, 93.739)
(4501, 95.434)
(4502, 98.028)
(4503, 98.331)
(4504, 97.542)
(4505, 84.78)
(4506, 98.123)
(4507, 93.417)
(4508, 94.335)
(4509, 90.422)
(4510, 79.344)
(4511, 86.344)
(4512, 86.859)
(4513, 80.382)
(4514, 84.916)
(4515, 84.618)
(4516, 92.051)
(4517, 95.643)
(4518, 94.899)
(4519, 91.808)
(4520, 93.646)
(4521, 86.744)
(4522, 91.524)
(4523, 94.429)
(4524, 91.012)
(4525, 85.879)
(4526, 89.333)
(4527, 90.134)
(4528, 90.157)
(4529, 86.849)
(4530, 79.829)
(4531, 84.395)
(4532, 93.534)
(4533, 94.563)
(4534, 93.826)
(4535, 92.35)
(4536, 93.374)
(4537, 90.764)
(4538, 92.024)
(4539, 90.226)
(4540, 85.016)
(4541, 78.56)
(4542, 84.632)
(4543, 88.836)
(4544, 89.044)
(4545, 87.93)
(4546, 91.928)
(4547, 93.682)
(4548, 90.171)
(4549, 94.416)
(4550, 92.516)
(4551, 90.821)
(4552, 90.019)
(4553, 91.498)
(4554, 97.356)
(4555, 95.534)
(4556, 89.901)
(4557, 88.362)
(4558, 95.663)
(4559, 95.725)
(4560, 96.654)
(4561, 97.358)
(4562, 94.764)
(4563, 94.449)
(4564, 93.02)
(4565, 92.722)
(4566, 95.287)
(4567, 95.36)
(4568, 95.506)
(4569, 87.95)
(4570, 98.395)
(4571, 98.501)
(4572, 98.209)
(4573, 98.11)
(4574, 98.388)
(4575, 99.206)
(4576, 99.062)
(4577, 96.378)
(4578, 98.654)
(4579, 97.744)
(4580, 94.062)
(4581, 95.463)
(4582, 95.423)
(4583, 95.825)
(4584, 97.295)
(4585, 96.226)
(4586, 94.696)
(4587, 94.403)
(4588, 92.834)
(4589, 97.387)
(4590, 93.906)
(4591, 94.97)
(4592, 97.03)
(4593, 97.926)
(4594, 94.287)
(4595, 97.645)
(4596, 97.796)
(4597, 98.132)
(4598, 97.792)
(4599, 95.777)
(4600, 96.384)
(4601, 99.059)
(4602, 98.35)
(4603, 97.995)
(4604, 92.267)
(4605, 94.421)
(4606, 95.021)
(4607, 96.316)
(4608, 96.784)
(4609, 97.095)
(4610, 96.45)
(4611, 94.133)
(4612, 90.502)
(4613, 93.03)
(4614, 96.781)
(4615, 96.856)
(4616, 93.947)
(4617, 95.602)
(4618, 95.551)
(4619, 97.081)
(4620, 96.373)
(4621, 94.191)
(4622, 93.991)
(4623, 91.615)
(4624, 93.702)
(4625, 95.779)
(4626, 97.874)
(4627, 96.83)
(4628, 95.455)
(4629, 94.944)
(4630, 97.29)
(4631, 94.193)
(4632, 96.216)
(4633, 96.768)
(4634, 95.086)
(4635, 96.096)
(4636, 96.478)
(4637, 97.362)
(4638, 98.851)
(4639, 89.9688888888889)
(4640, 0)
};



==> covgraphs/graph.2.500.tex <==
\addplot[const plot,fill=lightblue,draw=lightblue] coordinates {
(-1, 0)
(0, 94.448)
(1, 92.87)
(2, 96.49)
(3, 97.57)
(4, 97.922)
(5, 96.8)
(6, 94.216)
(7, 95.236)
(8, 94.788)
(9, 96.956)
(10, 96.668)
(11, 98.6)
(12, 97.412)
(13, 96.594)
(14, 96.106)
(15, 95.456)
(16, 97.806)
(17, 97.502)
(18, 97.102)
(19, 97.284)
(20, 98.348)
(21, 95.196)
(22, 97.098)
(23, 96.776)
(24, 97.084)
(25, 96.32)
(26, 97.902)
(27, 97.498)
(28, 96.976)
(29, 95.652)
(30, 97.846)
(31, 99.454)
(32, 99.974)
(33, 95.576)
(34, 97.992)
(35, 97.238)
(36, 97.758)
(37, 97.62)
(38, 98.334)
(39, 98.22)
(40, 98.674)
(41, 98.452)
(42, 98.338)
(43, 97.84)
(44, 98.194)
(45, 97.038)
(46, 96.184)
(47, 96.682)
(48, 96.862)
(49, 97.12)
(50, 96.088)
(51, 94.78)
(52, 96.404)
(53, 97.22)
(54, 96.796)
(55, 94.168)
(56, 95.194)
(57, 98.098)
(58, 98.412)
(59, 98.112)
(60, 95.888)
(61, 97.522)
(62, 95.416)
(63, 96.708)
(64, 95.778)
(65, 93.444)
(66, 94.952)
(67, 97.128)
(68, 99.428)
(69, 97.544)
(70, 95.828)
(71, 91.778)
(72, 98.65)
(73, 94.754)
(74, 95.446)
(75, 96.614)
(76, 96.568)
(77, 91.942)
(78, 94.728)
(79, 95.902)
(80, 93.23)
(81, 94.978)
(82, 96.304)
(83, 96.156)
(84, 97.684)
(85, 92.544)
(86, 94.308)
(87, 91.208)
(88, 93.164)
(89, 93.864)
(90, 94.734)
(91, 93.838)
(92, 93.644)
(93, 95.184)
(94, 93.676)
(95, 84.642)
(96, 91.642)
(97, 94.128)
(98, 96.072)
(99, 94.854)
(100, 94.51)
(101, 89.546)
(102, 96.264)
(103, 96.922)
(104, 93.392)
(105, 95.186)
(106, 95.424)
(107, 93.554)
(108, 92.77)
(109, 94.712)
(110, 94.716)
(111, 97.46)
(112, 96.354)
(113, 94.856)
(114, 94.904)
(115, 94.612)
(116, 98.204)
(117, 98.63)
(118, 96.462)
(119, 96.962)
(120, 93.786)
(121, 94.634)
(122, 95.77)
(123, 86.164)
(124, 89.808)
(125, 90.044)
(126, 93.454)
(127, 88.866)
(128, 89.808)
(129, 89.43)
(130, 91.038)
(131, 90.85)
(132, 86.39)
(133, 84.538)
(134, 91.968)
(135, 81.84)
(136, 91.214)
(137, 87.29)
(138, 86.254)
(139, 92.842)
(140, 95.478)
(141, 92.352)
(142, 92.488)
(143, 82.11)
(144, 91.912)
(145, 92.902)
(146, 83.122)
(147, 71.264)
(148, 82.206)
(149, 88.678)
(150, 85.648)
(151, 92.83)
(152, 94.522)
(153, 93.898)
(154, 93.848)
(155, 94.762)
(156, 94.858)
(157, 95.058)
(158, 87.334)
(159, 86.37)
(160, 88.978)
(161, 87.78)
(162, 88.198)
(163, 72.998)
(164, 84.722)
(165, 87.002)
(166, 89.1)
(167, 95.528)
(168, 96.864)
(169, 95.728)
(170, 93.93)
(171, 90.244)
(172, 79.808)
(173, 89.49)
(174, 91.428)
(175, 95.218)
(176, 92.182)
(177, 89.84)
(178, 95.518)
(179, 94.51)
(180, 86.224)
(181, 79.836)
(182, 87.76)
(183, 91.218)
(184, 93.118)
(185, 80.514)
(186, 61.796)
(187, 85.204)
(188, 83.386)
(189, 82.84)
(190, 88.412)
(191, 90.588)
(192, 90.188)
(193, 93.91)
(194, 88.208)
(195, 93.236)
(196, 85.726)
(197, 93.554)
(198, 91.122)
(199, 93.018)
(200, 86.268)
(201, 94.226)
(202, 89.542)
(203, 89.458)
(204, 94.07)
(205, 97.826)
(206, 93.51)
(207, 96.696)
(208, 97.386)
(209, 95.12)
(210, 97.278)
(211, 97.554)
(212, 97.034)
(213, 97.898)
(214, 98.634)
(215, 96.292)
(216, 98.044)
(217, 97.356)
(218, 97.804)
(219, 95.832)
(220, 98.392)
(221, 96.404)
(222, 97.688)
(223, 98.138)
(224, 95.96)
(225, 97.392)
(226, 99.026)
(227, 98.344)
(228, 95.752)
(229, 98.488)
(230, 97.622)
(231, 94.726)
(232, 95.964)
(233, 91.84)
(234, 95.946)
(235, 97.138)
(236, 95.66)
(237, 94.658)
(238, 95.724)
(239, 94.168)
(240, 97.068)
(241, 94.27)
(242, 95.76)
(243, 97.94)
(244, 88.642)
(245, 89.442)
(246, 84.154)
(247, 89.802)
(248, 89.418)
(249, 84.042)
(250, 81.314)
(251, 82.578)
(252, 74.872)
(253, 67.094)
(254, 87.424)
(255, 91.774)
(256, 94.258)
(257, 93.314)
(258, 91.484)
(259, 79.442)
(260, 24.78)
(261, 13.818)
(262, 37.576)
(263, 48.288)
(264, 18.34)
(265, 5.07)
(266, 57.492)
(267, 57.206)
(268, 49.844)
(269, 62.382)
(270, 78.268)
(271, 80.31)
(272, 86.426)
(273, 86.858)
(274, 62.624)
(275, 67.618)
(276, 82.43)
(277, 88.76)
(278, 77.738)
(279, 80.074)
(280, 91.174)
(281, 84.134)
(282, 86.724)
(283, 88.5)
(284, 86.796)
(285, 94.916)
(286, 95.488)
(287, 94.854)
(288, 92.406)
(289, 94.732)
(290, 92.206)
(291, 93.568)
(292, 91.09)
(293, 94.362)
(294, 95.892)
(295, 97.622)
(296, 96.742)
(297, 92.374)
(298, 91.796)
(299, 97.46)
(300, 98.882)
(301, 98.368)
(302, 98.224)
(303, 96.996)
(304, 98.028)
(305, 98.58)
(306, 97.118)
(307, 96.814)
(308, 96.686)
(309, 96.764)
(310, 97.698)
(311, 97.326)
(312, 97.266)
(313, 96.41)
(314, 97.026)
(315, 93.062)
(316, 92.482)
(317, 93.386)
(318, 93.592)
(319, 92.998)
(320, 91.796)
(321, 97.302)
(322, 96.482)
(323, 89.934)
(324, 83.976)
(325, 90.672)
(326, 78.268)
(327, 86.502)
(328, 90.102)
(329, 88.65)
(330, 95.558)
(331, 95.83)
(332, 95.142)
(333, 95.258)
(334, 95.25)
(335, 93.492)
(336, 94.646)
(337, 97.696)
(338, 97.35)
(339, 94.93)
(340, 90.898)
(341, 93.842)
(342, 94.886)
(343, 89.336)
(344, 86.614)
(345, 87.172)
(346, 90.19)
(347, 94.838)
(348, 94.35)
(349, 97.222)
(350, 93.458)
(351, 95.218)
(352, 96.268)
(353, 96.99)
(354, 94.034)
(355, 97.794)
(356, 96.916)
(357, 96.408)
(358, 97.804)
(359, 96.354)
(360, 98.724)
(361, 97.848)
(362, 97.382)
(363, 97.75)
(364, 98.568)
(365, 96.368)
(366, 96.848)
(367, 98.118)
(368, 97.704)
(369, 97.646)
(370, 96.354)
(371, 97.086)
(372, 96.35)
(373, 96.424)
(374, 95.268)
(375, 95.376)
(376, 96.422)
(377, 96.934)
(378, 96.742)
(379, 98.414)
(380, 98.294)
(381, 98.224)
(382, 98.28)
(383, 97.678)
(384, 96.796)
(385, 97.978)
(386, 97.572)
(387, 95.428)
(388, 97.336)
(389, 98.418)
(390, 98.784)
(391, 97.962)
(392, 98.368)
(393, 97.836)
(394, 98.672)
(395, 98.108)
(396, 99.04)
(397, 98.916)
(398, 98.922)
(399, 99.06)
(400, 98.916)
(401, 99.364)
(402, 99.116)
(403, 98.77)
(404, 99.244)
(405, 98.524)
(406, 98.71)
(407, 99.372)
(408, 96.35)
(409, 98.21)
(410, 98.406)
(411, 98.248)
(412, 98.406)
(413, 92.804)
(414, 93.38)
(415, 99.14)
(416, 98.988)
(417, 99.416)
(418, 99.112)
(419, 99.82)
(420, 99.47)
(421, 99.058)
(422, 99.206)
(423, 99.776)
(424, 99.414)
(425, 98.222)
(426, 96.75)
(427, 99.528)
(428, 99.688)
(429, 99.374)
(430, 99.078)
(431, 99.674)
(432, 99.818)
(433, 99.74)
(434, 99.48)
(435, 99.496)
(436, 95.9)
(437, 99.048)
(438, 99.368)
(439, 99.662)
(440, 99.776)
(441, 99.692)
(442, 99.424)
(443, 98.99)
(444, 99.558)
(445, 99.798)
(446, 99.57)
(447, 89.104)
(448, 99.408)
(449, 93.81)
(450, 99.716)
(451, 82.59)
(452, 85.216)
(453, 89.332)
(454, 99.916)
(455, 99.722)
(456, 99.596)
(457, 99.974)
(458, 100)
(459, 100)
(460, 100)
(461, 99.978)
(462, 99.878)
(463, 99.802)
(464, 99.994)
(465, 99.984)
(466, 99.862)
(467, 99.998)
(468, 100)
(469, 99.97)
(470, 99.782)
(471, 99.916)
(472, 99.874)
(473, 99.936)
(474, 99.996)
(475, 99.984)
(476, 99.996)
(477, 99.99)
(478, 99.768)
(479, 95.022)
(480, 99.938)
(481, 99.678)
(482, 99.262)
(483, 98.752)
(484, 97.69)
(485, 97.74)
(486, 99.716)
(487, 99.146)
(488, 99.628)
(489, 99.398)
(490, 99.426)
(491, 99.726)
(492, 99.744)
(493, 99.264)
(494, 98.608)
(495, 99.734)
(496, 98.912)
(497, 98.364)
(498, 91.992)
(499, 95.5)
(500, 98.846)
(501, 97.004)
(502, 98.926)
(503, 99.134)
(504, 99.762)
(505, 99.674)
(506, 99.692)
(507, 98.41)
(508, 99.494)
(509, 99.438)
(510, 97.996)
(511, 99.686)
(512, 98.854)
(513, 95.698)
(514, 98.786)
(515, 94.592)
(516, 99.252)
(517, 99.446)
(518, 99.214)
(519, 97.32)
(520, 94.264)
(521, 94.576)
(522, 97.598)
(523, 98.324)
(524, 99.446)
(525, 97.154)
(526, 85.996)
(527, 97.568)
(528, 97.324)
(529, 98.938)
(530, 99.508)
(531, 98.374)
(532, 97.36)
(533, 97.97)
(534, 97.522)
(535, 98.224)
(536, 98.98)
(537, 99.492)
(538, 99.514)
(539, 98.526)
(540, 97.544)
(541, 99.472)
(542, 98.116)
(543, 98.586)
(544, 96.594)
(545, 99.176)
(546, 99.522)
(547, 98.256)
(548, 98.414)
(549, 97.164)
(550, 98.24)
(551, 98.706)
(552, 96.94)
(553, 95.664)
(554, 98.404)
(555, 97.5)
(556, 93.116)
(557, 89.166)
(558, 99.446)
(559, 99.434)
(560, 95.5)
(561, 89.174)
(562, 95.974)
(563, 94.046)
(564, 90.774)
(565, 82.91)
(566, 69.302)
(567, 89.894)
(568, 88.508)
(569, 95.432)
(570, 90.276)
(571, 90.646)
(572, 88.036)
(573, 84.092)
(574, 92.078)
(575, 86.324)
(576, 96.866)
(577, 92.232)
(578, 96.3)
(579, 93.82)
(580, 88.544)
(581, 98.728)
(582, 99.59)
(583, 99.62)
(584, 99.702)
(585, 99.752)
(586, 99.802)
(587, 99.8)
(588, 99.548)
(589, 99.832)
(590, 99.812)
(591, 94.976)
(592, 99.816)
(593, 98.766)
(594, 95.746)
(595, 97.06)
(596, 98.566)
(597, 93.022)
(598, 95.088)
(599, 91.46)
(600, 96.962)
(601, 94.914)
(602, 98.11)
(603, 97.306)
(604, 99.728)
(605, 99.786)
(606, 99.574)
(607, 99.244)
(608, 98.98)
(609, 98.862)
(610, 98.604)
(611, 98.522)
(612, 98.538)
(613, 93.662)
(614, 97.166)
(615, 96.212)
(616, 98.802)
(617, 97.292)
(618, 99.246)
(619, 99.444)
(620, 99.71)
(621, 99.886)
(622, 99.752)
(623, 99.82)
(624, 99.89)
(625, 99.868)
(626, 99.888)
(627, 99.61)
(628, 99.65)
(629, 94.366)
(630, 92.506)
(631, 95.036)
(632, 99.86)
(633, 99.934)
(634, 99.844)
(635, 99.938)
(636, 99.488)
(637, 99.746)
(638, 99.77)
(639, 99.384)
(640, 99.712)
(641, 99.756)
(642, 99.516)
(643, 99.57)
(644, 99.696)
(645, 99.702)
(646, 99.72)
(647, 99.918)
(648, 99.956)
(649, 99.716)
(650, 96.462)
(651, 98.358)
(652, 98.716)
(653, 98.156)
(654, 96.074)
(655, 95.168)
(656, 97.698)
(657, 99.404)
(658, 98.41)
(659, 98.002)
(660, 98.228)
(661, 99.706)
(662, 99.974)
(663, 99.936)
(664, 99.868)
(665, 99.914)
(666, 99.64)
(667, 99.646)
(668, 99.738)
(669, 99.742)
(670, 99.704)
(671, 99.778)
(672, 99.21)
(673, 95.51)
(674, 98.556)
(675, 96.022)
(676, 97.798)
(677, 97.7)
(678, 95.16)
(679, 96.598)
(680, 99.096)
(681, 98.02)
(682, 99.302)
(683, 99.544)
(684, 99.208)
(685, 99.032)
(686, 99.978)
(687, 99.828)
(688, 99.988)
(689, 99.922)
(690, 99.626)
(691, 99.97)
(692, 98.994)
(693, 98.004)
(694, 99.202)
(695, 99.88)
(696, 98.512)
(697, 77.344)
(698, 90.74)
(699, 96.238)
(700, 99.348)
(701, 96.146)
(702, 98.808)
(703, 99.382)
(704, 97.996)
(705, 96.692)
(706, 97.22)
(707, 99.164)
(708, 99.554)
(709, 98.876)
(710, 99.37)
(711, 99.666)
(712, 99.184)
(713, 89.092)
(714, 92.512)
(715, 98.552)
(716, 98.306)
(717, 97.948)
(718, 98.21)
(719, 96.548)
(720, 99.258)
(721, 99.8)
(722, 99.476)
(723, 99.604)
(724, 99.408)
(725, 98.852)
(726, 97.938)
(727, 98.264)
(728, 97.996)
(729, 98.64)
(730, 98.406)
(731, 98.392)
(732, 98.2)
(733, 98.51)
(734, 97.068)
(735, 98.874)
(736, 98.44)
(737, 94.15)
(738, 96.752)
(739, 96.864)
(740, 98.044)
(741, 97.254)
(742, 99.06)
(743, 97.186)
(744, 98.548)
(745, 97.87)
(746, 98.862)
(747, 93.65)
(748, 64.748)
(749, 98.692)
(750, 96.636)
(751, 98.858)
(752, 99.796)
(753, 99.036)
(754, 99.702)
(755, 99.676)
(756, 99.464)
(757, 99.442)
(758, 96.042)
(759, 99.724)
(760, 99.876)
(761, 96.816)
(762, 92.794)
(763, 99.374)
(764, 98.438)
(765, 99.598)
(766, 99.928)
(767, 99.93)
(768, 99.922)
(769, 98.904)
(770, 98.808)
(771, 98.738)
(772, 96.002)
(773, 99)
(774, 99.58)
(775, 99.592)
(776, 98.858)
(777, 99.786)
(778, 99.996)
(779, 99.99)
(780, 99.988)
(781, 99.968)
(782, 98.362)
(783, 99.62)
(784, 99.912)
(785, 99.86)
(786, 99.918)
(787, 99.98)
(788, 99.852)
(789, 99.032)
(790, 99.314)
(791, 99.67)
(792, 99.798)
(793, 99.148)
(794, 99.59)
(795, 99.49)
(796, 98.582)
(797, 99.882)
(798, 99.778)
(799, 99.768)
(800, 99.98)
(801, 99.968)
(802, 99.272)
(803, 99.694)
(804, 99.568)
(805, 99.79)
(806, 98.814)
(807, 99.77)
(808, 99.386)
(809, 99.748)
(810, 99.252)
(811, 99.584)
(812, 99.978)
(813, 99.962)
(814, 99.946)
(815, 99.75)
(816, 99.814)
(817, 99.852)
(818, 99.606)
(819, 98.948)
(820, 99.472)
(821, 99.826)
(822, 99.104)
(823, 99.652)
(824, 99.738)
(825, 99.418)
(826, 98.574)
(827, 98.636)
(828, 99.102)
(829, 98.986)
(830, 99.402)
(831, 98.792)
(832, 99.662)
(833, 97.676)
(834, 98.86)
(835, 99.338)
(836, 99.776)
(837, 98.034)
(838, 98.22)
(839, 98.98)
(840, 98.998)
(841, 98.846)
(842, 99.212)
(843, 98.84)
(844, 97.99)
(845, 97.962)
(846, 98.84)
(847, 99.014)
(848, 99.412)
(849, 98.94)
(850, 99.458)
(851, 99.432)
(852, 99.786)
(853, 99.658)
(854, 99.476)
(855, 99.592)
(856, 99.78)
(857, 99.22)
(858, 99.478)
(859, 99.948)
(860, 99.84)
(861, 99.766)
(862, 99.926)
(863, 99.964)
(864, 99.682)
(865, 97.302)
(866, 99.474)
(867, 99.54)
(868, 99.15)
(869, 99.796)
(870, 98.786)
(871, 99.594)
(872, 99.542)
(873, 99.7)
(874, 99.2)
(875, 99.262)
(876, 99.692)
(877, 99.784)
(878, 99.514)
(879, 99.686)
(880, 99.04)
(881, 99.466)
(882, 99.138)
(883, 99.59)
(884, 96.976)
(885, 98.38)
(886, 99.46)
(887, 99.772)
(888, 99.842)
(889, 97.724)
(890, 99.23)
(891, 99.22)
(892, 96.368)
(893, 99.396)
(894, 98.886)
(895, 99.302)
(896, 99.066)
(897, 98.248)
(898, 98.568)
(899, 98.194)
(900, 98.596)
(901, 99.664)
(902, 98.458)
(903, 97.71)
(904, 98.284)
(905, 99.028)
(906, 99.462)
(907, 99.73)
(908, 99.682)
(909, 99.6)
(910, 99.112)
(911, 99.798)
(912, 99.562)
(913, 99.554)
(914, 99.346)
(915, 99.49)
(916, 99.598)
(917, 99.584)
(918, 99.426)
(919, 99.58)
(920, 99.61)
(921, 99.806)
(922, 99.778)
(923, 99.334)
(924, 98.73)
(925, 99.528)
(926, 99.784)
(927, 99.93)
(928, 99.574)
(929, 99.628)
(930, 99.362)
(931, 99.604)
(932, 99.532)
(933, 99.848)
(934, 99.726)
(935, 98.88)
(936, 99.546)
(937, 99.7)
(938, 99.774)
(939, 98.032)
(940, 98.876)
(941, 99.654)
(942, 99.042)
(943, 99.618)
(944, 99.65)
(945, 98.822)
(946, 96.998)
(947, 99.76)
(948, 99.87)
(949, 99.612)
(950, 99.484)
(951, 99.738)
(952, 99.91)
(953, 99.81)
(954, 99.958)
(955, 99.922)
(956, 99.976)
(957, 99.95)
(958, 99.986)
(959, 99.994)
(960, 99.942)
(961, 99.72)
(962, 99.756)
(963, 99.866)
(964, 99.484)
(965, 98.43)
(966, 99.258)
(967, 99.47)
(968, 99.732)
(969, 99.786)
(970, 99.954)
(971, 99.896)
(972, 99.792)
(973, 99.772)
(974, 99.694)
(975, 99.376)
(976, 99.81)
(977, 99.846)
(978, 99.71)
(979, 95.41)
(980, 99.344)
(981, 99.788)
(982, 99.164)
(983, 98.912)
(984, 97.068)
(985, 92.274)
(986, 99.818)
(987, 99.23)
(988, 99.778)
(989, 99.696)
(990, 99.884)
(991, 99.688)
(992, 99.824)
(993, 99.546)
(994, 98.922)
(995, 98.208)
(996, 99.506)
(997, 99.74)
(998, 99.694)
(999, 99.712)
(1000, 99.268)
(1001, 99.68)
(1002, 99.456)
(1003, 99.238)
(1004, 99.186)
(1005, 99.534)
(1006, 98.618)
(1007, 98.968)
(1008, 99.704)
(1009, 99.352)
(1010, 99.858)
(1011, 99.462)
(1012, 99.866)
(1013, 99.512)
(1014, 99.564)
(1015, 89.328)
(1016, 98.992)
(1017, 96.894)
(1018, 98.084)
(1019, 97.746)
(1020, 96.44)
(1021, 99.736)
(1022, 99.372)
(1023, 99.086)
(1024, 99.376)
(1025, 98.644)
(1026, 98.674)
(1027, 96.614)
(1028, 99.13)
(1029, 99.714)
(1030, 99.834)
(1031, 99.826)
(1032, 99.794)
(1033, 99.474)
(1034, 99.47)
(1035, 99.182)
(1036, 98.98)
(1037, 99.072)
(1038, 98.788)
(1039, 97.856)
(1040, 98.894)
(1041, 97.026)
(1042, 98.034)
(1043, 98.386)
(1044, 99.834)
(1045, 92.266)
(1046, 92.17)
(1047, 94.394)
(1048, 89.806)
(1049, 90.002)
(1050, 89.774)
(1051, 95.554)
(1052, 99.84)
(1053, 99.994)
(1054, 96.368)
(1055, 100)
(1056, 100)
(1057, 99.948)
(1058, 99.892)
(1059, 99.786)
(1060, 99.482)
(1061, 99.704)
(1062, 99.81)
(1063, 99.89)
(1064, 99.82)
(1065, 99.808)
(1066, 99.86)
(1067, 99.77)
(1068, 99.842)
(1069, 99.958)
(1070, 99.916)
(1071, 99.99)
(1072, 99.972)
(1073, 99.976)
(1074, 99.992)
(1075, 99.95)
(1076, 99.98)
(1077, 99.904)
(1078, 99.95)
(1079, 99.96)
(1080, 99.648)
(1081, 99.838)
(1082, 99.404)
(1083, 99.28)
(1084, 99.984)
(1085, 99.994)
(1086, 99.972)
(1087, 99.936)
(1088, 99.246)
(1089, 99.76)
(1090, 99.522)
(1091, 99.958)
(1092, 99.408)
(1093, 97.652)
(1094, 98.2)
(1095, 87.742)
(1096, 99.666)
(1097, 99.3)
(1098, 99.452)
(1099, 98.956)
(1100, 99.352)
(1101, 99.574)
(1102, 99.616)
(1103, 98.96)
(1104, 99.724)
(1105, 99.714)
(1106, 99.896)
(1107, 99.99)
(1108, 99.428)
(1109, 99.726)
(1110, 99.602)
(1111, 99.758)
(1112, 99.788)
(1113, 98.71)
(1114, 99.528)
(1115, 99.96)
(1116, 99.976)
(1117, 99.984)
(1118, 99.994)
(1119, 99.95)
(1120, 99.91)
(1121, 99.574)
(1122, 99.938)
(1123, 99.992)
(1124, 99.724)
(1125, 99.58)
(1126, 100)
(1127, 99.994)
(1128, 99.968)
(1129, 99.96)
(1130, 99.886)
(1131, 99.75)
(1132, 94.898)
(1133, 92.838)
(1134, 95.142)
(1135, 99.926)
(1136, 99.998)
(1137, 99.99)
(1138, 100)
(1139, 100)
(1140, 99.996)
(1141, 100)
(1142, 100)
(1143, 99.992)
(1144, 99.826)
(1145, 99.896)
(1146, 99.99)
(1147, 99.906)
(1148, 98.882)
(1149, 98.008)
(1150, 100)
(1151, 99.968)
(1152, 99.988)
(1153, 99.996)
(1154, 100)
(1155, 99.938)
(1156, 100)
(1157, 100)
(1158, 100)
(1159, 99.98)
(1160, 99.814)
(1161, 99.944)
(1162, 100)
(1163, 100)
(1164, 100)
(1165, 100)
(1166, 100)
(1167, 100)
(1168, 99.996)
(1169, 99.988)
(1170, 100)
(1171, 99.922)
(1172, 99.956)
(1173, 99.776)
(1174, 99.926)
(1175, 98.708)
(1176, 99.796)
(1177, 99.682)
(1178, 99.896)
(1179, 99.872)
(1180, 99.902)
(1181, 99.776)
(1182, 99.902)
(1183, 99.774)
(1184, 99.942)
(1185, 99.8)
(1186, 99.9)
(1187, 99.912)
(1188, 99.646)
(1189, 99.94)
(1190, 97.682)
(1191, 98.194)
(1192, 99.936)
(1193, 98.788)
(1194, 97.488)
(1195, 98.072)
(1196, 99.036)
(1197, 96.53)
(1198, 99.016)
(1199, 97.776)
(1200, 98.268)
(1201, 97.978)
(1202, 99.328)
(1203, 99.052)
(1204, 99.744)
(1205, 99.792)
(1206, 99.608)
(1207, 99.692)
(1208, 99.374)
(1209, 99.85)
(1210, 99.51)
(1211, 99.496)
(1212, 99.044)
(1213, 99.66)
(1214, 99.39)
(1215, 99.664)
(1216, 99.964)
(1217, 99.792)
(1218, 99.514)
(1219, 99.276)
(1220, 99.31)
(1221, 98.412)
(1222, 97.156)
(1223, 99.334)
(1224, 98.456)
(1225, 98.028)
(1226, 97.104)
(1227, 98.244)
(1228, 95.192)
(1229, 97.426)
(1230, 97.384)
(1231, 94.596)
(1232, 96.074)
(1233, 98.198)
(1234, 99.426)
(1235, 98.754)
(1236, 99.446)
(1237, 98.972)
(1238, 98.224)
(1239, 97.024)
(1240, 97.118)
(1241, 94.448)
(1242, 95.902)
(1243, 97.726)
(1244, 93.198)
(1245, 98.454)
(1246, 96.958)
(1247, 98.312)
(1248, 97.468)
(1249, 98.818)
(1250, 98.27)
(1251, 99.106)
(1252, 97.97)
(1253, 98.714)
(1254, 98.626)
(1255, 98.862)
(1256, 98.192)
(1257, 98.722)
(1258, 98.164)
(1259, 99.3)
(1260, 98.506)
(1261, 99.484)
(1262, 99.792)
(1263, 99.264)
(1264, 98.75)
(1265, 99.696)
(1266, 99.176)
(1267, 99.794)
(1268, 99.808)
(1269, 99.93)
(1270, 99.832)
(1271, 99.984)
(1272, 99.99)
(1273, 99.992)
(1274, 99.766)
(1275, 99.986)
(1276, 99.904)
(1277, 98.924)
(1278, 98.754)
(1279, 98.12)
(1280, 98.236)
(1281, 98.946)
(1282, 99.652)
(1283, 98.928)
(1284, 98.652)
(1285, 99.29)
(1286, 99.672)
(1287, 98.856)
(1288, 99.388)
(1289, 99.32)
(1290, 97.282)
(1291, 97.766)
(1292, 97.778)
(1293, 97.612)
(1294, 98.458)
(1295, 98.302)
(1296, 98.286)
(1297, 96.612)
(1298, 97.508)
(1299, 97.39)
(1300, 98.044)
(1301, 99.418)
(1302, 99.754)
(1303, 99.304)
(1304, 99.338)
(1305, 99.286)
(1306, 99.572)
(1307, 99.3)
(1308, 99.684)
(1309, 98.048)
(1310, 99.818)
(1311, 99.798)
(1312, 99.75)
(1313, 99.724)
(1314, 99.608)
(1315, 98.32)
(1316, 99.72)
(1317, 99.392)
(1318, 99.362)
(1319, 99.784)
(1320, 99.866)
(1321, 99.956)
(1322, 99.732)
(1323, 99.942)
(1324, 99.88)
(1325, 99.662)
(1326, 99.428)
(1327, 98.396)
(1328, 97.696)
(1329, 99.29)
(1330, 99.642)
(1331, 99.342)
(1332, 99.336)
(1333, 99.316)
(1334, 99.46)
(1335, 95.904)
(1336, 99.524)
(1337, 99.684)
(1338, 99.35)
(1339, 99.024)
(1340, 99.568)
(1341, 99.074)
(1342, 98.748)
(1343, 98.462)
(1344, 98.988)
(1345, 97.474)
(1346, 98.328)
(1347, 94.21)
(1348, 99.418)
(1349, 99.556)
(1350, 99.266)
(1351, 99.666)
(1352, 99.604)
(1353, 99.508)
(1354, 99.558)
(1355, 99.382)
(1356, 99.516)
(1357, 99.806)
(1358, 98.912)
(1359, 99.512)
(1360, 99.634)
(1361, 97.71)
(1362, 99.63)
(1363, 99.054)
(1364, 99.634)
(1365, 99.738)
(1366, 98.996)
(1367, 99.526)
(1368, 99.39)
(1369, 99.25)
(1370, 93.256)
(1371, 99.37)
(1372, 99.426)
(1373, 99.322)
(1374, 99.068)
(1375, 98.572)
(1376, 99.062)
(1377, 97.554)
(1378, 98.806)
(1379, 97.346)
(1380, 99.124)
(1381, 99.108)
(1382, 99.05)
(1383, 99.162)
(1384, 95.588)
(1385, 98.768)
(1386, 96.588)
(1387, 97.602)
(1388, 98.202)
(1389, 98.38)
(1390, 97.844)
(1391, 98.912)
(1392, 99.23)
(1393, 99.16)
(1394, 99.578)
(1395, 99.384)
(1396, 99.404)
(1397, 99.432)
(1398, 98.952)
(1399, 99.28)
(1400, 99.04)
(1401, 97.96)
(1402, 99.498)
(1403, 99.194)
(1404, 99.428)
(1405, 99.302)
(1406, 98.384)
(1407, 94.036)
(1408, 98.93)
(1409, 97.874)
(1410, 99.554)
(1411, 99.488)
(1412, 99.072)
(1413, 99.548)
(1414, 99.634)
(1415, 99.37)
(1416, 99.29)
(1417, 99.07)
(1418, 99.706)
(1419, 99.772)
(1420, 99.674)
(1421, 99.5)
(1422, 99.48)
(1423, 99.286)
(1424, 99.606)
(1425, 99.494)
(1426, 97.096)
(1427, 98.652)
(1428, 98.544)
(1429, 99.67)
(1430, 99.852)
(1431, 99.818)
(1432, 99.772)
(1433, 99.384)
(1434, 99.416)
(1435, 99.512)
(1436, 99.788)
(1437, 99.292)
(1438, 99.424)
(1439, 99.666)
(1440, 99.332)
(1441, 97.558)
(1442, 98.898)
(1443, 96.258)
(1444, 97.584)
(1445, 95.468)
(1446, 94.85)
(1447, 97.232)
(1448, 97.724)
(1449, 95.746)
(1450, 94.714)
(1451, 95.766)
(1452, 96.888)
(1453, 92.414)
(1454, 98.042)
(1455, 97.374)
(1456, 98.524)
(1457, 92.646)
(1458, 66.51)
(1459, 83.14)
(1460, 93.346)
(1461, 72.816)
(1462, 81.238)
(1463, 67.842)
(1464, 81.06)
(1465, 99.338)
(1466, 91.43)
(1467, 69.714)
(1468, 90.068)
(1469, 99.648)
(1470, 99.734)
(1471, 99.862)
(1472, 81.45)
(1473, 64.604)
(1474, 99.85)
(1475, 94.238)
(1476, 94.404)
(1477, 92.966)
(1478, 97.076)
(1479, 97.27)
(1480, 99.478)
(1481, 99.67)
(1482, 98.96)
(1483, 99.698)
(1484, 99.012)
(1485, 95.192)
(1486, 98.144)
(1487, 98.558)
(1488, 99.54)
(1489, 98.358)
(1490, 99.458)
(1491, 99.578)
(1492, 98.472)
(1493, 99.492)
(1494, 99.938)
(1495, 99.918)
(1496, 99.81)
(1497, 99.864)
(1498, 99.49)
(1499, 99.7)
(1500, 99.498)
(1501, 99.374)
(1502, 99.114)
(1503, 99.772)
(1504, 98.072)
(1505, 99.606)
(1506, 99.596)
(1507, 99.94)
(1508, 99.554)
(1509, 99.502)
(1510, 98.336)
(1511, 98.082)
(1512, 98.796)
(1513, 99.188)
(1514, 98.974)
(1515, 99.102)
(1516, 99.324)
(1517, 99.008)
(1518, 98.636)
(1519, 98.556)
(1520, 98.124)
(1521, 98.742)
(1522, 98.276)
(1523, 98.918)
(1524, 99.352)
(1525, 99.168)
(1526, 98.89)
(1527, 99.022)
(1528, 99.412)
(1529, 99.756)
(1530, 99.056)
(1531, 93.59)
(1532, 98.238)
(1533, 99.246)
(1534, 99.146)
(1535, 99.122)
(1536, 99.606)
(1537, 99.896)
(1538, 99.74)
(1539, 99.786)
(1540, 99.924)
(1541, 99.87)
(1542, 99.638)
(1543, 99.12)
(1544, 99.57)
(1545, 99.474)
(1546, 99.788)
(1547, 99.906)
(1548, 99.934)
(1549, 99.524)
(1550, 99.53)
(1551, 97.86)
(1552, 94.686)
(1553, 99.96)
(1554, 99.606)
(1555, 99.854)
(1556, 99.872)
(1557, 99.91)
(1558, 99.612)
(1559, 99.782)
(1560, 99.36)
(1561, 99.75)
(1562, 99.97)
(1563, 99.568)
(1564, 99.542)
(1565, 99.97)
(1566, 99.828)
(1567, 99.848)
(1568, 98.088)
(1569, 99.99)
(1570, 99.638)
(1571, 99.222)
(1572, 99.936)
(1573, 99.948)
(1574, 99.524)
(1575, 99.142)
(1576, 99.43)
(1577, 99.684)
(1578, 99.402)
(1579, 99.384)
(1580, 99.32)
(1581, 99.626)
(1582, 99.896)
(1583, 99.478)
(1584, 99.818)
(1585, 99.678)
(1586, 99.662)
(1587, 99.746)
(1588, 99.85)
(1589, 99.756)
(1590, 99.54)
(1591, 99.776)
(1592, 99.806)
(1593, 99.662)
(1594, 99.842)
(1595, 99.79)
(1596, 99.456)
(1597, 99.792)
(1598, 99.742)
(1599, 99.986)
(1600, 99.666)
(1601, 99.936)
(1602, 99.736)
(1603, 99.776)
(1604, 99.824)
(1605, 99.638)
(1606, 99.312)
(1607, 99.668)
(1608, 99.806)
(1609, 99.714)
(1610, 99.602)
(1611, 99.846)
(1612, 99.608)
(1613, 99.8)
(1614, 98.946)
(1615, 99.398)
(1616, 99.316)
(1617, 99.624)
(1618, 99.656)
(1619, 95.956)
(1620, 98.86)
(1621, 90.424)
(1622, 99.03)
(1623, 99.088)
(1624, 99.838)
(1625, 99.86)
(1626, 99.892)
(1627, 98.482)
(1628, 99.91)
(1629, 99.944)
(1630, 99.864)
(1631, 99.544)
(1632, 99.692)
(1633, 98.894)
(1634, 99.7)
(1635, 99.438)
(1636, 98.968)
(1637, 99.27)
(1638, 99.922)
(1639, 99.93)
(1640, 99.986)
(1641, 99.934)
(1642, 99.742)
(1643, 99.32)
(1644, 99.436)
(1645, 99.498)
(1646, 99.072)
(1647, 99.838)
(1648, 99.296)
(1649, 99.836)
(1650, 99.718)
(1651, 99.754)
(1652, 99.514)
(1653, 98.172)
(1654, 99.642)
(1655, 99.356)
(1656, 98.446)
(1657, 98.702)
(1658, 98.364)
(1659, 99.292)
(1660, 98.282)
(1661, 99.526)
(1662, 94.394)
(1663, 99.716)
(1664, 99.518)
(1665, 99.328)
(1666, 98.242)
(1667, 99.61)
(1668, 99.542)
(1669, 97.35)
(1670, 98.902)
(1671, 98.214)
(1672, 98.996)
(1673, 97.828)
(1674, 99.882)
(1675, 99.62)
(1676, 99.062)
(1677, 99.094)
(1678, 99.108)
(1679, 99.482)
(1680, 98.524)
(1681, 99.712)
(1682, 99.696)
(1683, 99.726)
(1684, 99.016)
(1685, 99.394)
(1686, 99.286)
(1687, 99.784)
(1688, 99.382)
(1689, 99.466)
(1690, 99.692)
(1691, 99.724)
(1692, 99.7)
(1693, 99.772)
(1694, 99.93)
(1695, 99.798)
(1696, 99.95)
(1697, 99.512)
(1698, 99.932)
(1699, 99.89)
(1700, 99.928)
(1701, 99.824)
(1702, 99.802)
(1703, 99.82)
(1704, 99.966)
(1705, 99.812)
(1706, 99.786)
(1707, 99.852)
(1708, 98.87)
(1709, 99.506)
(1710, 99.706)
(1711, 99.712)
(1712, 99.902)
(1713, 99.678)
(1714, 99.898)
(1715, 99.826)
(1716, 99.892)
(1717, 99.96)
(1718, 99.96)
(1719, 98.28)
(1720, 98.986)
(1721, 99.746)
(1722, 99.516)
(1723, 99.822)
(1724, 99.618)
(1725, 99.666)
(1726, 99.642)
(1727, 99.896)
(1728, 99.632)
(1729, 99.504)
(1730, 99.126)
(1731, 99.866)
(1732, 99.082)
(1733, 99.288)
(1734, 99.714)
(1735, 99.668)
(1736, 99.584)
(1737, 99.87)
(1738, 99.768)
(1739, 99.808)
(1740, 99.382)
(1741, 98.954)
(1742, 99.85)
(1743, 99.788)
(1744, 99.998)
(1745, 100)
(1746, 100)
(1747, 99.99)
(1748, 100)
(1749, 100)
(1750, 99.928)
(1751, 100)
(1752, 99.994)
(1753, 99.798)
(1754, 100)
(1755, 100)
(1756, 99.952)
(1757, 99.992)
(1758, 100)
(1759, 100)
(1760, 100)
(1761, 99.978)
(1762, 99.998)
(1763, 99.972)
(1764, 99.966)
(1765, 100)
(1766, 99.832)
(1767, 99.798)
(1768, 100)
(1769, 100)
(1770, 99.774)
(1771, 99.74)
(1772, 99.966)
(1773, 99.99)
(1774, 99.972)
(1775, 99.984)
(1776, 99.946)
(1777, 99.99)
(1778, 99.998)
(1779, 99.992)
(1780, 99.98)
(1781, 99.872)
(1782, 99.83)
(1783, 99.61)
(1784, 99.968)
(1785, 99.996)
(1786, 99.974)
(1787, 99.94)
(1788, 99.814)
(1789, 99.824)
(1790, 99.89)
(1791, 99.968)
(1792, 99.83)
(1793, 99.79)
(1794, 99.92)
(1795, 99.932)
(1796, 99.048)
(1797, 99.986)
(1798, 99.998)
(1799, 99.966)
(1800, 99.968)
(1801, 99.814)
(1802, 99.902)
(1803, 99.944)
(1804, 99.924)
(1805, 99.976)
(1806, 99.956)
(1807, 99.964)
(1808, 99.72)
(1809, 99.888)
(1810, 99.748)
(1811, 99.994)
(1812, 99.848)
(1813, 99.786)
(1814, 99.464)
(1815, 99.868)
(1816, 98.178)
(1817, 99.836)
(1818, 99.948)
(1819, 99.628)
(1820, 93.872)
(1821, 99.466)
(1822, 99.79)
(1823, 99.818)
(1824, 99.536)
(1825, 99.768)
(1826, 99.834)
(1827, 99.73)
(1828, 99.15)
(1829, 99.872)
(1830, 99.89)
(1831, 99.434)
(1832, 99.516)
(1833, 99.818)
(1834, 99.702)
(1835, 99.868)
(1836, 99.932)
(1837, 99.404)
(1838, 99.924)
(1839, 99.726)
(1840, 97.688)
(1841, 99.824)
(1842, 99.962)
(1843, 99.994)
(1844, 99.958)
(1845, 99.908)
(1846, 99.972)
(1847, 99.964)
(1848, 99.998)
(1849, 99.99)
(1850, 99.936)
(1851, 100)
(1852, 99.972)
(1853, 99.998)
(1854, 99.998)
(1855, 99.966)
(1856, 99.926)
(1857, 99.87)
(1858, 99.948)
(1859, 99.88)
(1860, 99.98)
(1861, 99.88)
(1862, 99.986)
(1863, 99.986)
(1864, 99.99)
(1865, 99.926)
(1866, 99.418)
(1867, 99.652)
(1868, 99.566)
(1869, 95.726)
(1870, 99.968)
(1871, 99.86)
(1872, 99.928)
(1873, 99.89)
(1874, 99.49)
(1875, 99.914)
(1876, 99.68)
(1877, 99.952)
(1878, 99.908)
(1879, 99.68)
(1880, 99.352)
(1881, 98.614)
(1882, 99.736)
(1883, 99.958)
(1884, 99.73)
(1885, 98.702)
(1886, 99.792)
(1887, 99.702)
(1888, 99.93)
(1889, 99.98)
(1890, 99.862)
(1891, 99.94)
(1892, 99.98)
(1893, 99.944)
(1894, 99.968)
(1895, 98.772)
(1896, 99.914)
(1897, 99.98)
(1898, 99.996)
(1899, 99.99)
(1900, 99.946)
(1901, 99.922)
(1902, 99.92)
(1903, 99.934)
(1904, 99.896)
(1905, 99.99)
(1906, 99.92)
(1907, 99.806)
(1908, 99.664)
(1909, 99.954)
(1910, 99.822)
(1911, 99.914)
(1912, 99.92)
(1913, 99.962)
(1914, 99.758)
(1915, 99.914)
(1916, 99.376)
(1917, 99.916)
(1918, 99.988)
(1919, 99.95)
(1920, 99.892)
(1921, 99.738)
(1922, 99.968)
(1923, 99.942)
(1924, 99.836)
(1925, 99.874)
(1926, 99.956)
(1927, 99.912)
(1928, 99.868)
(1929, 99.8)
(1930, 99.96)
(1931, 99.906)
(1932, 99.972)
(1933, 99.898)
(1934, 99.012)
(1935, 89.236)
(1936, 96.904)
(1937, 98.158)
(1938, 98.096)
(1939, 98.98)
(1940, 96.798)
(1941, 98.992)
(1942, 98.1)
(1943, 98.078)
(1944, 98.676)
(1945, 98.026)
(1946, 98.44)
(1947, 96.598)
(1948, 96.006)
(1949, 98.898)
(1950, 98.762)
(1951, 96.32)
(1952, 98.226)
(1953, 97.788)
(1954, 97.97)
(1955, 98.918)
(1956, 98.8)
(1957, 98.888)
(1958, 99.3)
(1959, 99.086)
(1960, 95.628)
(1961, 98.096)
(1962, 98.54)
(1963, 99.278)
(1964, 99.352)
(1965, 99.418)
(1966, 99.222)
(1967, 99.516)
(1968, 99.06)
(1969, 99.064)
(1970, 99.78)
(1971, 99.544)
(1972, 99.726)
(1973, 99.424)
(1974, 99.218)
(1975, 98.516)
(1976, 98.79)
(1977, 98.84)
(1978, 98.678)
(1979, 99.478)
(1980, 98.612)
(1981, 99.158)
(1982, 98.402)
(1983, 97.816)
(1984, 96.894)
(1985, 96.298)
(1986, 95.298)
(1987, 94.316)
(1988, 93.002)
(1989, 91.738)
(1990, 97.528)
(1991, 96.662)
(1992, 96.858)
(1993, 99.06)
(1994, 98.842)
(1995, 99.178)
(1996, 98.586)
(1997, 99.126)
(1998, 98.956)
(1999, 99.136)
(2000, 99.03)
(2001, 98.77)
(2002, 98.71)
(2003, 99.138)
(2004, 99.052)
(2005, 99.246)
(2006, 97.832)
(2007, 99.162)
(2008, 99.186)
(2009, 99.43)
(2010, 99.496)
(2011, 98.9)
(2012, 98.842)
(2013, 99.488)
(2014, 98.278)
(2015, 96.254)
(2016, 98.902)
(2017, 98.812)
(2018, 99.238)
(2019, 98.716)
(2020, 98.624)
(2021, 98.508)
(2022, 98.93)
(2023, 98.684)
(2024, 99.51)
(2025, 99.212)
(2026, 99.356)
(2027, 99.102)
(2028, 99.044)
(2029, 99.658)
(2030, 98.74)
(2031, 99.74)
(2032, 99.484)
(2033, 98.92)
(2034, 99.108)
(2035, 99.57)
(2036, 99.644)
(2037, 99.196)
(2038, 99.466)
(2039, 99.652)
(2040, 99.686)
(2041, 99.488)
(2042, 99.26)
(2043, 99.398)
(2044, 99.084)
(2045, 98.264)
(2046, 99.508)
(2047, 99.272)
(2048, 98.486)
(2049, 99.528)
(2050, 99.444)
(2051, 98.958)
(2052, 99.702)
(2053, 99.53)
(2054, 99.554)
(2055, 99.446)
(2056, 99.1)
(2057, 97.698)
(2058, 97.114)
(2059, 98.344)
(2060, 99.268)
(2061, 99.508)
(2062, 98.658)
(2063, 96.762)
(2064, 93.688)
(2065, 98.346)
(2066, 97.93)
(2067, 96.716)
(2068, 95.366)
(2069, 96.88)
(2070, 96.7)
(2071, 96.856)
(2072, 97.938)
(2073, 99.14)
(2074, 99.042)
(2075, 98.732)
(2076, 99.128)
(2077, 98.126)
(2078, 99.358)
(2079, 99.254)
(2080, 98.696)
(2081, 98.988)
(2082, 98.344)
(2083, 99.138)
(2084, 99.202)
(2085, 99.252)
(2086, 99.498)
(2087, 99.37)
(2088, 99.19)
(2089, 99.51)
(2090, 99.134)
(2091, 98.47)
(2092, 99.238)
(2093, 99.2)
(2094, 99.222)
(2095, 99.184)
(2096, 99.336)
(2097, 94.608)
(2098, 86.834)
(2099, 89.612)
(2100, 99.866)
(2101, 99.774)
(2102, 99.77)
(2103, 99.548)
(2104, 99.292)
(2105, 99.132)
(2106, 98.908)
(2107, 98.794)
(2108, 98.728)
(2109, 98.546)
(2110, 99.372)
(2111, 98.924)
(2112, 98.476)
(2113, 99.414)
(2114, 99.682)
(2115, 99.144)
(2116, 99.394)
(2117, 97.548)
(2118, 99.382)
(2119, 99.354)
(2120, 99.186)
(2121, 99.01)
(2122, 98.842)
(2123, 99.204)
(2124, 98.982)
(2125, 97.926)
(2126, 99.974)
(2127, 99.996)
(2128, 99.998)
(2129, 99.55)
(2130, 99.672)
(2131, 99.918)
(2132, 99.67)
(2133, 99.688)
(2134, 93.444)
(2135, 95.698)
(2136, 99.612)
(2137, 98.634)
(2138, 98.038)
(2139, 98.528)
(2140, 98.202)
(2141, 97.802)
(2142, 99.304)
(2143, 96.406)
(2144, 99.528)
(2145, 99.494)
(2146, 99.886)
(2147, 99.566)
(2148, 97.39)
(2149, 98.134)
(2150, 99.396)
(2151, 99.098)
(2152, 99.238)
(2153, 99.416)
(2154, 99.484)
(2155, 98.638)
(2156, 99.932)
(2157, 99.398)
(2158, 99.258)
(2159, 99.298)
(2160, 99.608)
(2161, 99.842)
(2162, 99.696)
(2163, 99.926)
(2164, 99.54)
(2165, 99.378)
(2166, 99.948)
(2167, 98.644)
(2168, 99.988)
(2169, 99.822)
(2170, 99.996)
(2171, 99.996)
(2172, 99.99)
(2173, 99.984)
(2174, 100)
(2175, 100)
(2176, 99.998)
(2177, 99.85)
(2178, 99.994)
(2179, 99.952)
(2180, 99.978)
(2181, 99.948)
(2182, 99.976)
(2183, 99.996)
(2184, 100)
(2185, 100)
(2186, 99.986)
(2187, 99.374)
(2188, 99.008)
(2189, 99.988)
(2190, 99.998)
(2191, 99.994)
(2192, 81.196)
(2193, 99.394)
(2194, 99.996)
(2195, 99.956)
(2196, 99.982)
(2197, 99.882)
(2198, 99.024)
(2199, 99.926)
(2200, 99.964)
(2201, 99.954)
(2202, 100)
(2203, 99.968)
(2204, 99.998)
(2205, 99.908)
(2206, 99.256)
(2207, 99.942)
(2208, 99.998)
(2209, 99.998)
(2210, 99.742)
(2211, 99.842)
(2212, 99.87)
(2213, 99.942)
(2214, 99.982)
(2215, 99.974)
(2216, 99.976)
(2217, 99.994)
(2218, 99.944)
(2219, 99.902)
(2220, 99.772)
(2221, 99.924)
(2222, 99.076)
(2223, 99.888)
(2224, 99.676)
(2225, 99.91)
(2226, 99.924)
(2227, 99.692)
(2228, 98.36)
(2229, 99.934)
(2230, 99.83)
(2231, 99.986)
(2232, 99.924)
(2233, 99.602)
(2234, 99.76)
(2235, 98.566)
(2236, 99.88)
(2237, 99.538)
(2238, 99.554)
(2239, 99.33)
(2240, 99.88)
(2241, 97.072)
(2242, 99.294)
(2243, 98.724)
(2244, 99.728)
(2245, 97.24)
(2246, 98.854)
(2247, 98.776)
(2248, 99.038)
(2249, 99.64)
(2250, 99.654)
(2251, 99.22)
(2252, 98.974)
(2253, 99.184)
(2254, 98.614)
(2255, 98.264)
(2256, 99.378)
(2257, 99.332)
(2258, 99.25)
(2259, 98.962)
(2260, 99.07)
(2261, 98.838)
(2262, 98.978)
(2263, 98.822)
(2264, 99.424)
(2265, 98.786)
(2266, 95.918)
(2267, 99.276)
(2268, 98.436)
(2269, 98.378)
(2270, 98.714)
(2271, 98.972)
(2272, 97.806)
(2273, 99.132)
(2274, 98.492)
(2275, 97.58)
(2276, 99.322)
(2277, 98.902)
(2278, 99.382)
(2279, 98.662)
(2280, 99.382)
(2281, 96.632)
(2282, 97.374)
(2283, 94.004)
(2284, 99.31)
(2285, 96.878)
(2286, 99.128)
(2287, 99.566)
(2288, 99.108)
(2289, 99.43)
(2290, 99.388)
(2291, 99.784)
(2292, 99.6)
(2293, 99.416)
(2294, 99.078)
(2295, 99.188)
(2296, 99.208)
(2297, 99.224)
(2298, 95.216)
(2299, 99.442)
(2300, 99.654)
(2301, 99.854)
(2302, 99.722)
(2303, 99.58)
(2304, 99.606)
(2305, 99.744)
(2306, 99.83)
(2307, 99.8)
(2308, 99.87)
(2309, 99.728)
(2310, 99.68)
(2311, 99.834)
(2312, 99.862)
(2313, 99.92)
(2314, 99.384)
(2315, 99.19)
(2316, 99.778)
(2317, 99.73)
(2318, 99.48)
(2319, 99.896)
(2320, 99.758)
(2321, 99.874)
(2322, 99.792)
(2323, 99.324)
(2324, 99.594)
(2325, 99.268)
(2326, 99.72)
(2327, 99.886)
(2328, 99.966)
(2329, 99.914)
(2330, 99.506)
(2331, 99.848)
(2332, 99.794)
(2333, 99.212)
(2334, 99.838)
(2335, 99.976)
(2336, 99.964)
(2337, 99.778)
(2338, 99.204)
(2339, 99.894)
(2340, 99.592)
(2341, 99.562)
(2342, 99.006)
(2343, 99.572)
(2344, 98.03)
(2345, 99.57)
(2346, 99.75)
(2347, 97.762)
(2348, 99.888)
(2349, 99.85)
(2350, 99.856)
(2351, 99.684)
(2352, 99.418)
(2353, 99.616)
(2354, 99.89)
(2355, 99.912)
(2356, 99.836)
(2357, 99.934)
(2358, 99.96)
(2359, 99.984)
(2360, 99.99)
(2361, 99.994)
(2362, 99.978)
(2363, 99.93)
(2364, 99.932)
(2365, 99.888)
(2366, 99.936)
(2367, 99.998)
(2368, 99.938)
(2369, 99.99)
(2370, 99.972)
(2371, 99.996)
(2372, 99.932)
(2373, 99.976)
(2374, 99.786)
(2375, 99.91)
(2376, 99.96)
(2377, 99.928)
(2378, 99.984)
(2379, 99.996)
(2380, 99.982)
(2381, 99.854)
(2382, 99.81)
(2383, 99.444)
(2384, 99.96)
(2385, 99.972)
(2386, 99.204)
(2387, 99.826)
(2388, 99.99)
(2389, 99.99)
(2390, 99.964)
(2391, 99.996)
(2392, 100)
(2393, 100)
(2394, 100)
(2395, 100)
(2396, 100)
(2397, 100)
(2398, 99.998)
(2399, 99.992)
(2400, 99.85)
(2401, 99.99)
(2402, 99.988)
(2403, 99.972)
(2404, 99.968)
(2405, 99.942)
(2406, 99.956)
(2407, 99.408)
(2408, 99.858)
(2409, 99.682)
(2410, 99.712)
(2411, 99.692)
(2412, 99.402)
(2413, 99.784)
(2414, 99.992)
(2415, 99.986)
(2416, 99.996)
(2417, 99.978)
(2418, 99.98)
(2419, 100)
(2420, 100)
(2421, 100)
(2422, 100)
(2423, 100)
(2424, 100)
(2425, 99.958)
(2426, 99.996)
(2427, 100)
(2428, 99.992)
(2429, 100)
(2430, 100)
(2431, 100)
(2432, 100)
(2433, 100)
(2434, 100)
(2435, 99.998)
(2436, 100)
(2437, 100)
(2438, 100)
(2439, 100)
(2440, 100)
(2441, 99.988)
(2442, 99.004)
(2443, 99.974)
(2444, 100)
(2445, 100)
(2446, 99.996)
(2447, 100)
(2448, 99.994)
(2449, 99.992)
(2450, 100)
(2451, 99.996)
(2452, 100)
(2453, 99.998)
(2454, 99.084)
(2455, 99.992)
(2456, 99.984)
(2457, 100)
(2458, 99.994)
(2459, 99.998)
(2460, 99.986)
(2461, 99.984)
(2462, 99.966)
(2463, 99.654)
(2464, 99.962)
(2465, 99.976)
(2466, 99.916)
(2467, 99.966)
(2468, 99.988)
(2469, 99.936)
(2470, 99.988)
(2471, 99.984)
(2472, 99.966)
(2473, 99.856)
(2474, 99.636)
(2475, 99.838)
(2476, 99.818)
(2477, 98.008)
(2478, 99.768)
(2479, 99.864)
(2480, 99.874)
(2481, 99.852)
(2482, 99.962)
(2483, 99.84)
(2484, 99.878)
(2485, 99.92)
(2486, 99.968)
(2487, 99.944)
(2488, 99.73)
(2489, 99.932)
(2490, 99.85)
(2491, 99.808)
(2492, 99.972)
(2493, 99.994)
(2494, 99.974)
(2495, 99.884)
(2496, 99.666)
(2497, 99.7)
(2498, 99.708)
(2499, 98.92)
(2500, 99.824)
(2501, 99.72)
(2502, 99.682)
(2503, 99.73)
(2504, 99.8)
(2505, 99.91)
(2506, 99.51)
(2507, 99.294)
(2508, 99.192)
(2509, 99.762)
(2510, 99.888)
(2511, 99.92)
(2512, 99.604)
(2513, 99.67)
(2514, 99.632)
(2515, 99.534)
(2516, 96.164)
(2517, 93.328)
(2518, 96.95)
(2519, 96.952)
(2520, 96.376)
(2521, 96.074)
(2522, 96.968)
(2523, 90.034)
(2524, 90.08)
(2525, 90.65)
(2526, 87.562)
(2527, 88.68)
(2528, 94.052)
(2529, 79.728)
(2530, 90.078)
(2531, 79.326)
(2532, 90.602)
(2533, 89.636)
(2534, 93.514)
(2535, 91.58)
(2536, 70.15)
(2537, 73.69)
(2538, 83.734)
(2539, 87.51)
(2540, 93.248)
(2541, 84.49)
(2542, 94.706)
(2543, 91.638)
(2544, 91.484)
(2545, 95.424)
(2546, 93.646)
(2547, 92.29)
(2548, 91.958)
(2549, 94.552)
(2550, 90.78)
(2551, 76.714)
(2552, 73.908)
(2553, 94.04)
(2554, 93.452)
(2555, 90.528)
(2556, 87.706)
(2557, 95.116)
(2558, 92.052)
(2559, 88.676)
(2560, 89.724)
(2561, 61.072)
(2562, 89.854)
(2563, 84.148)
(2564, 90.224)
(2565, 85.036)
(2566, 90.756)
(2567, 89.726)
(2568, 91.466)
(2569, 88.618)
(2570, 91.73)
(2571, 87.144)
(2572, 91.088)
(2573, 97.25)
(2574, 97.962)
(2575, 97.256)
(2576, 97.666)
(2577, 97.256)
(2578, 96.892)
(2579, 97.202)
(2580, 98.16)
(2581, 97.814)
(2582, 97.736)
(2583, 97.862)
(2584, 98.846)
(2585, 98.91)
(2586, 98.364)
(2587, 95.09)
(2588, 92.81)
(2589, 97.138)
(2590, 97.988)
(2591, 97.488)
(2592, 96.586)
(2593, 97.46)
(2594, 97.872)
(2595, 98.766)
(2596, 98.062)
(2597, 93.804)
(2598, 98.22)
(2599, 98.902)
(2600, 98.31)
(2601, 98.52)
(2602, 98.042)
(2603, 98.496)
(2604, 96.612)
(2605, 98.068)
(2606, 98.256)
(2607, 97.356)
(2608, 98.686)
(2609, 98.496)
(2610, 98.236)
(2611, 97.984)
(2612, 97.968)
(2613, 98.544)
(2614, 99.114)
(2615, 99.158)
(2616, 99.25)
(2617, 98.352)
(2618, 93.138)
(2619, 97.582)
(2620, 96.966)
(2621, 98.466)
(2622, 98.258)
(2623, 99.11)
(2624, 97.118)
(2625, 99.174)
(2626, 99.014)
(2627, 97.122)
(2628, 97.42)
(2629, 97.218)
(2630, 96.952)
(2631, 96.028)
(2632, 96.976)
(2633, 96.404)
(2634, 96.306)
(2635, 94.266)
(2636, 86.668)
(2637, 87.208)
(2638, 94.724)
(2639, 91.908)
(2640, 93.512)
(2641, 96.89)
(2642, 95.664)
(2643, 95.034)
(2644, 97.616)
(2645, 96.84)
(2646, 97.994)
(2647, 96.97)
(2648, 97.218)
(2649, 96.13)
(2650, 96.248)
(2651, 96.888)
(2652, 94.766)
(2653, 96.13)
(2654, 96.686)
(2655, 95.844)
(2656, 97.008)
(2657, 98.056)
(2658, 96.992)
(2659, 97.018)
(2660, 97.812)
(2661, 97.404)
(2662, 97.324)
(2663, 98.122)
(2664, 97.754)
(2665, 97.784)
(2666, 97.95)
(2667, 96.408)
(2668, 94.66)
(2669, 96.172)
(2670, 94.41)
(2671, 97.044)
(2672, 96.698)
(2673, 97.528)
(2674, 98.08)
(2675, 96.588)
(2676, 97.396)
(2677, 95.55)
(2678, 96.76)
(2679, 98.222)
(2680, 97.052)
(2681, 96.536)
(2682, 98.328)
(2683, 98.784)
(2684, 98.008)
(2685, 97.974)
(2686, 97.84)
(2687, 98.642)
(2688, 97.088)
(2689, 95.63)
(2690, 95.298)
(2691, 95.042)
(2692, 96.55)
(2693, 96.006)
(2694, 97.546)
(2695, 95.602)
(2696, 96.456)
(2697, 98.076)
(2698, 93.712)
(2699, 96.058)
(2700, 96.082)
(2701, 95.794)
(2702, 95.76)
(2703, 94.18)
(2704, 88.476)
(2705, 94.93)
(2706, 95.712)
(2707, 91.76)
(2708, 87.164)
(2709, 93.99)
(2710, 96.074)
(2711, 93.382)
(2712, 89.708)
(2713, 86.488)
(2714, 89.656)
(2715, 83.396)
(2716, 71.316)
(2717, 78.83)
(2718, 83.866)
(2719, 90.046)
(2720, 92.166)
(2721, 83.848)
(2722, 68.816)
(2723, 72.95)
(2724, 84.976)
(2725, 82.168)
(2726, 53.686)
(2727, 76.006)
(2728, 72.674)
(2729, 87.604)
(2730, 89.812)
(2731, 89.47)
(2732, 90.7)
(2733, 94.028)
(2734, 89.726)
(2735, 92.43)
(2736, 94.818)
(2737, 95.122)
(2738, 93.016)
(2739, 95.938)
(2740, 94.03)
(2741, 92.61)
(2742, 77.184)
(2743, 92.676)
(2744, 89.084)
(2745, 89.59)
(2746, 76.396)
(2747, 82.166)
(2748, 83.584)
(2749, 76.4)
(2750, 85.476)
(2751, 90.744)
(2752, 91.926)
(2753, 87.956)
(2754, 83.416)
(2755, 93.714)
(2756, 93.94)
(2757, 89.62)
(2758, 88.944)
(2759, 96.558)
(2760, 93.754)
(2761, 91.572)
(2762, 96.732)
(2763, 95.884)
(2764, 94.692)
(2765, 72.846)
(2766, 93.286)
(2767, 90.06)
(2768, 92.842)
(2769, 96.552)
(2770, 95.156)
(2771, 95.24)
(2772, 96.156)
(2773, 97.072)
(2774, 96.412)
(2775, 96.93)
(2776, 95.926)
(2777, 98.09)
(2778, 95.38)
(2779, 97.358)
(2780, 97.48)
(2781, 98.048)
(2782, 96.954)
(2783, 97.236)
(2784, 97.848)
(2785, 97.97)
(2786, 97.33)
(2787, 98.266)
(2788, 99.608)
(2789, 98.798)
(2790, 98.532)
(2791, 97.122)
(2792, 95.706)
(2793, 95.73)
(2794, 94.946)
(2795, 96.186)
(2796, 96.34)
(2797, 97.144)
(2798, 94.084)
(2799, 96.1)
(2800, 93.156)
(2801, 92.612)
(2802, 95.014)
(2803, 92.736)
(2804, 95.432)
(2805, 96.598)
(2806, 95.73)
(2807, 97.372)
(2808, 93.13)
(2809, 95.51)
(2810, 96.42)
(2811, 97.884)
(2812, 94.29)
(2813, 96.61)
(2814, 96.534)
(2815, 93.998)
(2816, 96.912)
(2817, 94.698)
(2818, 96.916)
(2819, 97.536)
(2820, 94.406)
(2821, 96.12)
(2822, 95.154)
(2823, 94.006)
(2824, 91.5)
(2825, 89.684)
(2826, 69.57)
(2827, 65.052)
(2828, 54.516)
(2829, 70.054)
(2830, 89.394)
(2831, 67.822)
(2832, 76.038)
(2833, 58.514)
(2834, 62.494)
(2835, 44.066)
(2836, 67.092)
(2837, 59.724)
(2838, 46.69)
(2839, 49.792)
(2840, 24.06)
(2841, 66.11)
(2842, 55.49)
(2843, 67.092)
(2844, 71.918)
(2845, 84.58)
(2846, 71.182)
(2847, 64.73)
(2848, 84.718)
(2849, 74.926)
(2850, 61.778)
(2851, 77.512)
(2852, 82.722)
(2853, 82.75)
(2854, 53.174)
(2855, 12.552)
(2856, 25.974)
(2857, 81.514)
(2858, 83.624)
(2859, 73.99)
(2860, 83.648)
(2861, 87.542)
(2862, 82.76)
(2863, 88.892)
(2864, 88.954)
(2865, 90.326)
(2866, 92.944)
(2867, 90.188)
(2868, 84.398)
(2869, 89.262)
(2870, 74.974)
(2871, 67.312)
(2872, 58.102)
(2873, 47.08)
(2874, 78.968)
(2875, 51.702)
(2876, 53.872)
(2877, 49.54)
(2878, 43.064)
(2879, 64.552)
(2880, 59.386)
(2881, 56.718)
(2882, 38.248)
(2883, 27.738)
(2884, 65.582)
(2885, 24.648)
(2886, 60.24)
(2887, 73.53)
(2888, 67.8)
(2889, 53.264)
(2890, 40.85)
(2891, 37.494)
(2892, 27.712)
(2893, 37.136)
(2894, 52.448)
(2895, 41.994)
(2896, 34.954)
(2897, 57.614)
(2898, 59.468)
(2899, 41.242)
(2900, 11.87)
(2901, 47.134)
(2902, 19.354)
(2903, 16.648)
(2904, 4.11)
(2905, 12.87)
(2906, 19.774)
(2907, 9.702)
(2908, 13.71)
(2909, 6.916)
(2910, 16.946)
(2911, 4.556)
(2912, 11.078)
(2913, 16.76)
(2914, 26.706)
(2915, 3.306)
(2916, 0)
(2917, 8.19)
(2918, 25.444)
(2919, 34.28)
(2920, 19.154)
(2921, 8.436)
(2922, 54.41)
(2923, 45.372)
(2924, 27.69)
(2925, 52.108)
(2926, 79.632)
(2927, 74.608)
(2928, 59.96)
(2929, 43.14)
(2930, 79.694)
(2931, 92.19)
(2932, 99.778)
(2933, 92.726)
(2934, 95.576)
(2935, 96.22)
(2936, 68.64)
(2937, 90.498)
(2938, 92.576)
(2939, 89.68)
(2940, 92.54)
(2941, 87.124)
(2942, 87.904)
(2943, 86.016)
(2944, 95.386)
(2945, 92.124)
(2946, 93.964)
(2947, 96.782)
(2948, 97.648)
(2949, 97.522)
(2950, 95.656)
(2951, 97.794)
(2952, 95.718)
(2953, 97.178)
(2954, 96.616)
(2955, 95.366)
(2956, 93.46)
(2957, 95.438)
(2958, 95.394)
(2959, 89.164)
(2960, 94.196)
(2961, 95.684)
(2962, 95.436)
(2963, 91.876)
(2964, 94.646)
(2965, 95.464)
(2966, 92.582)
(2967, 91.318)
(2968, 94.768)
(2969, 95.362)
(2970, 93.966)
(2971, 96.732)
(2972, 96.82)
(2973, 96.61)
(2974, 95.026)
(2975, 96.75)
(2976, 97.118)
(2977, 98.322)
(2978, 96.638)
(2979, 97.684)
(2980, 97.774)
(2981, 97.332)
(2982, 94.756)
(2983, 95.208)
(2984, 97.486)
(2985, 97.892)
(2986, 97.71)
(2987, 97.482)
(2988, 96.812)
(2989, 97.152)
(2990, 96.702)
(2991, 96.726)
(2992, 95.422)
(2993, 98.446)
(2994, 97.866)
(2995, 98.054)
(2996, 97.582)
(2997, 96.26)
(2998, 95.254)
(2999, 98)
(3000, 98.504)
(3001, 97.968)
(3002, 98.27)
(3003, 98.818)
(3004, 97.362)
(3005, 95.04)
(3006, 95.874)
(3007, 96.03)
(3008, 98.336)
(3009, 97.156)
(3010, 98.048)
(3011, 97.1)
(3012, 96.142)
(3013, 98.558)
(3014, 98.624)
(3015, 98.878)
(3016, 97.202)
(3017, 96.806)
(3018, 97.472)
(3019, 96.438)
(3020, 97.654)
(3021, 97.342)
(3022, 98.092)
(3023, 96.676)
(3024, 97.378)
(3025, 96.444)
(3026, 97.424)
(3027, 98.002)
(3028, 97.478)
(3029, 98.34)
(3030, 98.816)
(3031, 97.684)
(3032, 98.162)
(3033, 97.44)
(3034, 97.31)
(3035, 97.132)
(3036, 91.014)
(3037, 99.432)
(3038, 98.56)
(3039, 97.544)
(3040, 96.986)
(3041, 94.706)
(3042, 98.636)
(3043, 96.932)
(3044, 98.204)
(3045, 97.584)
(3046, 96.094)
(3047, 96.174)
(3048, 97.94)
(3049, 98.358)
(3050, 98.92)
(3051, 96.868)
(3052, 80.256)
(3053, 87.166)
(3054, 92.324)
(3055, 98.638)
(3056, 99.21)
(3057, 99.402)
(3058, 99.574)
(3059, 89.612)
(3060, 86.548)
(3061, 94.394)
(3062, 99.34)
(3063, 99.448)
(3064, 98.702)
(3065, 99.092)
(3066, 99.368)
(3067, 99.07)
(3068, 98.902)
(3069, 99.028)
(3070, 96.078)
(3071, 97.71)
(3072, 97.924)
(3073, 91.576)
(3074, 96.664)
(3075, 96.83)
(3076, 97.04)
(3077, 95.5)
(3078, 96.754)
(3079, 91.136)
(3080, 90.252)
(3081, 97.27)
(3082, 97.212)
(3083, 99.002)
(3084, 99.21)
(3085, 99.314)
(3086, 99.554)
(3087, 99.042)
(3088, 98.064)
(3089, 99.064)
(3090, 97.648)
(3091, 98.02)
(3092, 97.932)
(3093, 97.386)
(3094, 97.664)
(3095, 96.058)
(3096, 98.454)
(3097, 94.984)
(3098, 98.036)
(3099, 98.824)
(3100, 99.122)
(3101, 98.532)
(3102, 95.674)
(3103, 97.262)
(3104, 93.348)
(3105, 96.108)
(3106, 91.836)
(3107, 97.954)
(3108, 98.382)
(3109, 94.248)
(3110, 93.824)
(3111, 93)
(3112, 92.696)
(3113, 94.158)
(3114, 82.09)
(3115, 66.544)
(3116, 0)
(3117, 0)
(3118, 0)
(3119, 7.444)
(3120, 5.242)
(3121, 0)
(3122, 0)
(3123, 2.002)
(3124, 1.274)
(3125, 18.062)
(3126, 5.852)
(3127, 0)
(3128, 0)
(3129, 0.006)
(3130, 8.808)
(3131, 0)
(3132, 0)
(3133, 5.112)
(3134, 0)
(3135, 5.172)
(3136, 0)
(3137, 49.852)
(3138, 74.304)
(3139, 58.074)
(3140, 6.244)
(3141, 71.59)
(3142, 70.348)
(3143, 80.272)
(3144, 91.44)
(3145, 89.26)
(3146, 88.85)
(3147, 92.482)
(3148, 87.862)
(3149, 89.322)
(3150, 92.564)
(3151, 93.062)
(3152, 94.002)
(3153, 96.53)
(3154, 94.786)
(3155, 96.306)
(3156, 97.312)
(3157, 95.898)
(3158, 95.972)
(3159, 90.734)
(3160, 96.466)
(3161, 97.464)
(3162, 97.428)
(3163, 98.244)
(3164, 97.92)
(3165, 96.118)
(3166, 95.91)
(3167, 97.288)
(3168, 97.358)
(3169, 97.916)
(3170, 97.214)
(3171, 97.998)
(3172, 98.404)
(3173, 98.248)
(3174, 98.162)
(3175, 98.556)
(3176, 98.038)
(3177, 98.472)
(3178, 90.584)
(3179, 97.706)
(3180, 96.854)
(3181, 97.648)
(3182, 93.994)
(3183, 92.254)
(3184, 87.868)
(3185, 88.07)
(3186, 89.08)
(3187, 94.95)
(3188, 94.852)
(3189, 94.884)
(3190, 93.512)
(3191, 86.7)
(3192, 93.064)
(3193, 86.906)
(3194, 85.752)
(3195, 84.65)
(3196, 82.66)
(3197, 63.338)
(3198, 91.86)
(3199, 79.374)
(3200, 62.234)
(3201, 74.874)
(3202, 34.016)
(3203, 12.532)
(3204, 28.444)
(3205, 51.412)
(3206, 63.38)
(3207, 59.156)
(3208, 80.126)
(3209, 74.504)
(3210, 87.054)
(3211, 80.436)
(3212, 90.93)
(3213, 88.272)
(3214, 87.596)
(3215, 82.74)
(3216, 84.762)
(3217, 90.768)
(3218, 82.644)
(3219, 83.102)
(3220, 62.976)
(3221, 73.514)
(3222, 78.46)
(3223, 57.618)
(3224, 61.944)
(3225, 77.256)
(3226, 77.796)
(3227, 73.452)
(3228, 89.532)
(3229, 73.866)
(3230, 69.348)
(3231, 75.93)
(3232, 59.624)
(3233, 66.834)
(3234, 67.2)
(3235, 43.526)
(3236, 71.782)
(3237, 29.036)
(3238, 56.974)
(3239, 46.008)
(3240, 34.828)
(3241, 42.622)
(3242, 48.912)
(3243, 70.99)
(3244, 56.05)
(3245, 62.278)
(3246, 27.51)
(3247, 54.298)
(3248, 33.042)
(3249, 5.106)
(3250, 23.79)
(3251, 13.522)
(3252, 35.056)
(3253, 47.468)
(3254, 19.988)
(3255, 25.862)
(3256, 13.702)
(3257, 5.402)
(3258, 14.222)
(3259, 84.114)
(3260, 84.982)
(3261, 54.608)
(3262, 81.174)
(3263, 62.288)
(3264, 76.27)
(3265, 81.214)
(3266, 49.602)
(3267, 66.5)
(3268, 53.708)
(3269, 58.932)
(3270, 88.878)
(3271, 81.586)
(3272, 87.398)
(3273, 82.87)
(3274, 81.364)
(3275, 99.996)
(3276, 99.98)
(3277, 100)
(3278, 100)
(3279, 100)
(3280, 86.306)
(3281, 69.684)
(3282, 63.73)
(3283, 77.05)
(3284, 37.696)
(3285, 67.752)
(3286, 82.592)
(3287, 91.18)
(3288, 83.182)
(3289, 78.638)
(3290, 72.214)
(3291, 66.714)
(3292, 90.624)
(3293, 84.556)
(3294, 66.746)
(3295, 72.348)
(3296, 67.426)
(3297, 84.988)
(3298, 92.114)
(3299, 93.002)
(3300, 90.826)
(3301, 91.846)
(3302, 85.684)
(3303, 90.378)
(3304, 87.42)
(3305, 91.828)
(3306, 91.056)
(3307, 91.926)
(3308, 93.82)
(3309, 94.662)
(3310, 94.942)
(3311, 88.496)
(3312, 80.658)
(3313, 81.258)
(3314, 85.232)
(3315, 89.45)
(3316, 79.648)
(3317, 87.51)
(3318, 71.34)
(3319, 79.888)
(3320, 93.86)
(3321, 87.862)
(3322, 71.96)
(3323, 88.454)
(3324, 92.484)
(3325, 87.316)
(3326, 93.192)
(3327, 83.132)
(3328, 92.22)
(3329, 89.674)
(3330, 95.096)
(3331, 88.714)
(3332, 86.25)
(3333, 89.422)
(3334, 80.232)
(3335, 86.424)
(3336, 93.602)
(3337, 90.716)
(3338, 89.654)
(3339, 90.336)
(3340, 88.814)
(3341, 82.62)
(3342, 85)
(3343, 95.896)
(3344, 92.572)
(3345, 88.674)
(3346, 95.058)
(3347, 83.856)
(3348, 93.004)
(3349, 89.926)
(3350, 88.008)
(3351, 93.926)
(3352, 94.94)
(3353, 92.866)
(3354, 85.674)
(3355, 85.78)
(3356, 91.692)
(3357, 93.19)
(3358, 90.348)
(3359, 92.014)
(3360, 94.98)
(3361, 95.282)
(3362, 92.394)
(3363, 91.04)
(3364, 91.314)
(3365, 82.458)
(3366, 92.618)
(3367, 91.754)
(3368, 89.876)
(3369, 85.472)
(3370, 91.964)
(3371, 92.218)
(3372, 91.476)
(3373, 92.166)
(3374, 91.822)
(3375, 93.194)
(3376, 92.84)
(3377, 92.502)
(3378, 93.92)
(3379, 86.024)
(3380, 91.962)
(3381, 90.77)
(3382, 88.592)
(3383, 82.41)
(3384, 55.5)
(3385, 85.898)
(3386, 83.494)
(3387, 86.72)
(3388, 73.922)
(3389, 86.21)
(3390, 86.198)
(3391, 88.418)
(3392, 88.852)
(3393, 80.41)
(3394, 84.794)
(3395, 70.89)
(3396, 50.596)
(3397, 86.698)
(3398, 87.17)
(3399, 65.422)
(3400, 81.48)
(3401, 79.166)
(3402, 79.908)
(3403, 60.628)
(3404, 92.11)
(3405, 94.254)
(3406, 88.218)
(3407, 78.742)
(3408, 72.396)
(3409, 77.77)
(3410, 76.432)
(3411, 78.63)
(3412, 68.052)
(3413, 30.02)
(3414, 76.524)
(3415, 88.798)
(3416, 78.022)
(3417, 88.868)
(3418, 90.226)
(3419, 92.124)
(3420, 95.89)
(3421, 93.978)
(3422, 86.488)
(3423, 90.92)
(3424, 88.642)
(3425, 92.728)
(3426, 84.172)
(3427, 89.76)
(3428, 90.562)
(3429, 90.232)
(3430, 85.832)
(3431, 81.244)
(3432, 92.654)
(3433, 83.366)
(3434, 84.878)
(3435, 94.69)
(3436, 87.74)
(3437, 93.56)
(3438, 92.834)
(3439, 86.3)
(3440, 88.886)
(3441, 87.864)
(3442, 90.128)
(3443, 75.728)
(3444, 75.564)
(3445, 79.834)
(3446, 81.088)
(3447, 81.366)
(3448, 91.542)
(3449, 66.22)
(3450, 79.328)
(3451, 87.508)
(3452, 88.728)
(3453, 70.908)
(3454, 47.862)
(3455, 42.972)
(3456, 83.56)
(3457, 68.154)
(3458, 81.376)
(3459, 89.17)
(3460, 86.078)
(3461, 83.986)
(3462, 91.124)
(3463, 87.688)
(3464, 96.678)
(3465, 93.5)
(3466, 95.882)
(3467, 94.654)
(3468, 94.656)
(3469, 84.45)
(3470, 91.996)
(3471, 95.386)
(3472, 89.572)
(3473, 84.492)
(3474, 92.72)
(3475, 90.496)
(3476, 90.144)
(3477, 92.516)
(3478, 94.308)
(3479, 94.156)
(3480, 95.672)
(3481, 95.056)
(3482, 95.734)
(3483, 89.386)
(3484, 90.746)
(3485, 87.958)
(3486, 92.322)
(3487, 87.874)
(3488, 89.75)
(3489, 87.92)
(3490, 83.466)
(3491, 87.288)
(3492, 87.912)
(3493, 77.168)
(3494, 74.014)
(3495, 78.17)
(3496, 58.702)
(3497, 52.342)
(3498, 33.762)
(3499, 45.948)
(3500, 58.726)
(3501, 30.152)
(3502, 21.298)
(3503, 16.656)
(3504, 11.882)
(3505, 36.486)
(3506, 4.748)
(3507, 0)
(3508, 0)
(3509, 0)
(3510, 0)
(3511, 0)
(3512, 0)
(3513, 2.806)
(3514, 2.45)
(3515, 0)
(3516, 0)
(3517, 0)
(3518, 0)
(3519, 0)
(3520, 0)
(3521, 0)
(3522, 0)
(3523, 0)
(3524, 0)
(3525, 4.16)
(3526, 2.84)
(3527, 0.24)
(3528, 0)
(3529, 0)
(3530, 0)
(3531, 0)
(3532, 0)
(3533, 0)
(3534, 0)
(3535, 0)
(3536, 0)
(3537, 0)
(3538, 0)
(3539, 0)
(3540, 0)
(3541, 0)
(3542, 0)
(3543, 0)
(3544, 0)
(3545, 0)
(3546, 0)
(3547, 0)
(3548, 0)
(3549, 0)
(3550, 5.112)
(3551, 0)
(3552, 0)
(3553, 0)
(3554, 0)
(3555, 0)
(3556, 0)
(3557, 0)
(3558, 0)
(3559, 0)
(3560, 0)
(3561, 4.16)
(3562, 0)
(3563, 0)
(3564, 0)
(3565, 0)
(3566, 0)
(3567, 0)
(3568, 0)
(3569, 0)
(3570, 0)
(3571, 6.03)
(3572, 1.98)
(3573, 0)
(3574, 0)
(3575, 4.97)
(3576, 0)
(3577, 0)
(3578, 0)
(3579, 0)
(3580, 0)
(3581, 0)
(3582, 0)
(3583, 8.736)
(3584, 0)
(3585, 0)
(3586, 0)
(3587, 0)
(3588, 0)
(3589, 6.8)
(3590, 4.106)
(3591, 0.87)
(3592, 0)
(3593, 0)
(3594, 0)
(3595, 7.656)
(3596, 0)
(3597, 0)
(3598, 0)
(3599, 0)
(3600, 0)
(3601, 8.742)
(3602, 0)
(3603, 0)
(3604, 0)
(3605, 0)
(3606, 0)
(3607, 0)
(3608, 4.826)
(3609, 9.29)
(3610, 0)
(3611, 0)
(3612, 0)
(3613, 0)
(3614, 0)
(3615, 0)
(3616, 0)
(3617, 9.312)
(3618, 0)
(3619, 0)
(3620, 0)
(3621, 0)
(3622, 0)
(3623, 3.192)
(3624, 0)
(3625, 0)
(3626, 0)
(3627, 0)
(3628, 0)
(3629, 0)
(3630, 1.56)
(3631, 0)
(3632, 0)
(3633, 0)
(3634, 0)
(3635, 0)
(3636, 0)
(3637, 9.702)
(3638, 0)
(3639, 0)
(3640, 0)
(3641, 0)
(3642, 0)
(3643, 0)
(3644, 0)
(3645, 0)
(3646, 0)
(3647, 0)
(3648, 0)
(3649, 0)
(3650, 0)
(3651, 0)
(3652, 0)
(3653, 0)
(3654, 0)
(3655, 0)
(3656, 0)
(3657, 0)
(3658, 0)
(3659, 0)
(3660, 0)
(3661, 0)
(3662, 0)
(3663, 4.556)
(3664, 0)
(3665, 0)
(3666, 0)
(3667, 0)
(3668, 0)
(3669, 0)
(3670, 0)
(3671, 0)
(3672, 0)
(3673, 0)
(3674, 0)
(3675, 0)
(3676, 0)
(3677, 0)
(3678, 0)
(3679, 3.306)
(3680, 0)
(3681, 1.19)
(3682, 2.97)
(3683, 0)
(3684, 8.372)
(3685, 0)
(3686, 5.7)
(3687, 0)
(3688, 0)
(3689, 0)
(3690, 0)
(3691, 8.556)
(3692, 0)
(3693, 0)
(3694, 0)
(3695, 4.97)
(3696, 0)
(3697, 0)
(3698, 0)
(3699, 0)
(3700, 0)
(3701, 5.148)
(3702, 9.342)
(3703, 38.056)
(3704, 0.38)
(3705, 6.48)
(3706, 0)
(3707, 3.422)
(3708, 0)
(3709, 0)
(3710, 0)
(3711, 0)
(3712, 0)
(3713, 0)
(3714, 0)
(3715, 0)
(3716, 0)
(3717, 0)
(3718, 1.032)
(3719, 10.302)
(3720, 13.662)
(3721, 0)
(3722, 0)
(3723, 0)
(3724, 0)
(3725, 4.102)
(3726, 18.338)
(3727, 43.242)
(3728, 22.746)
(3729, 21.248)
(3730, 37.406)
(3731, 32.796)
(3732, 33.228)
(3733, 64.588)
(3734, 21.492)
(3735, 24.886)
(3736, 30.558)
(3737, 64.856)
(3738, 77.084)
(3739, 77.988)
(3740, 51.834)
(3741, 29.446)
(3742, 57.04)
(3743, 33.194)
(3744, 60.526)
(3745, 29.642)
(3746, 37.132)
(3747, 43.42)
(3748, 18.402)
(3749, 37.07)
(3750, 8.982)
(3751, 40.762)
(3752, 60.196)
(3753, 56.622)
(3754, 56.922)
(3755, 66.916)
(3756, 64.922)
(3757, 57.566)
(3758, 63.042)
(3759, 41.12)
(3760, 53.292)
(3761, 64.454)
(3762, 88.744)
(3763, 61.682)
(3764, 68.956)
(3765, 84.132)
(3766, 73.734)
(3767, 90.584)
(3768, 81.686)
(3769, 83.916)
(3770, 85.552)
(3771, 86.296)
(3772, 80.474)
(3773, 85.88)
(3774, 81.482)
(3775, 83.426)
(3776, 57.276)
(3777, 52.926)
(3778, 62.104)
(3779, 66.722)
(3780, 83.134)
(3781, 77.202)
(3782, 77.718)
(3783, 89.79)
(3784, 93.932)
(3785, 93.672)
(3786, 90.874)
(3787, 92.408)
(3788, 89.032)
(3789, 92.902)
(3790, 92.142)
(3791, 88.468)
(3792, 93.924)
(3793, 93.54)
(3794, 95.604)
(3795, 91.856)
(3796, 91.358)
(3797, 92.606)
(3798, 93.956)
(3799, 97.302)
(3800, 95.48)
(3801, 96.498)
(3802, 98.126)
(3803, 97.852)
(3804, 94.628)
(3805, 97.67)
(3806, 98.696)
(3807, 96.58)
(3808, 97.186)
(3809, 96.722)
(3810, 98.65)
(3811, 99.402)
(3812, 99.454)
(3813, 99.392)
(3814, 99.328)
(3815, 98.916)
(3816, 98.39)
(3817, 97.132)
(3818, 95.02)
(3819, 96.516)
(3820, 96.554)
(3821, 98.49)
(3822, 96.042)
(3823, 95.024)
(3824, 97.544)
(3825, 97.048)
(3826, 95.282)
(3827, 96.548)
(3828, 97.52)
(3829, 95.67)
(3830, 96.632)
(3831, 95.302)
(3832, 95.652)
(3833, 94.73)
(3834, 94.014)
(3835, 96.648)
(3836, 97.08)
(3837, 96.97)
(3838, 96.708)
(3839, 95.564)
(3840, 98.276)
(3841, 98.414)
(3842, 98.692)
(3843, 98.288)
(3844, 97.258)
(3845, 98.148)
(3846, 98.348)
(3847, 98.526)
(3848, 97.7)
(3849, 97.862)
(3850, 98.766)
(3851, 97.728)
(3852, 98.088)
(3853, 98.756)
(3854, 98.144)
(3855, 98.31)
(3856, 98.58)
(3857, 98.142)
(3858, 98.266)
(3859, 97.93)
(3860, 97.302)
(3861, 97.662)
(3862, 98.138)
(3863, 96.536)
(3864, 97.578)
(3865, 98.636)
(3866, 98.934)
(3867, 98.74)
(3868, 98.792)
(3869, 98.866)
(3870, 98.306)
(3871, 98.672)
(3872, 98.04)
(3873, 98.062)
(3874, 98.612)
(3875, 98.182)
(3876, 97.834)
(3877, 99.094)
(3878, 98.246)
(3879, 99.394)
(3880, 99.06)
(3881, 99.37)
(3882, 99.362)
(3883, 98.608)
(3884, 98.69)
(3885, 99.084)
(3886, 98.188)
(3887, 99.076)
(3888, 99.85)
(3889, 98.816)
(3890, 97.99)
(3891, 98.812)
(3892, 98.058)
(3893, 98.582)
(3894, 98.044)
(3895, 98.96)
(3896, 98.634)
(3897, 98.764)
(3898, 98.728)
(3899, 97.81)
(3900, 99.478)
(3901, 99.474)
(3902, 99.52)
(3903, 98.416)
(3904, 99.258)
(3905, 99.432)
(3906, 99.692)
(3907, 97.838)
(3908, 99.538)
(3909, 98.712)
(3910, 97.688)
(3911, 99.548)
(3912, 98.876)
(3913, 97.254)
(3914, 98.99)
(3915, 99.304)
(3916, 98.706)
(3917, 99.214)
(3918, 99.284)
(3919, 99.52)
(3920, 99.936)
(3921, 99.204)
(3922, 98.684)
(3923, 99.164)
(3924, 98.47)
(3925, 98.812)
(3926, 98.62)
(3927, 99.08)
(3928, 99.328)
(3929, 98.7)
(3930, 99.058)
(3931, 97.93)
(3932, 98.952)
(3933, 97.634)
(3934, 98.718)
(3935, 96.29)
(3936, 97.496)
(3937, 98.91)
(3938, 95.726)
(3939, 96.924)
(3940, 99.406)
(3941, 99.102)
(3942, 98.828)
(3943, 97.034)
(3944, 98.608)
(3945, 97.396)
(3946, 98.844)
(3947, 97.838)
(3948, 98.754)
(3949, 97.922)
(3950, 98.118)
(3951, 99.254)
(3952, 99.612)
(3953, 98.798)
(3954, 99.226)
(3955, 99.73)
(3956, 99.4)
(3957, 99.426)
(3958, 98.11)
(3959, 98.202)
(3960, 99.332)
(3961, 99.406)
(3962, 99.378)
(3963, 99.354)
(3964, 98.8)
(3965, 99.39)
(3966, 99.13)
(3967, 96.944)
(3968, 99.38)
(3969, 99.874)
(3970, 99.744)
(3971, 99.648)
(3972, 99.606)
(3973, 99.792)
(3974, 99.464)
(3975, 99.318)
(3976, 99.394)
(3977, 99.458)
(3978, 99.084)
(3979, 99.582)
(3980, 99.074)
(3981, 98.82)
(3982, 99.032)
(3983, 98.112)
(3984, 99.528)
(3985, 99.72)
(3986, 99.232)
(3987, 99.688)
(3988, 99.428)
(3989, 99.396)
(3990, 97.962)
(3991, 99.056)
(3992, 96.202)
(3993, 99.066)
(3994, 99.278)
(3995, 98.998)
(3996, 99.636)
(3997, 99.538)
(3998, 99.288)
(3999, 98.788)
(4000, 99.696)
(4001, 99.778)
(4002, 99.63)
(4003, 99.678)
(4004, 99.15)
(4005, 99.388)
(4006, 99.49)
(4007, 99.676)
(4008, 99.462)
(4009, 99.856)
(4010, 99.476)
(4011, 98.728)
(4012, 99.672)
(4013, 98.218)
(4014, 99.578)
(4015, 99.864)
(4016, 99.576)
(4017, 99.954)
(4018, 99.976)
(4019, 99.994)
(4020, 99.984)
(4021, 99.716)
(4022, 99.554)
(4023, 99.558)
(4024, 99.614)
(4025, 98.908)
(4026, 97.018)
(4027, 99.134)
(4028, 99.284)
(4029, 99.082)
(4030, 98.992)
(4031, 98.974)
(4032, 99.826)
(4033, 99.658)
(4034, 99.674)
(4035, 99.796)
(4036, 99.71)
(4037, 99.778)
(4038, 99.668)
(4039, 99.696)
(4040, 99.912)
(4041, 99.87)
(4042, 99.972)
(4043, 99.998)
(4044, 100)
(4045, 99.992)
(4046, 99.994)
(4047, 99.956)
(4048, 99.94)
(4049, 99.978)
(4050, 99.994)
(4051, 100)
(4052, 99.972)
(4053, 99.718)
(4054, 99.828)
(4055, 99.32)
(4056, 99.77)
(4057, 99.712)
(4058, 99.802)
(4059, 99.728)
(4060, 99.878)
(4061, 99.756)
(4062, 99.922)
(4063, 99.958)
(4064, 99.99)
(4065, 99.994)
(4066, 99.986)
(4067, 99.968)
(4068, 99.808)
(4069, 99.95)
(4070, 100)
(4071, 99.99)
(4072, 99.962)
(4073, 99.982)
(4074, 99.942)
(4075, 99.486)
(4076, 99.472)
(4077, 99.944)
(4078, 99.984)
(4079, 99.996)
(4080, 99.988)
(4081, 99.998)
(4082, 99.978)
(4083, 99.98)
(4084, 99.996)
(4085, 99.994)
(4086, 99.952)
(4087, 99.818)
(4088, 99.752)
(4089, 99.88)
(4090, 99.998)
(4091, 99.948)
(4092, 99.916)
(4093, 99.198)
(4094, 100)
(4095, 99.968)
(4096, 99.998)
(4097, 99.982)
(4098, 99.996)
(4099, 99.996)
(4100, 100)
(4101, 100)
(4102, 100)
(4103, 99.956)
(4104, 99.998)
(4105, 100)
(4106, 100)
(4107, 99.962)
(4108, 99.984)
(4109, 100)
(4110, 100)
(4111, 100)
(4112, 99.982)
(4113, 99.996)
(4114, 99.948)
(4115, 100)
(4116, 99.996)
(4117, 99.996)
(4118, 99.978)
(4119, 99.98)
(4120, 99.996)
(4121, 99.934)
(4122, 99.984)
(4123, 99.932)
(4124, 99.958)
(4125, 97.942)
(4126, 99.888)
(4127, 99.956)
(4128, 89.816)
(4129, 90.488)
(4130, 89.268)
(4131, 99.998)
(4132, 99.912)
(4133, 99.88)
(4134, 99.812)
(4135, 92.832)
(4136, 99.85)
(4137, 98.05)
(4138, 97.634)
(4139, 98.564)
(4140, 98.128)
(4141, 97.13)
(4142, 99.452)
(4143, 98.518)
(4144, 99.198)
(4145, 99.704)
(4146, 99.834)
(4147, 99.98)
(4148, 99.81)
(4149, 99.872)
(4150, 99.184)
(4151, 99.888)
(4152, 99.992)
(4153, 99.99)
(4154, 99.992)
(4155, 99.972)
(4156, 99.938)
(4157, 99.978)
(4158, 99.952)
(4159, 99.988)
(4160, 99.89)
(4161, 99.942)
(4162, 99.964)
(4163, 99.898)
(4164, 99.89)
(4165, 99.894)
(4166, 99.816)
(4167, 99.906)
(4168, 99.734)
(4169, 99.796)
(4170, 99.854)
(4171, 99.728)
(4172, 99.748)
(4173, 99.738)
(4174, 99.918)
(4175, 99.91)
(4176, 98.552)
(4177, 99.316)
(4178, 98.512)
(4179, 97.624)
(4180, 98.714)
(4181, 98.484)
(4182, 99.51)
(4183, 99.576)
(4184, 99.668)
(4185, 98.916)
(4186, 98.968)
(4187, 99.428)
(4188, 99.702)
(4189, 97.068)
(4190, 99.88)
(4191, 99.986)
(4192, 99.958)
(4193, 99.89)
(4194, 99.99)
(4195, 99.954)
(4196, 99.926)
(4197, 99.896)
(4198, 99.978)
(4199, 99.922)
(4200, 98.718)
(4201, 98.132)
(4202, 100)
(4203, 99.994)
(4204, 99.992)
(4205, 99.986)
(4206, 99.986)
(4207, 99.992)
(4208, 99.972)
(4209, 99.994)
(4210, 99.988)
(4211, 99.974)
(4212, 99.96)
(4213, 99.958)
(4214, 99.946)
(4215, 99.966)
(4216, 99.794)
(4217, 99.696)
(4218, 99.646)
(4219, 99.674)
(4220, 99.746)
(4221, 99.704)
(4222, 99.6)
(4223, 98.08)
(4224, 98.212)
(4225, 99.718)
(4226, 99.228)
(4227, 98.212)
(4228, 97.898)
(4229, 98.028)
(4230, 98.546)
(4231, 98.766)
(4232, 96.34)
(4233, 96.866)
(4234, 98.1)
(4235, 98)
(4236, 97.596)
(4237, 96.214)
(4238, 96.296)
(4239, 97.106)
(4240, 97.8)
(4241, 97.724)
(4242, 97.998)
(4243, 97.578)
(4244, 91.346)
(4245, 94.2)
(4246, 96.44)
(4247, 94.128)
(4248, 93.67)
(4249, 94.868)
(4250, 96.568)
(4251, 96.864)
(4252, 98.388)
(4253, 98.48)
(4254, 98.322)
(4255, 99.15)
(4256, 98.742)
(4257, 97.952)
(4258, 96.036)
(4259, 96.982)
(4260, 94.538)
(4261, 97.826)
(4262, 98.122)
(4263, 97.9)
(4264, 97.328)
(4265, 97.704)
(4266, 96.788)
(4267, 95.48)
(4268, 97.392)
(4269, 95.11)
(4270, 98.318)
(4271, 99.096)
(4272, 97.406)
(4273, 97.076)
(4274, 97.528)
(4275, 97.132)
(4276, 97.154)
(4277, 95.53)
(4278, 95.984)
(4279, 88.558)
(4280, 97.108)
(4281, 98.258)
(4282, 98.446)
(4283, 95.436)
(4284, 97.234)
(4285, 97.744)
(4286, 97.854)
(4287, 97.534)
(4288, 98.73)
(4289, 97.462)
(4290, 92.518)
(4291, 94.712)
(4292, 92.018)
(4293, 95.256)
(4294, 97.668)
(4295, 96.458)
(4296, 98.416)
(4297, 98.136)
(4298, 99.35)
(4299, 95.13)
(4300, 97.936)
(4301, 98.59)
(4302, 99.246)
(4303, 98.744)
(4304, 91.836)
(4305, 98.488)
(4306, 95.882)
(4307, 92.934)
(4308, 98.074)
(4309, 98.168)
(4310, 96.4)
(4311, 96.256)
(4312, 93.77)
(4313, 93.726)
(4314, 93.922)
(4315, 96.664)
(4316, 97.026)
(4317, 97.098)
(4318, 93.68)
(4319, 96.144)
(4320, 98.002)
(4321, 99.138)
(4322, 98.082)
(4323, 96.634)
(4324, 97.812)
(4325, 98.804)
(4326, 99.438)
(4327, 99.368)
(4328, 98.444)
(4329, 99.496)
(4330, 99.532)
(4331, 99.702)
(4332, 99.804)
(4333, 99.394)
(4334, 99.414)
(4335, 99.562)
(4336, 99.666)
(4337, 91.944)
(4338, 91.724)
(4339, 98.316)
(4340, 99.394)
(4341, 99.636)
(4342, 93.026)
(4343, 99.014)
(4344, 99.23)
(4345, 99.57)
(4346, 99.368)
(4347, 98.638)
(4348, 99.06)
(4349, 97.84)
(4350, 98.994)
(4351, 98.87)
(4352, 99.072)
(4353, 99.104)
(4354, 99.194)
(4355, 99.276)
(4356, 99.208)
(4357, 98.074)
(4358, 97.412)
(4359, 96.52)
(4360, 99.318)
(4361, 99.36)
(4362, 98.43)
(4363, 99.248)
(4364, 98.666)
(4365, 97.81)
(4366, 98.508)
(4367, 99.408)
(4368, 99.482)
(4369, 99.642)
(4370, 99.566)
(4371, 99.854)
(4372, 99.842)
(4373, 99.572)
(4374, 99.562)
(4375, 91.936)
(4376, 99.674)
(4377, 99.69)
(4378, 99.616)
(4379, 99.488)
(4380, 99.298)
(4381, 99.152)
(4382, 99.03)
(4383, 98.808)
(4384, 99.03)
(4385, 98.534)
(4386, 98.562)
(4387, 97.974)
(4388, 98.176)
(4389, 99.53)
(4390, 99.586)
(4391, 99.42)
(4392, 99.594)
(4393, 98.542)
(4394, 98.68)
(4395, 97.924)
(4396, 98.942)
(4397, 96.51)
(4398, 98.956)
(4399, 96.896)
(4400, 99.644)
(4401, 99.506)
(4402, 99.668)
(4403, 99.672)
(4404, 99.896)
(4405, 99.438)
(4406, 98.85)
(4407, 97.49)
(4408, 99.448)
(4409, 97.654)
(4410, 98.706)
(4411, 98.404)
(4412, 99.192)
(4413, 98.882)
(4414, 94.44)
(4415, 97.954)
(4416, 98.738)
(4417, 99.256)
(4418, 99.968)
(4419, 99.814)
(4420, 99.676)
(4421, 99.904)
(4422, 99.804)
(4423, 99.76)
(4424, 99.22)
(4425, 99.782)
(4426, 99.49)
(4427, 98.692)
(4428, 98.944)
(4429, 98.17)
(4430, 99.472)
(4431, 98.372)
(4432, 97.558)
(4433, 95.324)
(4434, 97.26)
(4435, 99.34)
(4436, 98.9)
(4437, 99.07)
(4438, 98.784)
(4439, 99.388)
(4440, 97.788)
(4441, 98.616)
(4442, 99.284)
(4443, 98.524)
(4444, 99.432)
(4445, 96.496)
(4446, 99.406)
(4447, 99.606)
(4448, 99.27)
(4449, 98.514)
(4450, 99.216)
(4451, 98.474)
(4452, 98.034)
(4453, 99.708)
(4454, 87.706)
(4455, 98.504)
(4456, 99.29)
(4457, 99.884)
(4458, 98.282)
(4459, 99.774)
(4460, 99.558)
(4461, 99.53)
(4462, 99.918)
(4463, 99.896)
(4464, 99.744)
(4465, 99.58)
(4466, 99.786)
(4467, 99.714)
(4468, 99.796)
(4469, 99.694)
(4470, 99.824)
(4471, 99.96)
(4472, 99.898)
(4473, 99.924)
(4474, 99.92)
(4475, 99.896)
(4476, 99.902)
(4477, 99.676)
(4478, 99.93)
(4479, 99.772)
(4480, 97.9)
(4481, 99.646)
(4482, 99.938)
(4483, 99.942)
(4484, 99.594)
(4485, 99.73)
(4486, 99.874)
(4487, 99.092)
(4488, 99.694)
(4489, 99.884)
(4490, 99.496)
(4491, 99.694)
(4492, 99.88)
(4493, 99.912)
(4494, 99.474)
(4495, 99.856)
(4496, 99.3)
(4497, 99.82)
(4498, 99.748)
(4499, 99.852)
(4500, 99.856)
(4501, 99.172)
(4502, 99.77)
(4503, 99.918)
(4504, 99.714)
(4505, 99.32)
(4506, 99.88)
(4507, 99.97)
(4508, 99.844)
(4509, 99.736)
(4510, 99.862)
(4511, 99.796)
(4512, 99.158)
(4513, 99.826)
(4514, 99.988)
(4515, 99.648)
(4516, 99.076)
(4517, 98.92)
(4518, 99.036)
(4519, 99.19)
(4520, 99.664)
(4521, 98.364)
(4522, 99.462)
(4523, 99.82)
(4524, 99.138)
(4525, 99.188)
(4526, 99.61)
(4527, 99.524)
(4528, 99.92)
(4529, 99.59)
(4530, 98.696)
(4531, 99.86)
(4532, 99.718)
(4533, 99.86)
(4534, 99.972)
(4535, 99.99)
(4536, 99.988)
(4537, 99.846)
(4538, 99.96)
(4539, 99.896)
(4540, 99.904)
(4541, 99.898)
(4542, 99.944)
(4543, 99.74)
(4544, 99.59)
(4545, 99.82)
(4546, 99.852)
(4547, 99.272)
(4548, 99.794)
(4549, 99.65)
(4550, 99.91)
(4551, 99.984)
(4552, 99.976)
(4553, 99.042)
(4554, 98.488)
(4555, 99.078)
(4556, 99.908)
(4557, 99.36)
(4558, 99.948)
(4559, 99.804)
(4560, 99.538)
(4561, 99.934)
(4562, 99.942)
(4563, 99.982)
(4564, 99.85)
(4565, 99.792)
(4566, 99.93)
(4567, 99.986)
(4568, 99.928)
(4569, 99.94)
(4570, 99.776)
(4571, 99.99)
(4572, 99.934)
(4573, 99.89)
(4574, 98.804)
(4575, 98.244)
(4576, 99.958)
(4577, 99.838)
(4578, 99.8)
(4579, 99.35)
(4580, 97.118)
(4581, 99.28)
(4582, 98.712)
(4583, 99.188)
(4584, 99.198)
(4585, 98.688)
(4586, 99.554)
(4587, 99.01)
(4588, 98.578)
(4589, 98.382)
(4590, 98.314)
(4591, 99.424)
(4592, 99.078)
(4593, 98.338)
(4594, 98.882)
(4595, 98.284)
(4596, 95.82)
(4597, 98.626)
(4598, 98.07)
(4599, 99.23)
(4600, 98.842)
(4601, 90.962)
(4602, 98.292)
(4603, 99.406)
(4604, 98.626)
(4605, 83.65)
(4606, 98.486)
(4607, 99.436)
(4608, 98.11)
(4609, 99.388)
(4610, 99.154)
(4611, 98.674)
(4612, 99.452)
(4613, 99.19)
(4614, 96.772)
(4615, 98.89)
(4616, 99.506)
(4617, 95.586)
(4618, 99.232)
(4619, 99.796)
(4620, 99.528)
(4621, 99.902)
(4622, 99.93)
(4623, 99.658)
(4624, 99.45)
(4625, 99.65)
(4626, 99.838)
(4627, 99.892)
(4628, 99.932)
(4629, 99.936)
(4630, 99.696)
(4631, 99.418)
(4632, 99.702)
(4633, 99.9)
(4634, 99.852)
(4635, 99.89)
(4636, 99.91)
(4637, 99.78)
(4638, 99.824)
(4639, 99.898)
(4640, 99.632)
(4641, 99.794)
(4642, 99.826)
(4643, 99.74)
(4644, 99.062)
(4645, 99.686)
(4646, 99.78)
(4647, 99.742)
(4648, 99.722)
(4649, 98.71)
(4650, 99.798)
(4651, 99.762)
(4652, 99.522)
(4653, 99.486)
(4654, 99.89)
(4655, 99.812)
(4656, 98.658)
(4657, 99.008)
(4658, 98.8)
(4659, 99.224)
(4660, 99.9)
(4661, 98.908)
(4662, 99.19)
(4663, 97.214)
(4664, 99.714)
(4665, 97.632)
(4666, 99.826)
(4667, 99.712)
(4668, 99.954)
(4669, 99.85)
(4670, 99.778)
(4671, 99.304)
(4672, 99.6)
(4673, 99.776)
(4674, 99.546)
(4675, 99.652)
(4676, 99.87)
(4677, 99.464)
(4678, 99.084)
(4679, 99.824)
(4680, 99.428)
(4681, 99.516)
(4682, 99.802)
(4683, 99.876)
(4684, 99.96)
(4685, 99.946)
(4686, 99.456)
(4687, 99.498)
(4688, 99.71)
(4689, 99.788)
(4690, 99.206)
(4691, 99.914)
(4692, 99.854)
(4693, 99.79)
(4694, 99.818)
(4695, 99.972)
(4696, 99.972)
(4697, 99.84)
(4698, 99.248)
(4699, 98.102)
(4700, 99.65)
(4701, 98.744)
(4702, 99.484)
(4703, 98.706)
(4704, 99.574)
(4705, 99.612)
(4706, 98.972)
(4707, 99.16)
(4708, 99.888)
(4709, 99.954)
(4710, 99.91)
(4711, 97.07)
(4712, 99.62)
(4713, 99.282)
(4714, 99.424)
(4715, 99.81)
(4716, 99.908)
(4717, 99.724)
(4718, 99.564)
(4719, 99.59)
(4720, 99.854)
(4721, 99.696)
(4722, 99.528)
(4723, 99.636)
(4724, 99.758)
(4725, 99.928)
(4726, 99.962)
(4727, 99.974)
(4728, 99.912)
(4729, 99.476)
(4730, 98.59)
(4731, 99.856)
(4732, 99.846)
(4733, 99.476)
(4734, 99.914)
(4735, 99.866)
(4736, 99.46)
(4737, 99.968)
(4738, 99.928)
(4739, 99.554)
(4740, 99.856)
(4741, 99.742)
(4742, 99.998)
(4743, 99.94)
(4744, 98.948)
(4745, 99.26)
(4746, 98.276)
(4747, 99.542)
(4748, 98.954)
(4749, 99.578)
(4750, 99.482)
(4751, 99.448)
(4752, 99.138)
(4753, 98.804)
(4754, 97.892)
(4755, 99.684)
(4756, 99.588)
(4757, 99.92)
(4758, 99.986)
(4759, 99.93)
(4760, 99.71)
(4761, 100)
(4762, 99.996)
(4763, 99.986)
(4764, 99.988)
(4765, 99.92)
(4766, 99.92)
(4767, 99.886)
(4768, 99.798)
(4769, 99.942)
(4770, 99.982)
(4771, 99.996)
(4772, 99.97)
(4773, 99.986)
(4774, 99.99)
(4775, 99.928)
(4776, 99.112)
(4777, 98.32)
(4778, 99.74)
(4779, 99.502)
(4780, 98.618)
(4781, 99.688)
(4782, 99.628)
(4783, 99.508)
(4784, 98.834)
(4785, 98.81)
(4786, 98.1)
(4787, 99.842)
(4788, 97.326)
(4789, 98.862)
(4790, 99.504)
(4791, 98.824)
(4792, 99.62)
(4793, 99.436)
(4794, 99.504)
(4795, 99.572)
(4796, 99.32)
(4797, 99.244)
(4798, 98.96)
(4799, 99.588)
(4800, 99.388)
(4801, 99.014)
(4802, 99.756)
(4803, 99.902)
(4804, 99.934)
(4805, 99.612)
(4806, 99.994)
(4807, 99.442)
(4808, 99.91)
(4809, 99.878)
(4810, 99.982)
(4811, 99.932)
(4812, 99.856)
(4813, 99.868)
(4814, 99.9)
(4815, 99.498)
(4816, 99.7)
(4817, 99.138)
(4818, 99.816)
(4819, 98.942)
(4820, 99.794)
(4821, 99.61)
(4822, 99.94)
(4823, 99.72)
(4824, 99.484)
(4825, 99.128)
(4826, 99.576)
(4827, 97.688)
(4828, 99.622)
(4829, 99.492)
(4830, 99.852)
(4831, 99.448)
(4832, 99.704)
(4833, 99.562)
(4834, 99.872)
(4835, 99.446)
(4836, 99.782)
(4837, 99.32)
(4838, 99.742)
(4839, 99.792)
(4840, 99.144)
(4841, 99.876)
(4842, 99.97)
(4843, 99.808)
(4844, 99.748)
(4845, 99.836)
(4846, 99.826)
(4847, 99.832)
(4848, 99.806)
(4849, 99.96)
(4850, 99.824)
(4851, 99.91)
(4852, 99.896)
(4853, 99.918)
(4854, 99.716)
(4855, 99.472)
(4856, 99.89)
(4857, 99.922)
(4858, 98.39)
(4859, 99.406)
(4860, 98.896)
(4861, 98.862)
(4862, 99.424)
(4863, 99.912)
(4864, 99.726)
(4865, 99.44)
(4866, 98.922)
(4867, 98.626)
(4868, 98.826)
(4869, 99.736)
(4870, 99.516)
(4871, 99.428)
(4872, 99.54)
(4873, 99.482)
(4874, 98.828)
(4875, 99.326)
(4876, 99.46)
(4877, 99.128)
(4878, 98.812)
(4879, 99.682)
(4880, 99.342)
(4881, 98.216)
(4882, 99.812)
(4883, 99.746)
(4884, 99.576)
(4885, 99.614)
(4886, 99.47)
(4887, 99.762)
(4888, 97.952)
(4889, 99.358)
(4890, 98.574)
(4891, 99.73)
(4892, 99.8)
(4893, 99.744)
(4894, 98.862)
(4895, 99.978)
(4896, 99.964)
(4897, 99.994)
(4898, 99.984)
(4899, 99.932)
(4900, 98.402)
(4901, 99.458)
(4902, 99.774)
(4903, 99.634)
(4904, 99.824)
(4905, 99.988)
(4906, 99.966)
(4907, 99.966)
(4908, 99.998)
(4909, 99.954)
(4910, 99.95)
(4911, 99.99)
(4912, 99.862)
(4913, 99.838)
(4914, 99.326)
(4915, 99.792)
(4916, 99.794)
(4917, 99.97)
(4918, 99.984)
(4919, 99.966)
(4920, 99.994)
(4921, 99.972)
(4922, 100)
(4923, 100)
(4924, 99.946)
(4925, 99.968)
(4926, 99.908)
(4927, 99.972)
(4928, 99.996)
(4929, 99.994)
(4930, 99.992)
(4931, 99.996)
(4932, 100)
(4933, 100)
(4934, 100)
(4935, 100)
(4936, 100)
(4937, 99.998)
(4938, 99.998)
(4939, 99.98)
(4940, 99.978)
(4941, 99.942)
(4942, 99.98)
(4943, 99.996)
(4944, 99.736)
(4945, 100)
(4946, 100)
(4947, 99.998)
(4948, 100)
(4949, 100)
(4950, 100)
(4951, 100)
(4952, 100)
(4953, 99.982)
(4954, 99.994)
(4955, 100)
(4956, 99.99)
(4957, 99.998)
(4958, 100)
(4959, 100)
(4960, 100)
(4961, 99.996)
(4962, 100)
(4963, 100)
(4964, 100)
(4965, 100)
(4966, 100)
(4967, 100)
(4968, 100)
(4969, 100)
(4970, 100)
(4971, 100)
(4972, 99.998)
(4973, 100)
(4974, 99.882)
(4975, 100)
(4976, 99.972)
(4977, 99.972)
(4978, 99.458)
(4979, 99.984)
(4980, 100)
(4981, 99.988)
(4982, 100)
(4983, 100)
(4984, 99.998)
(4985, 99.996)
(4986, 99.994)
(4987, 100)
(4988, 99.99)
(4989, 100)
(4990, 99.958)
(4991, 99.946)
(4992, 99.916)
(4993, 99.9)
(4994, 99.91)
(4995, 99.996)
(4996, 99.992)
(4997, 99.994)
(4998, 99.922)
(4999, 99.984)
(5000, 99.996)
(5001, 99.886)
(5002, 98.024)
(5003, 99.94)
(5004, 99.756)
(5005, 99.404)
(5006, 99.264)
(5007, 99.886)
(5008, 99.742)
(5009, 99.442)
(5010, 99.176)
(5011, 99.516)
(5012, 99.934)
(5013, 99.938)
(5014, 99.998)
(5015, 99.82)
(5016, 99.872)
(5017, 99.288)
(5018, 99.906)
(5019, 99.88)
(5020, 99.982)
(5021, 99.988)
(5022, 99.998)
(5023, 99.936)
(5024, 99.748)
(5025, 99.652)
(5026, 99.974)
(5027, 99.988)
(5028, 99.998)
(5029, 99.98)
(5030, 98.914)
(5031, 99.996)
(5032, 99.994)
(5033, 100)
(5034, 99.916)
(5035, 99.968)
(5036, 99.94)
(5037, 99.96)
(5038, 99.788)
(5039, 100)
(5040, 99.998)
(5041, 100)
(5042, 99.994)
(5043, 99.988)
(5044, 99.92)
(5045, 99.948)
(5046, 99.988)
(5047, 99.286)
(5048, 99.776)
(5049, 99.982)
(5050, 99.752)
(5051, 99.956)
(5052, 99.924)
(5053, 99.86)
(5054, 99.862)
(5055, 99.544)
(5056, 99.978)
(5057, 98.93)
(5058, 99.866)
(5059, 99.896)
(5060, 99.862)
(5061, 99.302)
(5062, 99.958)
(5063, 99.856)
(5064, 99.966)
(5065, 99.908)
(5066, 97.138)
(5067, 99.988)
(5068, 99.87)
(5069, 99.888)
(5070, 99.922)
(5071, 99.986)
(5072, 99.998)
(5073, 99.382)
(5074, 99.746)
(5075, 98.89)
(5076, 98.706)
(5077, 98.31)
(5078, 98.802)
(5079, 99.44)
(5080, 98.8)
(5081, 99.384)
(5082, 98.72)
(5083, 98.986)
(5084, 98.856)
(5085, 99.802)
(5086, 99.61)
(5087, 99.256)
(5088, 98.938)
(5089, 99.784)
(5090, 99.426)
(5091, 96.394)
(5092, 99.578)
(5093, 99.504)
(5094, 99.282)
(5095, 99.688)
(5096, 99.3)
(5097, 99.804)
(5098, 99.37)
(5099, 99.682)
(5100, 99.72)
(5101, 99.838)
(5102, 98.966)
(5103, 97.306)
(5104, 97.494)
(5105, 99.71)
(5106, 95.404)
(5107, 98.658)
(5108, 98.604)
(5109, 98.872)
(5110, 98.778)
(5111, 99.372)
(5112, 99.602)
(5113, 99.584)
(5114, 99.598)
(5115, 98.084)
(5116, 99.934)
(5117, 99.944)
(5118, 99.968)
(5119, 99.98)
(5120, 99.902)
(5121, 99.946)
(5122, 99.838)
(5123, 99.94)
(5124, 100)
(5125, 99.97)
(5126, 99.994)
(5127, 99.826)
(5128, 99.452)
(5129, 99.918)
(5130, 99.908)
(5131, 99.74)
(5132, 99.674)
(5133, 99.804)
(5134, 99.788)
(5135, 99.806)
(5136, 96.402)
(5137, 99.128)
(5138, 99.372)
(5139, 98.462)
(5140, 99.092)
(5141, 98.156)
(5142, 99.726)
(5143, 98.246)
(5144, 99.004)
(5145, 99.578)
(5146, 99.914)
(5147, 99.9)
(5148, 99.922)
(5149, 99.788)
(5150, 98.58)
(5151, 99.276)
(5152, 99.924)
(5153, 99.936)
(5154, 99.888)
(5155, 99.77)
(5156, 99.642)
(5157, 99.622)
(5158, 99.434)
(5159, 99.796)
(5160, 99.47)
(5161, 99.806)
(5162, 99.938)
(5163, 99.41)
(5164, 99.278)
(5165, 99.652)
(5166, 99.52)
(5167, 99.968)
(5168, 99.862)
(5169, 99.912)
(5170, 99.9)
(5171, 99.948)
(5172, 99.868)
(5173, 99.894)
(5174, 99.976)
(5175, 99.828)
(5176, 99.412)
(5177, 99.952)
(5178, 99.942)
(5179, 99.842)
(5180, 99.932)
(5181, 99.984)
(5182, 99.5)
(5183, 99.966)
(5184, 99.626)
(5185, 99.782)
(5186, 98.662)
(5187, 99.874)
(5188, 99.872)
(5189, 99.826)
(5190, 99.962)
(5191, 99.928)
(5192, 99.774)
(5193, 99.748)
(5194, 99.108)
(5195, 99.96)
(5196, 99.968)
(5197, 99.992)
(5198, 99.888)
(5199, 99.87)
(5200, 99.302)
(5201, 99.67)
(5202, 99.6)
(5203, 99.356)
(5204, 99.858)
(5205, 99.852)
(5206, 99.104)
(5207, 98.246)
(5208, 99.794)
(5209, 99.774)
(5210, 99.962)
(5211, 99.658)
(5212, 97.638)
(5213, 99.686)
(5214, 99.89)
(5215, 99.804)
(5216, 99.782)
(5217, 98.53)
(5218, 96.546)
(5219, 98.832)
(5220, 99.964)
(5221, 99.964)
(5222, 99.804)
(5223, 99.914)
(5224, 99.87)
(5225, 99.718)
(5226, 99.93)
(5227, 98.4)
(5228, 99.986)
(5229, 99.754)
(5230, 99.51)
(5231, 99.962)
(5232, 99.918)
(5233, 99.9)
(5234, 99.238)
(5235, 97.902)
(5236, 99.968)
(5237, 99.968)
(5238, 100)
(5239, 99.974)
(5240, 99.974)
(5241, 99.882)
(5242, 99.998)
(5243, 99.976)
(5244, 99.714)
(5245, 99.896)
(5246, 99.98)
(5247, 99.996)
(5248, 99.046)
(5249, 99.99)
(5250, 100)
(5251, 99.998)
(5252, 100)
(5253, 100)
(5254, 100)
(5255, 100)
(5256, 99.902)
(5257, 99.934)
(5258, 99.99)
(5259, 99.958)
(5260, 99.964)
(5261, 99.95)
(5262, 99.968)
(5263, 99.994)
(5264, 99.992)
(5265, 99.884)
(5266, 99.764)
(5267, 99.988)
(5268, 99.968)
(5269, 99.99)
(5270, 99.974)
(5271, 99.98)
(5272, 99.972)
(5273, 99.996)
(5274, 99.98)
(5275, 99.932)
(5276, 99.912)
(5277, 99.928)
(5278, 99.758)
(5279, 99.978)
(5280, 97.466)
(5281, 99.986)
(5282, 99.94)
(5283, 99.86)
(5284, 99.876)
(5285, 99.954)
(5286, 99.602)
(5287, 99.15)
(5288, 99.938)
(5289, 99.702)
(5290, 99.352)
(5291, 99.896)
(5292, 99.94)
(5293, 99.922)
(5294, 99.75)
(5295, 99.894)
(5296, 99.78)
(5297, 99.952)
(5298, 99.946)
(5299, 99.81)
(5300, 99.866)
(5301, 99.932)
(5302, 98.874)
(5303, 99.986)
(5304, 99.98)
(5305, 99.93)
(5306, 98.088)
(5307, 99.926)
(5308, 99.906)
(5309, 99.968)
(5310, 99.75)
(5311, 99.606)
(5312, 99.214)
(5313, 96.296)
(5314, 99.798)
(5315, 99.944)
(5316, 99.888)
(5317, 99.92)
(5318, 99.9)
(5319, 99.916)
(5320, 99.518)
(5321, 99.662)
(5322, 99.632)
(5323, 98.888)
(5324, 99.326)
(5325, 99.834)
(5326, 99.932)
(5327, 99.648)
(5328, 99.608)
(5329, 99.76)
(5330, 99.43)
(5331, 99.904)
(5332, 99.966)
(5333, 99.96)
(5334, 99.838)
(5335, 99.864)
(5336, 99.468)
(5337, 99.712)
(5338, 99.634)
(5339, 99.532)
(5340, 99.56)
(5341, 99.586)
(5342, 99.956)
(5343, 99.888)
(5344, 98.238)
(5345, 99.934)
(5346, 99.886)
(5347, 99.454)
(5348, 99.436)
(5349, 99.95)
(5350, 99.82)
(5351, 99.338)
(5352, 99.292)
(5353, 99.946)
(5354, 99.684)
(5355, 99.818)
(5356, 99.812)
(5357, 99.56)
(5358, 99.514)
(5359, 99.916)
(5360, 98.694)
(5361, 99.88)
(5362, 99.784)
(5363, 99.91)
(5364, 99.934)
(5365, 99.846)
(5366, 99.954)
(5367, 99.994)
(5368, 99.9)
(5369, 99.908)
(5370, 99.97)
(5371, 99.93)
(5372, 99.406)
(5373, 99.892)
(5374, 99.55)
(5375, 99.982)
(5376, 99.96)
(5377, 99.886)
(5378, 99.99)
(5379, 99.96)
(5380, 99.886)
(5381, 99.83)
(5382, 97.258)
(5383, 98.92)
(5384, 98.02)
(5385, 99.606)
(5386, 99.784)
(5387, 99.952)
(5388, 99.988)
(5389, 99.98)
(5390, 99.99)
(5391, 99.938)
(5392, 99.906)
(5393, 99.33)
(5394, 99.734)
(5395, 100)
(5396, 100)
(5397, 99.95)
(5398, 99.904)
(5399, 99.904)
(5400, 99.858)
(5401, 99.994)
(5402, 99.84)
(5403, 99.98)
(5404, 99.852)
(5405, 99.98)
(5406, 99.622)
(5407, 99.974)
(5408, 99.95)
(5409, 99.746)
(5410, 99.956)
(5411, 99.922)
(5412, 99.994)
(5413, 99.99)
(5414, 99.964)
(5415, 99.99)
(5416, 99.982)
(5417, 99.938)
(5418, 99.96)
(5419, 99.958)
(5420, 99.762)
(5421, 99.41)
(5422, 99.468)
(5423, 99.974)
(5424, 99.998)
(5425, 99.996)
(5426, 99.992)
(5427, 99.992)
(5428, 100)
(5429, 100)
(5430, 99.97)
(5431, 99.918)
(5432, 99.872)
(5433, 99.95)
(5434, 99.998)
(5435, 99.966)
(5436, 99.902)
(5437, 99.578)
(5438, 99.992)
(5439, 99.906)
(5440, 100)
(5441, 100)
(5442, 100)
(5443, 100)
(5444, 99.892)
(5445, 100)
(5446, 100)
(5447, 99.994)
(5448, 99.996)
(5449, 99.994)
(5450, 99.996)
(5451, 99.982)
(5452, 99.988)
(5453, 99.966)
(5454, 99.994)
(5455, 99.984)
(5456, 99.94)
(5457, 94.28)
(5458, 99.948)
(5459, 99.996)
(5460, 99.974)
(5461, 99.974)
(5462, 99.928)
(5463, 99.942)
(5464, 99.874)
(5465, 98.826)
(5466, 99.072)
(5467, 99.962)
(5468, 99.91)
(5469, 99.906)
(5470, 99.998)
(5471, 99.994)
(5472, 99.982)
(5473, 99.95)
(5474, 99.988)
(5475, 99.922)
(5476, 99.76)
(5477, 99.864)
(5478, 99.992)
(5479, 99.996)
(5480, 100)
(5481, 99.95)
(5482, 99.978)
(5483, 99.974)
(5484, 99.94)
(5485, 99.976)
(5486, 99.836)
(5487, 99.968)
(5488, 99.852)
(5489, 99.522)
(5490, 99.6)
(5491, 99.828)
(5492, 99.622)
(5493, 99.902)
(5494, 99.914)
(5495, 99.892)
(5496, 99.868)
(5497, 99.986)
(5498, 99.898)
(5499, 99.702)
(5500, 99.856)
(5501, 99.892)
(5502, 99.784)
(5503, 99.974)
(5504, 99.892)
(5505, 99.864)
(5506, 99.882)
(5507, 99.928)
(5508, 99.954)
(5509, 99.97)
(5510, 99.954)
(5511, 100)
(5512, 100)
(5513, 99.982)
(5514, 99.998)
(5515, 99.996)
(5516, 100)
(5517, 100)
(5518, 99.994)
(5519, 100)
(5520, 99.988)
(5521, 99.998)
(5522, 99.99)
(5523, 100)
(5524, 99.998)
(5525, 100)
(5526, 100)
(5527, 99.994)
(5528, 100)
(5529, 100)
(5530, 100)
(5531, 99.986)
(5532, 99.976)
(5533, 99.946)
(5534, 99.976)
(5535, 99.666)
(5536, 99.902)
(5537, 99.924)
(5538, 100)
(5539, 99.958)
(5540, 99.98)
(5541, 99.774)
(5542, 99.954)
(5543, 100)
(5544, 100)
(5545, 100)
(5546, 99.998)
(5547, 99.964)
(5548, 99.944)
(5549, 99.936)
(5550, 98.714)
(5551, 99.982)
(5552, 99.942)
(5553, 98.866)
(5554, 98.192)
(5555, 99.8)
(5556, 99.924)
(5557, 99.992)
(5558, 99.888)
(5559, 99.98)
(5560, 99.992)
(5561, 100)
(5562, 99.982)
(5563, 99.996)
(5564, 99.996)
(5565, 99.992)
(5566, 99.962)
(5567, 99.97)
(5568, 99.986)
(5569, 99.944)
(5570, 99.954)
(5571, 99.972)
(5572, 99.93)
(5573, 99.794)
(5574, 99.294)
(5575, 99.198)
(5576, 97.582)
(5577, 98.342)
(5578, 98.362)
(5579, 94.456)
(5580, 97.548)
(5581, 98.848)
(5582, 98.384)
(5583, 96.414)
(5584, 98.338)
(5585, 99.094)
(5586, 99.806)
(5587, 99.48)
(5588, 99.468)
(5589, 99.69)
(5590, 99.768)
(5591, 99.89)
(5592, 99.686)
(5593, 99.932)
(5594, 99.802)
(5595, 99.338)
(5596, 99.56)
(5597, 99.398)
(5598, 98.25)
(5599, 99.12)
(5600, 99.736)
(5601, 99.264)
(5602, 99.466)
(5603, 99.652)
(5604, 99.842)
(5605, 99.91)
(5606, 99.786)
(5607, 99.69)
(5608, 97.312)
(5609, 96.206)
(5610, 99.38)
(5611, 99.692)
(5612, 99.42)
(5613, 98.726)
(5614, 98.586)
(5615, 98.95)
(5616, 99.174)
(5617, 99.682)
(5618, 99.67)
(5619, 99.362)
(5620, 98.806)
(5621, 99.282)
(5622, 98.028)
(5623, 95.214)
(5624, 99.432)
(5625, 98.728)
(5626, 99.41)
(5627, 99.81)
(5628, 99.694)
(5629, 99.778)
(5630, 99.616)
(5631, 99.634)
(5632, 99.272)
(5633, 99.434)
(5634, 98.944)
(5635, 99.262)
(5636, 99.52)
(5637, 99.714)
(5638, 99.08)
(5639, 99.526)
(5640, 99.482)
(5641, 99.678)
(5642, 98.722)
(5643, 97.28)
(5644, 97.546)
(5645, 97.048)
(5646, 98.264)
(5647, 99.668)
(5648, 94.746)
(5649, 97.672)
(5650, 97.28)
(5651, 97.77)
(5652, 98.956)
(5653, 97.9)
(5654, 99.062)
(5655, 98.966)
(5656, 95.838)
(5657, 96.404)
(5658, 96.748)
(5659, 97.046)
(5660, 98.728)
(5661, 98.938)
(5662, 98.42)
(5663, 95.898)
(5664, 98.086)
(5665, 97.77)
(5666, 96.412)
(5667, 92.866)
(5668, 98.186)
(5669, 93.552)
(5670, 95.156)
(5671, 95.878)
(5672, 99.056)
(5673, 97.714)
(5674, 98.372)
(5675, 97.412)
(5676, 96.866)
(5677, 83.726)
(5678, 98.148)
(5679, 98.394)
(5680, 98.482)
(5681, 94.652)
(5682, 98.198)
(5683, 91.804)
(5684, 96.396)
(5685, 95.834)
(5686, 94.94)
(5687, 98.06)
(5688, 98.182)
(5689, 95.114)
(5690, 92.474)
(5691, 93.548)
(5692, 95.724)
(5693, 92.582)
(5694, 94.97)
(5695, 93.088)
(5696, 98.598)
(5697, 97.344)
(5698, 97.992)
(5699, 96.778)
(5700, 98.43)
(5701, 98.328)
(5702, 96.724)
(5703, 96.336)
(5704, 99.004)
(5705, 99.14)
(5706, 99.03)
(5707, 98.346)
(5708, 97.438)
(5709, 99.27)
(5710, 98.89)
(5711, 98.174)
(5712, 96.666)
(5713, 99.092)
(5714, 97.886)
(5715, 99.43)
(5716, 99.702)
(5717, 98.018)
(5718, 99.432)
(5719, 98.614)
(5720, 99.076)
(5721, 98.622)
(5722, 98.688)
(5723, 99)
(5724, 99.48)
(5725, 99.202)
(5726, 99.526)
(5727, 98.158)
(5728, 99.294)
(5729, 99.702)
(5730, 99.448)
(5731, 99.47)
(5732, 99.22)
(5733, 99.24)
(5734, 98.976)
(5735, 94.608)
(5736, 98.92)
(5737, 98.758)
(5738, 99.13)
(5739, 98.238)
(5740, 97.94)
(5741, 99.148)
(5742, 99.738)
(5743, 99.092)
(5744, 97.29)
(5745, 99.012)
(5746, 99.296)
(5747, 99.294)
(5748, 99.43)
(5749, 99.304)
(5750, 99.792)
(5751, 98.798)
(5752, 97.218)
(5753, 99.66)
(5754, 99.698)
(5755, 99.652)
(5756, 99.708)
(5757, 99.284)
(5758, 99.788)
(5759, 99.75)
(5760, 99.402)
(5761, 99.828)
(5762, 99.548)
(5763, 99.626)
(5764, 99.556)
(5765, 99.184)
(5766, 99.252)
(5767, 99.358)
(5768, 99.286)
(5769, 99.522)
(5770, 99.354)
(5771, 99.132)
(5772, 98.582)
(5773, 97.176)
(5774, 95.466)
(5775, 95.476)
(5776, 97.374)
(5777, 95.886)
(5778, 96.556)
(5779, 98.26)
(5780, 98.988)
(5781, 98.188)
(5782, 97.988)
(5783, 97.89)
(5784, 98.85)
(5785, 98.44)
(5786, 97.696)
(5787, 97.136)
(5788, 96.15)
(5789, 97.5)
(5790, 97.76)
(5791, 98.142)
(5792, 98.13)
(5793, 98.448)
(5794, 99.152)
(5795, 99.37)
(5796, 99.51)
(5797, 99.374)
(5798, 99.422)
(5799, 98.844)
(5800, 98.946)
(5801, 99.454)
(5802, 99.578)
(5803, 99.85)
(5804, 99.354)
(5805, 99.816)
(5806, 99.488)
(5807, 99.964)
(5808, 99.878)
(5809, 99.438)
(5810, 99.816)
(5811, 99.452)
(5812, 99.282)
(5813, 99.804)
(5814, 99.564)
(5815, 99.132)
(5816, 99.624)
(5817, 99.818)
(5818, 99.72)
(5819, 98.378)
(5820, 98.32)
(5821, 99.464)
(5822, 98.772)
(5823, 99.258)
(5824, 99.46)
(5825, 99.564)
(5826, 99.586)
(5827, 99.394)
(5828, 99.664)
(5829, 99.452)
(5830, 99.608)
(5831, 99.854)
(5832, 99.06)
(5833, 99.088)
(5834, 99.706)
(5835, 98.582)
(5836, 99.248)
(5837, 99.45)
(5838, 99.474)
(5839, 99.54)
(5840, 99.784)
(5841, 99.648)
(5842, 98.824)
(5843, 99.202)
(5844, 99.788)
(5845, 99.916)
(5846, 99.832)
(5847, 99.798)
(5848, 99.754)
(5849, 99.246)
(5850, 99.154)
(5851, 99.856)
(5852, 99.276)
(5853, 99.688)
(5854, 99.758)
(5855, 99.578)
(5856, 98.814)
(5857, 98.824)
(5858, 95.498)
(5859, 99.406)
(5860, 99.662)
(5861, 99.696)
(5862, 99.346)
(5863, 99.88)
(5864, 99.782)
(5865, 99.734)
(5866, 99.508)
(5867, 98.2)
(5868, 99.212)
(5869, 96.732)
(5870, 99.446)
(5871, 99.726)
(5872, 99.63)
(5873, 99.906)
(5874, 99.642)
(5875, 99.966)
(5876, 99.202)
(5877, 99.828)
(5878, 99.61)
(5879, 97.118)
(5880, 99.876)
(5881, 99.934)
(5882, 99.882)
(5883, 99.768)
(5884, 99.418)
(5885, 99.742)
(5886, 99.584)
(5887, 99.872)
(5888, 99.654)
(5889, 99.66)
(5890, 99.394)
(5891, 99.526)
(5892, 99.778)
(5893, 99.462)
(5894, 99.854)
(5895, 99.564)
(5896, 99.824)
(5897, 99.614)
(5898, 99.338)
(5899, 98.368)
(5900, 99.73)
(5901, 99.682)
(5902, 99.35)
(5903, 99.536)
(5904, 98.79)
(5905, 99.688)
(5906, 99.452)
(5907, 99.078)
(5908, 99.75)
(5909, 99.458)
(5910, 99.766)
(5911, 99.772)
(5912, 99.796)
(5913, 99.644)
(5914, 99.72)
(5915, 98.886)
(5916, 99.724)
(5917, 99.038)
(5918, 99.494)
(5919, 99.512)
(5920, 99.522)
(5921, 99.602)
(5922, 99.78)
(5923, 99.57)
(5924, 99.464)
(5925, 99.76)
(5926, 99.862)
(5927, 99.446)
(5928, 99.736)
(5929, 99.874)
(5930, 99.766)
(5931, 98.536)
(5932, 99.884)
(5933, 99.938)
(5934, 99.996)
(5935, 99.946)
(5936, 99.914)
(5937, 99.976)
(5938, 100)
(5939, 99.494)
(5940, 99.974)
(5941, 99.926)
(5942, 99.726)
(5943, 99.948)
(5944, 99.788)
(5945, 99.988)
(5946, 99.912)
(5947, 99.982)
(5948, 100)
(5949, 99.992)
(5950, 99.86)
(5951, 99.968)
(5952, 99.972)
(5953, 99.624)
(5954, 99.988)
(5955, 99.942)
(5956, 99.966)
(5957, 99.992)
(5958, 99.99)
(5959, 99.988)
(5960, 100)
(5961, 99.998)
(5962, 99.954)
(5963, 99.996)
(5964, 99.99)
(5965, 99.876)
(5966, 99.994)
(5967, 100)
(5968, 100)
(5969, 100)
(5970, 100)
(5971, 100)
(5972, 100)
(5973, 100)
(5974, 99.998)
(5975, 100)
(5976, 100)
(5977, 100)
(5978, 100)
(5979, 100)
(5980, 100)
(5981, 100)
(5982, 100)
(5983, 100)
(5984, 100)
(5985, 100)
(5986, 100)
(5987, 100)
(5988, 99.98)
(5989, 99.738)
(5990, 91.826)
(5991, 99.998)
(5992, 99.994)
(5993, 100)
(5994, 99.99)
(5995, 99.974)
(5996, 99.99)
(5997, 99.922)
(5998, 99.86)
(5999, 99.95)
(6000, 99.956)
(6001, 99.97)
(6002, 99.86)
(6003, 99.046)
(6004, 100)
(6005, 99.992)
(6006, 100)
(6007, 99.998)
(6008, 99.99)
(6009, 99.972)
(6010, 99.986)
(6011, 99.952)
(6012, 99.826)
(6013, 99.958)
(6014, 99.998)
(6015, 99.986)
(6016, 99.964)
(6017, 99.954)
(6018, 99.988)
(6019, 99.956)
(6020, 99.982)
(6021, 99.998)
(6022, 99.988)
(6023, 99.976)
(6024, 99.774)
(6025, 99.972)
(6026, 100)
(6027, 99.998)
(6028, 99.572)
(6029, 99.95)
(6030, 99.676)
(6031, 98.952)
(6032, 99.77)
(6033, 99.828)
(6034, 99.932)
(6035, 99.866)
(6036, 99.946)
(6037, 99.358)
(6038, 99.208)
(6039, 99.946)
(6040, 99.784)
(6041, 99.826)
(6042, 99.952)
(6043, 99.968)
(6044, 99.986)
(6045, 99.992)
(6046, 99.76)
(6047, 99.992)
(6048, 99.998)
(6049, 99.996)
(6050, 99.992)
(6051, 99.976)
(6052, 99.904)
(6053, 99.55)
(6054, 99.896)
(6055, 99.742)
(6056, 99.93)
(6057, 99.938)
(6058, 99.998)
(6059, 99.78)
(6060, 99.93)
(6061, 99.982)
(6062, 99.99)
(6063, 99.984)
(6064, 99.984)
(6065, 99.824)
(6066, 99.966)
(6067, 99.796)
(6068, 99.82)
(6069, 98.444)
(6070, 99.706)
(6071, 99.87)
(6072, 99.89)
(6073, 99.944)
(6074, 99.806)
(6075, 99.842)
(6076, 99.854)
(6077, 99.924)
(6078, 99.732)
(6079, 99.792)
(6080, 99.578)
(6081, 99.394)
(6082, 99.99)
(6083, 99.962)
(6084, 99.886)
(6085, 99.918)
(6086, 98.412)
(6087, 99.722)
(6088, 99.332)
(6089, 99.562)
(6090, 99.128)
(6091, 99.412)
(6092, 99.736)
(6093, 99.35)
(6094, 99.806)
(6095, 99.596)
(6096, 99.242)
(6097, 99.912)
(6098, 99.662)
(6099, 99.826)
(6100, 97.908)
(6101, 99.104)
(6102, 96.852)
(6103, 99.842)
(6104, 99.408)
(6105, 99.742)
(6106, 99.798)
(6107, 99.96)
(6108, 99.698)
(6109, 99.92)
(6110, 99.802)
(6111, 99.252)
(6112, 99.844)
(6113, 99.78)
(6114, 99.784)
(6115, 99.312)
(6116, 99.152)
(6117, 99.712)
(6118, 98.79)
(6119, 99.722)
(6120, 99.014)
(6121, 99.188)
(6122, 99.472)
(6123, 99.786)
(6124, 99.666)
(6125, 99.72)
(6126, 99.656)
(6127, 99.792)
(6128, 99.948)
(6129, 99.982)
(6130, 99.956)
(6131, 99.896)
(6132, 99.978)
(6133, 99.964)
(6134, 99.854)
(6135, 99.936)
(6136, 99.958)
(6137, 99.916)
(6138, 99.962)
(6139, 99.792)
(6140, 99.844)
(6141, 99.954)
(6142, 99.914)
(6143, 99.974)
(6144, 99.976)
(6145, 99.968)
(6146, 99.81)
(6147, 99.114)
(6148, 98.374)
(6149, 98.636)
(6150, 99.902)
(6151, 99.776)
(6152, 99.722)
(6153, 99.85)
(6154, 99.916)
(6155, 99.482)
(6156, 99.04)
(6157, 99.16)
(6158, 99.158)
(6159, 99.872)
(6160, 99.678)
(6161, 99.624)
(6162, 99.506)
(6163, 99.32)
(6164, 99.72)
(6165, 99.466)
(6166, 99.706)
(6167, 99.886)
(6168, 99.93)
(6169, 99.922)
(6170, 99.74)
(6171, 99.796)
(6172, 99.836)
(6173, 99.694)
(6174, 99.778)
(6175, 99.652)
(6176, 99.574)
(6177, 99.576)
(6178, 99.778)
(6179, 99.606)
(6180, 99.506)
(6181, 98.892)
(6182, 99.842)
(6183, 99.712)
(6184, 99.822)
(6185, 99.448)
(6186, 99.78)
(6187, 96.808)
(6188, 99.528)
(6189, 99.848)
(6190, 99.678)
(6191, 99.71)
(6192, 99.714)
(6193, 99.988)
(6194, 99.946)
(6195, 99.128)
(6196, 99.812)
(6197, 99.99)
(6198, 99.962)
(6199, 99.906)
(6200, 99.928)
(6201, 99.67)
(6202, 99.574)
(6203, 93.734)
(6204, 99.802)
(6205, 99.89)
(6206, 92.09)
(6207, 99.972)
(6208, 99.97)
(6209, 99.934)
(6210, 99.922)
(6211, 99.398)
(6212, 99.778)
(6213, 99.396)
(6214, 99.84)
(6215, 99.992)
(6216, 99.942)
(6217, 99.656)
(6218, 99.834)
(6219, 98.068)
(6220, 99.892)
(6221, 99.938)
(6222, 99.96)
(6223, 99.824)
(6224, 99.604)
(6225, 99.778)
(6226, 99.592)
(6227, 99.916)
(6228, 99.948)
(6229, 99.85)
(6230, 99.806)
(6231, 99.7)
(6232, 99.808)
(6233, 99.568)
(6234, 99.898)
(6235, 98.948)
(6236, 99.808)
(6237, 98.818)
(6238, 99.964)
(6239, 99.936)
(6240, 99.82)
(6241, 99.838)
(6242, 98.146)
(6243, 99.41)
(6244, 99.5)
(6245, 98.634)
(6246, 99.074)
(6247, 98.38)
(6248, 98.068)
(6249, 99.41)
(6250, 98.186)
(6251, 98.38)
(6252, 99.448)
(6253, 97.718)
(6254, 99.47)
(6255, 99.832)
(6256, 99.876)
(6257, 99.126)
(6258, 99.052)
(6259, 99.436)
(6260, 99.632)
(6261, 99.692)
(6262, 99.388)
(6263, 99.918)
(6264, 99.942)
(6265, 98.678)
(6266, 99.576)
(6267, 99.754)
(6268, 99.82)
(6269, 99.794)
(6270, 99.758)
(6271, 99.792)
(6272, 99.598)
(6273, 99.752)
(6274, 99.6)
(6275, 99.562)
(6276, 98.108)
(6277, 99.522)
(6278, 99.648)
(6279, 99.838)
(6280, 98.994)
(6281, 99.842)
(6282, 99.592)
(6283, 97.318)
(6284, 99.332)
(6285, 99.218)
(6286, 98.628)
(6287, 96.804)
(6288, 99.678)
(6289, 99.854)
(6290, 98.724)
(6291, 99.892)
(6292, 99.6)
(6293, 98.278)
(6294, 99.92)
(6295, 99.794)
(6296, 99.496)
(6297, 99.85)
(6298, 99.51)
(6299, 99.592)
(6300, 99.826)
(6301, 99.262)
(6302, 99.812)
(6303, 98.454)
(6304, 99.526)
(6305, 99.246)
(6306, 99.848)
(6307, 99.252)
(6308, 99.476)
(6309, 99.742)
(6310, 99.744)
(6311, 99.826)
(6312, 99.714)
(6313, 99.648)
(6314, 98.458)
(6315, 99.642)
(6316, 99.342)
(6317, 98.898)
(6318, 99.4)
(6319, 99.23)
(6320, 98.976)
(6321, 98.748)
(6322, 99.688)
(6323, 99.148)
(6324, 99.072)
(6325, 99.402)
(6326, 99.204)
(6327, 99.238)
(6328, 99.542)
(6329, 99.592)
(6330, 99.242)
(6331, 99.714)
(6332, 99.97)
(6333, 99.408)
(6334, 99.708)
(6335, 99.828)
(6336, 99.654)
(6337, 99.886)
(6338, 99.818)
(6339, 99.81)
(6340, 99.982)
(6341, 99.87)
(6342, 99.95)
(6343, 99.888)
(6344, 99.58)
(6345, 99.482)
(6346, 99.464)
(6347, 97.884)
(6348, 98.654)
(6349, 99.762)
(6350, 99.35)
(6351, 99.532)
(6352, 99.696)
(6353, 99.418)
(6354, 99.77)
(6355, 99.59)
(6356, 96.07)
(6357, 99.646)
(6358, 99.842)
(6359, 99.488)
(6360, 99.36)
(6361, 98.86)
(6362, 99.614)
(6363, 99.836)
(6364, 99.584)
(6365, 99.564)
(6366, 99.966)
(6367, 99.834)
(6368, 97.94)
(6369, 94.854)
(6370, 95.914)
(6371, 99.986)
(6372, 99.972)
(6373, 99.978)
(6374, 99.944)
(6375, 99.758)
(6376, 99.99)
(6377, 99.988)
(6378, 99.952)
(6379, 99.978)
(6380, 99.978)
(6381, 99.95)
(6382, 99.934)
(6383, 99.832)
(6384, 99.418)
(6385, 99.954)
(6386, 99.932)
(6387, 99.238)
(6388, 99.826)
(6389, 99.54)
(6390, 99.324)
(6391, 98.66)
(6392, 99.11)
(6393, 99.28)
(6394, 93.418)
(6395, 97.544)
(6396, 98.836)
(6397, 96.716)
(6398, 99.736)
(6399, 98.384)
(6400, 99.406)
(6401, 98.63)
(6402, 98.43)
(6403, 98.898)
(6404, 98.442)
(6405, 97.322)
(6406, 98.674)
(6407, 99.27)
(6408, 99.344)
(6409, 97.852)
(6410, 91.388)
(6411, 98.136)
(6412, 98.27)
(6413, 96.724)
(6414, 98.228)
(6415, 93.546)
(6416, 96.734)
(6417, 98.784)
(6418, 98.894)
(6419, 96.192)
(6420, 98.46)
(6421, 98.84)
(6422, 98.452)
(6423, 98.944)
(6424, 98.942)
(6425, 97.088)
(6426, 98.888)
(6427, 97.672)
(6428, 95.842)
(6429, 97.83)
(6430, 97.796)
(6431, 96.666)
(6432, 96.792)
(6433, 97.076)
(6434, 99.406)
(6435, 97.688)
(6436, 95.332)
(6437, 97.304)
(6438, 99.296)
(6439, 98.202)
(6440, 98.024)
(6441, 98.398)
(6442, 98.74)
(6443, 98.018)
(6444, 97.732)
(6445, 96.044)
(6446, 95.598)
(6447, 97.798)
(6448, 98.87)
(6449, 97.046)
(6450, 97.918)
(6451, 98.566)
(6452, 97.732)
(6453, 97.512)
(6454, 98.238)
(6455, 97.528)
(6456, 96.738)
(6457, 96.198)
(6458, 95.404)
(6459, 95.976)
(6460, 95.728)
(6461, 93.854)
(6462, 96.2)
(6463, 98.318)
(6464, 99.552)
(6465, 98.122)
(6466, 97.79)
(6467, 98.212)
(6468, 98.832)
(6469, 98.554)
(6470, 98.546)
(6471, 95.772)
(6472, 98.5)
(6473, 98.212)
(6474, 97.792)
(6475, 96.148)
(6476, 98.784)
(6477, 96.66)
(6478, 98.298)
(6479, 98.936)
(6480, 97.648)
(6481, 98.094)
(6482, 97.992)
(6483, 98.268)
(6484, 97.77)
(6485, 99.114)
(6486, 97.564)
(6487, 97.842)
(6488, 98.236)
(6489, 99.09)
(6490, 99.184)
(6491, 97.584)
(6492, 98.622)
(6493, 99.132)
(6494, 99.698)
(6495, 98.814)
(6496, 98.75)
(6497, 99.588)
(6498, 99.42)
(6499, 99.472)
(6500, 99.766)
(6501, 99.37)
(6502, 99.258)
(6503, 98.168)
(6504, 99.374)
(6505, 99.526)
(6506, 99.08)
(6507, 98.21)
(6508, 96.278)
(6509, 99.318)
(6510, 98.432)
(6511, 99.388)
(6512, 99.37)
(6513, 97.934)
(6514, 98.356)
(6515, 98.532)
(6516, 98.684)
(6517, 98.108)
(6518, 98.616)
(6519, 98.984)
(6520, 99.186)
(6521, 99.414)
(6522, 98.028)
(6523, 99.382)
(6524, 99.516)
(6525, 99.506)
(6526, 99.572)
(6527, 99.534)
(6528, 99.674)
(6529, 99.18)
(6530, 99.656)
(6531, 99.524)
(6532, 99.716)
(6533, 99.772)
(6534, 99.692)
(6535, 99.206)
(6536, 81.596)
(6537, 97.426)
(6538, 96.114)
(6539, 97.176)
(6540, 97.332)
(6541, 95.474)
(6542, 97.41)
(6543, 98.244)
(6544, 98.284)
(6545, 98.52)
(6546, 99.322)
(6547, 97.458)
(6548, 98.844)
(6549, 98.254)
(6550, 94.79)
(6551, 99.552)
(6552, 99.05)
(6553, 99.664)
(6554, 95.652)
(6555, 98.566)
(6556, 98.88)
(6557, 98.46)
(6558, 97.974)
(6559, 99.44)
(6560, 96.73)
(6561, 98.536)
(6562, 97.36)
(6563, 99.018)
(6564, 99.768)
(6565, 99.412)
(6566, 97.644)
(6567, 98.78)
(6568, 99.506)
(6569, 99.554)
(6570, 99.906)
(6571, 99.696)
(6572, 99.742)
(6573, 99.77)
(6574, 99.874)
(6575, 99.802)
(6576, 99.696)
(6577, 96.16)
(6578, 99.83)
(6579, 99.736)
(6580, 99.62)
(6581, 95.944)
(6582, 99.626)
(6583, 97.662)
(6584, 92.81)
(6585, 98.838)
(6586, 98.856)
(6587, 95.058)
(6588, 97.13)
(6589, 99.348)
(6590, 99.286)
(6591, 98.862)
(6592, 99.726)
(6593, 99.212)
(6594, 99.564)
(6595, 99.55)
(6596, 98.9)
(6597, 99.586)
(6598, 99.858)
(6599, 98.216)
(6600, 98.806)
(6601, 99.072)
(6602, 97.92)
(6603, 98.228)
(6604, 99.18)
(6605, 99.226)
(6606, 99.706)
(6607, 99.576)
(6608, 97.01)
(6609, 99.416)
(6610, 99.502)
(6611, 99.868)
(6612, 99.904)
(6613, 99.822)
(6614, 99.558)
(6615, 99.194)
(6616, 97.902)
(6617, 99.67)
(6618, 99.646)
(6619, 99.826)
(6620, 99.772)
(6621, 99.734)
(6622, 99.924)
(6623, 99.89)
(6624, 99.45)
(6625, 99.12)
(6626, 99.512)
(6627, 99.734)
(6628, 99.534)
(6629, 98.84)
(6630, 99.68)
(6631, 99.686)
(6632, 99.774)
(6633, 99.258)
(6634, 99.684)
(6635, 99.734)
(6636, 99.486)
(6637, 99.892)
(6638, 99.934)
(6639, 99.976)
(6640, 99.806)
(6641, 99.572)
(6642, 99.242)
(6643, 98.99)
(6644, 99.078)
(6645, 99.73)
(6646, 99.694)
(6647, 98.94)
(6648, 98.914)
(6649, 99.838)
(6650, 99.622)
(6651, 99.824)
(6652, 99.812)
(6653, 99.728)
(6654, 98.306)
(6655, 97.978)
(6656, 99.188)
(6657, 99.748)
(6658, 98.186)
(6659, 98.642)
(6660, 99.23)
(6661, 99.03)
(6662, 99.322)
(6663, 98.968)
(6664, 98.582)
(6665, 99.47)
(6666, 99.312)
(6667, 98.698)
(6668, 99.332)
(6669, 99.37)
(6670, 98.802)
(6671, 99.37)
(6672, 99.466)
(6673, 98.15)
(6674, 98.938)
(6675, 98.984)
(6676, 99.36)
(6677, 98.49)
(6678, 99.49)
(6679, 99.614)
(6680, 99.816)
(6681, 99.3)
(6682, 99.924)
(6683, 99.954)
(6684, 99.454)
(6685, 99.8)
(6686, 99.46)
(6687, 99.902)
(6688, 99.974)
(6689, 99.854)
(6690, 99.894)
(6691, 99.86)
(6692, 99.972)
(6693, 99.974)
(6694, 99.818)
(6695, 99.858)
(6696, 99.92)
(6697, 99.908)
(6698, 99.868)
(6699, 98.6)
(6700, 99.19)
(6701, 99.7)
(6702, 99.444)
(6703, 99.234)
(6704, 99.928)
(6705, 98.7)
(6706, 97.552)
(6707, 98.458)
(6708, 99.11)
(6709, 98.602)
(6710, 98.048)
(6711, 98.598)
(6712, 97.87)
(6713, 95.676)
(6714, 99.46)
(6715, 98.734)
(6716, 99.084)
(6717, 99.606)
(6718, 99.94)
(6719, 99.914)
(6720, 99.952)
(6721, 99.804)
(6722, 99.936)
(6723, 99.832)
(6724, 99.88)
(6725, 99.858)
(6726, 99.928)
(6727, 99.19)
(6728, 98.448)
(6729, 98.838)
(6730, 99.908)
(6731, 99.946)
(6732, 99.748)
(6733, 99.922)
(6734, 99.714)
(6735, 95.652)
(6736, 98.386)
(6737, 95.722)
(6738, 99.258)
(6739, 99.154)
(6740, 98.912)
(6741, 99.586)
(6742, 98.698)
(6743, 99.75)
(6744, 99.76)
(6745, 99.742)
(6746, 99.408)
(6747, 99.672)
(6748, 99.478)
(6749, 99.594)
(6750, 99.77)
(6751, 99.904)
(6752, 99.74)
(6753, 99.938)
(6754, 99.724)
(6755, 99.774)
(6756, 99.766)
(6757, 99.81)
(6758, 99.842)
(6759, 99.512)
(6760, 99.75)
(6761, 99.536)
(6762, 99.884)
(6763, 99.774)
(6764, 99.884)
(6765, 99.97)
(6766, 99.944)
(6767, 99.87)
(6768, 99.484)
(6769, 99.52)
(6770, 99.546)
(6771, 99.592)
(6772, 99.21)
(6773, 99.174)
(6774, 99.848)
(6775, 99.568)
(6776, 98.334)
(6777, 99.874)
(6778, 97.88)
(6779, 99.482)
(6780, 95.626)
(6781, 98.696)
(6782, 99.706)
(6783, 98.028)
(6784, 99.878)
(6785, 99.72)
(6786, 99.336)
(6787, 99.346)
(6788, 99.678)
(6789, 99.682)
(6790, 99.49)
(6791, 99.664)
(6792, 99.338)
(6793, 98.674)
(6794, 98.288)
(6795, 98.836)
(6796, 98.118)
(6797, 98.67)
(6798, 99.634)
(6799, 99.588)
(6800, 99.494)
(6801, 99.606)
(6802, 99.818)
(6803, 98.326)
(6804, 99.324)
(6805, 99.954)
(6806, 99.894)
(6807, 99.14)
(6808, 98.742)
(6809, 99.584)
(6810, 99.808)
(6811, 98.468)
(6812, 99.604)
(6813, 99.432)
(6814, 99.66)
(6815, 99.61)
(6816, 99.952)
(6817, 99.922)
(6818, 99.97)
(6819, 99.982)
(6820, 99.962)
(6821, 99.986)
(6822, 99.99)
(6823, 99.986)
(6824, 99.77)
(6825, 99.988)
(6826, 99.798)
(6827, 99.984)
(6828, 99.996)
(6829, 100)
(6830, 99.976)
(6831, 99.996)
(6832, 100)
(6833, 99.992)
(6834, 99.902)
(6835, 100)
(6836, 100)
(6837, 100)
(6838, 99.888)
(6839, 99.992)
(6840, 100)
(6841, 100)
(6842, 99.952)
(6843, 99.998)
(6844, 89.486)
(6845, 99.998)
(6846, 99.988)
(6847, 99.96)
(6848, 99.952)
(6849, 98.74)
(6850, 99.992)
(6851, 99.95)
(6852, 99.054)
(6853, 93.09)
(6854, 99.998)
(6855, 99.996)
(6856, 99.998)
(6857, 99.992)
(6858, 99.982)
(6859, 100)
(6860, 100)
(6861, 99.802)
(6862, 99.936)
(6863, 99.998)
(6864, 99.97)
(6865, 99.99)
(6866, 99.994)
(6867, 99.962)
(6868, 100)
(6869, 99.986)
(6870, 99.986)
(6871, 99.996)
(6872, 100)
(6873, 100)
(6874, 100)
(6875, 98.952)
(6876, 99.99)
(6877, 99.984)
(6878, 100)
(6879, 99.984)
(6880, 99.992)
(6881, 100)
(6882, 99.972)
(6883, 99.986)
(6884, 99.9)
(6885, 99.96)
(6886, 99.976)
(6887, 99.946)
(6888, 99.942)
(6889, 99.822)
(6890, 99.916)
(6891, 99.974)
(6892, 99.958)
(6893, 99.968)
(6894, 99.806)
(6895, 99.958)
(6896, 99.966)
(6897, 99.896)
(6898, 99.832)
(6899, 99.94)
(6900, 99.892)
(6901, 99.81)
(6902, 99.84)
(6903, 99.796)
(6904, 99.894)
(6905, 99.828)
(6906, 99.222)
(6907, 99.95)
(6908, 99.872)
(6909, 99.668)
(6910, 99.762)
(6911, 99.596)
(6912, 99.67)
(6913, 99.786)
(6914, 99.6)
(6915, 99.798)
(6916, 99.89)
(6917, 99.69)
(6918, 99.812)
(6919, 99.596)
(6920, 99.856)
(6921, 99.748)
(6922, 99.712)
(6923, 99.908)
(6924, 99.846)
(6925, 99.878)
(6926, 99.906)
(6927, 99.866)
(6928, 99.65)
(6929, 99.936)
(6930, 99.818)
(6931, 99.846)
(6932, 99.628)
(6933, 99.132)
(6934, 99.442)
(6935, 99.792)
(6936, 98.858)
(6937, 98.022)
(6938, 99.262)
(6939, 99.746)
(6940, 99.714)
(6941, 99.612)
(6942, 99.53)
(6943, 99.642)
(6944, 99.672)
(6945, 99.756)
(6946, 99.468)
(6947, 99.73)
(6948, 99.726)
(6949, 99.42)
(6950, 99.75)
(6951, 97.474)
(6952, 99.342)
(6953, 99.016)
(6954, 98.452)
(6955, 97.046)
(6956, 97.178)
(6957, 94.036)
(6958, 96.714)
(6959, 97.912)
(6960, 98.344)
(6961, 98.178)
(6962, 96.97)
(6963, 95.72)
(6964, 98.718)
(6965, 98.566)
(6966, 99.344)
(6967, 99.308)
(6968, 99.294)
(6969, 99.09)
(6970, 98.462)
(6971, 97.994)
(6972, 98.11)
(6973, 98.226)
(6974, 97.976)
(6975, 97.956)
(6976, 98.934)
(6977, 97.814)
(6978, 94.558)
(6979, 96.344)
(6980, 98.816)
(6981, 97.61)
(6982, 98.338)
(6983, 98.106)
(6984, 97.406)
(6985, 97.662)
(6986, 96.26)
(6987, 96.784)
(6988, 96.792)
(6989, 98.448)
(6990, 95.984)
(6991, 96.934)
(6992, 95.846)
(6993, 98.812)
(6994, 99.166)
(6995, 98.544)
(6996, 96.976)
(6997, 98.128)
(6998, 98.568)
(6999, 96.194)
(7000, 96.702)
(7001, 98.76)
(7002, 98.214)
(7003, 97.892)
(7004, 98.526)
(7005, 98.24)
(7006, 97.638)
(7007, 94.164)
(7008, 97.266)
(7009, 98.388)
(7010, 97.108)
(7011, 99.16)
(7012, 98.01)
(7013, 97.576)
(7014, 98.038)
(7015, 97.542)
(7016, 98.56)
(7017, 97.62)
(7018, 97.956)
(7019, 96.298)
(7020, 98.456)
(7021, 97.752)
(7022, 97.984)
(7023, 95.964)
(7024, 96.658)
(7025, 97.468)
(7026, 97.35)
(7027, 97.642)
(7028, 92.002)
(7029, 93.65)
(7030, 97.692)
(7031, 93.406)
(7032, 95.314)
(7033, 96.462)
(7034, 97.626)
(7035, 94.882)
(7036, 92.776)
(7037, 92.95)
(7038, 94.204)
(7039, 88.33)
(7040, 74.128)
(7041, 91.75)
(7042, 84.674)
(7043, 80.872)
(7044, 81.032)
(7045, 83.95)
(7046, 91.324)
(7047, 92.132)
(7048, 95.13)
(7049, 95.062)
(7050, 91.67)
(7051, 93.986)
(7052, 88.99)
(7053, 94.652)
(7054, 90.572)
(7055, 94.798)
(7056, 91.476)
(7057, 96.026)
(7058, 91.766)
(7059, 91.794)
(7060, 95.216)
(7061, 94.978)
(7062, 92.348)
(7063, 92.022)
(7064, 85.394)
(7065, 77.916)
(7066, 85.014)
(7067, 89.782)
(7068, 83.51)
(7069, 95.924)
(7070, 92.266)
(7071, 90.042)
(7072, 78.596)
(7073, 89.604)
(7074, 93.818)
(7075, 90.338)
(7076, 97.506)
(7077, 93.596)
(7078, 90.87)
(7079, 92.766)
(7080, 94.054)
(7081, 91.004)
(7082, 97.48)
(7083, 96.23)
(7084, 89.606)
(7085, 93.424)
(7086, 85.02)
(7087, 95.508)
(7088, 96.072)
(7089, 93.24)
(7090, 91.94)
(7091, 92.644)
(7092, 92.074)
(7093, 89.852)
(7094, 90.104)
(7095, 85.622)
(7096, 91.088)
(7097, 91.832)
(7098, 88.562)
(7099, 81.7)
(7100, 91.226)
(7101, 95.116)
(7102, 94.504)
(7103, 96.05)
(7104, 87.066)
(7105, 92.258)
(7106, 94.99)
(7107, 90.318)
(7108, 80.58)
(7109, 86.466)
(7110, 95.9)
(7111, 88.608)
(7112, 94.078)
(7113, 89.182)
(7114, 88.248)
(7115, 83.52)
(7116, 81.356)
(7117, 94.626)
(7118, 89.38)
(7119, 92.682)
(7120, 92.274)
(7121, 92.466)
(7122, 85.7)
(7123, 97.37)
(7124, 96.126)
(7125, 95.694)
(7126, 94.452)
(7127, 90.494)
(7128, 89.646)
(7129, 91.418)
(7130, 77.96)
(7131, 90.756)
(7132, 87.358)
(7133, 89.352)
(7134, 89.116)
(7135, 96.864)
(7136, 88.294)
(7137, 92.842)
(7138, 84.426)
(7139, 92.85)
(7140, 94.544)
(7141, 94.862)
(7142, 95.452)
(7143, 89.5)
(7144, 92.4)
(7145, 97.61)
(7146, 97.892)
(7147, 94.118)
(7148, 95.47)
(7149, 96.088)
(7150, 98.168)
(7151, 96.032)
(7152, 96.888)
(7153, 96.442)
(7154, 97.766)
(7155, 97.616)
(7156, 97.352)
(7157, 98.178)
(7158, 97.27)
(7159, 99.124)
(7160, 99.358)
(7161, 99.538)
(7162, 99.28)
(7163, 98.384)
(7164, 99.234)
(7165, 99.362)
(7166, 96.728)
(7167, 98.402)
(7168, 98.016)
(7169, 94.9)
(7170, 97.842)
(7171, 94.936)
(7172, 91.234)
(7173, 96.996)
(7174, 96.596)
(7175, 97.17)
(7176, 95.978)
(7177, 94.524)
(7178, 96.334)
(7179, 97.462)
(7180, 99.286)
(7181, 98.74)
(7182, 97.49)
(7183, 97.132)
(7184, 97.244)
(7185, 93.022)
(7186, 95.868)
(7187, 94.602)
(7188, 96.904)
(7189, 95.322)
(7190, 96.392)
(7191, 99.14)
(7192, 96.428)
(7193, 96.276)
(7194, 95.704)
(7195, 98.26)
(7196, 97.312)
(7197, 98.38)
(7198, 95.956)
(7199, 97.02)
(7200, 93.206)
(7201, 97.372)
(7202, 96.154)
(7203, 87.152)
(7204, 95.446)
(7205, 95.098)
(7206, 97.198)
(7207, 97.37)
(7208, 94.976)
(7209, 95.964)
(7210, 90.498)
(7211, 84.256)
(7212, 93.95)
(7213, 96.198)
(7214, 98.842)
(7215, 96.022)
(7216, 97.932)
(7217, 92.986)
(7218, 94.592)
(7219, 98.546)
(7220, 97.992)
(7221, 98.564)
(7222, 96.536)
(7223, 97.546)
(7224, 98.364)
(7225, 98.092)
(7226, 92.014)
(7227, 93.12)
(7228, 89.858)
(7229, 93.302)
(7230, 87.53)
(7231, 96.604)
(7232, 91.092)
(7233, 97.464)
(7234, 86.226)
(7235, 76.368)
(7236, 91.614)
(7237, 92.388)
(7238, 87.938)
(7239, 85.278)
(7240, 69.11)
(7241, 91.074)
(7242, 99.458)
(7243, 99.69)
(7244, 99.838)
(7245, 99.194)
(7246, 95.272)
(7247, 99.128)
(7248, 99.23)
(7249, 98.142)
(7250, 98.942)
(7251, 94.696)
(7252, 97.326)
(7253, 96.376)
(7254, 97.836)
(7255, 96.17)
(7256, 96.298)
(7257, 99.364)
(7258, 99.896)
(7259, 99.882)
(7260, 99.928)
(7261, 99.826)
(7262, 99.836)
(7263, 99.856)
(7264, 99.808)
(7265, 99.79)
(7266, 99.354)
(7267, 99.626)
(7268, 98.82)
(7269, 97.962)
(7270, 99.316)
(7271, 98.938)
(7272, 98.402)
(7273, 98.102)
(7274, 98.984)
(7275, 98.674)
(7276, 98.902)
(7277, 99.44)
(7278, 98.584)
(7279, 99.352)
(7280, 98.87)
(7281, 96.41)
(7282, 97.566)
(7283, 98.252)
(7284, 99.02)
(7285, 98.23)
(7286, 98.796)
(7287, 98.908)
(7288, 95.748)
(7289, 98.12)
(7290, 98.598)
(7291, 99.608)
(7292, 99.882)
(7293, 99.418)
(7294, 98.38)
(7295, 99.348)
(7296, 99.776)
(7297, 99.836)
(7298, 99.942)
(7299, 99.946)
(7300, 98.998)
(7301, 97.956)
(7302, 99.584)
(7303, 99.872)
(7304, 99.758)
(7305, 99.816)
(7306, 99.704)
(7307, 98.308)
(7308, 99.566)
(7309, 99.766)
(7310, 99.664)
(7311, 99.724)
(7312, 99.932)
(7313, 99.882)
(7314, 99.126)
(7315, 97.444)
(7316, 98.774)
(7317, 99.364)
(7318, 98.776)
(7319, 99.138)
(7320, 99.252)
(7321, 98.43)
(7322, 99.398)
(7323, 99.652)
(7324, 99.85)
(7325, 99.86)
(7326, 99.822)
(7327, 99.828)
(7328, 98.584)
(7329, 96.732)
(7330, 98.764)
(7331, 99.44)
(7332, 99.472)
(7333, 99.382)
(7334, 99.764)
(7335, 99.134)
(7336, 98.532)
(7337, 98.464)
(7338, 98.812)
(7339, 99.662)
(7340, 99.852)
(7341, 99.342)
(7342, 97.466)
(7343, 98.404)
(7344, 99.162)
(7345, 98.274)
(7346, 97.07)
(7347, 98.844)
(7348, 98.942)
(7349, 98.342)
(7350, 97.832)
(7351, 98.46)
(7352, 96.978)
(7353, 98.662)
(7354, 98.202)
(7355, 95.984)
(7356, 96.872)
(7357, 98.326)
(7358, 94.956)
(7359, 96.458)
(7360, 96.974)
(7361, 93.916)
(7362, 98.94)
(7363, 98.31)
(7364, 98.504)
(7365, 98.528)
(7366, 97.54)
(7367, 95.024)
(7368, 97.226)
(7369, 92.546)
(7370, 92.538)
(7371, 94.122)
(7372, 95.248)
(7373, 96.452)
(7374, 96.588)
(7375, 96.41)
(7376, 94.652)
(7377, 96.064)
(7378, 96.864)
(7379, 96.528)
(7380, 95.176)
(7381, 96.522)
(7382, 96.292)
(7383, 95.502)
(7384, 96.436)
(7385, 95.238)
(7386, 90.82)
(7387, 95.86)
(7388, 97.908)
(7389, 97.93)
(7390, 94.694)
(7391, 96.354)
(7392, 95.604)
(7393, 93.414)
(7394, 94.482)
(7395, 92.958)
(7396, 96.582)
(7397, 97.326)
(7398, 96.966)
(7399, 89.612)
(7400, 91.334)
(7401, 90.786)
(7402, 91.076)
(7403, 93.206)
(7404, 86.296)
(7405, 85.092)
(7406, 93.014)
(7407, 94.314)
(7408, 95.024)
(7409, 94.24)
(7410, 94.98)
(7411, 97.534)
(7412, 90.502)
(7413, 93.668)
(7414, 94.868)
(7415, 95.388)
(7416, 93.072)
(7417, 97.232)
(7418, 97.022)
(7419, 95.078)
(7420, 95.94)
(7421, 95.922)
(7422, 96.526)
(7423, 95.968)
(7424, 94.814)
(7425, 90.364)
(7426, 92.874)
(7427, 95.302)
(7428, 94.692)
(7429, 89.724)
(7430, 94.612)
(7431, 94.538)
(7432, 94.728)
(7433, 97.538)
(7434, 97.668)
(7435, 97.132)
(7436, 96.09)
(7437, 97.684)
(7438, 97.226)
(7439, 98.336)
(7440, 96.744)
(7441, 95.116)
(7442, 93.512)
(7443, 92.486)
(7444, 91.294)
(7445, 94.028)
(7446, 95.816)
(7447, 97.184)
(7448, 96.14)
(7449, 97.304)
(7450, 98.5)
(7451, 97.134)
(7452, 87.9)
(7453, 93.836)
(7454, 89.744)
(7455, 95.024)
(7456, 94.102)
(7457, 94.432)
(7458, 95.742)
(7459, 92.29)
(7460, 95.2)
(7461, 95.862)
(7462, 91.598)
(7463, 92.608)
(7464, 91.084)
(7465, 88.734)
(7466, 93.644)
(7467, 94.574)
(7468, 96.172)
(7469, 97.022)
(7470, 97.446)
(7471, 93.242)
(7472, 93.914)
(7473, 95.412)
(7474, 91.906)
(7475, 94.698)
(7476, 96.3)
(7477, 97.228)
(7478, 84.842)
(7479, 96.836)
(7480, 95.842)
(7481, 96.816)
(7482, 93.19)
(7483, 95.728)
(7484, 98.212)
(7485, 94.958)
(7486, 80.14)
(7487, 96.562)
(7488, 97.402)
(7489, 96.378)
(7490, 86.536)
(7491, 94.222)
(7492, 86.456)
(7493, 91.912)
(7494, 82.832)
(7495, 94.88)
(7496, 94.254)
(7497, 96.032)
(7498, 96.022)
(7499, 97.912)
(7500, 98.658)
(7501, 97.342)
(7502, 94.814)
(7503, 96.3)
(7504, 98.952)
(7505, 97.998)
(7506, 92.734)
(7507, 96.912)
(7508, 94.826)
(7509, 97.096)
(7510, 86.444)
(7511, 96.646)
(7512, 95.886)
(7513, 83.976)
(7514, 89.854)
(7515, 94.188)
(7516, 92.168)
(7517, 86.982)
(7518, 96.146)
(7519, 95.888)
(7520, 89.54)
(7521, 78.816)
(7522, 86.96)
(7523, 91.348)
(7524, 80.782)
(7525, 85.07)
(7526, 67.024)
(7527, 95.978)
(7528, 80.082)
(7529, 89.78)
(7530, 85.084)
(7531, 99.45)
(7532, 99.89)
(7533, 99.902)
(7534, 99.974)
(7535, 99.938)
(7536, 99.788)
(7537, 99.544)
(7538, 99.388)
(7539, 99.53)
(7540, 97.284)
(7541, 99.192)
(7542, 99.57)
(7543, 99.556)
(7544, 99.268)
(7545, 99.592)
(7546, 99.45)
(7547, 99.646)
(7548, 99.614)
(7549, 99.824)
(7550, 99.946)
(7551, 99.284)
(7552, 98.88)
(7553, 99.134)
(7554, 99.302)
(7555, 99.55)
(7556, 99.278)
(7557, 99.502)
(7558, 99.476)
(7559, 99.268)
(7560, 99.656)
(7561, 98.712)
(7562, 99.032)
(7563, 99.648)
(7564, 99.768)
(7565, 99.772)
(7566, 99.744)
(7567, 99.42)
(7568, 99.718)
(7569, 99.758)
(7570, 99.824)
(7571, 97.974)
(7572, 99.528)
(7573, 99.926)
(7574, 99.992)
(7575, 99.812)
(7576, 99.968)
(7577, 99.526)
(7578, 99.922)
(7579, 99.012)
(7580, 99.796)
(7581, 99.994)
(7582, 99.986)
(7583, 99.972)
(7584, 99.606)
(7585, 99.82)
(7586, 99.422)
(7587, 99.214)
(7588, 99.838)
(7589, 99.81)
(7590, 99.998)
(7591, 100)
(7592, 99.998)
(7593, 100)
(7594, 99.996)
(7595, 100)
(7596, 99.998)
(7597, 100)
(7598, 100)
(7599, 99.996)
(7600, 99.992)
(7601, 99.996)
(7602, 99.992)
(7603, 99.98)
(7604, 99.99)
(7605, 99.978)
(7606, 99.978)
(7607, 99.946)
(7608, 99.048)
(7609, 99.964)
(7610, 99.924)
(7611, 99.914)
(7612, 99.964)
(7613, 99.55)
(7614, 98.61)
(7615, 99.63)
(7616, 99.546)
(7617, 99.548)
(7618, 99.798)
(7619, 99.858)
(7620, 99.836)
(7621, 96.644)
(7622, 97.484)
(7623, 97.158)
(7624, 99.346)
(7625, 99.644)
(7626, 99.224)
(7627, 99.542)
(7628, 98.916)
(7629, 99.412)
(7630, 99.326)
(7631, 99.886)
(7632, 99.546)
(7633, 98.798)
(7634, 99.55)
(7635, 99.488)
(7636, 94.8)
(7637, 99.386)
(7638, 99.5)
(7639, 99.17)
(7640, 98.554)
(7641, 98.916)
(7642, 98.79)
(7643, 97.398)
(7644, 97.61)
(7645, 98.04)
(7646, 99.006)
(7647, 96.668)
(7648, 96.998)
(7649, 97.724)
(7650, 97.964)
(7651, 98.454)
(7652, 98.542)
(7653, 99.404)
(7654, 97.84)
(7655, 97.744)
(7656, 96.332)
(7657, 98.564)
(7658, 98.068)
(7659, 95.964)
(7660, 98.936)
(7661, 97.956)
(7662, 99.36)
(7663, 99.15)
(7664, 99.54)
(7665, 99.284)
(7666, 99.444)
(7667, 99.592)
(7668, 98.85)
(7669, 99.588)
(7670, 99.358)
(7671, 99.428)
(7672, 99.58)
(7673, 99.35)
(7674, 99.368)
(7675, 99.472)
(7676, 99.778)
(7677, 98.684)
(7678, 98.092)
(7679, 99.072)
(7680, 98.63)
(7681, 98.942)
(7682, 99.158)
(7683, 99.242)
(7684, 98.464)
(7685, 97.07)
(7686, 95.152)
(7687, 97.026)
(7688, 98.376)
(7689, 97.3)
(7690, 97.634)
(7691, 96.626)
(7692, 96.626)
(7693, 97.798)
(7694, 97.404)
(7695, 94.406)
(7696, 95.68)
(7697, 96.69)
(7698, 96.746)
(7699, 95.464)
(7700, 95.616)
(7701, 95.116)
(7702, 98.138)
(7703, 98.52)
(7704, 96.866)
(7705, 89.07)
(7706, 90.588)
(7707, 98.33)
(7708, 97.754)
(7709, 97.486)
(7710, 97.768)
(7711, 98.04)
(7712, 94.574)
(7713, 96.866)
(7714, 95.788)
(7715, 97.966)
(7716, 99.224)
(7717, 97.832)
(7718, 97.134)
(7719, 97.24)
(7720, 98.078)
(7721, 93.34)
(7722, 98.132)
(7723, 98.292)
(7724, 96.092)
(7725, 96.604)
(7726, 96.442)
(7727, 98.254)
(7728, 99.024)
(7729, 98.456)
(7730, 98.174)
(7731, 97.968)
(7732, 97.012)
(7733, 97.35)
(7734, 96.612)
(7735, 97.834)
(7736, 98.38)
(7737, 97.574)
(7738, 97.098)
(7739, 98.342)
(7740, 92.782)
(7741, 96.066)
(7742, 94.376)
(7743, 94.67)
(7744, 97.012)
(7745, 97.03)
(7746, 98.648)
(7747, 99.322)
(7748, 98.848)
(7749, 95.33)
(7750, 97.768)
(7751, 90.912)
(7752, 93.4)
(7753, 92.556)
(7754, 97.246)
(7755, 96.242)
(7756, 97.508)
(7757, 96.918)
(7758, 97.582)
(7759, 94.332)
(7760, 94.524)
(7761, 97.51)
(7762, 92.98)
(7763, 96.766)
(7764, 97.768)
(7765, 95.896)
(7766, 94.256)
(7767, 97.136)
(7768, 97.294)
(7769, 96.23)
(7770, 96.556)
(7771, 95.262)
(7772, 97.634)
(7773, 91.508)
(7774, 98.602)
(7775, 96.068)
(7776, 98.99)
(7777, 98.424)
(7778, 97.312)
(7779, 94.244)
(7780, 97.556)
(7781, 96.432)
(7782, 96.028)
(7783, 97.114)
(7784, 96.878)
(7785, 94.836)
(7786, 96.694)
(7787, 95.98)
(7788, 96.9)
(7789, 98.466)
(7790, 97.444)
(7791, 98.604)
(7792, 98.796)
(7793, 98.35)
(7794, 98.374)
(7795, 96.722)
(7796, 98.346)
(7797, 98.646)
(7798, 98.604)
(7799, 98.074)
(7800, 98.414)
(7801, 97.384)
(7802, 93.53)
(7803, 96.876)
(7804, 94.568)
(7805, 93.318)
(7806, 96.028)
(7807, 96.622)
(7808, 96.534)
(7809, 95.226)
(7810, 90.198)
(7811, 93.926)
(7812, 90.024)
(7813, 80.71)
(7814, 77.306)
(7815, 72.954)
(7816, 78.588)
(7817, 92.786)
(7818, 88.266)
(7819, 91.298)
(7820, 84.66)
(7821, 93.214)
(7822, 90.922)
(7823, 84.686)
(7824, 88.13)
(7825, 76.016)
(7826, 92.056)
(7827, 83.44)
(7828, 85.534)
(7829, 87.21)
(7830, 62.686)
(7831, 52.09)
(7832, 65.21)
(7833, 86.932)
(7834, 79.094)
(7835, 85.078)
(7836, 81.728)
(7837, 74.992)
(7838, 54.674)
(7839, 69.978)
(7840, 76.32)
(7841, 83.306)
(7842, 71.068)
(7843, 64.476)
(7844, 43)
(7845, 28.83)
(7846, 21.12)
(7847, 47.962)
(7848, 57.35)
(7849, 58.084)
(7850, 57.984)
(7851, 28.792)
(7852, 34.686)
(7853, 26.608)
(7854, 69.168)
(7855, 37.03)
(7856, 28.458)
(7857, 47.766)
(7858, 31.09)
(7859, 17.888)
(7860, 6.914)
(7861, 16.314)
(7862, 23.08)
(7863, 7.832)
(7864, 3.782)
(7865, 21.274)
(7866, 6.918)
(7867, 0)
(7868, 8.01)
(7869, 35.344)
(7870, 24.254)
(7871, 20.6)
(7872, 16.352)
(7873, 18.976)
(7874, 26.468)
(7875, 17.832)
(7876, 0.218)
(7877, 38.348)
(7878, 48.628)
(7879, 66.398)
(7880, 91.056)
(7881, 99.216)
(7882, 90.006)
(7883, 86.58)
(7884, 87.7)
(7885, 99.06)
(7886, 99.826)
(7887, 84.858)
(7888, 89.86)
(7889, 80.5)
(7890, 90.162)
(7891, 80.916)
(7892, 90.822)
(7893, 74.864)
(7894, 77.11)
(7895, 86.214)
(7896, 84.024)
(7897, 64.632)
(7898, 66.384)
(7899, 63.76)
(7900, 77.61)
(7901, 62.648)
(7902, 71.1)
(7903, 35.102)
(7904, 62.648)
(7905, 40.432)
(7906, 58.618)
(7907, 20.146)
(7908, 53.072)
(7909, 50.068)
(7910, 27.48)
(7911, 53.614)
(7912, 67.584)
(7913, 67.326)
(7914, 86.352)
(7915, 85.284)
(7916, 90.588)
(7917, 65.152)
(7918, 61.182)
(7919, 92.606)
(7920, 81.256)
(7921, 91.912)
(7922, 91.576)
(7923, 90.182)
(7924, 90.684)
(7925, 90.298)
(7926, 80.548)
(7927, 89.486)
(7928, 86.418)
(7929, 90.636)
(7930, 89.946)
(7931, 93.976)
(7932, 90.922)
(7933, 89.476)
(7934, 80.098)
(7935, 88.704)
(7936, 80.532)
(7937, 88.782)
(7938, 87.34)
(7939, 91.396)
(7940, 84.284)
(7941, 85.954)
(7942, 87.338)
(7943, 90.444)
(7944, 89.67)
(7945, 91.868)
(7946, 79.922)
(7947, 88.98)
(7948, 85.968)
(7949, 94.222)
(7950, 95.432)
(7951, 94.806)
(7952, 96.406)
(7953, 96.318)
(7954, 94.908)
(7955, 96.372)
(7956, 95.196)
(7957, 95.366)
(7958, 93.352)
(7959, 92.19)
(7960, 96.188)
(7961, 96.424)
(7962, 94.982)
(7963, 95.114)
(7964, 92.796)
(7965, 94.698)
(7966, 94.59)
(7967, 92.9)
(7968, 98.374)
(7969, 93.406)
(7970, 96.166)
(7971, 93.064)
(7972, 97.532)
(7973, 95.548)
(7974, 97.046)
(7975, 94.246)
(7976, 92.378)
(7977, 97.776)
(7978, 97.454)
(7979, 96.482)
(7980, 95.724)
(7981, 96.554)
(7982, 96.918)
(7983, 89.638)
(7984, 96.936)
(7985, 94.212)
(7986, 94.336)
(7987, 92.988)
(7988, 95.408)
(7989, 94.662)
(7990, 94.818)
(7991, 92.996)
(7992, 80.9)
(7993, 93.648)
(7994, 90.774)
(7995, 92.042)
(7996, 97.468)
(7997, 98.46)
(7998, 98.54)
(7999, 94.646)
(8000, 96.9)
(8001, 99.144)
(8002, 96.936)
(8003, 94.548)
(8004, 94.238)
(8005, 98.066)
(8006, 97.01)
(8007, 97.628)
(8008, 92.908)
(8009, 92.134)
(8010, 96.542)
(8011, 97.514)
(8012, 96.334)
(8013, 97.458)
(8014, 98.024)
(8015, 95.832)
(8016, 98.212)
(8017, 96.52)
(8018, 97.21)
(8019, 94.464)
(8020, 95.7)
(8021, 92.036)
(8022, 96.774)
(8023, 96.45)
(8024, 96.544)
(8025, 96.298)
(8026, 96.512)
(8027, 97.026)
(8028, 98.584)
(8029, 96.668)
(8030, 98.482)
(8031, 97.48)
(8032, 97.088)
(8033, 98.488)
(8034, 97.288)
(8035, 98.026)
(8036, 95.882)
(8037, 98.254)
(8038, 99.148)
(8039, 99.01)
(8040, 98.276)
(8041, 98.646)
(8042, 99.26)
(8043, 94.552)
(8044, 98.698)
(8045, 98.682)
(8046, 98.348)
(8047, 97.814)
(8048, 99.474)
(8049, 99.174)
(8050, 98.238)
(8051, 97.972)
(8052, 95.69)
(8053, 94.898)
(8054, 97.5)
(8055, 98.448)
(8056, 97.788)
(8057, 97.17)
(8058, 98.31)
(8059, 98.26)
(8060, 98.494)
(8061, 94.076)
(8062, 98.012)
(8063, 98.366)
(8064, 97.748)
(8065, 99.324)
(8066, 95.712)
(8067, 82.19)
(8068, 98.594)
(8069, 99.89)
(8070, 99.774)
(8071, 83.252)
(8072, 99.316)
(8073, 99.742)
(8074, 99.806)
(8075, 99.896)
(8076, 94.5)
(8077, 99.552)
(8078, 99.98)
(8079, 99.97)
(8080, 99.98)
(8081, 96.222)
(8082, 99.842)
(8083, 99.956)
(8084, 99.986)
(8085, 100)
(8086, 99.994)
(8087, 99.98)
(8088, 99.998)
(8089, 99.998)
(8090, 99.358)
(8091, 99.886)
(8092, 99.976)
(8093, 99.916)
(8094, 99.824)
(8095, 99.91)
(8096, 99.912)
(8097, 99.942)
(8098, 99.944)
(8099, 97.36)
(8100, 99.866)
(8101, 99.838)
(8102, 99.984)
(8103, 99.496)
(8104, 97.688)
(8105, 99.668)
(8106, 99.502)
(8107, 99.24)
(8108, 99.788)
(8109, 99.824)
(8110, 99.86)
(8111, 99.91)
(8112, 99.914)
(8113, 99.266)
(8114, 99.688)
(8115, 99.662)
(8116, 99.774)
(8117, 99.598)
(8118, 99.942)
(8119, 99.962)
(8120, 99.982)
(8121, 99.924)
(8122, 99.766)
(8123, 99.902)
(8124, 99.806)
(8125, 99.93)
(8126, 99.75)
(8127, 99.704)
(8128, 99.29)
(8129, 99.288)
(8130, 99.116)
(8131, 98.588)
(8132, 99.604)
(8133, 99.696)
(8134, 99.906)
(8135, 99.8)
(8136, 99.334)
(8137, 98.472)
(8138, 99.204)
(8139, 98.98)
(8140, 98.894)
(8141, 96.168)
(8142, 98.476)
(8143, 98.78)
(8144, 98.618)
(8145, 99.104)
(8146, 99.452)
(8147, 99.61)
(8148, 99.726)
(8149, 99.514)
(8150, 99.164)
(8151, 99.258)
(8152, 98.96)
(8153, 99.658)
(8154, 99.592)
(8155, 99.75)
(8156, 99.414)
(8157, 98.984)
(8158, 98.312)
(8159, 98.608)
(8160, 97.536)
(8161, 97.528)
(8162, 95.618)
(8163, 97.822)
(8164, 98.644)
(8165, 98.198)
(8166, 97.732)
(8167, 98.216)
(8168, 97.766)
(8169, 97.69)
(8170, 99.304)
(8171, 99.374)
(8172, 98.528)
(8173, 98.19)
(8174, 98.992)
(8175, 97.978)
(8176, 97.552)
(8177, 98.434)
(8178, 88.534)
(8179, 95.902)
(8180, 98.624)
(8181, 98.922)
(8182, 99.038)
(8183, 97.768)
(8184, 85.744)
(8185, 93.094)
(8186, 98.042)
(8187, 98.77)
(8188, 98.378)
(8189, 97.7)
(8190, 98.972)
(8191, 99.294)
(8192, 98.12)
(8193, 98.966)
(8194, 98.87)
(8195, 98.188)
(8196, 99.206)
(8197, 98.302)
(8198, 98.134)
(8199, 98.596)
(8200, 98.284)
(8201, 98.648)
(8202, 98.29)
(8203, 96.684)
(8204, 98.586)
(8205, 97.866)
(8206, 98.94)
(8207, 99.16)
(8208, 99.1)
(8209, 97.738)
(8210, 98.67)
(8211, 98.172)
(8212, 98.01)
(8213, 99.21)
(8214, 98.97)
(8215, 98.482)
(8216, 97.838)
(8217, 98.756)
(8218, 96.402)
(8219, 99.128)
(8220, 98.924)
(8221, 99.278)
(8222, 99.348)
(8223, 98.872)
(8224, 98.708)
(8225, 97.308)
(8226, 91.948)
(8227, 97.382)
(8228, 97.282)
(8229, 98.74)
(8230, 98.408)
(8231, 98.784)
(8232, 99.414)
(8233, 97.942)
(8234, 98.594)
(8235, 96.764)
(8236, 98.11)
(8237, 97.258)
(8238, 97.546)
(8239, 95.42)
(8240, 96.858)
(8241, 89.622)
(8242, 95.432)
(8243, 96.182)
(8244, 97.436)
(8245, 95.062)
(8246, 84.104)
(8247, 94.514)
(8248, 90.138)
(8249, 97.05)
(8250, 96.154)
(8251, 94.932)
(8252, 97.362)
(8253, 93.118)
(8254, 95.056)
(8255, 94.352)
(8256, 91.932)
(8257, 88.69)
(8258, 86.576)
(8259, 93.018)
(8260, 95.112)
(8261, 96.532)
(8262, 95.804)
(8263, 95.64)
(8264, 92.954)
(8265, 93.978)
(8266, 93.546)
(8267, 95.386)
(8268, 96.178)
(8269, 94.21)
(8270, 96.61)
(8271, 96.656)
(8272, 92.302)
(8273, 94.526)
(8274, 93.534)
(8275, 92.562)
(8276, 78.294)
(8277, 93.706)
(8278, 87.408)
(8279, 90.984)
(8280, 93.192)
(8281, 87.958)
(8282, 84.048)
(8283, 93.998)
(8284, 92.572)
(8285, 92.442)
(8286, 94.146)
(8287, 89.106)
(8288, 94.114)
(8289, 92.15)
(8290, 93.478)
(8291, 94.036)
(8292, 92.146)
(8293, 96.384)
(8294, 95.802)
(8295, 91.846)
(8296, 97.466)
(8297, 90.496)
(8298, 89.82)
(8299, 90.708)
(8300, 92.896)
(8301, 95.782)
(8302, 94.834)
(8303, 91.186)
(8304, 94.95)
(8305, 93.032)
(8306, 94.122)
(8307, 93.044)
(8308, 93.796)
(8309, 93.646)
(8310, 91.058)
(8311, 94.116)
(8312, 96.474)
(8313, 95.088)
(8314, 91.158)
(8315, 95.882)
(8316, 98.278)
(8317, 96.08)
(8318, 96.042)
(8319, 96.542)
(8320, 96.88)
(8321, 97.038)
(8322, 96.338)
(8323, 94.58)
(8324, 97.692)
(8325, 97.412)
(8326, 97.314)
(8327, 97.606)
(8328, 97.458)
(8329, 88.958)
(8330, 99.27)
(8331, 99.628)
(8332, 99.168)
(8333, 87.418)
(8334, 99.544)
(8335, 99.018)
(8336, 99.802)
(8337, 99.81)
(8338, 99.354)
(8339, 87.19)
(8340, 99.724)
(8341, 99.486)
(8342, 99.256)
(8343, 99.594)
(8344, 99.814)
(8345, 99.648)
(8346, 99.666)
(8347, 98.25)
(8348, 86.972)
(8349, 90.588)
(8350, 97.874)
(8351, 98.46)
(8352, 98.638)
(8353, 99.338)
(8354, 98.22)
(8355, 99.622)
(8356, 99.458)
(8357, 99.412)
(8358, 99.73)
(8359, 99.376)
(8360, 98.922)
(8361, 98.84)
(8362, 99.184)
(8363, 99.27)
(8364, 98.88)
(8365, 98.634)
(8366, 99.332)
(8367, 99.314)
(8368, 99.018)
(8369, 99.238)
(8370, 99.71)
(8371, 99.206)
(8372, 99.19)
(8373, 99.342)
(8374, 98.082)
(8375, 99.666)
(8376, 99.882)
(8377, 98.952)
(8378, 98.274)
(8379, 95.844)
(8380, 92.326)
(8381, 96.522)
(8382, 95.882)
(8383, 93.048)
(8384, 91.616)
(8385, 98.092)
(8386, 97.556)
(8387, 96.576)
(8388, 98.212)
(8389, 99.074)
(8390, 97.708)
(8391, 96.684)
(8392, 96.732)
(8393, 97.716)
(8394, 96.44)
(8395, 99.304)
(8396, 99.462)
(8397, 98.78)
(8398, 98.282)
(8399, 99.272)
(8400, 98.526)
(8401, 98.41)
(8402, 98.856)
(8403, 97.066)
(8404, 96.814)
(8405, 94.454)
(8406, 94.096)
(8407, 95.264)
(8408, 94.762)
(8409, 96.728)
(8410, 97.358)
(8411, 99.08)
(8412, 98.958)
(8413, 98.93)
(8414, 99.668)
(8415, 95.952)
(8416, 88.044)
(8417, 99.526)
(8418, 99.404)
(8419, 99.764)
(8420, 99.928)
(8421, 95.388)
(8422, 99.832)
(8423, 99.686)
(8424, 99.768)
(8425, 99.642)
(8426, 99.602)
(8427, 99.632)
(8428, 98.946)
(8429, 98.844)
(8430, 98.068)
(8431, 97.428)
(8432, 98.76)
(8433, 98.932)
(8434, 96.688)
(8435, 98.396)
(8436, 97.164)
(8437, 99.334)
(8438, 99.386)
(8439, 95.95)
(8440, 98.78)
(8441, 98.604)
(8442, 96.982)
(8443, 97.756)
(8444, 92.082)
(8445, 90.754)
(8446, 97.482)
(8447, 94.734)
(8448, 95.85)
(8449, 91.444)
(8450, 97.352)
(8451, 97.306)
(8452, 94.272)
(8453, 96.63)
(8454, 97.252)
(8455, 96.13)
(8456, 97.114)
(8457, 97.046)
(8458, 97.126)
(8459, 96.724)
(8460, 96.074)
(8461, 93.778)
(8462, 94.8)
(8463, 96.198)
(8464, 96.182)
(8465, 94.978)
(8466, 95.288)
(8467, 94.214)
(8468, 82.182)
(8469, 89.25)
(8470, 77.618)
(8471, 90.65)
(8472, 93.846)
(8473, 90.398)
(8474, 93.27)
(8475, 94.288)
(8476, 94.248)
(8477, 94.622)
(8478, 95.034)
(8479, 94.664)
(8480, 94.814)
(8481, 91.176)
(8482, 91.154)
(8483, 89.732)
(8484, 93.274)
(8485, 94.56)
(8486, 95.262)
(8487, 95.206)
(8488, 95.364)
(8489, 94.084)
(8490, 90.286)
(8491, 86.734)
(8492, 92.762)
(8493, 95.52)
(8494, 91.346)
(8495, 93.548)
(8496, 86.952)
(8497, 96.938)
(8498, 97.532)
(8499, 97.914)
(8500, 96.864)
(8501, 93.134)
(8502, 93.792)
(8503, 96.402)
(8504, 94.6)
(8505, 95.752)
(8506, 92.9)
(8507, 92.218)
(8508, 93.22)
(8509, 96.366)
(8510, 93.078)
(8511, 95.46)
(8512, 95.322)
(8513, 81.08)
(8514, 95.938)
(8515, 97.226)
(8516, 98.066)
(8517, 98.298)
(8518, 98.678)
(8519, 97.22)
(8520, 94.876)
(8521, 96.606)
(8522, 97.784)
(8523, 95.696)
(8524, 93.312)
(8525, 96.638)
(8526, 95.708)
(8527, 95.442)
(8528, 92.21)
(8529, 94.684)
(8530, 95.612)
(8531, 95.194)
(8532, 97.524)
(8533, 98.146)
(8534, 98.406)
(8535, 95.852)
(8536, 96.168)
(8537, 96.056)
(8538, 93.59)
(8539, 92.44)
(8540, 90.276)
(8541, 93.256)
(8542, 87.652)
(8543, 94.416)
(8544, 92.048)
(8545, 87.508)
(8546, 97.476)
(8547, 97.092)
(8548, 97.408)
(8549, 96.174)
(8550, 94.096)
(8551, 95.284)
(8552, 97.092)
(8553, 94.73)
(8554, 91.358)
(8555, 93.668)
(8556, 91.63)
(8557, 82.842)
(8558, 89.726)
(8559, 96.606)
(8560, 97.826)
(8561, 97.404)
(8562, 92.422)
(8563, 86.026)
(8564, 92.69)
(8565, 89.77)
(8566, 93.012)
(8567, 86.382)
(8568, 78.092)
(8569, 72.638)
(8570, 93.422)
(8571, 94.33)
(8572, 88.874)
(8573, 93.666)
(8574, 92.084)
(8575, 78.526)
(8576, 83.36)
(8577, 83.182)
(8578, 69.772)
(8579, 76.534)
(8580, 73.848)
(8581, 82.624)
(8582, 92.334)
(8583, 90.782)
(8584, 95.596)
(8585, 88.59)
(8586, 91.666)
(8587, 93.306)
(8588, 77.364)
(8589, 94.114)
(8590, 93.262)
(8591, 87.628)
(8592, 88.134)
(8593, 92.886)
(8594, 87.366)
(8595, 73.53)
(8596, 90.112)
(8597, 86.798)
(8598, 85.832)
(8599, 87.894)
(8600, 87.214)
(8601, 90.246)
(8602, 76.014)
(8603, 76.392)
(8604, 95.814)
(8605, 90.362)
(8606, 83.744)
(8607, 88.228)
(8608, 85.298)
(8609, 94.064)
(8610, 90.858)
(8611, 93.79)
(8612, 92.796)
(8613, 92.872)
(8614, 87.198)
(8615, 94.312)
(8616, 95.636)
(8617, 94.424)
(8618, 92.454)
(8619, 94.012)
(8620, 95.434)
(8621, 93.65)
(8622, 93.054)
(8623, 91.118)
(8624, 85.88)
(8625, 84.43)
(8626, 86.416)
(8627, 65.012)
(8628, 78.002)
(8629, 37.524)
(8630, 72.88)
(8631, 80.612)
(8632, 52.46)
(8633, 81.152)
(8634, 74.746)
(8635, 70.554)
(8636, 44.522)
(8637, 74.154)
(8638, 71.942)
(8639, 56.804)
(8640, 86.634)
(8641, 65.096)
(8642, 80.174)
(8643, 92.364)
(8644, 93.188)
(8645, 85.308)
(8646, 95.398)
(8647, 82.248)
(8648, 83.676)
(8649, 98.322)
(8650, 98.066)
(8651, 94.756)
(8652, 94.934)
(8653, 97.816)
(8654, 97.392)
(8655, 95.998)
(8656, 97.638)
(8657, 98.416)
(8658, 97.878)
(8659, 95.684)
(8660, 97.914)
(8661, 95.476)
(8662, 96.182)
(8663, 96.86)
(8664, 97.17)
(8665, 94.716)
(8666, 97.39)
(8667, 98.022)
(8668, 87.794)
(8669, 95.554)
(8670, 98.138)
(8671, 98.33)
(8672, 97.802)
(8673, 97.082)
(8674, 91.972)
(8675, 97.238)
(8676, 95.402)
(8677, 97.9)
(8678, 97.982)
(8679, 97.64)
(8680, 96.522)
(8681, 96.67)
(8682, 96.93)
(8683, 98.956)
(8684, 99.082)
(8685, 98.874)
(8686, 97.718)
(8687, 96.058)
(8688, 97.616)
(8689, 95.664)
(8690, 97.92)
(8691, 97.2)
(8692, 98.676)
(8693, 99.162)
(8694, 99.138)
(8695, 98.314)
(8696, 98.558)
(8697, 98.794)
(8698, 97.984)
(8699, 99.12)
(8700, 99.642)
(8701, 99.778)
(8702, 99.244)
(8703, 99.514)
(8704, 99.11)
(8705, 99.302)
(8706, 97.96)
(8707, 97.906)
(8708, 96.92)
(8709, 98.898)
(8710, 98.378)
(8711, 98.974)
(8712, 99.334)
(8713, 98.754)
(8714, 98.004)
(8715, 99.108)
(8716, 99.33)
(8717, 99.298)
(8718, 98.968)
(8719, 97.186)
(8720, 98.99)
(8721, 97.088)
(8722, 97.51)
(8723, 97.418)
(8724, 94.246)
(8725, 96.128)
(8726, 96.49)
(8727, 97.34)
(8728, 97.752)
(8729, 98.154)
(8730, 97.178)
(8731, 98.52)
(8732, 99.118)
(8733, 97.308)
(8734, 95.736)
(8735, 96.518)
(8736, 92.086)
(8737, 95.394)
(8738, 97.36)
(8739, 96.96)
(8740, 95.964)
(8741, 94.408)
(8742, 97.708)
(8743, 98.446)
(8744, 98.45)
(8745, 97.66)
(8746, 95.998)
(8747, 98.23)
(8748, 97.464)
(8749, 97.932)
(8750, 90.638)
(8751, 96.104)
(8752, 94.312)
(8753, 86.752)
(8754, 95.798)
(8755, 91.322)
(8756, 95.064)
(8757, 92.018)
(8758, 89.994)
(8759, 86.36)
(8760, 93.582)
(8761, 93.4)
(8762, 94.026)
(8763, 96.582)
(8764, 95.27)
(8765, 94.718)
(8766, 92.71)
(8767, 94.874)
(8768, 84.628)
(8769, 92.478)
(8770, 88.064)
(8771, 87.528)
(8772, 81.284)
(8773, 87.396)
(8774, 81.876)
(8775, 92.728)
(8776, 93.386)
(8777, 77.184)
(8778, 89.692)
(8779, 93.44)
(8780, 92.076)
(8781, 94.164)
(8782, 84.044)
(8783, 91.956)
(8784, 68.01)
(8785, 76.096)
(8786, 67.28)
(8787, 83.176)
(8788, 81.122)
(8789, 83.7)
(8790, 91.45)
(8791, 85.056)
(8792, 87.528)
(8793, 87.322)
(8794, 84.974)
(8795, 87.646)
(8796, 93.512)
(8797, 92.254)
(8798, 90.664)
(8799, 92.336)
(8800, 89.766)
(8801, 94.966)
(8802, 95.722)
(8803, 94.26)
(8804, 95.834)
(8805, 97.458)
(8806, 96.17)
(8807, 93.436)
(8808, 96.686)
(8809, 95.52)
(8810, 93.45)
(8811, 95.74)
(8812, 93.77)
(8813, 97.4)
(8814, 97.536)
(8815, 94.216)
(8816, 99.196)
(8817, 99.06)
(8818, 88.468)
(8819, 98.866)
(8820, 98.436)
(8821, 98.016)
(8822, 97.836)
(8823, 97.936)
(8824, 97.78)
(8825, 97.482)
(8826, 98.576)
(8827, 99.056)
(8828, 99.454)
(8829, 99.396)
(8830, 97.73)
(8831, 98.262)
(8832, 98.966)
(8833, 98.062)
(8834, 96.554)
(8835, 99.29)
(8836, 98.934)
(8837, 97.886)
(8838, 96.368)
(8839, 97.764)
(8840, 98.232)
(8841, 93.434)
(8842, 97.13)
(8843, 95.35)
(8844, 98.414)
(8845, 99.568)
(8846, 98.722)
(8847, 97.108)
(8848, 98.708)
(8849, 99.586)
(8850, 99.752)
(8851, 99.672)
(8852, 98.246)
(8853, 94.976)
(8854, 98.432)
(8855, 99.32)
(8856, 97.956)
(8857, 98.506)
(8858, 98.432)
(8859, 98.78)
(8860, 97.778)
(8861, 98.458)
(8862, 97.086)
(8863, 97.668)
(8864, 97.304)
(8865, 95.348)
(8866, 97.552)
(8867, 98.674)
(8868, 98.624)
(8869, 98.316)
(8870, 91.922)
(8871, 99.304)
(8872, 99.408)
(8873, 99.136)
(8874, 98.202)
(8875, 98.718)
(8876, 97.724)
(8877, 97.334)
(8878, 98.918)
(8879, 92.57)
(8880, 98.352)
(8881, 98.406)
(8882, 97.9)
(8883, 97.11)
(8884, 96.65)
(8885, 97.84)
(8886, 96.302)
(8887, 95.688)
(8888, 96.224)
(8889, 95.032)
(8890, 98.68)
(8891, 99.024)
(8892, 99.006)
(8893, 98.828)
(8894, 98.396)
(8895, 98.826)
(8896, 98.172)
(8897, 98.732)
(8898, 98.872)
(8899, 98.276)
(8900, 96.92)
(8901, 88.094)
(8902, 95.788)
(8903, 98.834)
(8904, 97.628)
(8905, 98.448)
(8906, 98.268)
(8907, 98.334)
(8908, 97.53)
(8909, 95.12)
(8910, 98.244)
(8911, 98.082)
(8912, 96.232)
(8913, 96.812)
(8914, 98.686)
(8915, 98.938)
(8916, 98.412)
(8917, 97.716)
(8918, 96.912)
(8919, 93.85)
(8920, 95.332)
(8921, 98.588)
(8922, 96.7)
(8923, 97.442)
(8924, 96.93)
(8925, 95.032)
(8926, 96.002)
(8927, 96.744)
(8928, 96.288)
(8929, 98.24)
(8930, 97.934)
(8931, 96.956)
(8932, 95.372)
(8933, 98.038)
(8934, 96.87)
(8935, 97.464)
(8936, 96.4)
(8937, 97.338)
(8938, 98.044)
(8939, 97.444)
(8940, 96.146)
(8941, 98.814)
(8942, 97.876)
(8943, 94.818)
(8944, 96.854)
(8945, 95.932)
(8946, 98.622)
(8947, 99.1)
(8948, 99.382)
(8949, 99.472)
(8950, 99.256)
(8951, 97.944)
(8952, 98.644)
(8953, 99.006)
(8954, 97.746)
(8955, 99.256)
(8956, 99.186)
(8957, 99.124)
(8958, 95.18)
(8959, 94.866)
(8960, 97.076)
(8961, 96.012)
(8962, 95.616)
(8963, 96.206)
(8964, 95.31)
(8965, 91.028)
(8966, 95.406)
(8967, 97.096)
(8968, 96.186)
(8969, 95.35)
(8970, 96.65)
(8971, 93.812)
(8972, 92.158)
(8973, 95.652)
(8974, 95.352)
(8975, 94.658)
(8976, 96.438)
(8977, 96.78)
(8978, 90.046)
(8979, 95.376)
(8980, 88.976)
(8981, 93.202)
(8982, 94.766)
(8983, 94.29)
(8984, 95.406)
(8985, 95.874)
(8986, 87.952)
(8987, 89.13)
(8988, 93.838)
(8989, 94.154)
(8990, 96.28)
(8991, 95.308)
(8992, 97.53)
(8993, 96.996)
(8994, 92.656)
(8995, 97.184)
(8996, 97.208)
(8997, 96.364)
(8998, 92.258)
(8999, 95.402)
(9000, 97.088)
(9001, 88.568)
(9002, 90.82)
(9003, 97.032)
(9004, 98.288)
(9005, 97.724)
(9006, 97.88)
(9007, 98.61)
(9008, 97.008)
(9009, 97.43)
(9010, 98.454)
(9011, 70.658)
(9012, 98.624)
(9013, 97.57)
(9014, 93.084)
(9015, 93.418)
(9016, 95.586)
(9017, 92.606)
(9018, 94.65)
(9019, 85.208)
(9020, 63.848)
(9021, 83.518)
(9022, 86.348)
(9023, 85.09)
(9024, 82.664)
(9025, 90.55)
(9026, 86.442)
(9027, 66.528)
(9028, 69.318)
(9029, 93.336)
(9030, 78.558)
(9031, 86.43)
(9032, 96.204)
(9033, 87.746)
(9034, 97.046)
(9035, 93.594)
(9036, 96.168)
(9037, 93.282)
(9038, 90.794)
(9039, 91.012)
(9040, 94.166)
(9041, 91.834)
(9042, 83.034)
(9043, 75.142)
(9044, 92.184)
(9045, 90.428)
(9046, 96.164)
(9047, 92.622)
(9048, 90.804)
(9049, 89.588)
(9050, 82.836)
(9051, 81.748)
(9052, 88.632)
(9053, 89.33)
(9054, 88.79)
(9055, 86.96)
(9056, 82.888)
(9057, 90.814)
(9058, 77.454)
(9059, 93.292)
(9060, 91.448)
(9061, 64.596)
(9062, 77.962)
(9063, 86.222)
(9064, 93.07)
(9065, 93.672)
(9066, 92.716)
(9067, 95.462)
(9068, 94.058)
(9069, 93.226)
(9070, 90.758)
(9071, 92.756)
(9072, 92.332)
(9073, 94.064)
(9074, 84.802)
(9075, 94.61)
(9076, 91.794)
(9077, 91.934)
(9078, 90.614)
(9079, 89.238)
(9080, 85.114)
(9081, 83.04)
(9082, 78.306)
(9083, 72.956)
(9084, 69.002)
(9085, 93.54)
(9086, 84.08)
(9087, 91.486)
(9088, 90.118)
(9089, 86.622)
(9090, 78.914)
(9091, 91.776)
(9092, 92.682)
(9093, 89.682)
(9094, 93.17)
(9095, 93.244)
(9096, 93.786)
(9097, 84.174)
(9098, 94.356)
(9099, 93.606)
(9100, 93.096)
(9101, 88.014)
(9102, 91.438)
(9103, 89.134)
(9104, 84.894)
(9105, 90.55)
(9106, 86.43)
(9107, 96.18)
(9108, 97.446)
(9109, 97.08)
(9110, 95.736)
(9111, 94.95)
(9112, 94.328)
(9113, 79.536)
(9114, 90.014)
(9115, 86.86)
(9116, 93.166)
(9117, 97.634)
(9118, 96.294)
(9119, 94.394)
(9120, 95.104)
(9121, 97.734)
(9122, 98.086)
(9123, 96.526)
(9124, 95.088)
(9125, 93.568)
(9126, 92.116)
(9127, 95.32)
(9128, 92.204)
(9129, 92.954)
(9130, 89.316)
(9131, 94.698)
(9132, 92.852)
(9133, 97.23)
(9134, 92.966)
(9135, 97.462)
(9136, 95.98)
(9137, 94.278)
(9138, 78.412)
(9139, 96.732)
(9140, 98.538)
(9141, 97.962)
(9142, 98.376)
(9143, 98.486)
(9144, 98.532)
(9145, 97.528)
(9146, 98.02)
(9147, 98.012)
(9148, 98.524)
(9149, 98.102)
(9150, 99.206)
(9151, 99.118)
(9152, 99.14)
(9153, 98.908)
(9154, 98.438)
(9155, 93.612)
(9156, 98.12)
(9157, 99.068)
(9158, 98.956)
(9159, 96.214)
(9160, 90.77)
(9161, 96.812)
(9162, 95.79)
(9163, 94.956)
(9164, 95.158)
(9165, 95.512)
(9166, 94.974)
(9167, 96.42)
(9168, 96.818)
(9169, 97.454)
(9170, 95.782)
(9171, 96.056)
(9172, 94.55)
(9173, 94.096)
(9174, 96.832)
(9175, 91.418)
(9176, 93.752)
(9177, 86.184)
(9178, 97.146)
(9179, 97.412)
(9180, 94.65)
(9181, 92.592)
(9182, 93.402)
(9183, 96.344)
(9184, 96.32)
(9185, 97.534)
(9186, 97.112)
(9187, 98.396)
(9188, 94.122)
(9189, 92.356)
(9190, 97.756)
(9191, 97.382)
(9192, 97.65)
(9193, 97.67)
(9194, 97.342)
(9195, 98.814)
(9196, 97.862)
(9197, 97.548)
(9198, 94.58)
(9199, 96.554)
(9200, 94.294)
(9201, 98.142)
(9202, 99.036)
(9203, 98.938)
(9204, 98.198)
(9205, 98.354)
(9206, 98.024)
(9207, 97.798)
(9208, 89.516)
(9209, 94.618)
(9210, 94.204)
(9211, 94.074)
(9212, 93.688)
(9213, 95.396)
(9214, 95.71)
(9215, 96.45)
(9216, 96.33)
(9217, 96.946)
(9218, 97.94)
(9219, 96.158)
(9220, 97.272)
(9221, 94.598)
(9222, 93.51)
(9223, 93.408)
(9224, 87.496)
(9225, 92.304)
(9226, 89.614)
(9227, 95.278)
(9228, 96.716)
(9229, 96.68)
(9230, 98.072)
(9231, 95.188)
(9232, 94.672)
(9233, 92.874)
(9234, 94.048)
(9235, 96.57)
(9236, 94.724)
(9237, 95.952)
(9238, 97.214)
(9239, 96.794)
(9240, 95.886)
(9241, 96.17)
(9242, 94.574)
(9243, 93.234)
(9244, 90.424)
(9245, 95.87)
(9246, 92.496)
(9247, 85.766)
(9248, 92.506)
(9249, 94.048)
(9250, 95.074)
(9251, 96.268)
(9252, 97.44)
(9253, 98.19)
(9254, 96.63)
(9255, 96.946)
(9256, 95.64)
(9257, 94.62)
(9258, 94.074)
(9259, 94.748)
(9260, 97.472)
(9261, 96.97)
(9262, 93.614)
(9263, 93.74)
(9264, 95.834)
(9265, 96.058)
(9266, 96.572)
(9267, 96.718)
(9268, 95.246)
(9269, 94.62)
(9270, 95.626)
(9271, 96.23)
(9272, 97.268)
(9273, 95.412)
(9274, 97.566)
(9275, 97.102)
(9276, 98.664)
(9277, 98.802)
(9278, 96.662)
(9279, 70.36)
(9280, 0)
};


==> covgraphs/graph.2.errors.tex <==
\addplot [sharp plot,color=lightblue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.00010385727004924)
(1, 7.03562945509368e-05)
(2, 2.64526080297125e-05)
(3, 6.70868710865903e-06)
(4, 4.75552503904944e-06)
(5, 2.25038238455018e-06)
(6, 1.52856161969446e-06)
(7, 1.3162613947369e-06)
(8, 5.9444062988118e-07)
(9, 1.01904107979631e-06)
(10, 9.34120989813283e-07)
(11, 7.64280809847232e-07)
(12, 6.36900674872693e-07)
(13, 6.36900674872693e-07)
(14, 9.76581034804796e-07)
(15, 1.06150112478782e-06)
(16, 9.76581034804796e-07)
(17, 1.35872143972841e-06)
(18, 1.40118148471992e-06)
(19, 1.18888125976236e-06)
(20, 8.49200899830257e-07)
(21, 1.06150112478782e-06)
(22, 7.21820764855719e-07)
(23, 6.79360719864206e-07)
(24, 8.9166094482177e-07)
(25, 7.64280809847232e-07)
(26, 3.39680359932103e-07)
(27, 8.9166094482177e-07)
(28, 3.82140404923616e-07)
(29, 7.21820764855719e-07)
(30, 7.64280809847232e-07)
(31, 7.64280809847232e-07)
(32, 5.09520539898154e-07)
(33, 4.67060494906642e-07)
(34, 1.14642121477085e-06)
(35, 5.09520539898154e-07)
(36, 5.9444062988118e-07)
(37, 6.36900674872693e-07)
(38, 5.9444062988118e-07)
(39, 7.64280809847232e-07)
(40, 6.36900674872693e-07)
(41, 1.10396116977933e-06)
(42, 5.51980584889667e-07)
(43, 5.09520539898154e-07)
(44, 8.49200899830257e-07)
(45, 8.49200899830257e-07)
(46, 1.3162613947369e-06)
(47, 8.06740854838745e-07)
(48, 9.34120989813283e-07)
(49, 1.35872143972841e-06)
(50, 8.49200899830257e-07)
(51, 1.44364152971144e-06)
(52, 1.61348170967749e-06)
(53, 4.11862436417675e-06)
(54, 9.80827039303947e-06)
(55, 6.10159409154413e-06)
(56, 5.85727540414743e-06)
(57, 5.79424657986548e-06)
(58, 4.99220776459337e-06)
(59, 5.01913965254169e-06)
(60, 5.56311198614551e-06)
(61, 5.88174013305155e-06)
(62, 5.87404261987417e-06)
(63, 5.67594954700914e-06)
(64, 6.72609233300902e-06)
(65, 1.05190690362138e-05)
(66, 6.26346001654238e-06)
(67, 6.46682786345831e-06)
(68, 6.5262308147496e-06)
(69, 8.35858279926521e-06)
(70, 7.69003868038529e-06)
(71, 7.11248293841615e-06)
(72, 8.45849513033471e-06)
(73, 9.05034033538645e-06)
(74, 8.04496150809877e-06)
(75, 9.57919368478246e-06)
(76, 8.60880917081907e-06)
(77, 8.33812350020131e-06)
(78, 9.84705564686316e-06)
(79, 1.02347638433515e-05)
(80, 1.11275717186874e-05)
(81, 9.85501340553894e-06)
(82, 1.06492693308553e-05)
(83, 1.00746430932533e-05)
(84, 1.15313535592001e-05)
(85, 1.00055823352873e-05)
(86, 1.18186608421473e-05)
(87, 1.05884679309702e-05)
(88, 1.17279542579607e-05)
(89, 1.16560830130877e-05)
(90, 1.23708121068446e-05)
(91, 1.21778470175365e-05)
(92, 1.50349900509842e-05)
(93, 1.66063404069266e-05)
(94, 1.87757349373251e-05)
(95, 1.76408484954112e-05)
(96, 3.00976669291852e-05)
(97, 4.75928864977903e-05)
(98, 8.25379277650759e-05)
(99, 9.95222391052658e-05)
(100, 0)
};



==> covgraphs/graph.errors.tex <==
\addplot [const plot,color=lightblue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=2pt] coordinates {
(-1, 0)
(0, 0.0126731801073116)
(1, 0.0132437735244654)
(2, 0.00828862016497157)
(3, 0.00562585088492032)
(4, 0.00427444542324017)
(5, 0.0086590053655802)
(6, 0.00574597581484744)
(7, 0.0056558821174021)
(8, 0.00831865139745335)
(9, 0.00651677744854649)
(10, 0.00510530952190278)
(11, 0.00669696484343717)
(12, 0.00355369584367742)
(13, 0.00331344598382318)
(14, 0.00220229038199728)
(15, 0.00393409145511332)
(16, 0.00364378954112277)
(17, 0.00375390406022263)
(18, 0.00234243613357892)
(19, 0.0029030191399055)
(20, 0.00311323776727797)
(21, 0.00170176984063426)
(22, 0.00180187394890686)
(23, 0.0038640185793225)
(24, 0.00171178025146152)
(25, 0.00189196764635221)
(26, 0.00209217586289741)
(27, 0.00110114519099864)
(28, 0.0012112597100985)
(29, 0.00205213421958837)
(30, 0.0011111556018259)
(31, 0.00137142628333467)
(32, 0.00147153039160727)
(33, 0.00240249859854248)
(34, 0.00137142628333467)
(35, 0.000940978617762473)
(36, 0.00135140546168015)
(37, 0.0010611035476896)
(38, 0.000960999439416994)
(39, 0.000920957796107952)
(40, 0.00110114519099864)
(41, 0.00105109313686234)
(42, 0.000790822455353568)
(43, 0.000900936974453432)
(44, 0.0010110514935533)
(45, 0.000991030671898775)
(46, 0.00108112436934412)
(47, 0.000920957796107952)
(48, 0.000910947385280692)
(49, 0.000950989028589733)
(50, 0.000870905741971651)
(51, 0.000870905741971651)
(52, 0.000730759990390006)
(53, 0.000840874509489869)
(54, 0.000900936974453432)
(55, 0.00109113478017138)
(56, 0.000910947385280692)
(57, 0.000940978617762473)
(58, 0.0012112597100985)
(59, 0.00110114519099864)
(60, 0.000981020261071514)
(61, 0.00105109313686234)
(62, 0.00103107231520782)
(63, 0.0012613117642348)
(64, 0.00103107231520782)
(65, 0.00151157203491631)
(66, 0.0021722591495155)
(67, 0.00150156162408905)
(68, 0.000960999439416994)
(69, 0.00112116601265316)
(70, 0.00208216545207015)
(71, 0.000930968206935213)
(72, 0.00114118683430768)
(73, 0.00206214463041563)
(74, 0.00127132217506206)
(75, 0.00150156162408905)
(76, 0.00373388323856811)
(77, 0.0015916553215344)
(78, 0.00158164491070714)
(79, 0.0034836229678866)
(80, 0.00250260270681509)
(81, 0.00233242572275166)
(82, 0.00309321694562345)
(83, 0.00341355009209578)
(84, 0.00331344598382318)
(85, 0.00193200928966125)
(86, 0.00322335228637783)
(87, 0.00347361255705934)
(88, 0.00626651717786498)
(89, 0.00483502842956675)
(90, 0.00632657964282854)
(91, 0.00862897413309842)
(92, 0.00561584047409306)
(93, 0.00591615279891087)
(94, 0.00768799551533595)
(95, 0.00388403940097702)
(96, 0.00513534075438456)
(97, 0.007497797709618)
(98, 0.0130035236646112)
(99, 0.0119324097060943)
(100, 0)
(101, 0)
};


==> covgraphs/graph.s.500.tex <==
\addplot[const plot,fill=lightred,draw=lightred] coordinates {
(-1, 0)
(0, 98.094)
(1, 97.41)
(2, 97.622)
(3, 98.888)
(4, 98.976)
(5, 98.484)
(6, 98.252)
(7, 98.14)
(8, 98.484)
(9, 98.958)
(10, 98.734)
(11, 99.428)
(12, 98.95)
(13, 99.138)
(14, 98.256)
(15, 97.03)
(16, 98.892)
(17, 98.764)
(18, 98.636)
(19, 98.654)
(20, 99.086)
(21, 97.596)
(22, 98.276)
(23, 98.116)
(24, 98.444)
(25, 98.302)
(26, 98.806)
(27, 98.744)
(28, 97.914)
(29, 97.992)
(30, 98.934)
(31, 99.946)
(32, 99.996)
(33, 98.168)
(34, 98.52)
(35, 98.642)
(36, 98.846)
(37, 98.552)
(38, 99.202)
(39, 99.212)
(40, 99.406)
(41, 99.034)
(42, 98.968)
(43, 98.73)
(44, 98.982)
(45, 98.602)
(46, 98.538)
(47, 98.532)
(48, 98.496)
(49, 98.84)
(50, 98.46)
(51, 98.284)
(52, 98.494)
(53, 98.944)
(54, 98.778)
(55, 97.712)
(56, 98.076)
(57, 98.926)
(58, 99.158)
(59, 98.966)
(60, 98.522)
(61, 98.758)
(62, 98.45)
(63, 98.832)
(64, 98.608)
(65, 97.992)
(66, 98.116)
(67, 99.118)
(68, 99.69)
(69, 99.046)
(70, 98.844)
(71, 97.182)
(72, 99)
(73, 97.676)
(74, 97.452)
(75, 98.056)
(76, 98.11)
(77, 96.458)
(78, 97.524)
(79, 97.572)
(80, 96.684)
(81, 97.046)
(82, 97.574)
(83, 97.398)
(84, 98.252)
(85, 96.744)
(86, 96.54)
(87, 95.578)
(88, 95.128)
(89, 96.382)
(90, 96.798)
(91, 96.286)
(92, 96.572)
(93, 96.786)
(94, 97.12)
(95, 94.118)
(96, 95.508)
(97, 96.942)
(98, 97.99)
(99, 97.762)
(100, 96.99)
(101, 96.616)
(102, 97.994)
(103, 97.946)
(104, 97.212)
(105, 97.07)
(106, 97.574)
(107, 97.32)
(108, 97.362)
(109, 97.928)
(110, 97.618)
(111, 98.262)
(112, 97.57)
(113, 97.4)
(114, 96.814)
(115, 97.112)
(116, 98.786)
(117, 98.928)
(118, 98.002)
(119, 98.41)
(120, 96.766)
(121, 96.916)
(122, 97.208)
(123, 96.004)
(124, 93.4)
(125, 95.286)
(126, 96.646)
(127, 93.766)
(128, 95.132)
(129, 95.424)
(130, 94.956)
(131, 93.948)
(132, 92.592)
(133, 95.392)
(134, 95.772)
(135, 91.004)
(136, 94.498)
(137, 93.058)
(138, 93.282)
(139, 95.362)
(140, 96.79)
(141, 96.192)
(142, 96.146)
(143, 88.048)
(144, 95.602)
(145, 96.32)
(146, 93)
(147, 86.504)
(148, 92.958)
(149, 94.888)
(150, 93.49)
(151, 96.306)
(152, 96.212)
(153, 97.188)
(154, 95.908)
(155, 96.298)
(156, 96.774)
(157, 97.04)
(158, 94.314)
(159, 94.622)
(160, 95.556)
(161, 93.262)
(162, 94.906)
(163, 89.368)
(164, 94.082)
(165, 95.056)
(166, 94.984)
(167, 96.17)
(168, 97.31)
(169, 97.128)
(170, 96.37)
(171, 94.74)
(172, 91.106)
(173, 92.298)
(174, 95.334)
(175, 95.97)
(176, 94.812)
(177, 93.444)
(178, 96.434)
(179, 96.106)
(180, 95.218)
(181, 91.27)
(182, 94.222)
(183, 95.298)
(184, 94.31)
(185, 88.736)
(186, 85.326)
(187, 92.476)
(188, 92.082)
(189, 94.412)
(190, 94.034)
(191, 95.37)
(192, 94.882)
(193, 95.376)
(194, 93.812)
(195, 96.358)
(196, 93.172)
(197, 95.598)
(198, 94.588)
(199, 95.654)
(200, 94.612)
(201, 96.258)
(202, 95.53)
(203, 93.458)
(204, 97.426)
(205, 98.472)
(206, 97.404)
(207, 97.946)
(208, 98.592)
(209, 97.382)
(210, 98.726)
(211, 98.896)
(212, 98.72)
(213, 98.96)
(214, 99.22)
(215, 98.358)
(216, 98.766)
(217, 98.484)
(218, 98.898)
(219, 97.906)
(220, 99.17)
(221, 98.676)
(222, 98.738)
(223, 99.13)
(224, 98.464)
(225, 98.79)
(226, 99.288)
(227, 98.898)
(228, 97.342)
(229, 99.012)
(230, 98.66)
(231, 97.556)
(232, 98.046)
(233, 96.792)
(234, 97.226)
(235, 98.344)
(236, 97.548)
(237, 96.608)
(238, 97.38)
(239, 97.122)
(240, 98.23)
(241, 97.21)
(242, 97.406)
(243, 98.324)
(244, 92.752)
(245, 91.808)
(246, 92.62)
(247, 92.966)
(248, 94.54)
(249, 91.594)
(250, 91)
(251, 93.192)
(252, 90.93)
(253, 90.602)
(254, 94.068)
(255, 94.98)
(256, 96.09)
(257, 95.888)
(258, 95.022)
(259, 90.764)
(260, 78.26)
(261, 59.48)
(262, 65.14)
(263, 73.3)
(264, 72.344)
(265, 73.642)
(266, 81.294)
(267, 82.74)
(268, 78.338)
(269, 84.538)
(270, 87.138)
(271, 84.156)
(272, 92.236)
(273, 90.088)
(274, 82.944)
(275, 88.372)
(276, 90.644)
(277, 93.982)
(278, 86.702)
(279, 90.458)
(280, 93.41)
(281, 91.966)
(282, 91.758)
(283, 93.09)
(284, 94.614)
(285, 96.686)
(286, 96.564)
(287, 95.582)
(288, 95.508)
(289, 95.916)
(290, 94.236)
(291, 96.532)
(292, 96.058)
(293, 96.514)
(294, 97.432)
(295, 98.252)
(296, 98.03)
(297, 96.146)
(298, 95.562)
(299, 98.478)
(300, 99.138)
(301, 98.774)
(302, 98.878)
(303, 97.82)
(304, 98.488)
(305, 98.91)
(306, 98.08)
(307, 97.806)
(308, 97.854)
(309, 97.836)
(310, 97.906)
(311, 97.808)
(312, 97.946)
(313, 97.224)
(314, 97.61)
(315, 96.27)
(316, 95.578)
(317, 96.472)
(318, 96.568)
(319, 95.386)
(320, 94.24)
(321, 97.764)
(322, 97.558)
(323, 93.552)
(324, 93.61)
(325, 95.402)
(326, 90.944)
(327, 94.388)
(328, 95.958)
(329, 94.74)
(330, 97.918)
(331, 98.106)
(332, 97.956)
(333, 98.05)
(334, 97.51)
(335, 97.638)
(336, 97.89)
(337, 98.476)
(338, 98.08)
(339, 97.396)
(340, 95.838)
(341, 96.816)
(342, 97.23)
(343, 95.402)
(344, 95.898)
(345, 92.478)
(346, 96.03)
(347, 98.128)
(348, 97.31)
(349, 98.392)
(350, 96.192)
(351, 97.226)
(352, 97.896)
(353, 98.75)
(354, 97.214)
(355, 98.684)
(356, 98.41)
(357, 98.744)
(358, 98.662)
(359, 98.388)
(360, 99.048)
(361, 98.67)
(362, 98.848)
(363, 98.626)
(364, 98.962)
(365, 98.604)
(366, 98.404)
(367, 99.194)
(368, 98.758)
(369, 98.766)
(370, 98.67)
(371, 98.576)
(372, 98.37)
(373, 98.25)
(374, 97.148)
(375, 97.628)
(376, 98.432)
(377, 98.652)
(378, 98.668)
(379, 98.972)
(380, 98.87)
(381, 98.804)
(382, 99.016)
(383, 98.71)
(384, 98.888)
(385, 99.006)
(386, 98.864)
(387, 97.966)
(388, 98.93)
(389, 99.236)
(390, 99.412)
(391, 99.064)
(392, 99.192)
(393, 98.926)
(394, 99.446)
(395, 99.182)
(396, 99.522)
(397, 99.526)
(398, 99.55)
(399, 99.626)
(400, 99.562)
(401, 99.768)
(402, 99.716)
(403, 99.554)
(404, 99.704)
(405, 99.454)
(406, 99.622)
(407, 99.8)
(408, 99.008)
(409, 99.582)
(410, 99.522)
(411, 99.666)
(412, 99.656)
(413, 98.142)
(414, 98.556)
(415, 99.842)
(416, 99.738)
(417, 99.896)
(418, 99.864)
(419, 99.962)
(420, 99.846)
(421, 99.806)
(422, 99.864)
(423, 99.962)
(424, 99.838)
(425, 99.794)
(426, 99.554)
(427, 99.892)
(428, 99.926)
(429, 99.88)
(430, 99.842)
(431, 99.92)
(432, 99.976)
(433, 99.97)
(434, 99.956)
(435, 99.926)
(436, 99.242)
(437, 99.77)
(438, 99.874)
(439, 99.938)
(440, 99.936)
(441, 99.932)
(442, 99.852)
(443, 99.858)
(444, 99.908)
(445, 99.962)
(446, 99.854)
(447, 99.772)
(448, 99.906)
(449, 99.908)
(450, 99.996)
(451, 99.976)
(452, 99.968)
(453, 99.974)
(454, 100)
(455, 99.994)
(456, 99.986)
(457, 100)
(458, 100)
(459, 100)
(460, 100)
(461, 100)
(462, 99.994)
(463, 99.992)
(464, 100)
(465, 100)
(466, 99.996)
(467, 100)
(468, 100)
(469, 99.996)
(470, 99.996)
(471, 99.994)
(472, 99.992)
(473, 99.994)
(474, 100)
(475, 99.998)
(476, 100)
(477, 100)
(478, 99.982)
(479, 99.288)
(480, 99.996)
(481, 99.934)
(482, 99.894)
(483, 99.872)
(484, 99.542)
(485, 99.648)
(486, 99.924)
(487, 99.76)
(488, 99.908)
(489, 99.85)
(490, 99.834)
(491, 99.938)
(492, 99.93)
(493, 99.69)
(494, 99.744)
(495, 99.906)
(496, 99.674)
(497, 99.554)
(498, 98.186)
(499, 98.912)
(500, 99.588)
(501, 99.466)
(502, 99.718)
(503, 99.71)
(504, 99.91)
(505, 99.902)
(506, 99.872)
(507, 99.59)
(508, 99.87)
(509, 99.83)
(510, 99.544)
(511, 99.884)
(512, 99.738)
(513, 98.768)
(514, 99.61)
(515, 97.918)
(516, 99.684)
(517, 99.714)
(518, 99.556)
(519, 98.828)
(520, 97.564)
(521, 98.608)
(522, 99.092)
(523, 99.534)
(524, 99.732)
(525, 99.402)
(526, 99.488)
(527, 99.4)
(528, 99.254)
(529, 99.668)
(530, 99.848)
(531, 99.528)
(532, 99.66)
(533, 99.454)
(534, 99.51)
(535, 99.608)
(536, 99.742)
(537, 99.91)
(538, 99.84)
(539, 99.246)
(540, 98.782)
(541, 99.73)
(542, 99.564)
(543, 99.616)
(544, 99.296)
(545, 99.774)
(546, 99.872)
(547, 99.716)
(548, 99.702)
(549, 99.19)
(550, 99.35)
(551, 99.494)
(552, 99.234)
(553, 98.992)
(554, 99.438)
(555, 99.458)
(556, 99.442)
(557, 99.398)
(558, 99.748)
(559, 99.754)
(560, 98.56)
(561, 96.582)
(562, 98.234)
(563, 97.94)
(564, 97.75)
(565, 92.16)
(566, 81.83)
(567, 96.57)
(568, 97.206)
(569, 98.1)
(570, 97.22)
(571, 96.92)
(572, 96.048)
(573, 95.312)
(574, 97.658)
(575, 95.93)
(576, 99.092)
(577, 97.494)
(578, 98.672)
(579, 99.518)
(580, 99.384)
(581, 99.428)
(582, 99.8)
(583, 99.836)
(584, 99.87)
(585, 99.848)
(586, 99.878)
(587, 99.862)
(588, 99.716)
(589, 99.93)
(590, 99.908)
(591, 98.856)
(592, 99.926)
(593, 99.546)
(594, 98.898)
(595, 99.36)
(596, 99.506)
(597, 98.508)
(598, 98.856)
(599, 97.218)
(600, 99.354)
(601, 98.766)
(602, 99.498)
(603, 99.492)
(604, 99.912)
(605, 99.864)
(606, 99.902)
(607, 99.924)
(608, 99.778)
(609, 99.714)
(610, 99.808)
(611, 99.704)
(612, 99.712)
(613, 98.656)
(614, 99.412)
(615, 99.16)
(616, 99.826)
(617, 99.562)
(618, 99.812)
(619, 99.832)
(620, 99.838)
(621, 99.934)
(622, 99.924)
(623, 99.954)
(624, 99.96)
(625, 99.96)
(626, 99.964)
(627, 99.87)
(628, 99.914)
(629, 99.102)
(630, 97.868)
(631, 97.402)
(632, 99.968)
(633, 99.978)
(634, 99.952)
(635, 99.974)
(636, 99.888)
(637, 99.896)
(638, 99.89)
(639, 99.782)
(640, 99.868)
(641, 99.924)
(642, 99.81)
(643, 99.932)
(644, 99.922)
(645, 99.942)
(646, 99.938)
(647, 99.984)
(648, 99.996)
(649, 99.946)
(650, 99.364)
(651, 99.684)
(652, 99.746)
(653, 99.74)
(654, 99.14)
(655, 99.04)
(656, 99.498)
(657, 99.892)
(658, 99.796)
(659, 99.602)
(660, 99.56)
(661, 99.944)
(662, 99.99)
(663, 99.994)
(664, 99.976)
(665, 99.986)
(666, 99.966)
(667, 99.94)
(668, 99.94)
(669, 99.95)
(670, 99.94)
(671, 99.93)
(672, 99.818)
(673, 99.032)
(674, 99.782)
(675, 99.14)
(676, 99.582)
(677, 99.484)
(678, 99.572)
(679, 99.294)
(680, 99.772)
(681, 99.532)
(682, 99.836)
(683, 99.902)
(684, 99.866)
(685, 99.822)
(686, 99.994)
(687, 99.99)
(688, 100)
(689, 99.988)
(690, 99.93)
(691, 99.994)
(692, 99.902)
(693, 99.546)
(694, 99.832)
(695, 99.968)
(696, 99.732)
(697, 99.852)
(698, 99.88)
(699, 99.234)
(700, 99.872)
(701, 99.366)
(702, 99.742)
(703, 99.832)
(704, 99.478)
(705, 99.082)
(706, 99.4)
(707, 99.9)
(708, 99.866)
(709, 99.766)
(710, 99.852)
(711, 99.91)
(712, 99.786)
(713, 98.152)
(714, 97.816)
(715, 99.762)
(716, 99.572)
(717, 99.576)
(718, 99.61)
(719, 99.038)
(720, 99.848)
(721, 99.928)
(722, 99.872)
(723, 99.898)
(724, 99.778)
(725, 99.786)
(726, 99.566)
(727, 99.406)
(728, 99.624)
(729, 99.664)
(730, 99.676)
(731, 99.472)
(732, 99.612)
(733, 99.574)
(734, 99.184)
(735, 99.604)
(736, 99.462)
(737, 98.062)
(738, 99.078)
(739, 99.18)
(740, 99.318)
(741, 99.316)
(742, 99.712)
(743, 99.372)
(744, 99.632)
(745, 99.438)
(746, 99.692)
(747, 98.656)
(748, 99.284)
(749, 99.654)
(750, 99.416)
(751, 99.798)
(752, 99.954)
(753, 99.95)
(754, 99.952)
(755, 99.936)
(756, 99.9)
(757, 99.894)
(758, 99.44)
(759, 99.946)
(760, 99.978)
(761, 98.142)
(762, 99.226)
(763, 99.938)
(764, 99.836)
(765, 99.938)
(766, 99.978)
(767, 99.986)
(768, 99.986)
(769, 99.788)
(770, 99.852)
(771, 99.708)
(772, 99.398)
(773, 99.854)
(774, 99.93)
(775, 99.92)
(776, 99.914)
(777, 99.98)
(778, 100)
(779, 100)
(780, 100)
(781, 99.998)
(782, 99.758)
(783, 99.976)
(784, 99.992)
(785, 99.978)
(786, 99.99)
(787, 99.998)
(788, 99.966)
(789, 99.82)
(790, 99.888)
(791, 99.938)
(792, 99.972)
(793, 99.94)
(794, 99.922)
(795, 99.934)
(796, 99.828)
(797, 99.99)
(798, 99.956)
(799, 99.98)
(800, 99.99)
(801, 99.992)
(802, 99.932)
(803, 99.954)
(804, 99.956)
(805, 99.964)
(806, 99.852)
(807, 99.974)
(808, 99.94)
(809, 99.954)
(810, 99.91)
(811, 99.944)
(812, 100)
(813, 99.998)
(814, 99.994)
(815, 99.98)
(816, 99.974)
(817, 99.99)
(818, 99.94)
(819, 99.802)
(820, 99.96)
(821, 99.98)
(822, 99.832)
(823, 99.954)
(824, 99.958)
(825, 99.92)
(826, 99.712)
(827, 99.744)
(828, 99.772)
(829, 99.68)
(830, 99.808)
(831, 99.58)
(832, 99.9)
(833, 99.506)
(834, 99.662)
(835, 99.836)
(836, 99.952)
(837, 99.118)
(838, 99.628)
(839, 99.746)
(840, 99.782)
(841, 99.77)
(842, 99.8)
(843, 99.804)
(844, 99.438)
(845, 99.62)
(846, 99.72)
(847, 99.792)
(848, 99.864)
(849, 99.71)
(850, 99.866)
(851, 99.892)
(852, 99.962)
(853, 99.942)
(854, 99.93)
(855, 99.94)
(856, 99.976)
(857, 99.92)
(858, 99.922)
(859, 99.994)
(860, 99.978)
(861, 99.962)
(862, 99.988)
(863, 99.996)
(864, 99.946)
(865, 99.652)
(866, 99.894)
(867, 99.91)
(868, 99.9)
(869, 99.962)
(870, 99.882)
(871, 99.928)
(872, 99.964)
(873, 99.968)
(874, 99.922)
(875, 99.904)
(876, 99.906)
(877, 99.97)
(878, 99.942)
(879, 99.956)
(880, 99.82)
(881, 99.86)
(882, 99.834)
(883, 99.944)
(884, 99.536)
(885, 99.802)
(886, 99.864)
(887, 99.954)
(888, 99.96)
(889, 99.388)
(890, 99.78)
(891, 99.75)
(892, 99.162)
(893, 99.806)
(894, 99.736)
(895, 99.756)
(896, 99.73)
(897, 99.528)
(898, 99.598)
(899, 99.498)
(900, 99.598)
(901, 99.85)
(902, 99.498)
(903, 99.144)
(904, 99.406)
(905, 99.71)
(906, 99.842)
(907, 99.896)
(908, 99.902)
(909, 99.892)
(910, 99.858)
(911, 99.948)
(912, 99.884)
(913, 99.86)
(914, 99.846)
(915, 99.882)
(916, 99.89)
(917, 99.906)
(918, 99.842)
(919, 99.91)
(920, 99.934)
(921, 99.96)
(922, 99.97)
(923, 99.908)
(924, 99.848)
(925, 99.934)
(926, 99.964)
(927, 99.99)
(928, 99.944)
(929, 99.952)
(930, 99.936)
(931, 99.94)
(932, 99.952)
(933, 99.97)
(934, 99.966)
(935, 99.87)
(936, 99.936)
(937, 99.942)
(938, 99.974)
(939, 99.652)
(940, 99.894)
(941, 99.956)
(942, 99.876)
(943, 99.972)
(944, 99.964)
(945, 99.832)
(946, 99.674)
(947, 99.99)
(948, 99.984)
(949, 99.982)
(950, 99.952)
(951, 99.976)
(952, 99.99)
(953, 99.986)
(954, 99.996)
(955, 99.994)
(956, 99.998)
(957, 99.998)
(958, 100)
(959, 99.998)
(960, 99.988)
(961, 99.966)
(962, 99.968)
(963, 99.984)
(964, 99.954)
(965, 99.804)
(966, 99.918)
(967, 99.936)
(968, 99.952)
(969, 99.976)
(970, 99.988)
(971, 99.954)
(972, 99.976)
(973, 99.982)
(974, 99.958)
(975, 99.914)
(976, 99.974)
(977, 99.986)
(978, 99.956)
(979, 99.336)
(980, 99.898)
(981, 99.966)
(982, 99.858)
(983, 99.858)
(984, 99.44)
(985, 98.198)
(986, 99.98)
(987, 99.864)
(988, 99.986)
(989, 99.954)
(990, 99.994)
(991, 99.976)
(992, 99.98)
(993, 99.966)
(994, 99.78)
(995, 99.832)
(996, 99.938)
(997, 99.964)
(998, 99.976)
(999, 99.978)
(1000, 99.92)
(1001, 99.92)
(1002, 99.906)
(1003, 99.856)
(1004, 99.77)
(1005, 99.88)
(1006, 99.6)
(1007, 99.712)
(1008, 99.926)
(1009, 99.87)
(1010, 99.99)
(1011, 99.898)
(1012, 99.97)
(1013, 99.946)
(1014, 99.93)
(1015, 99.984)
(1016, 99.866)
(1017, 99.676)
(1018, 99.682)
(1019, 99.63)
(1020, 99.496)
(1021, 99.934)
(1022, 99.9)
(1023, 99.786)
(1024, 99.874)
(1025, 99.762)
(1026, 99.744)
(1027, 99.268)
(1028, 99.772)
(1029, 99.934)
(1030, 99.97)
(1031, 99.972)
(1032, 99.946)
(1033, 99.902)
(1034, 99.89)
(1035, 99.848)
(1036, 99.782)
(1037, 99.808)
(1038, 99.754)
(1039, 99.484)
(1040, 99.766)
(1041, 99.46)
(1042, 99.66)
(1043, 99.698)
(1044, 99.896)
(1045, 98.386)
(1046, 98.81)
(1047, 99.382)
(1048, 98.966)
(1049, 97.896)
(1050, 97.332)
(1051, 99.19)
(1052, 99.98)
(1053, 100)
(1054, 99.812)
(1055, 100)
(1056, 100)
(1057, 99.998)
(1058, 99.998)
(1059, 99.986)
(1060, 99.954)
(1061, 99.974)
(1062, 99.994)
(1063, 99.998)
(1064, 99.976)
(1065, 99.982)
(1066, 99.986)
(1067, 99.98)
(1068, 99.996)
(1069, 99.998)
(1070, 99.992)
(1071, 100)
(1072, 100)
(1073, 100)
(1074, 100)
(1075, 99.992)
(1076, 100)
(1077, 99.998)
(1078, 100)
(1079, 99.998)
(1080, 99.978)
(1081, 99.994)
(1082, 99.942)
(1083, 99.952)
(1084, 99.998)
(1085, 100)
(1086, 99.998)
(1087, 99.996)
(1088, 99.902)
(1089, 99.968)
(1090, 99.936)
(1091, 99.988)
(1092, 99.942)
(1093, 99.676)
(1094, 99.854)
(1095, 96.092)
(1096, 99.962)
(1097, 99.898)
(1098, 99.922)
(1099, 99.93)
(1100, 99.868)
(1101, 99.988)
(1102, 99.99)
(1103, 99.904)
(1104, 99.962)
(1105, 99.964)
(1106, 99.994)
(1107, 100)
(1108, 99.938)
(1109, 99.948)
(1110, 99.964)
(1111, 99.976)
(1112, 99.984)
(1113, 99.868)
(1114, 99.974)
(1115, 99.998)
(1116, 100)
(1117, 99.998)
(1118, 100)
(1119, 100)
(1120, 99.996)
(1121, 99.958)
(1122, 100)
(1123, 100)
(1124, 99.984)
(1125, 99.948)
(1126, 100)
(1127, 100)
(1128, 100)
(1129, 99.992)
(1130, 99.976)
(1131, 99.956)
(1132, 98.176)
(1133, 96.374)
(1134, 98.438)
(1135, 99.996)
(1136, 100)
(1137, 100)
(1138, 100)
(1139, 100)
(1140, 100)
(1141, 100)
(1142, 100)
(1143, 100)
(1144, 99.998)
(1145, 99.986)
(1146, 100)
(1147, 99.972)
(1148, 99.754)
(1149, 99.732)
(1150, 100)
(1151, 100)
(1152, 99.998)
(1153, 100)
(1154, 100)
(1155, 99.998)
(1156, 100)
(1157, 100)
(1158, 100)
(1159, 99.992)
(1160, 99.992)
(1161, 99.998)
(1162, 100)
(1163, 100)
(1164, 100)
(1165, 100)
(1166, 100)
(1167, 100)
(1168, 100)
(1169, 100)
(1170, 100)
(1171, 99.998)
(1172, 99.998)
(1173, 99.99)
(1174, 100)
(1175, 99.942)
(1176, 99.984)
(1177, 99.988)
(1178, 99.986)
(1179, 100)
(1180, 99.992)
(1181, 99.992)
(1182, 99.982)
(1183, 99.992)
(1184, 99.998)
(1185, 99.98)
(1186, 99.996)
(1187, 99.996)
(1188, 99.976)
(1189, 99.994)
(1190, 99.836)
(1191, 99.6)
(1192, 99.996)
(1193, 99.696)
(1194, 99.364)
(1195, 99.524)
(1196, 99.712)
(1197, 98.992)
(1198, 99.746)
(1199, 99.51)
(1200, 99.66)
(1201, 99.556)
(1202, 99.872)
(1203, 99.808)
(1204, 99.96)
(1205, 99.962)
(1206, 99.9)
(1207, 99.934)
(1208, 99.782)
(1209, 99.944)
(1210, 99.892)
(1211, 99.85)
(1212, 99.81)
(1213, 99.9)
(1214, 99.95)
(1215, 99.974)
(1216, 99.992)
(1217, 99.982)
(1218, 99.938)
(1219, 99.808)
(1220, 99.812)
(1221, 99.646)
(1222, 98.874)
(1223, 99.736)
(1224, 99.616)
(1225, 99.416)
(1226, 99.26)
(1227, 99.458)
(1228, 98.298)
(1229, 99.324)
(1230, 99.308)
(1231, 98.42)
(1232, 99.06)
(1233, 99.394)
(1234, 99.666)
(1235, 99.506)
(1236, 99.784)
(1237, 99.71)
(1238, 99.472)
(1239, 99.234)
(1240, 99.278)
(1241, 98.662)
(1242, 98.676)
(1243, 98.954)
(1244, 96.62)
(1245, 99.582)
(1246, 99.348)
(1247, 99.64)
(1248, 99.184)
(1249, 99.662)
(1250, 99.626)
(1251, 99.762)
(1252, 99.606)
(1253, 99.71)
(1254, 99.754)
(1255, 99.72)
(1256, 99.53)
(1257, 99.792)
(1258, 99.734)
(1259, 99.834)
(1260, 99.788)
(1261, 99.918)
(1262, 99.948)
(1263, 99.906)
(1264, 99.796)
(1265, 99.934)
(1266, 99.828)
(1267, 99.966)
(1268, 99.982)
(1269, 99.99)
(1270, 99.982)
(1271, 99.998)
(1272, 99.998)
(1273, 100)
(1274, 99.974)
(1275, 100)
(1276, 99.988)
(1277, 99.638)
(1278, 99.572)
(1279, 99.272)
(1280, 99.494)
(1281, 99.594)
(1282, 99.824)
(1283, 99.572)
(1284, 99.548)
(1285, 99.762)
(1286, 99.866)
(1287, 99.728)
(1288, 99.824)
(1289, 99.786)
(1290, 99.018)
(1291, 99.294)
(1292, 99.372)
(1293, 99.378)
(1294, 99.512)
(1295, 99.476)
(1296, 99.402)
(1297, 98.872)
(1298, 99.22)
(1299, 99.168)
(1300, 99.336)
(1301, 99.778)
(1302, 99.844)
(1303, 99.752)
(1304, 99.8)
(1305, 99.81)
(1306, 99.868)
(1307, 99.808)
(1308, 99.92)
(1309, 99.474)
(1310, 99.918)
(1311, 99.942)
(1312, 99.93)
(1313, 99.922)
(1314, 99.908)
(1315, 99.62)
(1316, 99.916)
(1317, 99.834)
(1318, 99.86)
(1319, 99.938)
(1320, 99.982)
(1321, 99.984)
(1322, 99.926)
(1323, 99.978)
(1324, 99.98)
(1325, 99.968)
(1326, 99.914)
(1327, 99.694)
(1328, 99.68)
(1329, 99.792)
(1330, 99.918)
(1331, 99.88)
(1332, 99.864)
(1333, 99.878)
(1334, 99.872)
(1335, 99.044)
(1336, 99.878)
(1337, 99.92)
(1338, 99.814)
(1339, 99.716)
(1340, 99.854)
(1341, 99.828)
(1342, 99.78)
(1343, 99.578)
(1344, 99.666)
(1345, 99.36)
(1346, 99.418)
(1347, 99.054)
(1348, 99.786)
(1349, 99.802)
(1350, 99.726)
(1351, 99.796)
(1352, 99.82)
(1353, 99.782)
(1354, 99.788)
(1355, 99.768)
(1356, 99.8)
(1357, 99.89)
(1358, 99.64)
(1359, 99.88)
(1360, 99.906)
(1361, 99.476)
(1362, 99.862)
(1363, 99.73)
(1364, 99.894)
(1365, 99.912)
(1366, 99.716)
(1367, 99.87)
(1368, 99.792)
(1369, 99.718)
(1370, 98.204)
(1371, 99.746)
(1372, 99.754)
(1373, 99.686)
(1374, 99.842)
(1375, 99.76)
(1376, 99.818)
(1377, 99.152)
(1378, 99.65)
(1379, 99.372)
(1380, 99.746)
(1381, 99.69)
(1382, 99.658)
(1383, 99.648)
(1384, 98.746)
(1385, 99.43)
(1386, 99.006)
(1387, 99.052)
(1388, 99.364)
(1389, 99.366)
(1390, 99.37)
(1391, 99.714)
(1392, 99.76)
(1393, 99.718)
(1394, 99.858)
(1395, 99.76)
(1396, 99.778)
(1397, 99.83)
(1398, 99.752)
(1399, 99.772)
(1400, 99.696)
(1401, 99.332)
(1402, 99.844)
(1403, 99.83)
(1404, 99.844)
(1405, 99.832)
(1406, 99.542)
(1407, 98.962)
(1408, 99.714)
(1409, 99.532)
(1410, 99.834)
(1411, 99.856)
(1412, 99.692)
(1413, 99.874)
(1414, 99.846)
(1415, 99.784)
(1416, 99.848)
(1417, 99.79)
(1418, 99.932)
(1419, 99.9)
(1420, 99.902)
(1421, 99.87)
(1422, 99.854)
(1423, 99.842)
(1424, 99.902)
(1425, 99.886)
(1426, 99.504)
(1427, 99.766)
(1428, 99.7)
(1429, 99.93)
(1430, 99.944)
(1431, 99.956)
(1432, 99.944)
(1433, 99.818)
(1434, 99.846)
(1435, 99.834)
(1436, 99.93)
(1437, 99.754)
(1438, 99.79)
(1439, 99.836)
(1440, 99.746)
(1441, 99.384)
(1442, 99.654)
(1443, 99.02)
(1444, 99.376)
(1445, 98.448)
(1446, 98.942)
(1447, 99.244)
(1448, 99.208)
(1449, 98.912)
(1450, 98.364)
(1451, 98.688)
(1452, 98.738)
(1453, 97.372)
(1454, 98.922)
(1455, 98.578)
(1456, 99.068)
(1457, 97.982)
(1458, 92.992)
(1459, 93.49)
(1460, 97.818)
(1461, 96.034)
(1462, 96.082)
(1463, 95.46)
(1464, 96.286)
(1465, 99.56)
(1466, 99.362)
(1467, 95.652)
(1468, 98.976)
(1469, 99.792)
(1470, 99.856)
(1471, 99.902)
(1472, 99.91)
(1473, 99.926)
(1474, 99.936)
(1475, 99.976)
(1476, 99.916)
(1477, 99.236)
(1478, 99.498)
(1479, 99.38)
(1480, 99.908)
(1481, 99.894)
(1482, 99.696)
(1483, 99.916)
(1484, 99.774)
(1485, 98.89)
(1486, 99.654)
(1487, 99.696)
(1488, 99.92)
(1489, 99.768)
(1490, 99.906)
(1491, 99.872)
(1492, 99.7)
(1493, 99.872)
(1494, 99.986)
(1495, 99.984)
(1496, 99.962)
(1497, 99.97)
(1498, 99.908)
(1499, 99.96)
(1500, 99.9)
(1501, 99.876)
(1502, 99.83)
(1503, 99.92)
(1504, 99.678)
(1505, 99.894)
(1506, 99.938)
(1507, 99.976)
(1508, 99.91)
(1509, 99.886)
(1510, 99.484)
(1511, 99.52)
(1512, 99.732)
(1513, 99.816)
(1514, 99.816)
(1515, 99.826)
(1516, 99.844)
(1517, 99.75)
(1518, 99.646)
(1519, 99.672)
(1520, 99.69)
(1521, 99.766)
(1522, 99.578)
(1523, 99.754)
(1524, 99.844)
(1525, 99.804)
(1526, 99.748)
(1527, 99.778)
(1528, 99.926)
(1529, 99.938)
(1530, 99.694)
(1531, 99.006)
(1532, 99.484)
(1533, 99.816)
(1534, 99.696)
(1535, 99.864)
(1536, 99.898)
(1537, 99.984)
(1538, 99.936)
(1539, 99.962)
(1540, 99.962)
(1541, 99.98)
(1542, 99.952)
(1543, 99.886)
(1544, 99.924)
(1545, 99.918)
(1546, 99.974)
(1547, 99.972)
(1548, 99.984)
(1549, 99.89)
(1550, 99.954)
(1551, 99.71)
(1552, 99.134)
(1553, 99.992)
(1554, 99.952)
(1555, 99.99)
(1556, 99.964)
(1557, 99.996)
(1558, 99.976)
(1559, 99.972)
(1560, 99.968)
(1561, 99.98)
(1562, 99.998)
(1563, 99.976)
(1564, 99.954)
(1565, 100)
(1566, 99.992)
(1567, 99.992)
(1568, 99.904)
(1569, 99.998)
(1570, 99.98)
(1571, 99.96)
(1572, 99.994)
(1573, 99.992)
(1574, 99.932)
(1575, 99.914)
(1576, 99.918)
(1577, 99.948)
(1578, 99.89)
(1579, 99.882)
(1580, 99.934)
(1581, 99.942)
(1582, 99.986)
(1583, 99.944)
(1584, 99.982)
(1585, 99.98)
(1586, 99.94)
(1587, 99.958)
(1588, 99.97)
(1589, 99.968)
(1590, 99.962)
(1591, 99.98)
(1592, 99.98)
(1593, 99.968)
(1594, 99.978)
(1595, 99.972)
(1596, 99.944)
(1597, 99.986)
(1598, 99.978)
(1599, 99.994)
(1600, 99.956)
(1601, 99.992)
(1602, 99.962)
(1603, 99.97)
(1604, 99.97)
(1605, 99.966)
(1606, 99.942)
(1607, 99.97)
(1608, 99.976)
(1609, 99.982)
(1610, 99.98)
(1611, 99.99)
(1612, 99.956)
(1613, 99.974)
(1614, 99.872)
(1615, 99.908)
(1616, 99.934)
(1617, 99.952)
(1618, 99.928)
(1619, 99.112)
(1620, 99.908)
(1621, 99.042)
(1622, 99.896)
(1623, 99.876)
(1624, 99.986)
(1625, 99.994)
(1626, 99.994)
(1627, 99.824)
(1628, 99.994)
(1629, 100)
(1630, 99.986)
(1631, 99.974)
(1632, 99.97)
(1633, 99.914)
(1634, 99.97)
(1635, 99.94)
(1636, 99.806)
(1637, 99.948)
(1638, 99.988)
(1639, 99.974)
(1640, 100)
(1641, 99.994)
(1642, 99.964)
(1643, 99.962)
(1644, 99.93)
(1645, 99.882)
(1646, 99.824)
(1647, 99.988)
(1648, 99.924)
(1649, 99.982)
(1650, 99.96)
(1651, 99.972)
(1652, 99.942)
(1653, 99.804)
(1654, 99.962)
(1655, 99.844)
(1656, 99.72)
(1657, 99.846)
(1658, 99.736)
(1659, 99.832)
(1660, 99.702)
(1661, 99.888)
(1662, 98.496)
(1663, 99.938)
(1664, 99.916)
(1665, 99.876)
(1666, 99.742)
(1667, 99.876)
(1668, 99.882)
(1669, 99.49)
(1670, 99.79)
(1671, 99.548)
(1672, 99.856)
(1673, 99.732)
(1674, 99.978)
(1675, 99.946)
(1676, 99.886)
(1677, 99.888)
(1678, 99.812)
(1679, 99.836)
(1680, 99.772)
(1681, 99.962)
(1682, 99.982)
(1683, 99.96)
(1684, 99.83)
(1685, 99.924)
(1686, 99.804)
(1687, 99.988)
(1688, 99.888)
(1689, 99.914)
(1690, 99.976)
(1691, 99.956)
(1692, 99.974)
(1693, 99.968)
(1694, 99.982)
(1695, 99.984)
(1696, 99.996)
(1697, 99.878)
(1698, 99.986)
(1699, 99.988)
(1700, 99.988)
(1701, 99.992)
(1702, 99.97)
(1703, 99.962)
(1704, 99.992)
(1705, 99.966)
(1706, 99.946)
(1707, 99.982)
(1708, 99.924)
(1709, 99.976)
(1710, 99.982)
(1711, 99.978)
(1712, 99.996)
(1713, 99.988)
(1714, 99.998)
(1715, 99.994)
(1716, 99.978)
(1717, 100)
(1718, 100)
(1719, 99.922)
(1720, 99.88)
(1721, 99.996)
(1722, 99.976)
(1723, 99.97)
(1724, 99.976)
(1725, 99.972)
(1726, 99.968)
(1727, 99.996)
(1728, 99.982)
(1729, 99.972)
(1730, 99.956)
(1731, 99.982)
(1732, 99.92)
(1733, 99.906)
(1734, 99.986)
(1735, 99.976)
(1736, 99.942)
(1737, 99.996)
(1738, 99.994)
(1739, 99.97)
(1740, 99.942)
(1741, 99.952)
(1742, 99.994)
(1743, 99.996)
(1744, 100)
(1745, 100)
(1746, 100)
(1747, 100)
(1748, 100)
(1749, 100)
(1750, 100)
(1751, 100)
(1752, 100)
(1753, 99.998)
(1754, 100)
(1755, 100)
(1756, 100)
(1757, 100)
(1758, 100)
(1759, 100)
(1760, 100)
(1761, 100)
(1762, 100)
(1763, 100)
(1764, 100)
(1765, 100)
(1766, 99.996)
(1767, 99.99)
(1768, 100)
(1769, 100)
(1770, 99.996)
(1771, 99.976)
(1772, 100)
(1773, 100)
(1774, 100)
(1775, 100)
(1776, 100)
(1777, 100)
(1778, 100)
(1779, 99.998)
(1780, 100)
(1781, 99.998)
(1782, 99.982)
(1783, 99.978)
(1784, 100)
(1785, 100)
(1786, 99.998)
(1787, 99.996)
(1788, 99.99)
(1789, 99.998)
(1790, 99.996)
(1791, 100)
(1792, 99.994)
(1793, 99.98)
(1794, 100)
(1795, 99.996)
(1796, 99.978)
(1797, 100)
(1798, 100)
(1799, 99.998)
(1800, 100)
(1801, 99.994)
(1802, 99.998)
(1803, 99.998)
(1804, 100)
(1805, 100)
(1806, 99.996)
(1807, 99.998)
(1808, 99.988)
(1809, 99.998)
(1810, 99.996)
(1811, 100)
(1812, 99.994)
(1813, 99.998)
(1814, 99.988)
(1815, 99.998)
(1816, 99.878)
(1817, 99.996)
(1818, 100)
(1819, 99.986)
(1820, 99.282)
(1821, 99.92)
(1822, 99.99)
(1823, 99.99)
(1824, 99.98)
(1825, 99.98)
(1826, 99.97)
(1827, 99.986)
(1828, 99.93)
(1829, 99.986)
(1830, 99.998)
(1831, 99.944)
(1832, 99.962)
(1833, 99.978)
(1834, 99.976)
(1835, 99.988)
(1836, 99.994)
(1837, 99.956)
(1838, 99.998)
(1839, 99.992)
(1840, 99.784)
(1841, 99.992)
(1842, 99.998)
(1843, 100)
(1844, 100)
(1845, 100)
(1846, 100)
(1847, 100)
(1848, 100)
(1849, 100)
(1850, 100)
(1851, 100)
(1852, 100)
(1853, 100)
(1854, 100)
(1855, 100)
(1856, 100)
(1857, 99.996)
(1858, 99.998)
(1859, 100)
(1860, 100)
(1861, 99.996)
(1862, 100)
(1863, 100)
(1864, 100)
(1865, 99.998)
(1866, 99.998)
(1867, 99.996)
(1868, 99.956)
(1869, 99.674)
(1870, 100)
(1871, 99.992)
(1872, 99.998)
(1873, 99.994)
(1874, 99.948)
(1875, 100)
(1876, 99.986)
(1877, 99.998)
(1878, 100)
(1879, 99.942)
(1880, 99.918)
(1881, 99.732)
(1882, 99.964)
(1883, 100)
(1884, 99.98)
(1885, 99.812)
(1886, 99.984)
(1887, 99.982)
(1888, 99.998)
(1889, 100)
(1890, 99.996)
(1891, 100)
(1892, 100)
(1893, 99.992)
(1894, 100)
(1895, 99.98)
(1896, 99.99)
(1897, 99.998)
(1898, 100)
(1899, 100)
(1900, 99.998)
(1901, 99.996)
(1902, 99.996)
(1903, 99.994)
(1904, 99.992)
(1905, 99.998)
(1906, 99.996)
(1907, 99.978)
(1908, 99.97)
(1909, 99.994)
(1910, 99.99)
(1911, 99.992)
(1912, 99.986)
(1913, 99.992)
(1914, 99.988)
(1915, 99.998)
(1916, 99.964)
(1917, 99.998)
(1918, 99.998)
(1919, 99.996)
(1920, 99.996)
(1921, 99.984)
(1922, 100)
(1923, 99.994)
(1924, 99.992)
(1925, 99.998)
(1926, 99.994)
(1927, 99.992)
(1928, 99.99)
(1929, 99.994)
(1930, 99.99)
(1931, 100)
(1932, 99.998)
(1933, 99.986)
(1934, 99.616)
(1935, 96.148)
(1936, 98.712)
(1937, 99.378)
(1938, 99.078)
(1939, 99.472)
(1940, 99.086)
(1941, 99.5)
(1942, 99.196)
(1943, 99.262)
(1944, 99.346)
(1945, 98.928)
(1946, 99.18)
(1947, 99.068)
(1948, 98.968)
(1949, 99.644)
(1950, 99.48)
(1951, 99.188)
(1952, 99.436)
(1953, 99.132)
(1954, 99.454)
(1955, 99.658)
(1956, 99.652)
(1957, 99.722)
(1958, 99.826)
(1959, 99.7)
(1960, 99.218)
(1961, 99.526)
(1962, 99.584)
(1963, 99.802)
(1964, 99.752)
(1965, 99.786)
(1966, 99.718)
(1967, 99.87)
(1968, 99.772)
(1969, 99.674)
(1970, 99.924)
(1971, 99.868)
(1972, 99.818)
(1973, 99.75)
(1974, 99.76)
(1975, 99.434)
(1976, 99.554)
(1977, 99.616)
(1978, 99.486)
(1979, 99.792)
(1980, 99.322)
(1981, 99.6)
(1982, 99.416)
(1983, 99.418)
(1984, 99.122)
(1985, 99.02)
(1986, 98.228)
(1987, 98.066)
(1988, 97.14)
(1989, 96.312)
(1990, 98.708)
(1991, 98.484)
(1992, 98.686)
(1993, 99.346)
(1994, 99.404)
(1995, 99.444)
(1996, 99.294)
(1997, 99.528)
(1998, 99.476)
(1999, 99.55)
(2000, 99.518)
(2001, 99.31)
(2002, 99.506)
(2003, 99.688)
(2004, 99.606)
(2005, 99.698)
(2006, 99.29)
(2007, 99.632)
(2008, 99.704)
(2009, 99.754)
(2010, 99.82)
(2011, 99.608)
(2012, 99.592)
(2013, 99.758)
(2014, 99.456)
(2015, 98.86)
(2016, 99.61)
(2017, 99.634)
(2018, 99.72)
(2019, 99.548)
(2020, 99.554)
(2021, 99.524)
(2022, 99.718)
(2023, 99.472)
(2024, 99.81)
(2025, 99.78)
(2026, 99.762)
(2027, 99.822)
(2028, 99.78)
(2029, 99.928)
(2030, 99.742)
(2031, 99.9)
(2032, 99.832)
(2033, 99.754)
(2034, 99.782)
(2035, 99.874)
(2036, 99.884)
(2037, 99.76)
(2038, 99.818)
(2039, 99.862)
(2040, 99.872)
(2041, 99.824)
(2042, 99.812)
(2043, 99.82)
(2044, 99.716)
(2045, 99.516)
(2046, 99.82)
(2047, 99.696)
(2048, 99.534)
(2049, 99.84)
(2050, 99.846)
(2051, 99.728)
(2052, 99.922)
(2053, 99.84)
(2054, 99.852)
(2055, 99.884)
(2056, 99.69)
(2057, 99.47)
(2058, 99.182)
(2059, 99.482)
(2060, 99.736)
(2061, 99.774)
(2062, 99.542)
(2063, 99.25)
(2064, 97.646)
(2065, 99.494)
(2066, 99.344)
(2067, 99.04)
(2068, 98.824)
(2069, 99.146)
(2070, 99.262)
(2071, 99.302)
(2072, 99.03)
(2073, 99.706)
(2074, 99.562)
(2075, 99.582)
(2076, 99.792)
(2077, 99.612)
(2078, 99.806)
(2079, 99.764)
(2080, 99.632)
(2081, 99.68)
(2082, 99.754)
(2083, 99.778)
(2084, 99.77)
(2085, 99.802)
(2086, 99.806)
(2087, 99.776)
(2088, 99.788)
(2089, 99.822)
(2090, 99.702)
(2091, 99.55)
(2092, 99.742)
(2093, 99.72)
(2094, 99.75)
(2095, 99.722)
(2096, 99.744)
(2097, 99.318)
(2098, 99.638)
(2099, 99.854)
(2100, 99.924)
(2101, 99.9)
(2102, 99.898)
(2103, 99.874)
(2104, 99.826)
(2105, 99.702)
(2106, 99.706)
(2107, 99.618)
(2108, 99.64)
(2109, 99.664)
(2110, 99.722)
(2111, 99.738)
(2112, 99.554)
(2113, 99.856)
(2114, 99.906)
(2115, 99.776)
(2116, 99.792)
(2117, 99.6)
(2118, 99.832)
(2119, 99.82)
(2120, 99.892)
(2121, 99.836)
(2122, 99.9)
(2123, 99.92)
(2124, 99.826)
(2125, 99.406)
(2126, 99.986)
(2127, 100)
(2128, 99.998)
(2129, 99.894)
(2130, 99.986)
(2131, 99.992)
(2132, 99.954)
(2133, 99.964)
(2134, 99.186)
(2135, 99.5)
(2136, 99.956)
(2137, 99.81)
(2138, 99.606)
(2139, 99.766)
(2140, 99.808)
(2141, 99.636)
(2142, 99.924)
(2143, 99.424)
(2144, 99.912)
(2145, 99.89)
(2146, 99.978)
(2147, 99.956)
(2148, 99.774)
(2149, 99.782)
(2150, 99.95)
(2151, 99.902)
(2152, 99.87)
(2153, 99.94)
(2154, 99.936)
(2155, 99.798)
(2156, 99.98)
(2157, 99.85)
(2158, 99.836)
(2159, 99.91)
(2160, 99.946)
(2161, 99.988)
(2162, 99.988)
(2163, 99.996)
(2164, 99.992)
(2165, 99.984)
(2166, 99.996)
(2167, 99.938)
(2168, 100)
(2169, 99.998)
(2170, 100)
(2171, 100)
(2172, 100)
(2173, 100)
(2174, 100)
(2175, 100)
(2176, 100)
(2177, 99.996)
(2178, 100)
(2179, 99.994)
(2180, 100)
(2181, 99.996)
(2182, 99.998)
(2183, 100)
(2184, 100)
(2185, 100)
(2186, 100)
(2187, 99.926)
(2188, 99.796)
(2189, 99.998)
(2190, 100)
(2191, 100)
(2192, 99.878)
(2193, 99.962)
(2194, 100)
(2195, 100)
(2196, 100)
(2197, 99.996)
(2198, 99.946)
(2199, 99.992)
(2200, 100)
(2201, 100)
(2202, 100)
(2203, 99.996)
(2204, 100)
(2205, 99.996)
(2206, 99.974)
(2207, 99.994)
(2208, 100)
(2209, 100)
(2210, 99.972)
(2211, 99.992)
(2212, 99.998)
(2213, 99.996)
(2214, 100)
(2215, 100)
(2216, 100)
(2217, 99.998)
(2218, 99.998)
(2219, 99.996)
(2220, 99.98)
(2221, 99.994)
(2222, 99.956)
(2223, 99.994)
(2224, 99.996)
(2225, 99.988)
(2226, 99.988)
(2227, 99.974)
(2228, 99.89)
(2229, 99.998)
(2230, 99.99)
(2231, 99.998)
(2232, 99.992)
(2233, 99.932)
(2234, 99.934)
(2235, 99.792)
(2236, 99.956)
(2237, 99.91)
(2238, 99.9)
(2239, 99.856)
(2240, 99.958)
(2241, 99.218)
(2242, 99.856)
(2243, 99.868)
(2244, 99.906)
(2245, 99.53)
(2246, 99.704)
(2247, 99.792)
(2248, 99.83)
(2249, 99.912)
(2250, 99.906)
(2251, 99.844)
(2252, 99.79)
(2253, 99.84)
(2254, 99.6)
(2255, 99.7)
(2256, 99.772)
(2257, 99.852)
(2258, 99.768)
(2259, 99.652)
(2260, 99.736)
(2261, 99.748)
(2262, 99.768)
(2263, 99.596)
(2264, 99.824)
(2265, 99.654)
(2266, 98.852)
(2267, 99.744)
(2268, 99.536)
(2269, 99.518)
(2270, 99.634)
(2271, 99.692)
(2272, 99.396)
(2273, 99.7)
(2274, 99.514)
(2275, 99.53)
(2276, 99.79)
(2277, 99.632)
(2278, 99.832)
(2279, 99.702)
(2280, 99.802)
(2281, 99.352)
(2282, 99.518)
(2283, 98.99)
(2284, 99.764)
(2285, 99.462)
(2286, 99.758)
(2287, 99.818)
(2288, 99.636)
(2289, 99.814)
(2290, 99.78)
(2291, 99.912)
(2292, 99.912)
(2293, 99.844)
(2294, 99.744)
(2295, 99.79)
(2296, 99.832)
(2297, 99.766)
(2298, 98.868)
(2299, 99.898)
(2300, 99.962)
(2301, 99.99)
(2302, 99.974)
(2303, 99.958)
(2304, 99.878)
(2305, 99.96)
(2306, 99.982)
(2307, 99.968)
(2308, 99.994)
(2309, 99.984)
(2310, 99.978)
(2311, 99.984)
(2312, 99.99)
(2313, 99.998)
(2314, 99.944)
(2315, 99.81)
(2316, 99.97)
(2317, 99.95)
(2318, 99.946)
(2319, 99.986)
(2320, 99.97)
(2321, 99.962)
(2322, 99.978)
(2323, 99.904)
(2324, 99.938)
(2325, 99.888)
(2326, 99.96)
(2327, 99.996)
(2328, 99.998)
(2329, 99.998)
(2330, 99.932)
(2331, 99.986)
(2332, 99.984)
(2333, 99.944)
(2334, 99.986)
(2335, 99.998)
(2336, 99.994)
(2337, 99.974)
(2338, 99.918)
(2339, 99.992)
(2340, 99.956)
(2341, 99.968)
(2342, 99.862)
(2343, 99.936)
(2344, 99.764)
(2345, 99.962)
(2346, 99.976)
(2347, 99.836)
(2348, 99.98)
(2349, 99.996)
(2350, 99.982)
(2351, 99.97)
(2352, 99.958)
(2353, 99.964)
(2354, 99.996)
(2355, 100)
(2356, 99.998)
(2357, 99.998)
(2358, 100)
(2359, 100)
(2360, 99.998)
(2361, 100)
(2362, 100)
(2363, 100)
(2364, 99.998)
(2365, 100)
(2366, 100)
(2367, 100)
(2368, 100)
(2369, 100)
(2370, 100)
(2371, 100)
(2372, 99.996)
(2373, 100)
(2374, 99.998)
(2375, 99.996)
(2376, 100)
(2377, 99.996)
(2378, 100)
(2379, 100)
(2380, 100)
(2381, 100)
(2382, 99.996)
(2383, 99.95)
(2384, 99.996)
(2385, 100)
(2386, 99.94)
(2387, 99.994)
(2388, 100)
(2389, 100)
(2390, 100)
(2391, 99.998)
(2392, 100)
(2393, 100)
(2394, 100)
(2395, 100)
(2396, 100)
(2397, 100)
(2398, 100)
(2399, 100)
(2400, 99.99)
(2401, 100)
(2402, 100)
(2403, 100)
(2404, 100)
(2405, 99.994)
(2406, 99.996)
(2407, 99.958)
(2408, 99.998)
(2409, 99.986)
(2410, 99.992)
(2411, 99.982)
(2412, 99.964)
(2413, 99.984)
(2414, 100)
(2415, 100)
(2416, 100)
(2417, 100)
(2418, 99.994)
(2419, 100)
(2420, 100)
(2421, 100)
(2422, 100)
(2423, 100)
(2424, 100)
(2425, 99.998)
(2426, 100)
(2427, 100)
(2428, 100)
(2429, 100)
(2430, 100)
(2431, 100)
(2432, 100)
(2433, 100)
(2434, 100)
(2435, 100)
(2436, 100)
(2437, 100)
(2438, 100)
(2439, 100)
(2440, 100)
(2441, 100)
(2442, 99.964)
(2443, 100)
(2444, 100)
(2445, 100)
(2446, 100)
(2447, 100)
(2448, 100)
(2449, 100)
(2450, 100)
(2451, 100)
(2452, 100)
(2453, 100)
(2454, 99.972)
(2455, 100)
(2456, 100)
(2457, 100)
(2458, 100)
(2459, 100)
(2460, 99.998)
(2461, 100)
(2462, 100)
(2463, 99.996)
(2464, 100)
(2465, 100)
(2466, 100)
(2467, 100)
(2468, 99.998)
(2469, 100)
(2470, 99.998)
(2471, 100)
(2472, 99.998)
(2473, 99.998)
(2474, 99.97)
(2475, 99.998)
(2476, 99.992)
(2477, 99.882)
(2478, 99.992)
(2479, 99.996)
(2480, 99.996)
(2481, 99.992)
(2482, 100)
(2483, 99.988)
(2484, 99.994)
(2485, 99.992)
(2486, 100)
(2487, 99.998)
(2488, 99.986)
(2489, 99.994)
(2490, 99.998)
(2491, 99.99)
(2492, 100)
(2493, 100)
(2494, 99.998)
(2495, 99.996)
(2496, 99.954)
(2497, 99.966)
(2498, 99.948)
(2499, 99.766)
(2500, 99.98)
(2501, 99.952)
(2502, 99.902)
(2503, 99.964)
(2504, 99.948)
(2505, 99.98)
(2506, 99.928)
(2507, 99.826)
(2508, 99.81)
(2509, 99.932)
(2510, 99.928)
(2511, 99.96)
(2512, 99.898)
(2513, 99.912)
(2514, 99.85)
(2515, 99.844)
(2516, 99.276)
(2517, 98.25)
(2518, 98.404)
(2519, 98.278)
(2520, 97.948)
(2521, 97.54)
(2522, 97.984)
(2523, 92.884)
(2524, 93.472)
(2525, 94.146)
(2526, 91.864)
(2527, 92.044)
(2528, 94.818)
(2529, 90.932)
(2530, 93.65)
(2531, 89.696)
(2532, 93.064)
(2533, 94.066)
(2534, 94.678)
(2535, 94.902)
(2536, 86.488)
(2537, 90.406)
(2538, 93.608)
(2539, 95.372)
(2540, 94.812)
(2541, 89.882)
(2542, 95.636)
(2543, 94.318)
(2544, 94.594)
(2545, 97.152)
(2546, 95.028)
(2547, 95.078)
(2548, 94.784)
(2549, 95.288)
(2550, 92.858)
(2551, 93.618)
(2552, 90.258)
(2553, 94.614)
(2554, 95.538)
(2555, 92.944)
(2556, 91.904)
(2557, 96.59)
(2558, 94.326)
(2559, 94.138)
(2560, 93.652)
(2561, 84.918)
(2562, 92.702)
(2563, 90.79)
(2564, 94.178)
(2565, 93.69)
(2566, 93.816)
(2567, 94.98)
(2568, 95.842)
(2569, 93.234)
(2570, 95.312)
(2571, 96.6)
(2572, 97.43)
(2573, 98.334)
(2574, 98.636)
(2575, 98.402)
(2576, 98.372)
(2577, 98.348)
(2578, 98.086)
(2579, 98.444)
(2580, 98.916)
(2581, 98.666)
(2582, 98.692)
(2583, 98.672)
(2584, 99.2)
(2585, 99.232)
(2586, 99.206)
(2587, 98.028)
(2588, 97.506)
(2589, 98.882)
(2590, 99.014)
(2591, 98.512)
(2592, 98.384)
(2593, 98.664)
(2594, 98.894)
(2595, 99.138)
(2596, 99.044)
(2597, 95.82)
(2598, 99.054)
(2599, 99.228)
(2600, 99.326)
(2601, 99.196)
(2602, 99.12)
(2603, 99.12)
(2604, 98.488)
(2605, 99.186)
(2606, 99.294)
(2607, 98.928)
(2608, 99.374)
(2609, 99.264)
(2610, 99.258)
(2611, 98.96)
(2612, 98.896)
(2613, 99.302)
(2614, 99.444)
(2615, 99.394)
(2616, 99.526)
(2617, 99.34)
(2618, 97.422)
(2619, 99.064)
(2620, 98.896)
(2621, 99.296)
(2622, 99.174)
(2623, 99.354)
(2624, 98.868)
(2625, 99.52)
(2626, 99.314)
(2627, 98.696)
(2628, 98.332)
(2629, 98.68)
(2630, 98.498)
(2631, 97.966)
(2632, 98.298)
(2633, 98.194)
(2634, 97.984)
(2635, 97.002)
(2636, 94.7)
(2637, 95.144)
(2638, 96.984)
(2639, 96.318)
(2640, 96.682)
(2641, 98.358)
(2642, 97.296)
(2643, 97.532)
(2644, 98.452)
(2645, 98.124)
(2646, 98.676)
(2647, 97.764)
(2648, 98.148)
(2649, 97.958)
(2650, 98.146)
(2651, 97.996)
(2652, 97.514)
(2653, 98.006)
(2654, 98.088)
(2655, 98.064)
(2656, 98.392)
(2657, 98.8)
(2658, 98.252)
(2659, 98.552)
(2660, 98.968)
(2661, 98.652)
(2662, 98.562)
(2663, 98.834)
(2664, 98.894)
(2665, 98.772)
(2666, 98.582)
(2667, 97.94)
(2668, 97.344)
(2669, 97.936)
(2670, 97.416)
(2671, 98.474)
(2672, 97.948)
(2673, 98.914)
(2674, 98.92)
(2675, 98.466)
(2676, 98.226)
(2677, 97.802)
(2678, 98.152)
(2679, 98.84)
(2680, 98.422)
(2681, 98.422)
(2682, 98.962)
(2683, 99.142)
(2684, 98.878)
(2685, 98.768)
(2686, 98.708)
(2687, 99.124)
(2688, 98.754)
(2689, 97.166)
(2690, 97.65)
(2691, 97.286)
(2692, 97.674)
(2693, 97.816)
(2694, 98.406)
(2695, 97.73)
(2696, 98.168)
(2697, 98.784)
(2698, 96.854)
(2699, 97.978)
(2700, 97.57)
(2701, 97.114)
(2702, 97.622)
(2703, 95.836)
(2704, 95.588)
(2705, 96.532)
(2706, 97.302)
(2707, 95.42)
(2708, 92.052)
(2709, 96.164)
(2710, 97.532)
(2711, 95.38)
(2712, 94.726)
(2713, 92.94)
(2714, 94.382)
(2715, 91.71)
(2716, 87.2)
(2717, 92.868)
(2718, 92.528)
(2719, 93.57)
(2720, 94.074)
(2721, 92.09)
(2722, 87.69)
(2723, 87.758)
(2724, 91.114)
(2725, 90.47)
(2726, 87.136)
(2727, 92.102)
(2728, 88.322)
(2729, 92.472)
(2730, 93.616)
(2731, 92.728)
(2732, 91.69)
(2733, 95.216)
(2734, 94.012)
(2735, 94.528)
(2736, 96.016)
(2737, 96.746)
(2738, 94.572)
(2739, 96.562)
(2740, 95.624)
(2741, 94.044)
(2742, 89.892)
(2743, 95.546)
(2744, 92.792)
(2745, 93.394)
(2746, 89.374)
(2747, 93.35)
(2748, 90.684)
(2749, 87.812)
(2750, 89.5)
(2751, 93.954)
(2752, 95.604)
(2753, 94.49)
(2754, 92.742)
(2755, 96.208)
(2756, 96.13)
(2757, 93.418)
(2758, 93.682)
(2759, 97.39)
(2760, 95.154)
(2761, 95.874)
(2762, 97.624)
(2763, 96.994)
(2764, 97.016)
(2765, 93.328)
(2766, 94.508)
(2767, 95.65)
(2768, 96.804)
(2769, 97.764)
(2770, 96.58)
(2771, 97.104)
(2772, 97.986)
(2773, 98.238)
(2774, 98.066)
(2775, 98.34)
(2776, 98.034)
(2777, 99.008)
(2778, 97.75)
(2779, 98.746)
(2780, 98.606)
(2781, 98.716)
(2782, 98.29)
(2783, 98.39)
(2784, 98.77)
(2785, 98.612)
(2786, 98.294)
(2787, 98.654)
(2788, 99.816)
(2789, 99.934)
(2790, 99.082)
(2791, 98.326)
(2792, 97.43)
(2793, 97.814)
(2794, 97.166)
(2795, 97.594)
(2796, 97.898)
(2797, 98.158)
(2798, 96.4)
(2799, 97.722)
(2800, 96.862)
(2801, 95.696)
(2802, 96.71)
(2803, 96.264)
(2804, 96.976)
(2805, 97.278)
(2806, 97.658)
(2807, 98.082)
(2808, 96.59)
(2809, 97.912)
(2810, 97.144)
(2811, 98.214)
(2812, 96.642)
(2813, 97.906)
(2814, 97.208)
(2815, 95.102)
(2816, 98.072)
(2817, 97.7)
(2818, 97.954)
(2819, 98.218)
(2820, 96.128)
(2821, 96.948)
(2822, 96.114)
(2823, 94.68)
(2824, 92.492)
(2825, 92.278)
(2826, 77.8)
(2827, 81.494)
(2828, 82.54)
(2829, 81.008)
(2830, 89.954)
(2831, 58.38)
(2832, 75.65)
(2833, 64.954)
(2834, 64.464)
(2835, 53.782)
(2836, 55.806)
(2837, 73.344)
(2838, 48.932)
(2839, 67.782)
(2840, 36.878)
(2841, 63.722)
(2842, 70.12)
(2843, 76.534)
(2844, 73.74)
(2845, 84.68)
(2846, 64.874)
(2847, 72.718)
(2848, 87.79)
(2849, 81.044)
(2850, 80.818)
(2851, 95.034)
(2852, 98.35)
(2853, 91.306)
(2854, 77.044)
(2855, 40.466)
(2856, 58.428)
(2857, 86.442)
(2858, 89.258)
(2859, 84.614)
(2860, 85.634)
(2861, 87.282)
(2862, 84.234)
(2863, 88.242)
(2864, 89.85)
(2865, 91.098)
(2866, 92.796)
(2867, 92.06)
(2868, 88.622)
(2869, 89.254)
(2870, 79.33)
(2871, 73.474)
(2872, 81.506)
(2873, 54.984)
(2874, 85.54)
(2875, 64.904)
(2876, 61.592)
(2877, 54.276)
(2878, 72.47)
(2879, 83.874)
(2880, 73.308)
(2881, 73.336)
(2882, 69.906)
(2883, 64.298)
(2884, 74.286)
(2885, 49.094)
(2886, 64.966)
(2887, 77.788)
(2888, 67.116)
(2889, 65.34)
(2890, 50.562)
(2891, 58.95)
(2892, 33.1)
(2893, 66.794)
(2894, 59.614)
(2895, 71.596)
(2896, 37.95)
(2897, 61.82)
(2898, 65.81)
(2899, 52.952)
(2900, 60.374)
(2901, 58.472)
(2902, 43.108)
(2903, 10.1)
(2904, 23.054)
(2905, 28.388)
(2906, 59.638)
(2907, 45.008)
(2908, 34.448)
(2909, 30.144)
(2910, 15.298)
(2911, 13.88)
(2912, 39.93)
(2913, 51.658)
(2914, 44.172)
(2915, 5.384)
(2916, 52.598)
(2917, 38.328)
(2918, 52.362)
(2919, 44.668)
(2920, 54.786)
(2921, 37.928)
(2922, 74.408)
(2923, 74.27)
(2924, 63.442)
(2925, 74.728)
(2926, 83.172)
(2927, 89.19)
(2928, 76.45)
(2929, 79.076)
(2930, 87.58)
(2931, 92.92)
(2932, 99.986)
(2933, 98.76)
(2934, 95.92)
(2935, 98.504)
(2936, 97.692)
(2937, 91.928)
(2938, 94.728)
(2939, 93.662)
(2940, 93.86)
(2941, 89.964)
(2942, 94.174)
(2943, 93.872)
(2944, 96.548)
(2945, 94.592)
(2946, 95.118)
(2947, 97.536)
(2948, 98.156)
(2949, 98.062)
(2950, 97.272)
(2951, 98.334)
(2952, 97.188)
(2953, 98.076)
(2954, 97.778)
(2955, 96.736)
(2956, 95.352)
(2957, 97.178)
(2958, 97.048)
(2959, 95.498)
(2960, 96.888)
(2961, 96.906)
(2962, 97.216)
(2963, 96.868)
(2964, 96.676)
(2965, 97.982)
(2966, 94.9)
(2967, 95.386)
(2968, 96.026)
(2969, 97.448)
(2970, 95.96)
(2971, 97.94)
(2972, 97.97)
(2973, 97.726)
(2974, 96.832)
(2975, 98.006)
(2976, 98.126)
(2977, 98.866)
(2978, 98.148)
(2979, 98.228)
(2980, 98.35)
(2981, 98.454)
(2982, 97.346)
(2983, 95.3)
(2984, 98.776)
(2985, 98.396)
(2986, 98.49)
(2987, 98.552)
(2988, 98.346)
(2989, 98.674)
(2990, 98.546)
(2991, 98.24)
(2992, 96.216)
(2993, 98.932)
(2994, 98.8)
(2995, 98.806)
(2996, 98.526)
(2997, 98.032)
(2998, 98.226)
(2999, 98.788)
(3000, 98.926)
(3001, 98.702)
(3002, 99.13)
(3003, 99.226)
(3004, 98.742)
(3005, 97.834)
(3006, 98.246)
(3007, 98.42)
(3008, 99.026)
(3009, 98.818)
(3010, 99.078)
(3011, 98.66)
(3012, 98.488)
(3013, 99.272)
(3014, 99.042)
(3015, 99.296)
(3016, 98.456)
(3017, 98.364)
(3018, 98.696)
(3019, 98.12)
(3020, 99.002)
(3021, 98.524)
(3022, 99.034)
(3023, 98.608)
(3024, 98.876)
(3025, 98.462)
(3026, 98.942)
(3027, 99.142)
(3028, 99.01)
(3029, 99.236)
(3030, 99.196)
(3031, 98.64)
(3032, 99.15)
(3033, 99.11)
(3034, 98.774)
(3035, 98.892)
(3036, 98.236)
(3037, 99.67)
(3038, 99.296)
(3039, 98.9)
(3040, 98.698)
(3041, 97.532)
(3042, 99.19)
(3043, 98.586)
(3044, 99.174)
(3045, 98.554)
(3046, 98.212)
(3047, 98.336)
(3048, 98.868)
(3049, 98.8)
(3050, 99.164)
(3051, 98.99)
(3052, 95.558)
(3053, 97.392)
(3054, 96.998)
(3055, 99.224)
(3056, 99.3)
(3057, 99.644)
(3058, 99.768)
(3059, 99.902)
(3060, 99.916)
(3061, 99.936)
(3062, 99.78)
(3063, 99.804)
(3064, 99.608)
(3065, 99.628)
(3066, 99.782)
(3067, 99.744)
(3068, 99.634)
(3069, 99.56)
(3070, 98.908)
(3071, 99.34)
(3072, 99.002)
(3073, 97.572)
(3074, 98.556)
(3075, 98.374)
(3076, 98.832)
(3077, 97.848)
(3078, 98.448)
(3079, 96.84)
(3080, 96.544)
(3081, 98.454)
(3082, 98.678)
(3083, 99.326)
(3084, 99.406)
(3085, 99.508)
(3086, 99.698)
(3087, 99.448)
(3088, 99.124)
(3089, 99.422)
(3090, 98.684)
(3091, 98.842)
(3092, 99.214)
(3093, 98.902)
(3094, 99.16)
(3095, 98.468)
(3096, 99.318)
(3097, 98.324)
(3098, 99.264)
(3099, 99.336)
(3100, 99.566)
(3101, 99.354)
(3102, 98.374)
(3103, 98.666)
(3104, 96.544)
(3105, 97.876)
(3106, 96.248)
(3107, 98.498)
(3108, 98.798)
(3109, 96.518)
(3110, 97.014)
(3111, 95.982)
(3112, 95.726)
(3113, 96.78)
(3114, 89.97)
(3115, 79.25)
(3116, 0)
(3117, 33.936)
(3118, 0.012)
(3119, 0)
(3120, 10.1)
(3121, 0)
(3122, 31.676)
(3123, 25.162)
(3124, 58.636)
(3125, 11.73)
(3126, 26.996)
(3127, 22.192)
(3128, 20.09)
(3129, 14.098)
(3130, 0)
(3131, 0)
(3132, 20.2)
(3133, 10.1)
(3134, 10.1)
(3135, 44.966)
(3136, 18.13)
(3137, 69.328)
(3138, 81.63)
(3139, 71.522)
(3140, 17.914)
(3141, 82.09)
(3142, 82.344)
(3143, 84.576)
(3144, 93.038)
(3145, 93.346)
(3146, 89.766)
(3147, 92.862)
(3148, 92.508)
(3149, 92.97)
(3150, 94.448)
(3151, 93.634)
(3152, 95.022)
(3153, 97.204)
(3154, 95.706)
(3155, 97.122)
(3156, 97.696)
(3157, 96.62)
(3158, 97.198)
(3159, 92.692)
(3160, 97.592)
(3161, 97.71)
(3162, 97.85)
(3163, 98.462)
(3164, 98.352)
(3165, 97.868)
(3166, 97.52)
(3167, 97.982)
(3168, 98.424)
(3169, 98.426)
(3170, 98.322)
(3171, 98.362)
(3172, 98.982)
(3173, 98.894)
(3174, 98.716)
(3175, 98.98)
(3176, 98.978)
(3177, 98.996)
(3178, 96.912)
(3179, 98.636)
(3180, 97.564)
(3181, 98.412)
(3182, 96.476)
(3183, 95.814)
(3184, 94.45)
(3185, 95.248)
(3186, 94.664)
(3187, 96.29)
(3188, 96.326)
(3189, 95.848)
(3190, 94.526)
(3191, 90.704)
(3192, 93.764)
(3193, 91.586)
(3194, 92.476)
(3195, 88.932)
(3196, 89.546)
(3197, 79.948)
(3198, 93.13)
(3199, 85.308)
(3200, 87.824)
(3201, 84.49)
(3202, 65.486)
(3203, 74.346)
(3204, 78.532)
(3205, 80.45)
(3206, 81.95)
(3207, 84.342)
(3208, 89.708)
(3209, 82.932)
(3210, 92.564)
(3211, 88.036)
(3212, 92.698)
(3213, 91.602)
(3214, 90.792)
(3215, 90.104)
(3216, 91.438)
(3217, 92.806)
(3218, 89.954)
(3219, 89.32)
(3220, 86.382)
(3221, 87.516)
(3222, 89.116)
(3223, 81.594)
(3224, 81.564)
(3225, 89.674)
(3226, 88.446)
(3227, 87.138)
(3228, 90.084)
(3229, 83.69)
(3230, 82.85)
(3231, 86.44)
(3232, 85.498)
(3233, 89.37)
(3234, 82.716)
(3235, 73.204)
(3236, 82.786)
(3237, 69.642)
(3238, 85.636)
(3239, 77.112)
(3240, 74.272)
(3241, 60.392)
(3242, 70.216)
(3243, 81.478)
(3244, 76.874)
(3245, 84.01)
(3246, 67.108)
(3247, 77.728)
(3248, 56.326)
(3249, 40.86)
(3250, 56.636)
(3251, 59.65)
(3252, 68.826)
(3253, 73.748)
(3254, 38.152)
(3255, 59.972)
(3256, 45.778)
(3257, 25.914)
(3258, 62.886)
(3259, 86.814)
(3260, 85.546)
(3261, 86.952)
(3262, 85.62)
(3263, 82.07)
(3264, 76.906)
(3265, 87.764)
(3266, 76.62)
(3267, 84.04)
(3268, 87.428)
(3269, 86.618)
(3270, 90.458)
(3271, 84.31)
(3272, 90.552)
(3273, 87.812)
(3274, 88.504)
(3275, 100)
(3276, 100)
(3277, 100)
(3278, 100)
(3279, 100)
(3280, 95.48)
(3281, 83.158)
(3282, 82.858)
(3283, 85.456)
(3284, 65.892)
(3285, 83.344)
(3286, 86.988)
(3287, 92.654)
(3288, 85.576)
(3289, 89.456)
(3290, 84.378)
(3291, 85.698)
(3292, 90.94)
(3293, 89.404)
(3294, 84.73)
(3295, 80.948)
(3296, 82.71)
(3297, 88.658)
(3298, 99.008)
(3299, 93.734)
(3300, 93.534)
(3301, 93.08)
(3302, 90.164)
(3303, 92.066)
(3304, 90.568)
(3305, 93.054)
(3306, 92.44)
(3307, 93.426)
(3308, 94.934)
(3309, 95.546)
(3310, 96.236)
(3311, 92.522)
(3312, 88.744)
(3313, 92.264)
(3314, 92.178)
(3315, 91.598)
(3316, 85.998)
(3317, 91.422)
(3318, 85.928)
(3319, 89.086)
(3320, 94.366)
(3321, 92.6)
(3322, 87.01)
(3323, 91.146)
(3324, 95.104)
(3325, 92.83)
(3326, 95.33)
(3327, 92.694)
(3328, 93.95)
(3329, 93.708)
(3330, 95.66)
(3331, 93.118)
(3332, 91.306)
(3333, 93.21)
(3334, 91.968)
(3335, 91.08)
(3336, 95.406)
(3337, 93.374)
(3338, 93.058)
(3339, 93.506)
(3340, 93.678)
(3341, 88.54)
(3342, 92.27)
(3343, 96.512)
(3344, 95.07)
(3345, 94.12)
(3346, 95.958)
(3347, 92.462)
(3348, 93.9)
(3349, 91.544)
(3350, 91.964)
(3351, 95.342)
(3352, 95.434)
(3353, 95.632)
(3354, 92.786)
(3355, 93.674)
(3356, 94.426)
(3357, 94.27)
(3358, 94.514)
(3359, 93.804)
(3360, 96.726)
(3361, 96.518)
(3362, 95.216)
(3363, 94.234)
(3364, 93.96)
(3365, 92.624)
(3366, 96.254)
(3367, 94.928)
(3368, 93.182)
(3369, 91.288)
(3370, 93.002)
(3371, 93.404)
(3372, 93.41)
(3373, 94.562)
(3374, 93.738)
(3375, 95.006)
(3376, 94.536)
(3377, 94.696)
(3378, 95.684)
(3379, 92.424)
(3380, 93.868)
(3381, 92.764)
(3382, 91.886)
(3383, 90.632)
(3384, 85.152)
(3385, 88.534)
(3386, 90.634)
(3387, 91.458)
(3388, 84.128)
(3389, 92.678)
(3390, 89.56)
(3391, 91.65)
(3392, 91.322)
(3393, 89.732)
(3394, 89.774)
(3395, 80.896)
(3396, 82.91)
(3397, 89.858)
(3398, 89.966)
(3399, 84.088)
(3400, 85.992)
(3401, 89.418)
(3402, 87.306)
(3403, 85.888)
(3404, 92.674)
(3405, 94.706)
(3406, 90.374)
(3407, 87.088)
(3408, 84.998)
(3409, 88.928)
(3410, 83.744)
(3411, 85.788)
(3412, 87.888)
(3413, 78.746)
(3414, 89.828)
(3415, 93.37)
(3416, 88.568)
(3417, 92.598)
(3418, 92.7)
(3419, 94.678)
(3420, 96.596)
(3421, 94.312)
(3422, 91.12)
(3423, 94.682)
(3424, 93.434)
(3425, 95.074)
(3426, 92.084)
(3427, 91.48)
(3428, 92.96)
(3429, 93.65)
(3430, 92.828)
(3431, 89.136)
(3432, 94.288)
(3433, 91.882)
(3434, 91.34)
(3435, 95.184)
(3436, 94.726)
(3437, 94.968)
(3438, 95.236)
(3439, 91.608)
(3440, 91.356)
(3441, 91.452)
(3442, 92.54)
(3443, 88.556)
(3444, 88.342)
(3445, 89.15)
(3446, 91.256)
(3447, 90.328)
(3448, 94.354)
(3449, 84.002)
(3450, 86.988)
(3451, 87.88)
(3452, 91.87)
(3453, 83.324)
(3454, 80.658)
(3455, 83.062)
(3456, 91.034)
(3457, 87.508)
(3458, 90.2)
(3459, 93.298)
(3460, 92.578)
(3461, 92.188)
(3462, 95.114)
(3463, 94.714)
(3464, 97.502)
(3465, 95.048)
(3466, 97.368)
(3467, 96.676)
(3468, 96.318)
(3469, 91.724)
(3470, 94.602)
(3471, 96.914)
(3472, 94.644)
(3473, 93.13)
(3474, 96.286)
(3475, 93.09)
(3476, 94.878)
(3477, 94.706)
(3478, 95.92)
(3479, 96.04)
(3480, 96.772)
(3481, 96.27)
(3482, 96.978)
(3483, 95.124)
(3484, 94.534)
(3485, 93.296)
(3486, 95.264)
(3487, 92.686)
(3488, 93.12)
(3489, 91.85)
(3490, 88.02)
(3491, 91.726)
(3492, 92.028)
(3493, 90.768)
(3494, 89.602)
(3495, 89.342)
(3496, 83.496)
(3497, 82.546)
(3498, 75.644)
(3499, 78.144)
(3500, 74.454)
(3501, 55.596)
(3502, 71.112)
(3503, 70.622)
(3504, 56.482)
(3505, 69.304)
(3506, 32.294)
(3507, 51.304)
(3508, 26.204)
(3509, 0.002)
(3510, 0)
(3511, 24.804)
(3512, 28.684)
(3513, 8.596)
(3514, 5.7)
(3515, 0)
(3516, 0)
(3517, 0)
(3518, 0)
(3519, 20.2)
(3520, 0)
(3521, 0)
(3522, 10.1)
(3523, 0)
(3524, 0)
(3525, 23.646)
(3526, 16.742)
(3527, 7.844)
(3528, 12.428)
(3529, 10.228)
(3530, 0)
(3531, 0)
(3532, 0)
(3533, 0)
(3534, 0)
(3535, 0)
(3536, 0)
(3537, 0)
(3538, 0)
(3539, 0)
(3540, 0)
(3541, 13.07)
(3542, 0)
(3543, 17.65)
(3544, 0)
(3545, 0)
(3546, 0)
(3547, 0)
(3548, 0)
(3549, 3.938)
(3550, 24.01)
(3551, 0)
(3552, 20.2)
(3553, 5.408)
(3554, 14.792)
(3555, 32.398)
(3556, 21.818)
(3557, 22.364)
(3558, 39.286)
(3559, 0)
(3560, 0)
(3561, 13.368)
(3562, 18.842)
(3563, 19.03)
(3564, 23.732)
(3565, 43.418)
(3566, 0)
(3567, 26.98)
(3568, 6.856)
(3569, 29.624)
(3570, 22.746)
(3571, 19.3)
(3572, 41.486)
(3573, 16.902)
(3574, 40.434)
(3575, 50.368)
(3576, 5.256)
(3577, 0)
(3578, 6.006)
(3579, 10.1)
(3580, 20.2)
(3581, 26.14)
(3582, 17.756)
(3583, 55.608)
(3584, 40.732)
(3585, 20.2)
(3586, 26.94)
(3587, 27.392)
(3588, 39.716)
(3589, 28.49)
(3590, 7.086)
(3591, 8.03)
(3592, 18.318)
(3593, 58.41)
(3594, 9.968)
(3595, 23.586)
(3596, 25.346)
(3597, 37.9)
(3598, 14.844)
(3599, 20.2)
(3600, 11.432)
(3601, 18.276)
(3602, 35.426)
(3603, 21.98)
(3604, 2.142)
(3605, 0)
(3606, 0.488)
(3607, 0)
(3608, 10.1)
(3609, 0)
(3610, 20.2)
(3611, 39.896)
(3612, 20.452)
(3613, 23.658)
(3614, 14.124)
(3615, 39.938)
(3616, 9.828)
(3617, 21.26)
(3618, 30.3)
(3619, 10.112)
(3620, 16.95)
(3621, 31.288)
(3622, 18.718)
(3623, 31.306)
(3624, 3.872)
(3625, 20.2)
(3626, 0)
(3627, 0)
(3628, 18.038)
(3629, 19.392)
(3630, 2.97)
(3631, 0)
(3632, 0)
(3633, 20.2)
(3634, 0)
(3635, 0)
(3636, 23.16)
(3637, 19.282)
(3638, 21.136)
(3639, 0)
(3640, 0)
(3641, 10.13)
(3642, 15.502)
(3643, 0)
(3644, 10.21)
(3645, 9.9)
(3646, 0)
(3647, 0)
(3648, 0)
(3649, 0)
(3650, 10.1)
(3651, 0)
(3652, 0)
(3653, 0)
(3654, 0)
(3655, 0)
(3656, 0)
(3657, 0)
(3658, 0)
(3659, 0)
(3660, 10.1)
(3661, 16.918)
(3662, 0)
(3663, 0)
(3664, 0)
(3665, 0)
(3666, 0)
(3667, 0)
(3668, 17.944)
(3669, 0)
(3670, 0)
(3671, 0)
(3672, 0)
(3673, 0)
(3674, 0)
(3675, 0)
(3676, 0)
(3677, 0)
(3678, 0)
(3679, 15.778)
(3680, 0)
(3681, 0)
(3682, 0)
(3683, 0)
(3684, 14.944)
(3685, 11.066)
(3686, 0)
(3687, 0)
(3688, 0)
(3689, 0)
(3690, 0)
(3691, 0)
(3692, 10.1)
(3693, 16.294)
(3694, 8.742)
(3695, 10.1)
(3696, 10.1)
(3697, 0)
(3698, 0)
(3699, 0.02)
(3700, 0)
(3701, 10.062)
(3702, 43.47)
(3703, 68.082)
(3704, 47.12)
(3705, 23.316)
(3706, 27.644)
(3707, 28.518)
(3708, 0)
(3709, 10.21)
(3710, 10.21)
(3711, 0)
(3712, 19.606)
(3713, 0)
(3714, 10.1)
(3715, 10.1)
(3716, 0.756)
(3717, 9.108)
(3718, 36.778)
(3719, 26.376)
(3720, 28.742)
(3721, 0.788)
(3722, 18.86)
(3723, 29.558)
(3724, 40.286)
(3725, 56.038)
(3726, 57.238)
(3727, 70.066)
(3728, 62.19)
(3729, 71.844)
(3730, 76.31)
(3731, 74.426)
(3732, 71.536)
(3733, 83.416)
(3734, 77.692)
(3735, 81.586)
(3736, 78.666)
(3737, 80.164)
(3738, 86.762)
(3739, 86.952)
(3740, 72.98)
(3741, 56.782)
(3742, 71.28)
(3743, 68.5)
(3744, 80.922)
(3745, 78.014)
(3746, 78.1)
(3747, 67.328)
(3748, 72.994)
(3749, 71.31)
(3750, 44.254)
(3751, 75.102)
(3752, 78.144)
(3753, 81.472)
(3754, 76.828)
(3755, 79.33)
(3756, 80.934)
(3757, 84.092)
(3758, 77.376)
(3759, 71.162)
(3760, 76.53)
(3761, 86.578)
(3762, 90.016)
(3763, 83.004)
(3764, 87.592)
(3765, 85.524)
(3766, 81.978)
(3767, 90.926)
(3768, 90.456)
(3769, 91.138)
(3770, 91.904)
(3771, 92.352)
(3772, 91.314)
(3773, 91.078)
(3774, 92.29)
(3775, 92.056)
(3776, 84.378)
(3777, 79.416)
(3778, 87.874)
(3779, 88.92)
(3780, 91.306)
(3781, 88.642)
(3782, 88.78)
(3783, 93.762)
(3784, 95.708)
(3785, 95.646)
(3786, 94.882)
(3787, 93.782)
(3788, 92.03)
(3789, 94.62)
(3790, 94.87)
(3791, 94.094)
(3792, 96.274)
(3793, 95.688)
(3794, 96.576)
(3795, 94.402)
(3796, 95.696)
(3797, 96.326)
(3798, 96.592)
(3799, 98.268)
(3800, 97.788)
(3801, 98.182)
(3802, 99)
(3803, 98.808)
(3804, 98.15)
(3805, 98.68)
(3806, 99.162)
(3807, 97.83)
(3808, 98.85)
(3809, 98.604)
(3810, 99.324)
(3811, 99.542)
(3812, 99.624)
(3813, 99.642)
(3814, 99.554)
(3815, 99.354)
(3816, 99.07)
(3817, 98.454)
(3818, 97.516)
(3819, 98.536)
(3820, 98.29)
(3821, 98.942)
(3822, 97.958)
(3823, 97.256)
(3824, 98.208)
(3825, 98.21)
(3826, 96.63)
(3827, 97.95)
(3828, 98.254)
(3829, 97.382)
(3830, 98.016)
(3831, 97.288)
(3832, 97.366)
(3833, 97.28)
(3834, 97.634)
(3835, 98.016)
(3836, 98.324)
(3837, 98.62)
(3838, 98.346)
(3839, 98.4)
(3840, 98.898)
(3841, 99.006)
(3842, 98.958)
(3843, 98.958)
(3844, 98.55)
(3845, 98.758)
(3846, 99.02)
(3847, 99.222)
(3848, 98.812)
(3849, 99.028)
(3850, 99.3)
(3851, 98.886)
(3852, 99.18)
(3853, 99.248)
(3854, 99.09)
(3855, 99.13)
(3856, 99.248)
(3857, 99.036)
(3858, 99.324)
(3859, 99.152)
(3860, 99.054)
(3861, 99.066)
(3862, 99.078)
(3863, 98.782)
(3864, 98.914)
(3865, 99.334)
(3866, 99.496)
(3867, 99.342)
(3868, 99.306)
(3869, 99.45)
(3870, 99.152)
(3871, 99.216)
(3872, 99.134)
(3873, 99.214)
(3874, 99.526)
(3875, 99.386)
(3876, 99.224)
(3877, 99.612)
(3878, 99.548)
(3879, 99.732)
(3880, 99.586)
(3881, 99.764)
(3882, 99.752)
(3883, 99.546)
(3884, 99.648)
(3885, 99.736)
(3886, 99.548)
(3887, 99.692)
(3888, 99.922)
(3889, 99.764)
(3890, 99.528)
(3891, 99.692)
(3892, 99.532)
(3893, 99.81)
(3894, 99.54)
(3895, 99.508)
(3896, 99.532)
(3897, 99.676)
(3898, 99.454)
(3899, 99.404)
(3900, 99.856)
(3901, 99.812)
(3902, 99.814)
(3903, 99.658)
(3904, 99.788)
(3905, 99.828)
(3906, 99.878)
(3907, 99.608)
(3908, 99.858)
(3909, 99.628)
(3910, 99.444)
(3911, 99.79)
(3912, 99.572)
(3913, 99.426)
(3914, 99.558)
(3915, 99.776)
(3916, 99.428)
(3917, 99.766)
(3918, 99.77)
(3919, 99.87)
(3920, 99.972)
(3921, 99.814)
(3922, 99.736)
(3923, 99.826)
(3924, 99.67)
(3925, 99.58)
(3926, 99.684)
(3927, 99.734)
(3928, 99.836)
(3929, 99.578)
(3930, 99.75)
(3931, 99.244)
(3932, 99.636)
(3933, 99.384)
(3934, 99.514)
(3935, 98.986)
(3936, 99.138)
(3937, 99.496)
(3938, 98.652)
(3939, 98.8)
(3940, 99.692)
(3941, 99.564)
(3942, 99.566)
(3943, 99.028)
(3944, 99.512)
(3945, 99.234)
(3946, 99.524)
(3947, 99.44)
(3948, 99.574)
(3949, 99.476)
(3950, 99.486)
(3951, 99.566)
(3952, 99.776)
(3953, 99.516)
(3954, 99.684)
(3955, 99.862)
(3956, 99.856)
(3957, 99.82)
(3958, 99.67)
(3959, 99.736)
(3960, 99.75)
(3961, 99.788)
(3962, 99.878)
(3963, 99.788)
(3964, 99.664)
(3965, 99.864)
(3966, 99.754)
(3967, 99.312)
(3968, 99.842)
(3969, 99.934)
(3970, 99.888)
(3971, 99.854)
(3972, 99.892)
(3973, 99.912)
(3974, 99.844)
(3975, 99.754)
(3976, 99.834)
(3977, 99.83)
(3978, 99.734)
(3979, 99.848)
(3980, 99.722)
(3981, 99.692)
(3982, 99.724)
(3983, 99.332)
(3984, 99.832)
(3985, 99.892)
(3986, 99.744)
(3987, 99.852)
(3988, 99.774)
(3989, 99.782)
(3990, 99.384)
(3991, 99.764)
(3992, 99.33)
(3993, 99.74)
(3994, 99.79)
(3995, 99.768)
(3996, 99.862)
(3997, 99.822)
(3998, 99.856)
(3999, 99.642)
(4000, 99.94)
(4001, 99.928)
(4002, 99.916)
(4003, 99.898)
(4004, 99.826)
(4005, 99.844)
(4006, 99.88)
(4007, 99.922)
(4008, 99.798)
(4009, 99.968)
(4010, 99.942)
(4011, 99.848)
(4012, 99.946)
(4013, 99.798)
(4014, 99.922)
(4015, 99.988)
(4016, 99.96)
(4017, 99.996)
(4018, 99.998)
(4019, 99.996)
(4020, 99.998)
(4021, 99.97)
(4022, 99.908)
(4023, 99.926)
(4024, 99.898)
(4025, 99.876)
(4026, 99.546)
(4027, 99.892)
(4028, 99.942)
(4029, 99.894)
(4030, 99.87)
(4031, 99.934)
(4032, 99.99)
(4033, 99.978)
(4034, 99.978)
(4035, 99.99)
(4036, 99.964)
(4037, 99.974)
(4038, 99.968)
(4039, 99.984)
(4040, 99.996)
(4041, 99.992)
(4042, 100)
(4043, 100)
(4044, 100)
(4045, 100)
(4046, 100)
(4047, 100)
(4048, 100)
(4049, 100)
(4050, 100)
(4051, 100)
(4052, 100)
(4053, 99.982)
(4054, 99.982)
(4055, 99.956)
(4056, 99.984)
(4057, 99.988)
(4058, 99.998)
(4059, 99.978)
(4060, 99.994)
(4061, 99.992)
(4062, 99.994)
(4063, 99.992)
(4064, 100)
(4065, 99.998)
(4066, 100)
(4067, 99.998)
(4068, 99.98)
(4069, 99.998)
(4070, 100)
(4071, 99.998)
(4072, 99.992)
(4073, 100)
(4074, 99.996)
(4075, 99.91)
(4076, 99.934)
(4077, 99.998)
(4078, 100)
(4079, 100)
(4080, 100)
(4081, 100)
(4082, 99.994)
(4083, 99.998)
(4084, 100)
(4085, 100)
(4086, 99.998)
(4087, 99.996)
(4088, 99.99)
(4089, 99.998)
(4090, 100)
(4091, 99.998)
(4092, 99.998)
(4093, 99.988)
(4094, 100)
(4095, 100)
(4096, 100)
(4097, 100)
(4098, 100)
(4099, 100)
(4100, 100)
(4101, 100)
(4102, 100)
(4103, 100)
(4104, 100)
(4105, 100)
(4106, 100)
(4107, 99.998)
(4108, 100)
(4109, 100)
(4110, 100)
(4111, 100)
(4112, 100)
(4113, 100)
(4114, 100)
(4115, 100)
(4116, 100)
(4117, 100)
(4118, 99.996)
(4119, 100)
(4120, 100)
(4121, 99.998)
(4122, 100)
(4123, 100)
(4124, 99.998)
(4125, 99.806)
(4126, 99.99)
(4127, 99.998)
(4128, 99.964)
(4129, 99.764)
(4130, 99.868)
(4131, 100)
(4132, 99.988)
(4133, 99.988)
(4134, 99.976)
(4135, 98.764)
(4136, 99.978)
(4137, 99.722)
(4138, 99.722)
(4139, 99.82)
(4140, 99.804)
(4141, 99.812)
(4142, 99.946)
(4143, 99.888)
(4144, 99.902)
(4145, 99.974)
(4146, 99.99)
(4147, 100)
(4148, 99.978)
(4149, 99.996)
(4150, 99.914)
(4151, 99.998)
(4152, 100)
(4153, 100)
(4154, 100)
(4155, 99.998)
(4156, 100)
(4157, 100)
(4158, 100)
(4159, 100)
(4160, 99.994)
(4161, 99.994)
(4162, 100)
(4163, 99.998)
(4164, 99.998)
(4165, 99.986)
(4166, 99.97)
(4167, 99.988)
(4168, 99.936)
(4169, 99.978)
(4170, 99.962)
(4171, 99.966)
(4172, 99.964)
(4173, 99.956)
(4174, 99.988)
(4175, 99.984)
(4176, 99.794)
(4177, 99.856)
(4178, 99.798)
(4179, 99.658)
(4180, 99.796)
(4181, 99.696)
(4182, 99.922)
(4183, 99.906)
(4184, 99.934)
(4185, 99.866)
(4186, 99.8)
(4187, 99.912)
(4188, 99.98)
(4189, 99.564)
(4190, 99.998)
(4191, 99.996)
(4192, 99.992)
(4193, 99.998)
(4194, 99.998)
(4195, 99.996)
(4196, 99.998)
(4197, 99.992)
(4198, 100)
(4199, 99.968)
(4200, 99.77)
(4201, 99.774)
(4202, 100)
(4203, 99.992)
(4204, 99.998)
(4205, 99.998)
(4206, 99.992)
(4207, 99.996)
(4208, 99.986)
(4209, 99.996)
(4210, 99.994)
(4211, 99.988)
(4212, 99.982)
(4213, 99.984)
(4214, 99.992)
(4215, 99.992)
(4216, 99.95)
(4217, 99.92)
(4218, 99.874)
(4219, 99.844)
(4220, 99.904)
(4221, 99.868)
(4222, 99.802)
(4223, 99.258)
(4224, 99.642)
(4225, 99.846)
(4226, 99.644)
(4227, 99.418)
(4228, 99.28)
(4229, 99.348)
(4230, 99.546)
(4231, 99.446)
(4232, 98.75)
(4233, 99.104)
(4234, 99.256)
(4235, 98.974)
(4236, 99.264)
(4237, 98.964)
(4238, 98.698)
(4239, 99.132)
(4240, 99.184)
(4241, 99.07)
(4242, 99.118)
(4243, 98.76)
(4244, 97.552)
(4245, 98.114)
(4246, 98.572)
(4247, 98.254)
(4248, 97.498)
(4249, 97.664)
(4250, 98.442)
(4251, 98.45)
(4252, 99.03)
(4253, 98.986)
(4254, 98.926)
(4255, 99.438)
(4256, 99.146)
(4257, 99.05)
(4258, 98.526)
(4259, 98.574)
(4260, 97.474)
(4261, 98.968)
(4262, 99.114)
(4263, 99.038)
(4264, 98.722)
(4265, 98.908)
(4266, 98.632)
(4267, 98.032)
(4268, 98.75)
(4269, 97.47)
(4270, 99.044)
(4271, 99.396)
(4272, 98.748)
(4273, 98.944)
(4274, 98.73)
(4275, 99.056)
(4276, 99.042)
(4277, 98.246)
(4278, 98.132)
(4279, 96.37)
(4280, 98.764)
(4281, 99.156)
(4282, 99.066)
(4283, 98.416)
(4284, 98.558)
(4285, 98.936)
(4286, 99.056)
(4287, 98.802)
(4288, 99.314)
(4289, 98.93)
(4290, 97.558)
(4291, 98.78)
(4292, 96.33)
(4293, 98.232)
(4294, 99.168)
(4295, 98.568)
(4296, 99.244)
(4297, 99.236)
(4298, 99.65)
(4299, 98.694)
(4300, 99.248)
(4301, 99.502)
(4302, 99.53)
(4303, 99.42)
(4304, 98.014)
(4305, 99.362)
(4306, 98.776)
(4307, 97.922)
(4308, 99.184)
(4309, 99.202)
(4310, 99.058)
(4311, 98.508)
(4312, 97.894)
(4313, 97.382)
(4314, 98.016)
(4315, 99.04)
(4316, 99.178)
(4317, 98.908)
(4318, 97.282)
(4319, 98.722)
(4320, 99.39)
(4321, 99.658)
(4322, 99.388)
(4323, 98.986)
(4324, 99.402)
(4325, 99.588)
(4326, 99.816)
(4327, 99.81)
(4328, 99.634)
(4329, 99.88)
(4330, 99.858)
(4331, 99.902)
(4332, 99.888)
(4333, 99.752)
(4334, 99.8)
(4335, 99.842)
(4336, 99.914)
(4337, 97.254)
(4338, 96.6)
(4339, 99.458)
(4340, 99.746)
(4341, 99.776)
(4342, 97.62)
(4343, 99.612)
(4344, 99.68)
(4345, 99.784)
(4346, 99.678)
(4347, 99.524)
(4348, 99.592)
(4349, 99.306)
(4350, 99.608)
(4351, 99.542)
(4352, 99.652)
(4353, 99.698)
(4354, 99.71)
(4355, 99.764)
(4356, 99.702)
(4357, 99.486)
(4358, 99.184)
(4359, 99.336)
(4360, 99.814)
(4361, 99.746)
(4362, 99.61)
(4363, 99.718)
(4364, 99.568)
(4365, 99.35)
(4366, 99.56)
(4367, 99.76)
(4368, 99.824)
(4369, 99.86)
(4370, 99.882)
(4371, 99.936)
(4372, 99.936)
(4373, 99.89)
(4374, 99.87)
(4375, 98.282)
(4376, 99.87)
(4377, 99.836)
(4378, 99.786)
(4379, 99.704)
(4380, 99.556)
(4381, 99.598)
(4382, 99.636)
(4383, 99.54)
(4384, 99.682)
(4385, 99.468)
(4386, 99.338)
(4387, 99.458)
(4388, 99.48)
(4389, 99.806)
(4390, 99.858)
(4391, 99.794)
(4392, 99.868)
(4393, 99.59)
(4394, 99.634)
(4395, 99.286)
(4396, 99.664)
(4397, 99.586)
(4398, 99.784)
(4399, 99.564)
(4400, 99.888)
(4401, 99.896)
(4402, 99.916)
(4403, 99.916)
(4404, 99.962)
(4405, 99.88)
(4406, 99.824)
(4407, 99.454)
(4408, 99.892)
(4409, 99.592)
(4410, 99.692)
(4411, 99.646)
(4412, 99.792)
(4413, 99.774)
(4414, 98.842)
(4415, 99.614)
(4416, 99.72)
(4417, 99.888)
(4418, 99.996)
(4419, 99.974)
(4420, 99.946)
(4421, 99.99)
(4422, 99.964)
(4423, 99.968)
(4424, 99.828)
(4425, 99.952)
(4426, 99.94)
(4427, 99.748)
(4428, 99.798)
(4429, 99.726)
(4430, 99.904)
(4431, 99.578)
(4432, 99.55)
(4433, 99.198)
(4434, 98.966)
(4435, 99.85)
(4436, 99.77)
(4437, 99.802)
(4438, 99.724)
(4439, 99.8)
(4440, 99.11)
(4441, 99.628)
(4442, 99.728)
(4443, 99.654)
(4444, 99.872)
(4445, 99.282)
(4446, 99.888)
(4447, 99.876)
(4448, 99.826)
(4449, 99.706)
(4450, 99.846)
(4451, 99.768)
(4452, 99.614)
(4453, 99.938)
(4454, 99.712)
(4455, 99.782)
(4456, 99.81)
(4457, 99.966)
(4458, 99.55)
(4459, 99.976)
(4460, 99.924)
(4461, 99.942)
(4462, 99.986)
(4463, 99.982)
(4464, 99.946)
(4465, 99.92)
(4466, 99.958)
(4467, 99.958)
(4468, 99.982)
(4469, 99.988)
(4470, 99.982)
(4471, 99.988)
(4472, 99.992)
(4473, 99.998)
(4474, 99.994)
(4475, 99.978)
(4476, 99.994)
(4477, 99.968)
(4478, 99.992)
(4479, 99.966)
(4480, 99.766)
(4481, 99.966)
(4482, 99.996)
(4483, 99.992)
(4484, 99.93)
(4485, 99.986)
(4486, 99.996)
(4487, 99.838)
(4488, 99.97)
(4489, 99.966)
(4490, 99.968)
(4491, 99.96)
(4492, 99.98)
(4493, 99.986)
(4494, 99.972)
(4495, 99.972)
(4496, 99.86)
(4497, 99.984)
(4498, 99.968)
(4499, 99.99)
(4500, 99.996)
(4501, 99.92)
(4502, 99.966)
(4503, 99.986)
(4504, 99.934)
(4505, 99.92)
(4506, 99.996)
(4507, 99.996)
(4508, 99.968)
(4509, 99.974)
(4510, 99.992)
(4511, 99.972)
(4512, 99.89)
(4513, 99.968)
(4514, 99.994)
(4515, 99.956)
(4516, 99.89)
(4517, 99.814)
(4518, 99.822)
(4519, 99.864)
(4520, 99.932)
(4521, 99.736)
(4522, 99.904)
(4523, 99.962)
(4524, 99.848)
(4525, 99.816)
(4526, 99.89)
(4527, 99.864)
(4528, 99.978)
(4529, 99.962)
(4530, 99.916)
(4531, 99.986)
(4532, 99.976)
(4533, 99.98)
(4534, 99.998)
(4535, 100)
(4536, 100)
(4537, 99.986)
(4538, 99.994)
(4539, 99.99)
(4540, 99.992)
(4541, 99.994)
(4542, 99.988)
(4543, 99.986)
(4544, 99.954)
(4545, 99.994)
(4546, 99.984)
(4547, 99.944)
(4548, 99.984)
(4549, 99.964)
(4550, 99.996)
(4551, 99.998)
(4552, 100)
(4553, 99.784)
(4554, 99.904)
(4555, 99.906)
(4556, 99.996)
(4557, 99.924)
(4558, 99.998)
(4559, 99.982)
(4560, 99.924)
(4561, 99.998)
(4562, 99.998)
(4563, 100)
(4564, 100)
(4565, 99.994)
(4566, 100)
(4567, 100)
(4568, 100)
(4569, 100)
(4570, 99.99)
(4571, 100)
(4572, 99.986)
(4573, 99.974)
(4574, 99.76)
(4575, 99.716)
(4576, 99.992)
(4577, 99.986)
(4578, 99.978)
(4579, 99.902)
(4580, 99.476)
(4581, 99.856)
(4582, 99.84)
(4583, 99.842)
(4584, 99.854)
(4585, 99.806)
(4586, 99.928)
(4587, 99.87)
(4588, 99.782)
(4589, 99.728)
(4590, 99.766)
(4591, 99.834)
(4592, 99.748)
(4593, 99.578)
(4594, 99.754)
(4595, 99.55)
(4596, 99.06)
(4597, 99.65)
(4598, 99.598)
(4599, 99.786)
(4600, 99.642)
(4601, 97.214)
(4602, 99.522)
(4603, 99.732)
(4604, 99.81)
(4605, 99.252)
(4606, 99.78)
(4607, 99.85)
(4608, 99.594)
(4609, 99.82)
(4610, 99.848)
(4611, 99.714)
(4612, 99.872)
(4613, 99.854)
(4614, 99.27)
(4615, 99.774)
(4616, 99.92)
(4617, 99.314)
(4618, 99.826)
(4619, 99.94)
(4620, 99.912)
(4621, 99.988)
(4622, 99.972)
(4623, 99.926)
(4624, 99.886)
(4625, 99.908)
(4626, 99.96)
(4627, 99.988)
(4628, 99.996)
(4629, 99.994)
(4630, 99.948)
(4631, 99.936)
(4632, 99.948)
(4633, 99.986)
(4634, 99.968)
(4635, 99.99)
(4636, 99.984)
(4637, 99.956)
(4638, 99.982)
(4639, 99.982)
(4640, 99.952)
(4641, 99.948)
(4642, 99.956)
(4643, 99.968)
(4644, 99.87)
(4645, 99.95)
(4646, 99.98)
(4647, 99.97)
(4648, 99.918)
(4649, 99.906)
(4650, 99.968)
(4651, 99.978)
(4652, 99.942)
(4653, 99.966)
(4654, 99.996)
(4655, 99.98)
(4656, 99.856)
(4657, 99.89)
(4658, 99.812)
(4659, 99.912)
(4660, 99.986)
(4661, 99.826)
(4662, 99.932)
(4663, 99.67)
(4664, 99.968)
(4665, 99.706)
(4666, 99.986)
(4667, 99.978)
(4668, 99.998)
(4669, 99.994)
(4670, 99.976)
(4671, 99.948)
(4672, 99.952)
(4673, 99.976)
(4674, 99.976)
(4675, 99.958)
(4676, 99.988)
(4677, 99.958)
(4678, 99.932)
(4679, 99.976)
(4680, 99.93)
(4681, 99.916)
(4682, 99.966)
(4683, 99.952)
(4684, 99.988)
(4685, 99.982)
(4686, 99.926)
(4687, 99.924)
(4688, 99.974)
(4689, 99.99)
(4690, 99.914)
(4691, 99.994)
(4692, 99.994)
(4693, 99.958)
(4694, 99.972)
(4695, 99.992)
(4696, 99.99)
(4697, 99.956)
(4698, 99.812)
(4699, 99.764)
(4700, 99.93)
(4701, 99.784)
(4702, 99.902)
(4703, 99.818)
(4704, 99.934)
(4705, 99.92)
(4706, 99.874)
(4707, 99.9)
(4708, 99.99)
(4709, 100)
(4710, 99.996)
(4711, 99.33)
(4712, 99.974)
(4713, 99.922)
(4714, 99.942)
(4715, 99.992)
(4716, 99.99)
(4717, 99.968)
(4718, 99.936)
(4719, 99.94)
(4720, 99.984)
(4721, 99.962)
(4722, 99.936)
(4723, 99.98)
(4724, 99.974)
(4725, 99.996)
(4726, 99.998)
(4727, 99.996)
(4728, 99.994)
(4729, 99.968)
(4730, 99.806)
(4731, 99.968)
(4732, 99.976)
(4733, 99.936)
(4734, 100)
(4735, 99.996)
(4736, 99.968)
(4737, 99.998)
(4738, 99.996)
(4739, 99.984)
(4740, 99.998)
(4741, 99.986)
(4742, 100)
(4743, 100)
(4744, 99.938)
(4745, 99.956)
(4746, 99.884)
(4747, 99.94)
(4748, 99.95)
(4749, 99.976)
(4750, 99.932)
(4751, 99.952)
(4752, 99.878)
(4753, 99.858)
(4754, 99.794)
(4755, 99.954)
(4756, 99.962)
(4757, 99.994)
(4758, 99.998)
(4759, 99.996)
(4760, 99.994)
(4761, 100)
(4762, 99.998)
(4763, 100)
(4764, 99.998)
(4765, 99.996)
(4766, 99.996)
(4767, 99.982)
(4768, 99.976)
(4769, 99.982)
(4770, 99.996)
(4771, 100)
(4772, 99.996)
(4773, 99.996)
(4774, 99.998)
(4775, 100)
(4776, 99.896)
(4777, 99.83)
(4778, 99.988)
(4779, 99.964)
(4780, 99.826)
(4781, 99.968)
(4782, 99.952)
(4783, 99.93)
(4784, 99.836)
(4785, 99.942)
(4786, 99.872)
(4787, 99.988)
(4788, 99.544)
(4789, 99.918)
(4790, 99.94)
(4791, 99.858)
(4792, 99.944)
(4793, 99.93)
(4794, 99.964)
(4795, 99.952)
(4796, 99.888)
(4797, 99.904)
(4798, 99.946)
(4799, 99.942)
(4800, 99.9)
(4801, 99.838)
(4802, 99.972)
(4803, 99.992)
(4804, 99.996)
(4805, 99.968)
(4806, 100)
(4807, 99.938)
(4808, 99.99)
(4809, 99.984)
(4810, 99.996)
(4811, 99.992)
(4812, 99.984)
(4813, 99.972)
(4814, 99.994)
(4815, 99.91)
(4816, 99.976)
(4817, 99.92)
(4818, 99.968)
(4819, 99.834)
(4820, 99.952)
(4821, 99.954)
(4822, 99.986)
(4823, 99.894)
(4824, 99.904)
(4825, 99.918)
(4826, 99.908)
(4827, 99.79)
(4828, 99.914)
(4829, 99.962)
(4830, 99.974)
(4831, 99.908)
(4832, 99.964)
(4833, 99.956)
(4834, 99.984)
(4835, 99.948)
(4836, 99.964)
(4837, 99.864)
(4838, 99.962)
(4839, 99.978)
(4840, 99.87)
(4841, 99.99)
(4842, 99.994)
(4843, 99.97)
(4844, 99.97)
(4845, 99.992)
(4846, 99.972)
(4847, 99.982)
(4848, 99.98)
(4849, 99.986)
(4850, 99.984)
(4851, 99.992)
(4852, 99.988)
(4853, 99.99)
(4854, 99.974)
(4855, 99.928)
(4856, 99.994)
(4857, 99.994)
(4858, 99.558)
(4859, 99.882)
(4860, 99.85)
(4861, 99.794)
(4862, 99.92)
(4863, 99.986)
(4864, 99.96)
(4865, 99.91)
(4866, 99.866)
(4867, 99.824)
(4868, 99.836)
(4869, 99.956)
(4870, 99.912)
(4871, 99.872)
(4872, 99.894)
(4873, 99.876)
(4874, 99.74)
(4875, 99.844)
(4876, 99.934)
(4877, 99.792)
(4878, 99.732)
(4879, 99.974)
(4880, 99.908)
(4881, 99.66)
(4882, 99.962)
(4883, 99.986)
(4884, 99.962)
(4885, 99.95)
(4886, 99.946)
(4887, 99.99)
(4888, 99.798)
(4889, 99.944)
(4890, 99.866)
(4891, 99.954)
(4892, 99.994)
(4893, 99.988)
(4894, 99.864)
(4895, 99.998)
(4896, 99.996)
(4897, 100)
(4898, 100)
(4899, 99.996)
(4900, 99.836)
(4901, 99.988)
(4902, 99.99)
(4903, 99.982)
(4904, 99.99)
(4905, 100)
(4906, 99.996)
(4907, 100)
(4908, 100)
(4909, 99.998)
(4910, 100)
(4911, 100)
(4912, 99.998)
(4913, 99.996)
(4914, 99.966)
(4915, 99.976)
(4916, 100)
(4917, 100)
(4918, 100)
(4919, 100)
(4920, 100)
(4921, 99.998)
(4922, 100)
(4923, 100)
(4924, 100)
(4925, 99.998)
(4926, 99.99)
(4927, 100)
(4928, 100)
(4929, 100)
(4930, 99.998)
(4931, 100)
(4932, 100)
(4933, 100)
(4934, 100)
(4935, 100)
(4936, 100)
(4937, 100)
(4938, 100)
(4939, 100)
(4940, 100)
(4941, 99.998)
(4942, 100)
(4943, 100)
(4944, 99.996)
(4945, 100)
(4946, 100)
(4947, 100)
(4948, 100)
(4949, 100)
(4950, 100)
(4951, 100)
(4952, 100)
(4953, 100)
(4954, 100)
(4955, 100)
(4956, 100)
(4957, 99.998)
(4958, 100)
(4959, 100)
(4960, 100)
(4961, 100)
(4962, 100)
(4963, 100)
(4964, 100)
(4965, 100)
(4966, 100)
(4967, 100)
(4968, 100)
(4969, 100)
(4970, 100)
(4971, 100)
(4972, 100)
(4973, 100)
(4974, 99.998)
(4975, 100)
(4976, 100)
(4977, 100)
(4978, 99.998)
(4979, 100)
(4980, 100)
(4981, 100)
(4982, 100)
(4983, 100)
(4984, 100)
(4985, 100)
(4986, 100)
(4987, 100)
(4988, 100)
(4989, 100)
(4990, 100)
(4991, 99.998)
(4992, 100)
(4993, 99.996)
(4994, 99.998)
(4995, 100)
(4996, 100)
(4997, 100)
(4998, 100)
(4999, 100)
(5000, 100)
(5001, 100)
(5002, 99.89)
(5003, 100)
(5004, 99.994)
(5005, 99.958)
(5006, 99.99)
(5007, 99.996)
(5008, 99.986)
(5009, 99.944)
(5010, 99.99)
(5011, 99.988)
(5012, 100)
(5013, 99.998)
(5014, 100)
(5015, 100)
(5016, 100)
(5017, 99.97)
(5018, 99.994)
(5019, 99.998)
(5020, 99.998)
(5021, 100)
(5022, 100)
(5023, 99.998)
(5024, 99.974)
(5025, 99.968)
(5026, 99.996)
(5027, 100)
(5028, 100)
(5029, 100)
(5030, 99.968)
(5031, 100)
(5032, 100)
(5033, 100)
(5034, 100)
(5035, 100)
(5036, 100)
(5037, 100)
(5038, 100)
(5039, 100)
(5040, 100)
(5041, 100)
(5042, 100)
(5043, 100)
(5044, 99.998)
(5045, 100)
(5046, 100)
(5047, 99.96)
(5048, 99.992)
(5049, 100)
(5050, 99.986)
(5051, 99.996)
(5052, 100)
(5053, 99.996)
(5054, 99.994)
(5055, 99.968)
(5056, 99.998)
(5057, 99.904)
(5058, 99.986)
(5059, 99.976)
(5060, 99.99)
(5061, 99.828)
(5062, 99.998)
(5063, 99.988)
(5064, 99.998)
(5065, 99.988)
(5066, 99.792)
(5067, 100)
(5068, 99.996)
(5069, 99.984)
(5070, 99.992)
(5071, 100)
(5072, 100)
(5073, 99.946)
(5074, 99.958)
(5075, 99.846)
(5076, 99.848)
(5077, 99.802)
(5078, 99.838)
(5079, 99.918)
(5080, 99.836)
(5081, 99.824)
(5082, 99.894)
(5083, 99.938)
(5084, 99.778)
(5085, 99.954)
(5086, 99.922)
(5087, 99.9)
(5088, 99.838)
(5089, 99.974)
(5090, 99.882)
(5091, 99.432)
(5092, 99.922)
(5093, 99.874)
(5094, 99.848)
(5095, 99.976)
(5096, 99.868)
(5097, 99.986)
(5098, 99.846)
(5099, 99.94)
(5100, 99.966)
(5101, 99.966)
(5102, 99.8)
(5103, 99.47)
(5104, 99.608)
(5105, 99.926)
(5106, 99.278)
(5107, 99.78)
(5108, 99.862)
(5109, 99.808)
(5110, 99.826)
(5111, 99.894)
(5112, 99.908)
(5113, 99.866)
(5114, 99.934)
(5115, 99.744)
(5116, 99.976)
(5117, 99.992)
(5118, 99.994)
(5119, 100)
(5120, 99.996)
(5121, 100)
(5122, 99.996)
(5123, 99.998)
(5124, 100)
(5125, 100)
(5126, 100)
(5127, 100)
(5128, 99.984)
(5129, 100)
(5130, 100)
(5131, 100)
(5132, 100)
(5133, 99.996)
(5134, 100)
(5135, 99.984)
(5136, 99.376)
(5137, 99.972)
(5138, 99.956)
(5139, 99.964)
(5140, 99.93)
(5141, 99.926)
(5142, 99.984)
(5143, 99.848)
(5144, 99.94)
(5145, 99.988)
(5146, 99.998)
(5147, 99.99)
(5148, 100)
(5149, 99.988)
(5150, 99.782)
(5151, 99.932)
(5152, 99.986)
(5153, 99.998)
(5154, 99.982)
(5155, 99.978)
(5156, 99.984)
(5157, 99.988)
(5158, 99.926)
(5159, 99.99)
(5160, 99.972)
(5161, 99.99)
(5162, 99.996)
(5163, 99.958)
(5164, 99.974)
(5165, 99.976)
(5166, 99.94)
(5167, 100)
(5168, 99.988)
(5169, 99.994)
(5170, 99.998)
(5171, 99.998)
(5172, 100)
(5173, 100)
(5174, 100)
(5175, 99.996)
(5176, 99.974)
(5177, 100)
(5178, 100)
(5179, 99.99)
(5180, 100)
(5181, 100)
(5182, 99.994)
(5183, 100)
(5184, 99.988)
(5185, 99.992)
(5186, 99.934)
(5187, 99.992)
(5188, 100)
(5189, 100)
(5190, 99.998)
(5191, 99.996)
(5192, 99.998)
(5193, 99.994)
(5194, 99.944)
(5195, 99.996)
(5196, 99.998)
(5197, 100)
(5198, 99.99)
(5199, 99.992)
(5200, 99.938)
(5201, 99.974)
(5202, 99.968)
(5203, 99.954)
(5204, 99.986)
(5205, 99.996)
(5206, 99.92)
(5207, 99.844)
(5208, 99.98)
(5209, 99.99)
(5210, 99.998)
(5211, 99.978)
(5212, 99.648)
(5213, 99.99)
(5214, 99.998)
(5215, 99.998)
(5216, 99.996)
(5217, 99.88)
(5218, 99.704)
(5219, 99.966)
(5220, 100)
(5221, 100)
(5222, 99.99)
(5223, 99.994)
(5224, 99.998)
(5225, 99.988)
(5226, 100)
(5227, 99.86)
(5228, 99.998)
(5229, 99.99)
(5230, 99.994)
(5231, 99.996)
(5232, 100)
(5233, 100)
(5234, 99.96)
(5235, 99.782)
(5236, 100)
(5237, 99.998)
(5238, 100)
(5239, 100)
(5240, 100)
(5241, 99.998)
(5242, 100)
(5243, 99.998)
(5244, 99.994)
(5245, 99.992)
(5246, 100)
(5247, 100)
(5248, 99.94)
(5249, 100)
(5250, 100)
(5251, 100)
(5252, 100)
(5253, 100)
(5254, 100)
(5255, 100)
(5256, 100)
(5257, 99.998)
(5258, 100)
(5259, 100)
(5260, 100)
(5261, 100)
(5262, 100)
(5263, 100)
(5264, 100)
(5265, 100)
(5266, 100)
(5267, 100)
(5268, 100)
(5269, 100)
(5270, 100)
(5271, 100)
(5272, 100)
(5273, 100)
(5274, 100)
(5275, 99.998)
(5276, 100)
(5277, 99.996)
(5278, 99.978)
(5279, 100)
(5280, 99.798)
(5281, 100)
(5282, 100)
(5283, 99.994)
(5284, 99.998)
(5285, 100)
(5286, 99.978)
(5287, 99.972)
(5288, 100)
(5289, 99.974)
(5290, 99.978)
(5291, 100)
(5292, 99.994)
(5293, 99.998)
(5294, 99.996)
(5295, 99.998)
(5296, 99.974)
(5297, 100)
(5298, 100)
(5299, 99.998)
(5300, 99.978)
(5301, 99.994)
(5302, 99.938)
(5303, 100)
(5304, 100)
(5305, 99.994)
(5306, 99.896)
(5307, 100)
(5308, 100)
(5309, 99.994)
(5310, 99.982)
(5311, 99.964)
(5312, 99.942)
(5313, 99.54)
(5314, 99.996)
(5315, 100)
(5316, 99.998)
(5317, 100)
(5318, 100)
(5319, 99.996)
(5320, 99.972)
(5321, 99.99)
(5322, 99.972)
(5323, 99.882)
(5324, 99.982)
(5325, 99.984)
(5326, 99.998)
(5327, 99.984)
(5328, 99.98)
(5329, 99.982)
(5330, 99.914)
(5331, 99.99)
(5332, 100)
(5333, 99.996)
(5334, 99.992)
(5335, 99.99)
(5336, 99.868)
(5337, 99.988)
(5338, 99.988)
(5339, 99.98)
(5340, 99.952)
(5341, 99.984)
(5342, 100)
(5343, 99.996)
(5344, 99.888)
(5345, 100)
(5346, 99.994)
(5347, 99.994)
(5348, 99.976)
(5349, 100)
(5350, 100)
(5351, 99.95)
(5352, 99.956)
(5353, 99.998)
(5354, 99.974)
(5355, 99.99)
(5356, 99.974)
(5357, 99.976)
(5358, 99.976)
(5359, 99.998)
(5360, 99.852)
(5361, 99.984)
(5362, 99.986)
(5363, 99.996)
(5364, 100)
(5365, 99.996)
(5366, 99.998)
(5367, 100)
(5368, 100)
(5369, 100)
(5370, 100)
(5371, 99.998)
(5372, 99.958)
(5373, 99.998)
(5374, 99.99)
(5375, 99.996)
(5376, 100)
(5377, 99.99)
(5378, 100)
(5379, 99.998)
(5380, 99.998)
(5381, 99.998)
(5382, 99.73)
(5383, 99.916)
(5384, 99.684)
(5385, 99.96)
(5386, 99.998)
(5387, 99.998)
(5388, 100)
(5389, 100)
(5390, 100)
(5391, 100)
(5392, 99.998)
(5393, 99.946)
(5394, 99.998)
(5395, 100)
(5396, 100)
(5397, 99.998)
(5398, 99.998)
(5399, 99.996)
(5400, 99.99)
(5401, 100)
(5402, 99.996)
(5403, 100)
(5404, 100)
(5405, 100)
(5406, 99.986)
(5407, 100)
(5408, 100)
(5409, 99.994)
(5410, 100)
(5411, 99.998)
(5412, 100)
(5413, 100)
(5414, 100)
(5415, 100)
(5416, 100)
(5417, 100)
(5418, 100)
(5419, 100)
(5420, 99.998)
(5421, 99.988)
(5422, 99.996)
(5423, 100)
(5424, 100)
(5425, 100)
(5426, 100)
(5427, 100)
(5428, 100)
(5429, 100)
(5430, 100)
(5431, 100)
(5432, 100)
(5433, 100)
(5434, 100)
(5435, 100)
(5436, 100)
(5437, 99.988)
(5438, 100)
(5439, 99.998)
(5440, 100)
(5441, 100)
(5442, 100)
(5443, 100)
(5444, 100)
(5445, 100)
(5446, 100)
(5447, 100)
(5448, 100)
(5449, 100)
(5450, 100)
(5451, 100)
(5452, 100)
(5453, 100)
(5454, 100)
(5455, 100)
(5456, 100)
(5457, 99.986)
(5458, 99.998)
(5459, 100)
(5460, 100)
(5461, 100)
(5462, 100)
(5463, 100)
(5464, 99.986)
(5465, 99.918)
(5466, 99.954)
(5467, 100)
(5468, 100)
(5469, 99.998)
(5470, 100)
(5471, 100)
(5472, 100)
(5473, 100)
(5474, 100)
(5475, 100)
(5476, 99.992)
(5477, 99.994)
(5478, 99.998)
(5479, 100)
(5480, 100)
(5481, 100)
(5482, 99.998)
(5483, 99.998)
(5484, 100)
(5485, 99.998)
(5486, 99.98)
(5487, 100)
(5488, 99.992)
(5489, 99.968)
(5490, 99.942)
(5491, 99.982)
(5492, 99.934)
(5493, 99.994)
(5494, 99.994)
(5495, 99.986)
(5496, 99.996)
(5497, 99.998)
(5498, 99.996)
(5499, 99.966)
(5500, 99.99)
(5501, 99.998)
(5502, 99.972)
(5503, 100)
(5504, 99.988)
(5505, 99.984)
(5506, 99.988)
(5507, 99.994)
(5508, 99.996)
(5509, 100)
(5510, 99.994)
(5511, 100)
(5512, 100)
(5513, 100)
(5514, 100)
(5515, 100)
(5516, 100)
(5517, 100)
(5518, 100)
(5519, 100)
(5520, 100)
(5521, 100)
(5522, 100)
(5523, 100)
(5524, 100)
(5525, 100)
(5526, 100)
(5527, 100)
(5528, 100)
(5529, 100)
(5530, 100)
(5531, 100)
(5532, 100)
(5533, 99.998)
(5534, 100)
(5535, 100)
(5536, 100)
(5537, 99.996)
(5538, 100)
(5539, 100)
(5540, 100)
(5541, 99.998)
(5542, 100)
(5543, 100)
(5544, 100)
(5545, 100)
(5546, 100)
(5547, 100)
(5548, 100)
(5549, 100)
(5550, 99.992)
(5551, 100)
(5552, 100)
(5553, 99.926)
(5554, 99.882)
(5555, 100)
(5556, 100)
(5557, 100)
(5558, 99.996)
(5559, 100)
(5560, 100)
(5561, 100)
(5562, 100)
(5563, 100)
(5564, 100)
(5565, 100)
(5566, 99.99)
(5567, 99.996)
(5568, 99.992)
(5569, 99.986)
(5570, 99.998)
(5571, 99.988)
(5572, 99.98)
(5573, 99.916)
(5574, 99.888)
(5575, 99.84)
(5576, 99.52)
(5577, 99.646)
(5578, 99.66)
(5579, 99.124)
(5580, 99.396)
(5581, 99.724)
(5582, 99.662)
(5583, 99.31)
(5584, 99.68)
(5585, 99.79)
(5586, 99.958)
(5587, 99.912)
(5588, 99.866)
(5589, 99.942)
(5590, 99.954)
(5591, 99.98)
(5592, 99.938)
(5593, 99.962)
(5594, 99.934)
(5595, 99.834)
(5596, 99.9)
(5597, 99.882)
(5598, 99.728)
(5599, 99.81)
(5600, 99.92)
(5601, 99.854)
(5602, 99.896)
(5603, 99.924)
(5604, 99.95)
(5605, 99.964)
(5606, 99.948)
(5607, 99.936)
(5608, 99.688)
(5609, 99.492)
(5610, 99.912)
(5611, 99.938)
(5612, 99.854)
(5613, 99.758)
(5614, 99.642)
(5615, 99.816)
(5616, 99.78)
(5617, 99.948)
(5618, 99.918)
(5619, 99.894)
(5620, 99.874)
(5621, 99.85)
(5622, 99.666)
(5623, 99.144)
(5624, 99.91)
(5625, 99.858)
(5626, 99.866)
(5627, 99.942)
(5628, 99.924)
(5629, 99.934)
(5630, 99.856)
(5631, 99.93)
(5632, 99.934)
(5633, 99.932)
(5634, 99.882)
(5635, 99.93)
(5636, 99.91)
(5637, 99.916)
(5638, 99.738)
(5639, 99.89)
(5640, 99.85)
(5641, 99.904)
(5642, 99.728)
(5643, 99.508)
(5644, 99.342)
(5645, 99.328)
(5646, 99.556)
(5647, 99.836)
(5648, 98.564)
(5649, 99.274)
(5650, 99.096)
(5651, 99.42)
(5652, 99.616)
(5653, 99.31)
(5654, 99.7)
(5655, 99.608)
(5656, 99.046)
(5657, 98.858)
(5658, 98.908)
(5659, 99.054)
(5660, 99.506)
(5661, 99.606)
(5662, 99.512)
(5663, 98.812)
(5664, 99.516)
(5665, 99.244)
(5666, 99.118)
(5667, 97.634)
(5668, 99.218)
(5669, 98.322)
(5670, 98.878)
(5671, 98.928)
(5672, 99.624)
(5673, 99.156)
(5674, 99.298)
(5675, 99.118)
(5676, 99.016)
(5677, 93.922)
(5678, 99.248)
(5679, 99.214)
(5680, 99.47)
(5681, 98.904)
(5682, 99.28)
(5683, 98.12)
(5684, 99.264)
(5685, 98.626)
(5686, 98.62)
(5687, 99.318)
(5688, 99.36)
(5689, 98.606)
(5690, 98.018)
(5691, 98.184)
(5692, 98.674)
(5693, 98.024)
(5694, 97.714)
(5695, 97.138)
(5696, 99.264)
(5697, 98.994)
(5698, 99.308)
(5699, 99.052)
(5700, 99.32)
(5701, 99.446)
(5702, 98.97)
(5703, 99.202)
(5704, 99.706)
(5705, 99.648)
(5706, 99.672)
(5707, 99.458)
(5708, 99.362)
(5709, 99.724)
(5710, 99.584)
(5711, 99.424)
(5712, 99.368)
(5713, 99.72)
(5714, 99.388)
(5715, 99.766)
(5716, 99.836)
(5717, 99.602)
(5718, 99.752)
(5719, 99.638)
(5720, 99.72)
(5721, 99.682)
(5722, 99.68)
(5723, 99.75)
(5724, 99.832)
(5725, 99.846)
(5726, 99.828)
(5727, 99.594)
(5728, 99.864)
(5729, 99.934)
(5730, 99.838)
(5731, 99.854)
(5732, 99.792)
(5733, 99.8)
(5734, 99.598)
(5735, 98.754)
(5736, 99.714)
(5737, 99.626)
(5738, 99.69)
(5739, 99.59)
(5740, 99.48)
(5741, 99.792)
(5742, 99.924)
(5743, 99.76)
(5744, 99.406)
(5745, 99.734)
(5746, 99.804)
(5747, 99.734)
(5748, 99.802)
(5749, 99.83)
(5750, 99.95)
(5751, 99.834)
(5752, 99.624)
(5753, 99.922)
(5754, 99.868)
(5755, 99.838)
(5756, 99.882)
(5757, 99.834)
(5758, 99.908)
(5759, 99.902)
(5760, 99.726)
(5761, 99.91)
(5762, 99.77)
(5763, 99.79)
(5764, 99.72)
(5765, 99.624)
(5766, 99.694)
(5767, 99.674)
(5768, 99.704)
(5769, 99.74)
(5770, 99.604)
(5771, 99.592)
(5772, 99.302)
(5773, 98.734)
(5774, 98.626)
(5775, 98.634)
(5776, 98.794)
(5777, 98.532)
(5778, 98.916)
(5779, 99.184)
(5780, 99.446)
(5781, 99.262)
(5782, 99.336)
(5783, 99.096)
(5784, 99.376)
(5785, 99.458)
(5786, 99.068)
(5787, 99.02)
(5788, 98.174)
(5789, 98.97)
(5790, 99.116)
(5791, 99.226)
(5792, 99.336)
(5793, 99.478)
(5794, 99.592)
(5795, 99.706)
(5796, 99.726)
(5797, 99.682)
(5798, 99.764)
(5799, 99.642)
(5800, 99.762)
(5801, 99.88)
(5802, 99.926)
(5803, 99.908)
(5804, 99.88)
(5805, 99.964)
(5806, 99.896)
(5807, 99.98)
(5808, 99.946)
(5809, 99.836)
(5810, 99.958)
(5811, 99.874)
(5812, 99.898)
(5813, 99.948)
(5814, 99.884)
(5815, 99.836)
(5816, 99.904)
(5817, 99.94)
(5818, 99.896)
(5819, 99.62)
(5820, 99.57)
(5821, 99.822)
(5822, 99.58)
(5823, 99.744)
(5824, 99.808)
(5825, 99.834)
(5826, 99.84)
(5827, 99.858)
(5828, 99.908)
(5829, 99.764)
(5830, 99.908)
(5831, 99.954)
(5832, 99.832)
(5833, 99.786)
(5834, 99.908)
(5835, 99.716)
(5836, 99.906)
(5837, 99.884)
(5838, 99.81)
(5839, 99.854)
(5840, 99.952)
(5841, 99.956)
(5842, 99.836)
(5843, 99.868)
(5844, 99.956)
(5845, 99.964)
(5846, 99.952)
(5847, 99.954)
(5848, 99.958)
(5849, 99.868)
(5850, 99.822)
(5851, 99.95)
(5852, 99.856)
(5853, 99.942)
(5854, 99.97)
(5855, 99.878)
(5856, 99.736)
(5857, 99.684)
(5858, 98.846)
(5859, 99.864)
(5860, 99.938)
(5861, 99.942)
(5862, 99.872)
(5863, 99.95)
(5864, 99.902)
(5865, 99.908)
(5866, 99.844)
(5867, 99.77)
(5868, 99.818)
(5869, 99.522)
(5870, 99.864)
(5871, 99.95)
(5872, 99.948)
(5873, 99.974)
(5874, 99.98)
(5875, 99.994)
(5876, 99.94)
(5877, 99.984)
(5878, 99.976)
(5879, 99.704)
(5880, 99.984)
(5881, 99.986)
(5882, 99.992)
(5883, 99.964)
(5884, 99.97)
(5885, 99.988)
(5886, 99.978)
(5887, 99.982)
(5888, 99.946)
(5889, 99.954)
(5890, 99.906)
(5891, 99.88)
(5892, 99.974)
(5893, 99.906)
(5894, 99.976)
(5895, 99.95)
(5896, 99.978)
(5897, 99.956)
(5898, 99.968)
(5899, 99.738)
(5900, 99.958)
(5901, 99.952)
(5902, 99.944)
(5903, 99.938)
(5904, 99.868)
(5905, 99.954)
(5906, 99.93)
(5907, 99.892)
(5908, 99.928)
(5909, 99.944)
(5910, 99.948)
(5911, 99.958)
(5912, 99.966)
(5913, 99.918)
(5914, 99.942)
(5915, 99.812)
(5916, 99.974)
(5917, 99.816)
(5918, 99.948)
(5919, 99.878)
(5920, 99.936)
(5921, 99.964)
(5922, 99.978)
(5923, 99.924)
(5924, 99.908)
(5925, 99.972)
(5926, 99.976)
(5927, 99.89)
(5928, 99.98)
(5929, 99.986)
(5930, 99.984)
(5931, 99.75)
(5932, 99.992)
(5933, 99.996)
(5934, 100)
(5935, 99.996)
(5936, 99.998)
(5937, 100)
(5938, 100)
(5939, 99.986)
(5940, 100)
(5941, 99.998)
(5942, 99.992)
(5943, 100)
(5944, 100)
(5945, 100)
(5946, 99.992)
(5947, 100)
(5948, 100)
(5949, 100)
(5950, 100)
(5951, 100)
(5952, 100)
(5953, 99.992)
(5954, 100)
(5955, 100)
(5956, 100)
(5957, 100)
(5958, 99.998)
(5959, 100)
(5960, 100)
(5961, 100)
(5962, 100)
(5963, 100)
(5964, 100)
(5965, 99.996)
(5966, 100)
(5967, 100)
(5968, 100)
(5969, 100)
(5970, 100)
(5971, 100)
(5972, 100)
(5973, 100)
(5974, 100)
(5975, 100)
(5976, 100)
(5977, 100)
(5978, 100)
(5979, 100)
(5980, 100)
(5981, 100)
(5982, 100)
(5983, 100)
(5984, 100)
(5985, 100)
(5986, 100)
(5987, 100)
(5988, 99.998)
(5989, 99.992)
(5990, 98.934)
(5991, 99.998)
(5992, 100)
(5993, 100)
(5994, 100)
(5995, 100)
(5996, 100)
(5997, 100)
(5998, 99.996)
(5999, 100)
(6000, 100)
(6001, 100)
(6002, 99.998)
(6003, 99.942)
(6004, 100)
(6005, 100)
(6006, 100)
(6007, 100)
(6008, 100)
(6009, 99.998)
(6010, 100)
(6011, 100)
(6012, 100)
(6013, 100)
(6014, 100)
(6015, 100)
(6016, 100)
(6017, 100)
(6018, 100)
(6019, 99.998)
(6020, 100)
(6021, 100)
(6022, 100)
(6023, 100)
(6024, 99.994)
(6025, 100)
(6026, 100)
(6027, 100)
(6028, 99.966)
(6029, 100)
(6030, 99.976)
(6031, 99.942)
(6032, 99.99)
(6033, 99.996)
(6034, 99.998)
(6035, 99.992)
(6036, 100)
(6037, 99.972)
(6038, 99.97)
(6039, 99.998)
(6040, 99.996)
(6041, 99.99)
(6042, 99.996)
(6043, 100)
(6044, 100)
(6045, 100)
(6046, 99.998)
(6047, 100)
(6048, 100)
(6049, 100)
(6050, 100)
(6051, 100)
(6052, 100)
(6053, 99.988)
(6054, 100)
(6055, 99.996)
(6056, 100)
(6057, 100)
(6058, 100)
(6059, 99.992)
(6060, 99.998)
(6061, 100)
(6062, 100)
(6063, 100)
(6064, 100)
(6065, 100)
(6066, 100)
(6067, 99.998)
(6068, 100)
(6069, 99.886)
(6070, 99.974)
(6071, 99.996)
(6072, 100)
(6073, 100)
(6074, 99.982)
(6075, 99.998)
(6076, 99.992)
(6077, 99.992)
(6078, 99.958)
(6079, 99.982)
(6080, 99.978)
(6081, 99.96)
(6082, 99.998)
(6083, 99.992)
(6084, 99.994)
(6085, 99.996)
(6086, 99.91)
(6087, 99.964)
(6088, 99.93)
(6089, 99.942)
(6090, 99.91)
(6091, 99.954)
(6092, 99.966)
(6093, 99.952)
(6094, 99.99)
(6095, 99.952)
(6096, 99.91)
(6097, 99.992)
(6098, 99.97)
(6099, 99.994)
(6100, 99.642)
(6101, 99.92)
(6102, 99.636)
(6103, 99.984)
(6104, 99.96)
(6105, 99.98)
(6106, 99.97)
(6107, 99.998)
(6108, 99.968)
(6109, 99.988)
(6110, 99.954)
(6111, 99.938)
(6112, 99.972)
(6113, 99.978)
(6114, 99.972)
(6115, 99.904)
(6116, 99.884)
(6117, 99.98)
(6118, 99.86)
(6119, 99.972)
(6120, 99.866)
(6121, 99.926)
(6122, 99.912)
(6123, 99.986)
(6124, 99.974)
(6125, 99.964)
(6126, 99.984)
(6127, 99.984)
(6128, 99.998)
(6129, 100)
(6130, 100)
(6131, 99.996)
(6132, 99.998)
(6133, 100)
(6134, 99.98)
(6135, 99.996)
(6136, 100)
(6137, 99.994)
(6138, 99.996)
(6139, 99.976)
(6140, 100)
(6141, 100)
(6142, 99.984)
(6143, 100)
(6144, 100)
(6145, 99.998)
(6146, 99.988)
(6147, 99.918)
(6148, 99.802)
(6149, 99.898)
(6150, 99.99)
(6151, 99.956)
(6152, 99.938)
(6153, 99.972)
(6154, 99.972)
(6155, 99.96)
(6156, 99.874)
(6157, 99.868)
(6158, 99.922)
(6159, 99.984)
(6160, 99.954)
(6161, 99.962)
(6162, 99.96)
(6163, 99.93)
(6164, 99.988)
(6165, 99.922)
(6166, 99.972)
(6167, 99.992)
(6168, 99.99)
(6169, 99.994)
(6170, 99.976)
(6171, 99.986)
(6172, 99.976)
(6173, 99.95)
(6174, 99.972)
(6175, 99.964)
(6176, 99.95)
(6177, 99.94)
(6178, 99.95)
(6179, 99.97)
(6180, 99.928)
(6181, 99.878)
(6182, 99.978)
(6183, 99.958)
(6184, 99.978)
(6185, 99.936)
(6186, 99.968)
(6187, 99.776)
(6188, 99.978)
(6189, 99.98)
(6190, 99.974)
(6191, 99.988)
(6192, 99.988)
(6193, 100)
(6194, 99.998)
(6195, 99.948)
(6196, 99.996)
(6197, 100)
(6198, 99.998)
(6199, 99.994)
(6200, 99.992)
(6201, 99.966)
(6202, 99.958)
(6203, 98.85)
(6204, 99.988)
(6205, 99.998)
(6206, 99.06)
(6207, 99.996)
(6208, 99.996)
(6209, 100)
(6210, 99.998)
(6211, 99.922)
(6212, 99.97)
(6213, 99.972)
(6214, 99.992)
(6215, 100)
(6216, 99.996)
(6217, 99.98)
(6218, 99.986)
(6219, 99.81)
(6220, 99.986)
(6221, 99.996)
(6222, 99.99)
(6223, 99.982)
(6224, 99.984)
(6225, 99.984)
(6226, 100)
(6227, 99.988)
(6228, 99.996)
(6229, 99.978)
(6230, 99.962)
(6231, 99.946)
(6232, 99.968)
(6233, 99.93)
(6234, 99.972)
(6235, 99.87)
(6236, 99.972)
(6237, 99.854)
(6238, 100)
(6239, 99.994)
(6240, 99.974)
(6241, 99.97)
(6242, 99.802)
(6243, 99.846)
(6244, 99.88)
(6245, 99.72)
(6246, 99.8)
(6247, 99.704)
(6248, 99.67)
(6249, 99.856)
(6250, 99.72)
(6251, 99.666)
(6252, 99.904)
(6253, 99.728)
(6254, 99.906)
(6255, 99.958)
(6256, 99.992)
(6257, 99.964)
(6258, 99.638)
(6259, 99.928)
(6260, 99.938)
(6261, 99.95)
(6262, 99.878)
(6263, 99.972)
(6264, 99.996)
(6265, 99.926)
(6266, 99.95)
(6267, 99.974)
(6268, 99.98)
(6269, 99.99)
(6270, 99.976)
(6271, 99.99)
(6272, 99.93)
(6273, 99.97)
(6274, 99.926)
(6275, 99.946)
(6276, 99.536)
(6277, 99.958)
(6278, 99.946)
(6279, 99.97)
(6280, 99.85)
(6281, 99.96)
(6282, 99.922)
(6283, 99.638)
(6284, 99.862)
(6285, 99.852)
(6286, 99.824)
(6287, 99.634)
(6288, 99.966)
(6289, 99.972)
(6290, 99.778)
(6291, 99.966)
(6292, 99.948)
(6293, 99.826)
(6294, 99.986)
(6295, 99.948)
(6296, 99.912)
(6297, 99.988)
(6298, 99.892)
(6299, 99.944)
(6300, 99.974)
(6301, 99.868)
(6302, 99.974)
(6303, 99.676)
(6304, 99.938)
(6305, 99.906)
(6306, 99.964)
(6307, 99.844)
(6308, 99.932)
(6309, 99.96)
(6310, 99.968)
(6311, 99.946)
(6312, 99.928)
(6313, 99.938)
(6314, 99.872)
(6315, 99.914)
(6316, 99.896)
(6317, 99.88)
(6318, 99.9)
(6319, 99.878)
(6320, 99.86)
(6321, 99.794)
(6322, 99.95)
(6323, 99.892)
(6324, 99.82)
(6325, 99.888)
(6326, 99.866)
(6327, 99.91)
(6328, 99.942)
(6329, 99.914)
(6330, 99.92)
(6331, 99.932)
(6332, 99.99)
(6333, 99.962)
(6334, 99.972)
(6335, 99.958)
(6336, 99.972)
(6337, 99.992)
(6338, 99.99)
(6339, 99.976)
(6340, 99.998)
(6341, 99.982)
(6342, 99.988)
(6343, 99.99)
(6344, 99.92)
(6345, 99.942)
(6346, 99.866)
(6347, 99.68)
(6348, 99.854)
(6349, 99.96)
(6350, 99.902)
(6351, 99.858)
(6352, 99.942)
(6353, 99.874)
(6354, 99.952)
(6355, 99.934)
(6356, 99.346)
(6357, 99.932)
(6358, 99.976)
(6359, 99.93)
(6360, 99.854)
(6361, 99.736)
(6362, 99.894)
(6363, 99.972)
(6364, 99.94)
(6365, 99.89)
(6366, 99.986)
(6367, 99.952)
(6368, 99.408)
(6369, 99.174)
(6370, 99.388)
(6371, 99.998)
(6372, 99.994)
(6373, 100)
(6374, 99.992)
(6375, 99.982)
(6376, 99.996)
(6377, 99.998)
(6378, 99.984)
(6379, 99.996)
(6380, 99.996)
(6381, 99.992)
(6382, 99.994)
(6383, 99.974)
(6384, 99.956)
(6385, 99.994)
(6386, 99.992)
(6387, 99.902)
(6388, 99.984)
(6389, 99.94)
(6390, 99.908)
(6391, 99.862)
(6392, 99.81)
(6393, 99.868)
(6394, 98.682)
(6395, 99.746)
(6396, 99.772)
(6397, 99.318)
(6398, 99.912)
(6399, 99.676)
(6400, 99.88)
(6401, 99.708)
(6402, 99.754)
(6403, 99.754)
(6404, 99.66)
(6405, 99.404)
(6406, 99.458)
(6407, 99.69)
(6408, 99.658)
(6409, 99.292)
(6410, 97.99)
(6411, 99.346)
(6412, 99.402)
(6413, 99.006)
(6414, 99.45)
(6415, 97.798)
(6416, 99.068)
(6417, 99.484)
(6418, 99.586)
(6419, 99.086)
(6420, 99.432)
(6421, 99.578)
(6422, 99.518)
(6423, 99.546)
(6424, 99.704)
(6425, 99.144)
(6426, 99.584)
(6427, 99.32)
(6428, 98.836)
(6429, 99.272)
(6430, 99.318)
(6431, 98.962)
(6432, 99.098)
(6433, 99.092)
(6434, 99.68)
(6435, 99.224)
(6436, 98.196)
(6437, 99.084)
(6438, 99.646)
(6439, 99.268)
(6440, 99.202)
(6441, 99.126)
(6442, 99.322)
(6443, 99.202)
(6444, 98.848)
(6445, 98.584)
(6446, 98.604)
(6447, 99.222)
(6448, 99.396)
(6449, 98.822)
(6450, 98.898)
(6451, 99.238)
(6452, 99.002)
(6453, 99.076)
(6454, 99.108)
(6455, 98.676)
(6456, 98.838)
(6457, 98.954)
(6458, 98.892)
(6459, 98.402)
(6460, 98.382)
(6461, 97.558)
(6462, 98.686)
(6463, 99.388)
(6464, 99.722)
(6465, 99.184)
(6466, 99.272)
(6467, 99.42)
(6468, 99.416)
(6469, 99.398)
(6470, 99.432)
(6471, 99.022)
(6472, 99.436)
(6473, 99.376)
(6474, 99.348)
(6475, 98.89)
(6476, 99.456)
(6477, 98.714)
(6478, 99.436)
(6479, 99.486)
(6480, 99.162)
(6481, 99.34)
(6482, 99.382)
(6483, 99.238)
(6484, 99.09)
(6485, 99.48)
(6486, 99.206)
(6487, 99.32)
(6488, 99.438)
(6489, 99.618)
(6490, 99.72)
(6491, 99.21)
(6492, 99.554)
(6493, 99.74)
(6494, 99.874)
(6495, 99.632)
(6496, 99.682)
(6497, 99.868)
(6498, 99.818)
(6499, 99.896)
(6500, 99.93)
(6501, 99.858)
(6502, 99.828)
(6503, 99.656)
(6504, 99.714)
(6505, 99.902)
(6506, 99.808)
(6507, 99.578)
(6508, 99.21)
(6509, 99.732)
(6510, 99.754)
(6511, 99.802)
(6512, 99.778)
(6513, 99.386)
(6514, 99.608)
(6515, 99.638)
(6516, 99.66)
(6517, 99.55)
(6518, 99.54)
(6519, 99.694)
(6520, 99.65)
(6521, 99.716)
(6522, 99.366)
(6523, 99.794)
(6524, 99.824)
(6525, 99.8)
(6526, 99.83)
(6527, 99.808)
(6528, 99.854)
(6529, 99.628)
(6530, 99.738)
(6531, 99.758)
(6532, 99.818)
(6533, 99.836)
(6534, 99.754)
(6535, 99.756)
(6536, 99.324)
(6537, 99.358)
(6538, 98.338)
(6539, 99.128)
(6540, 98.964)
(6541, 98.142)
(6542, 99.062)
(6543, 99.124)
(6544, 99.076)
(6545, 99.202)
(6546, 99.616)
(6547, 98.876)
(6548, 99.458)
(6549, 99.548)
(6550, 99.02)
(6551, 99.792)
(6552, 99.708)
(6553, 99.872)
(6554, 98.912)
(6555, 99.568)
(6556, 99.56)
(6557, 99.5)
(6558, 99.562)
(6559, 99.858)
(6560, 99.106)
(6561, 99.566)
(6562, 99.458)
(6563, 99.668)
(6564, 99.886)
(6565, 99.794)
(6566, 99.36)
(6567, 99.608)
(6568, 99.86)
(6569, 99.864)
(6570, 99.948)
(6571, 99.934)
(6572, 99.968)
(6573, 99.926)
(6574, 99.974)
(6575, 99.95)
(6576, 99.914)
(6577, 99.484)
(6578, 99.978)
(6579, 99.944)
(6580, 99.926)
(6581, 99.42)
(6582, 99.926)
(6583, 99.468)
(6584, 98.388)
(6585, 99.706)
(6586, 99.804)
(6587, 99.21)
(6588, 99.682)
(6589, 99.92)
(6590, 99.88)
(6591, 99.718)
(6592, 99.946)
(6593, 99.81)
(6594, 99.91)
(6595, 99.954)
(6596, 99.78)
(6597, 99.918)
(6598, 99.944)
(6599, 99.608)
(6600, 99.736)
(6601, 99.81)
(6602, 99.574)
(6603, 99.702)
(6604, 99.782)
(6605, 99.882)
(6606, 99.946)
(6607, 99.904)
(6608, 99.662)
(6609, 99.954)
(6610, 99.952)
(6611, 99.97)
(6612, 99.976)
(6613, 99.972)
(6614, 99.96)
(6615, 99.922)
(6616, 99.752)
(6617, 99.972)
(6618, 99.974)
(6619, 99.98)
(6620, 99.986)
(6621, 99.974)
(6622, 99.992)
(6623, 99.982)
(6624, 99.96)
(6625, 99.878)
(6626, 99.946)
(6627, 99.95)
(6628, 99.934)
(6629, 99.75)
(6630, 99.882)
(6631, 99.906)
(6632, 99.92)
(6633, 99.842)
(6634, 99.92)
(6635, 99.96)
(6636, 99.916)
(6637, 99.97)
(6638, 99.978)
(6639, 99.992)
(6640, 99.97)
(6641, 99.948)
(6642, 99.8)
(6643, 99.746)
(6644, 99.77)
(6645, 99.92)
(6646, 99.94)
(6647, 99.806)
(6648, 99.79)
(6649, 99.962)
(6650, 99.9)
(6651, 99.95)
(6652, 99.948)
(6653, 99.902)
(6654, 99.616)
(6655, 99.248)
(6656, 99.842)
(6657, 99.946)
(6658, 99.65)
(6659, 99.662)
(6660, 99.752)
(6661, 99.77)
(6662, 99.782)
(6663, 99.68)
(6664, 99.69)
(6665, 99.768)
(6666, 99.852)
(6667, 99.68)
(6668, 99.796)
(6669, 99.782)
(6670, 99.862)
(6671, 99.87)
(6672, 99.864)
(6673, 99.644)
(6674, 99.692)
(6675, 99.722)
(6676, 99.858)
(6677, 99.608)
(6678, 99.882)
(6679, 99.934)
(6680, 99.96)
(6681, 99.91)
(6682, 99.998)
(6683, 99.996)
(6684, 99.952)
(6685, 99.982)
(6686, 99.954)
(6687, 99.996)
(6688, 100)
(6689, 99.992)
(6690, 100)
(6691, 99.996)
(6692, 99.994)
(6693, 100)
(6694, 99.984)
(6695, 99.986)
(6696, 100)
(6697, 99.972)
(6698, 99.982)
(6699, 99.762)
(6700, 99.894)
(6701, 99.966)
(6702, 99.942)
(6703, 99.888)
(6704, 99.966)
(6705, 99.668)
(6706, 99.322)
(6707, 99.574)
(6708, 99.786)
(6709, 99.714)
(6710, 99.626)
(6711, 99.682)
(6712, 99.728)
(6713, 99.212)
(6714, 99.88)
(6715, 99.798)
(6716, 99.848)
(6717, 99.944)
(6718, 99.98)
(6719, 99.988)
(6720, 99.99)
(6721, 99.96)
(6722, 99.982)
(6723, 99.98)
(6724, 99.984)
(6725, 99.976)
(6726, 99.98)
(6727, 99.868)
(6728, 99.648)
(6729, 99.85)
(6730, 99.986)
(6731, 99.996)
(6732, 99.978)
(6733, 99.994)
(6734, 99.932)
(6735, 99.246)
(6736, 99.716)
(6737, 99.458)
(6738, 99.844)
(6739, 99.822)
(6740, 99.746)
(6741, 99.934)
(6742, 99.858)
(6743, 99.95)
(6744, 99.958)
(6745, 99.96)
(6746, 99.872)
(6747, 99.956)
(6748, 99.934)
(6749, 99.96)
(6750, 99.966)
(6751, 99.98)
(6752, 99.968)
(6753, 99.986)
(6754, 99.956)
(6755, 99.966)
(6756, 99.984)
(6757, 99.986)
(6758, 99.976)
(6759, 99.944)
(6760, 99.996)
(6761, 99.91)
(6762, 99.992)
(6763, 99.972)
(6764, 99.982)
(6765, 99.998)
(6766, 99.986)
(6767, 99.972)
(6768, 99.922)
(6769, 99.912)
(6770, 99.912)
(6771, 99.908)
(6772, 99.854)
(6773, 99.796)
(6774, 99.966)
(6775, 99.94)
(6776, 99.758)
(6777, 99.984)
(6778, 99.56)
(6779, 99.948)
(6780, 99.606)
(6781, 99.686)
(6782, 99.932)
(6783, 99.618)
(6784, 99.98)
(6785, 99.928)
(6786, 99.93)
(6787, 99.904)
(6788, 99.94)
(6789, 99.952)
(6790, 99.932)
(6791, 99.914)
(6792, 99.87)
(6793, 99.602)
(6794, 99.638)
(6795, 99.792)
(6796, 99.66)
(6797, 99.726)
(6798, 99.876)
(6799, 99.918)
(6800, 99.878)
(6801, 99.852)
(6802, 99.938)
(6803, 99.668)
(6804, 99.822)
(6805, 99.994)
(6806, 99.984)
(6807, 99.87)
(6808, 99.822)
(6809, 99.924)
(6810, 99.972)
(6811, 99.686)
(6812, 99.924)
(6813, 99.95)
(6814, 99.972)
(6815, 99.968)
(6816, 99.996)
(6817, 99.996)
(6818, 100)
(6819, 100)
(6820, 100)
(6821, 100)
(6822, 100)
(6823, 100)
(6824, 99.984)
(6825, 100)
(6826, 99.994)
(6827, 100)
(6828, 100)
(6829, 100)
(6830, 100)
(6831, 100)
(6832, 100)
(6833, 100)
(6834, 99.998)
(6835, 100)
(6836, 100)
(6837, 100)
(6838, 100)
(6839, 100)
(6840, 100)
(6841, 100)
(6842, 99.998)
(6843, 100)
(6844, 97.686)
(6845, 100)
(6846, 100)
(6847, 100)
(6848, 99.998)
(6849, 100)
(6850, 100)
(6851, 100)
(6852, 99.996)
(6853, 99.998)
(6854, 100)
(6855, 100)
(6856, 100)
(6857, 100)
(6858, 100)
(6859, 100)
(6860, 100)
(6861, 99.994)
(6862, 99.996)
(6863, 100)
(6864, 100)
(6865, 100)
(6866, 100)
(6867, 100)
(6868, 100)
(6869, 100)
(6870, 100)
(6871, 100)
(6872, 100)
(6873, 100)
(6874, 100)
(6875, 99.97)
(6876, 100)
(6877, 100)
(6878, 100)
(6879, 99.996)
(6880, 100)
(6881, 100)
(6882, 99.996)
(6883, 100)
(6884, 99.998)
(6885, 100)
(6886, 100)
(6887, 99.998)
(6888, 99.994)
(6889, 99.994)
(6890, 100)
(6891, 99.998)
(6892, 100)
(6893, 99.998)
(6894, 99.988)
(6895, 99.998)
(6896, 99.998)
(6897, 99.988)
(6898, 99.984)
(6899, 99.998)
(6900, 99.982)
(6901, 99.98)
(6902, 99.986)
(6903, 99.96)
(6904, 99.988)
(6905, 99.976)
(6906, 99.926)
(6907, 99.978)
(6908, 99.964)
(6909, 99.962)
(6910, 99.93)
(6911, 99.956)
(6912, 99.964)
(6913, 99.96)
(6914, 99.92)
(6915, 99.966)
(6916, 99.986)
(6917, 99.928)
(6918, 99.968)
(6919, 99.972)
(6920, 99.986)
(6921, 99.962)
(6922, 99.98)
(6923, 99.986)
(6924, 99.984)
(6925, 99.972)
(6926, 99.968)
(6927, 99.966)
(6928, 99.966)
(6929, 99.974)
(6930, 99.966)
(6931, 99.966)
(6932, 99.944)
(6933, 99.806)
(6934, 99.868)
(6935, 99.93)
(6936, 99.764)
(6937, 99.292)
(6938, 99.858)
(6939, 99.946)
(6940, 99.914)
(6941, 99.858)
(6942, 99.868)
(6943, 99.9)
(6944, 99.912)
(6945, 99.958)
(6946, 99.834)
(6947, 99.914)
(6948, 99.914)
(6949, 99.796)
(6950, 99.902)
(6951, 99.226)
(6952, 99.774)
(6953, 99.672)
(6954, 99.41)
(6955, 99.286)
(6956, 99.03)
(6957, 97.876)
(6958, 98.872)
(6959, 99.162)
(6960, 99.27)
(6961, 99.252)
(6962, 99.092)
(6963, 99.05)
(6964, 99.524)
(6965, 99.556)
(6966, 99.71)
(6967, 99.714)
(6968, 99.732)
(6969, 99.55)
(6970, 99.422)
(6971, 99.406)
(6972, 99.322)
(6973, 99.384)
(6974, 99.136)
(6975, 99.174)
(6976, 99.488)
(6977, 99.014)
(6978, 98.67)
(6979, 98.69)
(6980, 99.378)
(6981, 99.046)
(6982, 99.126)
(6983, 99.284)
(6984, 98.85)
(6985, 99.054)
(6986, 98.63)
(6987, 98.616)
(6988, 98.788)
(6989, 99.16)
(6990, 98.48)
(6991, 98.856)
(6992, 98.936)
(6993, 99.464)
(6994, 99.528)
(6995, 99.332)
(6996, 98.832)
(6997, 99.28)
(6998, 99.382)
(6999, 98.89)
(7000, 99.062)
(7001, 99.544)
(7002, 99.34)
(7003, 99.09)
(7004, 99.482)
(7005, 99.358)
(7006, 99.282)
(7007, 98.24)
(7008, 99.124)
(7009, 99.394)
(7010, 99.068)
(7011, 99.65)
(7012, 99.132)
(7013, 98.954)
(7014, 99.374)
(7015, 99.296)
(7016, 99.402)
(7017, 99.114)
(7018, 99.052)
(7019, 98.548)
(7020, 99.094)
(7021, 99.054)
(7022, 99.008)
(7023, 98.472)
(7024, 98.228)
(7025, 98.86)
(7026, 98.662)
(7027, 98.594)
(7028, 97.132)
(7029, 97.774)
(7030, 98.74)
(7031, 96.826)
(7032, 97.578)
(7033, 97.4)
(7034, 98.116)
(7035, 97.236)
(7036, 96.63)
(7037, 95.654)
(7038, 95.492)
(7039, 93.702)
(7040, 86.132)
(7041, 93.888)
(7042, 93.11)
(7043, 88.286)
(7044, 90.814)
(7045, 93.112)
(7046, 93.158)
(7047, 95.312)
(7048, 96.636)
(7049, 96.79)
(7050, 95.232)
(7051, 95.796)
(7052, 92.506)
(7053, 96.152)
(7054, 94.61)
(7055, 96.332)
(7056, 95.058)
(7057, 97.118)
(7058, 95.64)
(7059, 93.46)
(7060, 96.58)
(7061, 95.702)
(7062, 95.438)
(7063, 95.21)
(7064, 92.446)
(7065, 89.51)
(7066, 89.854)
(7067, 94.198)
(7068, 92.312)
(7069, 96.682)
(7070, 94.666)
(7071, 94.086)
(7072, 91.56)
(7073, 94)
(7074, 96.034)
(7075, 95.75)
(7076, 98.02)
(7077, 96.686)
(7078, 95.438)
(7079, 95.206)
(7080, 97.24)
(7081, 95.106)
(7082, 98.134)
(7083, 97.678)
(7084, 95.006)
(7085, 96.754)
(7086, 93.498)
(7087, 97.232)
(7088, 97.114)
(7089, 95.384)
(7090, 95.822)
(7091, 96.298)
(7092, 94.282)
(7093, 94.928)
(7094, 91.198)
(7095, 92.65)
(7096, 94.412)
(7097, 95.506)
(7098, 90.228)
(7099, 90.33)
(7100, 94.294)
(7101, 95.83)
(7102, 96.73)
(7103, 97.628)
(7104, 94.584)
(7105, 95.946)
(7106, 96.664)
(7107, 97.072)
(7108, 88.964)
(7109, 93.716)
(7110, 97.36)
(7111, 93.762)
(7112, 95.668)
(7113, 93.628)
(7114, 94.01)
(7115, 91.726)
(7116, 88.87)
(7117, 96.132)
(7118, 92.05)
(7119, 94.418)
(7120, 95.334)
(7121, 96.772)
(7122, 90.644)
(7123, 98.16)
(7124, 97.282)
(7125, 97.052)
(7126, 97.144)
(7127, 95.896)
(7128, 94.9)
(7129, 95.132)
(7130, 92.642)
(7131, 95.326)
(7132, 92.966)
(7133, 94.036)
(7134, 94.942)
(7135, 98.358)
(7136, 94.998)
(7137, 96.14)
(7138, 94.99)
(7139, 96.452)
(7140, 97.304)
(7141, 97.08)
(7142, 97.12)
(7143, 95.026)
(7144, 96.072)
(7145, 98.362)
(7146, 98.724)
(7147, 96.822)
(7148, 97.482)
(7149, 97.57)
(7150, 98.864)
(7151, 98.466)
(7152, 98.188)
(7153, 98.51)
(7154, 98.974)
(7155, 98.474)
(7156, 98.656)
(7157, 98.944)
(7158, 98.902)
(7159, 99.306)
(7160, 99.578)
(7161, 99.63)
(7162, 99.676)
(7163, 99.806)
(7164, 99.828)
(7165, 99.6)
(7166, 98.83)
(7167, 99.28)
(7168, 99.14)
(7169, 97.48)
(7170, 99.194)
(7171, 98.432)
(7172, 96.838)
(7173, 98.978)
(7174, 98.476)
(7175, 98.888)
(7176, 98.794)
(7177, 98.31)
(7178, 98.924)
(7179, 99.05)
(7180, 99.622)
(7181, 99.414)
(7182, 99.054)
(7183, 99.096)
(7184, 98.786)
(7185, 97.03)
(7186, 98.218)
(7187, 97.884)
(7188, 98.628)
(7189, 97.904)
(7190, 98.526)
(7191, 99.298)
(7192, 98.578)
(7193, 98.058)
(7194, 98.24)
(7195, 99.132)
(7196, 98.714)
(7197, 99.31)
(7198, 98.176)
(7199, 98.572)
(7200, 98.068)
(7201, 98.696)
(7202, 98.232)
(7203, 94.418)
(7204, 97.656)
(7205, 97.31)
(7206, 98.346)
(7207, 98.82)
(7208, 97.908)
(7209, 97.698)
(7210, 96.49)
(7211, 92.46)
(7212, 97.242)
(7213, 98.322)
(7214, 99.296)
(7215, 98.544)
(7216, 99.014)
(7217, 97.606)
(7218, 97.998)
(7219, 99.338)
(7220, 99.122)
(7221, 99.378)
(7222, 98.876)
(7223, 98.994)
(7224, 99.13)
(7225, 99.04)
(7226, 97.222)
(7227, 97.88)
(7228, 96.642)
(7229, 97.28)
(7230, 95.324)
(7231, 98.262)
(7232, 96.198)
(7233, 98.836)
(7234, 96.386)
(7235, 91.118)
(7236, 96.844)
(7237, 97.11)
(7238, 96.786)
(7239, 95.838)
(7240, 93.424)
(7241, 98.242)
(7242, 99.686)
(7243, 99.826)
(7244, 99.892)
(7245, 99.944)
(7246, 99.974)
(7247, 99.864)
(7248, 99.846)
(7249, 99.732)
(7250, 99.73)
(7251, 99.078)
(7252, 99.61)
(7253, 99.454)
(7254, 99.64)
(7255, 99.556)
(7256, 99.276)
(7257, 99.76)
(7258, 99.944)
(7259, 99.946)
(7260, 99.95)
(7261, 99.902)
(7262, 99.924)
(7263, 99.92)
(7264, 99.906)
(7265, 99.894)
(7266, 99.804)
(7267, 99.868)
(7268, 99.674)
(7269, 99.22)
(7270, 99.616)
(7271, 99.586)
(7272, 99.554)
(7273, 99.486)
(7274, 99.714)
(7275, 99.564)
(7276, 99.734)
(7277, 99.75)
(7278, 99.618)
(7279, 99.72)
(7280, 99.66)
(7281, 99.012)
(7282, 99.356)
(7283, 99.442)
(7284, 99.588)
(7285, 99.42)
(7286, 99.576)
(7287, 99.68)
(7288, 99.078)
(7289, 99.54)
(7290, 99.586)
(7291, 99.9)
(7292, 99.966)
(7293, 99.886)
(7294, 99.654)
(7295, 99.866)
(7296, 99.946)
(7297, 99.956)
(7298, 99.978)
(7299, 99.972)
(7300, 99.854)
(7301, 99.718)
(7302, 99.916)
(7303, 99.914)
(7304, 99.928)
(7305, 99.884)
(7306, 99.89)
(7307, 99.68)
(7308, 99.844)
(7309, 99.884)
(7310, 99.874)
(7311, 99.906)
(7312, 99.96)
(7313, 99.942)
(7314, 99.644)
(7315, 99.49)
(7316, 99.74)
(7317, 99.852)
(7318, 99.75)
(7319, 99.744)
(7320, 99.772)
(7321, 99.516)
(7322, 99.84)
(7323, 99.896)
(7324, 99.932)
(7325, 99.938)
(7326, 99.922)
(7327, 99.922)
(7328, 99.652)
(7329, 98.954)
(7330, 99.56)
(7331, 99.818)
(7332, 99.798)
(7333, 99.83)
(7334, 99.862)
(7335, 99.764)
(7336, 99.58)
(7337, 99.568)
(7338, 99.688)
(7339, 99.892)
(7340, 99.92)
(7341, 99.764)
(7342, 99.318)
(7343, 99.474)
(7344, 99.746)
(7345, 99.612)
(7346, 99.144)
(7347, 99.696)
(7348, 99.694)
(7349, 99.552)
(7350, 99.376)
(7351, 99.44)
(7352, 99.204)
(7353, 99.582)
(7354, 99.292)
(7355, 98.782)
(7356, 98.974)
(7357, 99.366)
(7358, 98.228)
(7359, 98.976)
(7360, 98.956)
(7361, 98.122)
(7362, 99.472)
(7363, 99.396)
(7364, 99.404)
(7365, 99.388)
(7366, 99.088)
(7367, 98.034)
(7368, 98.71)
(7369, 97.502)
(7370, 98.202)
(7371, 97.954)
(7372, 98.07)
(7373, 98.104)
(7374, 98.744)
(7375, 98.456)
(7376, 97.474)
(7377, 97.86)
(7378, 98.716)
(7379, 98.384)
(7380, 98.224)
(7381, 98.244)
(7382, 98.398)
(7383, 97.748)
(7384, 98.242)
(7385, 97.512)
(7386, 96.098)
(7387, 98.054)
(7388, 98.578)
(7389, 98.28)
(7390, 97.51)
(7391, 98.354)
(7392, 97.628)
(7393, 96.932)
(7394, 96.758)
(7395, 96.754)
(7396, 97.992)
(7397, 98.062)
(7398, 97.886)
(7399, 95.024)
(7400, 96.098)
(7401, 96.438)
(7402, 95.722)
(7403, 96.942)
(7404, 89.82)
(7405, 94.204)
(7406, 96.372)
(7407, 95.346)
(7408, 96.22)
(7409, 96.946)
(7410, 96.838)
(7411, 97.988)
(7412, 95.742)
(7413, 96.91)
(7414, 97.162)
(7415, 97.07)
(7416, 95.364)
(7417, 98.51)
(7418, 98.098)
(7419, 96.984)
(7420, 97.82)
(7421, 96.91)
(7422, 97.632)
(7423, 97.82)
(7424, 96.588)
(7425, 95.19)
(7426, 96.374)
(7427, 97.21)
(7428, 96.416)
(7429, 94.578)
(7430, 95.696)
(7431, 96.81)
(7432, 96.884)
(7433, 97.93)
(7434, 98.348)
(7435, 97.798)
(7436, 97.452)
(7437, 98.122)
(7438, 98.058)
(7439, 98.65)
(7440, 98.14)
(7441, 97.596)
(7442, 96.902)
(7443, 96.378)
(7444, 95.438)
(7445, 97.052)
(7446, 97.358)
(7447, 97.944)
(7448, 97.254)
(7449, 98.504)
(7450, 98.774)
(7451, 98.262)
(7452, 95.224)
(7453, 95.754)
(7454, 94.342)
(7455, 96.672)
(7456, 95.666)
(7457, 96.242)
(7458, 95.968)
(7459, 93.646)
(7460, 96.236)
(7461, 96.754)
(7462, 93.974)
(7463, 95.652)
(7464, 94.846)
(7465, 94.886)
(7466, 95.952)
(7467, 96.962)
(7468, 97.258)
(7469, 98.138)
(7470, 97.628)
(7471, 96.24)
(7472, 95.62)
(7473, 97.402)
(7474, 96.086)
(7475, 97.638)
(7476, 97.752)
(7477, 98.406)
(7478, 95.668)
(7479, 97.982)
(7480, 97.278)
(7481, 97.768)
(7482, 96.278)
(7483, 96.756)
(7484, 98.608)
(7485, 97.04)
(7486, 92.304)
(7487, 98.328)
(7488, 98.382)
(7489, 97.504)
(7490, 93.472)
(7491, 97.362)
(7492, 95.658)
(7493, 95.392)
(7494, 91.312)
(7495, 97.54)
(7496, 97.83)
(7497, 98.374)
(7498, 98.04)
(7499, 98.48)
(7500, 99.082)
(7501, 98.788)
(7502, 98.012)
(7503, 98.036)
(7504, 99.224)
(7505, 98.9)
(7506, 96.904)
(7507, 98.38)
(7508, 97.962)
(7509, 98.68)
(7510, 94.92)
(7511, 97.8)
(7512, 98.332)
(7513, 93.598)
(7514, 95.436)
(7515, 97.202)
(7516, 96.402)
(7517, 94.464)
(7518, 97.902)
(7519, 97.604)
(7520, 96.486)
(7521, 88.344)
(7522, 94.628)
(7523, 96.46)
(7524, 96.71)
(7525, 95.788)
(7526, 95.954)
(7527, 98.53)
(7528, 99.73)
(7529, 99.71)
(7530, 98.272)
(7531, 99.74)
(7532, 99.946)
(7533, 99.974)
(7534, 99.99)
(7535, 99.962)
(7536, 99.962)
(7537, 99.916)
(7538, 99.84)
(7539, 99.902)
(7540, 99.614)
(7541, 99.91)
(7542, 99.914)
(7543, 99.932)
(7544, 99.874)
(7545, 99.964)
(7546, 99.92)
(7547, 99.944)
(7548, 99.934)
(7549, 99.964)
(7550, 99.988)
(7551, 99.896)
(7552, 99.802)
(7553, 99.844)
(7554, 99.856)
(7555, 99.93)
(7556, 99.892)
(7557, 99.93)
(7558, 99.898)
(7559, 99.878)
(7560, 99.924)
(7561, 99.712)
(7562, 99.744)
(7563, 99.94)
(7564, 99.936)
(7565, 99.958)
(7566, 99.948)
(7567, 99.932)
(7568, 99.946)
(7569, 99.976)
(7570, 99.972)
(7571, 99.662)
(7572, 99.956)
(7573, 99.996)
(7574, 100)
(7575, 99.99)
(7576, 99.998)
(7577, 99.966)
(7578, 99.998)
(7579, 99.862)
(7580, 99.972)
(7581, 99.994)
(7582, 100)
(7583, 99.996)
(7584, 99.936)
(7585, 99.978)
(7586, 99.944)
(7587, 99.88)
(7588, 99.988)
(7589, 99.964)
(7590, 100)
(7591, 100)
(7592, 100)
(7593, 100)
(7594, 100)
(7595, 100)
(7596, 99.998)
(7597, 100)
(7598, 100)
(7599, 100)
(7600, 100)
(7601, 99.998)
(7602, 99.998)
(7603, 99.996)
(7604, 99.996)
(7605, 99.984)
(7606, 99.994)
(7607, 99.986)
(7608, 99.952)
(7609, 99.994)
(7610, 99.988)
(7611, 99.982)
(7612, 99.988)
(7613, 99.936)
(7614, 99.92)
(7615, 99.96)
(7616, 99.964)
(7617, 99.878)
(7618, 99.952)
(7619, 99.976)
(7620, 99.932)
(7621, 99.408)
(7622, 99.356)
(7623, 99.428)
(7624, 99.926)
(7625, 99.94)
(7626, 99.766)
(7627, 99.93)
(7628, 99.79)
(7629, 99.84)
(7630, 99.912)
(7631, 99.938)
(7632, 99.914)
(7633, 99.762)
(7634, 99.894)
(7635, 99.892)
(7636, 99.128)
(7637, 99.848)
(7638, 99.836)
(7639, 99.65)
(7640, 99.454)
(7641, 99.672)
(7642, 99.584)
(7643, 99.288)
(7644, 99.554)
(7645, 99.294)
(7646, 99.708)
(7647, 98.848)
(7648, 99.16)
(7649, 99.542)
(7650, 99.6)
(7651, 99.496)
(7652, 99.468)
(7653, 99.748)
(7654, 99.43)
(7655, 99.476)
(7656, 99.3)
(7657, 99.596)
(7658, 99.522)
(7659, 98.764)
(7660, 99.698)
(7661, 99.292)
(7662, 99.754)
(7663, 99.75)
(7664, 99.786)
(7665, 99.694)
(7666, 99.852)
(7667, 99.856)
(7668, 99.744)
(7669, 99.812)
(7670, 99.686)
(7671, 99.792)
(7672, 99.848)
(7673, 99.776)
(7674, 99.724)
(7675, 99.754)
(7676, 99.872)
(7677, 99.494)
(7678, 99.3)
(7679, 99.712)
(7680, 99.492)
(7681, 99.536)
(7682, 99.586)
(7683, 99.598)
(7684, 99.384)
(7685, 99.09)
(7686, 98.202)
(7687, 98.92)
(7688, 99.364)
(7689, 98.974)
(7690, 98.742)
(7691, 98.74)
(7692, 98.822)
(7693, 99.022)
(7694, 99.102)
(7695, 97.588)
(7696, 98.434)
(7697, 98.626)
(7698, 98.686)
(7699, 98.206)
(7700, 98.386)
(7701, 98.41)
(7702, 99.048)
(7703, 99.288)
(7704, 98.412)
(7705, 95.796)
(7706, 97.508)
(7707, 99.148)
(7708, 98.922)
(7709, 98.908)
(7710, 99.048)
(7711, 98.908)
(7712, 98.116)
(7713, 98.348)
(7714, 98.048)
(7715, 98.994)
(7716, 99.53)
(7717, 99.112)
(7718, 98.642)
(7719, 98.696)
(7720, 99.072)
(7721, 97.798)
(7722, 98.942)
(7723, 99.018)
(7724, 98.508)
(7725, 98.616)
(7726, 98.204)
(7727, 99.384)
(7728, 99.316)
(7729, 99.258)
(7730, 99.192)
(7731, 99.218)
(7732, 98.806)
(7733, 98.74)
(7734, 98.8)
(7735, 98.944)
(7736, 99.038)
(7737, 98.966)
(7738, 98.86)
(7739, 99.192)
(7740, 97.678)
(7741, 98.47)
(7742, 97.856)
(7743, 98.128)
(7744, 98.46)
(7745, 98.662)
(7746, 99.208)
(7747, 99.554)
(7748, 99.302)
(7749, 98.336)
(7750, 98.912)
(7751, 97.362)
(7752, 97.988)
(7753, 97.232)
(7754, 98.71)
(7755, 98.502)
(7756, 98.696)
(7757, 98.64)
(7758, 98.9)
(7759, 97.398)
(7760, 97.772)
(7761, 98.886)
(7762, 96.334)
(7763, 98.466)
(7764, 98.746)
(7765, 97.712)
(7766, 98.052)
(7767, 98.622)
(7768, 98.842)
(7769, 98.556)
(7770, 98.4)
(7771, 97.974)
(7772, 98.678)
(7773, 95.474)
(7774, 99.12)
(7775, 98.208)
(7776, 99.4)
(7777, 98.956)
(7778, 98.49)
(7779, 96.816)
(7780, 98.486)
(7781, 98.006)
(7782, 98.23)
(7783, 98.11)
(7784, 98.222)
(7785, 97.388)
(7786, 98.1)
(7787, 97.976)
(7788, 98.558)
(7789, 99.098)
(7790, 98.676)
(7791, 99.212)
(7792, 99.204)
(7793, 99.102)
(7794, 99.03)
(7795, 98.786)
(7796, 99.132)
(7797, 99.038)
(7798, 99.186)
(7799, 98.828)
(7800, 98.858)
(7801, 98.278)
(7802, 96.164)
(7803, 98.006)
(7804, 96.99)
(7805, 96.488)
(7806, 97.766)
(7807, 97.28)
(7808, 97)
(7809, 96.036)
(7810, 95.274)
(7811, 95.934)
(7812, 94.974)
(7813, 90.262)
(7814, 90.468)
(7815, 88.742)
(7816, 90.036)
(7817, 94.696)
(7818, 92.832)
(7819, 94.24)
(7820, 89.194)
(7821, 95.892)
(7822, 93.852)
(7823, 91.148)
(7824, 90.824)
(7825, 88.002)
(7826, 93.456)
(7827, 89.55)
(7828, 90.8)
(7829, 90.63)
(7830, 86.864)
(7831, 76.716)
(7832, 83.846)
(7833, 89.754)
(7834, 89.514)
(7835, 89.27)
(7836, 88.076)
(7837, 78.978)
(7838, 76.648)
(7839, 86.654)
(7840, 85.584)
(7841, 88.384)
(7842, 80.968)
(7843, 79.94)
(7844, 70.666)
(7845, 79.712)
(7846, 63.18)
(7847, 71.616)
(7848, 72.952)
(7849, 79.508)
(7850, 78.246)
(7851, 75.224)
(7852, 56.118)
(7853, 63.976)
(7854, 83.576)
(7855, 67.976)
(7856, 69.458)
(7857, 79.19)
(7858, 65.976)
(7859, 58.256)
(7860, 65.232)
(7861, 60.838)
(7862, 62.036)
(7863, 63.218)
(7864, 70.764)
(7865, 69.846)
(7866, 57.894)
(7867, 46.862)
(7868, 45.828)
(7869, 73.994)
(7870, 58.726)
(7871, 77.264)
(7872, 43.584)
(7873, 50.518)
(7874, 77.562)
(7875, 71.712)
(7876, 62.04)
(7877, 70.22)
(7878, 75.648)
(7879, 91.412)
(7880, 99.074)
(7881, 99.934)
(7882, 97.244)
(7883, 97.446)
(7884, 96.878)
(7885, 99.956)
(7886, 99.988)
(7887, 95.694)
(7888, 99.218)
(7889, 97.664)
(7890, 92.32)
(7891, 88.328)
(7892, 93.172)
(7893, 90.166)
(7894, 90.068)
(7895, 90.038)
(7896, 85.896)
(7897, 80.61)
(7898, 83.58)
(7899, 86.158)
(7900, 88.258)
(7901, 83.062)
(7902, 83.988)
(7903, 77.98)
(7904, 80.988)
(7905, 78.714)
(7906, 87.02)
(7907, 74.732)
(7908, 86.664)
(7909, 85.606)
(7910, 78.36)
(7911, 80.516)
(7912, 85.42)
(7913, 87.388)
(7914, 91.138)
(7915, 85.47)
(7916, 92.52)
(7917, 84.552)
(7918, 86.242)
(7919, 93.818)
(7920, 90.166)
(7921, 94.548)
(7922, 94.822)
(7923, 94.054)
(7924, 93.238)
(7925, 92.052)
(7926, 90.968)
(7927, 93.81)
(7928, 91.186)
(7929, 91.996)
(7930, 92.882)
(7931, 94.724)
(7932, 94.054)
(7933, 93.2)
(7934, 90.314)
(7935, 92.978)
(7936, 90.998)
(7937, 93.996)
(7938, 94.184)
(7939, 93.308)
(7940, 93.34)
(7941, 93.592)
(7942, 93.49)
(7943, 95.026)
(7944, 92.084)
(7945, 95.282)
(7946, 91.706)
(7947, 93.148)
(7948, 93.758)
(7949, 97.064)
(7950, 96.954)
(7951, 96.366)
(7952, 97.89)
(7953, 97.476)
(7954, 96.44)
(7955, 97.744)
(7956, 97.072)
(7957, 96.812)
(7958, 96.338)
(7959, 96.188)
(7960, 97.684)
(7961, 97.728)
(7962, 97.632)
(7963, 97.75)
(7964, 96.604)
(7965, 97.56)
(7966, 97.798)
(7967, 97.038)
(7968, 98.856)
(7969, 97.4)
(7970, 98.41)
(7971, 96.424)
(7972, 98.86)
(7973, 98.384)
(7974, 98.548)
(7975, 96.878)
(7976, 96.832)
(7977, 98.698)
(7978, 98.622)
(7979, 97.974)
(7980, 97.828)
(7981, 98.08)
(7982, 98.042)
(7983, 96.52)
(7984, 98.328)
(7985, 97.386)
(7986, 97.342)
(7987, 97.032)
(7988, 98.052)
(7989, 97.778)
(7990, 97.576)
(7991, 97.122)
(7992, 94.67)
(7993, 96.622)
(7994, 96.092)
(7995, 96.692)
(7996, 98.676)
(7997, 99.212)
(7998, 99.19)
(7999, 97.968)
(8000, 98.742)
(8001, 99.29)
(8002, 98.234)
(8003, 98.348)
(8004, 97.494)
(8005, 98.89)
(8006, 98.712)
(8007, 98.492)
(8008, 96.826)
(8009, 96.17)
(8010, 98.092)
(8011, 98.716)
(8012, 98.534)
(8013, 98.66)
(8014, 98.95)
(8015, 98.13)
(8016, 99.094)
(8017, 98.686)
(8018, 98.674)
(8019, 97.782)
(8020, 98.326)
(8021, 97.888)
(8022, 97.974)
(8023, 98.248)
(8024, 98.558)
(8025, 98.738)
(8026, 98.446)
(8027, 98.688)
(8028, 99.15)
(8029, 98.484)
(8030, 99.196)
(8031, 98.982)
(8032, 98.798)
(8033, 99.318)
(8034, 98.972)
(8035, 99.17)
(8036, 98.882)
(8037, 99.284)
(8038, 99.582)
(8039, 99.448)
(8040, 99.426)
(8041, 99.54)
(8042, 99.652)
(8043, 98.176)
(8044, 99.562)
(8045, 99.66)
(8046, 99.498)
(8047, 99.396)
(8048, 99.784)
(8049, 99.712)
(8050, 99.498)
(8051, 99.46)
(8052, 98.772)
(8053, 98.536)
(8054, 99.228)
(8055, 99.398)
(8056, 99.068)
(8057, 99.23)
(8058, 99.45)
(8059, 99.362)
(8060, 99.474)
(8061, 98.106)
(8062, 99.192)
(8063, 99.296)
(8064, 99.126)
(8065, 99.664)
(8066, 99.512)
(8067, 99.534)
(8068, 99.884)
(8069, 99.986)
(8070, 99.96)
(8071, 99.02)
(8072, 99.91)
(8073, 99.992)
(8074, 99.992)
(8075, 100)
(8076, 99.998)
(8077, 99.966)
(8078, 100)
(8079, 100)
(8080, 100)
(8081, 99.474)
(8082, 99.98)
(8083, 99.992)
(8084, 99.998)
(8085, 100)
(8086, 100)
(8087, 100)
(8088, 100)
(8089, 100)
(8090, 99.966)
(8091, 100)
(8092, 100)
(8093, 99.994)
(8094, 99.978)
(8095, 99.998)
(8096, 99.996)
(8097, 99.994)
(8098, 99.994)
(8099, 99.47)
(8100, 99.988)
(8101, 99.99)
(8102, 99.998)
(8103, 99.958)
(8104, 99.82)
(8105, 99.978)
(8106, 99.93)
(8107, 99.91)
(8108, 99.968)
(8109, 99.984)
(8110, 99.994)
(8111, 99.988)
(8112, 99.99)
(8113, 99.878)
(8114, 99.962)
(8115, 99.956)
(8116, 99.97)
(8117, 99.942)
(8118, 99.996)
(8119, 99.992)
(8120, 99.996)
(8121, 99.978)
(8122, 99.942)
(8123, 99.988)
(8124, 99.946)
(8125, 99.984)
(8126, 99.912)
(8127, 99.912)
(8128, 99.798)
(8129, 99.892)
(8130, 99.806)
(8131, 99.706)
(8132, 99.872)
(8133, 99.924)
(8134, 99.982)
(8135, 99.976)
(8136, 99.864)
(8137, 99.778)
(8138, 99.768)
(8139, 99.674)
(8140, 99.668)
(8141, 98.664)
(8142, 99.596)
(8143, 99.586)
(8144, 99.59)
(8145, 99.768)
(8146, 99.868)
(8147, 99.902)
(8148, 99.932)
(8149, 99.89)
(8150, 99.8)
(8151, 99.836)
(8152, 99.814)
(8153, 99.758)
(8154, 99.746)
(8155, 99.852)
(8156, 99.79)
(8157, 99.634)
(8158, 99.48)
(8159, 99.602)
(8160, 99.454)
(8161, 99.566)
(8162, 98.472)
(8163, 99.206)
(8164, 99.522)
(8165, 99.436)
(8166, 99.204)
(8167, 99.166)
(8168, 98.94)
(8169, 99.33)
(8170, 99.642)
(8171, 99.754)
(8172, 99.344)
(8173, 99.426)
(8174, 99.646)
(8175, 99.198)
(8176, 99.134)
(8177, 99.396)
(8178, 97.27)
(8179, 98.766)
(8180, 99.388)
(8181, 99.472)
(8182, 99.508)
(8183, 99.288)
(8184, 99.372)
(8185, 98.912)
(8186, 99.246)
(8187, 99.562)
(8188, 99.422)
(8189, 99.236)
(8190, 99.644)
(8191, 99.76)
(8192, 99.458)
(8193, 99.638)
(8194, 99.628)
(8195, 99.37)
(8196, 99.664)
(8197, 99.368)
(8198, 98.928)
(8199, 99.25)
(8200, 99.128)
(8201, 99.344)
(8202, 99.362)
(8203, 98.674)
(8204, 99.466)
(8205, 99.228)
(8206, 99.496)
(8207, 99.582)
(8208, 99.632)
(8209, 99.068)
(8210, 99.434)
(8211, 99.372)
(8212, 99.302)
(8213, 99.572)
(8214, 99.534)
(8215, 99.356)
(8216, 99.278)
(8217, 99.482)
(8218, 98.938)
(8219, 99.556)
(8220, 99.458)
(8221, 99.648)
(8222, 99.682)
(8223, 99.504)
(8224, 99.43)
(8225, 99.116)
(8226, 98.092)
(8227, 99.09)
(8228, 98.788)
(8229, 99.468)
(8230, 99.194)
(8231, 99.48)
(8232, 99.654)
(8233, 98.834)
(8234, 99.29)
(8235, 98.612)
(8236, 98.95)
(8237, 98.882)
(8238, 98.838)
(8239, 98.296)
(8240, 98.634)
(8241, 95.558)
(8242, 98.158)
(8243, 97.93)
(8244, 98.48)
(8245, 96.852)
(8246, 93.334)
(8247, 96.696)
(8248, 94.922)
(8249, 98.116)
(8250, 97.474)
(8251, 96.924)
(8252, 98.156)
(8253, 96.432)
(8254, 97.124)
(8255, 97.268)
(8256, 96.45)
(8257, 94.352)
(8258, 92.922)
(8259, 96.414)
(8260, 97.78)
(8261, 97.928)
(8262, 97.322)
(8263, 97.664)
(8264, 96.782)
(8265, 96.672)
(8266, 97.664)
(8267, 98.128)
(8268, 98.254)
(8269, 96.562)
(8270, 97.924)
(8271, 97.742)
(8272, 94.438)
(8273, 96.77)
(8274, 96.302)
(8275, 94.878)
(8276, 88.666)
(8277, 95.548)
(8278, 93.882)
(8279, 94.458)
(8280, 95.658)
(8281, 92.162)
(8282, 90.866)
(8283, 95.936)
(8284, 95.394)
(8285, 96.034)
(8286, 96.446)
(8287, 93.534)
(8288, 96.912)
(8289, 95.02)
(8290, 96.114)
(8291, 96.732)
(8292, 96.92)
(8293, 98.014)
(8294, 97.442)
(8295, 96.666)
(8296, 98.066)
(8297, 96.214)
(8298, 96.072)
(8299, 96.508)
(8300, 96.41)
(8301, 97.722)
(8302, 97.64)
(8303, 95.852)
(8304, 97.146)
(8305, 97.366)
(8306, 97.052)
(8307, 95.812)
(8308, 96.908)
(8309, 96.864)
(8310, 94.962)
(8311, 96.4)
(8312, 97.916)
(8313, 97.608)
(8314, 96.12)
(8315, 97.198)
(8316, 98.882)
(8317, 97.954)
(8318, 97.78)
(8319, 98.368)
(8320, 98.18)
(8321, 98.252)
(8322, 98.064)
(8323, 97.522)
(8324, 98.762)
(8325, 98.28)
(8326, 98.378)
(8327, 98.564)
(8328, 98.198)
(8329, 99.556)
(8330, 99.906)
(8331, 99.954)
(8332, 99.762)
(8333, 98.362)
(8334, 99.944)
(8335, 99.962)
(8336, 99.998)
(8337, 99.99)
(8338, 99.986)
(8339, 99.864)
(8340, 99.882)
(8341, 99.82)
(8342, 99.756)
(8343, 99.83)
(8344, 99.892)
(8345, 99.872)
(8346, 99.848)
(8347, 99.662)
(8348, 99.524)
(8349, 99.71)
(8350, 99.518)
(8351, 99.578)
(8352, 99.63)
(8353, 99.812)
(8354, 99.624)
(8355, 99.824)
(8356, 99.834)
(8357, 99.808)
(8358, 99.894)
(8359, 99.78)
(8360, 99.682)
(8361, 99.734)
(8362, 99.804)
(8363, 99.772)
(8364, 99.72)
(8365, 99.582)
(8366, 99.82)
(8367, 99.788)
(8368, 99.84)
(8369, 99.808)
(8370, 99.892)
(8371, 99.79)
(8372, 99.758)
(8373, 99.798)
(8374, 99.546)
(8375, 99.87)
(8376, 99.946)
(8377, 99.7)
(8378, 99.404)
(8379, 99.25)
(8380, 98.648)
(8381, 98.94)
(8382, 98.93)
(8383, 97.938)
(8384, 98.59)
(8385, 99.058)
(8386, 99.084)
(8387, 98.534)
(8388, 99.142)
(8389, 99.582)
(8390, 99.04)
(8391, 99.014)
(8392, 98.748)
(8393, 99.246)
(8394, 98.96)
(8395, 99.73)
(8396, 99.766)
(8397, 99.59)
(8398, 99.332)
(8399, 99.624)
(8400, 99.478)
(8401, 99.432)
(8402, 99.536)
(8403, 99.214)
(8404, 99.192)
(8405, 98.228)
(8406, 98.618)
(8407, 98.374)
(8408, 98.832)
(8409, 99.074)
(8410, 99.094)
(8411, 99.606)
(8412, 99.694)
(8413, 99.856)
(8414, 99.96)
(8415, 99.706)
(8416, 97.23)
(8417, 99.976)
(8418, 99.972)
(8419, 99.994)
(8420, 99.998)
(8421, 99.99)
(8422, 99.996)
(8423, 99.954)
(8424, 99.946)
(8425, 99.86)
(8426, 99.85)
(8427, 99.87)
(8428, 99.608)
(8429, 99.686)
(8430, 99.458)
(8431, 99.42)
(8432, 99.758)
(8433, 99.634)
(8434, 98.412)
(8435, 99.21)
(8436, 99.07)
(8437, 99.576)
(8438, 99.608)
(8439, 98.674)
(8440, 99.092)
(8441, 99.094)
(8442, 98.526)
(8443, 98.578)
(8444, 95.754)
(8445, 97.096)
(8446, 98.602)
(8447, 97.952)
(8448, 98.184)
(8449, 97.402)
(8450, 98.582)
(8451, 98.726)
(8452, 97.226)
(8453, 98.268)
(8454, 98.542)
(8455, 97.8)
(8456, 98.636)
(8457, 98.046)
(8458, 98.39)
(8459, 98.276)
(8460, 97.862)
(8461, 97.002)
(8462, 96.938)
(8463, 97.49)
(8464, 97.39)
(8465, 96.614)
(8466, 97.636)
(8467, 95.536)
(8468, 90.14)
(8469, 93.55)
(8470, 92.944)
(8471, 95.18)
(8472, 95.764)
(8473, 94.43)
(8474, 95.968)
(8475, 96.532)
(8476, 96.314)
(8477, 96.91)
(8478, 96.778)
(8479, 96.712)
(8480, 96.6)
(8481, 95.41)
(8482, 95.162)
(8483, 95.29)
(8484, 96.038)
(8485, 96.582)
(8486, 96.816)
(8487, 96.946)
(8488, 96.956)
(8489, 96.26)
(8490, 94.59)
(8491, 90.926)
(8492, 95.468)
(8493, 96.614)
(8494, 95.176)
(8495, 95.378)
(8496, 91.38)
(8497, 97.234)
(8498, 97.666)
(8499, 98.214)
(8500, 97.488)
(8501, 96.262)
(8502, 95.828)
(8503, 97.674)
(8504, 97.12)
(8505, 97.308)
(8506, 96.778)
(8507, 94.92)
(8508, 96.574)
(8509, 97.9)
(8510, 97.708)
(8511, 96.878)
(8512, 96.62)
(8513, 93.178)
(8514, 98.166)
(8515, 98.262)
(8516, 98.33)
(8517, 98.566)
(8518, 98.848)
(8519, 98.188)
(8520, 97.672)
(8521, 97.982)
(8522, 98.52)
(8523, 97.68)
(8524, 96.95)
(8525, 98.082)
(8526, 97.27)
(8527, 97.872)
(8528, 97.088)
(8529, 97.81)
(8530, 97.874)
(8531, 97.78)
(8532, 98.296)
(8533, 98.416)
(8534, 98.696)
(8535, 97.528)
(8536, 97.886)
(8537, 97.846)
(8538, 96.894)
(8539, 96.202)
(8540, 95.698)
(8541, 95.194)
(8542, 95.146)
(8543, 97.246)
(8544, 95.782)
(8545, 93.032)
(8546, 98.298)
(8547, 97.938)
(8548, 98.22)
(8549, 97.764)
(8550, 96.168)
(8551, 97.164)
(8552, 98.238)
(8553, 97.204)
(8554, 95.656)
(8555, 97.264)
(8556, 94.552)
(8557, 92.464)
(8558, 95.284)
(8559, 97.656)
(8560, 98.124)
(8561, 97.69)
(8562, 95.708)
(8563, 93.756)
(8564, 95.088)
(8565, 94.608)
(8566, 96.258)
(8567, 90.542)
(8568, 91.834)
(8569, 91.442)
(8570, 95.746)
(8571, 96.164)
(8572, 94.214)
(8573, 96.108)
(8574, 94.942)
(8575, 93.8)
(8576, 92.156)
(8577, 91.272)
(8578, 87.506)
(8579, 91.078)
(8580, 89.83)
(8581, 92.028)
(8582, 94.784)
(8583, 95.096)
(8584, 96.524)
(8585, 93.46)
(8586, 94.992)
(8587, 96.964)
(8588, 83.46)
(8589, 96.658)
(8590, 95.484)
(8591, 93.942)
(8592, 94.21)
(8593, 95.416)
(8594, 93.462)
(8595, 91.226)
(8596, 94.024)
(8597, 92.776)
(8598, 92.734)
(8599, 93.11)
(8600, 95.09)
(8601, 92.986)
(8602, 93.234)
(8603, 90.27)
(8604, 96.47)
(8605, 94.866)
(8606, 89.14)
(8607, 93.942)
(8608, 90.798)
(8609, 96.434)
(8610, 93.814)
(8611, 95.752)
(8612, 94.232)
(8613, 94.752)
(8614, 93.104)
(8615, 96.186)
(8616, 97.172)
(8617, 95.942)
(8618, 93.764)
(8619, 95.402)
(8620, 96.452)
(8621, 95.872)
(8622, 93.83)
(8623, 95.69)
(8624, 92.78)
(8625, 91.884)
(8626, 92.892)
(8627, 89.78)
(8628, 90.716)
(8629, 78.234)
(8630, 92.02)
(8631, 92.96)
(8632, 81.204)
(8633, 89.222)
(8634, 88.262)
(8635, 89.256)
(8636, 85.272)
(8637, 87.036)
(8638, 90.776)
(8639, 81.286)
(8640, 93.436)
(8641, 91.648)
(8642, 95.296)
(8643, 95.37)
(8644, 96.27)
(8645, 93.78)
(8646, 97.216)
(8647, 96.346)
(8648, 97.286)
(8649, 98.742)
(8650, 98.684)
(8651, 97.256)
(8652, 97.88)
(8653, 98.7)
(8654, 98.494)
(8655, 97.878)
(8656, 98.498)
(8657, 99.008)
(8658, 98.884)
(8659, 98.044)
(8660, 98.592)
(8661, 97.74)
(8662, 98.216)
(8663, 98.286)
(8664, 98.258)
(8665, 97.234)
(8666, 98.46)
(8667, 98.768)
(8668, 94.918)
(8669, 97.786)
(8670, 98.914)
(8671, 98.864)
(8672, 98.42)
(8673, 98.492)
(8674, 95.988)
(8675, 98.578)
(8676, 98.034)
(8677, 98.99)
(8678, 98.784)
(8679, 98.518)
(8680, 97.936)
(8681, 98.664)
(8682, 99.042)
(8683, 99.338)
(8684, 99.516)
(8685, 99.482)
(8686, 98.962)
(8687, 98.63)
(8688, 99.068)
(8689, 98.712)
(8690, 99.306)
(8691, 98.822)
(8692, 99.49)
(8693, 99.608)
(8694, 99.548)
(8695, 99.408)
(8696, 99.37)
(8697, 99.444)
(8698, 99.28)
(8699, 99.562)
(8700, 99.798)
(8701, 99.866)
(8702, 99.678)
(8703, 99.728)
(8704, 99.568)
(8705, 99.61)
(8706, 99.176)
(8707, 99.332)
(8708, 98.852)
(8709, 99.46)
(8710, 99.27)
(8711, 99.5)
(8712, 99.52)
(8713, 99.414)
(8714, 99.088)
(8715, 99.462)
(8716, 99.496)
(8717, 99.5)
(8718, 99.442)
(8719, 99.06)
(8720, 99.37)
(8721, 98.742)
(8722, 99.174)
(8723, 98.464)
(8724, 97.192)
(8725, 98.37)
(8726, 98.534)
(8727, 98.958)
(8728, 98.954)
(8729, 98.964)
(8730, 98.926)
(8731, 99.166)
(8732, 99.38)
(8733, 98.276)
(8734, 97.754)
(8735, 97.724)
(8736, 96.442)
(8737, 97.476)
(8738, 98.332)
(8739, 98.338)
(8740, 97.79)
(8741, 97.648)
(8742, 98.788)
(8743, 98.868)
(8744, 98.772)
(8745, 98.618)
(8746, 98.372)
(8747, 98.964)
(8748, 98.652)
(8749, 98.74)
(8750, 95.674)
(8751, 97.774)
(8752, 97.412)
(8753, 94.352)
(8754, 97.586)
(8755, 94.04)
(8756, 96.634)
(8757, 96.464)
(8758, 94.684)
(8759, 94.418)
(8760, 96.44)
(8761, 95.42)
(8762, 95.866)
(8763, 97.616)
(8764, 96.274)
(8765, 96.62)
(8766, 95.048)
(8767, 96.048)
(8768, 94.172)
(8769, 96.218)
(8770, 94.428)
(8771, 91.066)
(8772, 92.39)
(8773, 93.752)
(8774, 92)
(8775, 95.754)
(8776, 95.742)
(8777, 89.008)
(8778, 94.848)
(8779, 95.63)
(8780, 95.108)
(8781, 95.612)
(8782, 92.98)
(8783, 93.806)
(8784, 83.024)
(8785, 90.528)
(8786, 84.106)
(8787, 92.842)
(8788, 92.03)
(8789, 92.718)
(8790, 94.854)
(8791, 92.672)
(8792, 91.926)
(8793, 92.518)
(8794, 93.612)
(8795, 92.306)
(8796, 95.338)
(8797, 95.854)
(8798, 94.674)
(8799, 95.642)
(8800, 94.482)
(8801, 97.42)
(8802, 97.93)
(8803, 97.338)
(8804, 98.15)
(8805, 98.692)
(8806, 98.038)
(8807, 97.466)
(8808, 98)
(8809, 97.946)
(8810, 97.018)
(8811, 98.158)
(8812, 97.356)
(8813, 98.748)
(8814, 98.52)
(8815, 97.53)
(8816, 99.382)
(8817, 99.45)
(8818, 97.356)
(8819, 99.45)
(8820, 99.268)
(8821, 99.008)
(8822, 99.076)
(8823, 99.332)
(8824, 99.42)
(8825, 98.938)
(8826, 99.406)
(8827, 99.68)
(8828, 99.856)
(8829, 99.786)
(8830, 99.404)
(8831, 99.544)
(8832, 99.4)
(8833, 99.226)
(8834, 98.966)
(8835, 99.524)
(8836, 99.56)
(8837, 99.32)
(8838, 98.522)
(8839, 98.952)
(8840, 99.208)
(8841, 97.726)
(8842, 98.744)
(8843, 98.368)
(8844, 99.428)
(8845, 99.786)
(8846, 99.564)
(8847, 99.29)
(8848, 99.602)
(8849, 99.774)
(8850, 99.864)
(8851, 99.838)
(8852, 99.308)
(8853, 98.236)
(8854, 99.554)
(8855, 99.668)
(8856, 99.19)
(8857, 99.394)
(8858, 99.48)
(8859, 99.46)
(8860, 99.084)
(8861, 99.38)
(8862, 99.022)
(8863, 98.994)
(8864, 99.216)
(8865, 98.614)
(8866, 99.042)
(8867, 99.398)
(8868, 99.302)
(8869, 99.114)
(8870, 97.764)
(8871, 99.442)
(8872, 99.568)
(8873, 99.554)
(8874, 99.216)
(8875, 99.412)
(8876, 98.974)
(8877, 99.022)
(8878, 99.458)
(8879, 98.192)
(8880, 99.096)
(8881, 99.304)
(8882, 98.93)
(8883, 98.92)
(8884, 98.336)
(8885, 99.138)
(8886, 98.606)
(8887, 98.882)
(8888, 99.154)
(8889, 98.652)
(8890, 99.42)
(8891, 99.572)
(8892, 99.57)
(8893, 99.446)
(8894, 99.386)
(8895, 99.608)
(8896, 99.332)
(8897, 99.526)
(8898, 99.584)
(8899, 99.294)
(8900, 99.238)
(8901, 97.388)
(8902, 98.826)
(8903, 99.552)
(8904, 98.94)
(8905, 99.408)
(8906, 99.228)
(8907, 99.38)
(8908, 98.892)
(8909, 98.356)
(8910, 99.236)
(8911, 98.86)
(8912, 98.15)
(8913, 98.676)
(8914, 99.332)
(8915, 99.458)
(8916, 99.282)
(8917, 99.12)
(8918, 98.878)
(8919, 97.826)
(8920, 98.336)
(8921, 99.074)
(8922, 98.28)
(8923, 98.748)
(8924, 98.352)
(8925, 98.232)
(8926, 98.302)
(8927, 98.556)
(8928, 98.346)
(8929, 99.024)
(8930, 98.876)
(8931, 98.182)
(8932, 98.104)
(8933, 99.052)
(8934, 98.828)
(8935, 98.746)
(8936, 98.684)
(8937, 98.862)
(8938, 99.1)
(8939, 98.806)
(8940, 98.07)
(8941, 99.194)
(8942, 98.856)
(8943, 97.82)
(8944, 98.344)
(8945, 98.208)
(8946, 99.148)
(8947, 99.328)
(8948, 99.51)
(8949, 99.578)
(8950, 99.574)
(8951, 99.084)
(8952, 99.422)
(8953, 99.454)
(8954, 99.052)
(8955, 99.45)
(8956, 99.5)
(8957, 99.436)
(8958, 97.958)
(8959, 97.414)
(8960, 98.578)
(8961, 98.074)
(8962, 97.846)
(8963, 98.23)
(8964, 97.894)
(8965, 95.87)
(8966, 97.962)
(8967, 98.562)
(8968, 97.474)
(8969, 97.284)
(8970, 98.304)
(8971, 97.272)
(8972, 96.508)
(8973, 96.882)
(8974, 96.642)
(8975, 97.254)
(8976, 97.554)
(8977, 97.326)
(8978, 96.278)
(8979, 97.324)
(8980, 94.198)
(8981, 95.378)
(8982, 96.066)
(8983, 96.436)
(8984, 96.456)
(8985, 96.814)
(8986, 92.92)
(8987, 91.638)
(8988, 95.942)
(8989, 96.084)
(8990, 97.43)
(8991, 96.046)
(8992, 97.844)
(8993, 97.896)
(8994, 98.826)
(8995, 98.378)
(8996, 98.138)
(8997, 97.576)
(8998, 96.348)
(8999, 97.406)
(9000, 97.852)
(9001, 94.262)
(9002, 95.25)
(9003, 97.36)
(9004, 98.508)
(9005, 98.02)
(9006, 98.396)
(9007, 98.954)
(9008, 97.828)
(9009, 98.038)
(9010, 98.716)
(9011, 98.37)
(9012, 99.536)
(9013, 98.088)
(9014, 96.278)
(9015, 95.372)
(9016, 96.852)
(9017, 95.564)
(9018, 96.252)
(9019, 92.824)
(9020, 87.874)
(9021, 92.782)
(9022, 92.194)
(9023, 90.654)
(9024, 93.95)
(9025, 94.448)
(9026, 92.436)
(9027, 89.464)
(9028, 86.038)
(9029, 96.404)
(9030, 87.138)
(9031, 94.94)
(9032, 97.178)
(9033, 96.908)
(9034, 98.168)
(9035, 96.714)
(9036, 97.008)
(9037, 94.446)
(9038, 93.604)
(9039, 93.32)
(9040, 95.664)
(9041, 94.73)
(9042, 92.65)
(9043, 91.01)
(9044, 94.722)
(9045, 93.8)
(9046, 96.68)
(9047, 92.954)
(9048, 92.386)
(9049, 92.816)
(9050, 90.73)
(9051, 89.6)
(9052, 92.252)
(9053, 90.426)
(9054, 92.514)
(9055, 91.64)
(9056, 92.164)
(9057, 94.084)
(9058, 89.674)
(9059, 94.416)
(9060, 93.416)
(9061, 83.626)
(9062, 91.752)
(9063, 91.26)
(9064, 94.026)
(9065, 95.262)
(9066, 94.638)
(9067, 96.042)
(9068, 94.036)
(9069, 93.92)
(9070, 94.514)
(9071, 94.384)
(9072, 93.828)
(9073, 95.168)
(9074, 90.132)
(9075, 95.292)
(9076, 93.216)
(9077, 91.316)
(9078, 91.776)
(9079, 89.56)
(9080, 87.87)
(9081, 85.094)
(9082, 87.202)
(9083, 86.484)
(9084, 82.332)
(9085, 94.388)
(9086, 91.096)
(9087, 94.154)
(9088, 92.082)
(9089, 88.966)
(9090, 89.818)
(9091, 95.24)
(9092, 95.672)
(9093, 94.338)
(9094, 95.288)
(9095, 95.924)
(9096, 96.06)
(9097, 94.98)
(9098, 96.228)
(9099, 95.754)
(9100, 94.608)
(9101, 94.14)
(9102, 94.784)
(9103, 93.092)
(9104, 93.446)
(9105, 95.56)
(9106, 94.936)
(9107, 96.828)
(9108, 97.77)
(9109, 97.506)
(9110, 96.706)
(9111, 97.076)
(9112, 97.004)
(9113, 92.354)
(9114, 94.438)
(9115, 93.794)
(9116, 95.512)
(9117, 98.102)
(9118, 97.586)
(9119, 97.104)
(9120, 97.184)
(9121, 98.57)
(9122, 98.544)
(9123, 98.006)
(9124, 97.068)
(9125, 97.118)
(9126, 96.178)
(9127, 96.92)
(9128, 95.718)
(9129, 96.034)
(9130, 92.334)
(9131, 96.87)
(9132, 95.752)
(9133, 97.618)
(9134, 96.35)
(9135, 98.266)
(9136, 98.046)
(9137, 97.316)
(9138, 87.724)
(9139, 97.876)
(9140, 98.882)
(9141, 98.658)
(9142, 98.85)
(9143, 99.018)
(9144, 99.12)
(9145, 99.042)
(9146, 98.894)
(9147, 99.186)
(9148, 99.302)
(9149, 99.07)
(9150, 99.408)
(9151, 99.388)
(9152, 99.454)
(9153, 99.304)
(9154, 99.11)
(9155, 97.822)
(9156, 99.08)
(9157, 99.324)
(9158, 99.324)
(9159, 98.182)
(9160, 95.618)
(9161, 98.068)
(9162, 97.868)
(9163, 97.426)
(9164, 97.224)
(9165, 97.564)
(9166, 97.074)
(9167, 98.116)
(9168, 98.19)
(9169, 98.424)
(9170, 97.878)
(9171, 97.442)
(9172, 97.638)
(9173, 96.314)
(9174, 98.052)
(9175, 95.91)
(9176, 96.996)
(9177, 94.974)
(9178, 98.516)
(9179, 98.444)
(9180, 97.714)
(9181, 96.654)
(9182, 97.618)
(9183, 98.606)
(9184, 98.602)
(9185, 98.56)
(9186, 98.716)
(9187, 99.03)
(9188, 96.788)
(9189, 97.61)
(9190, 98.962)
(9191, 98.82)
(9192, 98.846)
(9193, 98.884)
(9194, 98.608)
(9195, 99.178)
(9196, 98.906)
(9197, 98.742)
(9198, 97.19)
(9199, 97.952)
(9200, 97.506)
(9201, 98.67)
(9202, 99.262)
(9203, 99.25)
(9204, 98.942)
(9205, 99.046)
(9206, 98.958)
(9207, 98.904)
(9208, 97.594)
(9209, 97.592)
(9210, 97.428)
(9211, 96.652)
(9212, 97.546)
(9213, 97.32)
(9214, 97.488)
(9215, 98.046)
(9216, 97.924)
(9217, 98.39)
(9218, 98.7)
(9219, 98.254)
(9220, 98.314)
(9221, 97.786)
(9222, 97.408)
(9223, 97.44)
(9224, 95.928)
(9225, 96.774)
(9226, 95.742)
(9227, 97.282)
(9228, 97.788)
(9229, 98.052)
(9230, 98.45)
(9231, 96.888)
(9232, 97.074)
(9233, 96.864)
(9234, 97.076)
(9235, 98.43)
(9236, 97.734)
(9237, 98.268)
(9238, 98.412)
(9239, 98.378)
(9240, 97.566)
(9241, 97.922)
(9242, 96.638)
(9243, 96.482)
(9244, 96.148)
(9245, 97.63)
(9246, 96.394)
(9247, 95.808)
(9248, 96.896)
(9249, 96.94)
(9250, 97.464)
(9251, 98.092)
(9252, 98.782)
(9253, 99.14)
(9254, 98.384)
(9255, 98.668)
(9256, 98.094)
(9257, 98.106)
(9258, 97.594)
(9259, 97.342)
(9260, 98.654)
(9261, 98.238)
(9262, 97.398)
(9263, 96.644)
(9264, 97.68)
(9265, 97.778)
(9266, 98.014)
(9267, 98.18)
(9268, 97.868)
(9269, 97.24)
(9270, 97.816)
(9271, 98.212)
(9272, 98.412)
(9273, 97.956)
(9274, 98.64)
(9275, 98.786)
(9276, 99.292)
(9277, 99.176)
(9278, 98.532)
(9279, 84.4685714285714)
(9280, 0)
};


==> covgraphs/graph.s.errors.tex <==
\addplot [sharp plot,color=lightred,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.0052106312252827)
(1, 0.0019893759885293)
(2, 0.000872304186372179)
(3, 0.000573525942113621)
(4, 0.000528114251908174)
(5, 0.000435152757117086)
(6, 0.000417490073106779)
(7, 0.000423718493257782)
(8, 0.000419581706739578)
(9, 0.000435478122348854)
(10, 0.00139981418856421)
(11, 0.00174753665983028)
(12, 0.000432828719747308)
(13, 0.000426089011374954)
(14, 0.000445099637059732)
(15, 0.000445471483038896)
(16, 0.000451606941695108)
(17, 0.00172662032350228)
(18, 0.0004569057468982)
(19, 0.000445239079301919)
(20, 0.00043854585167696)
(21, 0.000482191273481376)
(22, 0.000484701233840736)
(23, 0.000469362587200206)
(24, 0.000475776930340791)
(25, 0.000502689283082811)
(26, 0.000536759670923745)
(27, 0.000531739750205027)
(28, 0.000568366579152715)
(29, 0.0005674834449522)
(30, 0.000564183311887117)
(31, 0.00105999344435539)
(32, 0.000575524614251629)
(33, 0.000586633512879164)
(34, 0.000594349316946825)
(35, 0.000588120896795822)
(36, 0.000627583051334639)
(37, 0.000633857952233037)
(38, 0.000676527278342147)
(39, 0.000643572428438706)
(40, 0.000665000052988052)
(41, 0.000701998727914905)
(42, 0.000700976151472203)
(43, 0.000715385183164822)
(44, 0.000732118252227218)
(45, 0.000727284254498081)
(46, 0.000758658758990074)
(47, 0.00272484085456899)
(48, 0.000947695958647752)
(49, 0.00449464179240174)
(50, 0.000971958908788227)
(51, 0.00447865241529767)
(52, 0.00100314749029064)
(53, 0.00139195894225436)
(54, 0.0020445951164352)
(55, 0.00111758309037847)
(56, 0.00160381818888326)
(57, 0.00126608907830723)
(58, 0.00124986729746619)
(59, 0.00127854591860924)
(60, 0.00170049814346599)
(61, 0.00170709840959615)
(62, 0.00164039853708355)
(63, 0.00168539190056244)
(64, 0.00185341980239733)
(65, 0.0028322113810527)
(66, 0.00256499356427572)
(67, 0.00200257652078963)
(68, 0.00206783549013297)
(69, 0.00251535212605727)
(70, 0.00224571731041572)
(71, 0.00232994042469645)
(72, 0.00318188604370938)
(73, 0.0046994824461739)
(74, 0.00299085017191369)
(75, 0.00341568420310897)
(76, 0.00408756340671156)
(77, 0.0042874306205124)
(78, 0.00446763647816492)
(79, 0.00500769628215375)
(80, 0.00537275607219836)
(81, 0.00526682644888391)
(82, 0.00562486764607179)
(83, 0.00634136836717411)
(84, 0.00629307487063014)
(85, 0.0065959434206595)
(86, 0.00711922367483854)
(87, 0.00831015338460717)
(88, 0.00918543233881267)
(89, 0.00922693964623689)
(90, 0.00958140182587531)
(91, 0.00980209241450936)
(92, 0.0110729225290509)
(93, 0.0115493966706027)
(94, 0.0149930158028963)
(95, 0.0109105187976509)
(96, 0.0121638721511718)
(97, 0.0161993771208003)
(98, 0.0201684146216532)
(99, 0.0193248355371715)
(100, 0)
};



==> covgraphs/graph.tex <==
\addplot[const plot,fill=lightblue,draw=lightblue] coordinates {
(0, 0)
(1, 0)
(2, 0)
(3, 0)
(4, 0)
(5, 0)
(6, 3.16)
(7, 0)
(8, 0)
(9, 0)
(10, 0)
(11, 0)
(12, 0)
(13, 0)
(14, 0)
(15, 0)
(16, 2.278)
(17, 0)
(18, 0)
(19, 0)
(20, 0)
(21, 0)
(22, 0)
(23, 0)
(24, 0)
(25, 0)
(26, 0)
(27, 0)
(28, 0)
(29, 0)
(30, 2.775)
(31, 0)
(32, 0)
(33, 0)
(34, 0)
(35, 0)
(36, 0)
(37, 0)
(38, 0)
(39, 0)
(40, 0)
(41, 0)
(42, 0)
(43, 0)
(44, 0)
(45, 0)
(46, 0)
(47, 0)
(48, 0)
(49, 0)
(50, 0)
(51, 0)
(52, 0)
(53, 0)
(54, 0)
(55, 2.08)
(56, 0)
(57, 0)
(58, 0)
(59, 3.081)
(60, 0)
(61, 0)
(62, 0)
(63, 0)
(64, 0)
(65, 0)
(66, 0)
(67, 0)
(68, 0)
(69, 0)
(70, 0)
(71, 0)
(72, 0)
(73, 0)
(74, 0)
(75, 0)
(76, 0)
(77, 0)
(78, 0)
(79, 0)
(80, 0)
(81, 0)
(82, 0)
(83, 0)
(84, 0)
(85, 0)
(86, 0)
(87, 0)
(88, 0)
(89, 0)
(90, 0)
(91, 0)
(92, 0)
(93, 1.15)
(94, 0.741)
(95, 0)
(96, 0)
(97, 0)
(98, 0)
(99, 0)
(100, 0)
(101, 0)
(102, 0)
(103, 0)
(104, 0)
(105, 1.54)
(106, 0)
(107, 0)
(108, 0)
(109, 0)
(110, 2.485)
(111, 0)
(112, 0)
(113, 0)
(114, 0)
(115, 0)
(116, 0)
(117, 0)
(118, 0)
(119, 0)
(120, 0)
(121, 0)
(122, 0)
(123, 0)
(124, 0)
(125, 0)
(126, 0)
(127, 0)
(128, 0)
(129, 0)
(130, 0)
(131, 0)
(132, 0)
(133, 0)
(134, 0)
(135, 0)
(136, 0)
(137, 0)
(138, 0)
(139, 0)
(140, 0)
(141, 0)
(142, 0)
(143, 0)
(144, 0)
(145, 0)
(146, 0)
(147, 0)
(148, 0)
(149, 0)
(150, 0)
(151, 0)
(152, 2.211)
(153, 0)
(154, 0)
(155, 0)
(156, 0)
(157, 0)
(158, 0)
(159, 0)
(160, 0)
(161, 0)
(162, 0)
(163, 0)
(164, 0)
(165, 0)
(166, 0)
(167, 0)
(168, 4.186)
(169, 0)
(170, 0)
(171, 0)
(172, 0)
(173, 0)
(174, 0)
(175, 0)
(176, 0)
(177, 0)
(178, 0)
(179, 0)
(180, 0)
(181, 0)
(182, 0)
(183, 0)
(184, 0)
(185, 0)
(186, 0)
(187, 0)
(188, 0)
(189, 0)
(190, 0)
(191, 0)
(192, 0)
(193, 0)
(194, 0)
(195, 0)
(196, 0)
(197, 0)
(198, 0)
(199, 1.891)
(200, 0)
(201, 0)
(202, 4.186)
(203, 0)
(204, 0)
(205, 0)
(206, 2.278)
(207, 0)
(208, 0)
(209, 0)
(210, 0)
(211, 0)
(212, 0)
(213, 0)
(214, 0)
(215, 2.628)
(216, 2.698)
(217, 2.778)
(218, 0)
(219, 0)
(220, 0)
(221, 2.08)
(222, 0)
(223, 0)
(224, 0)
(225, 0)
(226, 0)
(227, 0)
(228, 0)
(229, 3.003)
(230, 0)
(231, 3.16)
(232, 0)
(233, 0)
(234, 3.645)
(235, 0.01)
(236, 0)
(237, 1.54)
(238, 7.822)
(239, 0)
(240, 0)
(241, 1.54)
(242, 0)
(243, 0)
(244, 1.54)
(245, 0)
(246, 0)
(247, 0)
(248, 0)
(249, 0)
(250, 0)
(251, 1.54)
(252, 0)
(253, 0)
(254, 0)
(255, 0)
(256, 0)
(257, 0)
(258, 0)
(259, 0)
(260, 0)
(261, 0)
(262, 0)
(263, 0)
(264, 0)
(265, 0)
(266, 0)
(267, 0)
(268, 0)
(269, 0)
(270, 0)
(271, 0)
(272, 0)
(273, 4.005)
(274, 0)
(275, 0)
(276, 0)
(277, 0)
(278, 0)
(279, 0)
(280, 0)
(281, 0)
(282, 0)
(283, 0)
(284, 0)
(285, 0)
(286, 0)
(287, 0)
(288, 0)
(289, 0)
(290, 0)
(291, 2.926)
(292, 0)
(293, 0)
(294, 0)
(295, 0)
(296, 0)
(297, 0)
(298, 0)
(299, 0)
(300, 0)
(301, 0)
(302, 1.54)
(303, 0)
(304, 0)
(305, 0)
(306, 0)
(307, 0)
(308, 0)
(309, 0)
(310, 0)
(311, 0)
(312, 0)
(313, 0)
(314, 0)
(315, 0)
(316, 0)
(317, 4.186)
(318, 0)
(319, 0)
(320, 0)
(321, 0)
(322, 0)
(323, 5.05)
(324, 0)
(325, 0)
(326, 0)
(327, 0)
(328, 0)
(329, 0)
(330, 0)
(331, 3.403)
(332, 1.54)
(333, 0)
(334, 2.85)
(335, 6.048)
(336, 0)
(337, 0)
(338, 0)
(339, 0)
(340, 1.54)
(341, 0)
(342, 0)
(343, 0)
(344, 0)
(345, 0)
(346, 0)
(347, 0)
(348, 0)
(349, 0)
(350, 0)
(351, 0)
(352, 0)
(353, 0)
(354, 1.77)
(355, 0)
(356, 0)
(357, 2.701)
(358, 0)
(359, 0)
(360, 0)
(361, 0)
(362, 0)
(363, 0)
(364, 0)
(365, 0)
(366, 0)
(367, 0)
(368, 0)
(369, 0)
(370, 0)
(371, 0)
(372, 0)
(373, 2.415)
(374, 0)
(375, 0)
(376, 0)
(377, 0)
(378, 0)
(379, 0)
(380, 0)
(381, 0)
(382, 0)
(383, 10.107)
(384, 0)
(385, 0)
(386, 0)
(387, 4.315)
(388, 1.54)
(389, 5.05)
(390, 3.081)
(391, 0)
(392, 2.926)
(393, 3.403)
(394, 0)
(395, 0)
(396, 2.016)
(397, 0)
(398, 0)
(399, 1.86)
(400, 3.546)
(401, 1.54)
(402, 0)
(403, 0)
(404, 0)
(405, 0)
(406, 0)
(407, 2.08)
(408, 0)
(409, 0)
(410, 0)
(411, 0)
(412, 3.003)
(413, 0)
(414, 0)
(415, 0)
(416, 0)
(417, 2.016)
(418, 1.54)
(419, 1.77)
(420, 0)
(421, 0)
(422, 0)
(423, 0)
(424, 0)
(425, 2.485)
(426, 0)
(427, 0)
(428, 0)
(429, 0)
(430, 0)
(431, 0)
(432, 0)
(433, 2.08)
(434, 0)
(435, 0)
(436, 0)
(437, 2.628)
(438, 0)
(439, 0)
(440, 0)
(441, 0)
(442, 0)
(443, 0)
(444, 0)
(445, 0)
(446, 0)
(447, 0)
(448, 0)
(449, 0)
(450, 0)
(451, 0)
(452, 0)
(453, 0)
(454, 3.828)
(455, 0)
(456, 0)
(457, 0)
(458, 2.485)
(459, 0)
(460, 0)
(461, 0)
(462, 0)
(463, 0)
(464, 0)
(465, 0)
(466, 0)
(467, 0)
(468, 1.653)
(469, 0)
(470, 0)
(471, 0)
(472, 0)
(473, 0)
(474, 0)
(475, 0)
(476, 0.9)
(477, 3.724)
(478, 0)
(479, 1.54)
(480, 4.95)
(481, 0)
(482, 0)
(483, 0)
(484, 0)
(485, 0)
(486, 0)
(487, 0)
(488, 0)
(489, 1.54)
(490, 0)
(491, 0)
(492, 0)
(493, 3.321)
(494, 0)
(495, 0)
(496, 2.08)
(497, 0)
(498, 0)
(499, 0)
(500, 0)
(501, 0)
(502, 0)
(503, 0)
(504, 0)
(505, 0)
(506, 0)
(507, 0)
(508, 0)
(509, 0)
(510, 0)
(511, 0)
(512, 0)
(513, 0)
(514, 0)
(515, 0)
(516, 0)
(517, 0)
(518, 0)
(519, 0)
(520, 0)
(521, 0)
(522, 0)
(523, 0)
(524, 0)
(525, 0)
(526, 0)
(527, 1.54)
(528, 3.003)
(529, 0)
(530, 0)
(531, 0)
(532, 0)
(533, 0)
(534, 0)
(535, 3.62)
(536, 0)
(537, 0)
(538, 2.628)
(539, 1.653)
(540, 1.54)
(541, 0)
(542, 2.628)
(543, 0)
(544, 0)
(545, 0)
(546, 0)
(547, 0)
(548, 0)
(549, 0)
(550, 0)
(551, 2.211)
(552, 0)
(553, 0)
(554, 0)
(555, 3.235)
(556, 0)
(557, 1.794)
(558, 0.351)
(559, 0)
(560, 0)
(561, 1.54)
(562, 3.916)
(563, 0)
(564, 0)
(565, 0)
(566, 0)
(567, 0)
(568, 0)
(569, 4.81)
(570, 10.37)
(571, 0)
(572, 4.861)
(573, 0.21)
(574, 0)
(575, 3.57)
(576, 14.425)
(577, 5.461)
(578, 8.868)
(579, 1.54)
(580, 0)
(581, 0)
(582, 8.133)
(583, 3.321)
(584, 8.874)
(585, 0)
(586, 0)
(587, 0)
(588, 0)
(589, 0)
(590, 0)
(591, 0)
(592, 2.145)
(593, 4.78)
(594, 0)
(595, 0)
(596, 1.54)
(597, 0)
(598, 0)
(599, 2.926)
(600, 0)
(601, 0)
(602, 1.54)
(603, 0)
(604, 3.16)
(605, 0)
(606, 0)
(607, 1.54)
(608, 0)
(609, 0)
(610, 0)
(611, 0)
(612, 0)
(613, 0)
(614, 0)
(615, 0)
(616, 0)
(617, 0)
(618, 0)
(619, 0)
(620, 0)
(621, 0)
(622, 0)
(623, 0)
(624, 0)
(625, 0)
(626, 0)
(627, 0)
(628, 0)
(629, 0)
(630, 2.08)
(631, 0)
(632, 0)
(633, 0)
(634, 0)
(635, 0)
(636, 0)
(637, 0)
(638, 2.85)
(639, 0)
(640, 0)
(641, 1.54)
(642, 0)
(643, 0)
(644, 0)
(645, 0)
(646, 0)
(647, 0)
(648, 0)
(649, 0)
(650, 0)
(651, 4.005)
(652, 0)
(653, 0)
(654, 0)
(655, 2.85)
(656, 0)
(657, 0)
(658, 0)
(659, 0)
(660, 0)
(661, 0)
(662, 0)
(663, 0)
(664, 2.346)
(665, 2.211)
(666, 0)
(667, 0)
(668, 0)
(669, 0)
(670, 0)
(671, 2.485)
(672, 0)
(673, 0)
(674, 0)
(675, 0)
(676, 0)
(677, 0)
(678, 0)
(679, 0)
(680, 0)
(681, 0)
(682, 0)
(683, 6.034)
(684, 2.628)
(685, 0)
(686, 0)
(687, 0)
(688, 0)
(689, 0)
(690, 0)
(691, 0)
(692, 0)
(693, 0)
(694, 0)
(695, 0)
(696, 0)
(697, 0)
(698, 0)
(699, 0)
(700, 0)
(701, 0)
(702, 0)
(703, 0)
(704, 0)
(705, 0)
(706, 0)
(707, 0)
(708, 0)
(709, 0)
(710, 2.775)
(711, 0)
(712, 0)
(713, 0)
(714, 4.095)
(715, 0)
(716, 0)
(717, 0)
(718, 0)
(719, 0)
(720, 0)
(721, 0)
(722, 0)
(723, 0)
(724, 0)
(725, 0)
(726, 0)
(727, 0)
(728, 0)
(729, 1.54)
(730, 0)
(731, 0)
(732, 0)
(733, 0)
(734, 0)
(735, 0)
(736, 1.54)
(737, 1.54)
(738, 0)
(739, 0)
(740, 0)
(741, 0)
(742, 0)
(743, 0)
(744, 0)
(745, 0)
(746, 0)
(747, 3.57)
(748, 0)
(749, 0)
(750, 1.711)
(751, 0)
(752, 0)
(753, 0)
(754, 0)
(755, 0)
(756, 0)
(757, 0)
(758, 0)
(759, 0)
(760, 0)
(761, 0)
(762, 0)
(763, 0)
(764, 2.016)
(765, 0)
(766, 0)
(767, 1.54)
(768, 3.003)
(769, 0)
(770, 5.05)
(771, 2.016)
(772, 0)
(773, 0)
(774, 2.926)
(775, 0)
(776, 0)
(777, 0)
(778, 4.644)
(779, 4.315)
(780, 0)
(781, 2.145)
(782, 0)
(783, 1.54)
(784, 2.85)
(785, 1.54)
(786, 0)
(787, 0)
(788, 0)
(789, 0)
(790, 0)
(791, 0)
(792, 0)
(793, 0)
(794, 0)
(795, 0)
(796, 3.655)
(797, 0)
(798, 0)
(799, 0)
(800, 1.54)
(801, 0)
(802, 0)
(803, 0)
(804, 0)
(805, 0)
(806, 0)
(807, 0)
(808, 0)
(809, 0)
(810, 0)
(811, 0)
(812, 3.741)
(813, 0)
(814, 2.209)
(815, 2.292)
(816, 3.3)
(817, 0)
(818, 4.543)
(819, 0)
(820, 0)
(821, 0)
(822, 2.211)
(823, 0)
(824, 1.54)
(825, 0)
(826, 0)
(827, 0)
(828, 3.003)
(829, 0)
(830, 0)
(831, 0)
(832, 0)
(833, 0)
(834, 0)
(835, 0)
(836, 0)
(837, 4.168)
(838, 0)
(839, 0)
(840, 1.54)
(841, 1.54)
(842, 0)
(843, 0)
(844, 0)
(845, 0)
(846, 0)
(847, 0)
(848, 2.346)
(849, 0)
(850, 2.278)
(851, 0)
(852, 0)
(853, 0)
(854, 0)
(855, 0)
(856, 0)
(857, 0)
(858, 0)
(859, 1.54)
(860, 0)
(861, 0)
(862, 0)
(863, 0)
(864, 0)
(865, 0)
(866, 0)
(867, 0)
(868, 0)
(869, 0)
(870, 0)
(871, 0)
(872, 0)
(873, 0)
(874, 7.062)
(875, 0)
(876, 0)
(877, 0)
(878, 0)
(879, 0)
(880, 1.54)
(881, 4.537)
(882, 5.344)
(883, 0)
(884, 0)
(885, 0)
(886, 0)
(887, 1.54)
(888, 0.882)
(889, 4.231)
(890, 1.711)
(891, 0)
(892, 1.653)
(893, 0)
(894, 0)
(895, 0)
(896, 0)
(897, 0)
(898, 0)
(899, 3.321)
(900, 0)
(901, 2.145)
(902, 4.7)
(903, 2.278)
(904, 2.556)
(905, 0)
(906, 3.403)
(907, 0)
(908, 0)
(909, 2.556)
(910, 2.346)
(911, 4.161)
(912, 0)
(913, 2.278)
(914, 0)
(915, 0)
(916, 0)
(917, 0)
(918, 0)
(919, 0)
(920, 0)
(921, 0)
(922, 4.186)
(923, 9.198)
(924, 3.37)
(925, 2.85)
(926, 3.081)
(927, 1.54)
(928, 5.083)
(929, 0)
(930, 0)
(931, 0)
(932, 1.54)
(933, 1.54)
(934, 0)
(935, 1.54)
(936, 0)
(937, 2.775)
(938, 1.77)
(939, 0)
(940, 0)
(941, 0)
(942, 0)
(943, 0)
(944, 0)
(945, 4.543)
(946, 2.485)
(947, 2.701)
(948, 3.08)
(949, 6.505)
(950, 2.145)
(951, 0)
(952, 0)
(953, 0)
(954, 0)
(955, 4.095)
(956, 0)
(957, 0)
(958, 1.54)
(959, 0)
(960, 0)
(961, 0)
(962, 0)
(963, 0)
(964, 0)
(965, 4.095)
(966, 0)
(967, 0)
(968, 0)
(969, 0)
(970, 0)
(971, 0)
(972, 0)
(973, 0)
(974, 0)
(975, 0)
(976, 0)
(977, 0)
(978, 0)
(979, 0)
(980, 0)
(981, 0)
(982, 0)
(983, 0)
(984, 0)
(985, 0)
(986, 0)
(987, 0)
(988, 0)
(989, 0)
(990, 0)
(991, 0)
(992, 0)
(993, 0)
(994, 0)
(995, 0)
(996, 0)
(997, 0)
(998, 0)
(999, 0)
(1000, 0)
(1001, 0)
(1002, 0)
(1003, 0)
(1004, 1.944)
(1005, 0.136)
(1006, 0)
(1007, 0)
(1008, 0)
(1009, 0)
(1010, 0)
(1011, 0)
(1012, 1.83)
(1013, 3.57)
(1014, 0)
(1015, 0)
(1016, 0)
(1017, 0)
(1018, 0)
(1019, 0)
(1020, 1.83)
(1021, 0)
(1022, 0)
(1023, 0)
(1024, 0)
(1025, 0)
(1026, 0)
(1027, 2.59)
(1028, 1.326)
(1029, 0)
(1030, 0)
(1031, 0)
(1032, 0)
(1033, 0)
(1034, 0)
(1035, 0)
(1036, 0)
(1037, 1.596)
(1038, 0)
(1039, 0)
(1040, 0)
(1041, 8.406)
(1042, 0)
(1043, 0)
(1044, 0)
(1045, 0)
(1046, 0)
(1047, 0)
(1048, 0)
(1049, 0)
(1050, 3.16)
(1051, 0)
(1052, 3.081)
(1053, 3.003)
(1054, 0)
(1055, 0)
(1056, 0)
(1057, 2.701)
(1058, 1.54)
(1059, 0)
(1060, 0)
(1061, 0)
(1062, 0)
(1063, 0)
(1064, 0)
(1065, 0)
(1066, 0)
(1067, 0)
(1068, 0)
(1069, 0)
(1070, 0)
(1071, 0)
(1072, 0)
(1073, 0)
(1074, 0)
(1075, 0)
(1076, 0)
(1077, 0)
(1078, 0)
(1079, 0)
(1080, 0)
(1081, 0)
(1082, 0)
(1083, 0)
(1084, 3.081)
(1085, 7.903)
(1086, 0)
(1087, 4.358)
(1088, 2.556)
(1089, 0)
(1090, 4.88)
(1091, 0)
(1092, 4.371)
(1093, 0)
(1094, 0)
(1095, 6.001)
(1096, 10.813)
(1097, 0.3)
(1098, 0)
(1099, 1.54)
(1100, 1.596)
(1101, 1.653)
(1102, 3.003)
(1103, 0)
(1104, 2.701)
(1105, 0)
(1106, 0)
(1107, 0)
(1108, 0)
(1109, 0)
(1110, 0)
(1111, 0)
(1112, 0)
(1113, 1.653)
(1114, 0)
(1115, 0)
(1116, 0)
(1117, 0)
(1118, 0)
(1119, 0)
(1120, 0)
(1121, 0)
(1122, 3.403)
(1123, 0)
(1124, 0)
(1125, 0)
(1126, 2.415)
(1127, 0)
(1128, 0)
(1129, 0)
(1130, 0)
(1131, 0)
(1132, 0)
(1133, 0)
(1134, 0)
(1135, 0)
(1136, 0)
(1137, 0)
(1138, 0)
(1139, 0)
(1140, 0)
(1141, 0)
(1142, 0)
(1143, 0)
(1144, 0)
(1145, 0)
(1146, 0)
(1147, 0)
(1148, 0)
(1149, 0)
(1150, 0)
(1151, 0)
(1152, 0)
(1153, 0)
(1154, 0)
(1155, 1.891)
(1156, 0)
(1157, 0)
(1158, 0)
(1159, 0)
(1160, 0)
(1161, 0)
(1162, 0)
(1163, 0)
(1164, 0)
(1165, 0)
(1166, 0)
(1167, 1.54)
(1168, 0)
(1169, 6.016)
(1170, 0)
(1171, 0)
(1172, 0)
(1173, 0)
(1174, 0)
(1175, 0)
(1176, 2.926)
(1177, 0)
(1178, 1.54)
(1179, 3.57)
(1180, 0)
(1181, 4.95)
(1182, 3.003)
(1183, 0)
(1184, 2.85)
(1185, 0)
(1186, 3.16)
(1187, 0)
(1188, 0)
(1189, 2.278)
(1190, 0)
(1191, 0)
(1192, 0)
(1193, 3.486)
(1194, 0)
(1195, 3.62)
(1196, 3.003)
(1197, 5.551)
(1198, 5.195)
(1199, 6.964)
(1200, 0)
(1201, 2.85)
(1202, 3.193)
(1203, 0)
(1204, 0)
(1205, 0)
(1206, 2.016)
(1207, 6.59)
(1208, 2.08)
(1209, 5.05)
(1210, 1.54)
(1211, 6.373)
(1212, 0)
(1213, 2.088)
(1214, 3.435)
(1215, 6.253)
(1216, 7.32)
(1217, 6.086)
(1218, 2.415)
(1219, 10.586)
(1220, 0)
(1221, 3.08)
(1222, 15.098)
(1223, 0)
(1224, 1.596)
(1225, 6.964)
(1226, 4.56)
(1227, 0)
(1228, 3.16)
(1229, 0)
(1230, 2.08)
(1231, 0)
(1232, 6.646)
(1233, 0)
(1234, 2.145)
(1235, 0)
(1236, 0)
(1237, 0)
(1238, 0)
(1239, 2.278)
(1240, 2.211)
(1241, 1.54)
(1242, 1.711)
(1243, 0)
(1244, 0)
(1245, 0)
(1246, 0)
(1247, 0)
(1248, 1.54)
(1249, 0)
(1250, 0)
(1251, 0)
(1252, 0)
(1253, 0)
(1254, 0)
(1255, 0)
(1256, 0)
(1257, 1.54)
(1258, 0)
(1259, 0)
(1260, 0)
(1261, 0)
(1262, 0)
(1263, 0)
(1264, 0)
(1265, 0)
(1266, 0)
(1267, 0)
(1268, 0)
(1269, 0)
(1270, 0)
(1271, 0)
(1272, 0)
(1273, 0)
(1274, 0)
(1275, 0)
(1276, 0)
(1277, 0)
(1278, 0)
(1279, 0)
(1280, 0)
(1281, 0)
(1282, 0)
(1283, 0)
(1284, 0)
(1285, 0)
(1286, 0)
(1287, 0)
(1288, 0)
(1289, 0)
(1290, 0)
(1291, 0)
(1292, 0)
(1293, 0)
(1294, 0)
(1295, 0)
(1296, 0)
(1297, 3.916)
(1298, 0)
(1299, 0)
(1300, 0)
(1301, 0)
(1302, 0)
(1303, 0)
(1304, 0)
(1305, 0)
(1306, 0)
(1307, 0)
(1308, 0)
(1309, 0)
(1310, 1.54)
(1311, 0)
(1312, 0)
(1313, 0)
(1314, 0)
(1315, 0)
(1316, 1.77)
(1317, 0)
(1318, 0)
(1319, 0)
(1320, 0)
(1321, 3.16)
(1322, 0)
(1323, 0)
(1324, 0)
(1325, 0)
(1326, 0)
(1327, 0)
(1328, 0)
(1329, 0)
(1330, 0)
(1331, 0)
(1332, 0)
(1333, 0)
(1334, 0)
(1335, 0)
(1336, 0)
(1337, 0)
(1338, 0)
(1339, 0)
(1340, 0)
(1341, 0)
(1342, 0)
(1343, 0)
(1344, 0)
(1345, 0)
(1346, 0)
(1347, 0)
(1348, 0)
(1349, 0)
(1350, 0)
(1351, 0)
(1352, 0)
(1353, 0)
(1354, 0)
(1355, 0)
(1356, 0)
(1357, 0)
(1358, 0)
(1359, 0)
(1360, 0)
(1361, 0)
(1362, 0)
(1363, 0)
(1364, 0)
(1365, 0)
(1366, 0)
(1367, 0)
(1368, 0)
(1369, 0)
(1370, 0)
(1371, 0)
(1372, 0)
(1373, 0)
(1374, 0)
(1375, 0)
(1376, 0)
(1377, 0)
(1378, 0)
(1379, 0)
(1380, 0)
(1381, 0)
(1382, 0)
(1383, 1.54)
(1384, 0)
(1385, 0)
(1386, 0)
(1387, 0)
(1388, 0)
(1389, 0)
(1390, 0)
(1391, 0)
(1392, 0)
(1393, 0)
(1394, 0)
(1395, 3.403)
(1396, 0)
(1397, 0)
(1398, 0)
(1399, 0)
(1400, 0)
(1401, 0)
(1402, 0)
(1403, 0)
(1404, 0)
(1405, 0)
(1406, 0)
(1407, 0)
(1408, 0)
(1409, 0)
(1410, 0)
(1411, 0)
(1412, 0)
(1413, 0)
(1414, 0)
(1415, 0)
(1416, 0)
(1417, 0)
(1418, 0)
(1419, 0)
(1420, 0)
(1421, 0)
(1422, 0)
(1423, 0)
(1424, 0)
(1425, 0)
(1426, 0)
(1427, 0)
(1428, 0)
(1429, 0)
(1430, 0)
(1431, 0)
(1432, 0)
(1433, 0)
(1434, 0)
(1435, 0)
(1436, 0)
(1437, 0)
(1438, 0)
(1439, 0)
(1440, 0)
(1441, 0)
(1442, 0)
(1443, 0)
(1444, 0)
(1445, 0)
(1446, 0)
(1447, 0)
(1448, 0)
(1449, 0)
(1450, 0)
(1451, 0)
(1452, 0)
(1453, 0)
(1454, 0)
(1455, 0)
(1456, 0)
(1457, 0)
(1458, 0)
(1459, 0)
(1460, 0)
(1461, 0)
(1462, 0)
(1463, 0)
(1464, 0)
(1465, 0)
(1466, 0)
(1467, 0)
(1468, 0)
(1469, 0)
(1470, 0)
(1471, 0)
(1472, 0)
(1473, 0)
(1474, 0)
(1475, 0)
(1476, 0)
(1477, 0)
(1478, 0)
(1479, 0)
(1480, 0)
(1481, 0)
(1482, 0)
(1483, 0)
(1484, 0)
(1485, 0)
(1486, 0)
(1487, 0)
(1488, 0)
(1489, 0)
(1490, 0)
(1491, 0)
(1492, 0)
(1493, 0)
(1494, 0)
(1495, 0)
(1496, 0)
(1497, 0)
(1498, 0)
(1499, 0)
(1500, 0)
(1501, 0)
(1502, 0)
(1503, 0)
(1504, 0)
(1505, 0)
(1506, 0)
(1507, 0)
(1508, 0)
(1509, 0)
(1510, 0)
(1511, 0)
(1512, 0)
(1513, 0)
(1514, 0)
(1515, 0)
(1516, 0)
(1517, 0)
(1518, 0)
(1519, 0)
(1520, 0)
(1521, 0)
(1522, 0)
(1523, 0)
(1524, 0)
(1525, 0)
(1526, 0)
(1527, 0)
(1528, 0)
(1529, 0)
(1530, 0)
(1531, 0)
(1532, 0)
(1533, 0)
(1534, 0)
(1535, 0)
(1536, 0)
(1537, 0)
(1538, 0)
(1539, 0)
(1540, 0)
(1541, 0)
(1542, 0)
(1543, 0)
(1544, 0)
(1545, 0)
(1546, 0)
(1547, 0)
(1548, 0)
(1549, 2.926)
(1550, 0)
(1551, 0)
(1552, 0)
(1553, 0)
(1554, 0)
(1555, 0)
(1556, 0)
(1557, 0)
(1558, 0)
(1559, 0)
(1560, 0)
(1561, 0)
(1562, 0)
(1563, 0)
(1564, 0)
(1565, 0)
(1566, 0)
(1567, 0)
(1568, 0)
(1569, 0)
(1570, 0)
(1571, 0)
(1572, 0)
(1573, 0)
(1574, 0)
(1575, 0)
(1576, 0)
(1577, 0)
(1578, 0)
(1579, 0)
(1580, 0)
(1581, 0)
(1582, 0)
(1583, 0)
(1584, 0)
(1585, 0)
(1586, 0)
(1587, 0)
(1588, 0)
(1589, 0)
(1590, 0)
(1591, 0)
(1592, 0)
(1593, 0)
(1594, 0)
(1595, 0)
(1596, 0)
(1597, 0)
(1598, 0)
(1599, 0)
(1600, 0)
(1601, 0)
(1602, 0)
(1603, 0)
(1604, 0)
(1605, 0)
(1606, 0)
(1607, 0)
(1608, 0)
(1609, 0)
(1610, 0)
(1611, 0)
(1612, 0)
(1613, 0)
(1614, 0)
(1615, 0)
(1616, 0)
(1617, 0)
(1618, 0)
(1619, 0)
(1620, 0)
(1621, 0)
(1622, 0)
(1623, 0)
(1624, 0)
(1625, 0)
(1626, 0)
(1627, 0)
(1628, 0)
(1629, 0)
(1630, 0)
(1631, 0)
(1632, 0)
(1633, 0)
(1634, 0)
(1635, 0)
(1636, 0)
(1637, 13.226)
(1638, 4.241)
(1639, 19.836)
(1640, 3.081)
(1641, 0)
(1642, 0)
(1643, 0)
(1644, 0)
(1645, 0)
(1646, 0)
(1647, 0)
(1648, 0)
(1649, 0)
(1650, 0)
(1651, 0)
(1652, 0)
(1653, 0)
(1654, 0)
(1655, 0)
(1656, 0)
(1657, 0)
(1658, 0)
(1659, 0)
(1660, 0)
(1661, 0)
(1662, 0)
(1663, 0)
(1664, 0)
(1665, 0)
(1666, 0)
(1667, 0)
(1668, 0)
(1669, 0)
(1670, 0)
(1671, 0)
(1672, 0)
(1673, 0)
(1674, 0)
(1675, 0)
(1676, 0)
(1677, 0)
(1678, 0)
(1679, 0)
(1680, 0)
(1681, 0)
(1682, 0)
(1683, 0)
(1684, 0)
(1685, 0)
(1686, 0)
(1687, 0)
(1688, 0)
(1689, 0)
(1690, 0)
(1691, 0)
(1692, 0)
(1693, 0)
(1694, 0)
(1695, 0)
(1696, 0)
(1697, 0)
(1698, 0)
(1699, 0)
(1700, 0)
(1701, 0)
(1702, 0)
(1703, 0)
(1704, 0)
(1705, 0)
(1706, 0)
(1707, 0)
(1708, 0)
(1709, 0)
(1710, 0)
(1711, 0)
(1712, 0)
(1713, 0)
(1714, 0)
(1715, 0)
(1716, 0)
(1717, 0)
(1718, 0)
(1719, 0)
(1720, 0)
(1721, 0)
(1722, 0)
(1723, 0)
(1724, 0)
(1725, 0)
(1726, 0)
(1727, 0)
(1728, 0)
(1729, 0)
(1730, 0)
(1731, 0)
(1732, 0)
(1733, 0)
(1734, 0)
(1735, 0)
(1736, 0)
(1737, 0)
(1738, 0)
(1739, 0)
(1740, 0)
(1741, 0)
(1742, 0)
(1743, 0)
(1744, 0)
(1745, 0)
(1746, 0)
(1747, 0)
(1748, 0)
(1749, 0)
(1750, 0)
(1751, 0)
(1752, 0)
(1753, 0)
(1754, 0)
(1755, 0)
(1756, 0)
(1757, 0)
(1758, 0)
(1759, 0)
(1760, 0)
(1761, 0)
(1762, 0)
(1763, 0)
(1764, 0)
(1765, 0)
(1766, 0)
(1767, 0)
(1768, 0)
(1769, 0)
(1770, 0)
(1771, 0)
(1772, 0)
(1773, 0)
(1774, 0)
(1775, 0)
(1776, 0)
(1777, 0)
(1778, 0)
(1779, 0)
(1780, 0)
(1781, 0)
(1782, 0)
(1783, 0)
(1784, 0)
(1785, 0)
(1786, 0)
(1787, 0)
(1788, 0)
(1789, 0)
(1790, 0)
(1791, 0)
(1792, 0)
(1793, 0)
(1794, 0)
(1795, 0)
(1796, 0)
(1797, 0)
(1798, 0)
(1799, 0)
(1800, 0)
(1801, 0)
(1802, 0)
(1803, 0)
(1804, 0)
(1805, 0)
(1806, 0)
(1807, 0)
(1808, 0)
(1809, 0)
(1810, 0)
(1811, 0)
(1812, 0)
(1813, 0)
(1814, 0)
(1815, 0)
(1816, 0)
(1817, 0)
(1818, 0)
(1819, 0)
(1820, 0)
(1821, 0)
(1822, 0)
(1823, 0)
(1824, 0)
(1825, 0)
(1826, 0)
(1827, 0)
(1828, 0)
(1829, 0)
(1830, 0)
(1831, 0)
(1832, 0)
(1833, 0)
(1834, 0)
(1835, 0)
(1836, 0)
(1837, 0)
(1838, 0)
(1839, 0)
(1840, 0)
(1841, 0)
(1842, 0)
(1843, 0)
(1844, 0)
(1845, 0)
(1846, 0)
(1847, 0)
(1848, 0)
(1849, 0)
(1850, 0)
(1851, 0)
(1852, 0)
(1853, 0)
(1854, 0)
(1855, 0)
(1856, 0)
(1857, 0)
(1858, 0)
(1859, 0)
(1860, 0)
(1861, 0)
(1862, 0)
(1863, 0)
(1864, 0)
(1865, 0)
(1866, 0)
(1867, 0)
(1868, 0)
(1869, 0)
(1870, 0)
(1871, 0)
(1872, 0)
(1873, 0)
(1874, 0)
(1875, 0)
(1876, 0)
(1877, 0)
(1878, 0)
(1879, 0)
(1880, 0)
(1881, 0)
(1882, 0)
(1883, 0)
(1884, 0)
(1885, 0)
(1886, 0)
(1887, 0)
(1888, 0)
(1889, 0)
(1890, 0)
(1891, 0)
(1892, 0)
(1893, 0)
(1894, 0)
(1895, 0)
(1896, 0)
(1897, 0)
(1898, 0)
(1899, 0)
(1900, 0)
(1901, 2.85)
(1902, 0)
(1903, 0)
(1904, 0)
(1905, 0)
(1906, 0)
(1907, 0)
(1908, 0)
(1909, 0)
(1910, 0)
(1911, 0)
(1912, 0)
(1913, 0)
(1914, 0)
(1915, 0)
(1916, 0)
(1917, 0)
(1918, 0)
(1919, 0)
(1920, 0)
(1921, 0)
(1922, 0)
(1923, 0)
(1924, 0)
(1925, 0)
(1926, 0)
(1927, 0)
(1928, 0)
(1929, 0)
(1930, 0)
(1931, 0)
(1932, 0)
(1933, 0)
(1934, 0)
(1935, 0)
(1936, 0)
(1937, 0)
(1938, 0)
(1939, 0)
(1940, 0)
(1941, 0)
(1942, 0)
(1943, 0)
(1944, 0)
(1945, 0)
(1946, 1.54)
(1947, 0)
(1948, 0)
(1949, 0)
(1950, 0)
(1951, 0)
(1952, 0)
(1953, 0)
(1954, 0)
(1955, 0)
(1956, 0)
(1957, 0)
(1958, 0)
(1959, 0)
(1960, 0)
(1961, 0)
(1962, 0)
(1963, 0)
(1964, 0)
(1965, 0)
(1966, 0)
(1967, 0)
(1968, 0)
(1969, 0)
(1970, 0)
(1971, 0)
(1972, 0)
(1973, 0)
(1974, 0)
(1975, 0)
(1976, 0)
(1977, 0)
(1978, 0)
(1979, 0)
(1980, 0)
(1981, 0)
(1982, 0)
(1983, 0)
(1984, 0)
(1985, 0)
(1986, 0)
(1987, 0)
(1988, 0)
(1989, 0)
(1990, 0)
(1991, 0)
(1992, 0)
(1993, 0)
(1994, 4.168)
(1995, 0)
(1996, 0)
(1997, 0)
(1998, 0)
(1999, 0)
(2000, 0)
(2001, 1.653)
(2002, 0)
(2003, 3.655)
(2004, 0)
(2005, 0)
(2006, 0)
(2007, 0)
(2008, 4.095)
(2009, 0)
(2010, 0)
(2011, 0)
(2012, 0)
(2013, 0)
(2014, 0)
(2015, 0)
(2016, 0)
(2017, 0)
(2018, 0)
(2019, 0)
(2020, 0)
(2021, 1.653)
(2022, 0)
(2023, 0)
(2024, 0)
(2025, 0)
(2026, 0)
(2027, 0)
(2028, 0)
(2029, 0)
(2030, 0)
(2031, 4.278)
(2032, 1.54)
(2033, 3.886)
(2034, 4.186)
(2035, 0)
(2036, 1.54)
(2037, 9.157)
(2038, 0.12)
(2039, 2.701)
(2040, 0)
(2041, 0)
(2042, 0)
(2043, 0)
(2044, 0)
(2045, 0)
(2046, 0)
(2047, 3.24)
(2048, 5.742)
(2049, 0.001)
(2050, 4.005)
(2051, 0)
(2052, 6.243)
(2053, 5.545)
(2054, 0.476)
(2055, 6.196)
(2056, 1.54)
(2057, 5.522)
(2058, 2.09)
(2059, 4.476)
(2060, 2.346)
(2061, 0)
(2062, 0.792)
(2063, 2.211)
(2064, 0)
(2065, 0)
(2066, 0)
(2067, 0)
(2068, 0)
(2069, 3.003)
(2070, 0)
(2071, 0)
(2072, 0)
(2073, 0)
(2074, 0)
(2075, 0)
(2076, 7.473)
(2077, 0)
(2078, 2.556)
(2079, 4.186)
(2080, 0)
(2081, 4.656)
(2082, 0)
(2083, 0)
(2084, 1.54)
(2085, 0)
(2086, 2.701)
(2087, 0)
(2088, 0)
(2089, 0)
(2090, 0)
(2091, 0)
(2092, 0)
(2093, 0)
(2094, 0)
(2095, 0)
(2096, 0)
(2097, 3.003)
(2098, 1.54)
(2099, 1.54)
(2100, 0)
(2101, 2.211)
(2102, 0)
(2103, 0)
(2104, 0)
(2105, 5.856)
(2106, 0)
(2107, 2.485)
(2108, 0)
(2109, 0)
(2110, 0)
(2111, 0)
(2112, 0)
(2113, 0)
(2114, 0)
(2115, 0)
(2116, 0)
(2117, 0)
(2118, 0)
(2119, 0)
(2120, 0)
(2121, 0)
(2122, 0)
(2123, 0)
(2124, 0)
(2125, 0)
(2126, 0)
(2127, 0)
(2128, 0)
(2129, 0)
(2130, 1.596)
(2131, 0)
(2132, 0)
(2133, 0)
(2134, 0)
(2135, 0)
(2136, 0)
(2137, 0)
(2138, 0)
(2139, 0)
(2140, 0)
(2141, 0)
(2142, 0)
(2143, 0)
(2144, 0)
(2145, 0)
(2146, 0)
(2147, 0)
(2148, 0)
(2149, 0)
(2150, 0)
(2151, 0)
(2152, 0)
(2153, 0)
(2154, 0)
(2155, 0)
(2156, 0)
(2157, 0)
(2158, 0)
(2159, 0)
(2160, 0)
(2161, 0)
(2162, 0)
(2163, 0)
(2164, 0)
(2165, 0)
(2166, 3.486)
(2167, 0)
(2168, 0)
(2169, 0)
(2170, 0)
(2171, 0)
(2172, 0)
(2173, 0)
(2174, 0)
(2175, 0)
(2176, 0)
(2177, 0)
(2178, 0)
(2179, 0)
(2180, 0)
(2181, 0)
(2182, 0)
(2183, 0)
(2184, 0)
(2185, 0)
(2186, 0)
(2187, 0)
(2188, 0)
(2189, 0)
(2190, 4.851)
(2191, 0)
(2192, 0)
(2193, 0)
(2194, 0)
(2195, 0)
(2196, 0)
(2197, 0)
(2198, 0)
(2199, 0)
(2200, 0)
(2201, 0)
(2202, 3.003)
(2203, 0)
(2204, 0)
(2205, 0)
(2206, 0)
(2207, 0)
(2208, 0)
(2209, 0)
(2210, 0)
(2211, 2.145)
(2212, 0)
(2213, 0)
(2214, 0)
(2215, 0)
(2216, 0)
(2217, 0)
(2218, 0)
(2219, 0)
(2220, 0)
(2221, 0)
(2222, 0)
(2223, 0)
(2224, 0)
(2225, 0)
(2226, 0)
(2227, 0)
(2228, 0)
(2229, 0)
(2230, 0)
(2231, 0)
(2232, 1.276)
(2233, 0.435)
(2234, 0)
(2235, 0)
(2236, 0)
(2237, 0)
(2238, 0)
(2239, 0)
(2240, 0)
(2241, 0)
(2242, 0)
(2243, 0)
(2244, 0)
(2245, 0)
(2246, 0)
(2247, 2.346)
(2248, 0)
(2249, 0)
(2250, 0)
(2251, 2.08)
(2252, 3.16)
(2253, 0)
(2254, 1.552)
(2255, 0.528)
(2256, 0)
(2257, 0)
(2258, 0)
(2259, 0)
(2260, 0)
(2261, 0)
(2262, 1.54)
(2263, 0)
(2264, 0)
(2265, 0)
(2266, 0)
(2267, 1.54)
(2268, 0)
(2269, 2.926)
(2270, 0)
(2271, 0)
(2272, 0)
(2273, 0)
(2274, 0)
(2275, 4.912)
(2276, 0)
(2277, 1.54)
(2278, 0)
(2279, 0)
(2280, 0)
(2281, 0)
(2282, 0)
(2283, 0)
(2284, 0)
(2285, 0)
(2286, 6.574)
(2287, 3.009)
(2288, 3.003)
(2289, 2.926)
(2290, 0)
(2291, 0)
(2292, 0)
(2293, 0)
(2294, 0)
(2295, 0)
(2296, 0)
(2297, 0)
(2298, 0)
(2299, 0)
(2300, 0)
(2301, 0)
(2302, 0)
(2303, 0)
(2304, 0)
(2305, 0)
(2306, 0)
(2307, 0)
(2308, 0)
(2309, 0)
(2310, 0)
(2311, 0)
(2312, 0)
(2313, 0)
(2314, 2.628)
(2315, 0)
(2316, 0)
(2317, 0)
(2318, 3.081)
(2319, 0)
(2320, 0)
(2321, 0)
(2322, 0)
(2323, 0)
(2324, 0)
(2325, 0)
(2326, 1.54)
(2327, 0)
(2328, 0)
(2329, 0)
(2330, 0)
(2331, 0)
(2332, 0)
(2333, 5.257)
(2334, 0)
(2335, 0)
(2336, 0)
(2337, 0)
(2338, 2.08)
(2339, 2.415)
(2340, 0)
(2341, 0)
(2342, 4.278)
(2343, 0)
(2344, 0)
(2345, 4.753)
(2346, 1.54)
(2347, 0)
(2348, 0)
(2349, 0)
(2350, 0)
(2351, 1.54)
(2352, 0)
(2353, 2.86)
(2354, 0.066)
(2355, 3.003)
(2356, 0)
(2357, 0)
(2358, 0)
(2359, 0)
(2360, 5.05)
(2361, 0)
(2362, 0)
(2363, 0)
(2364, 0)
(2365, 0)
(2366, 3.57)
(2367, 0)
(2368, 0)
(2369, 1.891)
(2370, 5.05)
(2371, 0)
(2372, 0)
(2373, 0)
(2374, 0)
(2375, 0)
(2376, 1.953)
(2377, 0)
(2378, 0)
(2379, 0)
(2380, 0)
(2381, 0)
(2382, 0)
(2383, 0)
(2384, 4.465)
(2385, 6.228)
(2386, 2.278)
(2387, 1.54)
(2388, 0)
(2389, 0)
(2390, 0)
(2391, 0)
(2392, 2.926)
(2393, 5.55)
(2394, 0)
(2395, 0)
(2396, 0)
(2397, 0)
(2398, 0)
(2399, 0)
(2400, 0)
(2401, 0)
(2402, 5.559)
(2403, 0)
(2404, 0)
(2405, 0.3)
(2406, 5.578)
(2407, 0.465)
(2408, 0)
(2409, 0)
(2410, 0)
(2411, 0)
(2412, 0)
(2413, 0)
(2414, 0)
(2415, 2.211)
(2416, 0)
(2417, 0)
(2418, 0)
(2419, 0)
(2420, 0)
(2421, 0)
(2422, 0)
(2423, 0)
(2424, 0)
(2425, 0)
(2426, 0)
(2427, 0)
(2428, 0)
(2429, 2.346)
(2430, 0)
(2431, 0)
(2432, 0)
(2433, 0)
(2434, 0)
(2435, 1.54)
(2436, 0)
(2437, 0)
(2438, 0)
(2439, 0)
(2440, 3.486)
(2441, 0)
(2442, 0)
(2443, 0)
(2444, 0)
(2445, 0)
(2446, 0)
(2447, 1.54)
(2448, 0)
(2449, 0)
(2450, 0)
(2451, 4.56)
(2452, 3.24)
(2453, 0)
(2454, 0)
(2455, 0)
(2456, 0)
(2457, 0)
(2458, 0)
(2459, 1.54)
(2460, 3.16)
(2461, 3.655)
(2462, 2.556)
(2463, 0)
(2464, 0)
(2465, 3.486)
(2466, 1.77)
(2467, 5.05)
(2468, 9.703)
(2469, 8.408)
(2470, 5.033)
(2471, 0.82)
(2472, 1.596)
(2473, 2.211)
(2474, 0)
(2475, 2.85)
(2476, 1.54)
(2477, 5.776)
(2478, 1.653)
(2479, 9.805)
(2480, 10.245)
(2481, 19.045)
(2482, 10.492)
(2483, 6.526)
(2484, 4.186)
(2485, 9.335)
(2486, 14.451)
(2487, 7.079)
(2488, 3.62)
(2489, 6.084)
(2490, 0)
(2491, 8.142)
(2492, 4.543)
(2493, 3.741)
(2494, 0)
(2495, 4.084)
(2496, 1.378)
(2497, 0)
(2498, 0)
(2499, 3.081)
(2500, 0)
(2501, 0)
(2502, 0)
(2503, 0)
(2504, 0)
(2505, 0)
(2506, 2.278)
(2507, 4.56)
(2508, 0)
(2509, 0)
(2510, 3.003)
(2511, 0)
(2512, 3.486)
(2513, 3.081)
(2514, 1.891)
(2515, 0)
(2516, 1.54)
(2517, 0)
(2518, 0)
(2519, 0)
(2520, 0)
(2521, 1.77)
(2522, 0)
(2523, 0)
(2524, 0)
(2525, 0)
(2526, 0)
(2527, 3.861)
(2528, 1.595)
(2529, 3.486)
(2530, 3.321)
(2531, 0)
(2532, 0)
(2533, 0)
(2534, 1.54)
(2535, 0)
(2536, 0)
(2537, 0)
(2538, 0)
(2539, 0)
(2540, 0)
(2541, 1.54)
(2542, 1.77)
(2543, 0)
(2544, 0)
(2545, 1.54)
(2546, 0)
(2547, 2.278)
(2548, 0)
(2549, 0)
(2550, 0)
(2551, 2.278)
(2552, 0)
(2553, 1.953)
(2554, 0)
(2555, 0)
(2556, 3.62)
(2557, 0)
(2558, 0)
(2559, 0)
(2560, 4.465)
(2561, 4.095)
(2562, 0)
(2563, 0)
(2564, 0)
(2565, 10.487)
(2566, 0)
(2567, 0)
(2568, 0)
(2569, 2.769)
(2570, 0.006)
(2571, 0)
(2572, 2.08)
(2573, 1.54)
(2574, 0)
(2575, 0)
(2576, 0)
(2577, 0)
(2578, 0)
(2579, 0)
(2580, 0)
(2581, 0)
(2582, 0)
(2583, 1.83)
(2584, 0)
(2585, 0)
(2586, 0)
(2587, 2.145)
(2588, 0)
(2589, 0)
(2590, 0)
(2591, 0)
(2592, 0)
(2593, 6.59)
(2594, 1.54)
(2595, 0)
(2596, 4.315)
(2597, 0)
(2598, 0)
(2599, 3.971)
(2600, 2.278)
(2601, 0)
(2602, 2.016)
(2603, 4.428)
(2604, 0)
(2605, 0)
(2606, 0)
(2607, 0)
(2608, 0)
(2609, 1.77)
(2610, 4.422)
(2611, 6.166)
(2612, 0)
(2613, 0)
(2614, 1.474)
(2615, 0.066)
(2616, 0)
(2617, 2.926)
(2618, 2.278)
(2619, 0)
(2620, 0)
(2621, 4.278)
(2622, 0)
(2623, 1.54)
(2624, 0)
(2625, 3.382)
(2626, 1.326)
(2627, 13.49)
(2628, 2.926)
(2629, 5.13)
(2630, 0)
(2631, 2.628)
(2632, 0)
(2633, 3.31)
(2634, 0)
(2635, 0)
(2636, 0)
(2637, 7.067)
(2638, 2.485)
(2639, 0)
(2640, 4.656)
(2641, 0)
(2642, 2.08)
(2643, 0)
(2644, 0)
(2645, 1.54)
(2646, 0)
(2647, 0)
(2648, 0)
(2649, 4.402)
(2650, 4.39)
(2651, 0)
(2652, 4.543)
(2653, 0)
(2654, 1.653)
(2655, 0)
(2656, 0)
(2657, 0)
(2658, 4.309)
(2659, 0.741)
(2660, 1.891)
(2661, 3.16)
(2662, 0)
(2663, 0)
(2664, 0)
(2665, 3.08)
(2666, 2.346)
(2667, 0)
(2668, 3.57)
(2669, 0)
(2670, 4.186)
(2671, 0)
(2672, 1.953)
(2673, 0)
(2674, 1.54)
(2675, 0)
(2676, 1.111)
(2677, 2.32)
(2678, 0)
(2679, 2.08)
(2680, 2.775)
(2681, 0)
(2682, 0)
(2683, 0)
(2684, 1.54)
(2685, 0)
(2686, 0)
(2687, 2.628)
(2688, 2.278)
(2689, 0)
(2690, 0)
(2691, 0)
(2692, 0)
(2693, 0)
(2694, 0)
(2695, 0)
(2696, 0)
(2697, 2.85)
(2698, 6.084)
(2699, 0)
(2700, 0)
(2701, 1.711)
(2702, 0)
(2703, 0)
(2704, 1.54)
(2705, 7.871)
(2706, 1.653)
(2707, 0)
(2708, 0)
(2709, 0)
(2710, 0)
(2711, 2.08)
(2712, 1.54)
(2713, 6.772)
(2714, 8.434)
(2715, 0)
(2716, 0)
(2717, 3.403)
(2718, 6.646)
(2719, 0)
(2720, 4.95)
(2721, 9.531)
(2722, 7.96)
(2723, 3.003)
(2724, 0)
(2725, 0)
(2726, 1.54)
(2727, 10.561)
(2728, 1.54)
(2729, 0)
(2730, 2.346)
(2731, 1.891)
(2732, 5.05)
(2733, 0)
(2734, 0)
(2735, 0)
(2736, 0)
(2737, 3.003)
(2738, 0)
(2739, 2.926)
(2740, 0)
(2741, 3.08)
(2742, 6.019)
(2743, 0)
(2744, 0)
(2745, 0)
(2746, 0)
(2747, 0)
(2748, 0)
(2749, 0)
(2750, 0)
(2751, 0)
(2752, 2.145)
(2753, 4.466)
(2754, 3.081)
(2755, 10.387)
(2756, 4.371)
(2757, 5.05)
(2758, 0)
(2759, 2.278)
(2760, 6.716)
(2761, 6.358)
(2762, 3.31)
(2763, 0)
(2764, 3.655)
(2765, 1.596)
(2766, 3.431)
(2767, 4.7)
(2768, 0)
(2769, 3.16)
(2770, 3.818)
(2771, 4.753)
(2772, 14.365)
(2773, 1.54)
(2774, 4.7)
(2775, 0)
(2776, 0)
(2777, 0)
(2778, 1.54)
(2779, 0)
(2780, 5.368)
(2781, 3.62)
(2782, 3.08)
(2783, 0)
(2784, 0)
(2785, 2.346)
(2786, 0)
(2787, 0)
(2788, 0)
(2789, 0)
(2790, 0)
(2791, 0)
(2792, 0)
(2793, 0)
(2794, 0)
(2795, 1.54)
(2796, 0)
(2797, 0)
(2798, 0)
(2799, 0)
(2800, 0)
(2801, 0)
(2802, 0)
(2803, 0)
(2804, 0)
(2805, 0)
(2806, 0)
(2807, 0)
(2808, 0)
(2809, 0)
(2810, 0)
(2811, 0)
(2812, 2.556)
(2813, 0)
(2814, 0)
(2815, 0)
(2816, 0)
(2817, 0)
(2818, 0)
(2819, 0)
(2820, 0)
(2821, 0)
(2822, 0)
(2823, 1.711)
(2824, 0)
(2825, 0)
(2826, 0)
(2827, 0)
(2828, 0)
(2829, 0)
(2830, 0)
(2831, 0)
(2832, 0)
(2833, 0)
(2834, 0)
(2835, 0)
(2836, 0)
(2837, 0)
(2838, 0)
(2839, 0)
(2840, 0)
(2841, 0)
(2842, 0)
(2843, 0)
(2844, 0)
(2845, 0)
(2846, 0)
(2847, 0)
(2848, 0)
(2849, 0)
(2850, 0)
(2851, 0)
(2852, 0)
(2853, 0)
(2854, 0)
(2855, 0)
(2856, 0)
(2857, 0)
(2858, 0)
(2859, 0)
(2860, 0)
(2861, 2.139)
(2862, 1.431)
(2863, 0)
(2864, 0)
(2865, 0)
(2866, 0)
(2867, 0)
(2868, 0)
(2869, 0)
(2870, 0)
(2871, 0)
(2872, 0)
(2873, 2.85)
(2874, 0)
(2875, 0)
(2876, 0)
(2877, 0)
(2878, 1.54)
(2879, 0)
(2880, 0)
(2881, 0)
(2882, 0)
(2883, 0)
(2884, 0)
(2885, 2.775)
(2886, 0)
(2887, 0)
(2888, 0)
(2889, 0)
(2890, 0)
(2891, 0)
(2892, 0)
(2893, 0)
(2894, 0)
(2895, 0)
(2896, 0)
(2897, 0)
(2898, 0)
(2899, 0)
(2900, 0)
(2901, 0)
(2902, 0)
(2903, 0)
(2904, 0)
(2905, 0)
(2906, 0)
(2907, 0)
(2908, 0)
(2909, 0)
(2910, 1.54)
(2911, 0)
(2912, 0)
(2913, 0)
(2914, 0)
(2915, 0)
(2916, 0)
(2917, 0)
(2918, 0)
(2919, 1.54)
(2920, 0)
(2921, 0)
(2922, 0)
(2923, 0)
(2924, 0)
(2925, 0)
(2926, 0)
(2927, 2.211)
(2928, 0)
(2929, 0)
(2930, 0)
(2931, 4.78)
(2932, 0)
(2933, 0)
(2934, 0)
(2935, 0)
(2936, 0)
(2937, 0)
(2938, 0)
(2939, 2.926)
(2940, 0)
(2941, 0)
(2942, 0)
(2943, 0)
(2944, 0)
(2945, 1.891)
(2946, 2.08)
(2947, 0)
(2948, 0)
(2949, 1.653)
(2950, 0)
(2951, 0)
(2952, 3.112)
(2953, 0)
(2954, 0)
(2955, 4.56)
(2956, 2.08)
(2957, 0)
(2958, 0)
(2959, 0)
(2960, 1.54)
(2961, 0)
(2962, 0)
(2963, 0)
(2964, 0)
(2965, 0)
(2966, 1.54)
(2967, 0)
(2968, 3.003)
(2969, 5.11)
(2970, 2.08)
(2971, 0)
(2972, 0)
(2973, 0)
(2974, 1.54)
(2975, 4.531)
(2976, 2.926)
(2977, 0)
(2978, 2.145)
(2979, 0)
(2980, 0)
(2981, 2.211)
(2982, 2.85)
(2983, 0)
(2984, 4.7)
(2985, 4.465)
(2986, 10.049)
(2987, 2.54)
(2988, 7.543)
(2989, 16.254)
(2990, 2.256)
(2991, 5.32)
(2992, 7.665)
(2993, 7.8)
(2994, 0)
(2995, 2.775)
(2996, 10.874)
(2997, 1.045)
(2998, 4.005)
(2999, 2.016)
(3000, 1.534)
(3001, 4.473)
(3002, 0)
(3003, 5.05)
(3004, 5.944)
(3005, 1.54)
(3006, 1.891)
(3007, 3.003)
(3008, 6.623)
(3009, 0)
(3010, 2.346)
(3011, 0)
(3012, 2.628)
(3013, 4.241)
(3014, 0)
(3015, 0)
(3016, 4.095)
(3017, 2.145)
(3018, 1.54)
(3019, 0)
(3020, 0)
(3021, 3.003)
(3022, 0)
(3023, 8.266)
(3024, 7.933)
(3025, 5.977)
(3026, 0)
(3027, 2.278)
(3028, 0)
(3029, 0)
(3030, 0)
(3031, 0)
(3032, 2.278)
(3033, 0)
(3034, 1.596)
(3035, 0)
(3036, 4.753)
(3037, 5.214)
(3038, 2.016)
(3039, 0)
(3040, 1.54)
(3041, 0)
(3042, 0)
(3043, 1.8)
(3044, 0.153)
(3045, 2.415)
(3046, 0)
(3047, 0)
(3048, 0)
(3049, 0)
(3050, 0)
(3051, 0)
(3052, 0)
(3053, 1.54)
(3054, 0)
(3055, 0)
(3056, 0.35)
(3057, 2.278)
(3058, 0)
(3059, 0)
(3060, 0)
(3061, 0)
(3062, 0)
(3063, 0)
(3064, 0)
(3065, 0)
(3066, 0)
(3067, 4.186)
(3068, 2.485)
(3069, 0)
(3070, 2.628)
(3071, 1.54)
(3072, 3.828)
(3073, 0)
(3074, 0)
(3075, 2.628)
(3076, 0)
(3077, 0)
(3078, 0)
(3079, 0)
(3080, 0)
(3081, 0)
(3082, 0)
(3083, 4.098)
(3084, 3.081)
(3085, 2.85)
(3086, 0)
(3087, 0)
(3088, 0)
(3089, 0)
(3090, 2.346)
(3091, 0)
(3092, 0)
(3093, 0)
(3094, 0)
(3095, 2.08)
(3096, 0)
(3097, 1.54)
(3098, 0)
(3099, 2.701)
(3100, 0)
(3101, 2.211)
(3102, 0)
(3103, 0)
(3104, 0)
(3105, 0)
(3106, 0)
(3107, 0)
(3108, 0)
(3109, 0)
(3110, 0)
(3111, 3.081)
(3112, 0)
(3113, 6.086)
(3114, 1.54)
(3115, 2.08)
(3116, 0)
(3117, 4.005)
(3118, 4.644)
(3119, 2.346)
(3120, 0)
(3121, 0)
(3122, 0)
(3123, 0)
(3124, 0)
(3125, 0)
(3126, 0)
(3127, 0)
(3128, 0)
(3129, 0)
(3130, 0)
(3131, 4.059)
(3132, 0.561)
(3133, 0)
(3134, 5.545)
(3135, 0)
(3136, 0)
(3137, 0)
(3138, 0)
(3139, 3.655)
(3140, 0)
(3141, 0)
(3142, 0)
(3143, 0)
(3144, 3.655)
(3145, 0)
(3146, 0)
(3147, 0)
(3148, 2.926)
(3149, 0)
(3150, 0)
(3151, 0)
(3152, 0)
(3153, 0)
(3154, 0)
(3155, 0)
(3156, 0)
(3157, 0)
(3158, 0)
(3159, 1.653)
(3160, 0)
(3161, 0)
(3162, 0)
(3163, 0)
(3164, 0)
(3165, 0)
(3166, 0)
(3167, 2.016)
(3168, 0)
(3169, 0)
(3170, 0)
(3171, 0)
(3172, 0)
(3173, 0)
(3174, 0)
(3175, 0)
(3176, 1.54)
(3177, 0)
(3178, 0)
(3179, 0)
(3180, 0)
(3181, 0)
(3182, 0)
(3183, 0)
(3184, 0)
(3185, 0)
(3186, 0)
(3187, 4.753)
(3188, 4.95)
(3189, 3.136)
(3190, 0)
(3191, 0)
(3192, 0)
(3193, 0)
(3194, 0)
(3195, 0)
(3196, 0)
(3197, 0)
(3198, 0)
(3199, 0)
(3200, 0)
(3201, 0)
(3202, 0)
(3203, 0)
(3204, 0)
(3205, 0)
(3206, 0)
(3207, 0)
(3208, 0)
(3209, 0)
(3210, 0)
(3211, 2.775)
(3212, 0)
(3213, 0)
(3214, 0)
(3215, 0)
(3216, 0)
(3217, 0)
(3218, 0)
(3219, 0)
(3220, 0)
(3221, 0)
(3222, 0)
(3223, 0)
(3224, 0)
(3225, 0)
(3226, 0)
(3227, 0)
(3228, 0)
(3229, 0)
(3230, 0)
(3231, 0)
(3232, 0)
(3233, 0)
(3234, 0)
(3235, 0)
(3236, 0)
(3237, 0)
(3238, 0)
(3239, 0)
(3240, 0)
(3241, 0)
(3242, 0)
(3243, 0)
(3244, 0)
(3245, 3.003)
(3246, 0)
(3247, 0)
(3248, 0)
(3249, 1.54)
(3250, 0)
(3251, 0)
(3252, 0)
(3253, 1.14)
(3254, 0.63)
(3255, 0)
(3256, 0)
(3257, 0)
(3258, 0)
(3259, 0)
(3260, 0)
(3261, 0)
(3262, 0)
(3263, 0)
(3264, 0)
(3265, 0)
(3266, 0)
(3267, 0)
(3268, 0)
(3269, 0)
(3270, 0)
(3271, 0)
(3272, 0)
(3273, 0)
(3274, 0)
(3275, 0)
(3276, 0)
(3277, 0)
(3278, 0)
(3279, 0)
(3280, 0)
(3281, 0)
(3282, 2.701)
(3283, 0)
(3284, 0)
(3285, 0)
(3286, 0)
(3287, 0)
(3288, 0)
(3289, 0)
(3290, 0)
(3291, 0)
(3292, 0)
(3293, 0)
(3294, 0)
(3295, 0)
(3296, 0)
(3297, 0)
(3298, 0)
(3299, 3.321)
(3300, 0)
(3301, 0)
(3302, 0)
(3303, 0)
(3304, 0)
(3305, 0)
(3306, 4.906)
(3307, 0)
(3308, 0)
(3309, 0)
(3310, 4.278)
(3311, 0)
(3312, 0)
(3313, 4.005)
(3314, 0)
(3315, 0)
(3316, 0)
(3317, 0)
(3318, 0)
(3319, 0)
(3320, 0)
(3321, 0)
(3322, 0)
(3323, 0)
(3324, 0)
(3325, 0)
(3326, 1.83)
(3327, 0)
(3328, 0)
(3329, 0)
(3330, 0)
(3331, 0)
(3332, 0)
(3333, 0)
(3334, 0)
(3335, 0)
(3336, 0)
(3337, 0)
(3338, 0)
(3339, 0)
(3340, 0)
(3341, 3.655)
(3342, 0)
(3343, 0)
(3344, 3.24)
(3345, 0)
(3346, 0)
(3347, 2.145)
(3348, 0)
(3349, 3.16)
(3350, 0)
(3351, 0)
(3352, 0)
(3353, 0)
(3354, 0)
(3355, 0)
(3356, 0)
(3357, 0)
(3358, 0)
(3359, 2.85)
(3360, 2.628)
(3361, 0)
(3362, 0)
(3363, 0)
(3364, 0)
(3365, 2.926)
(3366, 2.211)
(3367, 1.953)
(3368, 0)
(3369, 0)
(3370, 0)
(3371, 0)
(3372, 0)
(3373, 2.016)
(3374, 0)
(3375, 0)
(3376, 1.54)
(3377, 3.24)
(3378, 0)
(3379, 0)
(3380, 0)
(3381, 3.24)
(3382, 0.21)
(3383, 2.346)
(3384, 0)
(3385, 0)
(3386, 0)
(3387, 0)
(3388, 0)
(3389, 0)
(3390, 0)
(3391, 0)
(3392, 0)
(3393, 0)
(3394, 0)
(3395, 0)
(3396, 1.54)
(3397, 0)
(3398, 0)
(3399, 1.83)
(3400, 0)
(3401, 0)
(3402, 0)
(3403, 0)
(3404, 0)
(3405, 0)
(3406, 1.54)
(3407, 0)
(3408, 0)
(3409, 0)
(3410, 0)
(3411, 0)
(3412, 0)
(3413, 2.701)
(3414, 5.898)
(3415, 0)
(3416, 0)
(3417, 0)
(3418, 6.909)
(3419, 3.003)
(3420, 4.095)
(3421, 5.368)
(3422, 1.891)
(3423, 0)
(3424, 0)
(3425, 2.775)
(3426, 0)
(3427, 1.953)
(3428, 0)
(3429, 0)
(3430, 5.05)
(3431, 0)
(3432, 0)
(3433, 0)
(3434, 2.85)
(3435, 4.56)
(3436, 0)
(3437, 4.371)
(3438, 1.596)
(3439, 2.145)
(3440, 2.926)
(3441, 2.701)
(3442, 2.628)
(3443, 2.024)
(3444, 3.136)
(3445, 3.31)
(3446, 0)
(3447, 0)
(3448, 0)
(3449, 0)
(3450, 0)
(3451, 1.711)
(3452, 0)
(3453, 0)
(3454, 0)
(3455, 3.321)
(3456, 0)
(3457, 0)
(3458, 0)
(3459, 0)
(3460, 0)
(3461, 0)
(3462, 0)
(3463, 0)
(3464, 0)
(3465, 0.5)
(3466, 4.714)
(3467, 0)
(3468, 0)
(3469, 0)
(3470, 0)
(3471, 0)
(3472, 5.05)
(3473, 0)
(3474, 4.467)
(3475, 0.028)
(3476, 0)
(3477, 0)
(3478, 0)
(3479, 0)
(3480, 0)
(3481, 0)
(3482, 0)
(3483, 0)
(3484, 0)
(3485, 0)
(3486, 0)
(3487, 0)
(3488, 0)
(3489, 0)
(3490, 0)
(3491, 0)
(3492, 0)
(3493, 0)
(3494, 0)
(3495, 0)
(3496, 0)
(3497, 0)
(3498, 0)
(3499, 0)
(3500, 0)
(3501, 0)
(3502, 2.145)
(3503, 4.89)
(3504, 0.105)
(3505, 0)
(3506, 0)
(3507, 0)
(3508, 0)
(3509, 0)
(3510, 0)
(3511, 0)
(3512, 1.54)
(3513, 0)
(3514, 0)
(3515, 0)
(3516, 0)
(3517, 0)
(3518, 0)
(3519, 0)
(3520, 0)
(3521, 0)
(3522, 0)
(3523, 0)
(3524, 0)
(3525, 0)
(3526, 0)
(3527, 0)
(3528, 0)
(3529, 0)
(3530, 0)
(3531, 0)
(3532, 0)
(3533, 0)
(3534, 0)
(3535, 0)
(3536, 0)
(3537, 0)
(3538, 0)
(3539, 0)
(3540, 0)
(3541, 0)
(3542, 0)
(3543, 0)
(3544, 0)
(3545, 0)
(3546, 0)
(3547, 0)
(3548, 0)
(3549, 0)
(3550, 0)
(3551, 0)
(3552, 0)
(3553, 0)
(3554, 0)
(3555, 0)
(3556, 0)
(3557, 0)
(3558, 0)
(3559, 0)
(3560, 0)
(3561, 0)
(3562, 0)
(3563, 0)
(3564, 0)
(3565, 0)
(3566, 0)
(3567, 0)
(3568, 0)
(3569, 0)
(3570, 0)
(3571, 0)
(3572, 0)
(3573, 0)
(3574, 0)
(3575, 0)
(3576, 0)
(3577, 0)
(3578, 0)
(3579, 0)
(3580, 0)
(3581, 0)
(3582, 0)
(3583, 0)
(3584, 0)
(3585, 0)
(3586, 0)
(3587, 0)
(3588, 0)
(3589, 0)
(3590, 0)
(3591, 0)
(3592, 0)
(3593, 0)
(3594, 0)
(3595, 0)
(3596, 0)
(3597, 0)
(3598, 0)
(3599, 0)
(3600, 0)
(3601, 0)
(3602, 0)
(3603, 0)
(3604, 0)
(3605, 0)
(3606, 0)
(3607, 0)
(3608, 0)
(3609, 0)
(3610, 0)
(3611, 0)
(3612, 0)
(3613, 0)
(3614, 0)
(3615, 0)
(3616, 0)
(3617, 0)
(3618, 0)
(3619, 0)
(3620, 0)
(3621, 0)
(3622, 0)
(3623, 1.54)
(3624, 0)
(3625, 0)
(3626, 0)
(3627, 0)
(3628, 0)
(3629, 0)
(3630, 0)
(3631, 0)
(3632, 0)
(3633, 0)
(3634, 0)
(3635, 0)
(3636, 0)
(3637, 0)
(3638, 0)
(3639, 0)
(3640, 2.701)
(3641, 1.83)
(3642, 0)
(3643, 0)
(3644, 0)
(3645, 0)
(3646, 0)
(3647, 0)
(3648, 0)
(3649, 0)
(3650, 0)
(3651, 0)
(3652, 0)
(3653, 0)
(3654, 3.619)
(3655, 5.001)
(3656, 0)
(3657, 0)
(3658, 0)
(3659, 0)
(3660, 0)
(3661, 0)
(3662, 0)
(3663, 0)
(3664, 0)
(3665, 0)
(3666, 0)
(3667, 0)
(3668, 0)
(3669, 0)
(3670, 0)
(3671, 0)
(3672, 0)
(3673, 3.486)
(3674, 3.751)
(3675, 0)
(3676, 0)
(3677, 0)
(3678, 0)
(3679, 0)
(3680, 0)
(3681, 0)
(3682, 0)
(3683, 0)
(3684, 0)
(3685, 2.775)
(3686, 0)
(3687, 0)
(3688, 0)
(3689, 0)
(3690, 0)
(3691, 0)
(3692, 0)
(3693, 0)
(3694, 0)
(3695, 0)
(3696, 0)
(3697, 0)
(3698, 0)
(3699, 0)
(3700, 0)
(3701, 0)
(3702, 0)
(3703, 0)
(3704, 0)
(3705, 0)
(3706, 0)
(3707, 0)
(3708, 0)
(3709, 0)
(3710, 0)
(3711, 0)
(3712, 0)
(3713, 0)
(3714, 0)
(3715, 0)
(3716, 0)
(3717, 0)
(3718, 0)
(3719, 0)
(3720, 2.145)
(3721, 0)
(3722, 0)
(3723, 0)
(3724, 0)
(3725, 0)
(3726, 0)
(3727, 0)
(3728, 0)
(3729, 0)
(3730, 0)
(3731, 0)
(3732, 0)
(3733, 0)
(3734, 0)
(3735, 0)
(3736, 0)
(3737, 0)
(3738, 0)
(3739, 0)
(3740, 0)
(3741, 0)
(3742, 0)
(3743, 0)
(3744, 0)
(3745, 0)
(3746, 0)
(3747, 0)
(3748, 0)
(3749, 0)
(3750, 0)
(3751, 0)
(3752, 0)
(3753, 0)
(3754, 0)
(3755, 0)
(3756, 0)
(3757, 0)
(3758, 0)
(3759, 0)
(3760, 0)
(3761, 0)
(3762, 0)
(3763, 0)
(3764, 0)
(3765, 0)
(3766, 1.54)
(3767, 1.891)
(3768, 0)
(3769, 0)
(3770, 0)
(3771, 0)
(3772, 0)
(3773, 0)
(3774, 0)
(3775, 1.54)
(3776, 0)
(3777, 0)
(3778, 0)
(3779, 0)
(3780, 0)
(3781, 0)
(3782, 1.54)
(3783, 0)
(3784, 0)
(3785, 0)
(3786, 0)
(3787, 0)
(3788, 2.415)
(3789, 0)
(3790, 1.54)
(3791, 0)
(3792, 0)
(3793, 0)
(3794, 3.151)
(3795, 3.94)
(3796, 2.145)
(3797, 4.186)
(3798, 9.477)
(3799, 0)
(3800, 5.05)
(3801, 0)
(3802, 4.851)
(3803, 0)
(3804, 2.775)
(3805, 0)
(3806, 0)
(3807, 0)
(3808, 0)
(3809, 0)
(3810, 0)
(3811, 0)
(3812, 5.939)
(3813, 0)
(3814, 0)
(3815, 0)
(3816, 0)
(3817, 2.448)
(3818, 0.253)
(3819, 0)
(3820, 0)
(3821, 0)
(3822, 0)
(3823, 0)
(3824, 0)
(3825, 0)
(3826, 0)
(3827, 0)
(3828, 0)
(3829, 0)
(3830, 0)
(3831, 0)
(3832, 0)
(3833, 3.24)
(3834, 0)
(3835, 0)
(3836, 0)
(3837, 0)
(3838, 0)
(3839, 0)
(3840, 0)
(3841, 0)
(3842, 0)
(3843, 0)
(3844, 0)
(3845, 0)
(3846, 0)
(3847, 0)
(3848, 0)
(3849, 0)
(3850, 0)
(3851, 0)
(3852, 0)
(3853, 0)
(3854, 0)
(3855, 0)
(3856, 0)
(3857, 0)
(3858, 0)
(3859, 0)
(3860, 0)
(3861, 0)
(3862, 0)
(3863, 0)
(3864, 0)
(3865, 0)
(3866, 0)
(3867, 0)
(3868, 0)
(3869, 0)
(3870, 0)
(3871, 0)
(3872, 0)
(3873, 0)
(3874, 0)
(3875, 0)
(3876, 0)
(3877, 0)
(3878, 0)
(3879, 0)
(3880, 0)
(3881, 0)
(3882, 0)
(3883, 0)
(3884, 0)
(3885, 0)
(3886, 0)
(3887, 0)
(3888, 0)
(3889, 0)
(3890, 0)
(3891, 0)
(3892, 0)
(3893, 0)
(3894, 0)
(3895, 0)
(3896, 0)
(3897, 0)
(3898, 0)
(3899, 0)
(3900, 0)
(3901, 0)
(3902, 0)
(3903, 3.003)
(3904, 0)
(3905, 0)
(3906, 0)
(3907, 0)
(3908, 0)
(3909, 0)
(3910, 0)
(3911, 0)
(3912, 0)
(3913, 0)
(3914, 0)
(3915, 0)
(3916, 0)
(3917, 0)
(3918, 0)
(3919, 0)
(3920, 0)
(3921, 0)
(3922, 0)
(3923, 0)
(3924, 0)
(3925, 0)
(3926, 0)
(3927, 0)
(3928, 0)
(3929, 0)
(3930, 0)
(3931, 0)
(3932, 0)
(3933, 0)
(3934, 0)
(3935, 0)
(3936, 0)
(3937, 0)
(3938, 0)
(3939, 0)
(3940, 0)
(3941, 0)
(3942, 3.081)
(3943, 1.07)
(3944, 0.946)
(3945, 0)
(3946, 0)
(3947, 0)
(3948, 0)
(3949, 0)
(3950, 0)
(3951, 0)
(3952, 0)
(3953, 0)
(3954, 0)
(3955, 0)
(3956, 0)
(3957, 0)
(3958, 0)
(3959, 0)
(3960, 0)
(3961, 0)
(3962, 0)
(3963, 0)
(3964, 0)
(3965, 0)
(3966, 0)
(3967, 0)
(3968, 0)
(3969, 0)
(3970, 0)
(3971, 0)
(3972, 0)
(3973, 0)
(3974, 0)
(3975, 0)
(3976, 0)
(3977, 0)
(3978, 0)
(3979, 0)
(3980, 0)
(3981, 0)
(3982, 0)
(3983, 0)
(3984, 0)
(3985, 0)
(3986, 0)
(3987, 0)
(3988, 0)
(3989, 0)
(3990, 0)
(3991, 0)
(3992, 0)
(3993, 0)
(3994, 0)
(3995, 0)
(3996, 0)
(3997, 0)
(3998, 0)
(3999, 0)
(4000, 0)
(4001, 0)
(4002, 0)
(4003, 0)
(4004, 0)
(4005, 0)
(4006, 0)
(4007, 0)
(4008, 0)
(4009, 0)
(4010, 0)
(4011, 0)
(4012, 0)
(4013, 0)
(4014, 0)
(4015, 0)
(4016, 0)
(4017, 0)
(4018, 0)
(4019, 0)
(4020, 0)
(4021, 0)
(4022, 0)
(4023, 0)
(4024, 0)
(4025, 0)
(4026, 0)
(4027, 0)
(4028, 0)
(4029, 0)
(4030, 0)
(4031, 0)
(4032, 0)
(4033, 0)
(4034, 0)
(4035, 2.295)
(4036, 0.406)
(4037, 0)
(4038, 2.34)
(4039, 0.435)
(4040, 0)
(4041, 0)
(4042, 4.108)
(4043, 0.078)
(4044, 8.053)
(4045, 0)
(4046, 0)
(4047, 0)
(4048, 0)
(4049, 0)
(4050, 0)
(4051, 0)
(4052, 0)
(4053, 0)
(4054, 1.54)
(4055, 0)
(4056, 0)
(4057, 0)
(4058, 0)
(4059, 0)
(4060, 0)
(4061, 0)
(4062, 0)
(4063, 0)
(4064, 0)
(4065, 0)
(4066, 0)
(4067, 0)
(4068, 0)
(4069, 0)
(4070, 0)
(4071, 0)
(4072, 1.862)
(4073, 1.378)
(4074, 0)
(4075, 0)
(4076, 0)
(4077, 0)
(4078, 0)
(4079, 0)
(4080, 0)
(4081, 0)
(4082, 0)
(4083, 0)
(4084, 0)
(4085, 0)
(4086, 0)
(4087, 0)
(4088, 0)
(4089, 0)
(4090, 0)
(4091, 0)
(4092, 0)
(4093, 0)
(4094, 0)
(4095, 0)
(4096, 0)
(4097, 0)
(4098, 0)
(4099, 0)
(4100, 0)
(4101, 0)
(4102, 0)
(4103, 0)
(4104, 0)
(4105, 1.54)
(4106, 0)
(4107, 0)
(4108, 0)
(4109, 0)
(4110, 0)
(4111, 0)
(4112, 0)
(4113, 0)
(4114, 0)
(4115, 0)
(4116, 0)
(4117, 0)
(4118, 0)
(4119, 0)
(4120, 0)
(4121, 0)
(4122, 0)
(4123, 0)
(4124, 0)
(4125, 0)
(4126, 0)
(4127, 0)
(4128, 0)
(4129, 0)
(4130, 0)
(4131, 1.54)
(4132, 0)
(4133, 0)
(4134, 0)
(4135, 0)
(4136, 0)
(4137, 0)
(4138, 0)
(4139, 0)
(4140, 0)
(4141, 0)
(4142, 0)
(4143, 0)
(4144, 0)
(4145, 0)
(4146, 0)
(4147, 0)
(4148, 0)
(4149, 0)
(4150, 0)
(4151, 0)
(4152, 0)
(4153, 0)
(4154, 0)
(4155, 0)
(4156, 0)
(4157, 0)
(4158, 0)
(4159, 0)
(4160, 0)
(4161, 0)
(4162, 0)
(4163, 0)
(4164, 2.211)
(4165, 0)
(4166, 3.003)
(4167, 2.701)
(4168, 2.926)
(4169, 0)
(4170, 0)
(4171, 0)
(4172, 0)
(4173, 0)
(4174, 0)
(4175, 0)
(4176, 0)
(4177, 0)
(4178, 0)
(4179, 0)
(4180, 0)
(4181, 4.005)
(4182, 0)
(4183, 0)
(4184, 0)
(4185, 0)
(4186, 0)
(4187, 1.596)
(4188, 0)
(4189, 0)
(4190, 0)
(4191, 0)
(4192, 0)
(4193, 0)
(4194, 0)
(4195, 1.54)
(4196, 0)
(4197, 0)
(4198, 0)
(4199, 0)
(4200, 0)
(4201, 0)
(4202, 1.891)
(4203, 0)
(4204, 0)
(4205, 0)
(4206, 0)
(4207, 2.415)
(4208, 0)
(4209, 0)
(4210, 1.596)
(4211, 0)
(4212, 0)
(4213, 3.24)
(4214, 0)
(4215, 0)
(4216, 0)
(4217, 0)
(4218, 3.486)
(4219, 0)
(4220, 0)
(4221, 0)
(4222, 0)
(4223, 0)
(4224, 0)
(4225, 0)
(4226, 0)
(4227, 0)
(4228, 0)
(4229, 0)
(4230, 1.54)
(4231, 0)
(4232, 0)
(4233, 0)
(4234, 0)
(4235, 0)
(4236, 0)
(4237, 0)
(4238, 0)
(4239, 0)
(4240, 0)
(4241, 0)
(4242, 0)
(4243, 0)
(4244, 0)
(4245, 0)
(4246, 0)
(4247, 0)
(4248, 0)
(4249, 0)
(4250, 0)
(4251, 0)
(4252, 0)
(4253, 0)
(4254, 0)
(4255, 0)
(4256, 0)
(4257, 0)
(4258, 0)
(4259, 0)
(4260, 0)
(4261, 0)
(4262, 0)
(4263, 0)
(4264, 0)
(4265, 0)
(4266, 0)
(4267, 0)
(4268, 0)
(4269, 0)
(4270, 0)
(4271, 0)
(4272, 0)
(4273, 0)
(4274, 0)
(4275, 0)
(4276, 0)
(4277, 0)
(4278, 0)
(4279, 0)
(4280, 0)
(4281, 0)
(4282, 0)
(4283, 0)
(4284, 0)
(4285, 0)
(4286, 0)
(4287, 0)
(4288, 0)
(4289, 0)
(4290, 0)
(4291, 0)
(4292, 0)
(4293, 0)
(4294, 0)
(4295, 0)
(4296, 0)
(4297, 0)
(4298, 0)
(4299, 0)
(4300, 0)
(4301, 0)
(4302, 0)
(4303, 0)
(4304, 0)
(4305, 0)
(4306, 0)
(4307, 0)
(4308, 0)
(4309, 0)
(4310, 0)
(4311, 0)
(4312, 0)
(4313, 0)
(4314, 0)
(4315, 0)
(4316, 0)
(4317, 0)
(4318, 0)
(4319, 0)
(4320, 0)
(4321, 0)
(4322, 0)
(4323, 0)
(4324, 0)
(4325, 0)
(4326, 0)
(4327, 0)
(4328, 0)
(4329, 0)
(4330, 0)
(4331, 0)
(4332, 0)
(4333, 0)
(4334, 0)
(4335, 3.916)
(4336, 0)
(4337, 0)
(4338, 0)
(4339, 0)
(4340, 0)
(4341, 0)
(4342, 0)
(4343, 0)
(4344, 0)
(4345, 0)
(4346, 0)
(4347, 0)
(4348, 0)
(4349, 0)
(4350, 0)
(4351, 0)
(4352, 0)
(4353, 0)
(4354, 0)
(4355, 0)
(4356, 0)
(4357, 0)
(4358, 0)
(4359, 0)
(4360, 0)
(4361, 0)
(4362, 0)
(4363, 0)
(4364, 0)
(4365, 0)
(4366, 0)
(4367, 0)
(4368, 0)
(4369, 0)
(4370, 0)
(4371, 0)
(4372, 0)
(4373, 0)
(4374, 0)
(4375, 0)
(4376, 0)
(4377, 0)
(4378, 0)
(4379, 0)
(4380, 0)
(4381, 0)
(4382, 0)
(4383, 0)
(4384, 0)
(4385, 0)
(4386, 2.205)
(4387, 0.351)
(4388, 0)
(4389, 0)
(4390, 0)
(4391, 0)
(4392, 0)
(4393, 0)
(4394, 0)
(4395, 0)
(4396, 0)
(4397, 0)
(4398, 0)
(4399, 0)
(4400, 0)
(4401, 0)
(4402, 0)
(4403, 0)
(4404, 0)
(4405, 0)
(4406, 0)
(4407, 0)
(4408, 0)
(4409, 0)
(4410, 0)
(4411, 0)
(4412, 0)
(4413, 2.08)
(4414, 0)
(4415, 0)
(4416, 0)
(4417, 0)
(4418, 0)
(4419, 0)
(4420, 0)
(4421, 0)
(4422, 0)
(4423, 0)
(4424, 0)
(4425, 0)
(4426, 0)
(4427, 0)
(4428, 0)
(4429, 0)
(4430, 1.435)
(4431, 2.25)
(4432, 0)
(4433, 0)
(4434, 0)
(4435, 0)
(4436, 0)
(4437, 0)
(4438, 0)
(4439, 0)
(4440, 0)
(4441, 0)
(4442, 0)
(4443, 0)
(4444, 0)
(4445, 3.24)
(4446, 2.701)
(4447, 0)
(4448, 0)
(4449, 0)
(4450, 0)
(4451, 0)
(4452, 0)
(4453, 0)
(4454, 0)
(4455, 0)
(4456, 0)
(4457, 0)
(4458, 0)
(4459, 0)
(4460, 0)
(4461, 0)
(4462, 0)
(4463, 0)
(4464, 0)
(4465, 0)
(4466, 0)
(4467, 0)
(4468, 0)
(4469, 0)
(4470, 0)
(4471, 0)
(4472, 0)
(4473, 0)
(4474, 0)
(4475, 0)
(4476, 0)
(4477, 0)
(4478, 0)
(4479, 0)
(4480, 0)
(4481, 0)
(4482, 0)
(4483, 0)
(4484, 0)
(4485, 0)
(4486, 0)
(4487, 0)
(4488, 0)
(4489, 0)
(4490, 0)
(4491, 0)
(4492, 0)
(4493, 0)
(4494, 0)
(4495, 0)
(4496, 0)
(4497, 0)
(4498, 0)
(4499, 0)
(4500, 0)
(4501, 0)
(4502, 0)
(4503, 0)
(4504, 0)
(4505, 0)
(4506, 0)
(4507, 0)
(4508, 0)
(4509, 0)
(4510, 0)
(4511, 0)
(4512, 0)
(4513, 0)
(4514, 0)
(4515, 0)
(4516, 0)
(4517, 0)
(4518, 0)
(4519, 0)
(4520, 0)
(4521, 0)
(4522, 0)
(4523, 0)
(4524, 0)
(4525, 0)
(4526, 0)
(4527, 0)
(4528, 0)
(4529, 0)
(4530, 0)
(4531, 0)
(4532, 0)
(4533, 0)
(4534, 0)
(4535, 0)
(4536, 0)
(4537, 0)
(4538, 0)
(4539, 0)
(4540, 0)
(4541, 0)
(4542, 0)
(4543, 0)
(4544, 0)
(4545, 0)
(4546, 0)
(4547, 0)
(4548, 0)
(4549, 0)
(4550, 0)
(4551, 0)
(4552, 0)
(4553, 0)
(4554, 0)
(4555, 0)
(4556, 0)
(4557, 0)
(4558, 0)
(4559, 0)
(4560, 0)
(4561, 0)
(4562, 0)
(4563, 0)
(4564, 0)
(4565, 0)
(4566, 0)
(4567, 0)
(4568, 0)
(4569, 0)
(4570, 0)
(4571, 0)
(4572, 0)
(4573, 0)
(4574, 0)
(4575, 0)
(4576, 2.701)
(4577, 0)
(4578, 0)
(4579, 0)
(4580, 0)
(4581, 0)
(4582, 0)
(4583, 0)
(4584, 0)
(4585, 0)
(4586, 0)
(4587, 0)
(4588, 0)
(4589, 0)
(4590, 0)
(4591, 0)
(4592, 0)
(4593, 1.54)
(4594, 0)
(4595, 0)
(4596, 0)
(4597, 0)
(4598, 2.926)
(4599, 0)
(4600, 0)
(4601, 0)
(4602, 0)
(4603, 0)
(4604, 0)
(4605, 0)
(4606, 0)
(4607, 0)
(4608, 0)
(4609, 0)
(4610, 0)
(4611, 0)
(4612, 0)
(4613, 0)
(4614, 0)
(4615, 0)
(4616, 0)
(4617, 0)
(4618, 0)
(4619, 0)
(4620, 0)
(4621, 0)
(4622, 0)
(4623, 0)
(4624, 0)
(4625, 0)
(4626, 0)
(4627, 0)
(4628, 0)
(4629, 0)
(4630, 0)
(4631, 0)
(4632, 0)
(4633, 0)
(4634, 0)
(4635, 0)
(4636, 0)
(4637, 0)
(4638, 0)
(4639, 0)
};


==> covgraphs/graph2.tex <==
\addplot[const plot,fill=lightblue,draw=lightblue] coordinates {
(-1, 0)
(0, 1)
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1.16)
(7, 1.16)
(8, 1.16)
(9, 1.16)
(10, 1.16)
(11, 1.16)
(12, 1.16)
(13, 1.16)
(14, 1.16)
(15, 1.16)
(16, 1.278)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1.775)
(31, 1)
(32, 1)
(33, 1)
(34, 1)
(35, 1)
(36, 1)
(37, 1)
(38, 1)
(39, 1)
(40, 1)
(41, 1)
(42, 1)
(43, 1)
(44, 1)
(45, 1)
(46, 1)
(47, 1)
(48, 1)
(49, 1)
(50, 1)
(51, 1)
(52, 1)
(53, 1)
(54, 0)
(55, 2.08)
(56, 0)
(57, 0)
(58, 0)
(59, 3.081)
(60, 0)
};



==> covgraphs/sau.euler.single.log.cov.errors.tex <==
\addplot [sharp plot,color=lightblue,mark=+,mark size=2pt,mark repeat=5,smooth,line width=1.5pt] coordinates {
(0, 0.131782945736434)
(1, 0)
(2, 0)
(3, 0)
(4, 0)
(5, 0)
(6, 0)
(7, 0)
(8, 0)
(9, 0)
(10, 0)
(11, 0)
(12, 0)
(13, 0)
(14, 0)
(15, 0)
(16, 0)
(17, 0)
(18, 0)
(19, 0)
(20, 0)
(21, 0)
(22, 0)
(23, 0)
(24, 0.00775193798449612)
(25, 0)
(26, 0)
(27, 0)
(28, 0)
(29, 0)
(30, 0)
(31, 0)
(32, 0)
(33, 0)
(34, 0)
(35, 0)
(36, 0.0155038759689922)
(37, 0)
(38, 0)
(39, 0)
(40, 0)
(41, 0)
(42, 0)
(43, 0)
(44, 0)
(45, 0)
(46, 0)
(47, 0)
(48, 0)
(49, 0)
(50, 0)
(51, 0)
(52, 0)
(53, 0)
(54, 0)
(55, 0.0232558139534884)
(56, 0.0310077519379845)
(57, 0.147286821705426)
(58, 0.186046511627907)
(59, 0.0232558139534884)
(60, 0.0232558139534884)
(61, 0.0155038759689922)
(62, 0)
(63, 0.0155038759689922)
(64, 0.00775193798449612)
(65, 0)
(66, 0)
(67, 0)
(68, 0)
(69, 0.00775193798449612)
(70, 0)
(71, 0.131782945736434)
(72, 0.147286821705426)
(73, 0.124031007751938)
(74, 0.147286821705426)
(75, 0.131782945736434)
(76, 0)
(77, 0.00775193798449612)
(78, 0)
(79, 0)
(80, 0.00775193798449612)
(81, 0.00775193798449612)
(82, 0)
(83, 0)
(84, 0)
(85, 0.00775193798449612)
(86, 0)
(87, 0)
(88, 0)
(89, 0.00775193798449612)
(90, 0)
(91, 0)
(92, 0)
(93, 0)
(94, 0)
(95, 0.0078740157480315)
(96, 0)
(97, 0)
(98, 0)
(99, 0)
(100, 0)
};

